Softmax parameterization of the occupation numbers for natural orbital functionals based on electron pairing approaches

Within the framework of natural orbital functional theory, having a convenient representation of the occupation numbers and orbitals becomes critical for the computational performance of the calculations. Recognizing this, we propose an innovative parametrization of the occupation numbers that takes advantage of the electron-pairing approach used in Piris natural orbital functionals through the adoption of the softmax function, a pivotal component in modern deep-learning models. Our approach not only ensures adherence to the N-representability of the first-order reduced density matrix (1RDM) but also significantly enhances the computational efficiency of 1RDM functional theory calculations. The effectiveness of this alternative parameterization approach was assessed using the W4-17-MR molecular set, which demonstrated faster and more robust convergence compared to previous implementations.

==> Figures/Figures_jctc/axis.tex <==
\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{B2}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI}, %Cumulative Occupancy \\ Iterations
xtick={0,1,2,3},
% ytick={0,-0.05,-0.1,-0.15,-0.2},
ytick distance=0.1,
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={4.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=4.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.213833999633789, ymax=0.0101825714111328,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c1)}
]
\addplot [ultra thick, brown, dashed]
table {%
2.12057399749756 -3.4332275390625e-05
2.51321768760681 -0.00278854370117188
2.60206007957458 -0.00467300415039062
2.8286600112915 -0.0169601440429688
2.98855900764465 -0.0329627990722656
3.11727118492126 -0.0589866638183594
3.17638063430786 -0.0932388305664062
3.23095965385437 -0.105026245117188
3.29159069061279 -0.109043121337891
3.34123659133911 -0.111949920654297
3.38237738609314 -0.116546630859375
3.41043972969055 -0.121997833251953
3.43568515777588 -0.129253387451172
3.45209312438965 -0.135730743408203
3.46194839477539 -0.139629364013672
3.47143840789795 -0.145408630371094
3.48115587234497 -0.151405334472656
3.48727989196777 -0.160797119140625
3.49582171440125 -0.167903900146484
3.50338196754456 -0.174999237060547
3.50960564613342 -0.175884246826172
3.51693177223206 -0.176593780517578
3.5250449180603 -0.178928375244141
3.53288173675537 -0.179718017578125
3.5393271446228 -0.180210113525391
3.54629588127136 -0.183376312255859
3.55364036560059 -0.184394836425781
3.56026530265808 -0.185478210449219
3.56960797309875 -0.187191009521484
3.57691693305969 -0.188137054443359
3.58478331565857 -0.189952850341797
3.59250974655151 -0.190380096435547
3.59868121147156 -0.190887451171875
3.60271096229553 -0.191226959228516
3.60863304138184 -0.191566467285156
3.615318775177 -0.191780090332031
3.6253125667572 -0.194015502929688
3.63144373893738 -0.195232391357422
3.63858914375305 -0.195846557617188
3.64276123046875 -0.196079254150391
3.64787173271179 -0.196552276611328
3.65069603919983 -0.196701049804688
3.65359830856323 -0.196903228759766
3.65638566017151 -0.197052001953125
3.66001129150391 -0.197124481201172
3.66313529014587 -0.197216033935547
3.66968870162964 -0.197658538818359
3.67385005950928 -0.1978759765625
3.67687654495239 -0.198024749755859
3.67851829528809 -0.198089599609375
3.68439650535583 -0.198333740234375
3.68663620948792 -0.198383331298828
3.68966388702393 -0.198417663574219
3.69548177719116 -0.199069976806641
3.6974036693573 -0.199138641357422
3.69992446899414 -0.199176788330078
3.70277500152588 -0.199234008789062
3.70440793037415 -0.199260711669922
3.70842099189758 -0.199329376220703
3.71121644973755 -0.199382781982422
3.71273374557495 -0.199405670166016
3.71825242042542 -0.199928283691406
3.7196626663208 -0.200019836425781
3.72123336791992 -0.200046539306641
3.72304511070251 -0.2000732421875
3.72550320625305 -0.200092315673828
3.72956967353821 -0.200401306152344
3.73287606239319 -0.200546264648438
3.73503971099854 -0.200599670410156
3.7371129989624 -0.200626373291016
3.73830485343933 -0.200645446777344
3.74233222007751 -0.200759887695312
3.74366641044617 -0.200782775878906
3.74764490127563 -0.200798034667969
3.75066256523132 -0.200862884521484
3.7537362575531 -0.200885772705078
3.75663614273071 -0.200916290283203
3.75838184356689 -0.200927734375
3.76447510719299 -0.201251983642578
3.76671028137207 -0.201423645019531
3.76849007606506 -0.201438903808594
3.77041006088257 -0.201454162597656
3.77451705932617 -0.201473236083984
3.77684640884399 -0.201496124267578
3.77901887893677 -0.201515197753906
3.78017330169678 -0.201530456542969
3.78218579292297 -0.201545715332031
3.78397488594055 -0.201568603515625
3.78632545471191 -0.201606750488281
3.78859257698059 -0.201652526855469
3.79063701629639 -0.201686859130859
3.79190111160278 -0.201713562011719
3.79434871673584 -0.20172119140625
3.79664373397827 -0.2017822265625
3.80037331581116 -0.201930999755859
3.80236315727234 -0.201969146728516
3.80407118797302 -0.202007293701172
3.80624771118164 -0.202056884765625
3.80794072151184 -0.202083587646484
3.80962705612183 -0.202117919921875
3.81123971939087 -0.202144622802734
3.81318044662476 -0.202167510986328
3.81524562835693 -0.202274322509766
3.81736707687378 -0.202423095703125
3.81967544555664 -0.202522277832031
3.82138252258301 -0.202548980712891
3.82386541366577 -0.20257568359375
3.82588028907776 -0.202610015869141
3.82749843597412 -0.202629089355469
3.82885313034058 -0.202644348144531
3.83174180984497 -0.202808380126953
3.83352947235107 -0.202835083007812
3.83499264717102 -0.202842712402344
3.83733582496643 -0.202857971191406
3.83859729766846 -0.202873229980469
3.83985495567322 -0.202877044677734
3.84092116355896 -0.202892303466797
3.84267163276672 -0.202919006347656
3.84341955184937 -0.202934265136719
3.84534621238708 -0.202938079833984
3.84726405143738 -0.202976226806641
3.85125827789307 -0.203018188476562
3.85186958312988 -0.203022003173828
3.85211396217346 -0.203029632568359
3.85454893112183 -0.203041076660156
3.85570073127747 -0.203048706054688
3.85697054862976 -0.203056335449219
3.85769414901733 -0.20306396484375
3.8596785068512 -0.203128814697266
3.86081695556641 -0.203136444091797
3.86308479309082 -0.203163146972656
3.86415505409241 -0.203170776367188
3.86545944213867 -0.203178405761719
3.86752653121948 -0.203205108642578
3.86805629730225 -0.203208923339844
3.870521068573 -0.203235626220703
3.87244772911072 -0.203239440917969
3.8726806640625 -0.203239440917969
3.87413382530212 -0.203273773193359
3.8747136592865 -0.203277587890625
3.87633323669434 -0.20330810546875
3.87748646736145 -0.203311920166016
3.87783193588257 -0.203315734863281
3.87886643409729 -0.203323364257812
3.87949728965759 -0.203327178955078
3.88189792633057 -0.203346252441406
3.88280916213989 -0.203350067138672
3.88417196273804 -0.203353881835938
3.8857569694519 -0.203380584716797
3.88609576225281 -0.203384399414062
3.88739228248596 -0.203388214111328
3.88772988319397 -0.203392028808594
};
\addplot [ultra thick, blue]
table {%
0.84509801864624 0
1.25527250766754 -0.00209808349609375
1.53147888183594 -0.00389862060546875
1.77085208892822 -0.00702667236328125
1.94448268413544 -0.01513671875
2.21218752861023 -0.0382270812988281
2.28780174255371 -0.0687103271484375
2.35793495178223 -0.0923004150390625
2.46982192993164 -0.103786468505859
2.5250449180603 -0.106815338134766
2.58206343650818 -0.109367370605469
2.62117624282837 -0.112087249755859
2.65705585479736 -0.115921020507812
2.71432971954346 -0.122020721435547
2.76342797279358 -0.131870269775391
2.79239177703857 -0.139530181884766
2.84073328971863 -0.152858734130859
2.88252449035645 -0.162639617919922
2.90955591201782 -0.173118591308594
2.93145799636841 -0.174350738525391
2.94250416755676 -0.174980163574219
2.95375967025757 -0.175411224365234
2.97266554832458 -0.176239013671875
2.99255347251892 -0.17779541015625
3.00346040725708 -0.178241729736328
3.0182843208313 -0.179218292236328
3.03981065750122 -0.180198669433594
3.05037975311279 -0.180732727050781
3.06483221054077 -0.182121276855469
3.07554697990417 -0.182662963867188
3.09656238555908 -0.186775207519531
3.11226987838745 -0.188243865966797
3.11859536170959 -0.188640594482422
3.13385820388794 -0.190776824951172
3.14643812179565 -0.191505432128906
3.15594291687012 -0.19195556640625
3.15806078910828 -0.192142486572266
3.17955183982849 -0.193984985351562
3.18497514724731 -0.194553375244141
3.19005131721497 -0.194797515869141
3.19975519180298 -0.194950103759766
3.20330500602722 -0.195098876953125
3.21298623085022 -0.195446014404297
3.22063112258911 -0.195693969726562
3.22582602500916 -0.195892333984375
3.23324990272522 -0.196250915527344
3.24649858474731 -0.19683837890625
3.24919843673706 -0.197124481201172
3.25406455993652 -0.197334289550781
3.25887656211853 -0.197429656982422
3.26623177528381 -0.197696685791016
3.27184152603149 -0.197853088378906
3.27323293685913 -0.197906494140625
3.28465628623962 -0.198436737060547
3.28465628623962 -0.198509216308594
3.28757786750793 -0.198585510253906
3.29292035102844 -0.198680877685547
3.29622626304626 -0.198757171630859
3.3001606464386 -0.198883056640625
3.30168104171753 -0.198928833007812
3.3062105178833 -0.199028015136719
3.30856442451477 -0.199119567871094
3.32014632225037 -0.199176788330078
3.32283926010132 -0.199226379394531
3.32592606544495 -0.199287414550781
3.32878708839417 -0.199356079101562
3.33405137062073 -0.199432373046875
3.33465480804443 -0.199462890625
3.33785843849182 -0.199512481689453
3.33885478973389 -0.199554443359375
3.34399914741516 -0.199588775634766
3.34537363052368 -0.199619293212891
3.35237550735474 -0.199775695800781
3.35410833358765 -0.199844360351562
3.35602593421936 -0.199874877929688
3.3602147102356 -0.199966430664062
3.36153888702393 -0.200004577636719
3.36380004882812 -0.200027465820312
3.37106776237488 -0.200389862060547
3.37511467933655 -0.200492858886719
3.37566351890564 -0.200508117675781
3.38003015518188 -0.200553894042969
3.38075375556946 -0.200580596923828
3.38075375556946 -0.200595855712891
3.38489079475403 -0.200614929199219
3.38596367835999 -0.200656890869141
3.38738989830017 -0.200672149658203
3.38845634460449 -0.200721740722656
3.3953263759613 -0.200736999511719
3.39984679222107 -0.200798034667969
3.40071058273315 -0.200832366943359
3.40312051773071 -0.200859069824219
3.40312051773071 -0.200870513916016
3.40602898597717 -0.200904846191406
3.40857911109924 -0.200912475585938
3.40874862670898 -0.200935363769531
3.40925669670105 -0.200946807861328
3.41597437858582 -0.201095581054688
3.41813540458679 -0.201145172119141
3.42193269729614 -0.201152801513672
3.42193269729614 -0.201164245605469
3.42340970039368 -0.201217651367188
3.42471837997437 -0.20123291015625
3.42732381820679 -0.201267242431641
3.42732381820679 -0.201278686523438
3.42748618125916 -0.201290130615234
3.42764830589294 -0.201297760009766
3.43296933174133 -0.201389312744141
3.43648076057434 -0.201442718505859
3.43933272361755 -0.201515197753906
3.44731307029724 -0.2015380859375
3.44762301445007 -0.201553344726562
3.449786901474 -0.201622009277344
3.449786901474 -0.201644897460938
3.4527063369751 -0.201663970947266
3.45606231689453 -0.201744079589844
3.4577305316925 -0.201763153076172
3.45999526977539 -0.201778411865234
3.46493649482727 -0.202045440673828
3.46731209754944 -0.202125549316406
3.46923279762268 -0.202152252197266
3.47099828720093 -0.202201843261719
3.47348690032959 -0.202243804931641
3.47523522377014 -0.202266693115234
3.47712135314941 -0.202297210693359
3.47856640815735 -0.202335357666016
3.48072528839111 -0.202358245849609
3.48201560974121 -0.202400207519531
3.48699688911438 -0.202480316162109
3.48869180679321 -0.202510833740234
3.49052023887634 -0.202568054199219
3.49206161499023 -0.202590942382812
3.49220132827759 -0.202602386474609
3.49401545524597 -0.202613830566406
3.49554443359375 -0.202663421630859
3.4962375164032 -0.202678680419922
3.49748253822327 -0.202701568603516
3.49762058258057 -0.202709197998047
3.49886178970337 -0.202720642089844
3.49886178970337 -0.202728271484375
3.49996185302734 -0.202747344970703
3.50310945510864 -0.202835083007812
3.50501418113708 -0.202842712402344
3.50501418113708 -0.202846527099609
3.50542140007019 -0.202869415283203
3.50623440742493 -0.202877044677734
3.50745105743408 -0.202896118164062
3.51188325881958 -0.202964782714844
3.51348400115967 -0.202999114990234
3.51388311386108 -0.2030029296875
3.51388311386108 -0.203010559082031
3.51388311386108 -0.203025817871094
3.51838231086731 -0.203037261962891
3.5187771320343 -0.203044891357422
3.5187771320343 -0.203056335449219
3.5187771320343 -0.203060150146484
3.51917147636414 -0.203071594238281
3.5196967124939 -0.203075408935547
3.51982808113098 -0.203086853027344
3.52100729942322 -0.203105926513672
3.5250449180603 -0.203113555908203
3.52543354034424 -0.203117370605469
3.52556300163269 -0.203128814697266
3.52569246292114 -0.203132629394531
3.52569246292114 -0.203136444091797
3.52582192420959 -0.203144073486328
3.52582192420959 -0.203147888183594
3.52595138549805 -0.203151702880859
3.52608060836792 -0.203159332275391
3.52621006965637 -0.203163146972656
3.52633929252625 -0.203166961669922
3.52646851539612 -0.203166961669922
3.52646851539612 -0.20318603515625
3.52737212181091 -0.203197479248047
3.52801632881165 -0.203205108642578
3.52801632881165 -0.203208923339844
3.52801632881165 -0.203212738037109
3.5287880897522 -0.203220367431641
3.52891683578491 -0.203224182128906
3.52891683578491 -0.203227996826172
3.53071188926697 -0.203231811523438
3.53071188926697 -0.203235626220703
3.53071188926697 -0.203239440917969
3.53071188926697 -0.203262329101562
3.53262710571289 -0.203292846679688
3.53339076042175 -0.203296661376953
3.53339076042175 -0.203300476074219
3.53339076042175 -0.203304290771484
3.53339076042175 -0.20330810546875
3.53351783752441 -0.203311920166016
3.53364491462708 -0.203315734863281
3.53377199172974 -0.203338623046875
3.53982853889465 -0.203483581542969
3.54220271110535 -0.20361328125
3.54282546043396 -0.203617095947266
3.54307413101196 -0.203617095947266
3.54307413101196 -0.203620910644531
3.54319858551025 -0.203620910644531
3.54617238044739 -0.203624725341797
3.54617238044739 -0.203628540039062
3.54617238044739 -0.203628540039062
3.54617238044739 -0.203632354736328
3.54629588127136 -0.203636169433594
3.54629588127136 -0.203643798828125
3.54641938209534 -0.203647613525391
3.54654264450073 -0.203651428222656
3.54666614532471 -0.203651428222656
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{BN}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},  
xtick={0,1,2,3},
extra x tick labels={\small$\text{log}_{10}$}, 
extra x ticks={4.9},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.2324214220047, xmax=4.9,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.292853546142578, ymax=0.0139533996582031,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c2)}
]
\addplot [ultra thick, brown, dashed]
table {%
1.64345264434814 7.62939453125e-06
1.77085208892822 -0.0002593994140625
2.23299622535706 -0.000701904296875
2.33645963668823 -0.000885009765625
2.45939254760742 -0.00115966796875
2.49276041984558 -0.0012664794921875
2.60314440727234 -0.002899169921875
2.75739598274231 -0.00389862060546875
2.84385538101196 -0.00614166259765625
2.90309000015259 -0.007965087890625
3.0301947593689 -0.01007080078125
3.11958575248718 -0.0124282836914062
3.18582534790039 -0.0159683227539062
3.26974630355835 -0.0232696533203125
3.38969755172729 -0.0355682373046875
3.45285940170288 -0.0592117309570312
3.51027679443359 -0.0891265869140625
3.54332280158997 -0.102729797363281
3.58285856246948 -0.1070556640625
3.63788986206055 -0.113960266113281
3.65176248550415 -0.119407653808594
3.67742443084717 -0.123970031738281
3.70517921447754 -0.129501342773438
3.74052047729492 -0.148246765136719
3.7627534866333 -0.169548034667969
3.80550074577332 -0.1881103515625
3.82497143745422 -0.199119567871094
3.84862017631531 -0.208145141601562
3.8671727180481 -0.211227416992188
3.8933732509613 -0.219688415527344
3.90778732299805 -0.225723266601562
3.92474436759949 -0.233360290527344
3.93986845016479 -0.239921569824219
3.95520663261414 -0.243080139160156
3.97676253318787 -0.246185302734375
3.99471306800842 -0.248519897460938
4.00194978713989 -0.249504089355469
4.01131677627563 -0.250999450683594
4.02118921279907 -0.251976013183594
4.0290994644165 -0.25244140625
4.03977108001709 -0.256393432617188
4.04735279083252 -0.257247924804688
4.05967712402344 -0.258346557617188
4.07236003875732 -0.259346008300781
4.07983207702637 -0.259796142578125
4.08884477615356 -0.2603759765625
4.09398174285889 -0.260673522949219
4.10394048690796 -0.261123657226562
4.10883569717407 -0.26141357421875
4.11723804473877 -0.262130737304688
4.12404775619507 -0.262489318847656
4.13075160980225 -0.263137817382812
4.13817644119263 -0.263641357421875
4.1432957649231 -0.263877868652344
4.14792346954346 -0.264030456542969
4.15697288513184 -0.26544189453125
4.16319131851196 -0.266166687011719
4.16829109191895 -0.2664794921875
4.18046998977661 -0.267402648925781
4.18766164779663 -0.267738342285156
4.19320821762085 -0.268142700195312
4.19639730453491 -0.268280029296875
4.2040114402771 -0.268905639648438
4.20964908599854 -0.269065856933594
4.21558475494385 -0.269172668457031
4.22326231002808 -0.269767761230469
4.22665166854858 -0.269889831542969
4.2288875579834 -0.269935607910156
4.23360538482666 -0.270050048828125
4.24132251739502 -0.270408630371094
4.24573469161987 -0.27056884765625
4.25027370452881 -0.270622253417969
4.25239181518555 -0.270698547363281
4.25844573974609 -0.2708740234375
4.2640380859375 -0.270942687988281
4.27207374572754 -0.271125793457031
4.27434253692627 -0.271163940429688
4.27875375747681 -0.271286010742188
4.28434038162231 -0.271408081054688
4.28654623031616 -0.271446228027344
4.28818225860596 -0.271476745605469
4.29161310195923 -0.27166748046875
4.29703807830811 -0.271697998046875
4.29826354980469 -0.271736145019531
4.30233097076416 -0.271842956542969
4.30306625366211 -0.271881103515625
4.30711078643799 -0.271926879882812
4.31092691421509 -0.271957397460938
4.31437301635742 -0.272003173828125
4.3171854019165 -0.27203369140625
4.31854343414307 -0.272087097167969
4.32277727127075 -0.272193908691406
4.32811450958252 -0.272209167480469
4.32882785797119 -0.272247314453125
4.33122491836548 -0.272354125976562
4.33282232284546 -0.272392272949219
4.33437347412109 -0.272415161132812
4.3393120765686 -0.272483825683594
4.34566783905029 -0.272544860839844
4.34719324111938 -0.2725830078125
4.35022878646851 -0.27264404296875
4.3511004447937 -0.272666931152344
4.35144853591919 -0.272689819335938
4.35247182846069 -0.272705078125
4.35547065734863 -0.272735595703125
4.35998725891113 -0.272781372070312
4.36720657348633 -0.273193359375
4.36891889572144 -0.273223876953125
4.37088298797607 -0.273239135742188
4.38010263442993 -0.273429870605469
4.38214302062988 -0.273460388183594
4.38379764556885 -0.273490905761719
4.38467597961426 -0.273521423339844
4.38699817657471 -0.273544311523438
4.38738965988159 -0.2735595703125
4.39185237884521 -0.273574829101562
4.39310121536255 -0.273605346679688
4.39471435546875 -0.273635864257812
4.40102100372314 -0.274085998535156
4.40198612213135 -0.274124145507812
4.40265703201294 -0.274139404296875
4.40491914749146 -0.274253845214844
4.40711879730225 -0.274261474609375
4.41006851196289 -0.2742919921875
4.41151857376099 -0.274307250976562
4.41190576553345 -0.274314880371094
4.41400337219238 -0.274330139160156
4.41952610015869 -0.274421691894531
4.42157125473022 -0.274436950683594
4.42427730560303 -0.274505615234375
4.42743730545044 -0.274520874023438
4.42857217788696 -0.2745361328125
4.42994594573975 -0.274551391601562
4.43702077865601 -0.274772644042969
4.4378457069397 -0.274787902832031
4.44138097763062 -0.27484130859375
4.44337272644043 -0.274856567382812
4.44441938400269 -0.274871826171875
4.44493436813354 -0.274879455566406
4.45141792297363 -0.274955749511719
4.4538836479187 -0.274978637695312
4.45496654510498 -0.275001525878906
4.46299648284912 -0.275123596191406
4.4643702507019 -0.275177001953125
4.46462345123291 -0.275184631347656
4.4663782119751 -0.275215148925781
4.46945381164551 -0.275222778320312
4.47570037841797 -0.275314331054688
4.4763822555542 -0.27532958984375
4.47940254211426 -0.275375366210938
4.48118448257446 -0.275405883789062
4.48168611526489 -0.275421142578125
4.48341608047485 -0.275436401367188
4.48512506484985 -0.275444030761719
4.4859766960144 -0.275466918945312
4.48781681060791 -0.275474548339844
4.49028158187866 -0.275497436523438
4.49200582504272 -0.2755126953125
4.49263477325439 -0.275527954101562
4.49553060531616 -0.27557373046875
4.50036001205444 -0.275634765625
4.50094985961914 -0.275657653808594
4.50332736968994 -0.275688171386719
4.50365447998047 -0.27569580078125
4.50689697265625 -0.275718688964844
4.50704574584961 -0.275726318359375
4.51042413711548 -0.275749206542969
4.51255083084106 -0.275779724121094
4.51313781738281 -0.275802612304688
4.51483964920044 -0.27581787109375
4.51652193069458 -0.275833129882812
4.5197491645813 -0.275909423828125
4.52092885971069 -0.275924682617188
4.52183103561401 -0.27593994140625
4.52580881118774 -0.276039123535156
4.5288782119751 -0.276046752929688
4.52900648117065 -0.276054382324219
4.52977657318115 -0.276069641113281
4.53130006790161 -0.276077270507812
4.53321266174316 -0.276092529296875
4.53373384475708 -0.276107788085938
4.53431797027588 -0.276123046875
4.53610372543335 -0.276138305664062
4.54084253311157 -0.27630615234375
4.54169178009033 -0.276374816894531
4.54194116592407 -0.276382446289062
4.54344701766968 -0.276405334472656
4.54757785797119 -0.276458740234375
4.54967737197876 -0.2764892578125
4.5507173538208 -0.276496887207031
4.55339765548706 -0.276542663574219
4.55498552322388 -0.27655029296875
4.5567364692688 -0.276565551757812
4.5575795173645 -0.276580810546875
4.56163787841797 -0.276657104492188
4.56286382675171 -0.276664733886719
4.56576538085938 -0.276702880859375
4.56745004653931 -0.276710510253906
4.5693507194519 -0.2767333984375
4.56978321075439 -0.276748657226562
4.57202291488647 -0.276771545410156
4.5735445022583 -0.276779174804688
4.57404279708862 -0.276786804199219
4.57601881027222 -0.276924133300781
4.57650279998779 -0.276939392089844
4.57830667495728 -0.276954650878906
4.57972621917725 -0.276985168457031
4.58154010772705 -0.277030944824219
4.58316469192505 -0.277046203613281
4.5832781791687 -0.277053833007812
4.58671092987061 -0.277168273925781
4.58750915527344 -0.277183532714844
4.58835029602051 -0.277191162109375
4.59204339981079 -0.277267456054688
4.59253215789795 -0.27728271484375
4.59339666366577 -0.277290344238281
4.59425973892212 -0.277320861816406
4.59523153305054 -0.277336120605469
4.59614610671997 -0.27734375
4.59796905517578 -0.277381896972656
4.59818840026855 -0.277389526367188
4.59939193725586 -0.27740478515625
4.6001558303833 -0.277412414550781
4.60075521469116 -0.277420043945312
4.60243988037109 -0.277442932128906
4.60292768478394 -0.277450561523438
4.6039776802063 -0.277458190917969
4.60413980484009 -0.277458190917969
4.60851526260376 -0.277603149414062
4.6092848777771 -0.277626037597656
4.60944509506226 -0.277626037597656
4.60948753356934 -0.277633666992188
4.61485481262207 -0.278289794921875
4.61544513702393 -0.278373718261719
4.61641263961792 -0.278388977050781
4.61667490005493 -0.278396606445312
4.61759805679321 -0.278404235839844
4.61811065673828 -0.278411865234375
4.6181526184082 -0.278411865234375
4.61822605133057 -0.278419494628906
4.62029218673706 -0.278419494628906
4.62037563323975 -0.278427124023438
4.62045860290527 -0.278434753417969
4.62207937240601 -0.2784423828125
4.62252473831177 -0.278450012207031
4.62266969680786 -0.278457641601562
4.6233115196228 -0.278457641601562
4.62353849411011 -0.278465270996094
4.62390041351318 -0.278472900390625
4.62591934204102 -0.278480529785156
4.6262993812561 -0.278488159179688
4.6264123916626 -0.278488159179688
4.62655591964722 -0.278488159179688
4.62708902359009 -0.278495788574219
4.6273250579834 -0.27850341796875
4.627366065979 -0.27850341796875
4.62745809555054 -0.278511047363281
4.62770366668701 -0.278511047363281
4.62814378738403 -0.278518676757812
4.62929725646973 -0.278549194335938
4.62960338592529 -0.278549194335938
4.62975597381592 -0.278556823730469
4.63014316558838 -0.278564453125
4.63060092926025 -0.278564453125
4.63109874725342 -0.278572082519531
4.63139295578003 -0.278572082519531
4.63144397735596 -0.278572082519531
4.63160610198975 -0.278579711914062
4.63188982009888 -0.278579711914062
4.63193035125732 -0.278579711914062
4.63208246231079 -0.278594970703125
4.63239669799805 -0.278594970703125
4.63359975814819 -0.278602600097656
4.63388252258301 -0.278610229492188
4.6339225769043 -0.278610229492188
4.63411426544189 -0.278617858886719
4.63417482376099 -0.278617858886719
4.63442707061768 -0.278617858886719
4.63449764251709 -0.27862548828125
4.63518190383911 -0.278633117675781
4.6355037689209 -0.278633117675781
4.63559436798096 -0.278640747070312
4.63814973831177 -0.278793334960938
4.63842916488647 -0.278800964355469
4.63850927352905 -0.278800964355469
4.63932704925537 -0.278816223144531
4.63944673538208 -0.278816223144531
4.64005374908447 -0.278831481933594
4.64092826843262 -0.278831481933594
4.64104747772217 -0.278831481933594
4.64167261123657 -0.278831481933594
4.64173173904419 -0.278839111328125
4.64190006256104 -0.278839111328125
4.64199924468994 -0.278846740722656
4.64275121688843 -0.278846740722656
4.64337348937988 -0.278846740722656
4.64345264434814 -0.278846740722656
4.6437292098999 -0.278861999511719
4.64407396316528 -0.27886962890625
4.64428091049194 -0.27886962890625
4.64523553848267 -0.278877258300781
4.64666843414307 -0.278892517089844
4.64692306518555 -0.278892517089844
4.64773511886597 -0.278892517089844
4.64786195755005 -0.278892517089844
4.6480278968811 -0.278900146484375
4.64821338653564 -0.278900146484375
4.64821338653564 -0.278900146484375
4.64838933944702 -0.278907775878906
4.64842844009399 -0.278907775878906
};
\addplot [ultra thick, blue]
table {%
0 0
0.30103000998497 -0.000244140625
0.477121233940125 -0.0004425048828125
0.84509801864624 -0.00086212158203125
0.954242527484894 -0.0010528564453125
1.20412003993988 -0.00212860107421875
1.32221925258636 -0.00254058837890625
1.54406809806824 -0.00421905517578125
1.59106457233429 -0.0050811767578125
1.78532981872559 -0.0093231201171875
1.90848505496979 -0.0166397094726562
2.09690999984741 -0.0293655395507812
2.16435289382935 -0.056976318359375
2.26007127761841 -0.0864791870117188
2.34830474853516 -0.103179931640625
2.36735582351685 -0.107757568359375
2.40483379364014 -0.111495971679688
2.43296933174133 -0.113937377929688
2.45788192749023 -0.116325378417969
2.50105929374695 -0.120498657226562
2.52633929252625 -0.124923706054688
2.63548374176025 -0.144111633300781
2.67117285728455 -0.1634521484375
2.75204849243164 -0.181312561035156
2.77959656715393 -0.194000244140625
2.82020139694214 -0.202995300292969
2.84695529937744 -0.207916259765625
2.8779468536377 -0.213798522949219
2.89542245864868 -0.215911865234375
2.92376184463501 -0.222625732421875
2.94890165328979 -0.228279113769531
2.97173953056335 -0.233184814453125
2.98811292648315 -0.236854553222656
3.0145206451416 -0.246940612792969
3.02366399765015 -0.249351501464844
3.0433623790741 -0.250480651855469
3.05576038360596 -0.251304626464844
3.0652060508728 -0.251907348632812
3.08026552200317 -0.254730224609375
3.10243368148804 -0.255653381347656
3.12024474143982 -0.257461547851562
3.13608598709106 -0.258674621582031
3.13956427574158 -0.259117126464844
3.14860272407532 -0.259933471679688
3.15351009368896 -0.260261535644531
3.16286301612854 -0.261138916015625
3.17347764968872 -0.26171875
3.18610835075378 -0.262527465820312
3.19117140769958 -0.262962341308594
3.19783163070679 -0.263160705566406
3.20844125747681 -0.263587951660156
3.21085333824158 -0.263725280761719
3.22193551063538 -0.264488220214844
3.22608423233032 -0.264724731445312
3.23248791694641 -0.26495361328125
3.24427700042725 -0.266204833984375
3.24993181228638 -0.266578674316406
3.25236749649048 -0.266792297363281
3.25406455993652 -0.26690673828125
3.25983262062073 -0.267127990722656
3.26268839836121 -0.267333984375
3.26834392547607 -0.267562866210938
3.28307485580444 -0.268417358398438
3.28533220291138 -0.268669128417969
3.28780174255371 -0.268989562988281
3.29047989845276 -0.269050598144531
3.30254745483398 -0.270675659179688
3.30362796783447 -0.270835876464844
3.30984306335449 -0.270889282226562
3.31005573272705 -0.270919799804688
3.31154203414917 -0.271087646484375
3.31617999076843 -0.271217346191406
3.31659936904907 -0.271278381347656
3.31806325912476 -0.271308898925781
3.32283926010132 -0.271438598632812
3.32756328582764 -0.271560668945312
3.32980442047119 -0.271598815917969
3.33142733573914 -0.271636962890625
3.33685970306396 -0.27178955078125
3.34084057807922 -0.271827697753906
3.34242272377014 -0.271873474121094
3.35082936286926 -0.2724609375
3.35314655303955 -0.27252197265625
3.3535315990448 -0.272552490234375
3.35964584350586 -0.272590637207031
3.35964584350586 -0.272605895996094
3.35983538627625 -0.272651672363281
3.3604040145874 -0.272666931152344
3.36116099357605 -0.272689819335938
3.36116099357605 -0.272712707519531
3.36172795295715 -0.272720336914062
3.36604928970337 -0.272926330566406
3.37566351890564 -0.273582458496094
3.37712407112122 -0.273666381835938
3.38183689117432 -0.273689270019531
3.38255739212036 -0.273750305175781
3.38291716575623 -0.273773193359375
3.38417410850525 -0.273796081542969
3.38614201545715 -0.273849487304688
3.39164066314697 -0.273994445800781
3.39480185508728 -0.2740478515625
3.39515161514282 -0.274070739746094
3.39654803276062 -0.274093627929688
3.39654803276062 -0.274101257324219
3.40534639358521 -0.274261474609375
3.40585851669312 -0.274322509765625
3.41896390914917 -0.274055480957031
3.42291808128357 -0.274131774902344
3.42308187484741 -0.274147033691406
3.42324590682983 -0.274162292480469
3.43456888198853 -0.274665832519531
3.43488812446594 -0.274703979492188
3.43901681900024 -0.274787902832031
3.43933272361755 -0.274818420410156
3.43964838981628 -0.27484130859375
3.44169521331787 -0.274864196777344
3.44185209274292 -0.274909973144531
3.44653725624084 -0.274932861328125
3.44700288772583 -0.274955749511719
3.44793295860291 -0.274993896484375
3.44808769226074 -0.275016784667969
3.4499409198761 -0.275047302246094
3.45454001426697 -0.275291442871094
3.4577305316925 -0.275321960449219
3.4601457118988 -0.275344848632812
3.4602963924408 -0.275360107421875
3.46044683456421 -0.275367736816406
3.4610481262207 -0.275398254394531
3.46553158760071 -0.275428771972656
3.46568012237549 -0.27545166015625
3.46568012237549 -0.275482177734375
3.46627426147461 -0.275497436523438
3.46627426147461 -0.2755126953125
3.46627426147461 -0.275527954101562
3.46819949150085 -0.275543212890625
3.47070455551147 -0.275550842285156
3.47697639465332 -0.275848388671875
3.48144268989563 -0.275894165039062
3.48158597946167 -0.275901794433594
3.48315930366516 -0.275947570800781
3.48358726501465 -0.275970458984375
3.48543739318848 -0.276008605957031
3.48586320877075 -0.276031494140625
3.48911428451538 -0.276039123535156
3.48925518989563 -0.276054382324219
3.49122166633606 -0.276138305664062
3.49164175987244 -0.276168823242188
3.49178171157837 -0.276191711425781
3.49415469169617 -0.276199340820312
3.49665284156799 -0.276321411132812
3.49899935722351 -0.276336669921875
3.500648021698 -0.276351928710938
3.50078511238098 -0.2763671875
3.50119614601135 -0.276374816894531
3.50133323669434 -0.276390075683594
3.50133323669434 -0.276397705078125
3.5055570602417 -0.276458740234375
3.50582814216614 -0.276473999023438
3.50582814216614 -0.276481628417969
3.50758600234985 -0.276504516601562
3.50772094726562 -0.276512145996094
3.5156090259552 -0.277206420898438
3.51640319824219 -0.277275085449219
3.51706385612488 -0.27728271484375
3.5171959400177 -0.277290344238281
3.5171959400177 -0.277305603027344
3.51732778549194 -0.277313232421875
3.51745986938477 -0.277320861816406
3.51745986938477 -0.277328491210938
3.5202214717865 -0.277336120605469
3.5202214717865 -0.27734375
3.5202214717865 -0.277351379394531
3.520352602005 -0.277359008789062
3.52633929252625 -0.277992248535156
3.52968692779541 -0.278076171875
3.53019976615906 -0.278083801269531
3.53249955177307 -0.278091430664062
3.53262710571289 -0.278099060058594
3.53275442123413 -0.278106689453125
3.53313636779785 -0.278114318847656
3.53326344490051 -0.278121948242188
3.53945255279541 -0.278160095214844
3.53957796096802 -0.278167724609375
3.53970313072205 -0.278167724609375
3.53982853889465 -0.278175354003906
3.53995394706726 -0.278175354003906
3.54007911682129 -0.278182983398438
3.54406809806824 -0.278251647949219
3.54456400871277 -0.278297424316406
3.54481196403503 -0.278297424316406
3.54505968093872 -0.278305053710938
3.54518342018127 -0.278305053710938
3.54530715942383 -0.278312683105469
3.54543089866638 -0.278312683105469
3.54543089866638 -0.278312683105469
3.54555439949036 -0.278327941894531
3.54555439949036 -0.278327941894531
3.54641938209534 -0.278335571289062
3.54654264450073 -0.278335571289062
3.54654264450073 -0.278335571289062
3.54654264450073 -0.278343200683594
3.54654264450073 -0.278343200683594
3.54826664924622 -0.278350830078125
3.54838943481445 -0.278358459472656
3.54851222038269 -0.278358459472656
3.54863500595093 -0.278366088867188
3.54875779151917 -0.278373718261719
3.5488805770874 -0.278373718261719
3.54961633682251 -0.27838134765625
3.54961633682251 -0.27838134765625
3.5505952835083 -0.27838134765625
3.5505952835083 -0.278388977050781
3.5507173538208 -0.278396606445312
3.55083966255188 -0.278396606445312
3.55083966255188 -0.278404235839844
3.55400443077087 -0.278457641601562
3.55400443077087 -0.278457641601562
3.55400443077087 -0.278457641601562
3.55424690246582 -0.278465270996094
3.554368019104 -0.278465270996094
3.55786800384521 -0.278541564941406
3.55822849273682 -0.278564453125
3.5583484172821 -0.278564453125
3.5583484172821 -0.278564453125
3.5583484172821 -0.278572082519531
3.56026530265808 -0.278579711914062
3.56026530265808 -0.278579711914062
3.56026530265808 -0.278579711914062
3.56026530265808 -0.278587341308594
3.56026530265808 -0.278587341308594
3.56038498878479 -0.278602600097656
3.56050443649292 -0.278602600097656
3.56050443649292 -0.278602600097656
3.56098198890686 -0.278617858886719
3.56157827377319 -0.278617858886719
3.56157827377319 -0.27862548828125
3.56181669235229 -0.27862548828125
3.56193590164185 -0.278633117675781
3.56193590164185 -0.278633117675781
3.56442928314209 -0.278648376464844
3.5645477771759 -0.278648376464844
3.5645477771759 -0.278648376464844
3.5645477771759 -0.278648376464844
3.56466603279114 -0.278656005859375
3.56831908226013 -0.278770446777344
3.57135939598083 -0.278816223144531
3.57159233093262 -0.278823852539062
3.5717089176178 -0.278823852539062
3.5718252658844 -0.278823852539062
3.571941614151 -0.278831481933594
3.5720579624176 -0.278831481933594
3.5721743106842 -0.278839111328125
3.5749568939209 -0.278846740722656
3.57518792152405 -0.278854370117188
3.57518792152405 -0.278854370117188
3.57530331611633 -0.278854370117188
3.57541871070862 -0.278861999511719
3.57541871070862 -0.278861999511719
3.57541871070862 -0.27886962890625
3.57553434371948 -0.27886962890625
3.57564973831177 -0.27886962890625
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{C2}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3},
extra x tick labels={\small$\text{log}_{10}$},  
extra x ticks={4.5},  
extra x tick style={grid=none, tickwidth=0,
tick label style={opacity=1}},
xmin=-0.23, xmax=4.64841993451118,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.281445693969727, ymax=0.0134021759033203,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c3)}
]
\addplot [ultra thick, brown, dashed]
table {%
1.6334685087204 -6.103515625e-05
2.04532289505005 -0.00099945068359375
2.20139718055725 -0.00160980224609375
2.63648796081543 -0.00820159912109375
2.7693772315979 -0.0133514404296875
2.85973858833313 -0.0147476196289062
2.93449854850769 -0.01617431640625
3.04178738594055 -0.0193252563476562
3.18212914466858 -0.0257415771484375
3.29092454910278 -0.0333328247070312
3.33405137062073 -0.037750244140625
3.45969390869141 -0.0483322143554688
3.51666760444641 -0.056793212890625
3.5635998249054 -0.0604248046875
3.58871984481812 -0.0623245239257812
3.67089486122131 -0.069091796875
3.70415043830872 -0.076812744140625
3.72811007499695 -0.079925537109375
3.7499680519104 -0.0832595825195312
3.77568316459656 -0.0863113403320312
3.80529689788818 -0.0902481079101562
3.83174180984497 -0.0945510864257812
3.85241889953613 -0.0970306396484375
3.8703453540802 -0.0984115600585938
3.90368676185608 -0.102340698242188
3.92396903038025 -0.104324340820312
3.94482803344727 -0.106513977050781
3.96862292289734 -0.108474731445312
3.98344588279724 -0.110313415527344
4.00813150405884 -0.11724853515625
4.02333498001099 -0.122703552246094
4.03718757629395 -0.12603759765625
4.04906272888184 -0.131385803222656
4.0666241645813 -0.146080017089844
4.07580232620239 -0.173751831054688
4.08504056930542 -0.185928344726562
4.0962495803833 -0.194633483886719
4.10445308685303 -0.201393127441406
4.1152777671814 -0.208511352539062
4.12142848968506 -0.214714050292969
4.12775230407715 -0.219444274902344
4.1353235244751 -0.226524353027344
4.14166927337646 -0.229934692382812
4.14921903610229 -0.231849670410156
4.15848302841187 -0.234329223632812
4.16357898712158 -0.235237121582031
4.16784858703613 -0.235939025878906
4.17266130447388 -0.236701965332031
4.17992496490479 -0.238723754882812
4.18656063079834 -0.240570068359375
4.19167470932007 -0.24139404296875
4.19865703582764 -0.242340087890625
4.20316886901855 -0.242935180664062
4.21128082275391 -0.245773315429688
4.2145791053772 -0.24639892578125
4.21916532516479 -0.246955871582031
4.22313213348389 -0.247276306152344
4.22652244567871 -0.24761962890625
4.23067855834961 -0.248268127441406
4.23390960693359 -0.248527526855469
4.23959970474243 -0.250640869140625
4.24345970153809 -0.251899719238281
4.24748229980469 -0.252723693847656
4.25002956390381 -0.253150939941406
4.25333786010742 -0.25396728515625
4.25529670715332 -0.254203796386719
4.26016664505005 -0.255599975585938
4.26161956787109 -0.255943298339844
4.26592588424683 -0.256759643554688
4.26766443252563 -0.256973266601562
4.26909255981445 -0.257156372070312
4.27119064331055 -0.257339477539062
4.27235221862793 -0.2574462890625
4.27406549453735 -0.257682800292969
4.27607107162476 -0.258308410644531
4.27765512466431 -0.258590698242188
4.27973556518555 -0.258705139160156
4.2813515663147 -0.258796691894531
4.28300714492798 -0.258926391601562
4.28447580337524 -0.258995056152344
4.28596210479736 -0.259124755859375
4.28764486312866 -0.259269714355469
4.28929901123047 -0.259330749511719
4.29039096832275 -0.259384155273438
4.29453229904175 -0.260604858398438
4.29635810852051 -0.260841369628906
4.29789161682129 -0.260910034179688
4.30005168914795 -0.261009216308594
4.30267715454102 -0.261520385742188
4.30386543273926 -0.261642456054688
4.30573797225952 -0.26171875
4.30794525146484 -0.261825561523438
4.3093318939209 -0.261924743652344
4.31103277206421 -0.262123107910156
4.31257915496826 -0.262191772460938
4.31506729125977 -0.26275634765625
4.3178334236145 -0.262931823730469
4.3190016746521 -0.262985229492188
4.32025003433228 -0.263137817382812
4.32178497314453 -0.26318359375
4.32339668273926 -0.263236999511719
4.32502269744873 -0.263404846191406
4.32608985900879 -0.263465881347656
4.32766532897949 -0.263656616210938
4.33086013793945 -0.263893127441406
4.33195352554321 -0.263938903808594
4.3335280418396 -0.263999938964844
4.33469486236572 -0.264030456542969
4.33641958236694 -0.264205932617188
4.33755922317505 -0.264236450195312
4.33825731277466 -0.264274597167969
4.3390736579895 -0.264312744140625
4.34040451049805 -0.264366149902344
4.34165191650391 -0.264389038085938
4.34299468994141 -0.264450073242188
4.34582424163818 -0.264595031738281
4.34752511978149 -0.264678955078125
4.35018968582153 -0.264755249023438
4.35206651687622 -0.264839172363281
4.35241413116455 -0.264846801757812
4.35351228713989 -0.264884948730469
4.35585355758667 -0.264999389648438
4.35635089874268 -0.2650146484375
4.35804891586304 -0.265068054199219
4.35958909988403 -0.265083312988281
4.35993051528931 -0.265098571777344
4.36104774475098 -0.265159606933594
4.36223745346069 -0.265182495117188
4.36466360092163 -0.265327453613281
4.36595582962036 -0.265342712402344
4.36851024627686 -0.265426635742188
4.36943864822388 -0.265464782714844
4.37029075622559 -0.265472412109375
4.37156677246094 -0.265518188476562
4.37224912643433 -0.265533447265625
4.37272787094116 -0.265541076660156
4.37379455566406 -0.265548706054688
4.37401485443115 -0.265556335449219
4.37480354309082 -0.26556396484375
4.3753342628479 -0.265579223632812
4.3759560585022 -0.265586853027344
4.3767409324646 -0.265602111816406
4.37750673294067 -0.265609741210938
4.37925100326538 -0.265701293945312
4.38003015518188 -0.265708923339844
4.38019323348999 -0.265716552734375
4.38367176055908 -0.266098022460938
4.38426399230957 -0.266128540039062
4.38458633422852 -0.266128540039062
4.38557052612305 -0.266151428222656
4.38623142242432 -0.266159057617188
4.38715839385986 -0.266181945800781
4.38920164108276 -0.266227722167969
4.38953828811646 -0.2662353515625
4.39022827148438 -0.266242980957031
4.39109420776367 -0.266250610351562
4.39158773422241 -0.266258239746094
4.3931713104248 -0.266273498535156
4.39877319335938 -0.266944885253906
4.39970827102661 -0.267158508300781
4.40065908432007 -0.267173767089844
4.40096950531006 -0.267181396484375
4.40158987045288 -0.267189025878906
4.40222692489624 -0.267204284667969
4.40318918228149 -0.267219543457031
4.4037036895752 -0.267227172851562
4.40402936935425 -0.267227172851562
4.40628480911255 -0.267303466796875
4.40761184692383 -0.267311096191406
4.40832471847534 -0.267326354980469
4.40925645828247 -0.267333984375
4.41069269180298 -0.267364501953125
4.41108083724976 -0.267372131347656
4.4127459526062 -0.267379760742188
4.41547393798828 -0.267433166503906
4.41634082794189 -0.2674560546875
4.41713953018188 -0.267471313476562
4.41780376434326 -0.267478942871094
4.41871547698975 -0.267486572265625
4.41970777511597 -0.267486572265625
4.42069816589355 -0.26751708984375
4.42127466201782 -0.26751708984375
4.42226123809814 -0.267524719238281
4.42234373092651 -0.267524719238281
4.42237663269043 -0.267532348632812
4.42393350601196 -0.267578125
4.42488145828247 -0.267593383789062
4.42512655258179 -0.267593383789062
4.4254035949707 -0.267601013183594
4.42582750320435 -0.267601013183594
4.42688512802124 -0.267608642578125
4.42704772949219 -0.267616271972656
4.42771339416504 -0.267623901367188
4.42852354049683 -0.26763916015625
4.43002653121948 -0.267654418945312
4.43115472793579 -0.267669677734375
4.43324184417725 -0.2677001953125
4.43373775482178 -0.2677001953125
4.43381786346436 -0.267707824707031
4.43428134918213 -0.267715454101562
4.4352388381958 -0.267715454101562
4.43554162979126 -0.267723083496094
4.43624210357666 -0.267730712890625
4.43630599975586 -0.267730712890625
4.43648052215576 -0.267738342285156
4.43743324279785 -0.267753601074219
4.43835258483887 -0.26776123046875
4.43882703781128 -0.267776489257812
4.43950653076172 -0.267776489257812
4.44037389755249 -0.267791748046875
4.44160079956055 -0.267791748046875
4.44200897216797 -0.267799377441406
4.44215059280396 -0.267799377441406
4.44421672821045 -0.267860412597656
4.44476270675659 -0.267868041992188
4.44533967971802 -0.267868041992188
4.44867563247681 -0.268028259277344
4.44906187057495 -0.268043518066406
4.44933938980103 -0.268043518066406
4.44978666305542 -0.268043518066406
};
\addplot [ultra thick, blue]
table {%
0.477121233940125 0
0.84509801864624 -0.000732421875
1.14612805843353 -0.0017852783203125
1.49136173725128 -0.00658416748046875
1.57978355884552 -0.0098114013671875
1.74036264419556 -0.0125732421875
1.79934048652649 -0.01409912109375
1.90309000015259 -0.0162582397460938
2.03742647171021 -0.0216827392578125
2.07918119430542 -0.0255126953125
2.15836238861084 -0.028839111328125
2.24303793907166 -0.0400238037109375
2.2810332775116 -0.0477066040039062
2.35793495178223 -0.0561447143554688
2.40140056610107 -0.060516357421875
2.44404482841492 -0.064727783203125
2.48000693321228 -0.0687255859375
2.53529405593872 -0.0725936889648438
2.56937384605408 -0.0784988403320312
2.63548374176025 -0.0849990844726562
2.65224623680115 -0.0888595581054688
2.67302083969116 -0.0921173095703125
2.70586371421814 -0.0945587158203125
2.72263383865356 -0.0968170166015625
2.74036264419556 -0.099273681640625
2.76117587089539 -0.100410461425781
2.77451705932617 -0.101783752441406
2.79028511047363 -0.102615356445312
2.82994675636292 -0.112022399902344
2.85003328323364 -0.11834716796875
2.86923170089722 -0.12176513671875
2.89265108108521 -0.125556945800781
2.92479610443115 -0.134391784667969
2.95808577537537 -0.153701782226562
2.99299502372742 -0.176658630371094
3.0182843208313 -0.184577941894531
3.04844188690186 -0.193069458007812
3.06781458854675 -0.199653625488281
3.0852906703949 -0.204864501953125
3.10071516036987 -0.210014343261719
3.11494445800781 -0.21527099609375
3.12839937210083 -0.221405029296875
3.14921903610229 -0.226966857910156
3.16761255264282 -0.230110168457031
3.18127179145813 -0.231559753417969
3.19617629051208 -0.233161926269531
3.20574545860291 -0.23492431640625
3.21218752861023 -0.235710144042969
3.21774697303772 -0.236892700195312
3.22453308105469 -0.237472534179688
3.23477029800415 -0.23931884765625
3.24303817749023 -0.240196228027344
3.2550311088562 -0.242172241210938
3.262451171875 -0.244338989257812
3.26787543296814 -0.245063781738281
3.27737998962402 -0.24542236328125
3.28510713577271 -0.246681213378906
3.28958892822266 -0.247123718261719
3.29710364341736 -0.247955322265625
3.30384373664856 -0.248359680175781
3.30792379379272 -0.248786926269531
3.31302309036255 -0.249221801757812
3.32345843315125 -0.250411987304688
3.32939791679382 -0.250862121582031
3.33324575424194 -0.251350402832031
3.33745932579041 -0.251739501953125
3.34498143196106 -0.252494812011719
3.35024809837341 -0.253089904785156
3.35237550735474 -0.253440856933594
3.3626708984375 -0.25421142578125
3.3651134967804 -0.254562377929688
3.36810088157654 -0.254806518554688
3.3725438117981 -0.255043029785156
3.38165640830994 -0.256698608398438
3.38345623016357 -0.25714111328125
3.3868556022644 -0.257415771484375
3.38952040672302 -0.257637023925781
3.39181685447693 -0.257865905761719
3.39585041999817 -0.258140563964844
3.4020893573761 -0.258491516113281
3.40346360206604 -0.258651733398438
3.4070508480072 -0.258720397949219
3.41077733039856 -0.258918762207031
3.4126284122467 -0.259025573730469
3.41547417640686 -0.259132385253906
3.4186327457428 -0.259246826171875
3.42143940925598 -0.259330749511719
3.42209720611572 -0.2593994140625
3.42488169670105 -0.25946044921875
3.42569732666016 -0.259521484375
3.43055868148804 -0.259696960449219
3.43552589416504 -0.260223388671875
3.43870043754578 -0.260292053222656
3.44326305389404 -0.26055908203125
3.44560408592224 -0.260696411132812
3.44684767723083 -0.260757446289062
3.44839715957642 -0.260826110839844
3.45117211341858 -0.260932922363281
3.45362401008606 -0.261001586914062
3.45788192749023 -0.261184692382812
3.45969390869141 -0.261299133300781
3.4631462097168 -0.261444091796875
3.46419143676758 -0.261558532714844
3.47070455551147 -0.262123107910156
3.47436189651489 -0.262321472167969
3.47625184059143 -0.26239013671875
3.48086881637573 -0.262565612792969
3.48230171203613 -0.262657165527344
3.48429989814758 -0.262718200683594
3.48784518241882 -0.26312255859375
3.48911428451538 -0.263221740722656
3.49359750747681 -0.263313293457031
3.49484992027283 -0.263404846191406
3.49651455879211 -0.263442993164062
3.50201725959778 -0.263877868652344
3.5029730796814 -0.263938903808594
3.50365447998047 -0.26397705078125
3.50528573989868 -0.264045715332031
3.50664019584656 -0.264076232910156
3.50772094726562 -0.264129638671875
3.50826025009155 -0.264167785644531
3.51054501533508 -0.264198303222656
3.51054501533508 -0.264205932617188
3.51388311386108 -0.264480590820312
3.51414918899536 -0.264511108398438
3.51428198814392 -0.264541625976562
3.51679968833923 -0.264556884765625
3.52061462402344 -0.264892578125
3.52387642860413 -0.264907836914062
3.52465581893921 -0.264968872070312
3.5250449180603 -0.264984130859375
3.52543354034424 -0.265007019042969
3.52556300163269 -0.265022277832031
3.52569246292114 -0.265037536621094
3.52685594558716 -0.265060424804688
3.52827382087708 -0.265113830566406
3.52904510498047 -0.26513671875
3.5294303894043 -0.265151977539062
3.52981519699097 -0.265167236328125
3.52994346618652 -0.265174865722656
3.5300714969635 -0.265182495117188
3.53019976615906 -0.26519775390625
3.53032779693604 -0.265220642089844
3.53198957443237 -0.265228271484375
3.53237199783325 -0.265243530273438
3.53237199783325 -0.265251159667969
3.53237199783325 -0.265266418457031
3.53529405593872 -0.265312194824219
3.53529405593872 -0.265350341796875
3.53554725646973 -0.265365600585938
3.53554725646973 -0.265380859375
3.53920149803162 -0.265411376953125
3.5393271446228 -0.265419006347656
3.54332280158997 -0.265609741210938
3.54357147216797 -0.265640258789062
3.54369568824768 -0.265655517578125
3.54419207572937 -0.265663146972656
3.5443160533905 -0.265670776367188
3.54505968093872 -0.265731811523438
3.54543089866638 -0.265739440917969
3.54777479171753 -0.265830993652344
3.55010604858398 -0.265899658203125
3.55010604858398 -0.265907287597656
3.55108380317688 -0.265960693359375
3.55120587348938 -0.265960693359375
3.55786800384521 -0.266220092773438
3.55798816680908 -0.266258239746094
3.55870866775513 -0.266281127929688
3.56050443649292 -0.266288757324219
3.56050443649292 -0.266288757324219
3.563481092453 -0.266372680664062
3.56490278244019 -0.266380310058594
3.56537556648254 -0.266403198242188
3.56831908226013 -0.266433715820312
3.56843638420105 -0.266441345214844
3.56937384605408 -0.266471862792969
3.56972503662109 -0.2664794921875
3.57147598266602 -0.266525268554688
3.5717089176178 -0.266532897949219
3.5718252658844 -0.26654052734375
3.57252311706543 -0.266548156738281
3.5749568939209 -0.266578674316406
3.57507228851318 -0.266593933105469
3.57611083984375 -0.266616821289062
3.57737684249878 -0.266639709472656
3.57749176025391 -0.266647338867188
3.58240437507629 -0.266670227050781
3.58251786231995 -0.266685485839844
3.58365201950073 -0.266708374023438
3.58455729484558 -0.2667236328125
3.58478331565857 -0.266738891601562
3.58860778808594 -0.266777038574219
3.58871984481812 -0.26678466796875
3.58950281143188 -0.266792297363281
3.58961462974548 -0.266807556152344
3.59050750732422 -0.266822814941406
3.59139847755432 -0.266845703125
3.59150981903076 -0.266853332519531
3.59461355209351 -0.266891479492188
3.59483432769775 -0.26690673828125
3.5990092754364 -0.267059326171875
3.59922790527344 -0.267097473144531
3.60010123252869 -0.267127990722656
3.60021042823792 -0.267135620117188
3.60042834281921 -0.26715087890625
3.60129928588867 -0.267158508300781
3.60303616523743 -0.267181396484375
3.60314440727234 -0.267181396484375
3.60487389564514 -0.267280578613281
3.61066007614136 -0.267288208007812
3.61076664924622 -0.267295837402344
3.61236000061035 -0.267341613769531
3.61267781257629 -0.267349243164062
3.61278390884399 -0.267364501953125
3.61288976669312 -0.267364501953125
3.61299562454224 -0.267372131347656
3.61909341812134 -0.267494201660156
3.61971926689148 -0.267585754394531
3.61982345581055 -0.267585754394531
3.61982345581055 -0.267593383789062
3.62128019332886 -0.267662048339844
3.62128019332886 -0.267662048339844
3.62407565116882 -0.267669677734375
3.62417888641357 -0.267677307128906
3.62417888641357 -0.267677307128906
3.62417888641357 -0.267684936523438
3.62582659721375 -0.267707824707031
3.62592959403992 -0.267707824707031
3.62603235244751 -0.267715454101562
3.62613487243652 -0.267730712890625
3.62623763084412 -0.267730712890625
3.62634038925171 -0.267738342285156
3.62644290924072 -0.267738342285156
3.62654566764832 -0.267745971679688
3.6306312084198 -0.26776123046875
3.63093614578247 -0.267768859863281
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{Cl2O}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.72904717922211,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.337033081054687, ymax=0.0160491943359375,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c4)}
]
\addplot [ultra thick, brown, dashed]
table {%
2.27184152603149 0
2.42324590682983 0
2.45939254760742 -6.103515625e-05
2.69284701347351 -6.103515625e-05
2.72835373878479 -6.103515625e-05
2.86923170089722 -0.0001220703125
2.93951916694641 -0.0001220703125
2.95951843261719 -0.0001220703125
2.98900461196899 -0.0001220703125
2.99475693702698 -0.0001220703125
3.04727482795715 -0.00018310546875
3.25478959083557 -0.00067138671875
3.30081272125244 -0.00079345703125
3.37639451026917 -0.00079345703125
3.39724469184875 -0.00079345703125
3.41747164726257 -0.0008544921875
3.47538065910339 -0.00091552734375
3.50542140007019 -0.00091552734375
3.51534390449524 -0.0009765625
3.5446879863739 -0.00103759765625
3.54604887962341 -0.00103759765625
3.59494471549988 -0.00115966796875
3.60281944274902 -0.001220703125
3.62335276603699 -0.00128173828125
3.63748979568481 -0.00128173828125
3.63968563079834 -0.00140380859375
3.67292881011963 -0.00152587890625
3.6801540851593 -0.00152587890625
3.68645763397217 -0.00164794921875
3.6929349899292 -0.001708984375
3.7196626663208 -0.00201416015625
3.72525811195374 -0.0020751953125
3.77224826812744 -0.0032958984375
3.78139638900757 -0.0035400390625
3.82321333885193 -0.004150390625
3.83960366249084 -0.0042724609375
3.8707549571991 -0.00543212890625
3.88468217849731 -0.00579833984375
3.90336132049561 -0.0059814453125
3.91460752487183 -0.0067138671875
3.94561624526978 -0.009521484375
3.96246409416199 -0.0101318359375
3.99211144447327 -0.01422119140625
4.02304649353027 -0.016357421875
4.05026388168335 -0.018310546875
4.0588812828064 -0.01922607421875
4.09415674209595 -0.02215576171875
4.14154386520386 -0.03326416015625
4.15237998962402 -0.03656005859375
4.17519283294678 -0.03973388671875
4.19578886032104 -0.0411376953125
4.2178258895874 -0.04193115234375
4.22988653182983 -0.042724609375
4.2831654548645 -0.04852294921875
4.29234457015991 -0.0499267578125
4.30168104171753 -0.05072021484375
4.31306552886963 -0.051025390625
4.33219623565674 -0.05450439453125
4.33949136734009 -0.05499267578125
4.34762287139893 -0.05548095703125
4.35852479934692 -0.05584716796875
4.37370252609253 -0.0576171875
4.37901544570923 -0.058349609375
4.39274978637695 -0.05926513671875
4.40674448013306 -0.06036376953125
4.44586896896362 -0.0694580078125
4.45284414291382 -0.07366943359375
4.47373485565186 -0.0816650390625
4.48910045623779 -0.08642578125
4.50672149658203 -0.089111328125
4.52386331558228 -0.0943603515625
4.55592823028564 -0.11505126953125
4.56520986557007 -0.12664794921875
4.57736539840698 -0.1297607421875
4.58939123153687 -0.1319580078125
4.59753084182739 -0.13525390625
4.60319852828979 -0.13665771484375
4.61429595947266 -0.1396484375
4.62209987640381 -0.140869140625
4.63249778747559 -0.14556884765625
4.64230632781982 -0.1475830078125
4.65082216262817 -0.1483154296875
4.65445566177368 -0.1488037109375
4.6594123840332 -0.14959716796875
4.66492366790771 -0.15008544921875
4.67050552368164 -0.151123046875
4.68252420425415 -0.16046142578125
4.69255590438843 -0.16510009765625
4.69916963577271 -0.1658935546875
4.70370388031006 -0.16632080078125
4.71386861801147 -0.17913818359375
4.72118377685547 -0.1827392578125
4.72489023208618 -0.18359375
4.73079013824463 -0.18682861328125
4.73515176773071 -0.18768310546875
4.74101781845093 -0.18896484375
4.74522304534912 -0.18994140625
4.75047779083252 -0.19110107421875
4.76138639450073 -0.19891357421875
4.76338291168213 -0.2003173828125
4.76772689819336 -0.20086669921875
4.77304744720459 -0.20159912109375
4.77522420883179 -0.20196533203125
4.7811017036438 -0.20379638671875
4.78466701507568 -0.20428466796875
4.78899526596069 -0.2052001953125
4.79633855819702 -0.207763671875
4.80230855941772 -0.20831298828125
4.80844736099243 -0.21160888671875
4.81210422515869 -0.212646484375
4.82048368453979 -0.2152099609375
4.82310247421265 -0.2156982421875
4.82750511169434 -0.21636962890625
4.82902050018311 -0.2166748046875
4.83234930038452 -0.21697998046875
4.83700752258301 -0.22076416015625
4.84035062789917 -0.22271728515625
4.84476900100708 -0.22308349609375
4.85076856613159 -0.22943115234375
4.85336351394653 -0.2310791015625
4.85726022720337 -0.231689453125
4.85945653915405 -0.2320556640625
4.86261415481567 -0.2330322265625
4.8655834197998 -0.23333740234375
4.86795043945312 -0.23382568359375
4.87025737762451 -0.234130859375
4.87565135955811 -0.237060546875
4.87860774993896 -0.239013671875
4.88011026382446 -0.239501953125
4.88330936431885 -0.24017333984375
4.88725709915161 -0.2432861328125
4.88865661621094 -0.243896484375
4.8894305229187 -0.2442626953125
4.89305114746094 -0.24468994140625
4.89446020126343 -0.24530029296875
4.89684581756592 -0.24591064453125
4.89793491363525 -0.24615478515625
4.90149641036987 -0.24774169921875
4.90305757522583 -0.2481689453125
4.90419054031372 -0.24835205078125
4.90880107879639 -0.25006103515625
4.90948629379272 -0.25048828125
4.911301612854 -0.25067138671875
4.91293907165527 -0.25103759765625
4.91720628738403 -0.2513427734375
4.91799879074097 -0.25146484375
4.9201807975769 -0.25177001953125
4.92136383056641 -0.251953125
4.92263746261597 -0.2520751953125
4.92871332168579 -0.254638671875
4.93035793304443 -0.2550048828125
4.93138647079468 -0.255126953125
4.93453359603882 -0.2557373046875
4.93660402297974 -0.25592041015625
4.93957901000977 -0.2559814453125
4.94075536727905 -0.25628662109375
4.94184446334839 -0.2564697265625
4.94340562820435 -0.256591796875
4.94650650024414 -0.2574462890625
4.94770336151123 -0.25762939453125
4.9489164352417 -0.2576904296875
4.95271968841553 -0.25830078125
4.95552444458008 -0.25848388671875
4.95712804794312 -0.258544921875
4.96510744094849 -0.259765625
4.96783351898193 -0.2598876953125
4.96876764297485 -0.25994873046875
4.96984434127808 -0.26007080078125
4.97617101669312 -0.26123046875
4.97754526138306 -0.26141357421875
4.97818040847778 -0.261474609375
4.98018503189087 -0.2615966796875
4.98256969451904 -0.26171875
4.98452281951904 -0.26171875
4.99330854415894 -0.265380859375
4.99488019943237 -0.266845703125
4.99775743484497 -0.2669677734375
5.00047731399536 -0.26702880859375
5.00362873077393 -0.26715087890625
5.00647449493408 -0.267333984375
5.00883436203003 -0.2674560546875
5.01079177856445 -0.267578125
5.01562786102295 -0.26800537109375
5.01693725585938 -0.2681884765625
5.02393531799316 -0.2685546875
5.02567863464355 -0.268798828125
5.02791595458984 -0.2689208984375
5.03027153015137 -0.26904296875
5.03447198867798 -0.26953125
5.03681659698486 -0.26959228515625
5.03893375396729 -0.26971435546875
5.04090309143066 -0.2698974609375
5.04256391525269 -0.2698974609375
5.04815053939819 -0.2716064453125
5.04910945892334 -0.27191162109375
5.05173873901367 -0.27203369140625
5.05588626861572 -0.272216796875
5.05690479278564 -0.27227783203125
5.05778408050537 -0.27227783203125
5.06095457077026 -0.273193359375
5.06287908554077 -0.2733154296875
5.0652174949646 -0.27349853515625
5.06786632537842 -0.27386474609375
5.06987905502319 -0.27398681640625
5.07314252853394 -0.27459716796875
5.07380247116089 -0.274658203125
5.08273887634277 -0.2781982421875
5.08397912979126 -0.28057861328125
5.08595037460327 -0.28082275390625
5.08932590484619 -0.28131103515625
5.09013080596924 -0.2816162109375
5.09194469451904 -0.28173828125
5.09281539916992 -0.2818603515625
5.09539937973022 -0.28228759765625
5.09810018539429 -0.2825927734375
5.1025915145874 -0.28717041015625
5.10504674911499 -0.28814697265625
5.10725736618042 -0.2884521484375
5.10849380493164 -0.288818359375
5.109787940979 -0.28912353515625
5.11141395568848 -0.289306640625
5.11277914047241 -0.2894287109375
5.11545419692993 -0.2911376953125
5.11680364608765 -0.29150390625
5.11825466156006 -0.29168701171875
5.1191668510437 -0.29180908203125
5.12099504470825 -0.29217529296875
5.12212085723877 -0.29248046875
5.12383508682251 -0.2928466796875
5.12462472915649 -0.2930908203125
5.12749338150024 -0.29327392578125
5.12864780426025 -0.2935791015625
5.12955760955811 -0.29376220703125
5.13072919845581 -0.29388427734375
5.13188171386719 -0.29412841796875
5.13282299041748 -0.29425048828125
5.13366031646729 -0.2943115234375
5.13564443588257 -0.2945556640625
5.13766431808472 -0.294677734375
5.13877630233765 -0.2947998046875
5.13980960845947 -0.2947998046875
5.14091300964355 -0.294921875
5.14194202423096 -0.2950439453125
5.14250230789185 -0.2950439453125
5.14479207992554 -0.29559326171875
5.1467137336731 -0.2957763671875
5.14803791046143 -0.29583740234375
5.14898490905762 -0.2958984375
5.15047073364258 -0.29595947265625
5.1520037651062 -0.2962646484375
5.15565156936646 -0.29766845703125
5.15661287307739 -0.2978515625
5.15778589248657 -0.29791259765625
5.15818452835083 -0.2979736328125
5.15865182876587 -0.29803466796875
5.16002988815308 -0.298095703125
5.16038131713867 -0.298095703125
5.16221189498901 -0.29815673828125
5.16337919235229 -0.29833984375
5.16538667678833 -0.29840087890625
5.16677331924438 -0.2984619140625
5.16824388504028 -0.298583984375
5.16918325424194 -0.298583984375
5.17067813873291 -0.298583984375
5.17440891265869 -0.2998046875
5.17493438720703 -0.29998779296875
5.17577266693115 -0.300048828125
5.17603635787964 -0.300048828125
5.17711782455444 -0.30010986328125
5.17935371398926 -0.30010986328125
5.18105983734131 -0.3001708984375
5.181640625 -0.3001708984375
5.18310737609863 -0.30023193359375
5.18369388580322 -0.30029296875
5.18457508087158 -0.30029296875
5.18472528457642 -0.30035400390625
5.18649578094482 -0.30047607421875
5.19174146652222 -0.30084228515625
5.19249773025513 -0.3011474609375
5.1939115524292 -0.3011474609375
5.19493293762207 -0.30120849609375
5.19509649276733 -0.30120849609375
5.20376682281494 -0.30426025390625
5.20465183258057 -0.30523681640625
5.20581865310669 -0.30535888671875
5.20740556716919 -0.305419921875
5.20978546142578 -0.30548095703125
5.21109914779663 -0.3055419921875
5.21376466751099 -0.30596923828125
5.2153491973877 -0.3060302734375
5.21693897247314 -0.30621337890625
5.21830940246582 -0.3062744140625
5.21922302246094 -0.3062744140625
5.22075653076172 -0.306396484375
5.2229790687561 -0.3067626953125
5.22398614883423 -0.306884765625
5.22476100921631 -0.30694580078125
5.22619771957397 -0.3070068359375
5.2288875579834 -0.30712890625
5.23061990737915 -0.30731201171875
5.23169898986816 -0.307373046875
5.23256921768188 -0.30743408203125
5.23456048965454 -0.3076171875
5.23649454116821 -0.30828857421875
5.23724222183228 -0.30853271484375
5.2388162612915 -0.3092041015625
5.23960208892822 -0.30938720703125
5.23990249633789 -0.3094482421875
5.24152660369873 -0.3099365234375
5.24219083786011 -0.31011962890625
5.242844581604 -0.3101806640625
5.24363565444946 -0.310302734375
5.24412870407104 -0.31036376953125
5.24460363388062 -0.3104248046875
5.24522399902344 -0.31072998046875
5.24582099914551 -0.31085205078125
5.24677896499634 -0.31103515625
5.24726343154907 -0.31109619140625
5.24749946594238 -0.31109619140625
5.24821615219116 -0.31121826171875
5.2491569519043 -0.31134033203125
5.24962615966797 -0.3114013671875
5.25007581710815 -0.31146240234375
5.25084924697876 -0.3116455078125
5.25115633010864 -0.3116455078125
5.25141191482544 -0.31170654296875
5.25173568725586 -0.31170654296875
5.25240135192871 -0.3118896484375
5.2526273727417 -0.31195068359375
5.25311279296875 -0.31201171875
5.25332355499268 -0.31207275390625
5.25434732437134 -0.3123779296875
5.25457715988159 -0.3125
5.25466156005859 -0.3125
5.2547173500061 -0.3125
5.25488138198853 -0.3125
5.25505781173706 -0.3125
5.25540018081665 -0.31256103515625
5.25561761856079 -0.31256103515625
5.25581741333008 -0.3126220703125
5.25616455078125 -0.3126220703125
5.25638103485107 -0.3126220703125
5.25667190551758 -0.3126220703125
5.25680685043335 -0.3126220703125
5.2569580078125 -0.31268310546875
5.2570686340332 -0.31268310546875
5.25714063644409 -0.31268310546875
5.25749158859253 -0.31268310546875
5.2575535774231 -0.31268310546875
5.25776958465576 -0.31268310546875
5.25790405273438 -0.31268310546875
5.25850820541382 -0.312744140625
5.25854873657227 -0.312744140625
5.25865411758423 -0.312744140625
5.25869464874268 -0.312744140625
5.25874042510986 -0.312744140625
5.25908946990967 -0.312744140625
5.25926637649536 -0.312744140625
5.25935506820679 -0.31280517578125
5.25960350036621 -0.31280517578125
5.26003551483154 -0.31280517578125
5.26021194458008 -0.31280517578125
5.26057958602905 -0.3128662109375
5.26072454452515 -0.3128662109375
5.26090574264526 -0.3128662109375
5.26132249832153 -0.31292724609375
5.26184558868408 -0.31292724609375
5.26201677322388 -0.31292724609375
5.26218271255493 -0.31292724609375
5.26254844665527 -0.31298828125
5.26294422149658 -0.31298828125
5.26307725906372 -0.31298828125
5.26370000839233 -0.31298828125
5.26403093338013 -0.31298828125
5.26430511474609 -0.31304931640625
5.26449680328369 -0.31304931640625
5.26478481292725 -0.31304931640625
5.26494741439819 -0.31304931640625
5.26513862609863 -0.31304931640625
5.26537466049194 -0.31304931640625
5.26565504074097 -0.31304931640625
5.26569747924805 -0.31304931640625
5.26591634750366 -0.3131103515625
5.26634216308594 -0.3131103515625
5.26663637161255 -0.3131103515625
5.26669502258301 -0.3131103515625
5.26675844192505 -0.3131103515625
5.26700735092163 -0.3131103515625
5.26715278625488 -0.3131103515625
5.26796436309814 -0.313232421875
5.26813554763794 -0.313232421875
5.26816368103027 -0.313232421875
5.26840734481812 -0.313232421875
5.2687816619873 -0.313232421875
5.26896619796753 -0.31329345703125
5.26916027069092 -0.31329345703125
5.26941728591919 -0.31329345703125
5.27011966705322 -0.31329345703125
5.27026414871216 -0.31329345703125
5.27029895782471 -0.3133544921875
5.2709789276123 -0.3133544921875
5.27100229263306 -0.3133544921875
5.27138137817383 -0.3133544921875
5.27160692214966 -0.3133544921875
5.27201366424561 -0.3133544921875
5.27201366424561 -0.3133544921875
5.27225732803345 -0.31341552734375
5.27275800704956 -0.31341552734375
5.27283430099487 -0.31341552734375
5.27294111251831 -0.31341552734375
5.27305459976196 -0.31341552734375
5.27309370040894 -0.31341552734375
5.27330446243286 -0.31341552734375
5.27334880828857 -0.31341552734375
5.27343893051147 -0.31341552734375
5.27378368377686 -0.31341552734375
5.2741322517395 -0.3134765625
5.27416944503784 -0.3134765625
5.27437019348145 -0.3134765625
5.27492618560791 -0.3134765625
5.27535533905029 -0.3134765625
5.2757396697998 -0.31353759765625
5.27594470977783 -0.31353759765625
5.27624368667603 -0.31353759765625
5.27626895904541 -0.31353759765625
5.27671003341675 -0.31353759765625
5.27681112289429 -0.31353759765625
5.27684307098389 -0.31353759765625
5.2774076461792 -0.3135986328125
5.27743482589722 -0.3135986328125
5.27807426452637 -0.3135986328125
5.27826881408691 -0.3135986328125
5.27886581420898 -0.31365966796875
5.27895927429199 -0.31365966796875
5.27950048446655 -0.31365966796875
5.27960062026978 -0.31365966796875
5.27965116500854 -0.31365966796875
5.27973747253418 -0.31365966796875
5.28333044052124 -0.31427001953125
5.28346395492554 -0.314453125
5.28366088867188 -0.314453125
5.2840313911438 -0.314453125
5.2843337059021 -0.31451416015625
5.2846155166626 -0.31451416015625
5.28503274917603 -0.31451416015625
5.2852783203125 -0.31451416015625
5.28544044494629 -0.31451416015625
5.28545808792114 -0.31451416015625
5.28576183319092 -0.31451416015625
5.28605890274048 -0.31451416015625
5.28661823272705 -0.31451416015625
5.28776597976685 -0.3145751953125
5.28811073303223 -0.3145751953125
5.28841924667358 -0.3145751953125
5.28868055343628 -0.3145751953125
5.28919410705566 -0.3145751953125
5.29001665115356 -0.3145751953125
5.29002141952515 -0.3145751953125
5.2902307510376 -0.31463623046875
5.29059553146362 -0.31463623046875
5.29198789596558 -0.31463623046875
5.29216766357422 -0.31463623046875
5.29240655899048 -0.31463623046875
5.29407596588135 -0.314697265625
5.29413080215454 -0.314697265625
5.29457855224609 -0.314697265625
5.29605054855347 -0.31475830078125
5.29619789123535 -0.31475830078125
5.29646110534668 -0.31475830078125
5.29685401916504 -0.31475830078125
5.29724836349487 -0.31475830078125
5.29802083969116 -0.3148193359375
5.29806900024414 -0.3148193359375
5.29825925827026 -0.3148193359375
5.29832458496094 -0.3148193359375
5.29852104187012 -0.3148193359375
5.29908847808838 -0.3148193359375
5.29931783676147 -0.3148193359375
5.29981660842896 -0.3148193359375
5.29990816116333 -0.3148193359375
5.30047369003296 -0.3148193359375
5.30065202713013 -0.31488037109375
5.30068683624268 -0.31488037109375
5.30247402191162 -0.31494140625
5.30327177047729 -0.31494140625
5.30344676971436 -0.31494140625
5.30381774902344 -0.31494140625
5.30521154403687 -0.31500244140625
5.30574893951416 -0.31500244140625
5.30594873428345 -0.31500244140625
5.30599784851074 -0.31500244140625
5.30660724639893 -0.31500244140625
5.30708312988281 -0.3150634765625
5.30826139450073 -0.3150634765625
5.30841732025146 -0.3150634765625
5.30885648727417 -0.3150634765625
5.30941295623779 -0.3150634765625
5.30971765518188 -0.3150634765625
5.31021499633789 -0.3150634765625
5.31035995483398 -0.3150634765625
5.3122239112854 -0.31536865234375
5.31280755996704 -0.3154296875
5.31346654891968 -0.3154296875
5.31391763687134 -0.3154296875
5.31417083740234 -0.3154296875
5.3145432472229 -0.3154296875
5.31454753875732 -0.3154296875
5.31509685516357 -0.3154296875
5.31584024429321 -0.31549072265625
5.31640672683716 -0.31549072265625
5.31662225723267 -0.31549072265625
5.31678771972656 -0.31549072265625
5.31754112243652 -0.31549072265625
5.31784009933472 -0.31549072265625
5.31786918640137 -0.31549072265625
5.3179087638855 -0.31549072265625
5.32152366638184 -0.31610107421875
5.32165002822876 -0.31610107421875
5.32176828384399 -0.31610107421875
5.32360696792603 -0.316162109375
5.32464027404785 -0.316162109375
5.32491207122803 -0.316162109375
5.32521820068359 -0.31622314453125
5.32564067840576 -0.31622314453125
5.32628870010376 -0.31622314453125
5.32681274414062 -0.31622314453125
5.32723617553711 -0.31622314453125
5.32731008529663 -0.3162841796875
5.32755327224731 -0.3162841796875
5.32794094085693 -0.3162841796875
5.32809019088745 -0.3162841796875
5.32836723327637 -0.3162841796875
5.32837152481079 -0.3162841796875
5.32849979400635 -0.3162841796875
5.3292088508606 -0.3162841796875
5.32947731018066 -0.3162841796875
5.32958316802979 -0.3162841796875
5.33032655715942 -0.3162841796875
5.33037137985229 -0.3162841796875
5.33069562911987 -0.3162841796875
5.33112144470215 -0.31634521484375
5.33112573623657 -0.31634521484375
5.33177137374878 -0.31634521484375
5.33177518844604 -0.31634521484375
5.33287858963013 -0.31640625
5.33341121673584 -0.31640625
5.33386421203613 -0.31640625
5.33411979675293 -0.31640625
5.33446979522705 -0.31640625
5.33475923538208 -0.31640625
5.33541774749756 -0.31640625
5.33583688735962 -0.31640625
5.33659601211548 -0.31646728515625
5.33692789077759 -0.31646728515625
5.33901977539062 -0.31658935546875
5.33967781066895 -0.31658935546875
5.33981513977051 -0.31658935546875
5.33991432189941 -0.31658935546875
5.34074926376343 -0.316650390625
5.3412938117981 -0.316650390625
5.34192276000977 -0.316650390625
5.34233570098877 -0.316650390625
5.34282541275024 -0.316650390625
5.34314632415771 -0.316650390625
5.34348726272583 -0.31671142578125
5.34430980682373 -0.31671142578125
5.34442758560181 -0.31671142578125
5.34454536437988 -0.31671142578125
5.34459638595581 -0.31671142578125
5.34525585174561 -0.31671142578125
5.34540128707886 -0.31671142578125
5.34598684310913 -0.31671142578125
5.34643316268921 -0.31671142578125
5.34644889831543 -0.31671142578125
5.34659337997437 -0.31671142578125
5.34662675857544 -0.31671142578125
5.34716415405273 -0.3167724609375
5.34728145599365 -0.3167724609375
5.34731245040894 -0.3167724609375
5.34773206710815 -0.3167724609375
5.34791326522827 -0.3167724609375
5.348228931427 -0.3167724609375
5.34845066070557 -0.3167724609375
5.34892749786377 -0.3167724609375
5.34925413131714 -0.3167724609375
5.34947776794434 -0.3167724609375
5.34974765777588 -0.3167724609375
5.35009860992432 -0.31683349609375
5.35039710998535 -0.31683349609375
5.35058116912842 -0.31683349609375
5.35184097290039 -0.31689453125
5.35198545455933 -0.31689453125
5.35204744338989 -0.31689453125
5.35208034515381 -0.31689453125
5.35210704803467 -0.31689453125
5.35211086273193 -0.31689453125
5.35503768920898 -0.317138671875
5.35526752471924 -0.317138671875
5.35549354553223 -0.317138671875
5.35550689697266 -0.317138671875
5.35579633712769 -0.317138671875
5.35599136352539 -0.317138671875
5.3561635017395 -0.317138671875
5.35644292831421 -0.317138671875
5.35654020309448 -0.317138671875
5.35663938522339 -0.317138671875
5.35672950744629 -0.317138671875
5.35734605789185 -0.31719970703125
5.35754585266113 -0.31719970703125
5.35869789123535 -0.31719970703125
5.35890913009644 -0.31719970703125
5.35920143127441 -0.31719970703125
5.35922241210938 -0.31719970703125
5.3597993850708 -0.3172607421875
5.35987520217896 -0.3172607421875
5.36121034622192 -0.3172607421875
5.36148977279663 -0.3172607421875
5.3615255355835 -0.3172607421875
5.36162185668945 -0.3172607421875
5.36180877685547 -0.3172607421875
5.36218452453613 -0.3172607421875
5.36278200149536 -0.3172607421875
5.3628101348877 -0.3172607421875
5.36302709579468 -0.3172607421875
5.36433506011963 -0.31732177734375
5.36458492279053 -0.31732177734375
5.36474227905273 -0.31732177734375
5.36520910263062 -0.31732177734375
5.36563396453857 -0.3173828125
5.36583995819092 -0.3173828125
5.36680936813354 -0.3173828125
5.36690092086792 -0.3173828125
5.36774730682373 -0.3173828125
5.36811590194702 -0.3173828125
5.36821985244751 -0.3173828125
5.36833524703979 -0.3173828125
5.36852693557739 -0.3173828125
5.36859941482544 -0.3173828125
5.36963319778442 -0.3173828125
5.36974239349365 -0.3173828125
5.36992788314819 -0.3173828125
5.36999273300171 -0.3173828125
5.37028169631958 -0.31744384765625
5.37050771713257 -0.31744384765625
5.3706111907959 -0.31744384765625
5.37079429626465 -0.31744384765625
5.37113809585571 -0.31744384765625
5.37139654159546 -0.31744384765625
5.37194299697876 -0.31744384765625
5.37211990356445 -0.31744384765625
5.37241649627686 -0.31744384765625
5.37273550033569 -0.31744384765625
5.37304449081421 -0.31744384765625
5.37332582473755 -0.31744384765625
5.37377786636353 -0.31744384765625
5.3737998008728 -0.31744384765625
5.3741888999939 -0.3175048828125
5.37448453903198 -0.3175048828125
5.37469530105591 -0.3175048828125
5.37485647201538 -0.3175048828125
5.37524271011353 -0.3175048828125
5.37580442428589 -0.3175048828125
5.37599802017212 -0.3175048828125
5.37642383575439 -0.3175048828125
5.37647294998169 -0.3175048828125
5.3771915435791 -0.3175048828125
5.37743902206421 -0.31756591796875
5.37768697738647 -0.31756591796875
5.37790870666504 -0.31756591796875
5.37833976745605 -0.31756591796875
5.3788013458252 -0.31756591796875
5.37886095046997 -0.31756591796875
5.37898254394531 -0.31756591796875
5.37903356552124 -0.31756591796875
5.38137149810791 -0.31768798828125
5.38170862197876 -0.3177490234375
5.38187646865845 -0.3177490234375
5.38197183609009 -0.3177490234375
5.3822979927063 -0.31781005859375
5.38254308700562 -0.31781005859375
5.38317441940308 -0.31781005859375
5.38387441635132 -0.31781005859375
5.38399314880371 -0.31781005859375
5.38454532623291 -0.31781005859375
5.38457727432251 -0.31781005859375
5.38465785980225 -0.31781005859375
5.38572406768799 -0.31787109375
5.3859691619873 -0.31787109375
5.38610982894897 -0.31787109375
5.38656663894653 -0.31787109375
5.38667917251587 -0.31787109375
5.38727235794067 -0.31793212890625
5.38738441467285 -0.31793212890625
5.38768672943115 -0.31793212890625
5.38814401626587 -0.31793212890625
5.38843154907227 -0.31793212890625
5.3890438079834 -0.31793212890625
5.38937711715698 -0.31793212890625
5.38993453979492 -0.31793212890625
5.39037704467773 -0.3179931640625
5.39072132110596 -0.3179931640625
5.39104795455933 -0.3179931640625
5.39126873016357 -0.3179931640625
5.39164447784424 -0.3179931640625
5.39207077026367 -0.3179931640625
5.39228200912476 -0.3179931640625
5.39290618896484 -0.31805419921875
5.39314699172974 -0.31805419921875
5.39367532730103 -0.318115234375
5.39416790008545 -0.318115234375
5.39437103271484 -0.318115234375
5.39462661743164 -0.318115234375
5.39489793777466 -0.318115234375
5.39510631561279 -0.31817626953125
5.39596557617188 -0.31817626953125
5.39607191085815 -0.31817626953125
5.39647483825684 -0.31817626953125
5.3967137336731 -0.3182373046875
5.39691543579102 -0.3182373046875
5.39722871780396 -0.3182373046875
5.39766883850098 -0.3182373046875
5.39790344238281 -0.3182373046875
5.39811372756958 -0.3182373046875
5.39870548248291 -0.3182373046875
5.39887380599976 -0.3182373046875
5.39924621582031 -0.3182373046875
5.3994574546814 -0.31829833984375
5.39990043640137 -0.31829833984375
5.40013694763184 -0.31829833984375
5.40055704116821 -0.31829833984375
5.4008264541626 -0.318359375
5.40102481842041 -0.318359375
5.40142965316772 -0.318359375
5.40167427062988 -0.318359375
5.40223741531372 -0.318359375
5.40262603759766 -0.318359375
5.40291786193848 -0.31842041015625
5.40320301055908 -0.31842041015625
5.40371227264404 -0.31842041015625
5.4039044380188 -0.31842041015625
5.40408420562744 -0.31842041015625
5.40437030792236 -0.31842041015625
5.40461492538452 -0.3184814453125
5.40485763549805 -0.3184814453125
5.40536880493164 -0.3184814453125
5.40611267089844 -0.31854248046875
5.40653848648071 -0.31854248046875
5.40683650970459 -0.31854248046875
5.40710878372192 -0.318603515625
5.4073314666748 -0.318603515625
5.40783071517944 -0.318603515625
5.40800094604492 -0.31866455078125
5.40823841094971 -0.31866455078125
5.40849113464355 -0.31866455078125
5.40884494781494 -0.31866455078125
5.40919923782349 -0.31866455078125
5.40951728820801 -0.31866455078125
5.40994501113892 -0.3187255859375
5.41027116775513 -0.3187255859375
5.41037225723267 -0.3187255859375
5.41052436828613 -0.3187255859375
5.41160297393799 -0.31890869140625
5.4117579460144 -0.3189697265625
5.41209936141968 -0.3189697265625
5.41231441497803 -0.3189697265625
5.41271734237671 -0.31903076171875
5.41316032409668 -0.31903076171875
5.41333818435669 -0.31903076171875
5.41354274749756 -0.31903076171875
5.41393804550171 -0.31903076171875
5.41407060623169 -0.31903076171875
5.4142427444458 -0.31903076171875
5.41469430923462 -0.31903076171875
5.41487312316895 -0.319091796875
5.41488981246948 -0.319091796875
5.41506671905518 -0.319091796875
5.41603088378906 -0.31915283203125
5.41626453399658 -0.31915283203125
5.416344165802 -0.31915283203125
5.41678380966187 -0.3192138671875
5.41689014434814 -0.3192138671875
5.41690683364868 -0.3192138671875
5.41704654693604 -0.3192138671875
5.41732740402222 -0.3192138671875
5.41760301589966 -0.3192138671875
5.417893409729 -0.3192138671875
5.41798639297485 -0.3192138671875
5.41878843307495 -0.31927490234375
5.41920375823975 -0.3193359375
5.4194483757019 -0.3193359375
5.41951274871826 -0.3193359375
5.42090082168579 -0.31951904296875
5.4214129447937 -0.319580078125
5.42179489135742 -0.319580078125
5.42192935943604 -0.319580078125
5.42208051681519 -0.31964111328125
5.42219066619873 -0.31964111328125
5.4223370552063 -0.31964111328125
5.42236185073853 -0.31964111328125
5.42258310317993 -0.31964111328125
5.42263078689575 -0.31964111328125
5.42292785644531 -0.31964111328125
5.42310476303101 -0.31964111328125
5.42359828948975 -0.31964111328125
5.42374563217163 -0.31964111328125
5.42393016815186 -0.31964111328125
5.42428350448608 -0.3197021484375
5.42458772659302 -0.3197021484375
5.42522430419922 -0.3197021484375
5.42542505264282 -0.31976318359375
5.42576885223389 -0.31976318359375
5.42590427398682 -0.31976318359375
5.426194190979 -0.31976318359375
5.42640733718872 -0.31976318359375
5.4266152381897 -0.31976318359375
5.42695999145508 -0.31976318359375
5.42705917358398 -0.31976318359375
5.4274697303772 -0.31976318359375
5.42772626876831 -0.31976318359375
5.42773771286011 -0.31976318359375
5.4278883934021 -0.31982421875
5.4278998374939 -0.31982421875
5.42806005477905 -0.31982421875
5.42818164825439 -0.31982421875
5.42858982086182 -0.31982421875
5.42877912521362 -0.31982421875
5.42888927459717 -0.31982421875
5.42923545837402 -0.31982421875
5.4294228553772 -0.31982421875
5.42969083786011 -0.31982421875
5.42992162704468 -0.31982421875
5.43009948730469 -0.31988525390625
5.43014097213745 -0.31988525390625
5.43031215667725 -0.31988525390625
5.43052816390991 -0.31988525390625
5.43076801300049 -0.31988525390625
5.43092918395996 -0.31988525390625
5.43095827102661 -0.31988525390625
5.43197774887085 -0.320068359375
5.43230676651001 -0.3201904296875
5.43240165710449 -0.3201904296875
5.43269014358521 -0.3201904296875
5.43276882171631 -0.3201904296875
5.43284130096436 -0.3201904296875
5.43299007415771 -0.32025146484375
5.43335199356079 -0.32025146484375
5.4336404800415 -0.32025146484375
5.4338436126709 -0.32025146484375
5.43388319015503 -0.32025146484375
5.43402099609375 -0.32025146484375
5.43439960479736 -0.32025146484375
5.43454170227051 -0.32025146484375
5.43457508087158 -0.32025146484375
5.43475723266602 -0.32025146484375
5.43489789962769 -0.32025146484375
5.43505859375 -0.32025146484375
5.43540334701538 -0.32025146484375
5.435471534729 -0.32025146484375
5.43573951721191 -0.32025146484375
5.43585395812988 -0.32025146484375
5.43622303009033 -0.3203125
5.43630266189575 -0.3203125
5.43652057647705 -0.3203125
5.43658876419067 -0.3203125
5.43670463562012 -0.3203125
5.43698263168335 -0.3203125
5.43700647354126 -0.3203125
5.43719530105591 -0.3203125
5.43726682662964 -0.3203125
5.43739366531372 -0.3203125
5.43820858001709 -0.32037353515625
5.43856430053711 -0.32037353515625
5.4386625289917 -0.32037353515625
5.43892812728882 -0.32037353515625
5.43899774551392 -0.32037353515625
5.43908452987671 -0.32037353515625
5.43921422958374 -0.32037353515625
5.4394383430481 -0.32037353515625
5.43965005874634 -0.32037353515625
5.43977308273315 -0.32037353515625
5.43998765945435 -0.32037353515625
5.44000482559204 -0.32037353515625
5.44001770019531 -0.3204345703125
5.44025564193726 -0.3204345703125
5.44030427932739 -0.3204345703125
5.44050312042236 -0.3204345703125
5.44067478179932 -0.3204345703125
5.44082546234131 -0.3204345703125
5.4408745765686 -0.3204345703125
5.44089651107788 -0.3204345703125
5.44102096557617 -0.3204345703125
5.44107913970947 -0.3204345703125
5.44125366210938 -0.3204345703125
5.44133520126343 -0.3204345703125
5.44142198562622 -0.3204345703125
5.44154453277588 -0.3204345703125
5.44170618057251 -0.3204345703125
5.44192743301392 -0.3204345703125
5.44199800491333 -0.3204345703125
5.44202470779419 -0.3204345703125
5.44209098815918 -0.3204345703125
5.44221639633179 -0.3204345703125
5.44292640686035 -0.32049560546875
5.44305324554443 -0.32049560546875
5.44339466094971 -0.32049560546875
5.44349765777588 -0.32049560546875
5.44357919692993 -0.32049560546875
5.4436821937561 -0.32049560546875
5.44385433197021 -0.320556640625
5.44406652450562 -0.320556640625
5.44407939910889 -0.320556640625
5.44413232803345 -0.320556640625
5.44427108764648 -0.320556640625
5.44457578659058 -0.320556640625
5.44463014602661 -0.320556640625
5.44475793838501 -0.320556640625
5.4450421333313 -0.320556640625
5.44509315490723 -0.320556640625
5.44569301605225 -0.32061767578125
5.44571781158447 -0.32061767578125
5.4460072517395 -0.32061767578125
5.44610357284546 -0.32061767578125
5.44610691070557 -0.32061767578125
5.44616556167603 -0.32061767578125
5.44678401947021 -0.3206787109375
5.44690847396851 -0.3206787109375
5.44766330718994 -0.3206787109375
5.44778251647949 -0.3206787109375
5.44779968261719 -0.3206787109375
5.44794511795044 -0.3206787109375
5.44809532165527 -0.3206787109375
5.44841241836548 -0.3206787109375
5.44860410690308 -0.3206787109375
5.44861364364624 -0.3206787109375
5.4487419128418 -0.32073974609375
5.44887018203735 -0.32073974609375
5.44891977310181 -0.32073974609375
5.44906949996948 -0.32073974609375
5.44913864135742 -0.32073974609375
5.44920539855957 -0.32073974609375
5.44934415817261 -0.32073974609375
5.44940280914307 -0.32073974609375
5.44952630996704 -0.32073974609375
5.44963884353638 -0.32073974609375
5.4496603012085 -0.32073974609375
5.44976234436035 -0.32073974609375
5.44983291625977 -0.32073974609375
5.45017194747925 -0.32073974609375
5.45018911361694 -0.32073974609375
5.45025539398193 -0.32073974609375
5.45025825500488 -0.32073974609375
5.45031547546387 -0.32073974609375
5.45044469833374 -0.32073974609375
5.45062637329102 -0.32073974609375
5.45083379745483 -0.32073974609375
5.45084762573242 -0.32073974609375
5.45092010498047 -0.32073974609375
5.45098638534546 -0.32073974609375
5.4510383605957 -0.32073974609375
5.45111083984375 -0.32073974609375
5.45115518569946 -0.32073974609375
5.45118761062622 -0.32073974609375
5.45142269134521 -0.32073974609375
5.45147943496704 -0.32073974609375
5.45157766342163 -0.32073974609375
5.45173406600952 -0.32073974609375
5.45177412033081 -0.32073974609375
5.45204591751099 -0.32073974609375
5.45211315155029 -0.32073974609375
5.4521164894104 -0.32073974609375
5.45230960845947 -0.32080078125
5.45232343673706 -0.32080078125
5.45236015319824 -0.32080078125
5.45245361328125 -0.32080078125
5.45277070999146 -0.32080078125
5.45279359817505 -0.32080078125
5.45295095443726 -0.32080078125
5.45331048965454 -0.32080078125
5.45331811904907 -0.32080078125
5.45351076126099 -0.32080078125
5.45351409912109 -0.32080078125
5.45372486114502 -0.32080078125
5.45372819900513 -0.32080078125
5.45482063293457 -0.3209228515625
5.45484352111816 -0.3209228515625
5.45485687255859 -0.3209228515625
5.45487976074219 -0.32098388671875
5.45515394210815 -0.32098388671875
5.45521354675293 -0.32098388671875
5.45537805557251 -0.32098388671875
5.45559072494507 -0.32098388671875
5.45559406280518 -0.32098388671875
5.45578384399414 -0.32098388671875
5.45582342147827 -0.32098388671875
5.45596790313721 -0.32098388671875
5.45602130889893 -0.32098388671875
5.45606374740601 -0.32098388671875
5.45609426498413 -0.32098388671875
5.45621395111084 -0.32098388671875
5.45623540878296 -0.32098388671875
};
\addplot [ultra thick, blue]
table {%
-inf 0
-inf 0
-inf 0
-inf 0
-inf -6.103515625e-05
-inf -6.103515625e-05
-inf -6.103515625e-05
-inf -6.103515625e-05
-inf -6.103515625e-05
-inf -0.0001220703125
0 -0.00018310546875
0.698970019817352 -0.00042724609375
0.698970019817352 -0.0009765625
0.698970019817352 -0.0009765625
0.698970019817352 -0.0009765625
0.778151273727417 -0.00103759765625
0.84509801864624 -0.00115966796875
0.84509801864624 -0.00115966796875
0.84509801864624 -0.00128173828125
0.903090000152588 -0.00128173828125
0.903090000152588 -0.00128173828125
1.04139268398285 -0.0015869140625
1.07918119430542 -0.00164794921875
1.07918119430542 -0.001708984375
1.17609131336212 -0.00189208984375
1.20412003993988 -0.0020751953125
1.23044896125793 -0.00213623046875
1.25527250766754 -0.002197265625
1.3979400396347 -0.00390625
1.56820178031921 -0.00494384765625
1.59106457233429 -0.00531005859375
1.6334685087204 -0.005615234375
1.67209792137146 -0.00592041015625
1.72427582740784 -0.0068359375
1.76342797279358 -0.00738525390625
1.79239177703857 -0.0078125
1.80618000030518 -0.00811767578125
1.88649070262909 -0.00885009765625
1.92427933216095 -0.0101318359375
1.9344984292984 -0.01055908203125
2.03342366218567 -0.01361083984375
2.06069779396057 -0.01495361328125
2.08990502357483 -0.01629638671875
2.12057399749756 -0.0172119140625
2.22530937194824 -0.0274658203125
2.25042009353638 -0.03204345703125
2.27415776252747 -0.0335693359375
2.290034532547 -0.03472900390625
2.37106800079346 -0.041259765625
2.3838152885437 -0.04541015625
2.38916611671448 -0.04608154296875
2.39794015884399 -0.04815673828125
2.42160391807556 -0.049560546875
2.42813467979431 -0.0501708984375
2.45024919509888 -0.05145263671875
2.45484495162964 -0.05181884765625
2.4828736782074 -0.0545654296875
2.5078558921814 -0.05584716796875
2.51982808113098 -0.056884765625
2.52762985229492 -0.05743408203125
2.5365583896637 -0.0579833984375
2.54777479171753 -0.05859375
2.57863926887512 -0.06231689453125
2.5854606628418 -0.063232421875
2.64246463775635 -0.0711669921875
2.65705585479736 -0.074951171875
2.66931676864624 -0.07672119140625
2.68394708633423 -0.07916259765625
2.71349048614502 -0.0814208984375
2.74585509300232 -0.0882568359375
2.75739598274231 -0.09259033203125
2.78103685379028 -0.09564208984375
2.81690382957458 -0.10040283203125
2.82994675636292 -0.10638427734375
2.87040400505066 -0.1217041015625
2.88592624664307 -0.12811279296875
2.89486956596375 -0.13128662109375
2.91169023513794 -0.135498046875
2.93550729751587 -0.13702392578125
2.94938993453979 -0.14404296875
2.95327639579773 -0.14532470703125
2.9666109085083 -0.14739990234375
2.97312784194946 -0.14825439453125
2.98317503929138 -0.14886474609375
2.99563527107239 -0.15130615234375
3.00086784362793 -0.15216064453125
3.0081741809845 -0.15277099609375
3.01494026184082 -0.1539306640625
3.02201581001282 -0.15496826171875
3.02857136726379 -0.15545654296875
3.03582978248596 -0.15625
3.0461049079895 -0.1575927734375
3.05153846740723 -0.158203125
3.05766606330872 -0.1591796875
3.06707096099854 -0.16033935546875
3.07151389122009 -0.16094970703125
3.0849335193634 -0.17071533203125
3.09551811218262 -0.17431640625
3.10311937332153 -0.176513671875
3.10822677612305 -0.1773681640625
3.11394333839417 -0.1793212890625
3.12221598625183 -0.18145751953125
3.12872219085693 -0.182373046875
3.14332723617554 -0.1873779296875
3.14550709724426 -0.19012451171875
3.15228843688965 -0.1910400390625
3.15472817420959 -0.19183349609375
3.15745687484741 -0.1925048828125
3.16613388061523 -0.1947021484375
3.16849756240845 -0.1951904296875
3.16996812820435 -0.19549560546875
3.17840123176575 -0.19989013671875
3.183269739151 -0.20159912109375
3.18497514724731 -0.20208740234375
3.1863911151886 -0.20245361328125
3.19061183929443 -0.2032470703125
3.20167016983032 -0.2115478515625
3.20763444900513 -0.212890625
3.20897841453552 -0.213134765625
3.21774697303772 -0.2144775390625
3.22089219093323 -0.21478271484375
3.23502326011658 -0.218505859375
3.23904895782471 -0.2193603515625
3.24229288101196 -0.21990966796875
3.24699068069458 -0.22064208984375
3.24821853637695 -0.22100830078125
3.25163817405701 -0.2213134765625
3.25671768188477 -0.22235107421875
3.25887656211853 -0.22271728515625
3.26221370697021 -0.22308349609375
3.26576089859009 -0.223876953125
3.26997971534729 -0.2244873046875
3.27253770828247 -0.22491455078125
3.27415776252747 -0.2252197265625
3.27577185630798 -0.22552490234375
3.27898216247559 -0.22613525390625
3.28126072883606 -0.22637939453125
3.2886962890625 -0.228515625
3.29225611686707 -0.2288818359375
3.29424571990967 -0.22930908203125
3.301029920578 -0.2308349609375
3.30556631088257 -0.23199462890625
3.30749607086182 -0.23236083984375
3.31196570396423 -0.233642578125
3.31491994857788 -0.234130859375
3.31722736358643 -0.23486328125
3.31973052024841 -0.23529052734375
3.32428240776062 -0.23583984375
3.32592606544495 -0.236328125
3.32695007324219 -0.23675537109375
3.32858347892761 -0.23699951171875
3.33324575424194 -0.23779296875
3.33625960350037 -0.2392578125
3.34064245223999 -0.2403564453125
3.3418300151825 -0.2408447265625
3.34262013435364 -0.24102783203125
3.34596157073975 -0.24151611328125
3.34693956375122 -0.2418212890625
3.35256838798523 -0.243408203125
3.35410833358765 -0.24395751953125
3.35679054260254 -0.24444580078125
3.35812520980835 -0.244873046875
3.36323571205139 -0.2470703125
3.36548805236816 -0.24755859375
3.36810088157654 -0.247802734375
3.369215965271 -0.24798583984375
3.37162184715271 -0.24810791015625
3.3752977848053 -0.24908447265625
3.37675929069519 -0.249267578125
3.38165640830994 -0.250244140625
3.38399481773376 -0.25079345703125
3.38863396644592 -0.25238037109375
3.39040517807007 -0.25262451171875
3.3935751914978 -0.253662109375
3.39515161514282 -0.25390625
3.39672231674194 -0.25396728515625
3.40329217910767 -0.2554931640625
3.40414929389954 -0.25579833984375
3.40619945526123 -0.2562255859375
3.40807032585144 -0.25653076171875
3.40959501266479 -0.2568359375
3.41128301620483 -0.257080078125
3.41195631027222 -0.25726318359375
3.41463923454285 -0.25738525390625
3.41580772399902 -0.257568359375
3.42193269729614 -0.25897216796875
3.42275404930115 -0.25982666015625
3.43152451515198 -0.262939453125
3.43216729164124 -0.26324462890625
3.43456888198853 -0.263427734375
3.44106650352478 -0.26397705078125
3.44138097763062 -0.26416015625
3.44200921058655 -0.26422119140625
3.44263648986816 -0.2642822265625
3.44947838783264 -0.26690673828125
3.45009517669678 -0.26715087890625
3.45086479187012 -0.2672119140625
3.45392966270447 -0.26739501953125
3.45423483848572 -0.2674560546875
3.45727610588074 -0.26751708984375
3.45757913589478 -0.267578125
3.46074748039246 -0.26776123046875
3.46149849891663 -0.267822265625
3.46164846420288 -0.26788330078125
3.46359443664551 -0.26800537109375
3.46359443664551 -0.26806640625
3.46389293670654 -0.26812744140625
3.46523404121399 -0.2681884765625
3.47712135314941 -0.27130126953125
3.47769999504089 -0.271728515625
3.47784447669983 -0.271728515625
3.48187232017517 -0.27178955078125
3.48330187797546 -0.27197265625
3.48756265640259 -0.27227783203125
3.48812747001648 -0.2723388671875
3.48869180679321 -0.2724609375
3.4893958568573 -0.2724609375
3.49066066741943 -0.27252197265625
3.49094128608704 -0.2725830078125
3.4952666759491 -0.27301025390625
3.49803471565247 -0.27313232421875
3.50105929374695 -0.273193359375
3.50201725959778 -0.2733154296875
3.50515007972717 -0.27337646484375
3.50542140007019 -0.2734375
3.50650501251221 -0.27349853515625
3.50650501251221 -0.2735595703125
3.50772094726562 -0.27362060546875
3.50772094726562 -0.273681640625
3.5171959400177 -0.27923583984375
3.52192234992981 -0.28094482421875
3.52322602272034 -0.28106689453125
3.52517437934875 -0.28131103515625
3.53364491462708 -0.28326416015625
3.53491401672363 -0.284423828125
3.53681087493896 -0.28460693359375
3.54007911682129 -0.2847900390625
3.54381990432739 -0.2855224609375
3.54703593254089 -0.28570556640625
3.54802060127258 -0.28582763671875
3.54838943481445 -0.2860107421875
3.54900336265564 -0.28619384765625
3.55557799339294 -0.2894287109375
3.55642318725586 -0.28985595703125
3.55906820297241 -0.29022216796875
3.5597870349884 -0.29034423828125
3.56276845932007 -0.29046630859375
3.56336236000061 -0.29058837890625
3.56572985649109 -0.29095458984375
3.57019257545471 -0.29144287109375
3.57054281234741 -0.29156494140625
3.57100963592529 -0.29168701171875
3.57275533676147 -0.2919921875
3.57588028907776 -0.29266357421875
3.57760667800903 -0.293212890625
3.57921171188354 -0.29327392578125
3.58376550674438 -0.2945556640625
3.58557343482971 -0.2947998046875
3.58703708648682 -0.29486083984375
3.5945029258728 -0.29718017578125
3.59494471549988 -0.29779052734375
3.59516549110413 -0.2978515625
3.59527564048767 -0.2978515625
3.59615707397461 -0.29791259765625
3.59615707397461 -0.2979736328125
3.59725618362427 -0.29803466796875
3.59835267066956 -0.298095703125
3.59846210479736 -0.29815673828125
3.59868121147156 -0.29815673828125
3.59889984130859 -0.2982177734375
3.59889984130859 -0.2982177734375
3.59922790527344 -0.2982177734375
3.60064625740051 -0.29840087890625
3.6011905670166 -0.2984619140625
3.6011905670166 -0.2984619140625
3.6011905670166 -0.2984619140625
3.6011905670166 -0.29852294921875
3.60702586174011 -0.29937744140625
3.6072404384613 -0.2996826171875
3.6073477268219 -0.29974365234375
3.6073477268219 -0.29974365234375
3.61204171180725 -0.30010986328125
3.61214780807495 -0.3001708984375
3.6133131980896 -0.30023193359375
3.61341905593872 -0.30029296875
3.61415863037109 -0.30035400390625
3.61700034141541 -0.30035400390625
3.61762928962708 -0.3004150390625
3.61825728416443 -0.3004150390625
3.61825728416443 -0.30047607421875
3.61888456344604 -0.30047607421875
3.61888456344604 -0.300537109375
3.61951065063477 -0.300537109375
3.62200665473938 -0.30084228515625
3.62324929237366 -0.30084228515625
3.62376594543457 -0.3009033203125
3.62376594543457 -0.30096435546875
3.62448835372925 -0.30096435546875
3.62623763084412 -0.30096435546875
3.62623763084412 -0.301025390625
3.62971544265747 -0.30133056640625
3.63012266159058 -0.30133056640625
3.63296318054199 -0.30157470703125
3.63346838951111 -0.3016357421875
3.63808965682983 -0.302001953125
3.63848924636841 -0.30206298828125
3.64058089256287 -0.3021240234375
3.64952945709229 -0.30377197265625
3.64972424507141 -0.30401611328125
3.6502103805542 -0.3040771484375
3.65030741691589 -0.3040771484375
3.65127801895142 -0.30413818359375
3.65446543693542 -0.30426025390625
3.65494632720947 -0.30426025390625
3.65504240989685 -0.3043212890625
3.65552258491516 -0.3043212890625
3.65925049781799 -0.30450439453125
3.65934562683105 -0.30450439453125
3.66020131111145 -0.3045654296875
3.66020131111145 -0.3045654296875
3.66275787353516 -0.30474853515625
3.66388940811157 -0.30474853515625
3.66511178016663 -0.3048095703125
3.66595602035522 -0.3048095703125
3.66698575019836 -0.30487060546875
3.66801309585571 -0.30487060546875
3.66903781890869 -0.30499267578125
3.67043137550354 -0.30499267578125
3.6714506149292 -0.3050537109375
3.67154312133789 -0.3050537109375
3.67320537567139 -0.30517578125
3.6741259098053 -0.30517578125
3.67623615264893 -0.30523681640625
3.67687654495239 -0.3052978515625
3.678062915802 -0.3052978515625
3.67879152297974 -0.30535888671875
3.67960953712463 -0.305419921875
3.68060731887817 -0.30548095703125
3.6820547580719 -0.3055419921875
3.68385720252991 -0.3056640625
3.68439650535583 -0.30572509765625
3.68833088874817 -0.30657958984375
3.69010734558105 -0.30694580078125
3.69196510314941 -0.30712890625
3.69319915771484 -0.30718994140625
3.69504356384277 -0.30731201171875
3.69670581817627 -0.3074951171875
3.7005307674408 -0.3079833984375
3.70087671279907 -0.3084716796875
3.70148158073425 -0.30865478515625
3.70174074172974 -0.3087158203125
3.70612001419067 -0.309814453125
3.70654702186584 -0.30999755859375
3.70688843727112 -0.31011962890625
3.7085907459259 -0.31024169921875
3.70901536941528 -0.310302734375
3.70952439308167 -0.3104248046875
3.70977854728699 -0.3104248046875
3.71028661727905 -0.31085205078125
3.71197581291199 -0.3109130859375
3.71222877502441 -0.31097412109375
3.71264982223511 -0.31109619140625
3.71264982223511 -0.3111572265625
3.71281790733337 -0.3111572265625
3.71307039260864 -0.31121826171875
3.71365857124329 -0.3114013671875
3.71491622924805 -0.31158447265625
3.71499991416931 -0.3116455078125
3.71533465385437 -0.31182861328125
3.71541833877563 -0.31182861328125
3.7155020236969 -0.31182861328125
3.71675443649292 -0.31182861328125
3.71675443649292 -0.3118896484375
3.71692109107971 -0.3118896484375
3.7170877456665 -0.31195068359375
3.7170877456665 -0.31195068359375
3.7173376083374 -0.31201171875
3.71750402450562 -0.31207275390625
3.71750402450562 -0.31207275390625
3.71800327301025 -0.3121337890625
3.71808624267578 -0.3121337890625
3.71808624267578 -0.3121337890625
3.71808624267578 -0.3121337890625
3.71808624267578 -0.31219482421875
3.71808624267578 -0.31219482421875
3.71908259391785 -0.312255859375
3.71908259391785 -0.312255859375
3.72015929222107 -0.31231689453125
3.72024202346802 -0.31231689453125
3.72024202346802 -0.31231689453125
3.72032475471497 -0.31231689453125
3.72040748596191 -0.31231689453125
3.72040748596191 -0.3123779296875
3.7208206653595 -0.3123779296875
3.72090315818787 -0.31243896484375
3.72098565101624 -0.31243896484375
3.72197532653809 -0.31243896484375
3.72205781936646 -0.31243896484375
3.72214007377625 -0.31243896484375
3.72222256660461 -0.3125
3.7223048210144 -0.3125
3.7223048210144 -0.3125
3.72238707542419 -0.3125
3.72246932983398 -0.3125
3.72246932983398 -0.3125
3.72361993789673 -0.31256103515625
3.72370195388794 -0.31256103515625
3.72378396987915 -0.3126220703125
3.72386598587036 -0.3126220703125
3.72386598587036 -0.3126220703125
3.72386598587036 -0.3126220703125
3.72386598587036 -0.3126220703125
3.72386598587036 -0.3126220703125
3.72542142868042 -0.31268310546875
3.72599315643311 -0.312744140625
3.72599315643311 -0.312744140625
3.72640109062195 -0.31280517578125
3.72656416893005 -0.31280517578125
3.72656416893005 -0.31280517578125
3.72664570808411 -0.31280517578125
3.72664570808411 -0.31280517578125
3.72664570808411 -0.31280517578125
3.72664570808411 -0.31280517578125
3.72664570808411 -0.31280517578125
3.72664570808411 -0.31280517578125
3.72754120826721 -0.3128662109375
3.72762250900269 -0.3128662109375
3.72770380973816 -0.3128662109375
3.72770380973816 -0.3128662109375
3.72770380973816 -0.3128662109375
3.72851610183716 -0.31292724609375
3.72875952720642 -0.31292724609375
3.72875952720642 -0.31292724609375
3.72875952720642 -0.31292724609375
3.72875952720642 -0.31292724609375
3.72875952720642 -0.31298828125
3.729407787323 -0.31298828125
3.729407787323 -0.31298828125
3.729407787323 -0.31298828125
3.73045921325684 -0.31304931640625
3.73045921325684 -0.3131103515625
3.73062086105347 -0.3131103515625
3.73110508918762 -0.3131103515625
3.73110508918762 -0.3131103515625
3.73110508918762 -0.3131103515625
3.73110508918762 -0.3131103515625
3.73110508918762 -0.31317138671875
3.73126626014709 -0.31317138671875
3.73126626014709 -0.31317138671875
3.73126626014709 -0.31317138671875
3.73126626014709 -0.313232421875
3.73126626014709 -0.313232421875
3.73271536827087 -0.313232421875
3.73271536827087 -0.313232421875
3.73287606239319 -0.31329345703125
3.73319721221924 -0.31329345703125
3.73319721221924 -0.31329345703125
3.73319721221924 -0.31329345703125
3.73319721221924 -0.31329345703125
3.7332775592804 -0.3133544921875
3.7332775592804 -0.3133544921875
3.7332775592804 -0.3133544921875
3.7332775592804 -0.31341552734375
3.7332775592804 -0.31341552734375
3.73367857933044 -0.31341552734375
3.73423957824707 -0.3134765625
3.7345597743988 -0.3134765625
3.7345597743988 -0.3134765625
3.73463988304138 -0.3134765625
3.73471975326538 -0.3134765625
3.73479986190796 -0.3134765625
3.73487973213196 -0.3134765625
3.73487973213196 -0.3134765625
3.73487973213196 -0.3134765625
3.73487973213196 -0.3134765625
3.73487973213196 -0.31353759765625
3.73487973213196 -0.31353759765625
3.73551917076111 -0.31353759765625
3.73559880256653 -0.31353759765625
3.73567867279053 -0.31353759765625
3.73567867279053 -0.31353759765625
3.73567867279053 -0.31353759765625
3.73695397377014 -0.3135986328125
3.73695397377014 -0.3135986328125
3.74044156074524 -0.3140869140625
3.74052047729492 -0.31414794921875
3.74075722694397 -0.31414794921875
3.74075722694397 -0.31414794921875
3.74107265472412 -0.31414794921875
3.7411515712738 -0.31414794921875
3.74193906784058 -0.314208984375
3.74241089820862 -0.314208984375
3.74248933792114 -0.31427001953125
3.74256801605225 -0.31427001953125
3.7428822517395 -0.31427001953125
3.7428822517395 -0.31427001953125
3.74296069145203 -0.31427001953125
3.74296069145203 -0.31427001953125
3.74296069145203 -0.31427001953125
3.74296069145203 -0.31427001953125
3.74296069145203 -0.31427001953125
3.74296069145203 -0.31427001953125
3.74366641044617 -0.31427001953125
3.74366641044617 -0.31427001953125
3.74382328987122 -0.3143310546875
3.74382328987122 -0.3143310546875
3.74382328987122 -0.3143310546875
3.74390149116516 -0.3143310546875
3.7472562789917 -0.314453125
3.74733400344849 -0.314453125
3.74733400344849 -0.314453125
3.74741172790527 -0.314453125
3.74741172790527 -0.314453125
3.74756717681885 -0.314453125
3.74756717681885 -0.314453125
3.74756717681885 -0.314453125
3.74756717681885 -0.31451416015625
3.74803280830383 -0.31451416015625
3.74811053276062 -0.31451416015625
3.74818801879883 -0.31451416015625
3.74826550483704 -0.31451416015625
3.74842071533203 -0.3145751953125
3.74849820137024 -0.3145751953125
3.74857568740845 -0.3145751953125
3.74857568740845 -0.3145751953125
3.74865317344666 -0.3145751953125
3.74865317344666 -0.3145751953125
3.74911761283875 -0.3145751953125
3.74919509887695 -0.3145751953125
3.74934983253479 -0.3145751953125
3.74934983253479 -0.3145751953125
3.74942708015442 -0.3145751953125
3.74950432777405 -0.31463623046875
3.74950432777405 -0.31463623046875
3.75151014328003 -0.314697265625
3.7515869140625 -0.314697265625
3.7515869140625 -0.314697265625
3.75166392326355 -0.314697265625
3.75166392326355 -0.314697265625
3.75166392326355 -0.314697265625
3.75166392326355 -0.314697265625
3.75166392326355 -0.314697265625
3.75204849243164 -0.314697265625
3.75204849243164 -0.314697265625
3.75204849243164 -0.31475830078125
3.75212526321411 -0.31475830078125
3.75220203399658 -0.31475830078125
3.75220203399658 -0.31475830078125
3.75220203399658 -0.31475830078125
3.75227904319763 -0.31475830078125
3.7523558139801 -0.31475830078125
3.7523558139801 -0.31475830078125
3.7523558139801 -0.31475830078125
3.7528932094574 -0.31475830078125
3.7528932094574 -0.31475830078125
3.7528932094574 -0.31475830078125
3.75296974182129 -0.31475830078125
3.75388932228088 -0.3148193359375
3.75396585464478 -0.31488037109375
3.75404238700867 -0.31488037109375
3.75411891937256 -0.31488037109375
3.75419545173645 -0.31488037109375
3.75587487220764 -0.31488037109375
3.75602722167969 -0.31488037109375
3.75602722167969 -0.31488037109375
3.75602722167969 -0.31488037109375
3.75617957115173 -0.31488037109375
3.75625562667847 -0.31494140625
3.7563316822052 -0.31494140625
3.7563316822052 -0.31494140625
3.7563316822052 -0.31494140625
3.75777554512024 -0.31500244140625
3.75777554512024 -0.31500244140625
3.76222825050354 -0.3153076171875
3.76230335235596 -0.31536865234375
3.76237845420837 -0.31536865234375
3.7627534866333 -0.31536865234375
3.7627534866333 -0.31536865234375
3.76282858848572 -0.31536865234375
3.76282858848572 -0.31536865234375
3.76282858848572 -0.3154296875
3.76350283622742 -0.3154296875
3.76357769966125 -0.3154296875
3.76357769966125 -0.3154296875
3.76357769966125 -0.3154296875
3.76357769966125 -0.3154296875
3.7643256187439 -0.31549072265625
3.7643256187439 -0.31549072265625
3.76440024375916 -0.31549072265625
3.76447510719299 -0.31549072265625
3.76447510719299 -0.31549072265625
3.76447510719299 -0.31549072265625
3.76447510719299 -0.31549072265625
3.76537036895752 -0.31561279296875
3.76537036895752 -0.31561279296875
3.76760101318359 -0.31573486328125
3.7679717540741 -0.3157958984375
3.7680459022522 -0.3157958984375
3.7680459022522 -0.3157958984375
3.7680459022522 -0.31585693359375
3.7680459022522 -0.31585693359375
3.7680459022522 -0.31585693359375
3.76989412307739 -0.31585693359375
3.76989412307739 -0.31585693359375
3.76996779441833 -0.31591796875
3.77004146575928 -0.31591796875
3.7701153755188 -0.31591796875
3.77077841758728 -0.31591796875
3.77085208892822 -0.31591796875
3.77092552185059 -0.31591796875
3.77217483520508 -0.316162109375
3.77320122718811 -0.316162109375
3.77327442169189 -0.31622314453125
3.77334761619568 -0.31622314453125
3.77364015579224 -0.31622314453125
3.77364015579224 -0.31622314453125
3.77364015579224 -0.31622314453125
3.77364015579224 -0.31622314453125
3.77371335029602 -0.31622314453125
3.77677392959595 -0.31658935546875
3.77793407440186 -0.3167724609375
3.77865767478943 -0.31683349609375
3.7787299156189 -0.31683349609375
3.77887439727783 -0.31683349609375
3.77887439727783 -0.31683349609375
3.77887439727783 -0.31683349609375
3.78168368339539 -0.31689453125
3.7817554473877 -0.31689453125
3.7817554473877 -0.31689453125
3.7817554473877 -0.31689453125
3.7817554473877 -0.31689453125
3.78182721138 -0.31689453125
3.78189897537231 -0.31689453125
3.78247261047363 -0.31695556640625
3.78247261047363 -0.31695556640625
3.7845458984375 -0.3170166015625
3.7846884727478 -0.31707763671875
3.78475999832153 -0.31707763671875
3.78483128547668 -0.31707763671875
3.78490257263184 -0.31707763671875
3.78497362136841 -0.31707763671875
3.78511619567871 -0.31707763671875
3.78511619567871 -0.31707763671875
3.78518748283386 -0.31707763671875
3.78518748283386 -0.317138671875
3.78518748283386 -0.317138671875
3.78525853157043 -0.317138671875
3.78532981872559 -0.317138671875
3.78532981872559 -0.317138671875
3.78532981872559 -0.317138671875
3.78532981872559 -0.317138671875
3.7858989238739 -0.317138671875
3.7858989238739 -0.317138671875
3.7858989238739 -0.317138671875
3.7858989238739 -0.317138671875
3.7858989238739 -0.31719970703125
3.7870352268219 -0.31719970703125
3.7870352268219 -0.31719970703125
3.7870352268219 -0.31719970703125
3.7870352268219 -0.31719970703125
3.78816843032837 -0.3172607421875
3.78816843032837 -0.3172607421875
3.78816843032837 -0.3172607421875
3.78816843032837 -0.3172607421875
3.78816843032837 -0.3172607421875
3.78816843032837 -0.3172607421875
3.78823900222778 -0.3172607421875
3.78830981254578 -0.3172607421875
3.78838062286377 -0.3172607421875
3.78838062286377 -0.3172607421875
3.78838062286377 -0.3172607421875
3.78943967819214 -0.31732177734375
3.78943967819214 -0.31732177734375
3.78943967819214 -0.31732177734375
3.78943967819214 -0.31732177734375
3.78943967819214 -0.31732177734375
3.78943967819214 -0.31732177734375
3.78943967819214 -0.31732177734375
3.78943967819214 -0.31732177734375
3.79056668281555 -0.31732177734375
3.79056668281555 -0.31732177734375
3.79056668281555 -0.31732177734375
3.79337120056152 -0.3173828125
3.79337120056152 -0.3173828125
3.79406952857971 -0.31744384765625
3.79413938522339 -0.31744384765625
3.79413938522339 -0.31744384765625
3.79420900344849 -0.31744384765625
3.79427886009216 -0.31744384765625
3.79455780982971 -0.3175048828125
3.79455780982971 -0.3175048828125
3.79455780982971 -0.3175048828125
3.79462742805481 -0.3175048828125
3.79469704627991 -0.3175048828125
3.79469704627991 -0.3175048828125
3.79469704627991 -0.3175048828125
3.79581046104431 -0.3175048828125
3.79588007926941 -0.3175048828125
3.79588007926941 -0.3175048828125
3.79588007926941 -0.3175048828125
3.79601907730103 -0.3175048828125
3.79601907730103 -0.3175048828125
3.79608845710754 -0.31756591796875
3.7963662147522 -0.31756591796875
3.7963662147522 -0.31756591796875
3.79782128334045 -0.31756591796875
3.79823613166809 -0.317626953125
3.79823613166809 -0.317626953125
3.79823613166809 -0.317626953125
3.79823613166809 -0.317626953125
3.79830527305603 -0.317626953125
3.79830527305603 -0.317626953125
3.79837441444397 -0.317626953125
3.79837441444397 -0.317626953125
3.79837441444397 -0.317626953125
3.79837441444397 -0.317626953125
3.79837441444397 -0.317626953125
3.79851245880127 -0.317626953125
3.79851245880127 -0.317626953125
3.79851245880127 -0.317626953125
3.79851245880127 -0.317626953125
3.80099177360535 -0.3179931640625
3.80099177360535 -0.3179931640625
3.80195212364197 -0.3179931640625
3.80311560630798 -0.3179931640625
3.80318379402161 -0.3179931640625
3.80318379402161 -0.3179931640625
3.80338883399963 -0.3179931640625
3.80345702171326 -0.31805419921875
3.80352544784546 -0.31805419921875
3.80352544784546 -0.31805419921875
3.80434393882751 -0.31805419921875
3.80434393882751 -0.31805419921875
3.80434393882751 -0.31805419921875
3.80434393882751 -0.31805419921875
3.80441212654114 -0.31805419921875
3.80441212654114 -0.31805419921875
3.80563688278198 -0.318115234375
3.80570459365845 -0.318115234375
3.80577254295349 -0.318115234375
3.80577254295349 -0.318115234375
3.80577254295349 -0.318115234375
3.80577254295349 -0.318115234375
3.80800819396973 -0.31817626953125
3.80807590484619 -0.31817626953125
3.80861592292786 -0.3182373046875
3.80868339538574 -0.3182373046875
3.80875086784363 -0.3182373046875
3.80881834030151 -0.3182373046875
3.8088858127594 -0.3182373046875
3.80895328521729 -0.3182373046875
3.80902075767517 -0.3182373046875
3.80902075767517 -0.3182373046875
3.80902075767517 -0.3182373046875
3.80902075767517 -0.3182373046875
3.80902075767517 -0.3182373046875
3.80922293663025 -0.3182373046875
3.80922293663025 -0.3182373046875
3.80929040908813 -0.3182373046875
3.80929040908813 -0.3182373046875
3.80935764312744 -0.3182373046875
3.80942511558533 -0.3182373046875
3.80996346473694 -0.3182373046875
3.80996346473694 -0.3182373046875
3.80996346473694 -0.3182373046875
3.80996346473694 -0.3182373046875
3.80996346473694 -0.3182373046875
3.81009793281555 -0.3182373046875
3.81009793281555 -0.31829833984375
3.81009793281555 -0.31829833984375
3.81036686897278 -0.31829833984375
3.81043410301208 -0.31829833984375
3.81043410301208 -0.31829833984375
3.81043410301208 -0.31829833984375
3.81097149848938 -0.31829833984375
3.81110572814941 -0.31829833984375
3.81110572814941 -0.31829833984375
3.81110572814941 -0.31829833984375
3.81110572814941 -0.31829833984375
3.81130695343018 -0.31829833984375
3.81130695343018 -0.31829833984375
3.81144094467163 -0.31829833984375
3.81144094467163 -0.31829833984375
3.81144094467163 -0.31829833984375
3.81144094467163 -0.31829833984375
3.81170892715454 -0.318359375
3.81170892715454 -0.318359375
3.81204390525818 -0.318359375
3.81204390525818 -0.318359375
3.81204390525818 -0.318359375
3.81204390525818 -0.318359375
3.81204390525818 -0.318359375
3.81211090087891 -0.318359375
3.81211090087891 -0.318359375
3.81211090087891 -0.318359375
3.81211090087891 -0.318359375
3.81244540214539 -0.318359375
3.81251239776611 -0.318359375
3.81398105621338 -0.318359375
3.81404781341553 -0.31842041015625
3.8141143321991 -0.31842041015625
3.8141143321991 -0.31842041015625
3.81438088417053 -0.31842041015625
3.81438088417053 -0.31842041015625
3.81438088417053 -0.31842041015625
3.8153121471405 -0.3184814453125
3.8153121471405 -0.3184814453125
3.81537842750549 -0.3184814453125
3.81537842750549 -0.3184814453125
3.81537842750549 -0.3184814453125
3.81657266616821 -0.3184814453125
3.81657266616821 -0.3184814453125
3.81657266616821 -0.3184814453125
3.81670522689819 -0.31854248046875
3.81670522689819 -0.31854248046875
3.81697010993958 -0.31854248046875
3.81736707687378 -0.31854248046875
3.81736707687378 -0.31854248046875
3.817631483078 -0.31854248046875
3.817631483078 -0.31854248046875
3.817631483078 -0.31854248046875
3.81782960891724 -0.31854248046875
3.81796169281006 -0.31854248046875
3.8182258605957 -0.31854248046875
3.81829190254211 -0.318603515625
3.81829190254211 -0.318603515625
3.81829190254211 -0.318603515625
3.81829190254211 -0.318603515625
3.81862163543701 -0.318603515625
3.81868767738342 -0.318603515625
3.81875348091125 -0.318603515625
3.81881952285767 -0.318603515625
3.8188853263855 -0.318603515625
3.81974124908447 -0.318603515625
3.8198070526123 -0.318603515625
3.82046413421631 -0.31866455078125
3.82052993774414 -0.31866455078125
3.82052993774414 -0.31866455078125
3.82072687149048 -0.31866455078125
3.82092356681824 -0.31866455078125
3.82092356681824 -0.31866455078125
3.82092356681824 -0.31866455078125
3.82092356681824 -0.31866455078125
3.82105469703674 -0.31866455078125
3.82105469703674 -0.31866455078125
3.82203722000122 -0.31866455078125
3.82203722000122 -0.3187255859375
3.82269096374512 -0.3187255859375
3.82282161712646 -0.3187255859375
3.82288694381714 -0.3187255859375
3.82288694381714 -0.3187255859375
3.82288694381714 -0.3187255859375
3.82366991043091 -0.31878662109375
3.823734998703 -0.31878662109375
3.823734998703 -0.31878662109375
3.82393050193787 -0.31878662109375
3.82393050193787 -0.31878662109375
3.82419085502625 -0.31878662109375
3.82419085502625 -0.31878662109375
3.82425594329834 -0.31878662109375
3.82600998878479 -0.31884765625
3.82607483863831 -0.31884765625
3.82607483863831 -0.31884765625
3.82652831077576 -0.31890869140625
3.82659292221069 -0.31890869140625
3.8268518447876 -0.31890869140625
3.82691669464111 -0.31890869140625
3.82736921310425 -0.31890869140625
3.82743382453918 -0.31890869140625
3.82743382453918 -0.31890869140625
3.82769227027893 -0.31890869140625
3.8279504776001 -0.31890869140625
3.82801508903503 -0.3189697265625
3.82814407348633 -0.3189697265625
3.82814407348633 -0.3189697265625
3.82814407348633 -0.3189697265625
3.82814407348633 -0.3189697265625
3.82962536811829 -0.31903076171875
3.82968974113464 -0.31903076171875
3.82981824874878 -0.319091796875
3.82981824874878 -0.319091796875
3.83001089096069 -0.319091796875
3.83013939857483 -0.319091796875
3.83013939857483 -0.319091796875
3.83013939857483 -0.319091796875
3.83071684837341 -0.319091796875
3.83116555213928 -0.319091796875
3.83135771751404 -0.31915283203125
3.83142185211182 -0.31915283203125
3.83231735229492 -0.31915283203125
3.83238124847412 -0.31915283203125
3.83276438713074 -0.31915283203125
3.83282804489136 -0.31915283203125
3.83295583724976 -0.31915283203125
3.83308339118958 -0.31915283203125
3.8331470489502 -0.31915283203125
3.8331470489502 -0.31915283203125
3.8331470489502 -0.31915283203125
3.83340215682983 -0.31915283203125
3.83372068405151 -0.3192138671875
3.83372068405151 -0.3192138671875
3.83372068405151 -0.3192138671875
3.83422994613647 -0.3192138671875
3.83499264717102 -0.3192138671875
3.83505606651306 -0.3192138671875
3.83505606651306 -0.3192138671875
3.83518314361572 -0.3192138671875
3.83518314361572 -0.3192138671875
3.8353099822998 -0.3192138671875
3.8353099822998 -0.3192138671875
3.8353099822998 -0.3192138671875
3.83562707901001 -0.3192138671875
3.83569049835205 -0.31927490234375
3.83613419532776 -0.31927490234375
3.83613419532776 -0.31927490234375
3.83657717704773 -0.31927490234375
3.83664059638977 -0.31927490234375
3.83664059638977 -0.31927490234375
3.83664059638977 -0.31927490234375
3.8368935585022 -0.3193359375
3.8368935585022 -0.3193359375
3.83727264404297 -0.3193359375
3.83803009986877 -0.31939697265625
3.83859729766846 -0.31939697265625
3.83866024017334 -0.31939697265625
3.83891201019287 -0.31939697265625
3.83897495269775 -0.31939697265625
3.83910083770752 -0.31939697265625
3.83910083770752 -0.31939697265625
3.83941507339478 -0.31939697265625
3.83947801589966 -0.31939697265625
3.83954095840454 -0.31939697265625
3.83966660499573 -0.31939697265625
3.83985495567322 -0.3194580078125
3.84004330635071 -0.3194580078125
3.84010601043701 -0.3194580078125
3.84010601043701 -0.3194580078125
3.8402943611145 -0.3194580078125
3.84035706520081 -0.3194580078125
3.84079599380493 -0.3194580078125
3.84085845947266 -0.3194580078125
3.84092116355896 -0.31951904296875
3.84160971641541 -0.31951904296875
3.84179735183716 -0.31951904296875
3.84185981750488 -0.31951904296875
3.84223461151123 -0.31951904296875
3.84229707717896 -0.31951904296875
3.84235954284668 -0.31951904296875
3.8424220085144 -0.31951904296875
3.84292101860046 -0.319580078125
3.84298348426819 -0.319580078125
3.8431704044342 -0.319580078125
3.84323287010193 -0.319580078125
3.84335732460022 -0.319580078125
3.84410429000854 -0.319580078125
3.84416651725769 -0.319580078125
3.84422850608826 -0.31964111328125
3.84435296058655 -0.31964111328125
3.84460139274597 -0.31964111328125
3.84472560882568 -0.31964111328125
3.84497404098511 -0.31964111328125
3.84553217887878 -0.31964111328125
3.84584188461304 -0.31964111328125
3.84584188461304 -0.31964111328125
3.8459038734436 -0.31964111328125
3.84608960151672 -0.31964111328125
3.84621334075928 -0.31964111328125
3.84788107872009 -0.31982421875
3.8479425907135 -0.31982421875
3.8480658531189 -0.31982421875
3.84812760353088 -0.31982421875
3.8485586643219 -0.31988525390625
3.84868168830872 -0.31988525390625
3.84868168830872 -0.31988525390625
3.84880471229553 -0.31988525390625
3.84966516494751 -0.3199462890625
3.84972643852234 -0.3199462890625
3.85003328323364 -0.3199462890625
3.85009455680847 -0.3199462890625
3.85076880455017 -0.32000732421875
3.85089111328125 -0.32000732421875
3.85095238685608 -0.32000732421875
3.85101366043091 -0.32000732421875
3.85174751281738 -0.320068359375
3.85174751281738 -0.320068359375
3.85211396217346 -0.32012939453125
3.85217499732971 -0.32012939453125
3.85229706764221 -0.32012939453125
3.85247993469238 -0.32012939453125
3.85308957099915 -0.32012939453125
3.85339403152466 -0.3201904296875
3.85412383079529 -0.3201904296875
3.85418462753296 -0.3201904296875
3.85430598258972 -0.3201904296875
3.85485243797302 -0.32025146484375
3.85485243797302 -0.32025146484375
3.85570073127747 -0.32025146484375
3.85582184791565 -0.3203125
3.85594296455383 -0.3203125
3.85618495941162 -0.3203125
};
\end{axis}


\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{ClF3}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xtick={0,1,2,3,4},
xlabel={COI},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.7077633947134,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.431814575195313, ymax=0.0204986572265625,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c5)}
]
\addplot [ultra thick, brown, dashed]
table {%
1.30103003978729 -6.103515625e-05
1.53147888183594 -0.00042724609375
1.66275787353516 -0.00042724609375
1.74036264419556 -0.00048828125
1.83884906768799 -0.00048828125
1.89209461212158 -0.00048828125
1.95424246788025 -0.00048828125
2.01283717155457 -0.00048828125
2.04921793937683 -0.00048828125
2.32428240776062 -0.00048828125
2.67669367790222 -0.0006103515625
2.75127911567688 -0.00067138671875
2.76267862319946 -0.00067138671875
2.8088858127594 -0.00067138671875
2.82085800170898 -0.000732421875
2.86213135719299 -0.000732421875
2.91487169265747 -0.0008544921875
3.05037975311279 -0.0008544921875
3.09864377975464 -0.0008544921875
3.15654921531677 -0.00091552734375
3.1883659362793 -0.0009765625
3.23653721809387 -0.0009765625
3.24229288101196 -0.0009765625
3.31576037406921 -0.0010986328125
3.31827211380005 -0.0010986328125
3.33645963668823 -0.00115966796875
3.34478521347046 -0.00115966796875
3.35506820678711 -0.001220703125
3.39776635169983 -0.001220703125
3.40534639358521 -0.00128173828125
3.43949055671692 -0.00128173828125
3.44824242591858 -0.0013427734375
3.56229281425476 -0.00213623046875
3.57714700698853 -0.002685546875
3.60108184814453 -0.003173828125
3.65166568756104 -0.0032958984375
3.68708276748657 -0.00384521484375
3.69931721687317 -0.004150390625
3.72378396987915 -0.00439453125
3.74616694450378 -0.00482177734375
3.76908183097839 -0.0050048828125
3.81802773475647 -0.0123291015625
3.82425594329834 -0.01556396484375
3.85497379302979 -0.01727294921875
3.87540864944458 -0.01763916015625
3.89998459815979 -0.017822265625
3.91613793373108 -0.01824951171875
3.92474436759949 -0.0184326171875
3.93651366233826 -0.0186767578125
3.95889830589294 -0.01885986328125
3.97854566574097 -0.01922607421875
3.98569583892822 -0.01947021484375
4.00676536560059 -0.0201416015625
4.02094125747681 -0.02056884765625
4.04143238067627 -0.02093505859375
4.05549287796021 -0.021240234375
4.06792593002319 -0.02178955078125
4.07481670379639 -0.02203369140625
4.0995078086853 -0.025390625
4.11287307739258 -0.02655029296875
4.12234687805176 -0.0272216796875
4.13417720794678 -0.02789306640625
4.15329647064209 -0.03106689453125
4.16645956039429 -0.033447265625
4.17998218536377 -0.03509521484375
4.18887233734131 -0.0355224609375
4.20183372497559 -0.03717041015625
4.21066617965698 -0.0379638671875
4.21743106842041 -0.03863525390625
4.23736763000488 -0.042724609375
4.24487066268921 -0.04473876953125
4.28470134735107 -0.05731201171875
4.28692770004272 -0.06707763671875
4.30187606811523 -0.0721435546875
4.31289625167847 -0.07427978515625
4.31902265548706 -0.0755615234375
4.33831691741943 -0.076904296875
4.34855794906616 -0.078125
4.36167097091675 -0.08050537109375
4.37814331054688 -0.08233642578125
4.38451480865479 -0.083251953125
4.39281988143921 -0.0845947265625
4.41662406921387 -0.0882568359375
4.42399930953979 -0.0894775390625
4.44090890884399 -0.0909423828125
4.45379209518433 -0.09429931640625
4.46100282669067 -0.09515380859375
4.48505401611328 -0.09954833984375
4.4944052696228 -0.1004638671875
4.51546335220337 -0.10784912109375
4.52649450302124 -0.109375
4.53069925308228 -0.10980224609375
4.54010391235352 -0.11041259765625
4.5516939163208 -0.11309814453125
4.56062364578247 -0.11376953125
4.56875324249268 -0.11456298828125
4.58682346343994 -0.1185302734375
4.59299802780151 -0.11962890625
4.60439872741699 -0.12353515625
4.61168098449707 -0.1256103515625
4.62236928939819 -0.12713623046875
4.62851142883301 -0.12835693359375
4.63695907592773 -0.130859375
4.64442873001099 -0.1324462890625
4.65274906158447 -0.13409423828125
4.66067600250244 -0.1376953125
4.66729402542114 -0.13983154296875
4.67442035675049 -0.14190673828125
4.68700265884399 -0.1470947265625
4.69202709197998 -0.14886474609375
4.69791793823242 -0.151611328125
4.70952415466309 -0.1636962890625
4.71695423126221 -0.1676025390625
4.7232666015625 -0.16986083984375
4.73906564712524 -0.17901611328125
4.74263858795166 -0.1837158203125
4.75111722946167 -0.18670654296875
4.75356006622314 -0.18902587890625
4.75888156890869 -0.19134521484375
4.76575040817261 -0.20233154296875
4.7731351852417 -0.20684814453125
4.78280925750732 -0.21343994140625
4.787672996521 -0.2191162109375
4.79389524459839 -0.22125244140625
4.79599809646606 -0.22369384765625
4.80088901519775 -0.22723388671875
4.80619335174561 -0.230224609375
4.80884552001953 -0.23236083984375
4.81313371658325 -0.23480224609375
4.81687068939209 -0.23614501953125
4.82508850097656 -0.2386474609375
4.83301305770874 -0.243896484375
4.8353796005249 -0.24505615234375
4.84144067764282 -0.24591064453125
4.84736919403076 -0.24725341796875
4.85182094573975 -0.2479248046875
4.8615403175354 -0.25299072265625
4.86524629592896 -0.25347900390625
4.87182378768921 -0.256103515625
4.8750147819519 -0.25653076171875
4.88004159927368 -0.25762939453125
4.88612413406372 -0.25897216796875
4.89034271240234 -0.2596435546875
4.89783048629761 -0.2615966796875
4.90002822875977 -0.263427734375
4.90417432785034 -0.26483154296875
4.90768527984619 -0.26544189453125
4.9103684425354 -0.26605224609375
4.91701173782349 -0.26922607421875
4.92052507400513 -0.27008056640625
4.92293834686279 -0.27056884765625
4.92570924758911 -0.2711181640625
4.92858028411865 -0.2720947265625
4.93106079101562 -0.27252197265625
4.93428134918213 -0.27325439453125
4.94174003601074 -0.27703857421875
4.94543886184692 -0.27838134765625
4.94694328308105 -0.27886962890625
4.9491605758667 -0.27923583984375
4.95355176925659 -0.28021240234375
4.956130027771 -0.28076171875
4.95881700515747 -0.28118896484375
4.96168231964111 -0.28216552734375
4.96477794647217 -0.28271484375
4.96704244613647 -0.2830810546875
4.97251272201538 -0.28570556640625
4.97612047195435 -0.287109375
4.97918844223022 -0.2882080078125
4.98169612884521 -0.2886962890625
4.98436546325684 -0.2894287109375
4.9882378578186 -0.2899169921875
4.99243879318237 -0.29144287109375
4.99536752700806 -0.2923583984375
5.00342607498169 -0.298583984375
5.00505590438843 -0.29986572265625
5.00698328018188 -0.300537109375
5.00814437866211 -0.30084228515625
5.01435232162476 -0.30511474609375
5.01559019088745 -0.30584716796875
5.01734638214111 -0.30621337890625
5.02038621902466 -0.30804443359375
5.02262210845947 -0.30853271484375
5.02349138259888 -0.30877685546875
5.02797698974609 -0.3109130859375
5.03176403045654 -0.31134033203125
5.03309774398804 -0.3116455078125
5.03400230407715 -0.31195068359375
5.03523778915405 -0.31219482421875
5.03709173202515 -0.3125
5.04360580444336 -0.3155517578125
5.04664325714111 -0.31585693359375
5.04971790313721 -0.3165283203125
5.05626440048218 -0.31793212890625
5.05785608291626 -0.3182373046875
5.0608377456665 -0.31878662109375
5.06363344192505 -0.3189697265625
5.06476879119873 -0.319091796875
5.06603527069092 -0.3192138671875
5.07751703262329 -0.325927734375
5.07859802246094 -0.32696533203125
5.08004522323608 -0.3271484375
5.08140850067139 -0.32720947265625
5.08489084243774 -0.32757568359375
5.08806896209717 -0.3280029296875
5.09107208251953 -0.32818603515625
5.0922327041626 -0.32830810546875
5.09593629837036 -0.32861328125
5.09908628463745 -0.32879638671875
5.10161304473877 -0.3291015625
5.10227584838867 -0.3292236328125
5.10986185073853 -0.33074951171875
5.11206865310669 -0.33111572265625
5.11268520355225 -0.33123779296875
5.11650800704956 -0.33148193359375
5.11850929260254 -0.3321533203125
5.11945056915283 -0.332275390625
5.1285285949707 -0.34124755859375
5.13103437423706 -0.34503173828125
5.13535213470459 -0.3455810546875
5.13641309738159 -0.3458251953125
5.13862466812134 -0.3460693359375
5.14056158065796 -0.34637451171875
5.14270830154419 -0.3465576171875
5.14405107498169 -0.34674072265625
5.14582061767578 -0.347412109375
5.14770412445068 -0.34759521484375
5.14981603622437 -0.3477783203125
5.15180492401123 -0.34796142578125
5.15435409545898 -0.34814453125
5.15559720993042 -0.3485107421875
5.15640068054199 -0.3486328125
5.16010236740112 -0.3505859375
5.16256761550903 -0.35107421875
5.16420412063599 -0.3519287109375
5.16553831100464 -0.35235595703125
5.16723442077637 -0.35260009765625
5.16823530197144 -0.35302734375
5.16963911056519 -0.35333251953125
5.17115306854248 -0.353759765625
5.17267608642578 -0.35406494140625
5.18044424057007 -0.35858154296875
5.18125152587891 -0.3590087890625
5.18191766738892 -0.359130859375
5.1824803352356 -0.35919189453125
5.18332386016846 -0.35955810546875
5.18477392196655 -0.35968017578125
5.18543148040771 -0.35980224609375
5.19021940231323 -0.36029052734375
5.1907320022583 -0.3607177734375
5.19326639175415 -0.361083984375
5.19385051727295 -0.36114501953125
5.19472503662109 -0.36126708984375
5.19609069824219 -0.361328125
5.19898414611816 -0.3619384765625
5.19977426528931 -0.362060546875
5.20053291320801 -0.36212158203125
5.20270347595215 -0.3623046875
5.2029185295105 -0.3624267578125
5.20497703552246 -0.36285400390625
5.20645618438721 -0.36297607421875
5.20685005187988 -0.363037109375
5.21029186248779 -0.3643798828125
5.21122217178345 -0.365478515625
5.21184110641479 -0.36553955078125
5.21281862258911 -0.36566162109375
5.21484899520874 -0.3660888671875
5.21587800979614 -0.3668212890625
5.21651697158813 -0.366943359375
5.21903657913208 -0.36859130859375
5.21988296508789 -0.36895751953125
5.22165155410767 -0.369140625
5.22259950637817 -0.36932373046875
5.22359466552734 -0.36944580078125
5.22551870346069 -0.36993408203125
5.22633171081543 -0.37005615234375
5.22724103927612 -0.37017822265625
5.22822046279907 -0.3704833984375
5.22954607009888 -0.37078857421875
5.23019599914551 -0.370849609375
5.23104619979858 -0.3709716796875
5.23335409164429 -0.37237548828125
5.23456811904907 -0.37249755859375
5.2357759475708 -0.3729248046875
5.23672342300415 -0.373046875
5.23849010467529 -0.37335205078125
5.23972749710083 -0.37347412109375
5.24111557006836 -0.3736572265625
5.24247694015503 -0.373779296875
5.24328851699829 -0.37396240234375
5.24410152435303 -0.37408447265625
5.24543857574463 -0.37420654296875
5.25074911117554 -0.3756103515625
5.25277519226074 -0.3759765625
5.25335741043091 -0.3760986328125
5.25922822952271 -0.3778076171875
5.25956773757935 -0.3780517578125
5.26148891448975 -0.37823486328125
5.26194524765015 -0.3782958984375
5.26264810562134 -0.37841796875
5.26305818557739 -0.37847900390625
5.26347017288208 -0.3785400390625
5.26738548278809 -0.37933349609375
5.26843070983887 -0.3795166015625
5.26903867721558 -0.379638671875
5.27142095565796 -0.38018798828125
5.27253293991089 -0.38031005859375
5.27312421798706 -0.38031005859375
5.27391290664673 -0.38043212890625
5.27423858642578 -0.38043212890625
5.27622747421265 -0.38055419921875
5.27688455581665 -0.38067626953125
5.27771472930908 -0.3807373046875
5.27856159210205 -0.38079833984375
5.27962112426758 -0.380859375
5.28046703338623 -0.38092041015625
5.28099679946899 -0.3809814453125
5.28176021575928 -0.38104248046875
5.28253173828125 -0.381103515625
5.28374433517456 -0.3812255859375
5.28529405593872 -0.3814697265625
5.28596687316895 -0.38153076171875
5.28715419769287 -0.38165283203125
5.28837871551514 -0.38189697265625
5.28904247283936 -0.3819580078125
5.29102659225464 -0.3822021484375
5.29169082641602 -0.38226318359375
5.29275226593018 -0.38238525390625
5.29387950897217 -0.38250732421875
5.29481220245361 -0.3828125
5.29578018188477 -0.3829345703125
5.29658603668213 -0.38299560546875
5.29735994338989 -0.38311767578125
5.29793310165405 -0.38323974609375
5.29882669448853 -0.38330078125
5.29966640472412 -0.3834228515625
5.30090427398682 -0.38348388671875
5.30147075653076 -0.383544921875
5.30252361297607 -0.38360595703125
5.30932331085205 -0.3868408203125
5.30970668792725 -0.38775634765625
5.3115611076355 -0.387939453125
5.31210517883301 -0.38800048828125
5.31283092498779 -0.3880615234375
5.31360149383545 -0.38812255859375
5.31470537185669 -0.38818359375
5.31633949279785 -0.3885498046875
5.31829690933228 -0.388916015625
5.31855392456055 -0.38897705078125
5.31945180892944 -0.3890380859375
5.31995105743408 -0.38909912109375
5.32142877578735 -0.3892822265625
5.32214260101318 -0.38934326171875
5.32396936416626 -0.38983154296875
5.32593011856079 -0.3902587890625
5.32668209075928 -0.390380859375
5.32727289199829 -0.39044189453125
5.3279390335083 -0.3905029296875
5.3288688659668 -0.39068603515625
5.32939195632935 -0.3907470703125
5.33040142059326 -0.39208984375
5.33084201812744 -0.39227294921875
5.33124685287476 -0.39239501953125
5.33184432983398 -0.3924560546875
5.33264255523682 -0.39251708984375
5.33301591873169 -0.392578125
5.33367300033569 -0.39263916015625
5.33390665054321 -0.3927001953125
5.33420658111572 -0.39276123046875
5.33563041687012 -0.3935546875
5.33662176132202 -0.3936767578125
5.33691596984863 -0.39373779296875
5.33743715286255 -0.393798828125
5.33793640136719 -0.39385986328125
5.33858394622803 -0.39447021484375
5.33920288085938 -0.39453125
5.33979892730713 -0.39453125
5.34104633331299 -0.395263671875
5.34112787246704 -0.39532470703125
5.34151363372803 -0.3953857421875
5.34179639816284 -0.3953857421875
5.34224319458008 -0.3953857421875
5.34304618835449 -0.39544677734375
5.34333181381226 -0.3955078125
5.34374332427979 -0.3955078125
5.34415435791016 -0.39556884765625
5.34493255615234 -0.3956298828125
5.34585189819336 -0.3956298828125
5.34671878814697 -0.39581298828125
5.3470253944397 -0.3958740234375
5.34777498245239 -0.39605712890625
5.34829139709473 -0.3961181640625
5.34863376617432 -0.3961181640625
5.34871578216553 -0.3961181640625
5.34915685653687 -0.39617919921875
5.34958267211914 -0.39617919921875
5.34969711303711 -0.396240234375
5.35012769699097 -0.39630126953125
5.350426197052 -0.39630126953125
5.35091638565063 -0.3963623046875
5.3510537147522 -0.3963623046875
5.35118913650513 -0.39642333984375
5.35166692733765 -0.396484375
5.35226917266846 -0.39654541015625
5.35239458084106 -0.3966064453125
5.3525915145874 -0.3966064453125
5.35323333740234 -0.39678955078125
5.35336971282959 -0.3968505859375
5.35391044616699 -0.3968505859375
5.35443878173828 -0.39691162109375
5.35449647903442 -0.39691162109375
5.35477685928345 -0.39697265625
5.35529613494873 -0.39703369140625
5.35547065734863 -0.39703369140625
5.35579442977905 -0.39703369140625
5.35624217987061 -0.3970947265625
5.35645246505737 -0.3970947265625
5.35684394836426 -0.39715576171875
5.3569393157959 -0.39715576171875
5.35721445083618 -0.397216796875
5.35746240615845 -0.397216796875
5.35796546936035 -0.3973388671875
5.35820722579956 -0.3973388671875
5.35853433609009 -0.39739990234375
5.35868644714355 -0.39739990234375
5.3589129447937 -0.39739990234375
5.35904407501221 -0.3974609375
5.35919952392578 -0.3974609375
5.3596363067627 -0.3974609375
5.3598051071167 -0.3974609375
5.36254835128784 -0.3990478515625
5.3627781867981 -0.399169921875
5.36303234100342 -0.39923095703125
5.36315679550171 -0.39923095703125
5.3632378578186 -0.3992919921875
5.36353302001953 -0.39935302734375
5.36372470855713 -0.39935302734375
5.36403656005859 -0.3994140625
5.36417007446289 -0.3994140625
5.36439323425293 -0.3994140625
5.36447048187256 -0.39947509765625
5.36470460891724 -0.39947509765625
5.36489248275757 -0.39947509765625
5.36508512496948 -0.3995361328125
5.36541318893433 -0.39959716796875
5.36565828323364 -0.39959716796875
5.36593914031982 -0.399658203125
5.36596155166626 -0.399658203125
5.36723279953003 -0.39996337890625
5.36756658554077 -0.4000244140625
5.36768579483032 -0.4000244140625
5.36781406402588 -0.4000244140625
5.36863660812378 -0.4000244140625
5.36888551712036 -0.40008544921875
5.36961460113525 -0.40020751953125
5.36996507644653 -0.40020751953125
5.37003183364868 -0.40020751953125
5.37341976165771 -0.40179443359375
5.37353515625 -0.40191650390625
5.37367677688599 -0.4019775390625
5.37384748458862 -0.4019775390625
5.37395620346069 -0.4019775390625
5.37418174743652 -0.4019775390625
5.37424755096436 -0.4019775390625
5.37430477142334 -0.40203857421875
5.37628650665283 -0.40240478515625
5.37654781341553 -0.40240478515625
5.37703466415405 -0.40240478515625
5.3771276473999 -0.40240478515625
5.37759208679199 -0.40240478515625
5.37788677215576 -0.40240478515625
5.37805271148682 -0.4024658203125
5.38032865524292 -0.40264892578125
5.38048791885376 -0.4027099609375
5.38058567047119 -0.4027099609375
5.38066864013672 -0.4027099609375
5.38078832626343 -0.4027099609375
5.3811206817627 -0.40277099609375
5.38127946853638 -0.40277099609375
5.38138961791992 -0.40277099609375
5.38193225860596 -0.40277099609375
5.38204956054688 -0.40283203125
5.3824257850647 -0.40283203125
5.38314008712769 -0.40283203125
5.38321018218994 -0.40289306640625
5.38333034515381 -0.40289306640625
5.38343811035156 -0.40289306640625
5.38351726531982 -0.40289306640625
5.38408470153809 -0.4029541015625
5.3841814994812 -0.4029541015625
5.38437652587891 -0.4029541015625
5.38462209701538 -0.4029541015625
5.38478326797485 -0.4029541015625
5.38510036468506 -0.40301513671875
5.38568830490112 -0.40301513671875
5.38598680496216 -0.403076171875
5.38639545440674 -0.403076171875
5.38658285140991 -0.403076171875
5.38699102401733 -0.403076171875
5.38844776153564 -0.4031982421875
5.38850259780884 -0.4031982421875
5.38883113861084 -0.40325927734375
5.38892507553101 -0.40325927734375
5.39118051528931 -0.40350341796875
5.39119434356689 -0.40350341796875
5.39177656173706 -0.403564453125
5.39198970794678 -0.403564453125
5.39205121994019 -0.403564453125
5.39267063140869 -0.403564453125
5.39273738861084 -0.403564453125
5.39286422729492 -0.403564453125
5.39570188522339 -0.40460205078125
5.3958888053894 -0.40484619140625
5.39596366882324 -0.40484619140625
5.39676761627197 -0.40496826171875
5.3968825340271 -0.40496826171875
5.39730548858643 -0.40496826171875
5.39734029769897 -0.405029296875
5.39771938323975 -0.405029296875
5.39838981628418 -0.40509033203125
5.39866209030151 -0.40509033203125
5.39899492263794 -0.40509033203125
5.3990626335144 -0.40509033203125
5.39927387237549 -0.4051513671875
5.40025997161865 -0.40521240234375
5.40064001083374 -0.4052734375
5.40085411071777 -0.4052734375
5.40121793746948 -0.4052734375
5.40159893035889 -0.4052734375
5.40185880661011 -0.40533447265625
5.4024829864502 -0.40533447265625
5.40255880355835 -0.40533447265625
5.40273571014404 -0.40533447265625
5.40286111831665 -0.40533447265625
5.40341377258301 -0.4053955078125
5.40356826782227 -0.4053955078125
5.40396928787231 -0.4053955078125
5.40404987335205 -0.4053955078125
5.40428304672241 -0.4053955078125
5.40439748764038 -0.4053955078125
5.40561962127686 -0.40545654296875
5.40586853027344 -0.405517578125
5.40615510940552 -0.405517578125
5.40628957748413 -0.405517578125
5.40643978118896 -0.40557861328125
5.40678691864014 -0.40557861328125
5.40714597702026 -0.40557861328125
5.40716981887817 -0.40557861328125
5.40755224227905 -0.40557861328125
5.40763568878174 -0.40557861328125
5.40957450866699 -0.4058837890625
5.40970659255981 -0.40594482421875
5.40988731384277 -0.40594482421875
5.40997552871704 -0.40594482421875
5.41024923324585 -0.40594482421875
5.41034030914307 -0.40594482421875
5.41049718856812 -0.40594482421875
5.41057300567627 -0.406005859375
5.41058158874512 -0.406005859375
5.41105556488037 -0.406005859375
5.41116857528687 -0.406005859375
5.41182518005371 -0.406005859375
5.41205024719238 -0.40606689453125
5.41214799880981 -0.40606689453125
5.41223526000977 -0.40606689453125
5.41242694854736 -0.40606689453125
5.41264677047729 -0.40606689453125
5.41349744796753 -0.40618896484375
5.41355276107788 -0.40618896484375
5.41367673873901 -0.40618896484375
5.41410207748413 -0.40618896484375
5.41421937942505 -0.40618896484375
5.41424131393433 -0.40618896484375
5.41524219512939 -0.40643310546875
5.41579103469849 -0.406494140625
5.41588449478149 -0.406494140625
5.4161262512207 -0.406494140625
5.41622447967529 -0.406494140625
5.41673374176025 -0.406494140625
5.41698312759399 -0.40655517578125
5.41754484176636 -0.4066162109375
5.41800785064697 -0.4066162109375
5.41812705993652 -0.40667724609375
5.41875028610229 -0.40667724609375
5.41891574859619 -0.40667724609375
5.41929149627686 -0.40667724609375
5.41947841644287 -0.40673828125
5.41971778869629 -0.40673828125
5.42051696777344 -0.40679931640625
5.42064523696899 -0.40679931640625
5.42073106765747 -0.40679931640625
5.42080020904541 -0.40679931640625
5.4208517074585 -0.40679931640625
5.42098665237427 -0.40679931640625
5.42118740081787 -0.40679931640625
5.42127656936646 -0.40679931640625
5.42171764373779 -0.40692138671875
5.42181301116943 -0.40692138671875
5.42196083068848 -0.40692138671875
5.42196893692017 -0.40692138671875
5.4223484992981 -0.40692138671875
5.42262601852417 -0.40692138671875
5.42271947860718 -0.40692138671875
5.42278003692627 -0.40692138671875
5.42316246032715 -0.406982421875
5.42321157455444 -0.406982421875
5.42379283905029 -0.40704345703125
5.42393016815186 -0.4071044921875
5.42415285110474 -0.4071044921875
5.42466926574707 -0.4071044921875
5.42486381530762 -0.4071044921875
5.42502212524414 -0.4071044921875
5.4254674911499 -0.4071044921875
5.4261531829834 -0.40716552734375
5.42630767822266 -0.40716552734375
5.42635202407837 -0.4072265625
5.42658615112305 -0.4072265625
5.42671632766724 -0.4072265625
5.42703485488892 -0.4072265625
5.42710304260254 -0.4072265625
5.42725229263306 -0.40728759765625
5.42739868164062 -0.40728759765625
5.42742109298706 -0.40728759765625
5.42772769927979 -0.40728759765625
5.42821073532104 -0.4073486328125
5.42829370498657 -0.4073486328125
5.42891216278076 -0.4073486328125
5.42909955978394 -0.4073486328125
5.42930793762207 -0.4073486328125
5.42983484268188 -0.40740966796875
5.42993450164795 -0.40740966796875
5.43004608154297 -0.40740966796875
5.43029928207397 -0.40740966796875
5.4303765296936 -0.407470703125
5.43054103851318 -0.407470703125
5.43069887161255 -0.407470703125
5.43078756332397 -0.407470703125
5.43115139007568 -0.407470703125
5.43119955062866 -0.407470703125
5.43140554428101 -0.407470703125
5.43164825439453 -0.407470703125
5.43290996551514 -0.40765380859375
5.43328666687012 -0.40771484375
5.43338108062744 -0.40771484375
5.43344163894653 -0.40771484375
5.4336576461792 -0.40771484375
5.43388175964355 -0.40771484375
5.43430233001709 -0.40771484375
5.43446016311646 -0.40771484375
5.43446350097656 -0.40771484375
5.43457221984863 -0.40777587890625
5.43476676940918 -0.40777587890625
5.43497610092163 -0.40777587890625
5.43504619598389 -0.40777587890625
5.43505382537842 -0.40777587890625
5.43545579910278 -0.40777587890625
5.43555784225464 -0.40777587890625
5.43573141098022 -0.40777587890625
5.43589210510254 -0.4078369140625
5.4362006187439 -0.4078369140625
5.43628215789795 -0.4078369140625
5.43636131286621 -0.4078369140625
5.43666362762451 -0.4078369140625
5.43667125701904 -0.4078369140625
5.43688726425171 -0.4078369140625
5.43696212768555 -0.4078369140625
5.43718433380127 -0.4078369140625
5.4372239112854 -0.40789794921875
5.43826198577881 -0.40814208984375
5.43852949142456 -0.40814208984375
5.43928194046021 -0.40814208984375
5.43929815292358 -0.40814208984375
5.4394211769104 -0.408203125
5.43984413146973 -0.408203125
5.43989944458008 -0.408203125
5.44009780883789 -0.40826416015625
5.44017839431763 -0.40826416015625
5.44064950942993 -0.40826416015625
5.44072198867798 -0.40826416015625
5.44072341918945 -0.40826416015625
5.44087266921997 -0.40826416015625
5.44095611572266 -0.40826416015625
5.4412693977356 -0.40826416015625
5.44131469726562 -0.40826416015625
5.44185543060303 -0.4083251953125
5.44223690032959 -0.4083251953125
5.44224452972412 -0.4083251953125
5.4422664642334 -0.4083251953125
5.44262552261353 -0.40838623046875
5.4429669380188 -0.40838623046875
5.44309377670288 -0.40838623046875
5.44311571121216 -0.40838623046875
5.4432315826416 -0.40838623046875
5.44355535507202 -0.40838623046875
5.44373989105225 -0.408447265625
5.44411182403564 -0.408447265625
5.44413375854492 -0.408447265625
5.4444694519043 -0.408447265625
5.4448127746582 -0.408447265625
5.44512462615967 -0.408447265625
5.44518041610718 -0.40850830078125
5.44522714614868 -0.40850830078125
5.44546270370483 -0.40850830078125
5.44561958312988 -0.40850830078125
5.4456992149353 -0.40850830078125
5.44634628295898 -0.4085693359375
5.4463586807251 -0.4085693359375
5.44640207290649 -0.4085693359375
5.44659614562988 -0.4085693359375
5.44709730148315 -0.40863037109375
5.4472804069519 -0.40863037109375
5.44745588302612 -0.40863037109375
5.44748067855835 -0.40863037109375
5.44768810272217 -0.40863037109375
5.44779348373413 -0.40869140625
5.44796514511108 -0.40869140625
5.44812488555908 -0.40869140625
5.44821453094482 -0.40869140625
5.44844341278076 -0.40869140625
5.44854259490967 -0.40869140625
5.44882822036743 -0.40869140625
5.45006132125854 -0.408935546875
5.45023965835571 -0.40899658203125
5.45026588439941 -0.40899658203125
5.45049238204956 -0.40899658203125
5.45050001144409 -0.40899658203125
5.45062160491943 -0.40899658203125
5.45094776153564 -0.40899658203125
5.45158529281616 -0.4090576171875
5.45175123214722 -0.40911865234375
5.4518723487854 -0.40911865234375
5.45196437835693 -0.40911865234375
5.45208549499512 -0.40911865234375
5.4537525177002 -0.4097900390625
5.45396757125854 -0.40997314453125
5.45464658737183 -0.40997314453125
5.45467281341553 -0.40997314453125
5.45476388931274 -0.40997314453125
5.45477151870728 -0.40997314453125
5.45494699478149 -0.40997314453125
5.45567464828491 -0.40997314453125
5.4557671546936 -0.40997314453125
5.45579147338867 -0.40997314453125
5.45591020584106 -0.40997314453125
5.45643901824951 -0.40997314453125
5.45664548873901 -0.40997314453125
5.45680475234985 -0.4100341796875
5.45683670043945 -0.4100341796875
5.45743656158447 -0.4100341796875
5.45745325088501 -0.4100341796875
5.45749139785767 -0.4100341796875
5.45812702178955 -0.41009521484375
5.45877838134766 -0.41009521484375
5.4588794708252 -0.41009521484375
5.45890522003174 -0.41009521484375
5.45894289016724 -0.41015625
5.45901966094971 -0.41015625
5.45915555953979 -0.41015625
5.45922517776489 -0.41015625
5.45922946929932 -0.41015625
5.45938491821289 -0.41015625
5.45953273773193 -0.41015625
5.45965909957886 -0.41015625
5.45974683761597 -0.41015625
5.45975112915039 -0.41015625
5.46013212203979 -0.41015625
5.46018505096436 -0.41015625
5.46036100387573 -0.41015625
5.46038198471069 -0.41015625
5.46045732498169 -0.41021728515625
5.46050071716309 -0.41021728515625
5.46112489700317 -0.41021728515625
5.46123743057251 -0.41021728515625
5.46159315109253 -0.4102783203125
5.46170425415039 -0.4102783203125
5.46189880371094 -0.4102783203125
5.46193218231201 -0.4102783203125
5.46237564086914 -0.4102783203125
5.4626030921936 -0.4102783203125
5.46277523040771 -0.4102783203125
5.46279001235962 -0.4102783203125
5.46311330795288 -0.4102783203125
5.46315670013428 -0.4102783203125
5.4631609916687 -0.4102783203125
5.46319675445557 -0.4102783203125
5.46382904052734 -0.4102783203125
5.46389007568359 -0.4102783203125
5.46411228179932 -0.41033935546875
5.46430921554565 -0.41033935546875
5.46435403823853 -0.41033935546875
5.46466827392578 -0.41033935546875
5.46476221084595 -0.41033935546875
5.46477556228638 -0.41033935546875
5.46485137939453 -0.41033935546875
5.46492147445679 -0.41033935546875
5.46492624282837 -0.41033935546875
5.46521615982056 -0.41033935546875
5.46533966064453 -0.41033935546875
5.46543788909912 -0.41033935546875
5.46600103378296 -0.410400390625
5.46621942520142 -0.410400390625
5.46629524230957 -0.410400390625
5.46645402908325 -0.410400390625
5.46657562255859 -0.410400390625
5.46680688858032 -0.410400390625
5.46695947647095 -0.41046142578125
5.46717739105225 -0.41046142578125
5.4676685333252 -0.41046142578125
5.46770429611206 -0.41046142578125
5.46812295913696 -0.41046142578125
5.46813011169434 -0.41046142578125
5.46824073791504 -0.41046142578125
5.46837997436523 -0.41046142578125
5.46859264373779 -0.41046142578125
5.46872520446777 -0.41046142578125
5.46886253356934 -0.41046142578125
5.46914005279541 -0.41046142578125
5.46922397613525 -0.41046142578125
5.46924877166748 -0.41046142578125
5.46925354003906 -0.41046142578125
5.46963787078857 -0.41046142578125
5.46986627578735 -0.41046142578125
5.46987056732178 -0.41046142578125
5.47002792358398 -0.41046142578125
5.47005319595337 -0.41046142578125
5.47015476226807 -0.4105224609375
5.47019863128662 -0.4105224609375
5.47020769119263 -0.4105224609375
5.47092628479004 -0.41058349609375
5.47118330001831 -0.41064453125
5.47118759155273 -0.41064453125
5.47123146057129 -0.41064453125
5.47123575210571 -0.41064453125
5.47153949737549 -0.41064453125
5.47163772583008 -0.41064453125
5.47191047668457 -0.41064453125
5.47193956375122 -0.41064453125
5.47202301025391 -0.41064453125
5.47233057022095 -0.41064453125
5.47254276275635 -0.41064453125
5.47322702407837 -0.41070556640625
5.47344923019409 -0.41070556640625
5.47371912002563 -0.41070556640625
5.47377300262451 -0.41070556640625
5.47378015518188 -0.41070556640625
5.47416543960571 -0.4107666015625
5.47422361373901 -0.4107666015625
5.47423648834229 -0.4107666015625
5.4743766784668 -0.4107666015625
5.4745135307312 -0.4107666015625
5.47473764419556 -0.4107666015625
5.47491836547852 -0.4107666015625
5.47532987594604 -0.4107666015625
5.47545480728149 -0.4107666015625
5.47552442550659 -0.4107666015625
5.47570466995239 -0.4107666015625
5.47585868835449 -0.4107666015625
5.47599363327026 -0.4107666015625
5.47607755661011 -0.4107666015625
5.47609949111938 -0.4107666015625
5.47610950469971 -0.4107666015625
5.4765419960022 -0.41082763671875
5.47669839859009 -0.41082763671875
5.47711706161499 -0.41082763671875
5.47767400741577 -0.41082763671875
5.47771739959717 -0.41082763671875
5.47778940200806 -0.41082763671875
5.47798585891724 -0.41082763671875
5.47801065444946 -0.41082763671875
5.4781060218811 -0.41082763671875
5.47836446762085 -0.41082763671875
5.47839164733887 -0.41082763671875
5.47855663299561 -0.41082763671875
5.47860383987427 -0.41082763671875
5.47864151000977 -0.41082763671875
5.47872829437256 -0.41082763671875
5.47874975204468 -0.41082763671875
5.47890090942383 -0.41082763671875
5.47933197021484 -0.41082763671875
5.47938537597656 -0.41082763671875
5.47945737838745 -0.41082763671875
5.47955083847046 -0.41082763671875
5.47994232177734 -0.41082763671875
5.47996807098389 -0.41082763671875
5.47997236251831 -0.41082763671875
5.48014640808105 -0.41082763671875
5.48016500473022 -0.41082763671875
5.48021841049194 -0.410888671875
5.48021984100342 -0.410888671875
5.48023700714111 -0.410888671875
5.48027420043945 -0.410888671875
5.48029899597168 -0.410888671875
5.48069095611572 -0.410888671875
5.4806981086731 -0.410888671875
5.48071670532227 -0.410888671875
5.48097658157349 -0.410888671875
5.48105382919312 -0.410888671875
5.48135089874268 -0.410888671875
5.48140525817871 -0.410888671875
};
\addplot [ultra thick, blue]
table {%
-inf 0
-inf -0.0003662109375
-inf -0.00042724609375
-inf -0.00042724609375
-inf -0.00042724609375
-inf -0.00042724609375
-inf -0.00042724609375
-inf -0.00042724609375
-inf -0.00048828125
-inf -0.00048828125
-inf -0.00048828125
-inf -0.00048828125
-inf -0.00048828125
0.954242527484894 -0.001708984375
0.954242527484894 -0.002197265625
0.954242527484894 -0.002197265625
1.04139268398285 -0.00225830078125
1.04139268398285 -0.0023193359375
1.07918119430542 -0.00238037109375
1.07918119430542 -0.00244140625
1.14612805843353 -0.00244140625
1.14612805843353 -0.00244140625
1.23044896125793 -0.00262451171875
1.25527250766754 -0.002685546875
1.27875363826752 -0.0028076171875
1.32221925258636 -0.00286865234375
1.46239805221558 -0.00396728515625
1.47712123394012 -0.00433349609375
1.50514996051788 -0.0045166015625
1.53147888183594 -0.004638671875
1.61278390884399 -0.00567626953125
1.68124127388 -0.0059814453125
1.70757019519806 -0.0064697265625
1.74036264419556 -0.0068359375
1.77085208892822 -0.00732421875
1.78532981872559 -0.0076904296875
1.81291329860687 -0.008056640625
1.91907811164856 -0.01348876953125
1.9344984292984 -0.01513671875
2.00432133674622 -0.01580810546875
2.04532289505005 -0.018310546875
2.06445789337158 -0.01904296875
2.13987898826599 -0.01995849609375
2.14612793922424 -0.020263671875
2.17609119415283 -0.02130126953125
2.19589972496033 -0.021728515625
2.21748399734497 -0.0220947265625
2.24797320365906 -0.0230712890625
2.2810332775116 -0.02374267578125
2.35602593421936 -0.02685546875
2.36361193656921 -0.028564453125
2.39269685745239 -0.03106689453125
2.41329979896545 -0.03179931640625
2.43616271018982 -0.0325927734375
2.48000693321228 -0.038818359375
2.49415469169617 -0.04058837890625
2.53275442123413 -0.04180908203125
2.57054305076599 -0.04669189453125
2.58319878578186 -0.04827880859375
2.59328603744507 -0.05010986328125
2.62117624282837 -0.052734375
2.63042783737183 -0.0545654296875
2.65127801895142 -0.05645751953125
2.66086554527283 -0.05780029296875
2.69019603729248 -0.05963134765625
2.69635629653931 -0.060546875
2.71600341796875 -0.06402587890625
2.72916483879089 -0.066650390625
2.73798727989197 -0.0697021484375
2.76117587089539 -0.07135009765625
2.76863813400269 -0.07403564453125
2.78675150871277 -0.0772705078125
2.78958082199097 -0.078369140625
2.81424760818481 -0.08251953125
2.82412576675415 -0.08447265625
2.8331470489502 -0.08575439453125
2.83758854866028 -0.0869140625
2.85612440109253 -0.0887451171875
2.86093664169312 -0.089599609375
2.88309335708618 -0.0914306640625
2.88930177688599 -0.09228515625
2.89597463607788 -0.09320068359375
2.90091300010681 -0.09393310546875
2.91750550270081 -0.0992431640625
2.93500328063965 -0.102783203125
2.94299960136414 -0.10394287109375
2.95327639579773 -0.10491943359375
2.95520663261414 -0.10546875
2.96520185470581 -0.1080322265625
2.98272347450256 -0.10894775390625
2.99782299995422 -0.11505126953125
3.00259804725647 -0.11639404296875
3.00774788856506 -0.117431640625
3.01911640167236 -0.1190185546875
3.02612447738647 -0.1195068359375
3.04414772987366 -0.1231689453125
3.05230903625488 -0.125
3.06333327293396 -0.1280517578125
3.07845687866211 -0.13134765625
3.08457636833191 -0.13311767578125
3.09760427474976 -0.135986328125
3.12057399749756 -0.1453857421875
3.1258065700531 -0.15191650390625
3.13449573516846 -0.15484619140625
3.13735413551331 -0.1568603515625
3.1489109992981 -0.1683349609375
3.16345953941345 -0.171142578125
3.17897701263428 -0.18634033203125
3.18440747261047 -0.19146728515625
3.19061183929443 -0.1966552734375
3.21642971038818 -0.199951171875
3.22505068778992 -0.20440673828125
3.22685766220093 -0.2066650390625
3.23223352432251 -0.21026611328125
3.23829698562622 -0.21307373046875
3.24649858474731 -0.2169189453125
3.25017595291138 -0.21942138671875
3.25527262687683 -0.22119140625
3.25671768188477 -0.2222900390625
3.25959396362305 -0.22369384765625
3.26904582977295 -0.236083984375
3.27067875862122 -0.23828125
3.27346420288086 -0.23883056640625
3.27921056747437 -0.2401123046875
3.28914284706116 -0.2452392578125
3.29092454910278 -0.24609375
3.29358339309692 -0.24713134765625
3.29490685462952 -0.24810791015625
3.30168104171753 -0.24969482421875
3.30276370048523 -0.2501220703125
3.30470585823059 -0.25048828125
3.30513620376587 -0.250732421875
3.31722736358643 -0.2581787109375
3.32283926010132 -0.2596435546875
3.32366442680359 -0.2598876953125
3.33344721794128 -0.26434326171875
3.33665990829468 -0.265869140625
3.34810996055603 -0.26934814453125
3.35102295875549 -0.2708740234375
3.35640835762024 -0.27166748046875
3.35869598388672 -0.27215576171875
3.3626708984375 -0.27325439453125
3.36492609977722 -0.27423095703125
3.37125253677368 -0.27752685546875
3.37401485443115 -0.2786865234375
3.37748837471008 -0.27972412109375
3.38093447685242 -0.28094482421875
3.38827896118164 -0.2852783203125
3.39164066314697 -0.28631591796875
3.39304852485657 -0.286865234375
3.39898109436035 -0.28753662109375
3.40790057182312 -0.29541015625
3.41027092933655 -0.29852294921875
3.4126284122467 -0.29901123046875
3.4163076877594 -0.2999267578125
3.41879820823669 -0.30224609375
3.42308187484741 -0.3028564453125
3.42390084266663 -0.30316162109375
3.43152451515198 -0.3077392578125
3.43280911445618 -0.30841064453125
3.4353666305542 -0.308837890625
3.43822574615479 -0.309814453125
3.43980622291565 -0.31024169921875
3.44669246673584 -0.3131103515625
3.44762301445007 -0.3134765625
3.44963264465332 -0.31390380859375
3.4527063369751 -0.3148193359375
3.45499730110168 -0.3153076171875
3.45545387268066 -0.3155517578125
3.45939254760742 -0.31585693359375
3.46089792251587 -0.3162841796875
3.46404218673706 -0.31671142578125
3.46434044837952 -0.31689453125
3.46508526802063 -0.31707763671875
3.47334098815918 -0.3203125
3.47421622276306 -0.3206787109375
3.47538065910339 -0.32086181640625
3.47712135314941 -0.32110595703125
3.4791431427002 -0.32122802734375
3.47957539558411 -0.3214111328125
3.48273062705994 -0.322265625
3.48685526847839 -0.32305908203125
3.48798632621765 -0.3232421875
3.48911428451538 -0.32354736328125
3.49317908287048 -0.32391357421875
3.49568295478821 -0.32421875
3.49982452392578 -0.32513427734375
3.50270009040833 -0.3253173828125
3.5039267539978 -0.3255615234375
3.50487852096558 -0.32574462890625
3.50772094726562 -0.32611083984375
3.50879907608032 -0.32623291015625
3.51825070381165 -0.3306884765625
3.51890850067139 -0.3316650390625
3.520352602005 -0.3319091796875
3.52100729942322 -0.33221435546875
3.52711415290833 -0.33502197265625
3.52840232849121 -0.3355712890625
3.53045582771301 -0.3363037109375
3.53605318069458 -0.3382568359375
3.53769326210022 -0.3388671875
3.53982853889465 -0.33929443359375
3.54132962226868 -0.33978271484375
3.54543089866638 -0.3408203125
3.5467894077301 -0.34124755859375
3.54863500595093 -0.34161376953125
3.54973864555359 -0.341796875
3.55545711517334 -0.34326171875
3.55654382705688 -0.34356689453125
3.5597870349884 -0.34490966796875
3.56133985519409 -0.34527587890625
3.5654935836792 -0.3463134765625
3.5659658908844 -0.34661865234375
3.56925678253174 -0.346923828125
3.56972503662109 -0.34722900390625
3.57054281234741 -0.3475341796875
3.57356786727905 -0.34844970703125
3.57634139060974 -0.348876953125
3.57680177688599 -0.349365234375
3.57909727096558 -0.349853515625
3.58172225952148 -0.3502197265625
3.58591175079346 -0.35162353515625
3.58636236190796 -0.35205078125
3.59117603302002 -0.35455322265625
3.59262084960938 -0.35479736328125
3.59284257888794 -0.35498046875
3.59339690208435 -0.35528564453125
3.59372901916504 -0.3553466796875
3.59648704528809 -0.355712890625
3.59714651107788 -0.3560791015625
3.59725618362427 -0.356201171875
3.59955549240112 -0.3565673828125
3.60053730010986 -0.35687255859375
3.60064625740051 -0.35693359375
3.60075521469116 -0.35699462890625
3.60433411598206 -0.35723876953125
3.60444211959839 -0.35736083984375
3.6049816608429 -0.357421875
3.60670375823975 -0.35760498046875
3.60670375823975 -0.357666015625
3.6073477268219 -0.3577880859375
3.60756230354309 -0.35784912109375
3.60948777198792 -0.35833740234375
3.61097931861877 -0.3585205078125
3.61119198799133 -0.35858154296875
3.61129832267761 -0.358642578125
3.61172342300415 -0.35870361328125
3.61182951927185 -0.3587646484375
3.6133131980896 -0.35906982421875
3.61394739151001 -0.359130859375
3.61479187011719 -0.35919189453125
3.61595010757446 -0.3592529296875
3.61825728416443 -0.35968017578125
3.61836194992065 -0.35968017578125
3.61930203437805 -0.35992431640625
3.6208643913269 -0.36004638671875
3.62096834182739 -0.36004638671875
3.62148785591125 -0.360107421875
3.62148785591125 -0.3602294921875
3.62293887138367 -0.36029052734375
3.62634038925171 -0.36114501953125
3.62644290924072 -0.3612060546875
3.62777543067932 -0.361328125
3.63042783737183 -0.36199951171875
3.63093614578247 -0.36212158203125
3.63286209106445 -0.3621826171875
3.63286209106445 -0.36224365234375
3.63457798957825 -0.3623046875
3.63457798957825 -0.36236572265625
3.64068007469177 -0.36627197265625
3.64147400856018 -0.366943359375
3.6428599357605 -0.3670654296875
3.64483237266541 -0.3671875
3.64532399177551 -0.36737060546875
3.64591336250305 -0.367431640625
3.64845752716064 -0.36773681640625
3.64991879463196 -0.3680419921875
3.65118098258972 -0.36810302734375
3.65388751029968 -0.36883544921875
3.65552258491516 -0.3695068359375
3.65619397163391 -0.3697509765625
3.65715146064758 -0.36981201171875
3.66039109230042 -0.370361328125
3.6624743938446 -0.3707275390625
3.66435980796814 -0.3709716796875
3.66482996940613 -0.37109375
3.67228269577026 -0.37530517578125
3.6727442741394 -0.376220703125
3.67329740524292 -0.3763427734375
3.67715048789978 -0.37750244140625
3.67733311653137 -0.37762451171875
3.67933702468872 -0.3780517578125
3.67979121208191 -0.37841796875
3.68024492263794 -0.3785400390625
3.68060731887817 -0.3785400390625
3.68609976768494 -0.3797607421875
3.68636798858643 -0.3800048828125
3.68726134300232 -0.380126953125
3.6873505115509 -0.38018798828125
3.68993020057678 -0.38031005859375
3.69028472900391 -0.38037109375
3.69240617752075 -0.3809814453125
3.69249439239502 -0.381103515625
3.69302296638489 -0.38116455078125
3.6945173740387 -0.38128662109375
3.69504356384277 -0.38140869140625
3.69548177719116 -0.3814697265625
3.69635629653931 -0.381591796875
3.69818758964539 -0.38177490234375
3.69957756996155 -0.382080078125
3.70009779930115 -0.3822021484375
3.70268893241882 -0.38262939453125
3.70406460762024 -0.3829345703125
3.70440793037415 -0.38311767578125
3.70791077613831 -0.3843994140625
3.70901536941528 -0.384765625
3.71248126029968 -0.3857421875
3.71281790733337 -0.385986328125
3.71382641792297 -0.3863525390625
3.71483254432678 -0.386474609375
3.7158362865448 -0.38671875
3.71758723258972 -0.386962890625
3.71841859817505 -0.38714599609375
3.71933126449585 -0.38720703125
3.71957993507385 -0.3873291015625
3.72040748596191 -0.387451171875
3.72098565101624 -0.38751220703125
3.72214007377625 -0.3875732421875
3.72288060188293 -0.38763427734375
3.72468543052673 -0.38775634765625
3.72558498382568 -0.3878173828125
3.72770380973816 -0.38885498046875
3.72989344596863 -0.38897705078125
3.7307014465332 -0.38922119140625
3.73287606239319 -0.38946533203125
3.7332775592804 -0.3895263671875
3.73367857933044 -0.38958740234375
3.73615741729736 -0.39007568359375
3.73655581474304 -0.39031982421875
3.73798727989197 -0.390380859375
3.73870134353638 -0.390625
3.739018201828 -0.39068603515625
3.7411515712738 -0.39117431640625
3.74146676063538 -0.39129638671875
3.74178171157837 -0.391357421875
3.74209642410278 -0.3914794921875
3.74248933792114 -0.3917236328125
3.74358820915222 -0.39178466796875
3.74491858482361 -0.39227294921875
3.74523091316223 -0.392333984375
3.74624490737915 -0.3924560546875
3.74655628204346 -0.39251708984375
3.74686765670776 -0.392578125
3.74717855453491 -0.39263916015625
3.74741172790527 -0.392822265625
3.74764490127563 -0.39288330078125
3.74795532226562 -0.39300537109375
3.7499680519104 -0.393310546875
3.75027680397034 -0.39337158203125
3.75050830841064 -0.3934326171875
3.750816822052 -0.39349365234375
3.75097107887268 -0.3935546875
3.75104808807373 -0.3935546875
3.75296974182129 -0.39361572265625
3.75327658653259 -0.393798828125
3.7537362575531 -0.393798828125
3.7551121711731 -0.3946533203125
3.7563316822052 -0.39471435546875
3.75640773773193 -0.39471435546875
3.75663614273071 -0.394775390625
3.75663614273071 -0.394775390625
3.75663614273071 -0.394775390625
3.75830626487732 -0.39501953125
3.75898742675781 -0.39520263671875
3.75906324386597 -0.395263671875
3.75936555862427 -0.395263671875
3.75944113731384 -0.395263671875
3.75981879234314 -0.3953857421875
3.76004528999329 -0.3953857421875
3.76012086868286 -0.39544677734375
3.76019620895386 -0.39544677734375
3.76057314872742 -0.3955078125
3.76064872741699 -0.3955078125
3.76064872741699 -0.3955078125
3.76064872741699 -0.39556884765625
3.76110053062439 -0.39556884765625
3.76522135734558 -0.39801025390625
3.76566863059998 -0.39837646484375
3.76581764221191 -0.3984375
3.76589202880859 -0.3984375
3.76604080200195 -0.39849853515625
3.76671028137207 -0.39849853515625
3.76671028137207 -0.39849853515625
3.76693296432495 -0.3985595703125
3.76693296432495 -0.3985595703125
3.76708173751831 -0.39862060546875
3.76708173751831 -0.398681640625
3.76760101318359 -0.39874267578125
3.76834201812744 -0.39874267578125
3.76841616630554 -0.39874267578125
3.76841616630554 -0.3988037109375
3.77004146575928 -0.39935302734375
3.77092552185059 -0.3994140625
3.77107286453247 -0.39947509765625
3.77114629745483 -0.39947509765625
3.77114629745483 -0.39947509765625
3.7723217010498 -0.3995361328125
3.7723217010498 -0.3995361328125
3.7723217010498 -0.3995361328125
3.77517342567444 -0.4002685546875
3.77524614334106 -0.40032958984375
3.77524614334106 -0.40032958984375
3.77524614334106 -0.40032958984375
3.77561044692993 -0.400390625
3.77575612068176 -0.400390625
3.77582883834839 -0.40045166015625
3.77590155601501 -0.40045166015625
3.77735424041748 -0.400634765625
3.77742671966553 -0.400634765625
3.77742671966553 -0.40069580078125
3.77815127372742 -0.40069580078125
3.77815127372742 -0.40069580078125
3.77815127372742 -0.40069580078125
3.77930784225464 -0.40093994140625
3.77938008308411 -0.40093994140625
3.779452085495 -0.40093994140625
3.779452085495 -0.40093994140625
3.779452085495 -0.4010009765625
3.779452085495 -0.4010009765625
3.7808210849762 -0.401123046875
3.7808210849762 -0.401123046875
3.78089308738708 -0.40118408203125
3.78089308738708 -0.40118408203125
3.78204250335693 -0.40118408203125
3.78204250335693 -0.40118408203125
3.78211402893066 -0.40118408203125
3.78218579292297 -0.4012451171875
3.78218579292297 -0.4012451171875
3.78625440597534 -0.40191650390625
3.78632545471191 -0.4019775390625
3.78639650344849 -0.4019775390625
3.78646755218506 -0.4019775390625
3.78653836250305 -0.4019775390625
3.78653836250305 -0.40203857421875
3.78653836250305 -0.40203857421875
3.78653836250305 -0.40203857421875
3.7870352268219 -0.40203857421875
3.78717708587646 -0.402099609375
3.78717708587646 -0.402099609375
3.788733959198 -0.40240478515625
3.78887510299683 -0.40240478515625
3.78894567489624 -0.40240478515625
3.78901624679565 -0.40240478515625
3.7892279624939 -0.4024658203125
3.7892279624939 -0.4024658203125
3.7892279624939 -0.4024658203125
3.79014444351196 -0.40252685546875
3.7902147769928 -0.40252685546875
3.79077768325806 -0.4027099609375
3.79112911224365 -0.40277099609375
3.79140996932983 -0.40277099609375
3.79239177703857 -0.40277099609375
3.7934410572052 -0.40289306640625
3.7934410572052 -0.40289306640625
3.79351091384888 -0.40289306640625
3.79386019706726 -0.4029541015625
3.79393005371094 -0.40301513671875
3.79393005371094 -0.40301513671875
3.79601907730103 -0.40325927734375
3.79608845710754 -0.40325927734375
3.79615783691406 -0.40325927734375
3.79643559455872 -0.4033203125
3.79650497436523 -0.4033203125
3.79664373397827 -0.4033203125
3.79671311378479 -0.40338134765625
3.79678249359131 -0.40338134765625
3.79733681678772 -0.4034423828125
3.79754447937012 -0.4034423828125
3.79754447937012 -0.4034423828125
3.79754447937012 -0.4034423828125
3.79754447937012 -0.4034423828125
3.79830527305603 -0.40350341796875
3.79851245880127 -0.40350341796875
3.79851245880127 -0.40350341796875
3.79851245880127 -0.40350341796875
3.79878878593445 -0.403564453125
3.79878878593445 -0.403564453125
3.80366182327271 -0.4051513671875
3.80393481254578 -0.40545654296875
3.8040030002594 -0.40545654296875
3.80407118797302 -0.40545654296875
3.80413937568665 -0.40545654296875
3.80420756340027 -0.40545654296875
3.80420756340027 -0.405517578125
3.80427575111389 -0.405517578125
3.80427575111389 -0.405517578125
3.80427575111389 -0.405517578125
3.80427575111389 -0.405517578125
3.80475258827209 -0.405517578125
3.80618000030518 -0.40576171875
3.80624771118164 -0.40576171875
3.80624771118164 -0.40576171875
3.80631566047668 -0.40576171875
3.80631566047668 -0.40576171875
3.80645132064819 -0.40576171875
3.80645132064819 -0.40576171875
3.80645132064819 -0.40582275390625
3.80787324905396 -0.40582275390625
3.80787324905396 -0.40582275390625
3.80787324905396 -0.40582275390625
3.80794072151184 -0.40582275390625
3.80794072151184 -0.40582275390625
3.80794072151184 -0.40582275390625
3.80800819396973 -0.4058837890625
3.80827856063843 -0.4058837890625
3.80827856063843 -0.4058837890625
3.80827856063843 -0.4058837890625
3.80827856063843 -0.4058837890625
3.80982899665833 -0.40594482421875
3.80982899665833 -0.40594482421875
3.80982899665833 -0.40594482421875
3.80982899665833 -0.40594482421875
3.80982899665833 -0.40594482421875
3.80982899665833 -0.40594482421875
3.81016540527344 -0.40606689453125
3.81016540527344 -0.40606689453125
3.81016540527344 -0.40606689453125
3.81023263931274 -0.40606689453125
3.81043410301208 -0.4061279296875
3.81050133705139 -0.4061279296875
3.8105685710907 -0.4061279296875
3.8105685710907 -0.4061279296875
3.8105685710907 -0.4061279296875
3.8105685710907 -0.40618896484375
3.8105685710907 -0.40618896484375
3.8105685710907 -0.40618896484375
3.81083726882935 -0.40618896484375
3.81083726882935 -0.40618896484375
3.81083726882935 -0.40618896484375
3.81117272377014 -0.40631103515625
3.81117272377014 -0.40631103515625
3.81117272377014 -0.40631103515625
3.81117272377014 -0.40631103515625
3.81257915496826 -0.40643310546875
3.81257915496826 -0.40643310546875
3.81257915496826 -0.40643310546875
3.81257915496826 -0.40643310546875
3.81257915496826 -0.406494140625
3.81257915496826 -0.406494140625
3.81378102302551 -0.406494140625
3.81378102302551 -0.406494140625
3.81378102302551 -0.406494140625
3.8141143321991 -0.40655517578125
3.8141143321991 -0.40655517578125
3.8141143321991 -0.40655517578125
3.81511259078979 -0.4066162109375
3.81517910957336 -0.4066162109375
3.81517910957336 -0.4066162109375
3.81517910957336 -0.4066162109375
3.81517910957336 -0.40667724609375
3.8166389465332 -0.40667724609375
3.81670522689819 -0.40667724609375
3.81670522689819 -0.40667724609375
3.81670522689819 -0.40667724609375
3.81690382957458 -0.40673828125
3.81690382957458 -0.40673828125
3.81690382957458 -0.40673828125
3.81723475456238 -0.40673828125
3.81723475456238 -0.40679931640625
3.81730079650879 -0.40679931640625
3.81730079650879 -0.40679931640625
3.8174991607666 -0.40679931640625
3.8174991607666 -0.40679931640625
3.8174991607666 -0.40679931640625
3.8174991607666 -0.40679931640625
3.8174991607666 -0.4068603515625
3.81934642791748 -0.4068603515625
3.81934642791748 -0.4068603515625
3.81954383850098 -0.40692138671875
3.81954383850098 -0.40692138671875
3.81954383850098 -0.40692138671875
3.81954383850098 -0.40692138671875
3.81954383850098 -0.40692138671875
3.82105469703674 -0.40728759765625
3.82105469703674 -0.40728759765625
3.82105469703674 -0.40728759765625
3.8238000869751 -0.407470703125
3.82393050193787 -0.40753173828125
3.82393050193787 -0.40753173828125
3.82393050193787 -0.40753173828125
3.82393050193787 -0.40753173828125
3.82406067848206 -0.4075927734375
3.82406067848206 -0.4075927734375
3.82406067848206 -0.4075927734375
3.82425594329834 -0.4075927734375
3.82425594329834 -0.4075927734375
3.82425594329834 -0.4075927734375
3.82490634918213 -0.40771484375
3.82490634918213 -0.40771484375
3.82503652572632 -0.40771484375
3.82503652572632 -0.40771484375
3.82503652572632 -0.40771484375
3.82503652572632 -0.40771484375
3.82503652572632 -0.40771484375
3.82503652572632 -0.40771484375
3.82536125183105 -0.40777587890625
3.82536125183105 -0.40777587890625
3.82536125183105 -0.40777587890625
3.82600998878479 -0.40777587890625
3.82600998878479 -0.40777587890625
3.82652831077576 -0.4078369140625
3.82659292221069 -0.4078369140625
3.82659292221069 -0.40789794921875
3.82659292221069 -0.40789794921875
3.82659292221069 -0.40789794921875
3.82659292221069 -0.40789794921875
3.82659292221069 -0.40789794921875
3.82659292221069 -0.40789794921875
3.82743382453918 -0.407958984375
3.82743382453918 -0.407958984375
3.82756304740906 -0.407958984375
3.82756304740906 -0.407958984375
3.82756304740906 -0.407958984375
3.82756304740906 -0.407958984375
3.82801508903503 -0.40802001953125
3.82801508903503 -0.40802001953125
3.82911062240601 -0.4080810546875
3.82911062240601 -0.4080810546875
3.82911062240601 -0.4080810546875
3.82911062240601 -0.4080810546875
3.82956099510193 -0.40814208984375
3.83065271377563 -0.408203125
3.83065271377563 -0.408203125
3.83110165596008 -0.40826416015625
3.83110165596008 -0.40826416015625
3.83110165596008 -0.40826416015625
3.83110165596008 -0.40826416015625
3.83199763298035 -0.4083251953125
3.83199763298035 -0.4083251953125
3.83199763298035 -0.4083251953125
3.83199763298035 -0.4083251953125
3.83199763298035 -0.4083251953125
3.83199763298035 -0.4083251953125
3.83206152915955 -0.4083251953125
3.83206152915955 -0.4083251953125
3.83206152915955 -0.4083251953125
3.83206152915955 -0.40838623046875
3.83206152915955 -0.40838623046875
3.83206152915955 -0.40838623046875
3.83295583724976 -0.408447265625
3.83295583724976 -0.408447265625
3.83295583724976 -0.40850830078125
3.83295583724976 -0.40850830078125
3.83295583724976 -0.40850830078125
3.83295583724976 -0.40850830078125
3.83403897285461 -0.40850830078125
3.83403897285461 -0.40850830078125
3.83448433876038 -0.4085693359375
3.83454775810242 -0.4085693359375
3.83461141586304 -0.4085693359375
3.83467507362366 -0.40863037109375
3.8347384929657 -0.40863037109375
3.83480215072632 -0.40863037109375
3.83486557006836 -0.40863037109375
3.8349289894104 -0.40863037109375
3.8349289894104 -0.40863037109375
3.8349289894104 -0.40863037109375
3.83543682098389 -0.40869140625
3.83550024032593 -0.40869140625
3.8363242149353 -0.40869140625
3.8363242149353 -0.40869140625
3.83638739585876 -0.40869140625
3.83638739585876 -0.40869140625
3.83638739585876 -0.40869140625
3.83638739585876 -0.40869140625
3.8368935585022 -0.40875244140625
3.83695673942566 -0.40875244140625
3.83695673942566 -0.40875244140625
3.83695673942566 -0.40875244140625
3.83701992034912 -0.40875244140625
3.83708310127258 -0.40875244140625
3.83708310127258 -0.40875244140625
3.83708310127258 -0.4088134765625
3.83803009986877 -0.4088134765625
3.83809304237366 -0.4088134765625
3.83815622329712 -0.4088134765625
3.838219165802 -0.4088134765625
3.83828234672546 -0.4088134765625
3.83828234672546 -0.40887451171875
3.83859729766846 -0.40887451171875
3.83866024017334 -0.40887451171875
3.83866024017334 -0.40887451171875
3.83872318267822 -0.40887451171875
3.83878612518311 -0.40887451171875
3.83878612518311 -0.40887451171875
3.83903789520264 -0.40887451171875
3.83903789520264 -0.40887451171875
3.83903789520264 -0.40887451171875
3.83910083770752 -0.408935546875
3.83910083770752 -0.408935546875
3.83991765975952 -0.408935546875
3.8399806022644 -0.408935546875
3.84010601043701 -0.40899658203125
3.84016895294189 -0.40899658203125
3.84016895294189 -0.40899658203125
3.84041976928711 -0.40899658203125
3.84048247337341 -0.40899658203125
3.84048247337341 -0.40899658203125
3.84048247337341 -0.40899658203125
3.84048247337341 -0.40899658203125
3.84054517745972 -0.4090576171875
3.84060788154602 -0.4090576171875
3.84060788154602 -0.4090576171875
3.84135937690735 -0.4090576171875
3.84142208099365 -0.4090576171875
3.84142208099365 -0.4090576171875
3.84142208099365 -0.4090576171875
3.842609167099 -0.40924072265625
3.84267163276672 -0.40924072265625
3.84267163276672 -0.40924072265625
3.84323287010193 -0.4093017578125
3.84329509735107 -0.4093017578125
3.84348201751709 -0.4093017578125
3.84354424476624 -0.40936279296875
3.84354424476624 -0.40936279296875
3.84354424476624 -0.40936279296875
3.84354424476624 -0.40936279296875
3.84435296058655 -0.409423828125
3.84441494941711 -0.409423828125
3.84441494941711 -0.409423828125
3.84441494941711 -0.409423828125
3.84441494941711 -0.409423828125
3.84441494941711 -0.409423828125
3.84441494941711 -0.409423828125
3.84441494941711 -0.409423828125
3.84441494941711 -0.409423828125
3.84441494941711 -0.409423828125
3.84460139274597 -0.409423828125
3.84460139274597 -0.409423828125
3.84460139274597 -0.409423828125
3.84460139274597 -0.409423828125
3.84460139274597 -0.40948486328125
3.8448498249054 -0.40948486328125
3.8448498249054 -0.40948486328125
3.8448498249054 -0.40948486328125
3.84584188461304 -0.4095458984375
3.8459038734436 -0.4095458984375
3.8459038734436 -0.4095458984375
3.8459038734436 -0.4095458984375
3.8459038734436 -0.4095458984375
3.8459038734436 -0.4095458984375
3.8459038734436 -0.4095458984375
3.8459038734436 -0.4095458984375
3.84608960151672 -0.4095458984375
3.84621334075928 -0.40960693359375
3.84627532958984 -0.40960693359375
3.8471405506134 -0.40960693359375
3.84726405143738 -0.40960693359375
3.84726405143738 -0.40960693359375
3.84769606590271 -0.40966796875
3.84775757789612 -0.40966796875
3.84775757789612 -0.40966796875
3.84775757789612 -0.40966796875
3.84781932830811 -0.40966796875
3.84781932830811 -0.40966796875
3.84781932830811 -0.40966796875
3.84781932830811 -0.40966796875
3.8480658531189 -0.40966796875
3.8480658531189 -0.40966796875
3.8480658531189 -0.40972900390625
3.84831237792969 -0.40972900390625
3.84831237792969 -0.40972900390625
3.84831237792969 -0.40972900390625
3.84831237792969 -0.40972900390625
3.8483738899231 -0.40972900390625
3.8484354019165 -0.40972900390625
3.84886622428894 -0.40972900390625
3.84892773628235 -0.4097900390625
3.84892773628235 -0.4097900390625
3.84898924827576 -0.4097900390625
3.84898924827576 -0.4097900390625
3.84898924827576 -0.4097900390625
3.84898924827576 -0.4097900390625
3.84898924827576 -0.4097900390625
3.84941935539246 -0.4097900390625
3.84941935539246 -0.4097900390625
3.84948086738586 -0.4097900390625
3.84954214096069 -0.4097900390625
3.8496036529541 -0.4097900390625
3.8496036529541 -0.4097900390625
3.8496036529541 -0.40985107421875
3.84978771209717 -0.40985107421875
3.85052371025085 -0.40985107421875
3.85058498382568 -0.40985107421875
3.85058498382568 -0.40985107421875
3.85058498382568 -0.40985107421875
3.85058498382568 -0.40985107421875
3.85058498382568 -0.40985107421875
3.85082983970642 -0.40985107421875
3.85089111328125 -0.40985107421875
3.85095238685608 -0.409912109375
3.85101366043091 -0.409912109375
3.85107469558716 -0.409912109375
3.85247993469238 -0.409912109375
3.85247993469238 -0.40997314453125
3.85247993469238 -0.40997314453125
3.85247993469238 -0.40997314453125
3.85247993469238 -0.40997314453125
3.85247993469238 -0.40997314453125
3.85247993469238 -0.40997314453125
3.85266304016113 -0.40997314453125
3.85266304016113 -0.40997314453125
3.85266304016113 -0.40997314453125
3.8528459072113 -0.40997314453125
3.8528459072113 -0.40997314453125
3.85357642173767 -0.41009521484375
3.85369825363159 -0.41009521484375
3.85375905036926 -0.41009521484375
3.85375905036926 -0.41009521484375
3.85375905036926 -0.41009521484375
3.85375905036926 -0.41009521484375
3.85375905036926 -0.41015625
3.85424518585205 -0.41015625
3.85424518585205 -0.41015625
3.85424518585205 -0.41015625
3.85430598258972 -0.41015625
3.85436677932739 -0.41015625
3.85436677932739 -0.41015625
3.85436677932739 -0.41015625
3.85588240623474 -0.41021728515625
3.85594296455383 -0.41021728515625
3.85600352287292 -0.41021728515625
3.85606384277344 -0.41021728515625
3.85612440109253 -0.41021728515625
3.85618495941162 -0.41021728515625
3.85642671585083 -0.4102783203125
3.85648727416992 -0.4102783203125
3.85654759407043 -0.4102783203125
3.85654759407043 -0.4102783203125
3.85654759407043 -0.4102783203125
3.85654759407043 -0.4102783203125
3.85672879219055 -0.4102783203125
3.85672879219055 -0.4102783203125
3.85672879219055 -0.4102783203125
3.85672879219055 -0.4102783203125
3.85672879219055 -0.4102783203125
3.85672879219055 -0.4102783203125
3.85672879219055 -0.4102783203125
3.85672879219055 -0.4102783203125
3.85672879219055 -0.4102783203125
3.85672879219055 -0.4102783203125
3.8571515083313 -0.410400390625
3.8571515083313 -0.410400390625
3.8571515083313 -0.410400390625
3.8571515083313 -0.410400390625
3.8571515083313 -0.410400390625
3.8571515083313 -0.410400390625
3.8571515083313 -0.410400390625
3.8571515083313 -0.410400390625
3.85757374763489 -0.410400390625
3.85781478881836 -0.410400390625
3.85781478881836 -0.410400390625
3.85781478881836 -0.410400390625
3.85805559158325 -0.410400390625
3.85823631286621 -0.410400390625
3.85823631286621 -0.410400390625
3.85823631286621 -0.410400390625
3.85823631286621 -0.41046142578125
3.85823631286621 -0.41046142578125
3.85823631286621 -0.41046142578125
3.8584771156311 -0.41046142578125
3.85871767997742 -0.41046142578125
3.85877776145935 -0.41046142578125
3.85883784294128 -0.41046142578125
3.85883784294128 -0.41046142578125
3.85883784294128 -0.41046142578125
3.85883784294128 -0.41046142578125
3.85883784294128 -0.41046142578125
3.85955858230591 -0.4105224609375
3.85961866378784 -0.4105224609375
3.85961866378784 -0.4105224609375
3.85961866378784 -0.4105224609375
3.85961866378784 -0.4105224609375
3.86003828048706 -0.41058349609375
3.86009836196899 -0.41058349609375
3.86015820503235 -0.41058349609375
3.8606972694397 -0.41058349609375
3.86075711250305 -0.41058349609375
3.86075711250305 -0.41058349609375
3.86081695556641 -0.41058349609375
3.86081695556641 -0.41058349609375
3.86081695556641 -0.41058349609375
3.86081695556641 -0.41058349609375
3.86087679862976 -0.41058349609375
3.86087679862976 -0.41058349609375
3.86117577552795 -0.41058349609375
3.86117577552795 -0.41058349609375
3.86117577552795 -0.41058349609375
3.86117577552795 -0.41058349609375
3.86117577552795 -0.41058349609375
3.86117577552795 -0.41064453125
3.86117577552795 -0.41064453125
3.86159420013428 -0.41064453125
3.86171364784241 -0.41064453125
3.86177325248718 -0.41064453125
3.86183309555054 -0.41064453125
3.86183309555054 -0.41064453125
3.86183309555054 -0.41064453125
3.86183309555054 -0.41064453125
3.86183309555054 -0.41064453125
3.86195230484009 -0.41064453125
3.86195230484009 -0.41064453125
3.86195230484009 -0.41064453125
3.86195230484009 -0.41064453125
3.86195230484009 -0.41064453125
3.86195230484009 -0.41064453125
3.86290621757507 -0.41064453125
3.86308479309082 -0.41064453125
3.8631443977356 -0.41070556640625
3.86320376396179 -0.41070556640625
3.86326336860657 -0.41070556640625
3.86344194412231 -0.41070556640625
3.86344194412231 -0.41070556640625
3.86344194412231 -0.41070556640625
3.86344194412231 -0.41070556640625
3.86344194412231 -0.41070556640625
3.86344194412231 -0.41070556640625
3.86344194412231 -0.41070556640625
3.86373901367188 -0.41070556640625
3.86373901367188 -0.41070556640625
3.8645703792572 -0.41082763671875
3.86468911170959 -0.41082763671875
3.86474847793579 -0.41082763671875
3.8648669719696 -0.41082763671875
3.8648669719696 -0.41082763671875
3.86498546600342 -0.41082763671875
3.86504459381104 -0.41082763671875
3.86504459381104 -0.41082763671875
3.86504459381104 -0.41082763671875
3.86504459381104 -0.41082763671875
3.86504459381104 -0.41082763671875
3.86569595336914 -0.41082763671875
3.86652374267578 -0.410888671875
3.86658263206482 -0.410888671875
3.86658263206482 -0.410888671875
3.86664175987244 -0.410888671875
3.86664175987244 -0.410888671875
3.86681890487671 -0.410888671875
3.86681890487671 -0.410888671875
3.86687779426575 -0.410888671875
3.86693692207336 -0.410888671875
3.86693692207336 -0.410888671875
3.86693692207336 -0.410888671875
3.86693692207336 -0.410888671875
3.86693692207336 -0.410888671875
3.86693692207336 -0.410888671875
3.86693692207336 -0.410888671875
3.8671727180481 -0.41094970703125
3.86723184585571 -0.41094970703125
3.86723184585571 -0.41094970703125
3.86723184585571 -0.41094970703125
3.86723184585571 -0.41094970703125
3.86723184585571 -0.41094970703125
3.86723184585571 -0.41094970703125
3.86723184585571 -0.41094970703125
3.86723184585571 -0.41094970703125
3.86776208877563 -0.41094970703125
3.86776208877563 -0.41094970703125
3.86776208877563 -0.41094970703125
3.86776208877563 -0.41094970703125
3.86776208877563 -0.41094970703125
3.86776208877563 -0.41094970703125
3.86776208877563 -0.41094970703125
3.86776208877563 -0.41094970703125
3.86776208877563 -0.41094970703125
3.86793875694275 -0.41094970703125
3.86799740791321 -0.4110107421875
3.86799740791321 -0.4110107421875
3.86799740791321 -0.4110107421875
3.86799740791321 -0.4110107421875
3.86799740791321 -0.4110107421875
3.86799740791321 -0.4110107421875
3.86858558654785 -0.4110107421875
3.86864447593689 -0.4110107421875
3.86864447593689 -0.4110107421875
3.86864447593689 -0.4110107421875
3.86864447593689 -0.4110107421875
3.86864447593689 -0.4110107421875
3.86864447593689 -0.4110107421875
3.86934900283813 -0.4110107421875
3.86934900283813 -0.41107177734375
3.86934900283813 -0.41107177734375
3.86934900283813 -0.41107177734375
3.86934900283813 -0.41107177734375
3.86934900283813 -0.41107177734375
3.86934900283813 -0.41107177734375
3.86934900283813 -0.41107177734375
3.86934900283813 -0.41107177734375
3.86934900283813 -0.41107177734375
3.87087202072144 -0.4112548828125
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{ClF5}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.86193981915712,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.635165405273437, ymax=0.0302459716796875,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c6)}
]
\addplot [ultra thick, brown, dashed]
table {%
1.49136173725128 0
2.23804616928101 -0.000244140625
2.51851391792297 -0.000244140625
2.52762985229492 -0.000244140625
2.53781914710999 -0.000244140625
2.54900336265564 -0.000244140625
2.55750727653503 -0.000244140625
2.56937384605408 -0.000244140625
2.57403135299683 -0.000244140625
2.70500802993774 -0.00030517578125
2.74896287918091 -0.00030517578125
2.75434827804565 -0.00030517578125
2.76342797279358 -0.00030517578125
2.76641273498535 -0.00030517578125
2.77451705932617 -0.00030517578125
2.77742671966553 -0.00030517578125
2.82282161712646 -0.00030517578125
2.82672262191772 -0.00030517578125
2.84385538101196 -0.00030517578125
2.84633708000183 -0.00030517578125
2.88309335708618 -0.00030517578125
2.8898618221283 -0.00030517578125
2.89209461212158 -0.00030517578125
2.90687346458435 -0.00030517578125
2.92992949485779 -0.00030517578125
2.93298077583313 -0.00030517578125
2.94987773895264 -0.00030517578125
2.99913048744202 -0.00030517578125
3.00086784362793 -0.0003662109375
3.00259804725647 -0.0003662109375
3.00774788856506 -0.0003662109375
3.01367974281311 -0.0003662109375
3.01535964012146 -0.0003662109375
3.03862023353577 -0.0003662109375
3.04296898841858 -0.0003662109375
3.04727482795715 -0.0003662109375
3.1010594367981 -0.0003662109375
3.10720992088318 -0.0003662109375
3.11092615127563 -0.0003662109375
3.12090277671814 -0.0003662109375
3.12450432777405 -0.0003662109375
3.15075635910034 -0.00042724609375
3.15228843688965 -0.00042724609375
3.15624618530273 -0.00042724609375
3.15896534919739 -0.00042724609375
3.16790771484375 -0.00042724609375
3.18808436393738 -0.00042724609375
3.19672870635986 -0.00042724609375
3.26787543296814 -0.00042724609375
3.290034532547 -0.00042724609375
3.31111788749695 -0.00048828125
3.3562171459198 -0.00048828125
3.35812520980835 -0.00048828125
3.35945606231689 -0.00048828125
3.36135005950928 -0.00048828125
3.36361193656921 -0.00048828125
3.38596367835999 -0.00048828125
3.39602494239807 -0.00048828125
3.39759254455566 -0.00048828125
3.39811372756958 -0.00054931640625
3.4072208404541 -0.00054931640625
3.41060853004456 -0.00054931640625
3.44263648986816 -0.00054931640625
3.44560408592224 -0.00054931640625
3.44607090950012 -0.00054931640625
3.44700288772583 -0.00054931640625
3.4622483253479 -0.00054931640625
3.51864552497864 -0.00067138671875
3.53744125366211 -0.00067138671875
3.63154530525208 -0.0040283203125
3.66086554527283 -0.01055908203125
3.68340730667114 -0.01165771484375
3.6984486579895 -0.01190185546875
3.71222877502441 -0.012451171875
3.72672724723816 -0.01287841796875
3.73878049850464 -0.0130615234375
3.74647855758667 -0.013427734375
3.77202820777893 -0.013916015625
3.7839035987854 -0.01458740234375
3.80556869506836 -0.01544189453125
3.82033276557922 -0.01556396484375
3.85205268859863 -0.0164794921875
3.86093664169312 -0.0166015625
3.86587357521057 -0.01666259765625
3.87133932113647 -0.0167236328125
3.88890933990479 -0.01690673828125
3.89453744888306 -0.0169677734375
3.93089818954468 -0.01727294921875
3.93721699714661 -0.01739501953125
3.94428515434265 -0.0174560546875
3.94655060768127 -0.01751708984375
3.96618866920471 -0.0179443359375
3.98833584785461 -0.01800537109375
3.99317169189453 -0.01800537109375
3.99690556526184 -0.01806640625
4.00065088272095 -0.01812744140625
4.00830221176147 -0.0181884765625
4.01123189926147 -0.0181884765625
4.01865911483765 -0.01824951171875
4.03064012527466 -0.01824951171875
4.03594970703125 -0.01837158203125
4.05739974975586 -0.0184326171875
4.06182909011841 -0.01849365234375
4.1060209274292 -0.01910400390625
4.13299560546875 -0.019287109375
4.14429378509521 -0.0194091796875
4.15639781951904 -0.01947021484375
4.17193126678467 -0.01959228515625
4.18026924133301 -0.01959228515625
4.18588209152222 -0.0196533203125
4.21966314315796 -0.02056884765625
4.235755443573 -0.02081298828125
4.24360847473145 -0.02093505859375
4.24578380584717 -0.02099609375
4.25088310241699 -0.0211181640625
4.26133441925049 -0.021484375
4.27160930633545 -0.02203369140625
4.28838348388672 -0.0224609375
4.2967529296875 -0.02264404296875
4.32951974868774 -0.0284423828125
4.33175134658813 -0.0343017578125
4.34279775619507 -0.03570556640625
4.34558916091919 -0.0362548828125
4.34692001342773 -0.0389404296875
4.3587532043457 -0.039794921875
4.3648509979248 -0.04071044921875
4.37280178070068 -0.0423583984375
4.3817286491394 -0.04345703125
4.3891658782959 -0.04437255859375
4.39369821548462 -0.04498291015625
4.40380668640137 -0.047607421875
4.40527820587158 -0.04864501953125
4.41151857376099 -0.04931640625
4.42245864868164 -0.05029296875
4.42448949813843 -0.05096435546875
4.4263162612915 -0.0518798828125
4.43795680999756 -0.05364990234375
4.44128656387329 -0.05426025390625
4.45325708389282 -0.0546875
4.46422100067139 -0.05523681640625
4.46576929092407 -0.05548095703125
4.47935914993286 -0.05621337890625
4.48304510116577 -0.056396484375
4.49064683914185 -0.0565185546875
4.50955200195312 -0.0589599609375
4.52258777618408 -0.05975341796875
4.52925062179565 -0.0599365234375
4.53655862808228 -0.06024169921875
4.54845094680786 -0.06146240234375
4.56267356872559 -0.06439208984375
4.5689172744751 -0.0653076171875
4.58028602600098 -0.066162109375
4.58884286880493 -0.06756591796875
4.59803485870361 -0.0687255859375
4.60109281539917 -0.06927490234375
4.60907125473022 -0.07061767578125
4.61517143249512 -0.07159423828125
4.62801074981689 -0.0743408203125
4.63178873062134 -0.0751953125
4.63603639602661 -0.0758056640625
4.64199924468994 -0.076416015625
4.64919853210449 -0.07720947265625
4.65876483917236 -0.0787353515625
4.67081165313721 -0.08209228515625
4.6746129989624 -0.08355712890625
4.67790794372559 -0.0843505859375
4.68819713592529 -0.08746337890625
4.69687175750732 -0.09039306640625
4.70670080184937 -0.09222412109375
4.71499156951904 -0.09539794921875
4.7188835144043 -0.0968017578125
4.72357892990112 -0.09814453125
4.73181438446045 -0.09954833984375
4.74104928970337 -0.102294921875
4.74979829788208 -0.10638427734375
4.75998497009277 -0.1097412109375
4.7679271697998 -0.11212158203125
4.77596712112427 -0.117919921875
4.78150415420532 -0.1199951171875
4.78864192962646 -0.12408447265625
4.80074453353882 -0.13336181640625
4.80362796783447 -0.13702392578125
4.80792713165283 -0.138427734375
4.81461381912231 -0.140869140625
4.81984663009644 -0.14453125
4.82110071182251 -0.14593505859375
4.82359170913696 -0.14691162109375
4.82961273193359 -0.15228271484375
4.83167791366577 -0.15374755859375
4.84120321273804 -0.1607666015625
4.84332609176636 -0.162109375
4.84945631027222 -0.16436767578125
4.85152149200439 -0.1649169921875
4.85405683517456 -0.16534423828125
4.86008644104004 -0.16766357421875
4.8669900894165 -0.16973876953125
4.86854457855225 -0.1705322265625
4.87178897857666 -0.1712646484375
4.87480068206787 -0.171875
4.8782057762146 -0.17425537109375
4.88072776794434 -0.1746826171875
4.8839225769043 -0.1759033203125
4.89028120040894 -0.17877197265625
4.89360094070435 -0.179443359375
4.89826965332031 -0.18011474609375
4.90123462677002 -0.1806640625
4.90524530410767 -0.1817626953125
4.9095721244812 -0.18267822265625
4.91136026382446 -0.18328857421875
4.91501951217651 -0.18408203125
4.91713762283325 -0.1844482421875
4.92180109024048 -0.1851806640625
4.92408275604248 -0.1856689453125
4.92726230621338 -0.18621826171875
4.92898464202881 -0.18658447265625
4.9362621307373 -0.18896484375
4.93991851806641 -0.1895751953125
4.94406795501709 -0.19036865234375
4.94932651519775 -0.19281005859375
4.95220613479614 -0.1937255859375
4.95692682266235 -0.19482421875
4.96060848236084 -0.1961669921875
4.96483469009399 -0.19696044921875
4.96672344207764 -0.19775390625
4.97338676452637 -0.2034912109375
4.97499942779541 -0.2052001953125
4.98139715194702 -0.2119140625
4.98418951034546 -0.21337890625
4.98733568191528 -0.2147216796875
4.99147415161133 -0.2161865234375
4.994215965271 -0.21722412109375
4.99669122695923 -0.2176513671875
4.99976539611816 -0.21820068359375
5.00746202468872 -0.22442626953125
5.00969314575195 -0.22601318359375
5.01307344436646 -0.22686767578125
5.01692485809326 -0.22735595703125
5.01902914047241 -0.22802734375
5.02374219894409 -0.23040771484375
5.02602243423462 -0.2310791015625
5.03938627243042 -0.249267578125
5.04348421096802 -0.25482177734375
5.04772281646729 -0.25933837890625
5.05135345458984 -0.26055908203125
5.05521392822266 -0.26226806640625
5.05883598327637 -0.263427734375
5.06365585327148 -0.26507568359375
5.06667995452881 -0.266357421875
5.07191133499146 -0.267822265625
5.07873249053955 -0.27838134765625
5.08169651031494 -0.2802734375
5.08681535720825 -0.28253173828125
5.0885968208313 -0.2835693359375
5.09578609466553 -0.294921875
5.09764242172241 -0.29736328125
5.10085964202881 -0.30059814453125
5.10653400421143 -0.3179931640625
5.1095986366272 -0.32379150390625
5.1140570640564 -0.3292236328125
5.11825132369995 -0.33251953125
5.11966800689697 -0.3338623046875
5.12553310394287 -0.34271240234375
5.12773942947388 -0.34564208984375
5.12965106964111 -0.346923828125
5.13288688659668 -0.348876953125
5.13714504241943 -0.3524169921875
5.13911056518555 -0.35400390625
5.14190101623535 -0.35687255859375
5.14346742630005 -0.3587646484375
5.14772891998291 -0.361572265625
5.1506028175354 -0.36431884765625
5.15272569656372 -0.3658447265625
5.15625238418579 -0.37384033203125
5.15969944000244 -0.37689208984375
5.16370964050293 -0.37921142578125
5.16540765762329 -0.38037109375
5.17215299606323 -0.39410400390625
5.17348337173462 -0.3990478515625
5.17674207687378 -0.4005126953125
5.18053007125854 -0.4012451171875
5.18156051635742 -0.40155029296875
5.18908023834229 -0.41064453125
5.19169950485229 -0.41387939453125
5.19607400894165 -0.41632080078125
5.19997978210449 -0.41766357421875
5.20342445373535 -0.4188232421875
5.20744848251343 -0.42132568359375
5.20976448059082 -0.4222412109375
5.21181726455688 -0.42291259765625
5.21445989608765 -0.42388916015625
5.21877717971802 -0.42620849609375
5.2204270362854 -0.42724609375
5.22235727310181 -0.427978515625
5.22656393051147 -0.43243408203125
5.22889041900635 -0.4334716796875
5.23194360733032 -0.4342041015625
5.23497533798218 -0.43524169921875
5.23667573928833 -0.4359130859375
5.23924207687378 -0.43731689453125
5.24102306365967 -0.43829345703125
5.24273252487183 -0.43878173828125
5.24482107162476 -0.44036865234375
5.24855947494507 -0.4427490234375
5.2533597946167 -0.4498291015625
5.25430870056152 -0.45355224609375
5.25611591339111 -0.45465087890625
5.25789928436279 -0.455810546875
5.25963449478149 -0.457763671875
5.26226854324341 -0.46002197265625
5.26322174072266 -0.4609375
5.26558208465576 -0.464599609375
5.26745796203613 -0.46685791015625
5.26872062683105 -0.46759033203125
5.27028751373291 -0.46893310546875
5.27087211608887 -0.46929931640625
5.27488708496094 -0.47857666015625
5.27714157104492 -0.482177734375
5.27818632125854 -0.48297119140625
5.27943181991577 -0.4833984375
5.28236389160156 -0.4873046875
5.28328561782837 -0.4881591796875
5.28385066986084 -0.48846435546875
5.28592395782471 -0.49017333984375
5.28982305526733 -0.49359130859375
5.29091358184814 -0.49432373046875
5.29155302047729 -0.49468994140625
5.2938175201416 -0.4984130859375
5.29466247558594 -0.4990234375
5.29612970352173 -0.4996337890625
5.29792881011963 -0.500244140625
5.30120801925659 -0.50238037109375
5.30178928375244 -0.502685546875
5.3033971786499 -0.50323486328125
5.30395793914795 -0.50347900390625
5.30622577667236 -0.505859375
5.30751323699951 -0.50677490234375
5.30832529067993 -0.507080078125
5.31005573272705 -0.507568359375
5.31085872650146 -0.50799560546875
5.31219434738159 -0.50836181640625
5.31280565261841 -0.50885009765625
5.31372594833374 -0.50921630859375
5.31460237503052 -0.509521484375
5.31638336181641 -0.51025390625
5.31823015213013 -0.51055908203125
5.31882905960083 -0.5108642578125
5.31938695907593 -0.51141357421875
5.31990528106689 -0.51171875
5.32111978530884 -0.51202392578125
5.32153224945068 -0.51226806640625
5.32202482223511 -0.5125732421875
5.32340669631958 -0.51348876953125
5.3253698348999 -0.513916015625
5.32774114608765 -0.51580810546875
5.32834482192993 -0.51611328125
5.32891368865967 -0.51629638671875
5.33006477355957 -0.5164794921875
5.33137273788452 -0.5167236328125
5.33284425735474 -0.51708984375
5.33318519592285 -0.5172119140625
5.33556842803955 -0.51806640625
5.33596324920654 -0.51837158203125
5.33659791946411 -0.51873779296875
5.33754301071167 -0.51898193359375
5.33832311630249 -0.51922607421875
5.33922481536865 -0.5194091796875
5.33959245681763 -0.51953125
5.34359359741211 -0.52252197265625
5.34390258789062 -0.52337646484375
5.34589290618896 -0.52423095703125
5.34647035598755 -0.52435302734375
5.3476128578186 -0.52471923828125
5.3488187789917 -0.5252685546875
5.34980773925781 -0.5255126953125
5.35064125061035 -0.52569580078125
5.3519082069397 -0.52593994140625
5.3529748916626 -0.5263671875
5.35351419448853 -0.526611328125
5.35445785522461 -0.52691650390625
5.35642147064209 -0.52880859375
5.35700798034668 -0.52935791015625
5.35751008987427 -0.5296630859375
5.35834980010986 -0.52978515625
5.35992288589478 -0.53143310546875
5.36062383651733 -0.53216552734375
5.3614559173584 -0.53240966796875
5.36188077926636 -0.5325927734375
5.36264085769653 -0.5328369140625
5.36319065093994 -0.5333251953125
5.36386394500732 -0.533447265625
5.36471796035767 -0.5345458984375
5.36543941497803 -0.53472900390625
5.36617612838745 -0.5361328125
5.36744928359985 -0.536376953125
5.36896133422852 -0.53680419921875
5.36932373046875 -0.53704833984375
5.37056112289429 -0.5372314453125
5.37199640274048 -0.5374755859375
5.37337732315063 -0.53778076171875
5.38151025772095 -0.53961181640625
5.38201332092285 -0.5399169921875
5.38486766815186 -0.54022216796875
5.38535594940186 -0.54046630859375
5.38579034805298 -0.54052734375
5.38620471954346 -0.5406494140625
5.38654708862305 -0.54071044921875
5.39060831069946 -0.54180908203125
5.39087867736816 -0.5419921875
5.39120149612427 -0.54205322265625
5.39173936843872 -0.542236328125
5.39214277267456 -0.54229736328125
5.39252805709839 -0.54241943359375
5.39326095581055 -0.542724609375
5.39369630813599 -0.54278564453125
5.39388370513916 -0.5428466796875
5.39441823959351 -0.54290771484375
5.39494705200195 -0.54302978515625
5.39517784118652 -0.54302978515625
5.3956127166748 -0.5430908203125
5.39628982543945 -0.5433349609375
5.3968300819397 -0.54339599609375
5.39757871627808 -0.54345703125
5.39779043197632 -0.54351806640625
5.39809799194336 -0.5435791015625
5.39901924133301 -0.54425048828125
5.39938831329346 -0.54437255859375
5.39985704421997 -0.54443359375
5.39995241165161 -0.54443359375
5.40183305740356 -0.5457763671875
5.40219068527222 -0.5458984375
5.40227842330933 -0.54595947265625
5.40380334854126 -0.54669189453125
5.40389919281006 -0.54669189453125
5.40445899963379 -0.54705810546875
5.4049243927002 -0.547119140625
5.40546607971191 -0.5472412109375
5.40614652633667 -0.54730224609375
5.40663719177246 -0.54730224609375
5.40733671188354 -0.54754638671875
5.40750122070312 -0.547607421875
5.40790557861328 -0.54766845703125
5.40815496444702 -0.54766845703125
5.4092264175415 -0.54791259765625
5.41004276275635 -0.5479736328125
5.41054105758667 -0.54815673828125
5.41082286834717 -0.5482177734375
5.41124057769775 -0.54827880859375
5.41151523590088 -0.54833984375
5.4117546081543 -0.54840087890625
5.41247749328613 -0.54876708984375
5.41306686401367 -0.54876708984375
5.41434669494629 -0.54913330078125
5.41498851776123 -0.54937744140625
5.41631603240967 -0.54974365234375
5.4170880317688 -0.54986572265625
5.41747856140137 -0.5499267578125
5.41782379150391 -0.54998779296875
5.41838598251343 -0.550048828125
5.41862773895264 -0.550048828125
5.41896200180054 -0.55010986328125
5.4194483757019 -0.55023193359375
5.42016553878784 -0.55029296875
5.42058277130127 -0.55029296875
5.42114782333374 -0.55047607421875
5.4229621887207 -0.55120849609375
5.42312145233154 -0.55126953125
5.42385339736938 -0.5513916015625
5.4242000579834 -0.55145263671875
5.42503976821899 -0.551513671875
5.42579030990601 -0.55157470703125
5.42642831802368 -0.55169677734375
5.42692899703979 -0.5517578125
5.42705917358398 -0.55181884765625
5.42766284942627 -0.5518798828125
5.42816257476807 -0.55194091796875
5.42863988876343 -0.552001953125
5.42976188659668 -0.55218505859375
5.43016719818115 -0.55224609375
5.43040418624878 -0.55224609375
5.43065214157104 -0.55230712890625
5.43103551864624 -0.5523681640625
5.4322361946106 -0.552490234375
5.43238067626953 -0.552490234375
5.43531370162964 -0.5548095703125
5.43544483184814 -0.5550537109375
5.43558311462402 -0.55511474609375
5.43609571456909 -0.55517578125
5.43720197677612 -0.5552978515625
5.43925523757935 -0.556640625
5.43965339660645 -0.55780029296875
5.44020175933838 -0.55792236328125
5.4407958984375 -0.5579833984375
5.44124889373779 -0.55804443359375
5.44317531585693 -0.559326171875
5.44351959228516 -0.5595703125
5.44541263580322 -0.56121826171875
5.44637250900269 -0.56146240234375
5.4473237991333 -0.56170654296875
5.44819736480713 -0.56207275390625
5.44905376434326 -0.56292724609375
5.45012903213501 -0.56353759765625
5.45065879821777 -0.5638427734375
5.45182180404663 -0.5640869140625
5.45272159576416 -0.56439208984375
5.45316410064697 -0.5648193359375
5.45400762557983 -0.565185546875
5.45487403869629 -0.5654296875
5.45534610748291 -0.5655517578125
5.45680332183838 -0.56683349609375
5.45761108398438 -0.5675048828125
5.45871496200562 -0.5677490234375
5.4600043296814 -0.568359375
5.46022129058838 -0.5684814453125
5.46165895462036 -0.56927490234375
5.46259260177612 -0.56939697265625
5.46356439590454 -0.56976318359375
5.46386337280273 -0.5699462890625
5.46399450302124 -0.57000732421875
5.4645357131958 -0.57012939453125
5.46576499938965 -0.5704345703125
5.46627426147461 -0.57061767578125
5.46659183502197 -0.5706787109375
5.46817588806152 -0.57171630859375
5.46849966049194 -0.57177734375
5.46929168701172 -0.5718994140625
5.46945953369141 -0.57196044921875
5.46969842910767 -0.572021484375
5.47086143493652 -0.5723876953125
5.47134160995483 -0.572509765625
5.47207164764404 -0.572509765625
5.47288227081299 -0.57269287109375
5.47314071655273 -0.57275390625
5.47365474700928 -0.57281494140625
5.47455549240112 -0.572998046875
5.47545766830444 -0.573486328125
5.47556495666504 -0.5738525390625
5.47623872756958 -0.573974609375
5.47702836990356 -0.574462890625
5.47746706008911 -0.57464599609375
5.47805547714233 -0.57489013671875
5.4783787727356 -0.57501220703125
5.47869348526001 -0.57513427734375
5.47955226898193 -0.57568359375
5.47971343994141 -0.5758056640625
5.48024129867554 -0.57598876953125
5.48050975799561 -0.576171875
5.48121023178101 -0.577392578125
5.48131799697876 -0.5775146484375
5.48187828063965 -0.57781982421875
5.48224306106567 -0.57806396484375
5.48261070251465 -0.5782470703125
5.48301362991333 -0.57855224609375
5.48343324661255 -0.57867431640625
5.48385238647461 -0.57879638671875
5.48419570922852 -0.5791015625
5.48444938659668 -0.5792236328125
5.48478507995605 -0.57928466796875
5.48504829406738 -0.57940673828125
5.48537921905518 -0.57952880859375
5.48575973510742 -0.5797119140625
5.48589468002319 -0.57977294921875
5.48632431030273 -0.57989501953125
5.48658752441406 -0.5799560546875
5.48691034317017 -0.580078125
5.48762464523315 -0.580810546875
5.48801898956299 -0.5809326171875
5.48811626434326 -0.5809326171875
5.48884105682373 -0.58111572265625
5.48892831802368 -0.5811767578125
5.48907899856567 -0.58123779296875
5.48925399780273 -0.58123779296875
5.48937892913818 -0.581298828125
5.48968839645386 -0.58135986328125
5.48975896835327 -0.58135986328125
5.49030685424805 -0.5816650390625
5.49090480804443 -0.5819091796875
5.49109268188477 -0.5819091796875
5.49141931533813 -0.5819091796875
5.49156475067139 -0.58203125
5.49199151992798 -0.58209228515625
5.49257326126099 -0.58233642578125
5.49286794662476 -0.58233642578125
5.49292230606079 -0.5823974609375
5.49316787719727 -0.5823974609375
5.49356698989868 -0.58251953125
5.49422979354858 -0.58258056640625
5.4945273399353 -0.582763671875
5.49473333358765 -0.582763671875
5.49494314193726 -0.58282470703125
5.49535703659058 -0.58294677734375
5.49547624588013 -0.5830078125
5.49561786651611 -0.5830078125
5.49583578109741 -0.5830078125
5.49650621414185 -0.583251953125
5.49737882614136 -0.58392333984375
5.49764966964722 -0.58392333984375
5.49818658828735 -0.583984375
5.49847316741943 -0.583984375
5.49879264831543 -0.5841064453125
5.4988808631897 -0.5841064453125
5.49927616119385 -0.58428955078125
5.49946594238281 -0.58428955078125
5.49955081939697 -0.5843505859375
5.49996757507324 -0.5843505859375
5.50017738342285 -0.58441162109375
5.50046300888062 -0.58441162109375
5.50059032440186 -0.58447265625
5.50063705444336 -0.58447265625
5.5007905960083 -0.58447265625
5.50150585174561 -0.58465576171875
5.50165367126465 -0.58465576171875
5.50181484222412 -0.584716796875
5.50197219848633 -0.58477783203125
5.50241470336914 -0.5848388671875
5.50258255004883 -0.58489990234375
5.50276279449463 -0.58489990234375
5.50292539596558 -0.5849609375
5.50346374511719 -0.5849609375
5.50376892089844 -0.58502197265625
5.50409412384033 -0.5850830078125
5.50426578521729 -0.5850830078125
5.50558423995972 -0.58563232421875
5.50588369369507 -0.585693359375
5.50598812103271 -0.585693359375
5.50626277923584 -0.5858154296875
5.50653600692749 -0.5858154296875
5.50663471221924 -0.5858154296875
5.5067834854126 -0.58587646484375
5.50712013244629 -0.58587646484375
5.50723886489868 -0.5859375
5.50742292404175 -0.5859375
5.5075306892395 -0.58599853515625
5.50837230682373 -0.58624267578125
5.50859832763672 -0.5863037109375
5.50883388519287 -0.58636474609375
5.50926446914673 -0.58636474609375
5.5096607208252 -0.58642578125
5.51022720336914 -0.58660888671875
5.51045370101929 -0.58660888671875
5.51074600219727 -0.58660888671875
5.51096963882446 -0.586669921875
5.51136064529419 -0.58673095703125
5.51142740249634 -0.58673095703125
5.51196241378784 -0.5867919921875
5.51211023330688 -0.5867919921875
5.51288175582886 -0.58697509765625
5.51330804824829 -0.58697509765625
5.51344013214111 -0.5870361328125
5.51360130310059 -0.5870361328125
5.51397895812988 -0.58709716796875
5.51425933837891 -0.587158203125
5.51433134078979 -0.587158203125
5.51507091522217 -0.58734130859375
5.51534938812256 -0.58746337890625
5.51555442810059 -0.58746337890625
5.51584482192993 -0.5875244140625
5.5161452293396 -0.58758544921875
5.51624059677124 -0.58758544921875
5.51638746261597 -0.58758544921875
5.51657772064209 -0.587646484375
5.51669025421143 -0.587646484375
5.51675081253052 -0.587646484375
5.51759576797485 -0.587890625
5.51781463623047 -0.587890625
5.51806735992432 -0.58795166015625
5.51842832565308 -0.58795166015625
5.51898622512817 -0.5880126953125
5.51907825469971 -0.58807373046875
5.51938676834106 -0.58807373046875
5.51956272125244 -0.588134765625
5.51976346969604 -0.588134765625
5.52003002166748 -0.58819580078125
5.52033567428589 -0.5882568359375
5.52057266235352 -0.5882568359375
5.52122163772583 -0.58831787109375
5.52141141891479 -0.58831787109375
5.52166509628296 -0.58837890625
5.52207612991333 -0.58837890625
5.52211141586304 -0.58837890625
5.52235412597656 -0.58843994140625
5.52266311645508 -0.58843994140625
5.52300357818604 -0.58856201171875
5.52331972122192 -0.588623046875
5.52403259277344 -0.588623046875
5.52455186843872 -0.58868408203125
5.52485656738281 -0.5887451171875
5.52505922317505 -0.58880615234375
5.52531433105469 -0.58880615234375
5.52571821212769 -0.5888671875
5.52592277526855 -0.58892822265625
5.52603673934937 -0.58892822265625
5.52628087997437 -0.58892822265625
5.52723026275635 -0.589111328125
5.52751111984253 -0.5892333984375
5.52761316299438 -0.5892333984375
5.52795219421387 -0.58941650390625
5.52824783325195 -0.58941650390625
5.52843952178955 -0.5894775390625
5.52862882614136 -0.5894775390625
5.52883577346802 -0.5894775390625
5.52980756759644 -0.58966064453125
5.52988719940186 -0.5897216796875
5.53063488006592 -0.58990478515625
5.53086280822754 -0.5899658203125
5.53103685379028 -0.5899658203125
5.53200101852417 -0.5902099609375
5.53201103210449 -0.5902099609375
5.53216695785522 -0.5902099609375
5.53234004974365 -0.59027099609375
5.53248023986816 -0.59027099609375
5.53256988525391 -0.59033203125
5.53269720077515 -0.59033203125
5.53281164169312 -0.59033203125
5.53340721130371 -0.5904541015625
5.5336742401123 -0.5904541015625
5.53374671936035 -0.59051513671875
5.5342698097229 -0.590576171875
5.53481388092041 -0.590576171875
5.53489017486572 -0.590576171875
5.53516626358032 -0.59063720703125
5.53540182113647 -0.59063720703125
5.5364031791687 -0.5909423828125
5.5366063117981 -0.5909423828125
5.53684377670288 -0.5909423828125
5.5369873046875 -0.59100341796875
5.53733682632446 -0.59100341796875
5.53743743896484 -0.59100341796875
5.53758096694946 -0.591064453125
5.5382080078125 -0.591064453125
5.53829097747803 -0.59112548828125
5.53853988647461 -0.5911865234375
5.53884506225586 -0.5911865234375
5.53933334350586 -0.5911865234375
5.53943347930908 -0.5911865234375
5.5398473739624 -0.59124755859375
5.54026794433594 -0.59130859375
5.54058742523193 -0.59130859375
5.54073238372803 -0.59136962890625
5.54085493087769 -0.59136962890625
5.54178142547607 -0.5916748046875
5.54192876815796 -0.59173583984375
5.54201221466064 -0.59173583984375
5.54235601425171 -0.59173583984375
5.54248809814453 -0.591796875
5.54284524917603 -0.591796875
5.54309558868408 -0.59185791015625
5.5434398651123 -0.59185791015625
5.54369926452637 -0.5919189453125
5.54397392272949 -0.5919189453125
5.54430770874023 -0.59197998046875
5.54453706741333 -0.59197998046875
5.54476737976074 -0.592041015625
5.54510545730591 -0.592041015625
5.54525375366211 -0.592041015625
5.54575109481812 -0.59210205078125
5.5460958480835 -0.59210205078125
5.54610061645508 -0.5921630859375
5.54621696472168 -0.5921630859375
5.54723310470581 -0.592529296875
5.54742908477783 -0.59259033203125
5.54770469665527 -0.59259033203125
5.54783391952515 -0.5926513671875
5.54804277420044 -0.59271240234375
5.54826021194458 -0.59271240234375
5.54874086380005 -0.5927734375
5.54883623123169 -0.5927734375
5.55133056640625 -0.59490966796875
5.55142545700073 -0.59521484375
5.55154037475586 -0.59521484375
5.5516037940979 -0.59521484375
5.55166578292847 -0.59521484375
5.55175733566284 -0.59527587890625
5.55235767364502 -0.595458984375
5.55245018005371 -0.595458984375
5.55254888534546 -0.595458984375
5.55335140228271 -0.59576416015625
5.55353593826294 -0.59576416015625
5.55359315872192 -0.5958251953125
5.5537109375 -0.5958251953125
5.55380058288574 -0.5958251953125
5.55441999435425 -0.59600830078125
5.55477237701416 -0.59600830078125
5.55508470535278 -0.5960693359375
5.55516242980957 -0.5960693359375
5.55525064468384 -0.5960693359375
5.55556344985962 -0.59613037109375
5.55563735961914 -0.59613037109375
5.55609512329102 -0.59613037109375
5.55620956420898 -0.59613037109375
5.55633878707886 -0.59619140625
5.556396484375 -0.59619140625
5.55646181106567 -0.59619140625
5.55663537979126 -0.59619140625
5.5566930770874 -0.59619140625
5.55697870254517 -0.59625244140625
5.55766487121582 -0.59637451171875
5.55806875228882 -0.59637451171875
5.55845642089844 -0.59637451171875
5.55847358703613 -0.596435546875
5.55855369567871 -0.596435546875
5.55960988998413 -0.5968017578125
5.55965518951416 -0.59686279296875
5.55985736846924 -0.596923828125
5.56002998352051 -0.596923828125
5.56036472320557 -0.596923828125
5.56077575683594 -0.59698486328125
5.5608434677124 -0.59698486328125
5.56098222732544 -0.59698486328125
5.56108808517456 -0.59698486328125
5.56118154525757 -0.5970458984375
5.56147813796997 -0.5970458984375
5.5617356300354 -0.5970458984375
5.56185817718506 -0.5970458984375
5.56224775314331 -0.59710693359375
5.56232976913452 -0.59710693359375
5.56242275238037 -0.59710693359375
5.56387853622437 -0.5986328125
5.56406211853027 -0.59881591796875
5.56414270401001 -0.59881591796875
5.56460475921631 -0.59881591796875
5.56488990783691 -0.598876953125
5.56499862670898 -0.598876953125
5.56524801254272 -0.598876953125
5.5653600692749 -0.598876953125
5.56552886962891 -0.598876953125
5.56686973571777 -0.59979248046875
5.56702184677124 -0.599853515625
5.56721591949463 -0.59991455078125
5.56738185882568 -0.59991455078125
5.56757211685181 -0.59991455078125
5.56769800186157 -0.59991455078125
5.56817722320557 -0.60003662109375
5.56830024719238 -0.60003662109375
5.56860542297363 -0.60003662109375
5.56958103179932 -0.60028076171875
5.56966543197632 -0.600341796875
5.56975650787354 -0.600341796875
5.57003021240234 -0.60040283203125
5.5701470375061 -0.60040283203125
5.57023572921753 -0.60040283203125
5.57040071487427 -0.60040283203125
5.57045555114746 -0.60040283203125
5.57060241699219 -0.60040283203125
5.57078695297241 -0.60040283203125
5.57082653045654 -0.60040283203125
5.57097244262695 -0.6004638671875
5.57111692428589 -0.6004638671875
5.57147121429443 -0.60052490234375
5.57169580459595 -0.60052490234375
5.57175636291504 -0.60052490234375
5.57185649871826 -0.60052490234375
5.57202768325806 -0.60052490234375
5.57250928878784 -0.6005859375
5.57260799407959 -0.6005859375
5.57269382476807 -0.6005859375
5.57286214828491 -0.6005859375
5.57307720184326 -0.60064697265625
5.57322549819946 -0.60064697265625
5.57338666915894 -0.60064697265625
5.57354116439819 -0.60064697265625
5.57360696792603 -0.60064697265625
5.57392024993896 -0.60064697265625
5.57396411895752 -0.60064697265625
5.57401275634766 -0.60064697265625
5.57414484024048 -0.60064697265625
5.5743579864502 -0.6007080078125
5.57443857192993 -0.6007080078125
5.57452440261841 -0.6007080078125
5.57464122772217 -0.6007080078125
5.57480907440186 -0.6007080078125
5.57511854171753 -0.6007080078125
5.57544994354248 -0.60076904296875
5.5755410194397 -0.60076904296875
5.5756402015686 -0.60076904296875
5.57596588134766 -0.60076904296875
5.57607173919678 -0.60076904296875
5.57622051239014 -0.60076904296875
5.57622718811035 -0.60076904296875
5.57643699645996 -0.600830078125
5.57673406600952 -0.600830078125
5.57686996459961 -0.600830078125
5.57705402374268 -0.600830078125
5.57721948623657 -0.600830078125
5.57727479934692 -0.600830078125
5.5775032043457 -0.60089111328125
5.57754802703857 -0.60089111328125
5.57789850234985 -0.6009521484375
5.57834672927856 -0.6009521484375
5.57841682434082 -0.6009521484375
5.57854175567627 -0.60101318359375
5.57870674133301 -0.60101318359375
5.57884883880615 -0.60101318359375
5.57892560958862 -0.60101318359375
5.57915115356445 -0.60101318359375
5.57927703857422 -0.60101318359375
5.57952737808228 -0.60107421875
5.57965087890625 -0.60107421875
5.57978248596191 -0.60107421875
5.57998466491699 -0.60107421875
5.58013677597046 -0.60107421875
5.58016157150269 -0.60107421875
5.5811243057251 -0.6015625
5.58117246627808 -0.60162353515625
5.58130645751953 -0.6016845703125
5.58142042160034 -0.6016845703125
5.58165168762207 -0.6016845703125
5.58183574676514 -0.6016845703125
5.58196449279785 -0.60174560546875
5.58206129074097 -0.60174560546875
5.58223628997803 -0.60174560546875
5.58243846893311 -0.60174560546875
5.58251333236694 -0.60174560546875
5.58334732055664 -0.60198974609375
5.58351182937622 -0.60211181640625
5.58358764648438 -0.60211181640625
5.58387279510498 -0.60211181640625
5.58411312103271 -0.6021728515625
5.5843243598938 -0.6021728515625
5.58441591262817 -0.6021728515625
5.58454704284668 -0.6021728515625
5.58470296859741 -0.6021728515625
5.58478355407715 -0.6021728515625
5.5848536491394 -0.6021728515625
5.58509492874146 -0.6021728515625
5.58518552780151 -0.6021728515625
5.58533573150635 -0.60223388671875
5.58551597595215 -0.60223388671875
5.58566284179688 -0.60223388671875
5.5858588218689 -0.60223388671875
5.58596706390381 -0.60223388671875
5.58634185791016 -0.602294921875
5.5864634513855 -0.602294921875
5.58655595779419 -0.602294921875
5.58665466308594 -0.602294921875
5.58691453933716 -0.602294921875
5.5870885848999 -0.602294921875
5.58724164962769 -0.602294921875
5.58744049072266 -0.602294921875
5.58754730224609 -0.60235595703125
5.58761548995972 -0.60235595703125
5.58791399002075 -0.60235595703125
5.58798122406006 -0.60235595703125
5.58829402923584 -0.60235595703125
5.58843994140625 -0.60235595703125
5.58869981765747 -0.6024169921875
5.58886766433716 -0.6024169921875
5.58899736404419 -0.6024169921875
5.58940458297729 -0.60247802734375
5.5896635055542 -0.6025390625
5.58974504470825 -0.6025390625
5.58980989456177 -0.6025390625
5.59002542495728 -0.6025390625
5.59007930755615 -0.6025390625
5.59025526046753 -0.6025390625
5.59036588668823 -0.6025390625
5.59047603607178 -0.6025390625
5.59052848815918 -0.6025390625
5.59076738357544 -0.6025390625
5.59083414077759 -0.6025390625
5.59097671508789 -0.60260009765625
5.59110021591187 -0.60260009765625
5.59113121032715 -0.60260009765625
5.59120941162109 -0.60260009765625
5.5913028717041 -0.60260009765625
5.5913987159729 -0.60260009765625
5.59152555465698 -0.60260009765625
5.59174108505249 -0.60260009765625
5.59181880950928 -0.60260009765625
5.59190130233765 -0.60260009765625
5.59202909469604 -0.60260009765625
5.59210586547852 -0.60260009765625
5.59242677688599 -0.6026611328125
5.59261417388916 -0.6026611328125
5.59265184402466 -0.6026611328125
5.59295892715454 -0.60272216796875
5.59307861328125 -0.60272216796875
5.59312295913696 -0.60272216796875
5.59324073791504 -0.602783203125
5.59389925003052 -0.60284423828125
5.5939302444458 -0.60284423828125
5.59396600723267 -0.60284423828125
5.5940375328064 -0.60284423828125
5.59412288665771 -0.60284423828125
5.59480333328247 -0.60296630859375
5.59483528137207 -0.60296630859375
5.59523820877075 -0.60302734375
5.59532403945923 -0.60302734375
5.59536933898926 -0.60302734375
5.59553384780884 -0.60302734375
5.59560537338257 -0.60302734375
5.59585857391357 -0.60302734375
5.59592819213867 -0.60302734375
5.59622001647949 -0.60308837890625
5.59625959396362 -0.60308837890625
5.59643220901489 -0.60308837890625
5.59668159484863 -0.60308837890625
5.59671592712402 -0.60308837890625
5.59689950942993 -0.60308837890625
5.59704542160034 -0.60308837890625
5.59713459014893 -0.6031494140625
};
\addplot [ultra thick, blue]
table {%
-inf 0
-inf -0.000244140625
-inf -0.000244140625
-inf -0.000244140625
-inf -0.000244140625
-inf -0.000244140625
-inf -0.000244140625
0.30103000998497 -0.00030517578125
0.30103000998497 -0.0003662109375
0.30103000998497 -0.0003662109375
0.30103000998497 -0.0003662109375
0.30103000998497 -0.0003662109375
0.30103000998497 -0.0003662109375
0.30103000998497 -0.0003662109375
0.30103000998497 -0.00042724609375
0.30103000998497 -0.00042724609375
0.30103000998497 -0.00042724609375
0.30103000998497 -0.00042724609375
0.30103000998497 -0.00042724609375
0.30103000998497 -0.00042724609375
0.30103000998497 -0.00042724609375
0.477121233940125 -0.00042724609375
0.477121233940125 -0.00042724609375
0.477121233940125 -0.00042724609375
0.477121233940125 -0.00042724609375
0.477121233940125 -0.00042724609375
0.477121233940125 -0.00048828125
0.477121233940125 -0.00048828125
0.698970019817352 -0.00048828125
0.698970019817352 -0.00048828125
0.698970019817352 -0.00048828125
0.698970019817352 -0.00048828125
0.698970019817352 -0.00048828125
0.698970019817352 -0.00054931640625
0.698970019817352 -0.00054931640625
0.698970019817352 -0.00054931640625
0.778151273727417 -0.00054931640625
0.778151273727417 -0.00054931640625
0.778151273727417 -0.00054931640625
0.778151273727417 -0.0006103515625
0.84509801864624 -0.0006103515625
0.84509801864624 -0.0006103515625
0.903090000152588 -0.0006103515625
0.903090000152588 -0.0006103515625
1 -0.00067138671875
1 -0.00067138671875
1 -0.00067138671875
1 -0.00067138671875
1.04139268398285 -0.000732421875
1.04139268398285 -0.000732421875
1.04139268398285 -0.000732421875
1.34242272377014 -0.00372314453125
1.53147888183594 -0.00982666015625
1.61278390884399 -0.01043701171875
1.66275787353516 -0.01116943359375
1.73239374160767 -0.011962890625
1.74818801879883 -0.0123291015625
1.80618000030518 -0.01312255859375
1.83884906768799 -0.01409912109375
1.84509801864624 -0.01434326171875
1.85125839710236 -0.01446533203125
1.85733246803284 -0.0145263671875
1.86923170089722 -0.01470947265625
1.87506127357483 -0.01483154296875
1.88081359863281 -0.014892578125
1.89209461212158 -0.01507568359375
1.90848505496979 -0.015625
1.9395192861557 -0.015869140625
1.94448268413544 -0.01593017578125
1.95424246788025 -0.01611328125
1.96378779411316 -0.0162353515625
1.97772359848022 -0.0166015625
2.00432133674622 -0.01678466796875
2.01283717155457 -0.01678466796875
2.02118921279907 -0.016845703125
2.02118921279907 -0.01690673828125
2.05307841300964 -0.01739501953125
2.06818580627441 -0.0177001953125
2.07188200950623 -0.0177001953125
2.0827853679657 -0.017822265625
2.11394333839417 -0.017822265625
2.11394333839417 -0.01788330078125
2.12385153770447 -0.0179443359375
2.13033366203308 -0.01800537109375
2.13672065734863 -0.01806640625
2.14301490783691 -0.01806640625
2.14301490783691 -0.01812744140625
2.14921903610229 -0.0181884765625
2.1553361415863 -0.01824951171875
2.18752074241638 -0.01824951171875
2.21484375 -0.01849365234375
2.21484375 -0.01849365234375
2.24054932594299 -0.01861572265625
2.24054932594299 -0.01873779296875
2.24054932594299 -0.018798828125
2.24551272392273 -0.018798828125
2.24551272392273 -0.01885986328125
2.24551272392273 -0.01885986328125
2.26007127761841 -0.01885986328125
2.26481771469116 -0.0189208984375
2.27415776252747 -0.01898193359375
2.27875351905823 -0.01904296875
2.27875351905823 -0.01904296875
2.28780174255371 -0.01910400390625
2.290034532547 -0.0191650390625
2.30319595336914 -0.01922607421875
2.33645963668823 -0.01953125
2.33645963668823 -0.01959228515625
2.43136382102966 -0.0238037109375
2.44404482841492 -0.03057861328125
2.46239805221558 -0.03118896484375
2.46982192993164 -0.03216552734375
2.47275638580322 -0.0328369140625
2.50515007972717 -0.03387451171875
2.51321768760681 -0.0352783203125
2.53019976615906 -0.03662109375
2.53781914710999 -0.03936767578125
2.55509448051453 -0.04107666015625
2.56937384605408 -0.042236328125
2.58771085739136 -0.04400634765625
2.59549617767334 -0.04486083984375
2.62428212165833 -0.045654296875
2.63144373893738 -0.0465087890625
2.65513849258423 -0.04986572265625
2.6618127822876 -0.05133056640625
2.70243048667908 -0.052978515625
2.76492309570312 -0.05633544921875
2.76715588569641 -0.05712890625
2.7723217010498 -0.0577392578125
2.78031730651855 -0.05841064453125
2.78746056556702 -0.05877685546875
2.80550098419189 -0.0596923828125
2.81557774543762 -0.0601806640625
2.85551905632019 -0.06317138671875
2.85913825035095 -0.06390380859375
2.86272764205933 -0.0643310546875
2.8709888458252 -0.0648193359375
2.87621784210205 -0.06549072265625
2.88817954063416 -0.0660400390625
2.9074113368988 -0.067626953125
2.90955591201782 -0.06805419921875
2.92788338661194 -0.06878662109375
2.93500328063965 -0.06982421875
2.94299960136414 -0.07049560546875
2.95375967025757 -0.0712890625
2.97220277786255 -0.07440185546875
2.97726631164551 -0.07568359375
2.97909283638 -0.07623291015625
2.9876663684845 -0.0770263671875
2.99651169776917 -0.07781982421875
3.01325869560242 -0.08221435546875
3.01535964012146 -0.08416748046875
3.01911640167236 -0.0853271484375
3.03901743888855 -0.09051513671875
3.04844188690186 -0.09271240234375
3.06069779396057 -0.094970703125
3.06707096099854 -0.0963134765625
3.0827853679657 -0.102783203125
3.08849048614502 -0.10540771484375
3.09482049942017 -0.10736083984375
3.10754919052124 -0.1090087890625
3.12417817115784 -0.1202392578125
3.13385820388794 -0.12548828125
3.13893389701843 -0.12799072265625
3.15806078910828 -0.13568115234375
3.16106843948364 -0.1387939453125
3.16286301612854 -0.13983154296875
3.17172646522522 -0.14404296875
3.17666983604431 -0.1455078125
3.19117140769958 -0.1474609375
3.19368100166321 -0.1488037109375
3.19810700416565 -0.15020751953125
3.2161660194397 -0.16204833984375
3.21748399734497 -0.1666259765625
3.22375535964966 -0.16802978515625
3.22582602500916 -0.1690673828125
3.23248791694641 -0.1695556640625
3.23426413536072 -0.170166015625
3.24054932594299 -0.1724853515625
3.25042009353638 -0.17327880859375
3.25163817405701 -0.1737060546875
3.25358033180237 -0.17437744140625
3.25599575042725 -0.1746826171875
3.27276968955994 -0.1807861328125
3.27485036849976 -0.182373046875
3.27623200416565 -0.1827392578125
3.28533220291138 -0.1854248046875
3.28712964057922 -0.18609619140625
3.2920343875885 -0.18658447265625
3.29446625709534 -0.18719482421875
3.29534721374512 -0.1876220703125
3.31175374984741 -0.1932373046875
3.31659936904907 -0.1959228515625
3.31785440444946 -0.19659423828125
3.32221937179565 -0.197509765625
3.32837963104248 -0.19903564453125
3.33203434944153 -0.1998291015625
3.33785843849182 -0.200927734375
3.33945155143738 -0.20147705078125
3.34103870391846 -0.2017822265625
3.34517765045166 -0.20318603515625
3.35024809837341 -0.20428466796875
3.35564303398132 -0.20562744140625
3.35850596427917 -0.206298828125
3.36229395866394 -0.207275390625
3.36567521095276 -0.20855712890625
3.36865878105164 -0.2098388671875
3.37327980995178 -0.2110595703125
3.37438178062439 -0.2117919921875
3.37984919548035 -0.21392822265625
3.38471174240112 -0.21685791015625
3.38596367835999 -0.218017578125
3.3907585144043 -0.21978759765625
3.39287281036377 -0.22027587890625
3.39932751655579 -0.2249755859375
3.40466260910034 -0.22576904296875
3.4075608253479 -0.226318359375
3.4126284122467 -0.22821044921875
3.4186327457428 -0.22900390625
3.42291808128357 -0.23175048828125
3.42732381820679 -0.2327880859375
3.43071985244751 -0.233642578125
3.4421660900116 -0.2568359375
3.44684767723083 -0.2662353515625
3.45101833343506 -0.26763916015625
3.45178651809692 -0.2684326171875
3.46059727668762 -0.2901611328125
3.4631462097168 -0.29632568359375
3.46701574325562 -0.29827880859375
3.4708514213562 -0.29998779296875
3.47392463684082 -0.30181884765625
3.48172926902771 -0.314453125
3.48387241363525 -0.318359375
3.48756265640259 -0.319580078125
3.49009895324707 -0.32159423828125
3.49471092224121 -0.32501220703125
3.49582171440125 -0.32623291015625
3.49899935722351 -0.32745361328125
3.50826025009155 -0.34039306640625
3.51161599159241 -0.343505859375
3.51268434524536 -0.3448486328125
3.5156090259552 -0.346435546875
3.51838231086731 -0.34912109375
3.52361631393433 -0.35260009765625
3.52517437934875 -0.35400390625
3.52801632881165 -0.35565185546875
3.53160667419434 -0.358154296875
3.53466057777405 -0.36004638671875
3.53554725646973 -0.36102294921875
3.53794503211975 -0.36236572265625
3.54270100593567 -0.37164306640625
3.54394388198853 -0.37359619140625
3.54728221893311 -0.375
3.54802060127258 -0.37579345703125
3.55364036560059 -0.38250732421875
3.55581974983215 -0.38421630859375
3.55642318725586 -0.384765625
3.56205487251282 -0.388427734375
3.56336236000061 -0.38983154296875
3.56667327880859 -0.392333984375
3.5679669380188 -0.3936767578125
3.56995892524719 -0.395263671875
3.57333588600159 -0.3970947265625
3.58172225952148 -0.41912841796875
3.58376550674438 -0.42822265625
3.58534789085388 -0.42974853515625
3.58602428436279 -0.43048095703125
3.58939099311829 -0.43316650390625
3.59006118774414 -0.43426513671875
3.59406089782715 -0.4356689453125
3.59780478477478 -0.44195556640625
3.60184288024902 -0.4442138671875
3.60292768478394 -0.44500732421875
3.60605883598328 -0.44573974609375
3.60691857337952 -0.44610595703125
3.60884690284729 -0.44647216796875
3.61426424980164 -0.44940185546875
3.61637043952942 -0.4505615234375
3.61836194992065 -0.45123291015625
3.62397241592407 -0.45770263671875
3.62572383880615 -0.462646484375
3.63255858421326 -0.4683837890625
3.63477945327759 -0.47027587890625
3.63658809661865 -0.4710693359375
3.6391875743866 -0.47265625
3.64018321037292 -0.47344970703125
3.64226651191711 -0.47442626953125
3.64305758476257 -0.47491455078125
3.64552044868469 -0.47589111328125
3.64659976959229 -0.47650146484375
3.64767622947693 -0.4771728515625
3.64836001396179 -0.47772216796875
3.65147185325623 -0.47821044921875
3.65253639221191 -0.4786376953125
3.65321254730225 -0.479248046875
3.6580114364624 -0.4801025390625
3.65906000137329 -0.480712890625
3.66029620170593 -0.481201171875
3.66454792022705 -0.48236083984375
3.66511178016663 -0.482666015625
3.66642427444458 -0.4835205078125
3.67098760604858 -0.48760986328125
3.67154312133789 -0.488525390625
3.67209792137146 -0.48883056640625
3.6749529838562 -0.48944091796875
3.67559504508972 -0.48968505859375
3.67623615264893 -0.49005126953125
3.67715048789978 -0.4906005859375
3.67915534973145 -0.491943359375
3.68024492263794 -0.492431640625
3.68286681175232 -0.4930419921875
3.68421673774719 -0.4937744140625
3.68663620948792 -0.494384765625
3.68761801719666 -0.49517822265625
3.68833088874817 -0.495361328125
3.69037342071533 -0.49578857421875
3.69469285011292 -0.497802734375
3.69556927680969 -0.49920654296875
3.69626903533936 -0.49957275390625
3.69696760177612 -0.50018310546875
3.69783926010132 -0.50067138671875
3.6984486579895 -0.50091552734375
3.7031192779541 -0.5037841796875
3.70363521575928 -0.5045166015625
3.70415043830872 -0.50482177734375
3.70509362220764 -0.50567626953125
3.70825099945068 -0.50628662109375
3.71239709854126 -0.5091552734375
3.71281790733337 -0.509765625
3.71382641792297 -0.51007080078125
3.71800327301025 -0.5115966796875
3.71841859817505 -0.511962890625
3.72172832489014 -0.51287841796875
3.72214007377625 -0.51318359375
3.72288060188293 -0.51385498046875
3.72867846488953 -0.5185546875
3.72884058952332 -0.51898193359375
3.73013591766357 -0.51947021484375
3.73150825500488 -0.520263671875
3.73207187652588 -0.5203857421875
3.7332775592804 -0.52056884765625
3.73335790634155 -0.52069091796875
3.73383903503418 -0.52081298828125
3.73607754707336 -0.5211181640625
3.73655581474304 -0.52130126953125
3.7374312877655 -0.5213623046875
3.74272513389587 -0.5224609375
3.7428035736084 -0.52264404296875
3.7428822517395 -0.522705078125
3.74460577964783 -0.523193359375
3.74632263183594 -0.52374267578125
3.74671196937561 -0.52386474609375
3.74748945236206 -0.52392578125
3.74857568740845 -0.52410888671875
3.74942708015442 -0.52423095703125
3.75135612487793 -0.52447509765625
3.75212526321411 -0.52459716796875
3.75296974182129 -0.52471923828125
3.75304651260376 -0.5247802734375
3.75732016563416 -0.52520751953125
3.75777554512024 -0.525390625
3.75830626487732 -0.5255126953125
3.75891184806824 -0.52569580078125
3.75944113731384 -0.5257568359375
3.76012086868286 -0.5260009765625
3.76064872741699 -0.526123046875
3.76140165328979 -0.5264892578125
3.76566863059998 -0.527099609375
3.76596641540527 -0.52716064453125
3.77407884597778 -0.53448486328125
3.77466297149658 -0.53790283203125
3.77539205551147 -0.5380859375
3.77590155601501 -0.5382080078125
3.77677392959595 -0.53851318359375
3.77742671966553 -0.53857421875
3.77858543395996 -0.5389404296875
3.77909111976624 -0.53900146484375
3.78795623779297 -0.5418701171875
3.78802680969238 -0.54229736328125
3.78816843032837 -0.54241943359375
3.7885217666626 -0.54248046875
3.79077768325806 -0.542724609375
3.79148006439209 -0.54302978515625
3.79155039787292 -0.5430908203125
3.79218149185181 -0.543212890625
3.79246163368225 -0.54327392578125
3.79427886009216 -0.54345703125
3.79434871673584 -0.54351806640625
3.79469704627991 -0.5435791015625
3.79532384872437 -0.54376220703125
3.79719829559326 -0.54425048828125
3.7972674369812 -0.5443115234375
3.79754447937012 -0.54437255859375
3.79789042472839 -0.54449462890625
3.79851245880127 -0.544677734375
3.79858160018921 -0.54473876953125
3.79954719543457 -0.544921875
3.79961609840393 -0.544921875
3.80133509635925 -0.5452880859375
3.80140376091003 -0.54534912109375
3.80174660682678 -0.54541015625
3.80208921432495 -0.5455322265625
3.80215787887573 -0.5455322265625
3.80277371406555 -0.54559326171875
3.80284214019775 -0.545654296875
3.8040030002594 -0.5458984375
3.80407118797302 -0.54595947265625
3.80407118797302 -0.54595947265625
3.80760264396667 -0.5482177734375
3.80814337730408 -0.54852294921875
3.80821084976196 -0.548583984375
3.80908823013306 -0.5487060546875
3.80908823013306 -0.54876708984375
3.81097149848938 -0.548828125
3.81103849411011 -0.54888916015625
3.81130695343018 -0.5489501953125
3.8113739490509 -0.5489501953125
3.81164193153381 -0.54901123046875
3.81170892715454 -0.549072265625
3.81217765808105 -0.54913330078125
3.81217765808105 -0.5491943359375
3.81344747543335 -0.54937744140625
3.81378102302551 -0.5494384765625
3.81424760818481 -0.54949951171875
3.81524562835693 -0.54962158203125
3.8153121471405 -0.5496826171875
3.81557774543762 -0.54974365234375
3.81564426422119 -0.54974365234375
3.81590962409973 -0.5498046875
3.82079243659973 -0.551513671875
3.82118582725525 -0.55169677734375
3.8212513923645 -0.55169677734375
3.82216811180115 -0.55181884765625
3.82223343849182 -0.5518798828125
3.82256031036377 -0.55194091796875
3.82288694381714 -0.55206298828125
3.82295227050781 -0.5521240234375
3.82295227050781 -0.5521240234375
3.82386541366577 -0.55224609375
3.82419085502625 -0.55224609375
3.82691669464111 -0.55267333984375
3.82704591751099 -0.55303955078125
3.82704591751099 -0.5531005859375
3.82988238334656 -0.5535888671875
3.82994675636292 -0.5537109375
3.83020353317261 -0.5537109375
3.8347384929657 -0.55828857421875
3.83505606651306 -0.5596923828125
3.83550024032593 -0.559814453125
3.83733582496643 -0.5601806640625
3.83765149116516 -0.5604248046875
3.83790397644043 -0.560546875
3.83815622329712 -0.5606689453125
3.84010601043701 -0.561279296875
3.84041976928711 -0.561767578125
3.84073328971863 -0.56201171875
3.84185981750488 -0.5621337890625
3.84223461151123 -0.56231689453125
3.84422850608826 -0.56304931640625
3.84491181373596 -0.5633544921875
3.84516000747681 -0.5634765625
3.84726405143738 -0.56402587890625
3.84751105308533 -0.56414794921875
3.84972643852234 -0.5653076171875
3.85027861595154 -0.56549072265625
3.85101366043091 -0.565673828125
3.8513195514679 -0.5657958984375
3.85296773910522 -0.56585693359375
3.85406303405762 -0.56658935546875
3.85582184791565 -0.56683349609375
3.85612440109253 -0.56695556640625
3.85660815238953 -0.567138671875
3.85745310783386 -0.5672607421875
3.85835671424866 -0.5675048828125
3.85949850082397 -0.567626953125
3.85991859436035 -0.5677490234375
3.86063742637634 -0.56793212890625
3.86135506629944 -0.5679931640625
3.86201214790344 -0.568115234375
3.86409568786621 -0.56842041015625
3.86415505409241 -0.56854248046875
3.86569595336914 -0.5692138671875
3.8669958114624 -0.5694580078125
3.86729073524475 -0.569580078125
3.8689968585968 -0.56976318359375
3.8703453540802 -0.57037353515625
3.87157297134399 -0.570556640625
3.87209796905518 -0.57073974609375
3.87320423126221 -0.5709228515625
3.87465572357178 -0.57122802734375
3.87563991546631 -0.57135009765625
3.87898111343384 -0.573486328125
3.8792679309845 -0.57403564453125
3.8803563117981 -0.57440185546875
3.88069915771484 -0.57452392578125
3.8808708190918 -0.5745849609375
3.88189792633057 -0.5748291015625
3.88292264938354 -0.5750732421875
3.88417196273804 -0.575439453125
3.8857569694519 -0.575927734375
3.88598275184631 -0.57623291015625
3.88620853424072 -0.57647705078125
3.88722324371338 -0.5765380859375
3.88744854927063 -0.57666015625
3.88958168029785 -0.57916259765625
3.89159321784973 -0.57977294921875
3.8918719291687 -0.579833984375
3.89209461212158 -0.57989501953125
3.89215040206909 -0.5799560546875
3.8935399055481 -0.58056640625
3.89359521865845 -0.58062744140625
3.8950355052948 -0.58135986328125
3.89509081840515 -0.5814208984375
3.89536714553833 -0.58148193359375
3.89542245864868 -0.58154296875
3.89575386047363 -0.58160400390625
3.89740705490112 -0.58172607421875
3.89762711524963 -0.581787109375
3.89768195152283 -0.58184814453125
3.89861559867859 -0.582275390625
3.89872527122498 -0.58233642578125
3.89878010749817 -0.5823974609375
3.89883470535278 -0.5823974609375
3.89905405044556 -0.5823974609375
3.89954686164856 -0.5826416015625
3.89960169792175 -0.5826416015625
3.89965629577637 -0.5826416015625
3.90107679367065 -0.5831298828125
3.90113115310669 -0.58319091796875
3.90140390396118 -0.583251953125
3.90140390396118 -0.58331298828125
3.90145826339722 -0.58331298828125
3.90151286125183 -0.5833740234375
3.90200281143188 -0.58343505859375
3.90493178367615 -0.58477783203125
3.90504002571106 -0.5849609375
3.90504002571106 -0.5849609375
3.90595769882202 -0.58563232421875
3.90611934661865 -0.585693359375
3.90617322921753 -0.585693359375
3.9074113368988 -0.5858154296875
3.9074649810791 -0.58587646484375
3.90757250785828 -0.5859375
3.90896725654602 -0.5860595703125
3.90912795066833 -0.58612060546875
3.90918159484863 -0.58612060546875
3.91030406951904 -0.58642578125
3.91035747528076 -0.5865478515625
3.9104642868042 -0.5865478515625
3.91057109832764 -0.58660888671875
3.91083765029907 -0.586669921875
3.91089105606079 -0.586669921875
3.91254091262817 -0.587158203125
3.91270017623901 -0.58721923828125
3.91275334358215 -0.58721923828125
3.91280651092529 -0.58721923828125
3.91328382492065 -0.58734130859375
3.91333699226379 -0.58740234375
3.91338992118835 -0.58740234375
3.91518878936768 -0.58770751953125
3.9153470993042 -0.5877685546875
3.91539978981018 -0.58782958984375
3.91545271873474 -0.58782958984375
3.91582179069519 -0.587890625
3.91587448120117 -0.587890625
3.91587448120117 -0.58795166015625
3.91771554946899 -0.5885009765625
3.9177680015564 -0.58868408203125
3.91829252243042 -0.58880615234375
3.91834497451782 -0.58880615234375
3.91839742660522 -0.5888671875
3.91844964027405 -0.5888671875
3.91892099380493 -0.5888671875
3.91897344589233 -0.58892822265625
3.91902565956116 -0.58892822265625
3.91902565956116 -0.58892822265625
3.91949653625488 -0.5889892578125
3.91949653625488 -0.5889892578125
3.91954874992371 -0.5889892578125
3.92267346382141 -0.590087890625
3.92272543907166 -0.5902099609375
3.92329573631287 -0.59033203125
3.92339944839478 -0.59039306640625
3.92345118522644 -0.59039306640625
3.92407250404358 -0.59051513671875
3.92412424087524 -0.590576171875
3.92417597770691 -0.590576171875
3.92515730857849 -0.59063720703125
3.92520880699158 -0.59063720703125
3.92520880699158 -0.59063720703125
3.92670249938965 -0.59100341796875
3.92675399780273 -0.591064453125
3.92685675621033 -0.591064453125
3.92711353302002 -0.59112548828125
3.92757558822632 -0.59124755859375
3.92762684822083 -0.59130859375
3.92767834663391 -0.59130859375
3.92788338661194 -0.59130859375
3.92793464660645 -0.59136962890625
3.9283447265625 -0.59136962890625
3.92839574813843 -0.59136962890625
3.92957210540771 -0.5914306640625
3.92962336540222 -0.59149169921875
3.93059253692627 -0.59161376953125
3.9306435585022 -0.59161376953125
3.93069434165955 -0.5916748046875
3.9310507774353 -0.5916748046875
3.93110179901123 -0.59173583984375
3.93323421478271 -0.592041015625
3.93328475952148 -0.59210205078125
3.93363904953003 -0.59222412109375
3.9336895942688 -0.59222412109375
3.93419528007507 -0.59222412109375
3.93424582481384 -0.59228515625
3.93424582481384 -0.59234619140625
3.93429636955261 -0.59234619140625
3.93434691429138 -0.59234619140625
3.93560791015625 -0.592529296875
3.93565845489502 -0.59259033203125
3.93611145019531 -0.5926513671875
3.9361617565155 -0.59271240234375
3.93621206283569 -0.59271240234375
3.93626236915588 -0.59271240234375
3.93631267547607 -0.5927734375
3.93636298179626 -0.5927734375
3.93676495552063 -0.5927734375
3.93796896934509 -0.5928955078125
3.9380190372467 -0.5928955078125
3.93836951255798 -0.59295654296875
3.93841958045959 -0.59295654296875
3.93846964836121 -0.593017578125
3.93851971626282 -0.593017578125
3.93926954269409 -0.5931396484375
3.9393196105957 -0.5931396484375
3.9393196105957 -0.5931396484375
3.9393196105957 -0.5931396484375
3.94101428985596 -0.59393310546875
3.94106388092041 -0.593994140625
3.94136238098145 -0.59405517578125
3.94245457649231 -0.5941162109375
3.94250416755676 -0.5941162109375
3.94260334968567 -0.59417724609375
3.94290065765381 -0.59423828125
3.94314813613892 -0.59429931640625
3.94319772720337 -0.59429931640625
3.94324707984924 -0.5943603515625
3.94334602355957 -0.5943603515625
3.94364285469055 -0.5943603515625
3.94497585296631 -0.59490966796875
3.94502520561218 -0.59490966796875
3.94527149200439 -0.594970703125
3.94527149200439 -0.594970703125
3.94527149200439 -0.594970703125
3.94640302658081 -0.5950927734375
3.94650149345398 -0.59515380859375
3.94664883613586 -0.59515380859375
3.94689416885376 -0.59521484375
3.94689416885376 -0.59521484375
3.94694328308105 -0.59521484375
3.94694328308105 -0.59521484375
3.94699239730835 -0.59527587890625
3.94699239730835 -0.59527587890625
3.94718861579895 -0.59527587890625
3.94718861579895 -0.59527587890625
3.94718861579895 -0.59527587890625
3.94723749160767 -0.5953369140625
3.94758081436157 -0.5953369140625
3.94782567024231 -0.595458984375
3.94816827774048 -0.59552001953125
3.94821739196777 -0.59552001953125
3.94826626777649 -0.5955810546875
3.94831514358521 -0.5955810546875
3.94836401939392 -0.5955810546875
3.94934129714966 -0.5958251953125
3.94938993453979 -0.5958251953125
3.94938993453979 -0.5958251953125
3.95036482810974 -0.59600830078125
3.95046210289001 -0.59600830078125
3.95051097869873 -0.59600830078125
3.95055961608887 -0.5960693359375
3.95055961608887 -0.5960693359375
3.95055961608887 -0.5960693359375
3.95055961608887 -0.5960693359375
3.95075416564941 -0.5960693359375
3.95080280303955 -0.5960693359375
3.95080280303955 -0.59613037109375
3.95085144042969 -0.59613037109375
3.95317959785461 -0.59722900390625
3.95322799682617 -0.5972900390625
3.95366311073303 -0.59735107421875
3.95371127128601 -0.59735107421875
3.95375967025757 -0.597412109375
3.95380806922913 -0.597412109375
3.9538562297821 -0.597412109375
3.95390462875366 -0.59747314453125
3.95390462875366 -0.59747314453125
3.95390462875366 -0.59747314453125
3.95414590835571 -0.59747314453125
3.95414590835571 -0.5975341796875
3.95414590835571 -0.5975341796875
3.95433902740479 -0.5975341796875
3.95433902740479 -0.59759521484375
3.95433902740479 -0.59759521484375
3.95438718795776 -0.59759521484375
3.95443558692932 -0.59759521484375
3.95443558692932 -0.59765625
3.95501399040222 -0.59765625
3.9550621509552 -0.59771728515625
3.95511031150818 -0.59771728515625
3.95511031150818 -0.59771728515625
3.95511031150818 -0.59771728515625
3.95515847206116 -0.5977783203125
3.95515847206116 -0.5977783203125
3.95549535751343 -0.5977783203125
3.95549535751343 -0.5977783203125
3.95636057853699 -0.59783935546875
3.95636057853699 -0.59783935546875
3.95640850067139 -0.597900390625
3.95640850067139 -0.597900390625
3.95640850067139 -0.597900390625
3.95640850067139 -0.597900390625
3.95640850067139 -0.597900390625
3.95660066604614 -0.59796142578125
3.95660066604614 -0.59796142578125
3.95794224739075 -0.598388671875
3.95794224739075 -0.59844970703125
3.95799016952515 -0.59844970703125
3.95803809165955 -0.59844970703125
3.95808577537537 -0.5985107421875
3.95842051506042 -0.59857177734375
3.95846843719482 -0.59857177734375
3.95846843719482 -0.59857177734375
3.95937538146973 -0.5986328125
3.95937538146973 -0.5986328125
3.9607560634613 -0.59893798828125
3.96080350875854 -0.5989990234375
3.96094608306885 -0.59906005859375
3.96094608306885 -0.59906005859375
3.96127867698669 -0.59912109375
3.96132612228394 -0.59912109375
3.96132612228394 -0.59912109375
3.96137356758118 -0.59918212890625
3.96137356758118 -0.59918212890625
3.96194291114807 -0.59918212890625
3.96194291114807 -0.59918212890625
3.96194291114807 -0.59918212890625
3.96194291114807 -0.5992431640625
3.96203780174255 -0.5992431640625
3.96203780174255 -0.5992431640625
3.96203780174255 -0.5992431640625
3.96241664886475 -0.59930419921875
3.96312642097473 -0.59930419921875
3.96312642097473 -0.59930419921875
3.96312642097473 -0.599365234375
3.96312642097473 -0.599365234375
3.96312642097473 -0.599365234375
3.96312642097473 -0.599365234375
3.96345734596252 -0.59942626953125
3.96345734596252 -0.59942626953125
3.96345734596252 -0.59942626953125
3.96345734596252 -0.59942626953125
3.96345734596252 -0.5994873046875
3.96345734596252 -0.5994873046875
3.96345734596252 -0.5994873046875
3.96515464782715 -0.59967041015625
3.96515464782715 -0.59967041015625
3.96520161628723 -0.59967041015625
3.96520161628723 -0.59967041015625
3.96520161628723 -0.5997314453125
3.96520161628723 -0.5997314453125
3.96520161628723 -0.5997314453125
3.96553087234497 -0.59979248046875
3.96553087234497 -0.59979248046875
3.96553087234497 -0.599853515625
3.96557807922363 -0.599853515625
3.96557807922363 -0.599853515625
3.96557807922363 -0.599853515625
3.96585988998413 -0.599853515625
3.96585988998413 -0.599853515625
3.96585988998413 -0.599853515625
3.96585988998413 -0.59991455078125
3.96637630462646 -0.5999755859375
3.96642327308655 -0.60003662109375
3.96642327308655 -0.60003662109375
3.96642327308655 -0.60003662109375
3.96642327308655 -0.60003662109375
3.96745443344116 -0.60009765625
3.96745443344116 -0.60009765625
3.96820259094238 -0.600341796875
3.96824932098389 -0.600341796875
3.96829605102539 -0.600341796875
3.96862292289734 -0.60040283203125
3.96866965293884 -0.60040283203125
3.96871638298035 -0.60040283203125
3.96871638298035 -0.60040283203125
3.96871638298035 -0.60040283203125
3.96871638298035 -0.60040283203125
3.96871638298035 -0.60040283203125
3.96871638298035 -0.60040283203125
3.96950912475586 -0.6004638671875
3.96955561637878 -0.6004638671875
3.96955561637878 -0.6004638671875
3.96955561637878 -0.60052490234375
3.96955561637878 -0.60052490234375
3.96964883804321 -0.60052490234375
3.96983504295349 -0.60052490234375
3.96983504295349 -0.6005859375
3.96983504295349 -0.6005859375
3.97234177589417 -0.60150146484375
3.97243428230286 -0.60162353515625
3.9724805355072 -0.60162353515625
3.97252678871155 -0.60162353515625
3.97275805473328 -0.60162353515625
3.97289681434631 -0.60162353515625
3.97289681434631 -0.60162353515625
3.97294306755066 -0.6016845703125
3.97331261634827 -0.6016845703125
3.97331261634827 -0.6016845703125
3.97368192672729 -0.60174560546875
3.97372817993164 -0.60174560546875
3.97377419471741 -0.60174560546875
3.97382020950317 -0.60174560546875
3.97414302825928 -0.60174560546875
3.97418928146362 -0.601806640625
3.97418928146362 -0.601806640625
3.97418928146362 -0.601806640625
3.97418928146362 -0.601806640625
3.97423529624939 -0.601806640625
3.97423529624939 -0.601806640625
3.9744656085968 -0.601806640625
3.97501802444458 -0.6019287109375
3.97506403923035 -0.6019287109375
3.97538590431213 -0.60198974609375
3.9754319190979 -0.60198974609375
3.9754319190979 -0.60198974609375
3.9754319190979 -0.60198974609375
3.9757993221283 -0.60205078125
3.97584533691406 -0.60205078125
3.97589111328125 -0.60205078125
3.97621250152588 -0.60205078125
3.97621250152588 -0.60205078125
3.97621250152588 -0.60205078125
3.97754073143005 -0.6021728515625
3.97758650779724 -0.6021728515625
3.97758650779724 -0.6021728515625
3.97763204574585 -0.6021728515625
3.97827196121216 -0.602294921875
3.97831749916077 -0.60235595703125
3.97831749916077 -0.60235595703125
3.97854566574097 -0.6024169921875
3.97891068458557 -0.6024169921875
3.97895622253418 -0.6024169921875
3.97895622253418 -0.6024169921875
3.97922968864441 -0.6024169921875
3.98118424415588 -0.6029052734375
3.98127484321594 -0.60308837890625
3.98132014274597 -0.60308837890625
3.981365442276 -0.60308837890625
3.98141074180603 -0.6031494140625
3.98145627975464 -0.6031494140625
3.9818639755249 -0.60321044921875
3.9818639755249 -0.60321044921875
3.98236179351807 -0.60321044921875
3.98240685462952 -0.60321044921875
3.98240685462952 -0.60321044921875
3.98240685462952 -0.603271484375
3.98258781433105 -0.603271484375
3.98312997817993 -0.60345458984375
3.98317503929138 -0.60345458984375
3.98403191566467 -0.60345458984375
3.98407697677612 -0.603515625
3.9843921661377 -0.603515625
3.9843921661377 -0.603515625
3.98443722724915 -0.603515625
3.98475217819214 -0.603515625
3.98475217819214 -0.603515625
3.98497724533081 -0.60357666015625
3.98502206802368 -0.60357666015625
3.98520183563232 -0.60357666015625
3.98520183563232 -0.60357666015625
3.98524689674377 -0.60357666015625
3.98556113243103 -0.6036376953125
3.98560619354248 -0.6036376953125
3.98560619354248 -0.6036376953125
3.98578572273254 -0.6036376953125
3.98578572273254 -0.6036376953125
3.98578572273254 -0.6036376953125
3.98583054542542 -0.6036376953125
3.98609972000122 -0.60369873046875
3.98609972000122 -0.60369873046875
3.98614454269409 -0.60369873046875
3.98632383346558 -0.60369873046875
3.98632383346558 -0.60369873046875
3.98636865615845 -0.60369873046875
3.98712968826294 -0.60382080078125
3.98721933364868 -0.60382080078125
3.98726391792297 -0.60382080078125
3.98730874061584 -0.60382080078125
3.98748755455017 -0.60382080078125
3.98793435096741 -0.60394287109375
3.98793435096741 -0.60394287109375
3.9879789352417 -0.60394287109375
3.98802351951599 -0.60394287109375
3.98806810379028 -0.60394287109375
3.98811292648315 -0.60394287109375
3.98811292648315 -0.60394287109375
3.98811292648315 -0.60394287109375
3.98811292648315 -0.60394287109375
3.98829126358032 -0.60394287109375
3.98829126358032 -0.60394287109375
3.98829126358032 -0.60400390625
3.98909378051758 -0.60400390625
3.98922729492188 -0.60400390625
3.98944973945618 -0.60406494140625
3.98949432373047 -0.60406494140625
3.98949432373047 -0.60406494140625
3.98953890800476 -0.60406494140625
3.98953890800476 -0.60406494140625
3.98962783813477 -0.6041259765625
3.98967218399048 -0.6041259765625
3.99064970016479 -0.6041259765625
3.99069404602051 -0.6041259765625
3.99069404602051 -0.6041259765625
3.99087142944336 -0.60418701171875
3.99091577529907 -0.60418701171875
3.99096012115479 -0.60418701171875
3.99096012115479 -0.60418701171875
3.99113750457764 -0.60418701171875
3.99118185043335 -0.60418701171875
3.99122619628906 -0.604248046875
3.9912703037262 -0.604248046875
3.9912703037262 -0.604248046875
3.9912703037262 -0.604248046875
3.99144768714905 -0.604248046875
3.99144768714905 -0.604248046875
3.99144768714905 -0.604248046875
3.99144768714905 -0.604248046875
3.99144768714905 -0.60430908203125
3.99149179458618 -0.60430908203125
3.99153614044189 -0.60430908203125
3.99206733703613 -0.60430908203125
3.99206733703613 -0.60430908203125
3.99206733703613 -0.60430908203125
3.99206733703613 -0.60430908203125
3.99206733703613 -0.60430908203125
3.99206733703613 -0.60430908203125
3.99255347251892 -0.60443115234375
3.99259757995605 -0.60443115234375
3.99259757995605 -0.60443115234375
3.99259757995605 -0.60443115234375
3.99277448654175 -0.6044921875
3.99281859397888 -0.6044921875
3.99281859397888 -0.6044921875
3.99281859397888 -0.6044921875
3.99281859397888 -0.6044921875
3.99281859397888 -0.6044921875
3.99286270141602 -0.6044921875
3.99356842041016 -0.6044921875
3.99387693405151 -0.60455322265625
3.99392104148865 -0.6046142578125
3.9939649105072 -0.6046142578125
3.9939649105072 -0.6046142578125
3.99400901794434 -0.6046142578125
3.99400901794434 -0.6046142578125
3.99400901794434 -0.6046142578125
3.99400901794434 -0.6046142578125
3.99400901794434 -0.6046142578125
3.99400901794434 -0.60467529296875
3.99524021148682 -0.60467529296875
3.99524021148682 -0.60467529296875
3.99524021148682 -0.60467529296875
3.99524021148682 -0.60467529296875
3.99524021148682 -0.60467529296875
3.99524021148682 -0.60467529296875
3.99524021148682 -0.60467529296875
3.99524021148682 -0.60467529296875
3.99524021148682 -0.60467529296875
3.99545979499817 -0.604736328125
3.99550366401672 -0.604736328125
3.99550366401672 -0.604736328125
3.99567914009094 -0.604736328125
3.9957230091095 -0.604736328125
3.9957230091095 -0.604736328125
3.996248960495 -0.6048583984375
3.99629282951355 -0.6048583984375
3.99629282951355 -0.6048583984375
3.99629282951355 -0.6048583984375
3.99629282951355 -0.6048583984375
3.99629282951355 -0.6048583984375
3.99646782875061 -0.6048583984375
3.99646782875061 -0.6048583984375
3.99646782875061 -0.6048583984375
3.99651169776917 -0.60491943359375
3.99655556678772 -0.60491943359375
3.99655556678772 -0.60491943359375
3.99734258651733 -0.60491943359375
3.99734258651733 -0.60491943359375
3.99738645553589 -0.60491943359375
3.99743008613586 -0.60491943359375
3.99743008613586 -0.60491943359375
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{ClO3}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.66514601707459,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.402017211914062, ymax=0.0191436767578125,
ytick style={color=black},
ytick distance = 0.2,
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c7)}
]
\addplot [ultra thick, brown, dashed]
table {%
2.27184152603149 0
2.88422870635986 -0.00018310546875
3.04060244560242 -0.000244140625
3.22634220123291 -0.0003662109375
3.29292035102844 -0.00048828125
3.47668671607971 -0.001220703125
3.522705078125 -0.0013427734375
3.63988471031189 -0.00146484375
3.67246723175049 -0.00152587890625
3.71206021308899 -0.00164794921875
3.72419381141663 -0.001708984375
3.73885989189148 -0.00177001953125
3.75876045227051 -0.00189208984375
3.79063701629639 -0.00189208984375
3.84633708000183 -0.00299072265625
3.86045789718628 -0.00421142578125
3.92541527748108 -0.0054931640625
3.93696594238281 -0.006591796875
3.94645237922668 -0.00689697265625
3.96750116348267 -0.00738525390625
4.04269361495972 -0.0147705078125
4.07404804229736 -0.0203857421875
4.08849048614502 -0.0218505859375
4.10625886917114 -0.0228271484375
4.12648868560791 -0.02337646484375
4.15271615982056 -0.0262451171875
4.16858577728271 -0.0277099609375
4.18015480041504 -0.02862548828125
4.1905837059021 -0.02947998046875
4.20980978012085 -0.0306396484375
4.22138833999634 -0.03143310546875
4.22729539871216 -0.0318603515625
4.26157188415527 -0.03411865234375
4.27341794967651 -0.034912109375
4.28786897659302 -0.03515625
4.30172443389893 -0.0352783203125
4.33435344696045 -0.038818359375
4.34654855728149 -0.04052734375
4.35700035095215 -0.041015625
4.36591815948486 -0.04132080078125
4.37226724624634 -0.04156494140625
4.38212537765503 -0.04254150390625
4.39008665084839 -0.04296875
4.40394353866577 -0.0433349609375
4.41500663757324 -0.043701171875
4.4228196144104 -0.04400634765625
4.43219947814941 -0.0447998046875
4.45595598220825 -0.05108642578125
4.462158203125 -0.05279541015625
4.4812273979187 -0.061279296875
4.49352788925171 -0.0670166015625
4.50438928604126 -0.07080078125
4.51145553588867 -0.07232666015625
4.51777648925781 -0.07342529296875
4.52908372879028 -0.07861328125
4.53974103927612 -0.0828857421875
4.54808235168457 -0.08599853515625
4.55742311477661 -0.088623046875
4.56803750991821 -0.09014892578125
4.5770206451416 -0.09149169921875
4.5882716178894 -0.09320068359375
4.5937180519104 -0.09454345703125
4.60137557983398 -0.095947265625
4.62252473831177 -0.10748291015625
4.6300311088562 -0.11138916015625
4.64227676391602 -0.1181640625
4.65295171737671 -0.1209716796875
4.65796375274658 -0.123046875
4.66139602661133 -0.12408447265625
4.66934490203857 -0.12750244140625
4.68290281295776 -0.14019775390625
4.69344568252563 -0.14398193359375
4.69716835021973 -0.1448974609375
4.70451927185059 -0.14581298828125
4.70717811584473 -0.14691162109375
4.71402788162231 -0.14886474609375
4.73018455505371 -0.15728759765625
4.7363486289978 -0.16259765625
4.74332141876221 -0.1663818359375
4.75023078918457 -0.16741943359375
4.7566819190979 -0.1680908203125
4.76324081420898 -0.1690673828125
4.7689266204834 -0.16973876953125
4.77488899230957 -0.17083740234375
4.77862167358398 -0.171142578125
4.78899526596069 -0.17852783203125
4.79328727722168 -0.18084716796875
4.80147933959961 -0.18231201171875
4.80792713165283 -0.1827392578125
4.81307363510132 -0.1834716796875
4.81829833984375 -0.183837890625
4.82307624816895 -0.1844482421875
4.82394361495972 -0.184814453125
4.84507942199707 -0.202392578125
4.85042572021484 -0.21356201171875
4.85815191268921 -0.215576171875
4.86287641525269 -0.2188720703125
4.86707830429077 -0.22076416015625
4.87680673599243 -0.223388671875
4.88334894180298 -0.2254638671875
4.88706016540527 -0.2271728515625
4.89023113250732 -0.22906494140625
4.89538955688477 -0.23291015625
4.90363788604736 -0.23828125
4.90736293792725 -0.24005126953125
4.91833448410034 -0.24786376953125
4.92197751998901 -0.24969482421875
4.92714977264404 -0.25201416015625
4.93119335174561 -0.25604248046875
4.93351268768311 -0.25726318359375
4.93735218048096 -0.26031494140625
4.94041681289673 -0.26251220703125
4.94140720367432 -0.2637939453125
4.94512367248535 -0.26513671875
4.94590187072754 -0.265869140625
4.9554328918457 -0.275146484375
4.95676374435425 -0.2781982421875
4.96168231964111 -0.279296875
4.96590232849121 -0.27960205078125
4.97121572494507 -0.28192138671875
4.97482919692993 -0.2822265625
4.98184108734131 -0.28289794921875
4.98465776443481 -0.283447265625
4.98626565933228 -0.28369140625
4.99111986160278 -0.2850341796875
4.99303913116455 -0.28558349609375
4.99662971496582 -0.285888671875
5.00588369369507 -0.29180908203125
5.00804615020752 -0.293701171875
5.01034259796143 -0.2939453125
5.01484394073486 -0.29449462890625
5.0187668800354 -0.29510498046875
5.02721118927002 -0.2977294921875
5.02961492538452 -0.29827880859375
5.03625345230103 -0.3026123046875
5.03845310211182 -0.30462646484375
5.03983020782471 -0.304931640625
5.04376697540283 -0.3062744140625
5.04773426055908 -0.3070068359375
5.04921436309814 -0.30743408203125
5.05119132995605 -0.30804443359375
5.05690860748291 -0.31085205078125
5.05869913101196 -0.31146240234375
5.06118488311768 -0.31231689453125
5.06282997131348 -0.31268310546875
5.0690016746521 -0.3179931640625
5.07138872146606 -0.31884765625
5.0735239982605 -0.31927490234375
5.07428979873657 -0.31951904296875
5.07791614532471 -0.320068359375
5.07886266708374 -0.3204345703125
5.0851583480835 -0.323486328125
5.08725595474243 -0.32421875
5.08817863464355 -0.3243408203125
5.09202194213867 -0.32611083984375
5.0933518409729 -0.326416015625
5.09475421905518 -0.32696533203125
5.09799289703369 -0.3272705078125
5.09964275360107 -0.327392578125
5.10135173797607 -0.32757568359375
5.10458612442017 -0.32769775390625
5.10707092285156 -0.32818603515625
5.10773229598999 -0.32830810546875
5.10913610458374 -0.32843017578125
5.11222267150879 -0.32879638671875
5.11351537704468 -0.32904052734375
5.11493444442749 -0.32916259765625
5.11556720733643 -0.3292236328125
5.12578392028809 -0.33489990234375
5.12866115570068 -0.336669921875
5.12941932678223 -0.3367919921875
5.13589572906494 -0.3375244140625
5.1361780166626 -0.33770751953125
5.13629245758057 -0.3377685546875
5.13921117782593 -0.33831787109375
5.14029121398926 -0.33843994140625
5.14108276367188 -0.3385009765625
5.14249563217163 -0.33880615234375
5.14283037185669 -0.3388671875
5.14426279067993 -0.3389892578125
5.14544200897217 -0.339111328125
5.14702033996582 -0.3392333984375
5.1479606628418 -0.33935546875
5.14913272857666 -0.339599609375
5.15031433105469 -0.33966064453125
5.15140342712402 -0.33978271484375
5.15472841262817 -0.3408203125
5.15576696395874 -0.34100341796875
5.15650081634521 -0.341064453125
5.15836238861084 -0.34130859375
5.15876340866089 -0.34136962890625
5.15954923629761 -0.34149169921875
5.16412973403931 -0.34649658203125
5.16495323181152 -0.347900390625
5.16580820083618 -0.34796142578125
5.16662549972534 -0.3480224609375
5.16724634170532 -0.34814453125
5.16994476318359 -0.34857177734375
5.17136669158936 -0.34869384765625
5.171790599823 -0.3487548828125
5.17307567596436 -0.348876953125
5.17337846755981 -0.34893798828125
5.17379808425903 -0.3489990234375
5.17534351348877 -0.3489990234375
5.17570018768311 -0.34906005859375
5.17677974700928 -0.34912109375
5.18171501159668 -0.35101318359375
5.18220329284668 -0.3511962890625
5.18288230895996 -0.351318359375
5.18369102478027 -0.351318359375
5.18443584442139 -0.35137939453125
5.1851167678833 -0.3514404296875
5.1864447593689 -0.35162353515625
5.18716239929199 -0.35174560546875
5.18844175338745 -0.35186767578125
5.18919849395752 -0.3519287109375
5.19079923629761 -0.35205078125
5.19142866134644 -0.35205078125
5.19268465042114 -0.35211181640625
5.19593000411987 -0.3544921875
5.1970100402832 -0.3548583984375
5.19789505004883 -0.35504150390625
5.19882726669312 -0.35552978515625
5.19959592819214 -0.35565185546875
5.20093536376953 -0.3558349609375
5.20233011245728 -0.35595703125
5.20290517807007 -0.35614013671875
5.20416879653931 -0.356201171875
5.20469522476196 -0.35626220703125
5.20651292800903 -0.3565673828125
5.20688533782959 -0.35662841796875
5.20899438858032 -0.35693359375
5.21096849441528 -0.35723876953125
5.21184396743774 -0.35736083984375
5.21282148361206 -0.35748291015625
5.21577501296997 -0.35797119140625
5.21626377105713 -0.35809326171875
5.22074842453003 -0.3590087890625
5.22100448608398 -0.35906982421875
5.22303342819214 -0.3592529296875
5.22488260269165 -0.359375
5.22632932662964 -0.35955810546875
5.22730302810669 -0.359619140625
5.22745990753174 -0.359619140625
5.22866487503052 -0.3597412109375
5.22924661636353 -0.35980224609375
5.2298150062561 -0.35992431640625
5.23085260391235 -0.3599853515625
5.23110771179199 -0.3599853515625
5.23159170150757 -0.36004638671875
5.23230981826782 -0.36016845703125
5.23264312744141 -0.3602294921875
5.23361539840698 -0.36029052734375
5.23489665985107 -0.3604736328125
5.23556613922119 -0.36053466796875
5.23608875274658 -0.36053466796875
5.23637104034424 -0.360595703125
5.23658752441406 -0.360595703125
5.23720455169678 -0.36065673828125
5.23839473724365 -0.36077880859375
5.23961973190308 -0.361083984375
5.23990726470947 -0.36114501953125
5.24129009246826 -0.36114501953125
5.24182033538818 -0.3612060546875
5.24237728118896 -0.36126708984375
5.24249410629272 -0.36126708984375
5.24276971817017 -0.361328125
5.24324417114258 -0.36151123046875
5.24403953552246 -0.361572265625
5.24453449249268 -0.36163330078125
5.24538660049438 -0.36163330078125
5.24556684494019 -0.3616943359375
5.24628686904907 -0.36181640625
5.24639987945557 -0.36181640625
5.24675464630127 -0.36212158203125
5.24734210968018 -0.36212158203125
5.25076866149902 -0.36370849609375
5.25094175338745 -0.36395263671875
5.25103187561035 -0.364013671875
5.25335741043091 -0.364990234375
5.25360202789307 -0.3651123046875
5.25406932830811 -0.36517333984375
5.25449466705322 -0.365234375
5.25462293624878 -0.365234375
5.25555944442749 -0.36529541015625
5.25593328475952 -0.3653564453125
5.25614261627197 -0.36541748046875
5.25688362121582 -0.36541748046875
5.2580189704895 -0.3656005859375
5.25815343856812 -0.3656005859375
5.258469581604 -0.36566162109375
5.25938844680786 -0.36566162109375
5.25952482223511 -0.36572265625
5.25990676879883 -0.36578369140625
5.26000928878784 -0.3658447265625
5.26035070419312 -0.3658447265625
5.26100587844849 -0.36590576171875
5.26135349273682 -0.365966796875
5.26189088821411 -0.365966796875
5.26218271255493 -0.36602783203125
5.26273822784424 -0.36602783203125
5.26592588424683 -0.36749267578125
5.2661280632019 -0.36761474609375
5.26680088043213 -0.36773681640625
5.26720905303955 -0.3677978515625
5.26744842529297 -0.3677978515625
5.26791048049927 -0.36785888671875
5.26873254776001 -0.367919921875
5.26881408691406 -0.367919921875
5.26933765411377 -0.3680419921875
5.26957368850708 -0.3680419921875
5.27004241943359 -0.36810302734375
5.27020597457886 -0.3681640625
5.27150917053223 -0.36834716796875
5.27169275283813 -0.36834716796875
5.27276945114136 -0.36846923828125
5.27282047271729 -0.36846923828125
5.27411842346191 -0.36871337890625
5.27452516555786 -0.3687744140625
5.27487564086914 -0.3687744140625
5.27520990371704 -0.36883544921875
5.27714395523071 -0.369140625
5.27769184112549 -0.3692626953125
5.27829170227051 -0.36932373046875
5.27854537963867 -0.36932373046875
5.28028678894043 -0.36956787109375
5.28046226501465 -0.36956787109375
5.28073310852051 -0.36962890625
5.28107643127441 -0.36962890625
5.28125143051147 -0.36962890625
5.28145837783813 -0.36968994140625
5.28173303604126 -0.36968994140625
5.28212356567383 -0.3697509765625
5.28224611282349 -0.3697509765625
5.28414869308472 -0.37030029296875
5.28455257415771 -0.37042236328125
5.28487062454224 -0.3704833984375
5.28519916534424 -0.3704833984375
5.28547382354736 -0.37054443359375
5.28627014160156 -0.37060546875
5.28645658493042 -0.37060546875
5.28694105148315 -0.37066650390625
5.28703784942627 -0.37066650390625
5.28753280639648 -0.3707275390625
5.28961133956909 -0.37139892578125
5.28983879089355 -0.37139892578125
5.29017925262451 -0.3714599609375
5.29065799713135 -0.3714599609375
5.29104661941528 -0.3714599609375
5.29129791259766 -0.37152099609375
5.29194784164429 -0.37152099609375
5.29223394393921 -0.37158203125
5.29243326187134 -0.37158203125
5.29305505752563 -0.37164306640625
5.29330968856812 -0.37164306640625
5.29376697540283 -0.3717041015625
5.29438018798828 -0.3717041015625
5.29455232620239 -0.3717041015625
5.29476356506348 -0.3717041015625
5.29498863220215 -0.37176513671875
5.29608774185181 -0.37200927734375
5.29652690887451 -0.37200927734375
5.29686260223389 -0.37200927734375
5.29704904556274 -0.3720703125
5.29735994338989 -0.3720703125
5.29791164398193 -0.3720703125
5.29806232452393 -0.3720703125
5.29966831207275 -0.372314453125
5.29979705810547 -0.37249755859375
5.2999472618103 -0.37249755859375
5.30086708068848 -0.37274169921875
5.30134916305542 -0.37274169921875
5.30179166793823 -0.372802734375
5.30180215835571 -0.372802734375
5.3022313117981 -0.37286376953125
5.30459594726562 -0.3741455078125
5.3057918548584 -0.375
5.30607748031616 -0.37506103515625
5.30628538131714 -0.37506103515625
5.30642938613892 -0.37506103515625
5.30693531036377 -0.37506103515625
5.30892276763916 -0.37530517578125
5.30932998657227 -0.37530517578125
5.30964708328247 -0.37530517578125
5.30989408493042 -0.37530517578125
5.31112194061279 -0.37542724609375
5.31176424026489 -0.37554931640625
5.31202697753906 -0.37554931640625
5.31211805343628 -0.37554931640625
5.31238269805908 -0.3756103515625
5.31246948242188 -0.3756103515625
5.31268930435181 -0.3756103515625
5.31294727325439 -0.3756103515625
5.31348323822021 -0.3756103515625
5.31359958648682 -0.37567138671875
5.31393671035767 -0.37567138671875
5.31450366973877 -0.37567138671875
5.31487369537354 -0.37567138671875
5.31570386886597 -0.37579345703125
5.3160228729248 -0.37579345703125
5.31650924682617 -0.37579345703125
5.31660556793213 -0.37579345703125
5.31675243377686 -0.37579345703125
5.31686115264893 -0.3758544921875
5.3190541267395 -0.377197265625
5.31923532485962 -0.37762451171875
5.31946611404419 -0.37762451171875
5.31956624984741 -0.37762451171875
5.32005071640015 -0.37762451171875
5.32018804550171 -0.37762451171875
5.32027292251587 -0.37762451171875
5.32055950164795 -0.37762451171875
5.32101631164551 -0.37762451171875
5.32117795944214 -0.377685546875
5.32130002975464 -0.377685546875
5.32153415679932 -0.377685546875
5.32157373428345 -0.377685546875
5.32239294052124 -0.37774658203125
5.32246971130371 -0.37774658203125
5.32264518737793 -0.37774658203125
5.32268857955933 -0.37774658203125
5.32274198532104 -0.37774658203125
5.32299423217773 -0.37774658203125
5.32319211959839 -0.3778076171875
5.32387495040894 -0.3778076171875
5.3240270614624 -0.37786865234375
5.32417726516724 -0.37786865234375
5.32496309280396 -0.3779296875
5.32535982131958 -0.3779296875
5.32542943954468 -0.3779296875
5.32549095153809 -0.3779296875
5.32572507858276 -0.3779296875
5.32618856430054 -0.37799072265625
5.3262619972229 -0.37799072265625
5.32701730728149 -0.3780517578125
5.32707071304321 -0.3780517578125
5.32736492156982 -0.3780517578125
5.32800006866455 -0.3780517578125
5.32818365097046 -0.3780517578125
5.32829618453979 -0.3780517578125
5.32848358154297 -0.37811279296875
5.32885026931763 -0.37811279296875
5.3291335105896 -0.37811279296875
5.32918405532837 -0.37811279296875
5.3304967880249 -0.37841796875
5.3310284614563 -0.37847900390625
5.33103847503662 -0.37847900390625
5.33132410049438 -0.37847900390625
5.33153438568115 -0.37847900390625
5.33154487609863 -0.37847900390625
5.33172082901001 -0.37847900390625
5.33184432983398 -0.3785400390625
5.3318886756897 -0.3785400390625
5.33215761184692 -0.3785400390625
5.33224630355835 -0.3785400390625
5.33270692825317 -0.3785400390625
5.33355617523193 -0.378662109375
5.33374929428101 -0.378662109375
5.3338098526001 -0.378662109375
5.33402538299561 -0.378662109375
5.3340916633606 -0.378662109375
5.33426666259766 -0.378662109375
5.33447170257568 -0.378662109375
5.33484172821045 -0.378662109375
5.33516883850098 -0.37872314453125
5.33522510528564 -0.37872314453125
5.33536577224731 -0.37872314453125
5.33566856384277 -0.37872314453125
5.33592510223389 -0.37872314453125
5.33603715896606 -0.37872314453125
5.33640384674072 -0.37872314453125
5.33647775650024 -0.37872314453125
5.33682203292847 -0.3787841796875
5.33739519119263 -0.3787841796875
5.33752107620239 -0.3787841796875
5.33762311935425 -0.3787841796875
5.33770275115967 -0.3787841796875
5.33795404434204 -0.3787841796875
5.33929252624512 -0.37908935546875
5.33942747116089 -0.379150390625
5.33951091766357 -0.379150390625
5.33973169326782 -0.37921142578125
5.33988857269287 -0.37921142578125
5.34019422531128 -0.37921142578125
5.34036493301392 -0.37921142578125
5.34042835235596 -0.37921142578125
5.34062051773071 -0.37921142578125
5.3409218788147 -0.37921142578125
5.34099102020264 -0.37921142578125
5.34103059768677 -0.37921142578125
5.34115743637085 -0.3792724609375
5.3412504196167 -0.3792724609375
5.34134769439697 -0.3792724609375
5.34157514572144 -0.3792724609375
5.34180641174316 -0.3792724609375
5.34209108352661 -0.3792724609375
5.34226083755493 -0.3792724609375
5.34232616424561 -0.37933349609375
5.34239292144775 -0.37933349609375
5.3427996635437 -0.37933349609375
5.34290599822998 -0.37933349609375
5.34302806854248 -0.37933349609375
5.34308338165283 -0.37933349609375
5.34342432022095 -0.37933349609375
5.3436427116394 -0.37933349609375
5.34365272521973 -0.37933349609375
5.34368991851807 -0.37933349609375
5.34408760070801 -0.37939453125
5.34418964385986 -0.37939453125
5.34440994262695 -0.37939453125
5.34451007843018 -0.37939453125
5.34472608566284 -0.37939453125
5.34473991394043 -0.37939453125
5.34505224227905 -0.37945556640625
5.34545421600342 -0.37945556640625
5.34552097320557 -0.37945556640625
5.34556198120117 -0.37945556640625
5.34568548202515 -0.37945556640625
5.34591245651245 -0.3795166015625
5.3467321395874 -0.379638671875
5.34691190719604 -0.379638671875
5.34737491607666 -0.3797607421875
5.34748029708862 -0.3797607421875
5.34775733947754 -0.3797607421875
5.34792709350586 -0.3797607421875
5.34813547134399 -0.3797607421875
5.34852695465088 -0.3797607421875
5.34872150421143 -0.37982177734375
5.3491005897522 -0.37982177734375
5.34933948516846 -0.37982177734375
5.34973764419556 -0.37982177734375
5.34981155395508 -0.37982177734375
5.34998607635498 -0.37982177734375
5.3501238822937 -0.37982177734375
5.3506121635437 -0.3798828125
5.3510479927063 -0.37994384765625
5.35129737854004 -0.37994384765625
5.35172080993652 -0.37994384765625
5.35182523727417 -0.3800048828125
5.35197973251343 -0.3800048828125
5.35205507278442 -0.3800048828125
5.35243511199951 -0.3800048828125
5.35251808166504 -0.3800048828125
5.35269737243652 -0.3800048828125
5.35279989242554 -0.3800048828125
5.35331583023071 -0.3800048828125
5.35341596603394 -0.38006591796875
5.35381412506104 -0.38006591796875
5.35391807556152 -0.38006591796875
5.35407018661499 -0.38006591796875
5.35423135757446 -0.380126953125
5.35451173782349 -0.380126953125
5.35453271865845 -0.380126953125
5.35467863082886 -0.380126953125
5.354736328125 -0.380126953125
5.35481691360474 -0.380126953125
5.35511636734009 -0.380126953125
5.35521602630615 -0.380126953125
5.35538816452026 -0.38018798828125
5.35553026199341 -0.38018798828125
5.35573863983154 -0.38018798828125
5.35634899139404 -0.3802490234375
5.35645437240601 -0.3802490234375
5.35664319992065 -0.3802490234375
5.35672569274902 -0.3802490234375
5.3568058013916 -0.3802490234375
5.35688018798828 -0.3802490234375
5.35691833496094 -0.3802490234375
5.35747957229614 -0.38037109375
5.35762023925781 -0.38037109375
5.35825681686401 -0.38037109375
5.35834217071533 -0.38037109375
5.35840320587158 -0.38037109375
5.35843944549561 -0.38037109375
5.35885381698608 -0.38043212890625
5.35906314849854 -0.3804931640625
5.35913324356079 -0.3804931640625
5.35924911499023 -0.3804931640625
5.35944080352783 -0.3804931640625
5.35945415496826 -0.3804931640625
5.35965156555176 -0.3804931640625
5.36004400253296 -0.3804931640625
5.36027336120605 -0.38055419921875
5.36043643951416 -0.38055419921875
5.36050844192505 -0.38055419921875
5.36069965362549 -0.38055419921875
5.36072397232056 -0.38055419921875
5.36082983016968 -0.38055419921875
5.36093807220459 -0.38055419921875
5.3611478805542 -0.38055419921875
5.36142015457153 -0.380615234375
5.36158609390259 -0.380615234375
5.36163520812988 -0.380615234375
5.36180543899536 -0.380615234375
5.36198854446411 -0.380615234375
5.36210346221924 -0.380615234375
5.36247873306274 -0.380615234375
5.36264085769653 -0.38067626953125
5.36268997192383 -0.38067626953125
5.36269903182983 -0.38067626953125
5.36276340484619 -0.38067626953125
5.3634991645813 -0.38079833984375
5.36387157440186 -0.38092041015625
5.36398029327393 -0.38092041015625
5.36422252655029 -0.38092041015625
5.36423206329346 -0.38092041015625
5.36457920074463 -0.38092041015625
5.36482095718384 -0.38092041015625
5.36499929428101 -0.38092041015625
5.36504411697388 -0.3809814453125
5.36522579193115 -0.3809814453125
5.36528968811035 -0.3809814453125
5.36553287506104 -0.3809814453125
5.36554622650146 -0.3809814453125
5.36583614349365 -0.3809814453125
5.36613893508911 -0.3809814453125
5.36624908447266 -0.3809814453125
5.3663501739502 -0.3809814453125
5.36644554138184 -0.3809814453125
5.36669731140137 -0.38104248046875
5.36670684814453 -0.38104248046875
5.36690664291382 -0.38104248046875
5.36715078353882 -0.38104248046875
5.36722898483276 -0.38104248046875
5.36733913421631 -0.38104248046875
5.36736154556274 -0.38104248046875
5.36803388595581 -0.38128662109375
5.36810255050659 -0.38134765625
5.36833524703979 -0.38134765625
5.36868476867676 -0.38134765625
5.36876821517944 -0.38134765625
5.36877202987671 -0.38134765625
5.36942195892334 -0.38140869140625
5.36951637268066 -0.3814697265625
5.36963129043579 -0.3814697265625
5.36979103088379 -0.3814697265625
5.37007617950439 -0.3814697265625
5.37012052536011 -0.3814697265625
5.37014865875244 -0.3814697265625
5.37023735046387 -0.3814697265625
5.37054634094238 -0.3814697265625
5.37067794799805 -0.3814697265625
5.37081623077393 -0.38153076171875
5.3709774017334 -0.38153076171875
5.37098455429077 -0.38153076171875
5.3709864616394 -0.38153076171875
5.37107181549072 -0.38153076171875
5.37118625640869 -0.38153076171875
5.37233018875122 -0.38189697265625
5.37246656417847 -0.3819580078125
5.37247371673584 -0.3819580078125
5.37264347076416 -0.3819580078125
5.37273359298706 -0.3819580078125
5.3727502822876 -0.3819580078125
5.37280702590942 -0.3819580078125
5.3729453086853 -0.3819580078125
5.3729453086853 -0.3819580078125
5.37352275848389 -0.38201904296875
5.37364768981934 -0.382080078125
5.37374496459961 -0.382080078125
5.37402772903442 -0.382080078125
5.37428617477417 -0.382080078125
5.37433767318726 -0.382080078125
5.37468957901001 -0.382080078125
5.37469863891602 -0.382080078125
5.37472820281982 -0.382080078125
5.37493705749512 -0.382080078125
5.37544059753418 -0.38214111328125
5.37544775009155 -0.38214111328125
5.37555742263794 -0.38214111328125
5.37565612792969 -0.38214111328125
5.37566375732422 -0.38214111328125
5.37612962722778 -0.38214111328125
5.37618255615234 -0.38214111328125
5.37621355056763 -0.38214111328125
5.37647485733032 -0.38214111328125
5.37657499313354 -0.38214111328125
5.37662601470947 -0.38214111328125
5.3768138885498 -0.38214111328125
5.37694549560547 -0.38214111328125
5.37713146209717 -0.38214111328125
5.3772497177124 -0.3822021484375
5.37748098373413 -0.3822021484375
5.37757015228271 -0.3822021484375
5.37759017944336 -0.3822021484375
5.3776650428772 -0.3822021484375
5.37783765792847 -0.3822021484375
5.37786865234375 -0.3822021484375
5.37804365158081 -0.3822021484375
5.37821626663208 -0.3822021484375
5.37834882736206 -0.3822021484375
5.37836503982544 -0.3822021484375
5.37850522994995 -0.3822021484375
5.37850522994995 -0.3822021484375
5.37871932983398 -0.3822021484375
5.37924194335938 -0.38226318359375
5.37924194335938 -0.38226318359375
5.37932205200195 -0.38226318359375
5.37940692901611 -0.38226318359375
5.37942171096802 -0.38226318359375
5.38015508651733 -0.38226318359375
5.38045167922974 -0.38226318359375
5.38045930862427 -0.38226318359375
5.38072681427002 -0.38226318359375
5.38083696365356 -0.38226318359375
5.38084411621094 -0.38226318359375
5.38094186782837 -0.38226318359375
5.38136577606201 -0.38232421875
5.38151597976685 -0.38232421875
5.38177394866943 -0.38232421875
5.38177537918091 -0.38232421875
5.38184404373169 -0.38232421875
5.38235378265381 -0.38232421875
5.38236093521118 -0.38232421875
5.38240957260132 -0.38238525390625
5.38259315490723 -0.38238525390625
5.3826060295105 -0.38238525390625
5.38272666931152 -0.38238525390625
5.38275337219238 -0.38238525390625
5.38296937942505 -0.38238525390625
5.38297653198242 -0.38238525390625
5.38300704956055 -0.38238525390625
5.38302516937256 -0.38238525390625
5.38305377960205 -0.38238525390625
5.3831615447998 -0.38238525390625
5.38326597213745 -0.38238525390625
5.38342380523682 -0.38238525390625
5.3836522102356 -0.38238525390625
5.38375806808472 -0.38238525390625
5.38398742675781 -0.38238525390625
5.38410949707031 -0.38238525390625
5.38417434692383 -0.38238525390625
5.38424968719482 -0.38238525390625
5.38494253158569 -0.3824462890625
5.38507318496704 -0.3824462890625
5.38510179519653 -0.3824462890625
5.38516807556152 -0.3824462890625
5.38526678085327 -0.3824462890625
5.38527536392212 -0.3824462890625
5.38532733917236 -0.3824462890625
5.38532733917236 -0.3824462890625
5.38564014434814 -0.38250732421875
5.38591194152832 -0.38250732421875
5.38597059249878 -0.38250732421875
5.38605642318726 -0.38250732421875
5.38639354705811 -0.38250732421875
5.38640069961548 -0.38250732421875
5.38649559020996 -0.38250732421875
5.3866720199585 -0.38250732421875
5.38677167892456 -0.38250732421875
5.38685035705566 -0.38250732421875
5.38694286346436 -0.38250732421875
5.38704442977905 -0.38250732421875
5.38705158233643 -0.38250732421875
5.38730096817017 -0.38250732421875
5.38730955123901 -0.38250732421875
5.38734006881714 -0.38250732421875
5.3873987197876 -0.38250732421875
5.38745021820068 -0.382568359375
5.38769054412842 -0.382568359375
5.38769769668579 -0.382568359375
5.38779735565186 -0.382568359375
5.38854360580444 -0.38262939453125
5.38863229751587 -0.38262939453125
5.3887882232666 -0.38262939453125
5.38899946212769 -0.38262939453125
5.38932371139526 -0.38262939453125
5.38939094543457 -0.38262939453125
5.38946723937988 -0.38262939453125
5.38946723937988 -0.38262939453125
5.38950634002686 -0.38262939453125
5.38961601257324 -0.38262939453125
5.38977384567261 -0.38262939453125
5.38977384567261 -0.38262939453125
5.38978099822998 -0.38262939453125
5.38989400863647 -0.38262939453125
5.38990116119385 -0.38262939453125
5.39008712768555 -0.38262939453125
5.39014863967896 -0.38262939453125
5.39015579223633 -0.38262939453125
5.3901629447937 -0.38262939453125
5.3901629447937 -0.38262939453125
5.39068603515625 -0.3826904296875
5.39082050323486 -0.38275146484375
5.39082717895508 -0.38275146484375
5.39103221893311 -0.38275146484375
5.39108514785767 -0.38275146484375
5.39119625091553 -0.38275146484375
5.3912034034729 -0.38275146484375
5.3912034034729 -0.38275146484375
5.39185762405396 -0.38275146484375
5.39196157455444 -0.38275146484375
5.39282178878784 -0.3828125
5.39292192459106 -0.3828125
5.39302396774292 -0.3828125
5.39303112030029 -0.3828125
5.3930869102478 -0.3828125
5.39309406280518 -0.3828125
5.39309406280518 -0.3828125
5.39318895339966 -0.3828125
5.39335918426514 -0.3828125
5.39336633682251 -0.3828125
5.39344882965088 -0.3828125
5.39366102218628 -0.3828125
5.39388370513916 -0.3828125
5.39389085769653 -0.3828125
5.39398384094238 -0.3828125
5.39439392089844 -0.3828125
5.39443778991699 -0.38287353515625
5.39448165893555 -0.38287353515625
5.39476490020752 -0.38287353515625
5.39495754241943 -0.38287353515625
5.39499950408936 -0.38287353515625
5.3950572013855 -0.38287353515625
5.3950572013855 -0.38287353515625
5.39537715911865 -0.38287353515625
};
\addplot [ultra thick, blue]
table {%
0 0
0.477121233940125 -0.00018310546875
0.477121233940125 -0.000244140625
0.698970019817352 -0.00042724609375
0.778151273727417 -0.00054931640625
1.11394333839417 -0.0008544921875
1.11394333839417 -0.0010986328125
1.17609131336212 -0.001220703125
1.23044896125793 -0.0013427734375
1.30103003978729 -0.00152587890625
1.34242272377014 -0.001708984375
1.38021123409271 -0.00177001953125
1.46239805221558 -0.00225830078125
1.49136173725128 -0.00238037109375
1.55630254745483 -0.00299072265625
1.57978355884552 -0.00311279296875
1.65321254730225 -0.0035400390625
1.68124127388 -0.00372314453125
1.70757019519806 -0.00384521484375
1.74818801879883 -0.00390625
1.77085208892822 -0.004150390625
1.96378779411316 -0.0098876953125
2.01283717155457 -0.01507568359375
2.05307841300964 -0.015869140625
2.11394333839417 -0.01776123046875
2.13987898826599 -0.01861572265625
2.20139718055725 -0.02099609375
2.22530937194824 -0.022705078125
2.262451171875 -0.02655029296875
2.26951289176941 -0.028564453125
2.28780174255371 -0.02978515625
2.33243846893311 -0.03265380859375
2.33845639228821 -0.03375244140625
2.34044408798218 -0.03399658203125
2.35410833358765 -0.03424072265625
2.35983562469482 -0.034423828125
2.39445161819458 -0.03631591796875
2.42651128768921 -0.0372314453125
2.42975234985352 -0.0377197265625
2.45788192749023 -0.03900146484375
2.4683473110199 -0.03936767578125
2.48572134971619 -0.0396728515625
2.49554443359375 -0.04010009765625
2.49831056594849 -0.040283203125
2.51454782485962 -0.0406494140625
2.56820178031921 -0.04364013671875
2.57403135299683 -0.045654296875
2.59328603744507 -0.0467529296875
2.61804819107056 -0.04791259765625
2.63648796081543 -0.04986572265625
2.65127801895142 -0.05096435546875
2.67669367790222 -0.0521240234375
2.68930888175964 -0.05426025390625
2.70329141616821 -0.05572509765625
2.71683764457703 -0.05816650390625
2.73319721221924 -0.0606689453125
2.74507474899292 -0.06475830078125
2.76192784309387 -0.07110595703125
2.78031730651855 -0.0767822265625
2.79309153556824 -0.07855224609375
2.80482077598572 -0.0811767578125
2.82282161712646 -0.08349609375
2.8286600112915 -0.0845947265625
2.84010601043701 -0.08563232421875
2.86153435707092 -0.09136962890625
2.87215638160706 -0.0926513671875
2.87679505348206 -0.09326171875
2.88649082183838 -0.09423828125
2.89042091369629 -0.0947265625
2.9084849357605 -0.09832763671875
2.93094897270203 -0.10162353515625
2.93500328063965 -0.10296630859375
2.95424246788025 -0.10418701171875
2.96473097801208 -0.10650634765625
2.96941590309143 -0.10748291015625
2.99166893959045 -0.11181640625
2.99782299995422 -0.11358642578125
3.01786780357361 -0.1221923828125
3.02160263061523 -0.12457275390625
3.02938365936279 -0.12713623046875
3.04218149185181 -0.1304931640625
3.05346250534058 -0.13616943359375
3.05994200706482 -0.1390380859375
3.07298469543457 -0.14044189453125
3.0852906703949 -0.14398193359375
3.08990502357483 -0.147216796875
3.1010594367981 -0.1514892578125
3.10924100875854 -0.15338134765625
3.11760258674622 -0.15557861328125
3.12024474143982 -0.1573486328125
3.12450432777405 -0.15838623046875
3.12645602226257 -0.1595458984375
3.13097667694092 -0.16082763671875
3.13545060157776 -0.1619873046875
3.14050793647766 -0.1632080078125
3.14705777168274 -0.16510009765625
3.14860272407532 -0.165771484375
3.15259408950806 -0.16668701171875
3.15411949157715 -0.1673583984375
3.15956711769104 -0.16864013671875
3.16106843948364 -0.169189453125
3.16375756263733 -0.16973876953125
3.16524434089661 -0.17022705078125
3.17724776268005 -0.175537109375
3.17955183982849 -0.17657470703125
3.18497514724731 -0.17755126953125
3.19145107269287 -0.17803955078125
3.19340300559998 -0.17840576171875
3.20002937316895 -0.1800537109375
3.20411992073059 -0.1805419921875
3.21351766586304 -0.18560791015625
3.21800994873047 -0.18682861328125
3.22634220123291 -0.1876220703125
3.22865700721741 -0.18829345703125
3.23502326011658 -0.19000244140625
3.24179553985596 -0.1907958984375
3.24649858474731 -0.1922607421875
3.25188136100769 -0.1932373046875
3.26316237449646 -0.20111083984375
3.26576089859009 -0.20361328125
3.27737998962402 -0.21734619140625
3.28035068511963 -0.2205810546875
3.29114675521851 -0.23321533203125
3.31175374984741 -0.24169921875
3.31848073005676 -0.24658203125
3.32139134407043 -0.24859619140625
3.32572078704834 -0.25091552734375
3.33525729179382 -0.26025390625
3.33725953102112 -0.2655029296875
3.33925271034241 -0.26629638671875
3.34163236618042 -0.26702880859375
3.34596157073975 -0.26824951171875
3.35024809837341 -0.26947021484375
3.3514096736908 -0.27044677734375
3.35506820678711 -0.2718505859375
3.35640835762024 -0.27252197265625
3.36002516746521 -0.27386474609375
3.36380004882812 -0.27496337890625
3.36473846435547 -0.275390625
3.36604928970337 -0.275634765625
3.37143731117249 -0.27728271484375
3.38345623016357 -0.28369140625
3.38453269004822 -0.28594970703125
3.38649892807007 -0.28668212890625
3.39128804206848 -0.287841796875
3.39619922637939 -0.28857421875
3.39759254455566 -0.2889404296875
3.39863443374634 -0.28912353515625
3.40312051773071 -0.289794921875
3.41010212898254 -0.29071044921875
3.41128301620483 -0.291015625
3.41279649734497 -0.29132080078125
3.41396999359131 -0.29150390625
3.42094540596008 -0.29290771484375
3.42942929267883 -0.29632568359375
3.43039751052856 -0.29693603515625
3.43312954902649 -0.29779052734375
3.43408966064453 -0.298095703125
3.43552589416504 -0.29840087890625
3.43854236602783 -0.298828125
3.44544839859009 -0.29974365234375
3.44746804237366 -0.30035400390625
3.44824242591858 -0.30059814453125
3.45560598373413 -0.3017578125
3.4569730758667 -0.3021240234375
3.45863795280457 -0.302490234375
3.4598445892334 -0.30291748046875
3.46493649482727 -0.30401611328125
3.46612596511841 -0.304443359375
3.46996927261353 -0.30511474609375
3.47114491462708 -0.3055419921875
3.47639679908752 -0.30859375
3.47986316680908 -0.30950927734375
3.48058176040649 -0.309814453125
3.48201560974121 -0.31011962890625
3.48358726501465 -0.3106689453125
3.48953652381897 -0.3121337890625
3.49080085754395 -0.312744140625
3.49415469169617 -0.31317138671875
3.49540567398071 -0.3134765625
3.49941205978394 -0.3150634765625
3.50037384033203 -0.3154296875
3.50229048728943 -0.31640625
3.50893354415894 -0.3167724609375
3.51041102409363 -0.3172607421875
3.51161599159241 -0.31756591796875
3.51308441162109 -0.318115234375
3.51454782485962 -0.318603515625
3.51600623130798 -0.3189697265625
3.52153038978577 -0.319580078125
3.52322602272034 -0.3203125
3.52569246292114 -0.32098388671875
3.52737212181091 -0.32122802734375
3.5291736125946 -0.32177734375
3.53415298461914 -0.32220458984375
3.54481196403503 -0.32684326171875
3.54530715942383 -0.32745361328125
3.54617238044739 -0.32763671875
3.55010604858398 -0.32879638671875
3.55096173286438 -0.32891845703125
3.55132794380188 -0.3291015625
3.55181574821472 -0.32916259765625
3.5571460723877 -0.32965087890625
3.55798816680908 -0.330078125
3.55858850479126 -0.33013916015625
3.5589485168457 -0.330322265625
3.55990672111511 -0.3304443359375
3.56050443649292 -0.33056640625
3.56098198890686 -0.33074951171875
3.56205487251282 -0.330810546875
3.56241178512573 -0.33087158203125
3.56300616264343 -0.33099365234375
3.5638370513916 -0.3311767578125
3.56690859794617 -0.33160400390625
3.56749701499939 -0.33197021484375
3.5678493976593 -0.33203125
3.56843638420105 -0.3321533203125
3.574378490448 -0.3345947265625
3.57449436187744 -0.3348388671875
3.5749568939209 -0.3349609375
3.57541871070862 -0.33502197265625
3.57576489448547 -0.3350830078125
3.57680177688599 -0.335205078125
3.58285856246948 -0.33795166015625
3.58331227302551 -0.33837890625
3.58342552185059 -0.33843994140625
3.58410501480103 -0.3385009765625
3.58433127403259 -0.338623046875
3.58512210845947 -0.33868408203125
3.59173226356506 -0.3409423828125
3.59217667579651 -0.34124755859375
3.59284257888794 -0.3414306640625
3.59328603744507 -0.34149169921875
3.59703660011292 -0.34307861328125
3.59747576713562 -0.34332275390625
3.59802412986755 -0.34344482421875
3.59944629669189 -0.34356689453125
3.6011905670166 -0.34393310546875
3.60162544250488 -0.34405517578125
3.60422611236572 -0.34521484375
3.60681104660034 -0.3455810546875
3.60713315010071 -0.345703125
3.6074550151825 -0.3458251953125
3.60799098014832 -0.34625244140625
3.61023426055908 -0.34637451171875
3.61257195472717 -0.346923828125
3.61373615264893 -0.34747314453125
3.61415863037109 -0.34765625
3.615318775177 -0.34771728515625
3.61542391777039 -0.3477783203125
3.61573958396912 -0.347900390625
3.61961507797241 -0.34796142578125
3.61992764472961 -0.34808349609375
3.62169551849365 -0.34832763671875
3.62179923057556 -0.3485107421875
3.62242126464844 -0.34857177734375
3.62366271018982 -0.34869384765625
3.62366271018982 -0.34869384765625
3.62397241592407 -0.34881591796875
3.62613487243652 -0.3489990234375
3.62675094604492 -0.34912109375
3.62695598602295 -0.3492431640625
3.62961339950562 -0.3494873046875
3.62961339950562 -0.3494873046875
3.63083457946777 -0.349609375
3.63113927841187 -0.34967041015625
3.63124084472656 -0.3497314453125
3.63205218315125 -0.34979248046875
3.63215351104736 -0.349853515625
3.63215351104736 -0.349853515625
3.63848924636841 -0.35150146484375
3.63858914375305 -0.3516845703125
3.63958597183228 -0.35186767578125
3.64077949523926 -0.3521728515625
3.64187049865723 -0.35223388671875
3.64216756820679 -0.35223388671875
3.64571690559387 -0.3525390625
3.64640378952026 -0.35272216796875
3.6466977596283 -0.352783203125
3.64748072624207 -0.35284423828125
3.64777398109436 -0.3529052734375
3.64826250076294 -0.3529052734375
3.6485550403595 -0.35296630859375
3.65369486808777 -0.35406494140625
3.65388751029968 -0.35430908203125
3.6604859828949 -0.35699462890625
3.66086554527283 -0.3582763671875
3.66171813011169 -0.35833740234375
3.6624743938446 -0.3583984375
3.66379523277283 -0.35888671875
3.66454792022705 -0.3590087890625
3.66642427444458 -0.35955810546875
3.66726613044739 -0.35968017578125
3.66810631752014 -0.3597412109375
3.66903781890869 -0.35980224609375
3.67033863067627 -0.360107421875
3.67209792137146 -0.3604736328125
3.67228269577026 -0.3604736328125
3.678062915802 -0.36077880859375
3.67815399169922 -0.36090087890625
3.67833614349365 -0.3609619140625
3.6786093711853 -0.36102294921875
3.68096971511841 -0.3612060546875
3.68106031417847 -0.3612060546875
3.68124127388 -0.36126708984375
3.68124127388 -0.36126708984375
3.68430662155151 -0.36175537109375
3.68797469139099 -0.36236572265625
3.688063621521 -0.3624267578125
3.68921995162964 -0.36273193359375
3.68939757347107 -0.36279296875
3.6895751953125 -0.36285400390625
3.68984150886536 -0.3629150390625
3.68993020057678 -0.36297607421875
3.69161176681519 -0.36358642578125
3.69196510314941 -0.3636474609375
3.69205331802368 -0.3636474609375
3.69214153289795 -0.36370849609375
3.69222974777222 -0.36370849609375
3.69267082214355 -0.36376953125
3.69275879859924 -0.36383056640625
3.69275879859924 -0.36383056640625
3.69346308708191 -0.3638916015625
3.69381475448608 -0.36395263671875
3.69381475448608 -0.36395263671875
3.69390273094177 -0.364013671875
3.69416618347168 -0.364013671875
3.69416618347168 -0.36407470703125
3.69425415992737 -0.36407470703125
3.69425415992737 -0.3641357421875
3.69548177719116 -0.3642578125
3.69556927680969 -0.36431884765625
3.69635629653931 -0.364501953125
3.69644379615784 -0.36456298828125
3.69714212417603 -0.3646240234375
3.69714212417603 -0.3646240234375
3.69714212417603 -0.3646240234375
3.69775223731995 -0.364990234375
3.69783926010132 -0.364990234375
3.69862246513367 -0.36505126953125
3.698970079422 -0.365234375
3.69905686378479 -0.365234375
3.69966435432434 -0.3653564453125
3.69983768463135 -0.36541748046875
3.70191311836243 -0.36578369140625
3.70199942588806 -0.3658447265625
3.7020857334137 -0.3658447265625
3.704665184021 -0.36614990234375
3.70475101470947 -0.36614990234375
3.70535039901733 -0.36627197265625
3.70543599128723 -0.3663330078125
3.70552158355713 -0.3663330078125
3.70629096031189 -0.36651611328125
3.70637631416321 -0.36651611328125
3.70646166801453 -0.3665771484375
3.70714426040649 -0.36663818359375
3.70714426040649 -0.36669921875
3.70722937583923 -0.36669921875
3.70722937583923 -0.36676025390625
3.70799565315247 -0.36688232421875
3.70808076858521 -0.366943359375
3.70808076858521 -0.366943359375
3.70884561538696 -0.366943359375
3.7091851234436 -0.36712646484375
3.7091851234436 -0.36712646484375
3.70952439308167 -0.3671875
3.70952439308167 -0.3671875
3.70960903167725 -0.36724853515625
3.70960903167725 -0.3673095703125
3.71028661727905 -0.3673095703125
3.71037125587463 -0.367431640625
3.7106249332428 -0.36749267578125
3.71070957183838 -0.3675537109375
3.71121644973755 -0.36761474609375
3.71155405044556 -0.36761474609375
3.71163845062256 -0.36767578125
3.71214437484741 -0.36773681640625
3.71533465385437 -0.367919921875
3.71558547019958 -0.367919921875
3.71692109107971 -0.36859130859375
3.7170877456665 -0.36865234375
3.71742081642151 -0.36871337890625
3.71750402450562 -0.36871337890625
3.71750402450562 -0.3687744140625
3.71775364875793 -0.36883544921875
3.71816945075989 -0.36883544921875
3.71816945075989 -0.36883544921875
3.71833562850952 -0.368896484375
3.71833562850952 -0.368896484375
3.71833562850952 -0.36895751953125
3.72197532653809 -0.369384765625
3.7223048210144 -0.36944580078125
3.72238707542419 -0.36944580078125
3.72246932983398 -0.3695068359375
3.72255158424377 -0.3695068359375
3.72288060188293 -0.3695068359375
3.72296285629272 -0.36956787109375
3.72296285629272 -0.36956787109375
3.72320938110352 -0.36962890625
3.72353768348694 -0.36968994140625
3.72353768348694 -0.36968994140625
3.72361993789673 -0.36981201171875
3.72361993789673 -0.36981201171875
3.72427582740784 -0.369873046875
3.72435784339905 -0.36993408203125
3.72435784339905 -0.3699951171875
3.72435784339905 -0.3699951171875
3.72509455680847 -0.37005615234375
3.72509455680847 -0.37005615234375
3.72533988952637 -0.3701171875
3.72533988952637 -0.37017822265625
3.72533988952637 -0.37017822265625
3.72542142868042 -0.37017822265625
3.72623801231384 -0.370361328125
3.72623801231384 -0.370361328125
3.7263195514679 -0.37042236328125
3.72875952720642 -0.37066650390625
3.72884058952332 -0.3707275390625
3.72884058952332 -0.3707275390625
3.72924590110779 -0.37078857421875
3.729407787323 -0.370849609375
3.72956967353821 -0.37091064453125
3.72956967353821 -0.37091064453125
3.73005509376526 -0.37091064453125
3.73013591766357 -0.37103271484375
3.73062086105347 -0.37109375
3.73062086105347 -0.37109375
3.7307014465332 -0.37109375
3.7307014465332 -0.37109375
3.7307014465332 -0.37115478515625
3.73078227043152 -0.37115478515625
3.7332775592804 -0.371337890625
3.73335790634155 -0.37139892578125
3.73343801498413 -0.3714599609375
3.73367857933044 -0.3714599609375
3.7337589263916 -0.37158203125
3.73423957824707 -0.37158203125
3.73431968688965 -0.37158203125
3.73439979553223 -0.37164306640625
3.73471975326538 -0.37164306640625
3.73479986190796 -0.37164306640625
3.73479986190796 -0.3717041015625
3.73479986190796 -0.3717041015625
3.73559880256653 -0.371826171875
3.73559880256653 -0.37188720703125
3.73751068115234 -0.37225341796875
3.73759007453918 -0.372314453125
3.73759007453918 -0.372314453125
3.73798727989197 -0.3724365234375
3.73798727989197 -0.3724365234375
3.73798727989197 -0.3724365234375
3.73806667327881 -0.37249755859375
3.73806667327881 -0.37249755859375
3.73806667327881 -0.37249755859375
3.73854279518127 -0.37255859375
3.73854279518127 -0.37255859375
3.73862195014954 -0.37261962890625
3.73909735679626 -0.37261962890625
3.73917651176453 -0.3726806640625
3.73925590515137 -0.3726806640625
3.73925590515137 -0.3726806640625
3.73933506011963 -0.37274169921875
3.73980951309204 -0.37274169921875
3.74004673957825 -0.37286376953125
3.74186038970947 -0.37286376953125
3.74186038970947 -0.37286376953125
3.74186038970947 -0.3729248046875
3.74186038970947 -0.3729248046875
3.74186038970947 -0.3729248046875
3.74186038970947 -0.3729248046875
3.74225378036499 -0.373046875
3.74225378036499 -0.373046875
3.74248933792114 -0.373046875
3.74248933792114 -0.373046875
3.7431960105896 -0.37322998046875
3.7431960105896 -0.373291015625
3.7431960105896 -0.373291015625
3.7431960105896 -0.373291015625
3.7431960105896 -0.373291015625
3.74390149116516 -0.37335205078125
3.74390149116516 -0.3734130859375
3.74390149116516 -0.3734130859375
3.74390149116516 -0.3734130859375
3.74538707733154 -0.37347412109375
3.74538707733154 -0.37347412109375
3.74538707733154 -0.37353515625
3.74538707733154 -0.37353515625
3.74857568740845 -0.37445068359375
3.74857568740845 -0.37445068359375
3.74865317344666 -0.37445068359375
3.74896287918091 -0.37451171875
3.74904036521912 -0.37457275390625
3.74911761283875 -0.37457275390625
3.74911761283875 -0.37457275390625
3.74934983253479 -0.3746337890625
3.74958181381226 -0.3746337890625
3.74958181381226 -0.3746337890625
3.74965906143188 -0.37469482421875
3.74965906143188 -0.37469482421875
3.74965906143188 -0.37469482421875
3.74965906143188 -0.37469482421875
3.74965906143188 -0.37469482421875
3.75312328338623 -0.37481689453125
3.75312328338623 -0.37481689453125
3.75312328338623 -0.3748779296875
3.75312328338623 -0.3748779296875
3.75312328338623 -0.3748779296875
3.75419545173645 -0.37506103515625
3.75434827804565 -0.3751220703125
3.75434827804565 -0.3751220703125
3.75434827804565 -0.3751220703125
3.75442481040955 -0.3751220703125
3.75442481040955 -0.3751220703125
3.75450134277344 -0.37518310546875
3.75488328933716 -0.375244140625
3.75488328933716 -0.375244140625
3.75518846511841 -0.37530517578125
3.75518846511841 -0.37530517578125
3.75526475906372 -0.37530517578125
3.75526475906372 -0.37530517578125
3.75526475906372 -0.37530517578125
3.75526475906372 -0.3753662109375
3.75526475906372 -0.3753662109375
3.75709223747253 -0.3753662109375
3.75709223747253 -0.3753662109375
3.75747203826904 -0.37542724609375
3.7575478553772 -0.37542724609375
3.75762367248535 -0.37548828125
3.75762367248535 -0.37548828125
3.7580029964447 -0.37554931640625
3.7580029964447 -0.37554931640625
3.7580029964447 -0.37554931640625
3.7580029964447 -0.37554931640625
3.75807881355286 -0.3756103515625
3.75807881355286 -0.3756103515625
3.75807881355286 -0.3756103515625
3.75807881355286 -0.3756103515625
3.75807881355286 -0.3756103515625
3.7585334777832 -0.3756103515625
3.7585334777832 -0.3756103515625
3.7585334777832 -0.37567138671875
3.7585334777832 -0.37567138671875
3.7585334777832 -0.37567138671875
3.75891184806824 -0.375732421875
3.75891184806824 -0.375732421875
3.75891184806824 -0.375732421875
3.75898742675781 -0.375732421875
3.75898742675781 -0.375732421875
3.75898742675781 -0.37579345703125
3.75966787338257 -0.37579345703125
3.75966787338257 -0.37579345703125
3.75966787338257 -0.37579345703125
3.76425075531006 -0.376220703125
3.7643256187439 -0.37628173828125
3.7643256187439 -0.37628173828125
3.7643256187439 -0.37628173828125
3.7643256187439 -0.37628173828125
3.76440024375916 -0.37628173828125
3.76952505111694 -0.37725830078125
3.76982021331787 -0.37744140625
3.76996779441833 -0.37744140625
3.77048373222351 -0.37750244140625
3.77048373222351 -0.37750244140625
3.77055740356445 -0.37750244140625
3.7706310749054 -0.37750244140625
3.77144050598145 -0.3775634765625
3.77151393890381 -0.3775634765625
3.77151393890381 -0.3775634765625
3.77151393890381 -0.3775634765625
3.77210164070129 -0.377685546875
3.77217483520508 -0.377685546875
3.77217483520508 -0.377685546875
3.7723217010498 -0.37774658203125
3.77246832847595 -0.37774658203125
3.77254176139832 -0.37774658203125
3.77276158332825 -0.37774658203125
3.77327442169189 -0.37774658203125
3.77327442169189 -0.3778076171875
3.77327442169189 -0.3778076171875
3.7737865447998 -0.37786865234375
3.7737865447998 -0.37786865234375
3.77385950088501 -0.37786865234375
3.77429795265198 -0.37786865234375
3.77429795265198 -0.37786865234375
3.77524614334106 -0.37799072265625
3.77531909942627 -0.37799072265625
3.77539205551147 -0.37799072265625
3.77561044692993 -0.37799072265625
3.77568316459656 -0.3780517578125
3.77590155601501 -0.3780517578125
3.77590155601501 -0.3780517578125
3.77590155601501 -0.3780517578125
3.77597427368164 -0.3780517578125
3.7766284942627 -0.3780517578125
3.77684640884399 -0.37811279296875
3.77691888809204 -0.37811279296875
3.77691888809204 -0.37811279296875
3.77706408500671 -0.37811279296875
3.77706408500671 -0.37811279296875
3.77706408500671 -0.37811279296875
3.77742671966553 -0.37811279296875
3.77742671966553 -0.37811279296875
3.7775719165802 -0.378173828125
3.7775719165802 -0.378173828125
3.7775719165802 -0.378173828125
3.7780065536499 -0.378173828125
3.7780065536499 -0.378173828125
3.77851295471191 -0.37823486328125
3.77851295471191 -0.37823486328125
3.77858543395996 -0.37823486328125
3.77966856956482 -0.3782958984375
3.77966856956482 -0.3782958984375
3.77966856956482 -0.3782958984375
3.77988505363464 -0.3782958984375
3.78010129928589 -0.37835693359375
3.78017330169678 -0.37835693359375
3.78024530410767 -0.37835693359375
3.78046131134033 -0.37835693359375
3.78046131134033 -0.37835693359375
3.78046131134033 -0.37835693359375
3.78046131134033 -0.37835693359375
3.78046131134033 -0.37841796875
3.78046131134033 -0.37841796875
3.78118062019348 -0.37841796875
3.78118062019348 -0.37841796875
3.78118062019348 -0.37841796875
3.7816116809845 -0.37847900390625
3.78168368339539 -0.37847900390625
3.78168368339539 -0.3785400390625
3.78211402893066 -0.3785400390625
3.78218579292297 -0.3785400390625
3.78218579292297 -0.3785400390625
3.78218579292297 -0.3785400390625
3.78232932090759 -0.3785400390625
3.78240084648132 -0.3785400390625
3.78254437446594 -0.3785400390625
3.78261590003967 -0.3785400390625
3.78261590003967 -0.37860107421875
3.78696417808533 -0.3790283203125
3.7870352268219 -0.37908935546875
3.78710603713989 -0.37908935546875
3.78710603713989 -0.37908935546875
3.78717708587646 -0.37908935546875
3.78724789619446 -0.37908935546875
3.78724789619446 -0.37908935546875
3.78738951683044 -0.379150390625
3.78738951683044 -0.379150390625
3.787602186203 -0.379150390625
3.78781461715698 -0.379150390625
3.78781461715698 -0.379150390625
3.78802680969238 -0.37921142578125
3.78802680969238 -0.37921142578125
3.78802680969238 -0.37921142578125
3.78809762001038 -0.37921142578125
3.78830981254578 -0.37921142578125
3.78830981254578 -0.37921142578125
3.78894567489624 -0.3792724609375
3.78901624679565 -0.3792724609375
3.78908681869507 -0.3792724609375
3.78908681869507 -0.3792724609375
3.78908681869507 -0.3792724609375
3.78908681869507 -0.3792724609375
3.78929853439331 -0.37933349609375
3.78929853439331 -0.37933349609375
3.78972172737122 -0.37933349609375
3.78986263275146 -0.37933349609375
3.78986263275146 -0.37933349609375
3.78986263275146 -0.37939453125
3.78986263275146 -0.37939453125
3.78986263275146 -0.37939453125
3.79049634933472 -0.37939453125
3.79049634933472 -0.37939453125
3.79049634933472 -0.37939453125
3.79056668281555 -0.37939453125
3.79070734977722 -0.37945556640625
3.79070734977722 -0.37945556640625
3.79070734977722 -0.37945556640625
3.79084777832031 -0.37945556640625
3.79084777832031 -0.37945556640625
3.79119920730591 -0.37945556640625
3.79126954078674 -0.3795166015625
3.79246163368225 -0.3795166015625
3.79253172874451 -0.3795166015625
3.79253172874451 -0.3795166015625
3.79330134391785 -0.379638671875
3.7934410572052 -0.379638671875
3.79351091384888 -0.379638671875
3.79372048377991 -0.379638671875
3.79379034042358 -0.379638671875
3.79386019706726 -0.37969970703125
3.79399991035461 -0.37969970703125
3.79399991035461 -0.37969970703125
3.79399991035461 -0.37969970703125
3.79399991035461 -0.37969970703125
3.79413938522339 -0.37969970703125
3.79413938522339 -0.37969970703125
3.79455780982971 -0.3797607421875
3.79455780982971 -0.3797607421875
3.79574108123779 -0.37982177734375
3.79588007926941 -0.37982177734375
3.79588007926941 -0.37982177734375
3.79588007926941 -0.37982177734375
3.79588007926941 -0.37982177734375
3.79594945907593 -0.37982177734375
3.79594945907593 -0.37982177734375
3.79629683494568 -0.3798828125
3.79629683494568 -0.3798828125
3.79629683494568 -0.3798828125
3.79629683494568 -0.3798828125
3.79629683494568 -0.3798828125
3.7963662147522 -0.3798828125
3.79657435417175 -0.3798828125
3.79657435417175 -0.37994384765625
3.79657435417175 -0.37994384765625
3.79719829559326 -0.37994384765625
3.79719829559326 -0.37994384765625
3.79733681678772 -0.37994384765625
3.79754447937012 -0.37994384765625
3.79754447937012 -0.37994384765625
3.79754447937012 -0.3800048828125
3.79754447937012 -0.3800048828125
3.79775214195251 -0.3800048828125
3.79795956611633 -0.3800048828125
3.79795956611633 -0.3800048828125
3.79802870750427 -0.3800048828125
3.79816699028015 -0.38006591796875
3.79816699028015 -0.38006591796875
3.79975390434265 -0.380126953125
3.79975390434265 -0.38018798828125
3.79989171028137 -0.38018798828125
3.79989171028137 -0.38018798828125
3.80002927780151 -0.38018798828125
3.80016708374023 -0.38018798828125
3.80030465126038 -0.38018798828125
3.80037331581116 -0.38018798828125
3.80044221878052 -0.38018798828125
3.80057954788208 -0.38018798828125
3.80057954788208 -0.38018798828125
3.800785779953 -0.3802490234375
3.80099177360535 -0.3802490234375
3.80106043815613 -0.3802490234375
3.80106043815613 -0.3802490234375
3.80106043815613 -0.3802490234375
3.80119776725769 -0.38031005859375
3.80126643180847 -0.38031005859375
3.80147218704224 -0.38031005859375
3.80147218704224 -0.38031005859375
3.80147218704224 -0.38031005859375
3.80338883399963 -0.3804931640625
3.80345702171326 -0.38055419921875
3.80345702171326 -0.38055419921875
3.80359363555908 -0.38055419921875
3.80359363555908 -0.38055419921875
3.80373024940491 -0.38055419921875
3.80407118797302 -0.38055419921875
3.80413937568665 -0.38055419921875
3.80413937568665 -0.380615234375
3.80413937568665 -0.380615234375
3.80482077598572 -0.38067626953125
3.80488872528076 -0.38067626953125
3.80502486228943 -0.38067626953125
3.80502486228943 -0.38067626953125
3.80522894859314 -0.3807373046875
3.80651903152466 -0.38079833984375
3.80679035186768 -0.38079833984375
3.80685806274414 -0.380859375
3.80692577362061 -0.380859375
3.80699348449707 -0.380859375
3.80719661712646 -0.380859375
3.80719661712646 -0.380859375
3.80719661712646 -0.380859375
3.80739974975586 -0.380859375
3.80746746063232 -0.380859375
3.80746746063232 -0.380859375
3.80760264396667 -0.380859375
3.80760264396667 -0.380859375
3.80760264396667 -0.380859375
3.80773782730103 -0.38092041015625
3.80787324905396 -0.38092041015625
3.80787324905396 -0.38092041015625
3.80787324905396 -0.38092041015625
3.80827856063843 -0.38092041015625
3.8084135055542 -0.38092041015625
3.8084135055542 -0.38092041015625
3.80854845046997 -0.3809814453125
3.80854845046997 -0.3809814453125
3.80861592292786 -0.3809814453125
3.80881834030151 -0.3809814453125
3.80902075767517 -0.3809814453125
3.80902075767517 -0.3809814453125
3.80962705612183 -0.3809814453125
3.80969429016113 -0.3809814453125
3.80969429016113 -0.3809814453125
3.80982899665833 -0.3809814453125
3.80982899665833 -0.38104248046875
3.80996346473694 -0.38104248046875
3.80996346473694 -0.38104248046875
3.80996346473694 -0.38104248046875
3.81016540527344 -0.38104248046875
3.81016540527344 -0.38104248046875
3.81023263931274 -0.381103515625
3.81036686897278 -0.381103515625
3.81036686897278 -0.381103515625
3.81063580513 -0.381103515625
3.81063580513 -0.381103515625
3.81103849411011 -0.381103515625
3.81110572814941 -0.381103515625
3.81110572814941 -0.381103515625
3.81123971939087 -0.381103515625
3.81123971939087 -0.381103515625
3.81130695343018 -0.38116455078125
3.81130695343018 -0.38116455078125
3.81144094467163 -0.38116455078125
3.81157493591309 -0.38116455078125
3.81157493591309 -0.38116455078125
3.81157493591309 -0.38116455078125
3.81157493591309 -0.38116455078125
3.81157493591309 -0.38116455078125
3.81170892715454 -0.38116455078125
3.81177592277527 -0.38116455078125
3.81177592277527 -0.38116455078125
3.81177592277527 -0.38116455078125
3.81190991401672 -0.38116455078125
3.81190991401672 -0.38116455078125
3.81190991401672 -0.38116455078125
3.81211090087891 -0.3812255859375
3.81257915496826 -0.3812255859375
3.81277966499329 -0.3812255859375
3.81284666061401 -0.3812255859375
3.81291341781616 -0.38128662109375
3.81304693222046 -0.38128662109375
3.81304693222046 -0.38128662109375
3.81304693222046 -0.38128662109375
3.81304693222046 -0.38128662109375
3.81304693222046 -0.38128662109375
3.81438088417053 -0.38128662109375
3.81438088417053 -0.38128662109375
3.81438088417053 -0.38134765625
3.8144474029541 -0.38134765625
3.8144474029541 -0.38134765625
3.8144474029541 -0.38134765625
3.81458044052124 -0.38134765625
3.81458044052124 -0.38134765625
3.81458044052124 -0.38134765625
3.81458044052124 -0.38134765625
3.81478023529053 -0.38134765625
3.81478023529053 -0.38134765625
3.81703615188599 -0.3814697265625
3.81703615188599 -0.3814697265625
3.81703615188599 -0.3814697265625
3.81710243225098 -0.3814697265625
3.81723475456238 -0.3814697265625
3.81723475456238 -0.3814697265625
3.81723475456238 -0.3814697265625
3.81723475456238 -0.3814697265625
3.81723475456238 -0.3814697265625
3.81736707687378 -0.3814697265625
3.81796169281006 -0.38165283203125
3.81868767738342 -0.38165283203125
3.81875348091125 -0.38165283203125
3.81875348091125 -0.38165283203125
3.81875348091125 -0.38165283203125
3.81881952285767 -0.38165283203125
3.8188853263855 -0.38165283203125
3.8188853263855 -0.38165283203125
3.8188853263855 -0.38165283203125
3.8188853263855 -0.38165283203125
3.8188853263855 -0.38165283203125
3.81901717185974 -0.38165283203125
3.81901717185974 -0.38165283203125
3.81908297538757 -0.38165283203125
3.81908297538757 -0.38165283203125
3.81908297538757 -0.38165283203125
3.81908297538757 -0.38165283203125
3.81908297538757 -0.38165283203125
3.82059550285339 -0.3817138671875
3.82059550285339 -0.38177490234375
3.82066106796265 -0.38177490234375
3.82066106796265 -0.38177490234375
3.82066106796265 -0.38177490234375
3.82066106796265 -0.38177490234375
3.821120262146 -0.38177490234375
3.821120262146 -0.38177490234375
3.821120262146 -0.38177490234375
3.821120262146 -0.38177490234375
3.821120262146 -0.3818359375
3.821120262146 -0.3818359375
3.821120262146 -0.3818359375
3.821120262146 -0.3818359375
3.82131695747375 -0.3818359375
3.82131695747375 -0.3818359375
3.82131695747375 -0.3818359375
3.82138252258301 -0.3818359375
3.82138252258301 -0.3818359375
3.82138252258301 -0.3818359375
3.82138252258301 -0.3818359375
3.82138252258301 -0.3818359375
3.82138252258301 -0.3818359375
3.82138252258301 -0.3818359375
3.82171010971069 -0.3818359375
3.82171010971069 -0.3818359375
3.82171010971069 -0.3818359375
3.82171010971069 -0.3818359375
3.82171010971069 -0.3818359375
3.82210254669189 -0.38189697265625
3.8222987651825 -0.38189697265625
3.82236433029175 -0.38189697265625
3.82236433029175 -0.38189697265625
3.82236433029175 -0.38189697265625
3.82366991043091 -0.3819580078125
3.82366991043091 -0.3819580078125
3.823734998703 -0.3819580078125
3.823734998703 -0.3819580078125
3.82386541366577 -0.38201904296875
3.82386541366577 -0.38201904296875
3.82393050193787 -0.38201904296875
3.82393050193787 -0.38201904296875
3.82425594329834 -0.38201904296875
3.82425594329834 -0.38201904296875
3.82432103157043 -0.38201904296875
3.82432103157043 -0.38201904296875
3.82432103157043 -0.38201904296875
3.82438611984253 -0.38201904296875
3.82438611984253 -0.38201904296875
3.82438611984253 -0.38201904296875
3.82438611984253 -0.38201904296875
3.82438611984253 -0.38201904296875
3.82445120811462 -0.38201904296875
3.82445120811462 -0.38201904296875
3.82445120811462 -0.382080078125
3.82445120811462 -0.382080078125
3.82445120811462 -0.382080078125
3.82477641105652 -0.382080078125
3.82484149932861 -0.382080078125
3.82490634918213 -0.382080078125
3.82536125183105 -0.38214111328125
3.82549095153809 -0.38214111328125
3.8255558013916 -0.38214111328125
3.8255558013916 -0.38214111328125
3.8255558013916 -0.38214111328125
3.8255558013916 -0.38214111328125
3.8255558013916 -0.38214111328125
3.8255558013916 -0.38214111328125
3.8255558013916 -0.38214111328125
3.82743382453918 -0.38238525390625
3.82762765884399 -0.3824462890625
3.82769227027893 -0.3824462890625
3.82775688171387 -0.3824462890625
3.8278214931488 -0.3824462890625
3.82801508903503 -0.3824462890625
3.82807970046997 -0.3824462890625
3.82807970046997 -0.3824462890625
3.82820868492126 -0.3824462890625
3.82820868492126 -0.3824462890625
3.83212566375732 -0.3824462890625
3.83212566375732 -0.3824462890625
3.83218955993652 -0.3824462890625
3.83218955993652 -0.38250732421875
3.83218955993652 -0.38250732421875
3.83218955993652 -0.38250732421875
3.83218955993652 -0.38250732421875
3.83218955993652 -0.38250732421875
3.83218955993652 -0.38250732421875
3.83225345611572 -0.38250732421875
3.83225345611572 -0.38250732421875
3.83225345611572 -0.38250732421875
3.83225345611572 -0.38250732421875
3.83225345611572 -0.38250732421875
3.83225345611572 -0.38250732421875
3.83225345611572 -0.38250732421875
3.83231735229492 -0.38250732421875
3.83238124847412 -0.38250732421875
3.83238124847412 -0.38250732421875
3.83238124847412 -0.38250732421875
3.83263659477234 -0.38250732421875
3.83263659477234 -0.382568359375
3.83263659477234 -0.382568359375
3.83270049095154 -0.382568359375
3.83276438713074 -0.382568359375
3.83276438713074 -0.382568359375
3.83276438713074 -0.382568359375
3.83276438713074 -0.382568359375
3.83276438713074 -0.382568359375
3.83282804489136 -0.382568359375
3.83282804489136 -0.382568359375
3.83282804489136 -0.382568359375
3.83282804489136 -0.382568359375
3.83282804489136 -0.382568359375
3.83282804489136 -0.382568359375
3.83448433876038 -0.3828125
3.83454775810242 -0.3828125
3.83454775810242 -0.3828125
3.83461141586304 -0.3828125
3.83461141586304 -0.3828125
3.83467507362366 -0.3828125
3.83467507362366 -0.3828125
3.8349289894104 -0.3828125
3.83499264717102 -0.3828125
3.83499264717102 -0.3828125
3.83505606651306 -0.3828125
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{ClOOCl}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.7184543132782,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.47347412109375, ymax=0.02254638671875,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c8)}
]
\addplot [ultra thick, brown, dashed]
table {%
1.07918119430542 0
1.86923170089722 -0.002685546875
1.92427933216095 -0.0028076171875
1.97312784194946 -0.0028076171875
2.02118921279907 -0.0028076171875
2.05307841300964 -0.0028076171875
2.07918119430542 -0.0028076171875
2.09690999984741 -0.0028076171875
2.43456888198853 -0.0030517578125
2.44870638847351 -0.0030517578125
2.51188325881958 -0.0030517578125
2.55145001411438 -0.0030517578125
2.56702637672424 -0.0030517578125
2.60852599143982 -0.0030517578125
2.83378434181213 -0.0030517578125
2.8457179069519 -0.0030517578125
3.03059983253479 -0.003173828125
3.04766416549683 -0.003173828125
3.06632590293884 -0.003173828125
3.06966805458069 -0.003173828125
3.07371830940247 -0.003173828125
3.0795431137085 -0.003173828125
3.08707118034363 -0.003173828125
3.10140323638916 -0.003173828125
3.10822677612305 -0.0032958984375
3.15654921531677 -0.0032958984375
3.16046857833862 -0.0032958984375
3.16554117202759 -0.0032958984375
3.1786892414093 -0.0032958984375
3.19173049926758 -0.0032958984375
3.19810700416565 -0.0032958984375
3.23754382133484 -0.0032958984375
3.26764106750488 -0.00341796875
3.26974630355835 -0.00341796875
3.33905363082886 -0.003662109375
3.36417555809021 -0.003662109375
3.36698293685913 -0.0037841796875
3.36865878105164 -0.0037841796875
3.37032794952393 -0.0037841796875
3.50160694122314 -0.004150390625
3.50731611251831 -0.004150390625
3.53019976615906 -0.004150390625
3.53173422813416 -0.0042724609375
3.53706312179565 -0.0042724609375
3.54282546043396 -0.00439453125
3.55594038963318 -0.00439453125
3.5569052696228 -0.00439453125
3.55858850479126 -0.00439453125
3.56949090957642 -0.0045166015625
3.57818055152893 -0.0045166015625
3.59417152404785 -0.0045166015625
3.59560656547546 -0.0045166015625
3.67513656616211 -0.005859375
3.67870044708252 -0.0062255859375
3.6845760345459 -0.0062255859375
3.69390273094177 -0.00634765625
3.80922293663025 -0.0078125
3.8153121471405 -0.0084228515625
3.84079599380493 -0.0087890625
3.84416651725769 -0.009033203125
3.84516000747681 -0.00927734375
3.8596785068512 -0.009521484375
3.8642144203186 -0.0096435546875
3.87932538986206 -0.0101318359375
3.92936778068542 -0.015380859375
3.94684505462646 -0.017333984375
3.95684051513672 -0.0177001953125
3.97552371025085 -0.0179443359375
4.00047731399536 -0.018798828125
4.00864267349243 -0.0191650390625
4.02563333511353 -0.019775390625
4.03498935699463 -0.020263671875
4.05926036834717 -0.024169921875
4.06625127792358 -0.026611328125
4.10030174255371 -0.03125
4.11347532272339 -0.0328369140625
4.12716960906982 -0.033935546875
4.14217042922974 -0.0352783203125
4.16524410247803 -0.0384521484375
4.18469142913818 -0.0430908203125
4.19189786911011 -0.0450439453125
4.20784950256348 -0.048583984375
4.22937440872192 -0.058349609375
4.24731016159058 -0.0635986328125
4.25918769836426 -0.0660400390625
4.27237558364868 -0.0684814453125
4.28575992584229 -0.071044921875
4.3095235824585 -0.077392578125
4.32399415969849 -0.0810546875
4.33843660354614 -0.0836181640625
4.34859704971313 -0.0855712890625
4.36000633239746 -0.08642578125
4.38129568099976 -0.09130859375
4.39567565917969 -0.09326171875
4.40534639358521 -0.0947265625
4.41695642471313 -0.09619140625
4.42566442489624 -0.0999755859375
4.43515920639038 -0.102783203125
4.44619512557983 -0.1048583984375
4.45562124252319 -0.1107177734375
4.47564220428467 -0.12060546875
4.49182367324829 -0.1279296875
4.50260448455811 -0.1328125
4.50972652435303 -0.1357421875
4.52967405319214 -0.1500244140625
4.53727769851685 -0.1558837890625
4.54693746566772 -0.16015625
4.5558557510376 -0.16357421875
4.56747341156006 -0.17041015625
4.57695150375366 -0.1754150390625
4.5839467048645 -0.1783447265625
4.59339666366577 -0.1815185546875
4.60234212875366 -0.1873779296875
4.60845136642456 -0.19140625
4.61526584625244 -0.1934814453125
4.62121772766113 -0.195556640625
4.62696599960327 -0.197265625
4.63309478759766 -0.2027587890625
4.63905811309814 -0.2042236328125
4.6476469039917 -0.212646484375
4.65138483047485 -0.216796875
4.66015386581421 -0.218505859375
4.66527128219604 -0.220947265625
4.66952133178711 -0.2218017578125
4.67321443557739 -0.22314453125
4.67837285995483 -0.2252197265625
4.68503379821777 -0.231201171875
4.68711853027344 -0.23291015625
4.69148826599121 -0.2340087890625
4.69726419448853 -0.235595703125
4.69975090026855 -0.2364501953125
4.70300769805908 -0.2374267578125
4.70665788650513 -0.23876953125
4.71283483505249 -0.2415771484375
4.7166543006897 -0.24267578125
4.71861791610718 -0.2431640625
4.72994184494019 -0.2509765625
4.734055519104 -0.2523193359375
4.73939037322998 -0.25537109375
4.74067831039429 -0.2567138671875
4.74537134170532 -0.2572021484375
4.74973630905151 -0.2589111328125
4.7533073425293 -0.2596435546875
4.75700092315674 -0.2608642578125
4.76027154922485 -0.2615966796875
4.76380205154419 -0.261962890625
4.77154350280762 -0.265625
4.77424669265747 -0.2664794921875
4.77725982666016 -0.267333984375
4.78011560440063 -0.267822265625
4.78589200973511 -0.2718505859375
4.78949594497681 -0.2728271484375
4.79246854782104 -0.2730712890625
4.79973316192627 -0.276123046875
4.80237674713135 -0.2767333984375
4.80467796325684 -0.2772216796875
4.80683088302612 -0.2777099609375
4.81009817123413 -0.2789306640625
4.81324052810669 -0.2808837890625
4.81791543960571 -0.282470703125
4.82060861587524 -0.282958984375
4.82326555252075 -0.2838134765625
4.8280987739563 -0.285400390625
4.83102464675903 -0.2874755859375
4.83359336853027 -0.28857421875
4.83539867401123 -0.2890625
4.83946561813354 -0.2911376953125
4.84330129623413 -0.2923583984375
4.84535217285156 -0.29296875
4.84733819961548 -0.29345703125
4.85008859634399 -0.2955322265625
4.8514232635498 -0.2958984375
4.85977458953857 -0.3099365234375
4.86125946044922 -0.3134765625
4.86483716964722 -0.3155517578125
4.86650609970093 -0.316650390625
4.86997079849243 -0.317138671875
4.88023042678833 -0.3243408203125
4.88113355636597 -0.325927734375
4.88258123397827 -0.3265380859375
4.88479518890381 -0.327392578125
4.88649082183838 -0.3280029296875
4.88968276977539 -0.328369140625
4.89252853393555 -0.3287353515625
4.89394474029541 -0.3292236328125
4.89682912826538 -0.3299560546875
4.90149116516113 -0.33056640625
4.902747631073 -0.3309326171875
4.90442323684692 -0.331298828125
4.91088581085205 -0.336181640625
4.91302394866943 -0.3370361328125
4.91798830032349 -0.3382568359375
4.92083787918091 -0.3392333984375
4.92557525634766 -0.3416748046875
4.92783212661743 -0.34228515625
4.93132066726685 -0.3426513671875
4.93911981582642 -0.3533935546875
4.94277667999268 -0.35595703125
4.94455194473267 -0.3563232421875
4.94848155975342 -0.358154296875
4.95085144042969 -0.358642578125
4.95500421524048 -0.359130859375
4.96225547790527 -0.35986328125
4.9634051322937 -0.3604736328125
4.96787548065186 -0.36279296875
4.9774169921875 -0.36474609375
4.97912931442261 -0.36669921875
4.98432493209839 -0.368408203125
4.98764371871948 -0.368896484375
4.98993921279907 -0.3692626953125
4.99587631225586 -0.3701171875
5.00032997131348 -0.37060546875
5.00443744659424 -0.3724365234375
5.00950193405151 -0.373779296875
5.01215791702271 -0.3746337890625
5.0148983001709 -0.3748779296875
5.01977682113647 -0.3798828125
5.02368879318237 -0.3804931640625
5.02619409561157 -0.381103515625
5.02797698974609 -0.3818359375
5.0296516418457 -0.383544921875
5.03126287460327 -0.384033203125
5.0363655090332 -0.388916015625
5.03725099563599 -0.389404296875
5.03923177719116 -0.3895263671875
5.04097414016724 -0.389892578125
5.04151487350464 -0.3900146484375
5.04281568527222 -0.3902587890625
5.04755115509033 -0.3909912109375
5.04827070236206 -0.39111328125
5.05053424835205 -0.3912353515625
5.05109071731567 -0.391357421875
5.05444812774658 -0.3916015625
5.05494213104248 -0.3916015625
5.05548524856567 -0.3917236328125
5.0612940788269 -0.3929443359375
5.06338214874268 -0.3929443359375
5.06394481658936 -0.39306640625
5.06777000427246 -0.393798828125
5.06892395019531 -0.3939208984375
5.07043695449829 -0.3939208984375
5.07233810424805 -0.39404296875
5.07298469543457 -0.39404296875
5.07941293716431 -0.3955078125
5.0797815322876 -0.395751953125
5.08708524703979 -0.397705078125
5.08933973312378 -0.3980712890625
5.09012413024902 -0.3980712890625
5.09408664703369 -0.3983154296875
5.09759044647217 -0.39892578125
5.09880638122559 -0.399169921875
5.09945964813232 -0.3992919921875
5.10087013244629 -0.3992919921875
5.10249519348145 -0.3994140625
5.10397148132324 -0.3995361328125
5.10678577423096 -0.400146484375
5.10824680328369 -0.400634765625
5.10907220840454 -0.4007568359375
5.11288642883301 -0.4027099609375
5.1151876449585 -0.403076171875
5.11599969863892 -0.4031982421875
5.12209129333496 -0.40771484375
5.12413215637207 -0.409912109375
5.12496376037598 -0.4100341796875
5.12614107131958 -0.4102783203125
5.12856101989746 -0.4110107421875
5.12897396087646 -0.4112548828125
5.13209009170532 -0.4117431640625
5.13259887695312 -0.4119873046875
5.13509130477905 -0.4130859375
5.13709783554077 -0.413330078125
5.13824892044067 -0.41357421875
5.13886451721191 -0.4136962890625
5.13929319381714 -0.413818359375
5.14356136322021 -0.4151611328125
5.14491033554077 -0.4154052734375
5.1456036567688 -0.4154052734375
5.14877557754517 -0.4156494140625
5.15015745162964 -0.415771484375
5.15081167221069 -0.4158935546875
5.15226078033447 -0.4158935546875
5.15359210968018 -0.416015625
5.15407705307007 -0.416015625
5.1559157371521 -0.4161376953125
5.15681838989258 -0.4161376953125
5.16074180603027 -0.4180908203125
5.16294050216675 -0.4183349609375
5.16564798355103 -0.4185791015625
5.16661977767944 -0.418701171875
5.16822338104248 -0.4188232421875
5.16866254806519 -0.4188232421875
5.17248344421387 -0.4208984375
5.17346906661987 -0.42138671875
5.17607402801514 -0.4217529296875
5.17691850662231 -0.421875
5.17813920974731 -0.4219970703125
5.18033218383789 -0.42236328125
5.18053007125854 -0.42236328125
5.18450975418091 -0.4229736328125
5.18558168411255 -0.4229736328125
5.18630075454712 -0.4229736328125
5.18671894073486 -0.423095703125
5.18743324279785 -0.423095703125
5.18776607513428 -0.4232177734375
5.18837451934814 -0.4232177734375
5.18992519378662 -0.42333984375
5.19054460525513 -0.42333984375
5.1919732093811 -0.42333984375
5.193528175354 -0.4234619140625
5.19419765472412 -0.4234619140625
5.19596862792969 -0.423583984375
5.19609069824219 -0.423583984375
5.19641399383545 -0.4237060546875
5.19673681259155 -0.4237060546875
5.19710683822632 -0.423828125
5.19769144058228 -0.423828125
5.19877243041992 -0.423828125
5.20076036453247 -0.4239501953125
5.20360374450684 -0.4241943359375
5.20391893386841 -0.42431640625
5.20430707931519 -0.4244384765625
5.20645093917847 -0.4248046875
5.2080864906311 -0.4248046875
5.20938348770142 -0.4248046875
5.20969438552856 -0.4249267578125
5.21039628982544 -0.4249267578125
5.21185159683228 -0.4249267578125
5.2134485244751 -0.425048828125
5.21586465835571 -0.4251708984375
5.21610498428345 -0.42529296875
5.21727323532104 -0.4254150390625
5.21825456619263 -0.4254150390625
5.21887397766113 -0.425537109375
5.21987533569336 -0.425537109375
5.22095775604248 -0.4256591796875
5.22193813323975 -0.4256591796875
5.22288799285889 -0.4256591796875
5.22529125213623 -0.4259033203125
5.22570466995239 -0.4259033203125
5.22690916061401 -0.4259033203125
5.22824382781982 -0.426025390625
5.22931575775146 -0.4261474609375
5.23013734817505 -0.4261474609375
5.23177528381348 -0.4261474609375
5.23425149917603 -0.4263916015625
5.23505115509033 -0.4263916015625
5.23802852630615 -0.4268798828125
5.23824167251587 -0.427001953125
5.24159622192383 -0.4285888671875
5.24252653121948 -0.428955078125
5.24339294433594 -0.428955078125
5.2447247505188 -0.42919921875
5.24804925918579 -0.4306640625
5.24909782409668 -0.431396484375
5.25056886672974 -0.431640625
5.25180101394653 -0.431884765625
5.25263452529907 -0.4320068359375
5.25333547592163 -0.43212890625
5.25505065917969 -0.4324951171875
5.25601243972778 -0.4326171875
5.25699663162231 -0.4326171875
5.25805282592773 -0.4327392578125
5.25956058502197 -0.4332275390625
5.26045799255371 -0.433349609375
5.26104879379272 -0.4334716796875
5.26218032836914 -0.43359375
5.26292085647583 -0.4337158203125
5.26364088058472 -0.433837890625
5.26493835449219 -0.43408203125
5.26549243927002 -0.43408203125
5.26696968078613 -0.4351806640625
5.26753330230713 -0.435302734375
5.26803016662598 -0.4354248046875
5.26879072189331 -0.4354248046875
5.26981163024902 -0.4364013671875
5.27029466629028 -0.4366455078125
5.27154636383057 -0.436767578125
5.27211093902588 -0.4368896484375
5.27273941040039 -0.4368896484375
5.27417612075806 -0.4373779296875
5.27468633651733 -0.4373779296875
5.2756290435791 -0.4375
5.27643203735352 -0.4376220703125
5.27671003341675 -0.4376220703125
5.27701044082642 -0.4376220703125
5.27726984024048 -0.4376220703125
5.27800989151001 -0.437744140625
5.27847242355347 -0.437744140625
5.27872610092163 -0.437744140625
5.27908706665039 -0.437744140625
5.27948904037476 -0.437744140625
5.28017282485962 -0.4378662109375
5.28058958053589 -0.43798828125
5.28078985214233 -0.43798828125
5.28118562698364 -0.43798828125
5.28144931793213 -0.43798828125
5.28234100341797 -0.4384765625
5.28258609771729 -0.4384765625
5.28302955627441 -0.438720703125
5.28323793411255 -0.438720703125
5.28360891342163 -0.438720703125
5.28381443023682 -0.438720703125
5.28434276580811 -0.438720703125
5.28575992584229 -0.43896484375
5.28603410720825 -0.4390869140625
5.28633499145508 -0.4390869140625
5.28638458251953 -0.4390869140625
5.28721952438354 -0.439208984375
5.28741884231567 -0.439208984375
5.28765392303467 -0.439208984375
5.28776168823242 -0.439208984375
5.28809022903442 -0.439208984375
5.28833436965942 -0.439208984375
5.28866958618164 -0.439208984375
5.28905344009399 -0.4393310546875
5.28927898406982 -0.4393310546875
5.28964900970459 -0.4393310546875
5.28972482681274 -0.4393310546875
5.28990745544434 -0.4393310546875
5.29020404815674 -0.4393310546875
5.29109573364258 -0.439453125
5.29143333435059 -0.439453125
5.291832447052 -0.4395751953125
5.29193258285522 -0.4395751953125
5.29214763641357 -0.4395751953125
5.29228258132935 -0.4395751953125
5.29248857498169 -0.4395751953125
5.29267930984497 -0.4395751953125
5.29303550720215 -0.4395751953125
5.29354381561279 -0.4395751953125
5.29400968551636 -0.439697265625
5.29436922073364 -0.439697265625
5.29447746276855 -0.439697265625
5.2949595451355 -0.439697265625
5.29514694213867 -0.439697265625
5.29547691345215 -0.439697265625
5.29550981521606 -0.439697265625
5.29582643508911 -0.439697265625
5.29594755172729 -0.439697265625
5.29607248306274 -0.439697265625
5.29635143280029 -0.4398193359375
5.29668712615967 -0.4398193359375
5.29675722122192 -0.4398193359375
5.2973575592041 -0.4398193359375
5.2976861000061 -0.4398193359375
5.29811477661133 -0.4398193359375
5.29824829101562 -0.4398193359375
5.29847097396851 -0.4398193359375
5.2986216545105 -0.4398193359375
5.30106258392334 -0.4412841796875
5.30179166793823 -0.4415283203125
5.30208396911621 -0.4415283203125
5.30278301239014 -0.4415283203125
5.30330419540405 -0.441650390625
5.30386972427368 -0.441650390625
5.30424499511719 -0.441650390625
5.30433320999146 -0.441650390625
5.30477285385132 -0.4417724609375
5.30597639083862 -0.4417724609375
5.30612897872925 -0.4417724609375
5.30633068084717 -0.4417724609375
5.30663108825684 -0.4417724609375
5.30684280395508 -0.4417724609375
5.30711936950684 -0.4417724609375
5.30740833282471 -0.4417724609375
5.30778026580811 -0.4417724609375
5.30801343917847 -0.44189453125
5.3083233833313 -0.44189453125
5.30873107910156 -0.44189453125
5.3105001449585 -0.4422607421875
5.31076145172119 -0.4423828125
5.31105613708496 -0.4423828125
5.31125783920288 -0.4423828125
5.31154203414917 -0.4423828125
5.31168174743652 -0.4423828125
5.31192111968994 -0.4425048828125
5.31216239929199 -0.4425048828125
5.31285810470581 -0.442626953125
5.31307363510132 -0.442626953125
5.31341171264648 -0.442626953125
5.31363105773926 -0.442626953125
5.31381893157959 -0.442626953125
5.31415796279907 -0.4427490234375
5.31572484970093 -0.4429931640625
5.31617784500122 -0.443115234375
5.31677293777466 -0.4432373046875
5.31701374053955 -0.4432373046875
5.31728172302246 -0.4432373046875
5.31758069992065 -0.4432373046875
5.31801128387451 -0.4432373046875
5.31862258911133 -0.4432373046875
5.3190541267395 -0.443359375
5.31916666030884 -0.443359375
5.31936836242676 -0.443359375
5.31960964202881 -0.443359375
5.31988430023193 -0.4434814453125
5.32080459594727 -0.4434814453125
5.32106781005859 -0.4434814453125
5.32160902023315 -0.4434814453125
5.32176208496094 -0.4434814453125
5.32194232940674 -0.4434814453125
5.32213258743286 -0.4434814453125
5.32233905792236 -0.4434814453125
5.32269287109375 -0.4434814453125
5.32287454605103 -0.4434814453125
5.32300233840942 -0.4434814453125
5.32327890396118 -0.4434814453125
5.3234395980835 -0.443603515625
5.32449865341187 -0.443603515625
5.32469177246094 -0.443603515625
5.32554626464844 -0.443603515625
5.32626008987427 -0.4437255859375
5.32632541656494 -0.4437255859375
5.32697677612305 -0.4437255859375
5.32719326019287 -0.4437255859375
5.32858562469482 -0.44384765625
5.32873201370239 -0.44384765625
5.32882976531982 -0.44384765625
5.32910680770874 -0.44384765625
5.32928991317749 -0.44384765625
5.3294792175293 -0.44384765625
5.32960319519043 -0.44384765625
5.3303165435791 -0.44384765625
5.33036088943481 -0.44384765625
5.33037328720093 -0.44384765625
5.33042573928833 -0.44384765625
5.33070182800293 -0.4439697265625
5.33113574981689 -0.4439697265625
5.33142948150635 -0.4439697265625
5.33221626281738 -0.4439697265625
5.33253955841064 -0.4439697265625
5.33261394500732 -0.4439697265625
5.33279180526733 -0.4439697265625
5.33328008651733 -0.4439697265625
5.33351564407349 -0.4439697265625
5.33427095413208 -0.4439697265625
5.33441352844238 -0.4439697265625
5.33492803573608 -0.444091796875
5.33510494232178 -0.444091796875
5.33727931976318 -0.4442138671875
5.33730554580688 -0.4442138671875
5.33790016174316 -0.4442138671875
5.33867979049683 -0.4443359375
5.3388466835022 -0.4443359375
5.3398609161377 -0.4443359375
5.34001350402832 -0.4443359375
5.34035873413086 -0.4443359375
5.34083652496338 -0.4443359375
5.34089183807373 -0.4443359375
5.34119892120361 -0.4443359375
5.34141492843628 -0.4443359375
5.34164237976074 -0.4443359375
5.34186744689941 -0.4443359375
5.34208297729492 -0.4444580078125
5.34217977523804 -0.4444580078125
5.34323310852051 -0.4444580078125
5.34331226348877 -0.4444580078125
5.34341430664062 -0.4444580078125
5.34419393539429 -0.4444580078125
5.34431934356689 -0.4444580078125
5.34450054168701 -0.4444580078125
5.34467315673828 -0.4444580078125
5.34479904174805 -0.4444580078125
5.34487152099609 -0.444580078125
5.34771251678467 -0.4454345703125
5.34838485717773 -0.445556640625
5.34847021102905 -0.445556640625
5.3491358757019 -0.445556640625
5.34921550750732 -0.445556640625
5.34933757781982 -0.445556640625
5.34960985183716 -0.445556640625
5.34965229034424 -0.445556640625
5.34969902038574 -0.445556640625
5.35241222381592 -0.4466552734375
5.35262060165405 -0.4468994140625
5.35322570800781 -0.4468994140625
5.35364723205566 -0.4468994140625
5.35402202606201 -0.4468994140625
5.35416603088379 -0.4468994140625
5.35435056686401 -0.4468994140625
5.35451936721802 -0.4468994140625
5.35461950302124 -0.4468994140625
5.35469055175781 -0.4468994140625
5.35598564147949 -0.447021484375
5.35650968551636 -0.447021484375
5.3566722869873 -0.447021484375
5.35755586624146 -0.447021484375
5.3576774597168 -0.4471435546875
5.35793304443359 -0.4471435546875
5.35810995101929 -0.4471435546875
5.35823392868042 -0.4471435546875
5.35848712921143 -0.4471435546875
5.35906314849854 -0.4471435546875
5.36011600494385 -0.4471435546875
5.3604588508606 -0.4471435546875
5.36061239242554 -0.4471435546875
5.3606595993042 -0.4471435546875
5.36077308654785 -0.4471435546875
5.36103439331055 -0.4471435546875
5.36128187179565 -0.4471435546875
5.36166191101074 -0.4471435546875
5.36171817779541 -0.4471435546875
5.36303615570068 -0.4473876953125
5.36318683624268 -0.4473876953125
5.36350679397583 -0.4473876953125
5.363844871521 -0.4473876953125
5.36386585235596 -0.4473876953125
5.3638768196106 -0.4473876953125
5.36468029022217 -0.4473876953125
5.36491107940674 -0.4473876953125
5.36502170562744 -0.4473876953125
5.3655252456665 -0.4473876953125
5.36574459075928 -0.4473876953125
5.36577224731445 -0.4473876953125
5.36581754684448 -0.4473876953125
5.36605501174927 -0.4473876953125
5.36635589599609 -0.4473876953125
5.36685228347778 -0.447509765625
5.36723470687866 -0.447509765625
5.36734104156494 -0.447509765625
5.36735391616821 -0.447509765625
5.36764097213745 -0.447509765625
5.36774921417236 -0.447509765625
5.36811399459839 -0.447509765625
5.36813831329346 -0.447509765625
5.36819410324097 -0.447509765625
5.36819744110107 -0.447509765625
5.36841726303101 -0.447509765625
5.36883163452148 -0.447509765625
5.36903762817383 -0.447509765625
5.36971282958984 -0.447509765625
5.36982774734497 -0.447509765625
5.37035942077637 -0.447509765625
5.37055206298828 -0.447509765625
5.37070369720459 -0.447509765625
5.37071466445923 -0.447509765625
5.37538385391235 -0.448486328125
5.37585210800171 -0.44873046875
5.37612962722778 -0.44873046875
5.37634325027466 -0.44873046875
5.37646389007568 -0.44873046875
5.37668466567993 -0.44873046875
5.37671375274658 -0.44873046875
5.37718963623047 -0.44873046875
5.37763929367065 -0.44873046875
5.37768697738647 -0.44873046875
5.37803983688354 -0.44873046875
5.37840700149536 -0.44873046875
5.37843036651611 -0.44873046875
5.37843608856201 -0.4488525390625
5.37858867645264 -0.4488525390625
5.37877368927002 -0.4488525390625
5.37936162948608 -0.4488525390625
5.37940359115601 -0.4488525390625
5.37940883636475 -0.4488525390625
5.38006830215454 -0.4488525390625
5.38026189804077 -0.4488525390625
5.38041400909424 -0.4488525390625
5.38122892379761 -0.4488525390625
5.38137149810791 -0.4488525390625
5.38169240951538 -0.4488525390625
5.38182973861694 -0.4488525390625
5.38184785842896 -0.4488525390625
5.38190174102783 -0.4488525390625
5.3823356628418 -0.4488525390625
5.38249588012695 -0.4488525390625
5.38261842727661 -0.4488525390625
5.38278245925903 -0.4488525390625
5.38279867172241 -0.4488525390625
5.38292789459229 -0.4488525390625
5.38351535797119 -0.4488525390625
5.38355493545532 -0.4488525390625
5.38357639312744 -0.4488525390625
5.38375091552734 -0.448974609375
5.38379573822021 -0.448974609375
5.38380098342896 -0.448974609375
5.38402700424194 -0.448974609375
5.38433742523193 -0.448974609375
5.38443565368652 -0.448974609375
5.38455581665039 -0.448974609375
5.38470649719238 -0.448974609375
5.38475656509399 -0.448974609375
5.38476181030273 -0.448974609375
5.38476705551147 -0.448974609375
5.38536310195923 -0.448974609375
5.38557767868042 -0.448974609375
5.38566160202026 -0.448974609375
5.38571357727051 -0.448974609375
5.38583326339722 -0.448974609375
5.38595485687256 -0.448974609375
5.3859601020813 -0.448974609375
5.38726902008057 -0.448974609375
5.38741493225098 -0.448974609375
5.38788986206055 -0.448974609375
5.38810634613037 -0.448974609375
5.38850784301758 -0.4490966796875
5.38851881027222 -0.4490966796875
5.38858413696289 -0.4490966796875
5.38858985900879 -0.4490966796875
5.38864803314209 -0.4490966796875
5.38865518569946 -0.4490966796875
5.38903474807739 -0.4490966796875
5.38904571533203 -0.4490966796875
5.38920164108276 -0.4490966796875
5.39078521728516 -0.44921875
5.39092254638672 -0.44921875
5.39106225967407 -0.44921875
5.39119100570679 -0.44921875
5.39136219024658 -0.44921875
5.39165496826172 -0.44921875
5.39207744598389 -0.44921875
5.39233112335205 -0.44921875
5.39247512817383 -0.44921875
5.39325761795044 -0.44921875
5.39343500137329 -0.44921875
5.39350318908691 -0.44921875
5.39355945587158 -0.44921875
5.39367341995239 -0.44921875
5.39378213882446 -0.44921875
5.39383506774902 -0.44921875
5.39383983612061 -0.44921875
5.3938455581665 -0.44921875
5.39484214782715 -0.44921875
5.39495038986206 -0.44921875
5.39527940750122 -0.44921875
5.39534902572632 -0.44921875
5.39549589157104 -0.4493408203125
5.3958592414856 -0.4493408203125
5.39602994918823 -0.4493408203125
5.39616250991821 -0.4493408203125
5.39632844924927 -0.4493408203125
5.39695024490356 -0.4493408203125
5.39725494384766 -0.4493408203125
5.3972601890564 -0.4493408203125
5.39742565155029 -0.4493408203125
5.39934825897217 -0.449462890625
5.39949035644531 -0.449462890625
5.39958047866821 -0.449462890625
5.40014600753784 -0.449462890625
5.400634765625 -0.449462890625
5.40068626403809 -0.449462890625
5.40082120895386 -0.449462890625
5.40136098861694 -0.4495849609375
5.40151786804199 -0.4495849609375
5.4015417098999 -0.4495849609375
5.40156412124634 -0.4495849609375
5.401686668396 -0.4495849609375
5.401771068573 -0.4495849609375
5.40188455581665 -0.4495849609375
5.40200996398926 -0.4495849609375
5.40202760696411 -0.4495849609375
5.40203237533569 -0.4495849609375
5.40229749679565 -0.4495849609375
5.40286827087402 -0.4495849609375
5.40301942825317 -0.4495849609375
5.40303993225098 -0.4495849609375
5.40308284759521 -0.4495849609375
5.40308809280396 -0.4495849609375
5.40359735488892 -0.4495849609375
5.40383243560791 -0.4495849609375
5.40383768081665 -0.4495849609375
5.40396404266357 -0.4495849609375
5.40428447723389 -0.4495849609375
5.40428972244263 -0.4495849609375
5.40429496765137 -0.4495849609375
5.40485095977783 -0.4495849609375
5.40485572814941 -0.4495849609375
5.4050235748291 -0.4495849609375
5.40523719787598 -0.4495849609375
5.40528297424316 -0.4495849609375
5.40535831451416 -0.4495849609375
5.40559387207031 -0.4495849609375
5.40559911727905 -0.4495849609375
5.40567398071289 -0.4495849609375
5.40567922592163 -0.4495849609375
5.40568447113037 -0.4495849609375
5.40596437454224 -0.4495849609375
5.40596914291382 -0.4495849609375
5.4065523147583 -0.4495849609375
5.4066424369812 -0.4495849609375
5.40664768218994 -0.4495849609375
5.40675115585327 -0.4495849609375
5.40675640106201 -0.4495849609375
5.40703725814819 -0.4495849609375
5.40710544586182 -0.4495849609375
5.4071102142334 -0.4495849609375
5.40716981887817 -0.4495849609375
5.40759992599487 -0.44970703125
5.40807723999023 -0.44970703125
5.40821599960327 -0.44970703125
5.40848588943481 -0.44970703125
5.40855884552002 -0.44970703125
5.40861129760742 -0.44970703125
5.40896558761597 -0.44970703125
5.40926504135132 -0.44970703125
5.40929555892944 -0.44970703125
5.40950727462769 -0.44970703125
5.41012048721313 -0.44970703125
5.41012763977051 -0.44970703125
5.41023731231689 -0.44970703125
5.41031980514526 -0.44970703125
5.410325050354 -0.44970703125
5.41059684753418 -0.44970703125
5.41092395782471 -0.44970703125
5.41099977493286 -0.44970703125
5.4114818572998 -0.44970703125
5.41177129745483 -0.44970703125
5.41184854507446 -0.44970703125
5.41208219528198 -0.44970703125
5.41239500045776 -0.44970703125
5.41246223449707 -0.44970703125
5.41264009475708 -0.44970703125
5.41266393661499 -0.44970703125
5.41266870498657 -0.44970703125
5.4128737449646 -0.44970703125
5.41289377212524 -0.44970703125
5.41381072998047 -0.4498291015625
5.41395998001099 -0.4498291015625
5.41399526596069 -0.4498291015625
5.41406726837158 -0.4498291015625
5.41441535949707 -0.4498291015625
5.41478967666626 -0.4498291015625
5.4148097038269 -0.4498291015625
5.41497325897217 -0.4498291015625
5.41511869430542 -0.4498291015625
5.41527080535889 -0.4498291015625
5.41552591323853 -0.4498291015625
5.4155707359314 -0.4498291015625
5.41557598114014 -0.4498291015625
5.41596603393555 -0.4498291015625
5.41598606109619 -0.4498291015625
5.41627073287964 -0.4498291015625
5.41629600524902 -0.4498291015625
5.41682004928589 -0.4498291015625
5.41717767715454 -0.4498291015625
5.41718244552612 -0.4498291015625
5.41738700866699 -0.4498291015625
5.41739177703857 -0.4498291015625
5.41749477386475 -0.4498291015625
5.4178204536438 -0.4498291015625
5.41896533966064 -0.449951171875
5.41921520233154 -0.449951171875
5.41944360733032 -0.449951171875
5.41975927352905 -0.449951171875
5.41976594924927 -0.449951171875
5.41998052597046 -0.449951171875
5.42000532150269 -0.449951171875
5.42001008987427 -0.449951171875
5.42032241821289 -0.449951171875
5.42032718658447 -0.449951171875
5.42033195495605 -0.449951171875
5.42050361633301 -0.449951171875
5.42093706130981 -0.449951171875
5.42133092880249 -0.449951171875
5.42186880111694 -0.449951171875
5.42192792892456 -0.449951171875
5.42195749282837 -0.449951171875
5.42203140258789 -0.449951171875
5.42224025726318 -0.449951171875
5.42326879501343 -0.4500732421875
5.42332601547241 -0.4500732421875
5.42334604263306 -0.4500732421875
5.42335081100464 -0.4500732421875
5.42336702346802 -0.4500732421875
5.42349147796631 -0.4500732421875
5.42349672317505 -0.4500732421875
5.42375183105469 -0.4500732421875
5.42380428314209 -0.4500732421875
5.42426061630249 -0.4500732421875
5.42427730560303 -0.4500732421875
5.4243016242981 -0.4500732421875
5.42440795898438 -0.4500732421875
5.42446327209473 -0.4500732421875
5.42473316192627 -0.4500732421875
5.42473793029785 -0.4500732421875
5.42512798309326 -0.4500732421875
5.42550992965698 -0.4500732421875
5.42556524276733 -0.4500732421875
5.42568111419678 -0.4500732421875
5.42571020126343 -0.4500732421875
5.42624759674072 -0.4500732421875
5.42636823654175 -0.4500732421875
5.42643308639526 -0.4500732421875
5.42653226852417 -0.4500732421875
5.42664480209351 -0.4500732421875
5.42664957046509 -0.4500732421875
5.42694520950317 -0.4500732421875
5.42699909210205 -0.4500732421875
5.42728662490845 -0.4500732421875
5.42733335494995 -0.4500732421875
5.42746019363403 -0.4500732421875
5.42755889892578 -0.4500732421875
5.42766952514648 -0.4500732421875
5.42781066894531 -0.4500732421875
5.42822551727295 -0.4500732421875
5.42826747894287 -0.4500732421875
5.42835521697998 -0.4500732421875
5.42835998535156 -0.4500732421875
5.42838096618652 -0.4500732421875
5.42890691757202 -0.4500732421875
5.42963933944702 -0.4501953125
5.42973136901855 -0.4501953125
5.42985868453979 -0.4501953125
5.42996072769165 -0.4501953125
5.43012809753418 -0.4501953125
5.43040227890015 -0.4501953125
5.43043327331543 -0.4501953125
5.43065071105957 -0.4501953125
5.43075037002563 -0.4501953125
5.43092584609985 -0.4501953125
5.43093109130859 -0.4501953125
5.43102407455444 -0.4501953125
5.43127679824829 -0.4501953125
5.43128156661987 -0.4501953125
5.43213653564453 -0.4501953125
5.43220567703247 -0.4501953125
5.43221855163574 -0.4501953125
5.43224763870239 -0.4501953125
5.4324254989624 -0.4501953125
5.43243026733398 -0.4501953125
5.43261957168579 -0.4501953125
5.43262481689453 -0.4501953125
5.43287467956543 -0.4501953125
5.43303155899048 -0.4501953125
5.43319845199585 -0.4501953125
5.43320322036743 -0.4501953125
5.43367719650269 -0.4501953125
5.43368196487427 -0.4501953125
5.43368673324585 -0.4501953125
5.43471717834473 -0.4503173828125
5.43476343154907 -0.4503173828125
5.43491983413696 -0.4503173828125
5.43513202667236 -0.4503173828125
5.43513679504395 -0.4503173828125
5.43525171279907 -0.4503173828125
5.43547010421753 -0.4503173828125
5.43547487258911 -0.4503173828125
5.43562126159668 -0.4503173828125
5.43568992614746 -0.4503173828125
5.43571519851685 -0.4503173828125
5.43604183197021 -0.4503173828125
5.43605899810791 -0.4503173828125
5.43609094619751 -0.4503173828125
5.43666648864746 -0.4503173828125
5.43669509887695 -0.4503173828125
5.43673181533813 -0.4503173828125
5.43824815750122 -0.450439453125
5.43834447860718 -0.450439453125
5.43842220306396 -0.450439453125
5.43851852416992 -0.450439453125
5.43854570388794 -0.450439453125
5.4385929107666 -0.450439453125
5.43864059448242 -0.450439453125
5.43912887573242 -0.450439453125
5.43917322158813 -0.450439453125
5.43955707550049 -0.450439453125
5.43964195251465 -0.450439453125
5.43973541259766 -0.450439453125
5.43994522094727 -0.450439453125
5.44019079208374 -0.4505615234375
5.44024753570557 -0.4505615234375
5.44035959243774 -0.4505615234375
5.44040822982788 -0.4505615234375
5.44118738174438 -0.4505615234375
5.4415397644043 -0.4505615234375
5.44156646728516 -0.4505615234375
5.44170141220093 -0.4505615234375
5.44174861907959 -0.4505615234375
5.44210624694824 -0.4505615234375
5.44215059280396 -0.4505615234375
5.44234800338745 -0.4505615234375
5.44247961044312 -0.4505615234375
5.44256591796875 -0.4505615234375
5.44258499145508 -0.4505615234375
5.44262075424194 -0.4505615234375
5.44282150268555 -0.4505615234375
5.44289684295654 -0.4505615234375
5.44290924072266 -0.4505615234375
5.44326305389404 -0.4505615234375
5.44337701797485 -0.4505615234375
5.44354009628296 -0.4505615234375
5.44380903244019 -0.4505615234375
5.44383716583252 -0.4505615234375
5.44384336471558 -0.4505615234375
5.44402456283569 -0.4505615234375
5.44406175613403 -0.4505615234375
5.44406652450562 -0.4505615234375
5.44406986236572 -0.4505615234375
5.4441351890564 -0.4505615234375
5.44423675537109 -0.4505615234375
5.4442400932312 -0.4505615234375
5.44492483139038 -0.45068359375
5.44495010375977 -0.45068359375
5.44506978988647 -0.45068359375
5.44555616378784 -0.45068359375
5.44578170776367 -0.45068359375
5.44580793380737 -0.45068359375
5.44605207443237 -0.45068359375
5.44612836837769 -0.45068359375
5.44614696502686 -0.45068359375
};
\addplot [ultra thick, blue]
table {%
-inf 0
-inf -0.0028076171875
-inf -0.0028076171875
-inf -0.0028076171875
0 -0.0028076171875
0 -0.0028076171875
0 -0.0028076171875
0 -0.0028076171875
0 -0.0028076171875
0 -0.0028076171875
0 -0.0028076171875
0 -0.0028076171875
0 -0.0028076171875
0 -0.0028076171875
0 -0.0029296875
0 -0.0029296875
0 -0.0029296875
0 -0.0029296875
0 -0.0029296875
0 -0.0029296875
0 -0.0029296875
0 -0.0029296875
0 -0.0029296875
0.60206001996994 -0.0035400390625
0.60206001996994 -0.003662109375
0.60206001996994 -0.003662109375
0.60206001996994 -0.003662109375
0.60206001996994 -0.003662109375
0.60206001996994 -0.003662109375
0.60206001996994 -0.0037841796875
0.60206001996994 -0.0037841796875
0.60206001996994 -0.0037841796875
0.698970019817352 -0.0037841796875
1.57978355884552 -0.0118408203125
1.62324929237366 -0.0220947265625
1.66275787353516 -0.02294921875
1.69896996021271 -0.0235595703125
1.78532981872559 -0.0264892578125
1.81954395771027 -0.0277099609375
1.97312784194946 -0.0313720703125
1.9956351518631 -0.032470703125
2.02118921279907 -0.033935546875
2.06069779396057 -0.03515625
2.11058974266052 -0.0379638671875
2.13033366203308 -0.0396728515625
2.17897701263428 -0.0408935546875
2.19589972496033 -0.042236328125
2.30963015556335 -0.053955078125
2.32633590698242 -0.058349609375
2.35218262672424 -0.062744140625
2.39269685745239 -0.0703125
2.47712135314941 -0.079345703125
2.56702637672424 -0.093017578125
2.58319878578186 -0.099609375
2.60206007957458 -0.1011962890625
2.63447737693787 -0.1094970703125
2.67669367790222 -0.1138916015625
2.70757007598877 -0.1170654296875
2.74663424491882 -0.123046875
2.75891184806824 -0.125732421875
2.78461718559265 -0.12841796875
2.79657435417175 -0.1314697265625
2.82020139694214 -0.1343994140625
2.838219165802 -0.1383056640625
2.85612440109253 -0.1417236328125
2.8727388381958 -0.1436767578125
2.88705444335938 -0.14599609375
2.91275334358215 -0.15380859375
2.9232439994812 -0.1561279296875
2.92788338661194 -0.1572265625
2.94200801849365 -0.16259765625
2.94694328308105 -0.1666259765625
2.95808577537537 -0.168212890625
2.97451162338257 -0.173095703125
2.98587536811829 -0.17578125
2.98989462852478 -0.1781005859375
3.00389122962952 -0.1800537109375
3.01199316978455 -0.181640625
3.01953172683716 -0.183837890625
3.03302145004272 -0.1873779296875
3.04139280319214 -0.189208984375
3.04883003234863 -0.191162109375
3.08098697662354 -0.197509765625
3.08707118034363 -0.1998291015625
3.10482835769653 -0.20947265625
3.11193418502808 -0.2149658203125
3.11527752876282 -0.21630859375
3.12287092208862 -0.2197265625
3.12645602226257 -0.2208251953125
3.13289976119995 -0.22265625
3.14519643783569 -0.224365234375
3.15381479263306 -0.225830078125
3.15685200691223 -0.2265625
3.17026162147522 -0.2354736328125
3.1737687587738 -0.23876953125
3.17753648757935 -0.2401123046875
3.18355464935303 -0.240966796875
3.18920946121216 -0.2421875
3.20411992073059 -0.2490234375
3.20870995521545 -0.2510986328125
3.21298623085022 -0.2520751953125
3.21800994873047 -0.253173828125
3.2234959602356 -0.25390625
3.22788667678833 -0.2548828125
3.23502326011658 -0.2569580078125
3.23954963684082 -0.2584228515625
3.24821853637695 -0.264404296875
3.25261044502258 -0.2652587890625
3.25983262062073 -0.267333984375
3.26173853874207 -0.2679443359375
3.27160930633545 -0.2762451171875
3.27485036849976 -0.2781982421875
3.27783823013306 -0.2789306640625
3.28057837486267 -0.2799072265625
3.28284859657288 -0.28076171875
3.28690528869629 -0.2816162109375
3.28981184959412 -0.2822265625
3.29292035102844 -0.2828369140625
3.29600667953491 -0.2835693359375
3.30578112602234 -0.2918701171875
3.30963015556335 -0.29541015625
3.31952238082886 -0.29931640625
3.32221937179565 -0.3031005859375
3.32695007324219 -0.3056640625
3.33000779151917 -0.3084716796875
3.33825731277466 -0.3160400390625
3.34163236618042 -0.322265625
3.34654855728149 -0.326904296875
3.35024809837341 -0.3306884765625
3.35410833358765 -0.3330078125
3.35583448410034 -0.3348388671875
3.36116099357605 -0.33740234375
3.36304759979248 -0.33837890625
3.36492609977722 -0.3392333984375
3.36847281455994 -0.3397216796875
3.36958694458008 -0.34033203125
3.37235951423645 -0.3406982421875
3.37584638595581 -0.3416748046875
3.37839794158936 -0.342041015625
3.37966799736023 -0.3424072265625
3.3838152885437 -0.3431396484375
3.39339971542358 -0.349365234375
3.39567589759827 -0.3505859375
3.3963737487793 -0.3507080078125
3.40260529518127 -0.35205078125
3.40483379364014 -0.3526611328125
3.4072208404541 -0.3529052734375
3.40976405143738 -0.353515625
3.41396999359131 -0.354248046875
3.42078065872192 -0.354736328125
3.42258977890015 -0.35498046875
3.43312954902649 -0.3594970703125
3.43679857254028 -0.361328125
3.43870043754578 -0.361572265625
3.44513702392578 -0.3623046875
3.44855165481567 -0.3624267578125
3.45209312438965 -0.36328125
3.45591020584106 -0.363525390625
3.45848679542542 -0.3638916015625
3.46344494819641 -0.3643798828125
3.46908521652222 -0.3656005859375
3.47114491462708 -0.3658447265625
3.47871065139771 -0.36669921875
3.48072528839111 -0.3671875
3.49136161804199 -0.374267578125
3.49206161499023 -0.37841796875
3.500648021698 -0.3814697265625
3.50160694122314 -0.383056640625
3.50447082519531 -0.3837890625
3.506098985672 -0.3846435546875
3.50906801223755 -0.385009765625
3.51348400115967 -0.385986328125
3.51388311386108 -0.38623046875
3.51732778549194 -0.3868408203125
3.51772356033325 -0.3870849609375
3.5202214717865 -0.3878173828125
3.52113819122314 -0.3880615234375
3.52139973640442 -0.3883056640625
3.52361631393433 -0.3885498046875
3.52439618110657 -0.388671875
3.52633929252625 -0.388671875
3.52646851539612 -0.3887939453125
3.52840232849121 -0.388916015625
3.52853107452393 -0.3890380859375
3.5287880897522 -0.38916015625
3.53173422813416 -0.38916015625
3.53339076042175 -0.389404296875
3.53351783752441 -0.389404296875
3.54319858551025 -0.3909912109375
3.54332280158997 -0.39111328125
3.54419207572937 -0.39111328125
3.54518342018127 -0.3912353515625
3.54592537879944 -0.391357421875
3.54666614532471 -0.391357421875
3.54777479171753 -0.3914794921875
3.54961633682251 -0.3916015625
3.54973864555359 -0.3916015625
3.55181574821472 -0.39208984375
3.55461025238037 -0.3922119140625
3.55545711517334 -0.3922119140625
3.55606126785278 -0.392333984375
3.56133985519409 -0.3929443359375
3.56157827377319 -0.3929443359375
3.56324362754822 -0.3931884765625
3.56584787368774 -0.393310546875
3.56643748283386 -0.393310546875
3.56737923622131 -0.3934326171875
3.56749701499939 -0.3935546875
3.57077646255493 -0.3936767578125
3.5718252658844 -0.393798828125
3.571941614151 -0.393798828125
3.57795119285583 -0.39501953125
3.58274507522583 -0.3953857421875
3.58353877067566 -0.3955078125
3.58399176597595 -0.3956298828125
3.5882716178894 -0.3966064453125
3.5897262096405 -0.3968505859375
3.59050750732422 -0.39697265625
3.59150981903076 -0.3970947265625
3.59472393989563 -0.3973388671875
3.59527564048767 -0.3974609375
3.60042834281921 -0.3994140625
3.60238552093506 -0.3997802734375
3.60292768478394 -0.39990234375
3.60616636276245 -0.400390625
3.6084189414978 -0.4005126953125
3.60970115661621 -0.400634765625
3.61214780807495 -0.4007568359375
3.61426424980164 -0.4014892578125
3.61668562889099 -0.4017333984375
3.61909341812134 -0.40185546875
3.623042345047 -0.4029541015625
3.62459135055542 -0.4031982421875
3.62562108039856 -0.4031982421875
3.62869548797607 -0.4036865234375
3.63032627105713 -0.4041748046875
3.63316535949707 -0.404541015625
3.63397312164307 -0.4046630859375
3.63628721237183 -0.4051513671875
3.64097809791565 -0.405517578125
3.64147400856018 -0.4056396484375
3.64266228675842 -0.406005859375
3.64443850517273 -0.40625
3.64601135253906 -0.40625
3.65030741691589 -0.4066162109375
3.65185928344727 -0.406982421875
3.65292286872864 -0.4072265625
3.65388751029968 -0.4073486328125
3.65896487236023 -0.4080810546875
3.65991616249084 -0.4083251953125
3.66105508804321 -0.4085693359375
3.6618127822876 -0.40869140625
3.6637008190155 -0.4088134765625
3.66435980796814 -0.408935546875
3.67006015777588 -0.4093017578125
3.67098760604858 -0.4097900390625
3.67135810852051 -0.409912109375
3.67467737197876 -0.4117431640625
3.67815399169922 -0.412353515625
3.67851829528809 -0.4124755859375
3.67897343635559 -0.4127197265625
3.6801540851593 -0.412841796875
3.68069791793823 -0.4129638671875
3.68187403678894 -0.4132080078125
3.68313717842102 -0.4134521484375
3.68349742889404 -0.41357421875
3.68547296524048 -0.4140625
3.68708276748657 -0.4141845703125
3.68877553939819 -0.414306640625
3.68930888175964 -0.4144287109375
3.69037342071533 -0.41455078125
3.69143509864807 -0.414794921875
3.69416618347168 -0.4151611328125
3.69521903991699 -0.415283203125
3.69731664657593 -0.4154052734375
3.69731664657593 -0.4154052734375
3.70139527320862 -0.41650390625
3.70217204093933 -0.4166259765625
3.70492219924927 -0.416748046875
3.70569276809692 -0.4168701171875
3.70629096031189 -0.4168701171875
3.70739984512329 -0.4171142578125
3.70808076858521 -0.417236328125
3.7091851234436 -0.417236328125
3.70986342430115 -0.4176025390625
3.71239709854126 -0.4180908203125
3.71432971954346 -0.4183349609375
3.71499991416931 -0.41845703125
3.7155020236969 -0.4185791015625
3.71591973304749 -0.418701171875
3.71767044067383 -0.4188232421875
3.71800327301025 -0.4189453125
3.71841859817505 -0.4189453125
3.724848985672 -0.4229736328125
3.72509455680847 -0.4237060546875
3.72542142868042 -0.4237060546875
3.72697162628174 -0.424072265625
3.72745990753174 -0.4241943359375
3.72754120826721 -0.4241943359375
3.73086309432983 -0.4246826171875
3.73110508918762 -0.4246826171875
3.73158884048462 -0.4248046875
3.73231339454651 -0.4249267578125
3.73239374160767 -0.4249267578125
3.73239374160767 -0.4249267578125
3.73255467414856 -0.425048828125
3.73319721221924 -0.425048828125
3.73319721221924 -0.4251708984375
3.73351836204529 -0.4251708984375
3.73535943031311 -0.4254150390625
3.73631691932678 -0.4254150390625
3.73631691932678 -0.425537109375
3.73790788650513 -0.4256591796875
3.74241089820862 -0.426513671875
3.74241089820862 -0.4266357421875
3.74476218223572 -0.427001953125
3.74507474899292 -0.4271240234375
3.74585509300232 -0.4271240234375
3.74624490737915 -0.42724609375
3.74702310562134 -0.42724609375
3.74880790710449 -0.427490234375
3.74934983253479 -0.427490234375
3.75073981285095 -0.4276123046875
3.75089383125305 -0.4276123046875
3.75220203399658 -0.4278564453125
3.75450134277344 -0.427978515625
3.75488328933716 -0.427978515625
3.75974345207214 -0.430419921875
3.76004528999329 -0.43115234375
3.7632782459259 -0.4320068359375
3.7649974822998 -0.43212890625
3.76544499397278 -0.4322509765625
3.76700735092163 -0.4324951171875
3.76745271682739 -0.4327392578125
3.7701153755188 -0.4334716796875
3.77166104316711 -0.43359375
3.7718813419342 -0.4337158203125
3.77276158332825 -0.4337158203125
3.77684640884399 -0.435791015625
3.77851295471191 -0.43603515625
3.78110885620117 -0.4361572265625
3.78132438659668 -0.436279296875
3.78189897537231 -0.4364013671875
3.78304553031921 -0.4365234375
3.78340339660645 -0.4365234375
3.78724789619446 -0.439208984375
3.78958082199097 -0.43994140625
3.78979206085205 -0.4400634765625
3.79014444351196 -0.4400634765625
3.79028511047363 -0.440185546875
3.79049634933472 -0.440185546875
3.791339635849 -0.4403076171875
3.79218149185181 -0.4403076171875
3.79253172874451 -0.4404296875
3.79413938522339 -0.440673828125
3.79553246498108 -0.440673828125
3.7956714630127 -0.440673828125
3.79588007926941 -0.4407958984375
3.79664373397827 -0.44091796875
3.79671311378479 -0.44091796875
3.79671311378479 -0.4410400390625
3.79761362075806 -0.4410400390625
3.79768300056458 -0.4410400390625
3.79961609840393 -0.4415283203125
3.79968500137329 -0.4415283203125
3.79968500137329 -0.4415283203125
3.79996061325073 -0.4415283203125
3.80037331581116 -0.441650390625
3.80044221878052 -0.441650390625
3.8005108833313 -0.441650390625
3.80064845085144 -0.441650390625
3.80126643180847 -0.4417724609375
3.80126643180847 -0.4417724609375
3.80140376091003 -0.4417724609375
3.80140376091003 -0.4417724609375
3.80147218704224 -0.44189453125
3.80338883399963 -0.442138671875
3.80345702171326 -0.4422607421875
3.80352544784546 -0.4422607421875
3.80352544784546 -0.4422607421875
3.80366182327271 -0.4423828125
3.80366182327271 -0.4423828125
3.80366182327271 -0.4423828125
3.80366182327271 -0.4423828125
3.80468440055847 -0.4425048828125
3.80482077598572 -0.4425048828125
3.80488872528076 -0.4425048828125
3.80488872528076 -0.4425048828125
3.80502486228943 -0.4425048828125
3.80631566047668 -0.4427490234375
3.80638360977173 -0.4427490234375
3.80645132064819 -0.4427490234375
3.80651903152466 -0.4427490234375
3.80651903152466 -0.4427490234375
3.8065869808197 -0.44287109375
3.80665469169617 -0.44287109375
3.80672240257263 -0.44287109375
3.80726432800293 -0.44287109375
3.80733203887939 -0.44287109375
3.80739974975586 -0.44287109375
3.80746746063232 -0.44287109375
3.80753493309021 -0.44287109375
3.80753493309021 -0.4429931640625
3.80753493309021 -0.4429931640625
3.80881834030151 -0.443359375
3.8088858127594 -0.443359375
3.80902075767517 -0.443359375
3.80902075767517 -0.443359375
3.8105685710907 -0.4434814453125
3.81063580513 -0.4434814453125
3.81090426445007 -0.4434814453125
3.81103849411011 -0.443603515625
3.81110572814941 -0.443603515625
3.81117272377014 -0.443603515625
3.81123971939087 -0.443603515625
3.81217765808105 -0.4437255859375
3.81224465370178 -0.4437255859375
3.81271290779114 -0.4437255859375
3.81277966499329 -0.4437255859375
3.81284666061401 -0.4437255859375
3.81284666061401 -0.44384765625
3.81291341781616 -0.44384765625
3.81458044052124 -0.44384765625
3.81458044052124 -0.44384765625
3.8148467540741 -0.4439697265625
3.81491327285767 -0.4439697265625
3.81557774543762 -0.4439697265625
3.81564426422119 -0.444091796875
3.81571054458618 -0.444091796875
3.81577682495117 -0.444091796875
3.81584334373474 -0.444091796875
3.81584334373474 -0.444091796875
3.81617498397827 -0.444091796875
3.81617498397827 -0.444091796875
3.81617498397827 -0.4442138671875
3.81670522689819 -0.4442138671875
3.81677150726318 -0.4442138671875
3.81683754920959 -0.4442138671875
3.81690382957458 -0.4442138671875
3.81697010993958 -0.4442138671875
3.81697010993958 -0.4442138671875
3.81743311882019 -0.4443359375
3.8174991607666 -0.4443359375
3.8174991607666 -0.4443359375
3.8174991607666 -0.4443359375
3.81855583190918 -0.4444580078125
3.81868767738342 -0.4444580078125
3.81928062438965 -0.4444580078125
3.81934642791748 -0.444580078125
3.81934642791748 -0.444580078125
3.81934642791748 -0.444580078125
3.81934642791748 -0.444580078125
3.82340908050537 -0.445556640625
3.823734998703 -0.445556640625
3.82386541366577 -0.445556640625
3.82393050193787 -0.445556640625
3.82393050193787 -0.4456787109375
3.82399559020996 -0.4456787109375
3.82412576675415 -0.4456787109375
3.82412576675415 -0.4456787109375
3.82490634918213 -0.44580078125
3.82497143745422 -0.44580078125
3.82594513893127 -0.44580078125
3.82607483863831 -0.44580078125
3.82607483863831 -0.44580078125
3.82607483863831 -0.4459228515625
3.82607483863831 -0.4459228515625
3.82607483863831 -0.4459228515625
3.82607483863831 -0.4459228515625
3.82607483863831 -0.4459228515625
3.82607483863831 -0.4459228515625
3.82775688171387 -0.4459228515625
3.8278214931488 -0.4459228515625
3.8278214931488 -0.4459228515625
3.8278214931488 -0.4459228515625
3.8278214931488 -0.4459228515625
3.8278214931488 -0.4459228515625
3.8278214931488 -0.4459228515625
3.82833766937256 -0.446044921875
3.82840204238892 -0.446044921875
3.82904624938965 -0.446044921875
3.82917499542236 -0.446044921875
3.82917499542236 -0.446044921875
3.82917499542236 -0.446044921875
3.82923936843872 -0.446044921875
3.82930374145508 -0.446044921875
3.82930374145508 -0.4461669921875
3.82930374145508 -0.4461669921875
3.83071684837341 -0.4461669921875
3.83071684837341 -0.4461669921875
3.83071684837341 -0.4461669921875
3.83071684837341 -0.4461669921875
3.83078098297119 -0.4461669921875
3.83084511756897 -0.4461669921875
3.83084511756897 -0.4461669921875
3.83084511756897 -0.4461669921875
3.83084511756897 -0.4461669921875
3.83403897285461 -0.4464111328125
3.83410263061523 -0.4464111328125
3.83410263061523 -0.4464111328125
3.83708310127258 -0.4468994140625
3.83714628219604 -0.4468994140625
3.83720946311951 -0.4468994140625
3.83727264404297 -0.4468994140625
3.83739900588989 -0.4468994140625
3.838219165802 -0.447021484375
3.83828234672546 -0.447021484375
3.83828234672546 -0.447021484375
3.83834528923035 -0.447021484375
3.83840823173523 -0.447021484375
3.83840823173523 -0.447021484375
3.83840823173523 -0.447021484375
3.83853435516357 -0.447021484375
3.83853435516357 -0.447021484375
3.83853435516357 -0.447021484375
3.83853435516357 -0.447021484375
3.83853435516357 -0.447021484375
3.83910083770752 -0.4471435546875
3.8391637802124 -0.4471435546875
3.83922648429871 -0.4471435546875
3.83922648429871 -0.4471435546875
3.83922648429871 -0.4471435546875
3.83922648429871 -0.4471435546875
3.83928942680359 -0.4471435546875
3.83935236930847 -0.4471435546875
3.83935236930847 -0.4471435546875
3.84098386764526 -0.4471435546875
3.84098386764526 -0.4471435546875
3.84104633331299 -0.4471435546875
3.84110903739929 -0.4471435546875
3.84160971641541 -0.447265625
3.84167218208313 -0.447265625
3.84179735183716 -0.447265625
3.84179735183716 -0.447265625
3.84559416770935 -0.447509765625
3.84577989578247 -0.4476318359375
3.84584188461304 -0.4476318359375
3.8459038734436 -0.4476318359375
3.84596586227417 -0.4476318359375
3.84627532958984 -0.4476318359375
3.8463990688324 -0.4476318359375
3.8463990688324 -0.4476318359375
3.84646081924438 -0.4476318359375
3.84646081924438 -0.4476318359375
3.84646081924438 -0.44775390625
3.84646081924438 -0.44775390625
3.84646081924438 -0.44775390625
3.84905076026917 -0.4483642578125
3.84911203384399 -0.448486328125
3.84935808181763 -0.448486328125
3.84941935539246 -0.448486328125
3.84954214096069 -0.448486328125
3.84954214096069 -0.448486328125
3.85052371025085 -0.448486328125
3.85064625740051 -0.448486328125
3.85070753097534 -0.448486328125
3.85095238685608 -0.448486328125
3.85101366043091 -0.448486328125
3.85113596916199 -0.448486328125
3.85113596916199 -0.448486328125
3.85113596916199 -0.448486328125
3.85113596916199 -0.448486328125
3.85339403152466 -0.4486083984375
3.85345482826233 -0.4486083984375
3.853515625 -0.44873046875
3.85363745689392 -0.44873046875
3.85363745689392 -0.44873046875
3.85363745689392 -0.44873046875
3.85363745689392 -0.44873046875
3.85381984710693 -0.44873046875
3.85381984710693 -0.44873046875
3.8538806438446 -0.44873046875
3.8538806438446 -0.44873046875
3.85430598258972 -0.44873046875
3.85442757606506 -0.44873046875
3.85442757606506 -0.44873046875
3.85442757606506 -0.44873046875
3.85442757606506 -0.44873046875
3.85442757606506 -0.44873046875
3.85448813438416 -0.44873046875
3.85448813438416 -0.44873046875
3.85448813438416 -0.44873046875
3.85448813438416 -0.44873046875
3.85454893112183 -0.44873046875
3.85454893112183 -0.44873046875
3.8546097278595 -0.44873046875
3.85467028617859 -0.44873046875
3.85491299629211 -0.44873046875
3.85521626472473 -0.44873046875
3.85527682304382 -0.44873046875
3.85533738136292 -0.4488525390625
3.85533738136292 -0.4488525390625
3.85606384277344 -0.4488525390625
3.85612440109253 -0.4488525390625
3.85612440109253 -0.4488525390625
3.85612440109253 -0.4488525390625
3.85612440109253 -0.4488525390625
3.85612440109253 -0.4488525390625
3.86051774024963 -0.4493408203125
3.86057758331299 -0.4493408203125
3.86063742637634 -0.4493408203125
3.86075711250305 -0.4493408203125
3.86159420013428 -0.4493408203125
3.86165380477905 -0.449462890625
3.86171364784241 -0.449462890625
3.86171364784241 -0.449462890625
3.86183309555054 -0.449462890625
3.86195230484009 -0.449462890625
3.86201214790344 -0.449462890625
3.86201214790344 -0.449462890625
3.86201214790344 -0.449462890625
3.86201214790344 -0.449462890625
3.8623104095459 -0.449462890625
3.8623104095459 -0.449462890625
3.8623104095459 -0.449462890625
3.86237001419067 -0.449462890625
3.86266803741455 -0.449462890625
3.86266803741455 -0.449462890625
3.86272764205933 -0.449462890625
3.86302518844604 -0.449462890625
3.86320376396179 -0.449462890625
3.86320376396179 -0.449462890625
3.86320376396179 -0.449462890625
3.86320376396179 -0.449462890625
3.86320376396179 -0.449462890625
3.86344194412231 -0.449462890625
3.86373901367188 -0.449462890625
3.86379861831665 -0.449462890625
3.86385798454285 -0.449462890625
3.86385798454285 -0.449462890625
3.86385798454285 -0.449462890625
3.86385798454285 -0.449462890625
3.86385798454285 -0.449462890625
3.86385798454285 -0.449462890625
3.86385798454285 -0.449462890625
3.86385798454285 -0.449462890625
3.86385798454285 -0.449462890625
3.8642737865448 -0.449462890625
3.8642737865448 -0.4495849609375
3.8642737865448 -0.4495849609375
3.8642737865448 -0.4495849609375
3.86451101303101 -0.4495849609375
3.86451101303101 -0.4495849609375
3.86451101303101 -0.4495849609375
3.86480760574341 -0.4495849609375
3.86480760574341 -0.4495849609375
3.86498546600342 -0.4495849609375
3.86504459381104 -0.4495849609375
3.86504459381104 -0.4495849609375
3.86504459381104 -0.4495849609375
3.86504459381104 -0.4495849609375
3.86575531959534 -0.4495849609375
3.86575531959534 -0.4495849609375
3.86581444740295 -0.4495849609375
3.86587357521057 -0.4495849609375
3.86611008644104 -0.4495849609375
3.86616921424866 -0.4495849609375
3.86616921424866 -0.4495849609375
3.86622834205627 -0.4495849609375
3.86628723144531 -0.4495849609375
3.86675977706909 -0.4495849609375
3.86675977706909 -0.4495849609375
3.86675977706909 -0.4495849609375
3.86681890487671 -0.4495849609375
3.8688793182373 -0.44970703125
3.86893820762634 -0.44970703125
3.86905574798584 -0.44970703125
3.8691143989563 -0.44970703125
3.86917304992676 -0.44970703125
3.86923170089722 -0.44970703125
3.86952495574951 -0.44970703125
3.86958360671997 -0.4498291015625
3.86981821060181 -0.4498291015625
3.86987686157227 -0.4498291015625
3.8703453540802 -0.4498291015625
3.87040400505066 -0.4498291015625
3.87046241760254 -0.4498291015625
3.870521068573 -0.4498291015625
3.87133932113647 -0.4498291015625
3.87145614624023 -0.4498291015625
3.87151455879211 -0.4498291015625
3.87157297134399 -0.4498291015625
3.87157297134399 -0.4498291015625
3.872971534729 -0.4498291015625
3.8730297088623 -0.4498291015625
3.87308788299561 -0.4498291015625
3.87314605712891 -0.4498291015625
3.87320423126221 -0.449951171875
3.87320423126221 -0.449951171875
3.87332057952881 -0.449951171875
3.87332057952881 -0.449951171875
3.87332057952881 -0.449951171875
3.87337875366211 -0.449951171875
3.87361121177673 -0.449951171875
3.87384343147278 -0.449951171875
3.87384343147278 -0.449951171875
3.87424993515015 -0.449951171875
3.87424993515015 -0.449951171875
3.87424993515015 -0.449951171875
3.87430787086487 -0.449951171875
3.87430787086487 -0.449951171875
3.87430787086487 -0.449951171875
3.87453985214233 -0.449951171875
3.87459778785706 -0.449951171875
3.87459778785706 -0.449951171875
3.87488746643066 -0.449951171875
3.87488746643066 -0.449951171875
3.87488746643066 -0.449951171875
3.87540864944458 -0.449951171875
3.87540864944458 -0.4500732421875
3.87540864944458 -0.4500732421875
3.87540864944458 -0.4500732421875
3.8759868144989 -0.4500732421875
3.8759868144989 -0.4500732421875
3.8759868144989 -0.4500732421875
3.87691020965576 -0.4500732421875
3.87691020965576 -0.4500732421875
3.87702560424805 -0.4500732421875
3.87708330154419 -0.4500732421875
3.87708330154419 -0.4500732421875
3.87708330154419 -0.4500732421875
3.87708330154419 -0.4500732421875
3.8773136138916 -0.4500732421875
3.8773136138916 -0.4500732421875
3.87737131118774 -0.4500732421875
3.87811946868896 -0.4500732421875
3.87811946868896 -0.4500732421875
3.87811946868896 -0.4500732421875
3.87811946868896 -0.4500732421875
3.87852191925049 -0.4500732421875
3.87852191925049 -0.4500732421875
3.87852191925049 -0.4500732421875
3.87852191925049 -0.4500732421875
3.87852191925049 -0.4500732421875
3.87852191925049 -0.4500732421875
3.87880897521973 -0.4500732421875
3.87880897521973 -0.4500732421875
3.87880897521973 -0.4500732421875
3.87880897521973 -0.4500732421875
3.88052773475647 -0.4501953125
3.88052773475647 -0.4501953125
3.88052773475647 -0.4501953125
3.88052773475647 -0.4501953125
3.88052773475647 -0.4501953125
3.88098502159119 -0.4501953125
3.88098502159119 -0.4501953125
3.88098502159119 -0.4501953125
3.88127040863037 -0.4501953125
3.88127040863037 -0.4501953125
3.88127040863037 -0.4501953125
3.88127040863037 -0.4501953125
3.88127040863037 -0.4501953125
3.88138461112976 -0.4503173828125
3.88138461112976 -0.4503173828125
3.88138461112976 -0.4503173828125
3.88155579566956 -0.4503173828125
3.88155579566956 -0.4503173828125
3.88155579566956 -0.4503173828125
3.88201189041138 -0.4503173828125
3.88201189041138 -0.4503173828125
3.88201189041138 -0.4503173828125
3.882239818573 -0.4503173828125
3.882239818573 -0.4503173828125
3.882239818573 -0.4503173828125
3.882239818573 -0.4503173828125
3.882239818573 -0.4503173828125
3.88246750831604 -0.4503173828125
3.88246750831604 -0.4503173828125
3.88246750831604 -0.4503173828125
3.88258147239685 -0.4503173828125
3.88258147239685 -0.4503173828125
3.88258147239685 -0.4503173828125
3.88462543487549 -0.450439453125
3.88468217849731 -0.450439453125
3.88519144058228 -0.450439453125
3.8852481842041 -0.450439453125
3.8852481842041 -0.450439453125
3.8852481842041 -0.450439453125
3.88553094863892 -0.450439453125
3.88558745384216 -0.450439453125
3.88564395904541 -0.450439453125
3.88564395904541 -0.450439453125
3.88581323623657 -0.450439453125
3.88581323623657 -0.450439453125
3.88581323623657 -0.450439453125
3.88581323623657 -0.450439453125
3.88598275184631 -0.450439453125
3.88598275184631 -0.450439453125
3.88620853424072 -0.450439453125
3.88620853424072 -0.450439453125
3.88620853424072 -0.450439453125
3.88643431663513 -0.450439453125
3.88643431663513 -0.450439453125
3.88688540458679 -0.450439453125
3.88688540458679 -0.450439453125
3.88688540458679 -0.450439453125
3.88688540458679 -0.450439453125
3.88688540458679 -0.450439453125
3.88705444335938 -0.450439453125
3.88705444335938 -0.450439453125
3.88727951049805 -0.450439453125
3.88727951049805 -0.450439453125
3.88727951049805 -0.450439453125
3.88756108283997 -0.4505615234375
3.88756108283997 -0.4505615234375
3.88756108283997 -0.4505615234375
3.88756108283997 -0.4505615234375
3.88756108283997 -0.4505615234375
3.88784217834473 -0.4505615234375
3.88784217834473 -0.4505615234375
3.88789844512939 -0.4505615234375
3.8880672454834 -0.4505615234375
3.88812327384949 -0.4505615234375
3.88817954063416 -0.4505615234375
3.88817954063416 -0.4505615234375
3.88907742500305 -0.4505615234375
3.88907742500305 -0.4505615234375
3.88913345336914 -0.4505615234375
3.88935780525208 -0.4505615234375
3.88935780525208 -0.4505615234375
3.88935780525208 -0.4505615234375
3.88935780525208 -0.4505615234375
3.88958168029785 -0.4505615234375
3.88958168029785 -0.4505615234375
3.88958168029785 -0.4505615234375
3.88958168029785 -0.4505615234375
3.89002966880798 -0.4505615234375
3.89019727706909 -0.45068359375
3.89131450653076 -0.45068359375
3.89137029647827 -0.45068359375
3.8914258480072 -0.45068359375
3.89153742790222 -0.45068359375
3.89153742790222 -0.45068359375
3.89176034927368 -0.45068359375
3.89176034927368 -0.45068359375
3.89176034927368 -0.45068359375
3.8918719291687 -0.45068359375
3.8918719291687 -0.45068359375
3.8918719291687 -0.45068359375
3.8918719291687 -0.45068359375
3.89220595359802 -0.45068359375
3.89220595359802 -0.45068359375
3.8924286365509 -0.45068359375
3.8924286365509 -0.45068359375
3.8924286365509 -0.45068359375
3.8924286365509 -0.45068359375
3.89253973960876 -0.45068359375
3.89253973960876 -0.45068359375
3.892817735672 -0.45068359375
3.892817735672 -0.45068359375
3.892817735672 -0.45068359375
3.892817735672 -0.45068359375
3.89309573173523 -0.45068359375
3.89320683479309 -0.45068359375
3.89331769943237 -0.45068359375
3.89342880249023 -0.45068359375
3.89342880249023 -0.45068359375
3.89370632171631 -0.45068359375
3.89370632171631 -0.45068359375
3.89370632171631 -0.45068359375
3.89370632171631 -0.45068359375
3.89370632171631 -0.45068359375
3.8939836025238 -0.45068359375
3.8939836025238 -0.45068359375
3.894371509552 -0.45068359375
3.89442682266235 -0.4508056640625
3.89442682266235 -0.4508056640625
3.89442682266235 -0.4508056640625
3.89442682266235 -0.4508056640625
3.89453744888306 -0.4508056640625
3.89475893974304 -0.4508056640625
3.89475893974304 -0.4508056640625
3.89475893974304 -0.4508056640625
3.8949248790741 -0.4508056640625
3.8949248790741 -0.4508056640625
3.8951461315155 -0.4508056640625
3.89520144462585 -0.4508056640625
3.89520144462585 -0.4508056640625
3.89520144462585 -0.4508056640625
3.89586424827576 -0.4508056640625
3.89586424827576 -0.4508056640625
3.89614033699036 -0.4508056640625
3.89614033699036 -0.4508056640625
3.89636087417603 -0.4508056640625
3.8964159488678 -0.4508056640625
3.8964159488678 -0.4508056640625
3.8964159488678 -0.4508056640625
3.89647102355957 -0.4508056640625
3.89658141136169 -0.4508056640625
3.89658141136169 -0.4508056640625
3.89680171012878 -0.4508056640625
3.89680171012878 -0.4508056640625
3.8969669342041 -0.4508056640625
3.8969669342041 -0.4508056640625
3.89718699455261 -0.4508056640625
3.89718699455261 -0.4508056640625
3.89724206924438 -0.4508056640625
3.89724206924438 -0.4508056640625
3.89724206924438 -0.4508056640625
3.8974621295929 -0.4508056640625
3.8974621295929 -0.4508056640625
3.8974621295929 -0.4508056640625
3.8974621295929 -0.4508056640625
3.8974621295929 -0.4508056640625
3.89762711524963 -0.4508056640625
3.89762711524963 -0.4508056640625
3.89779186248779 -0.4508056640625
3.89779186248779 -0.450927734375
3.89784693717957 -0.450927734375
3.89817643165588 -0.450927734375
3.89823150634766 -0.450927734375
3.89823150634766 -0.450927734375
3.89823150634766 -0.450927734375
3.89828634262085 -0.450927734375
3.89828634262085 -0.450927734375
3.89828634262085 -0.450927734375
3.89938259124756 -0.450927734375
3.89949226379395 -0.450927734375
3.89949226379395 -0.450927734375
3.89965629577637 -0.450927734375
3.89987516403198 -0.450927734375
3.89987516403198 -0.450927734375
3.89993000030518 -0.450927734375
3.89993000030518 -0.450927734375
3.89993000030518 -0.450927734375
3.9000940322876 -0.450927734375
3.9000940322876 -0.450927734375
3.9000940322876 -0.450927734375
3.90025782585144 -0.450927734375
3.90031242370605 -0.450927734375
3.90036725997925 -0.450927734375
3.90036725997925 -0.450927734375
3.90036725997925 -0.450927734375
3.90047645568848 -0.450927734375
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{ClOO}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0,
tick label style={opacity=1}},
xmin=-0.23, xmax=5.59967722892761,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.413482666015625, ymax=0.019561767578125,
ytick style={color=black},
ytick distance = 0.2,
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c9)}
]
\addplot [ultra thick, brown, dashed]
table {%
2.35024809837341 -0.0001220703125
2.57634139060974 -0.0006103515625
2.80140376091003 -0.00079345703125
2.9232439994812 -0.0009765625
2.93196606636047 -0.00103759765625
3.07845687866211 -0.00115966796875
3.13097667694092 -0.00140380859375
3.25115132331848 -0.00164794921875
3.28824925422668 -0.001953125
3.32283926010132 -0.0020751953125
3.35487651824951 -0.00213623046875
3.37675929069519 -0.00225830078125
3.40976405143738 -0.00244140625
3.50474262237549 -0.00665283203125
3.53567385673523 -0.00823974609375
3.56145906448364 -0.00848388671875
3.60042834281921 -0.00921630859375
3.66351246833801 -0.01251220703125
3.69046187400818 -0.01434326171875
3.71625375747681 -0.01593017578125
3.74264669418335 -0.0172119140625
3.78525853157043 -0.018798828125
3.82275629043579 -0.020751953125
3.83657717704773 -0.02142333984375
3.87725615501404 -0.02923583984375
3.90773367881775 -0.03289794921875
3.93429636955261 -0.03558349609375
3.96270084381104 -0.0372314453125
3.97492599487305 -0.0380859375
3.99042773246765 -0.03924560546875
4.01106262207031 -0.0408935546875
4.03205442428589 -0.0450439453125
4.05010890960693 -0.04754638671875
4.09092807769775 -0.06134033203125
4.10157537460327 -0.06866455078125
4.13567304611206 -0.07403564453125
4.14404487609863 -0.0771484375
4.15630674362183 -0.0794677734375
4.19016361236572 -0.08648681640625
4.21186780929565 -0.09033203125
4.23867321014404 -0.0999755859375
4.25447559356689 -0.111572265625
4.29036855697632 -0.12152099609375
4.32625389099121 -0.13751220703125
4.34564828872681 -0.148193359375
4.36396884918213 -0.1514892578125
4.38464021682739 -0.16156005859375
4.39953517913818 -0.163818359375
4.40671062469482 -0.16522216796875
4.41937732696533 -0.1700439453125
4.43964862823486 -0.17938232421875
4.44720458984375 -0.18231201171875
4.45604705810547 -0.18408203125
4.47001314163208 -0.1903076171875
4.47471141815186 -0.19207763671875
4.48154306411743 -0.1937255859375
4.48938179016113 -0.1953125
4.49650049209595 -0.19696044921875
4.50394058227539 -0.19842529296875
4.50983381271362 -0.19989013671875
4.51469373703003 -0.20062255859375
4.51879024505615 -0.201416015625
4.52312183380127 -0.20208740234375
4.53761768341064 -0.2159423828125
4.54403066635132 -0.2200927734375
4.5495548248291 -0.22088623046875
4.55729055404663 -0.22772216796875
4.56481981277466 -0.23004150390625
4.57780170440674 -0.23956298828125
4.58197259902954 -0.243408203125
4.58918952941895 -0.2454833984375
4.59420442581177 -0.24652099609375
4.59799098968506 -0.24713134765625
4.61043643951416 -0.25213623046875
4.61630725860596 -0.25701904296875
4.62029218673706 -0.258056640625
4.62591934204102 -0.259765625
4.63164663314819 -0.2606201171875
4.63555431365967 -0.26171875
4.6398549079895 -0.262451171875
4.64535331726074 -0.26348876953125
4.64950037002563 -0.26483154296875
4.66005897521973 -0.2711181640625
4.66423749923706 -0.27252197265625
4.66826486587524 -0.273193359375
4.6771411895752 -0.27679443359375
4.68258714675903 -0.2774658203125
4.68696689605713 -0.27789306640625
4.69219446182251 -0.28009033203125
4.69707250595093 -0.2806396484375
4.70476818084717 -0.2845458984375
4.70796155929565 -0.28521728515625
4.71092081069946 -0.28570556640625
4.71899127960205 -0.289794921875
4.72199201583862 -0.290283203125
4.72586250305176 -0.2911376953125
4.72839450836182 -0.29144287109375
4.73355054855347 -0.2926025390625
4.73930311203003 -0.293212890625
4.74466848373413 -0.29376220703125
4.74796295166016 -0.294189453125
4.75327682495117 -0.294921875
4.75913143157959 -0.296875
4.76748991012573 -0.297607421875
4.77543544769287 -0.29864501953125
4.78040361404419 -0.2991943359375
4.7828164100647 -0.29949951171875
4.79606056213379 -0.307861328125
4.80215072631836 -0.309814453125
4.80483436584473 -0.31011962890625
4.80748748779297 -0.31036376953125
4.81747961044312 -0.32147216796875
4.82099580764771 -0.32476806640625
4.82782793045044 -0.330078125
4.83118486404419 -0.33135986328125
4.8344144821167 -0.33221435546875
4.83866024017334 -0.33465576171875
4.84214115142822 -0.3353271484375
4.84693670272827 -0.33624267578125
4.84975099563599 -0.3369140625
4.85263872146606 -0.33770751953125
4.85798931121826 -0.3385009765625
4.86571359634399 -0.33984375
4.86790943145752 -0.34033203125
4.87426137924194 -0.34124755859375
4.87959480285645 -0.3419189453125
4.88763999938965 -0.34503173828125
4.88977766036987 -0.34539794921875
4.90037822723389 -0.34820556640625
4.90578508377075 -0.34918212890625
4.90728235244751 -0.34954833984375
4.90901565551758 -0.34967041015625
4.91420030593872 -0.350341796875
4.91572141647339 -0.35052490234375
4.91765260696411 -0.35064697265625
4.91908311843872 -0.3507080078125
4.92220640182495 -0.3509521484375
4.92438793182373 -0.35113525390625
4.93236207962036 -0.35357666015625
4.9347357749939 -0.35406494140625
4.93696069717407 -0.35430908203125
4.93980884552002 -0.3544921875
4.9412727355957 -0.3546142578125
4.94387006759644 -0.35479736328125
4.9458475112915 -0.35516357421875
4.94841289520264 -0.35552978515625
4.95135688781738 -0.35577392578125
4.95303916931152 -0.35595703125
4.95795679092407 -0.35723876953125
4.9592227935791 -0.3577880859375
4.9622745513916 -0.35809326171875
4.964919090271 -0.35833740234375
4.96710300445557 -0.35845947265625
4.97003984451294 -0.35894775390625
4.97186946868896 -0.3592529296875
4.97477436065674 -0.3594970703125
4.97683572769165 -0.35968017578125
4.97917509078979 -0.36016845703125
4.98301267623901 -0.36053466796875
4.98540830612183 -0.36090087890625
4.98863458633423 -0.3616943359375
4.99145650863647 -0.362060546875
4.99544668197632 -0.3631591796875
4.99706315994263 -0.3634033203125
5.00016498565674 -0.3638916015625
5.00296497344971 -0.364501953125
5.00428247451782 -0.36480712890625
5.00514602661133 -0.36492919921875
5.00817012786865 -0.3658447265625
5.01048231124878 -0.36602783203125
5.01287937164307 -0.3660888671875
5.01346921920776 -0.3662109375
5.01651954650879 -0.36663818359375
5.01745510101318 -0.36669921875
5.01972675323486 -0.36688232421875
5.02398443222046 -0.367919921875
5.02646780014038 -0.36846923828125
5.02948141098022 -0.36907958984375
5.03185653686523 -0.36920166015625
5.03291273117065 -0.36932373046875
5.03438377380371 -0.369384765625
5.03549766540527 -0.3695068359375
5.03702402114868 -0.36962890625
5.03855657577515 -0.3697509765625
5.04232358932495 -0.370361328125
5.04297685623169 -0.37042236328125
5.04455137252808 -0.37054443359375
5.04845333099365 -0.3712158203125
5.04874467849731 -0.371337890625
5.05019426345825 -0.37139892578125
5.0518045425415 -0.37158203125
5.05368518829346 -0.37164306640625
5.05685520172119 -0.3720703125
5.05718660354614 -0.37213134765625
5.05988502502441 -0.3726806640625
5.06153535842896 -0.372802734375
5.06311941146851 -0.37286376953125
5.0646824836731 -0.37298583984375
5.06589698791504 -0.37310791015625
5.06874990463257 -0.37432861328125
5.06961250305176 -0.3746337890625
5.07052564620972 -0.37469482421875
5.07339191436768 -0.37603759765625
5.07424592971802 -0.37628173828125
5.07552862167358 -0.3763427734375
5.07749891281128 -0.3770751953125
5.07862377166748 -0.377197265625
5.07952499389648 -0.37725830078125
5.08066987991333 -0.37738037109375
5.0814733505249 -0.37744140625
5.0824728012085 -0.3775634765625
5.08364248275757 -0.37762451171875
5.08501195907593 -0.37774658203125
5.08651638031006 -0.37823486328125
5.08766412734985 -0.37841796875
5.08863544464111 -0.37847900390625
5.08952379226685 -0.37860107421875
5.09039211273193 -0.378662109375
5.09173011779785 -0.3787841796875
5.09302234649658 -0.37921142578125
5.09420919418335 -0.3792724609375
5.09682655334473 -0.3814697265625
5.09762859344482 -0.3818359375
5.09871625900269 -0.38214111328125
5.09907245635986 -0.38214111328125
5.10028457641602 -0.3822021484375
5.10095596313477 -0.38232421875
5.10148572921753 -0.38232421875
5.10263252258301 -0.38287353515625
5.10352659225464 -0.3829345703125
5.10368394851685 -0.3829345703125
5.10407400131226 -0.38299560546875
5.10428905487061 -0.38299560546875
5.10473966598511 -0.383056640625
5.10497856140137 -0.383056640625
5.10548973083496 -0.38311767578125
5.10578918457031 -0.38311767578125
5.1065034866333 -0.38311767578125
5.10749483108521 -0.38323974609375
5.10784387588501 -0.38323974609375
5.1080846786499 -0.38330078125
5.10869026184082 -0.38330078125
5.10901117324829 -0.38336181640625
5.10948085784912 -0.38336181640625
5.11036396026611 -0.3836669921875
5.1108455657959 -0.38372802734375
5.11089944839478 -0.38372802734375
5.11253118515015 -0.38397216796875
5.11282920837402 -0.38397216796875
5.1133885383606 -0.384033203125
5.11354875564575 -0.384033203125
5.1139063835144 -0.384033203125
5.1146411895752 -0.38409423828125
5.11474418640137 -0.38409423828125
5.11500453948975 -0.38409423828125
5.11528778076172 -0.38409423828125
5.11560392379761 -0.3841552734375
5.1161527633667 -0.3841552734375
5.11653804779053 -0.3841552734375
5.11669731140137 -0.3841552734375
5.11772871017456 -0.38427734375
5.11943054199219 -0.38446044921875
5.11973094940186 -0.38446044921875
5.1199254989624 -0.384521484375
5.12081384658813 -0.38458251953125
5.12094879150391 -0.38458251953125
5.12138271331787 -0.38458251953125
5.12205219268799 -0.3846435546875
5.12215042114258 -0.3846435546875
5.1233057975769 -0.38470458984375
5.12356758117676 -0.38470458984375
5.12404108047485 -0.38470458984375
5.12430858612061 -0.38470458984375
5.12499952316284 -0.384765625
5.12589406967163 -0.38482666015625
5.12594604492188 -0.38482666015625
5.12613487243652 -0.38482666015625
5.12658262252808 -0.3848876953125
5.12677097320557 -0.3848876953125
5.12711143493652 -0.3848876953125
5.12771368026733 -0.38494873046875
5.12828636169434 -0.38494873046875
5.12859296798706 -0.38494873046875
5.12875461578369 -0.385009765625
5.13096714019775 -0.38525390625
5.13115310668945 -0.38525390625
5.1314263343811 -0.38525390625
5.13181734085083 -0.38531494140625
5.13258647918701 -0.38531494140625
5.13308525085449 -0.38531494140625
5.13352298736572 -0.3853759765625
5.13357734680176 -0.3853759765625
5.13384866714478 -0.3853759765625
5.13445138931274 -0.3853759765625
5.13462972640991 -0.3853759765625
5.1346583366394 -0.3853759765625
5.13504695892334 -0.38543701171875
5.13678693771362 -0.3856201171875
5.13757562637329 -0.38568115234375
5.13774967193604 -0.38568115234375
5.1396336555481 -0.3857421875
5.13982248306274 -0.38580322265625
5.14007091522217 -0.3858642578125
5.14030981063843 -0.3858642578125
5.14060544967651 -0.3858642578125
5.14102935791016 -0.3858642578125
5.14128017425537 -0.3858642578125
5.1416597366333 -0.38592529296875
5.1419825553894 -0.38592529296875
5.14207649230957 -0.38592529296875
5.14248037338257 -0.38592529296875
5.14262723922729 -0.385986328125
5.14352703094482 -0.38604736328125
5.14437198638916 -0.38604736328125
5.14468955993652 -0.38604736328125
5.14654350280762 -0.38623046875
5.14673233032227 -0.38629150390625
5.147141456604 -0.3863525390625
5.1473331451416 -0.3863525390625
5.1486611366272 -0.38653564453125
5.14896011352539 -0.38653564453125
5.14936685562134 -0.38653564453125
5.1496410369873 -0.38653564453125
5.14972066879272 -0.38653564453125
5.15229463577271 -0.3868408203125
5.15259408950806 -0.38690185546875
5.15262746810913 -0.38690185546875
5.1531925201416 -0.386962890625
5.15333318710327 -0.386962890625
5.15344285964966 -0.386962890625
5.15413188934326 -0.386962890625
5.15419244766235 -0.38702392578125
5.15425062179565 -0.38702392578125
5.15530586242676 -0.3870849609375
5.15555143356323 -0.3870849609375
5.15567302703857 -0.3870849609375
5.15622520446777 -0.3870849609375
5.16006326675415 -0.38861083984375
5.16090059280396 -0.38873291015625
5.16125440597534 -0.38873291015625
5.16127490997314 -0.38873291015625
5.16145801544189 -0.38873291015625
5.16153860092163 -0.38873291015625
5.16276741027832 -0.3887939453125
5.16298246383667 -0.3887939453125
5.16309881210327 -0.3887939453125
5.16349840164185 -0.3887939453125
5.16361474990845 -0.38885498046875
5.16362047195435 -0.38885498046875
5.16488218307495 -0.388916015625
5.16497993469238 -0.388916015625
5.16525602340698 -0.388916015625
5.16540765762329 -0.388916015625
5.16559457778931 -0.38897705078125
5.16581392288208 -0.38897705078125
5.1666579246521 -0.38897705078125
5.16722869873047 -0.38897705078125
5.16741180419922 -0.38897705078125
5.1681022644043 -0.3890380859375
5.16843557357788 -0.3890380859375
5.16844129562378 -0.3890380859375
5.17120838165283 -0.38934326171875
5.17139863967896 -0.389404296875
5.17243385314941 -0.3895263671875
5.17252111434937 -0.3895263671875
5.17271089553833 -0.3895263671875
5.17373657226562 -0.3895263671875
5.17379188537598 -0.3895263671875
5.17401885986328 -0.3895263671875
5.17443466186523 -0.3895263671875
5.17607402801514 -0.3896484375
5.17621850967407 -0.3896484375
5.1764702796936 -0.3896484375
5.17695617675781 -0.3896484375
5.17720460891724 -0.3896484375
5.17781352996826 -0.38970947265625
5.1778826713562 -0.38970947265625
5.17826318740845 -0.38970947265625
5.17853403091431 -0.38970947265625
5.17872095108032 -0.38970947265625
5.1788215637207 -0.38970947265625
5.17976713180542 -0.38970947265625
5.17980432510376 -0.38970947265625
5.17999410629272 -0.3897705078125
5.18106555938721 -0.3897705078125
5.18122005462646 -0.3897705078125
5.1814432144165 -0.3897705078125
5.1818208694458 -0.38983154296875
5.18230056762695 -0.38983154296875
5.18330097198486 -0.38983154296875
5.18381071090698 -0.38983154296875
5.18438482284546 -0.389892578125
5.18458080291748 -0.389892578125
5.18511152267456 -0.389892578125
5.18532133102417 -0.389892578125
5.18555355072021 -0.389892578125
5.18609142303467 -0.389892578125
5.18644762039185 -0.389892578125
5.18672466278076 -0.389892578125
5.18720769882202 -0.38995361328125
5.18738794326782 -0.38995361328125
5.18752908706665 -0.38995361328125
5.1876335144043 -0.38995361328125
5.18828439712524 -0.38995361328125
5.18829536437988 -0.38995361328125
5.1887035369873 -0.38995361328125
5.18902111053467 -0.38995361328125
5.18909978866577 -0.38995361328125
5.18918132781982 -0.38995361328125
5.19002628326416 -0.3900146484375
5.19023942947388 -0.3900146484375
5.19275426864624 -0.3902587890625
5.19284629821777 -0.3902587890625
5.19299364089966 -0.3902587890625
5.19318008422852 -0.3902587890625
5.19344758987427 -0.3902587890625
5.19377565383911 -0.39031982421875
5.19428968429565 -0.39031982421875
5.19444751739502 -0.39031982421875
5.19446706771851 -0.39031982421875
5.19483613967896 -0.39031982421875
5.19493055343628 -0.39031982421875
5.19507169723511 -0.39031982421875
5.19555377960205 -0.39031982421875
5.19563961029053 -0.39031982421875
5.19630336761475 -0.390380859375
5.19673156738281 -0.390380859375
5.19684457778931 -0.390380859375
5.19707632064819 -0.390380859375
5.19777679443359 -0.390380859375
5.19779586791992 -0.390380859375
5.19786739349365 -0.390380859375
5.19799423217773 -0.390380859375
5.19865703582764 -0.390380859375
5.19870662689209 -0.390380859375
5.19877243041992 -0.390380859375
5.19880819320679 -0.390380859375
5.1989426612854 -0.39044189453125
5.19948387145996 -0.39044189453125
5.19954395294189 -0.39044189453125
5.19962882995605 -0.39044189453125
5.19964265823364 -0.39044189453125
5.20007038116455 -0.39044189453125
5.2020411491394 -0.39068603515625
5.20223236083984 -0.39068603515625
5.20258903503418 -0.39068603515625
5.20267915725708 -0.3907470703125
5.20354700088501 -0.3907470703125
5.20381021499634 -0.3907470703125
5.20418262481689 -0.3907470703125
5.20432329177856 -0.3907470703125
5.20453786849976 -0.3907470703125
5.20543432235718 -0.39080810546875
5.20593214035034 -0.39080810546875
5.20644521713257 -0.39080810546875
5.20652389526367 -0.39080810546875
5.2065372467041 -0.39080810546875
5.20663166046143 -0.39080810546875
5.20718193054199 -0.39080810546875
5.20769071578979 -0.39080810546875
5.20784187316895 -0.39080810546875
5.20848989486694 -0.390869140625
5.20858383178711 -0.390869140625
5.20873165130615 -0.390869140625
5.20965433120728 -0.390869140625
5.20970249176025 -0.390869140625
5.20986604690552 -0.390869140625
5.20991945266724 -0.390869140625
5.21020603179932 -0.390869140625
5.21050024032593 -0.390869140625
5.21080541610718 -0.390869140625
5.21116876602173 -0.390869140625
5.21246480941772 -0.3909912109375
5.21258974075317 -0.3909912109375
5.21281337738037 -0.3909912109375
5.2131404876709 -0.3909912109375
5.21315383911133 -0.3909912109375
5.21316719055176 -0.3909912109375
5.21338224411011 -0.3909912109375
5.21339559555054 -0.3909912109375
5.21428728103638 -0.3909912109375
5.21442270278931 -0.3909912109375
5.21451807022095 -0.39105224609375
5.21748399734497 -0.39129638671875
5.21756029129028 -0.391357421875
5.21773672103882 -0.391357421875
5.21798896789551 -0.391357421875
5.21802568435669 -0.391357421875
5.21803379058838 -0.391357421875
5.21818351745605 -0.391357421875
5.21823883056641 -0.391357421875
5.21845674514771 -0.391357421875
5.21871423721313 -0.391357421875
5.21933841705322 -0.391357421875
5.21961355209351 -0.391357421875
5.21966028213501 -0.391357421875
5.2199535369873 -0.391357421875
5.2200140953064 -0.391357421875
5.22025203704834 -0.391357421875
5.22114276885986 -0.391357421875
5.22126817703247 -0.391357421875
5.22221946716309 -0.39141845703125
5.22273445129395 -0.39141845703125
5.22285413742065 -0.39141845703125
5.22295808792114 -0.39141845703125
5.22299480438232 -0.39141845703125
5.22435426712036 -0.3914794921875
5.2247166633606 -0.3914794921875
5.22494459152222 -0.3914794921875
5.22525501251221 -0.3914794921875
5.22544384002686 -0.3914794921875
5.22558832168579 -0.3914794921875
5.22582101821899 -0.3914794921875
5.22632932662964 -0.3914794921875
5.22633695602417 -0.3914794921875
5.22641706466675 -0.3914794921875
5.22682905197144 -0.3914794921875
5.22707366943359 -0.3914794921875
5.22814083099365 -0.39154052734375
5.22839784622192 -0.39154052734375
5.2284107208252 -0.39154052734375
5.22841835021973 -0.39154052734375
5.2290415763855 -0.39154052734375
5.22912359237671 -0.39154052734375
5.22923135757446 -0.39154052734375
5.22955131530762 -0.39154052734375
5.22998905181885 -0.39154052734375
5.2302827835083 -0.3916015625
5.23029041290283 -0.3916015625
5.23031616210938 -0.3916015625
5.23058938980103 -0.3916015625
5.2309136390686 -0.3916015625
5.23108959197998 -0.3916015625
5.23109722137451 -0.3916015625
5.23158931732178 -0.3916015625
5.23172426223755 -0.3916015625
5.23184394836426 -0.3916015625
5.23198175430298 -0.3916015625
5.23210906982422 -0.3916015625
5.23211669921875 -0.3916015625
5.23226165771484 -0.3916015625
5.23231220245361 -0.3916015625
5.23277997970581 -0.3916015625
5.23291969299316 -0.3916015625
5.23312568664551 -0.3916015625
5.2331714630127 -0.3916015625
5.23327541351318 -0.3916015625
5.23361778259277 -0.3916015625
5.23406887054443 -0.39166259765625
5.23493719100952 -0.39166259765625
5.23548555374146 -0.39166259765625
5.23565196990967 -0.39166259765625
5.23587417602539 -0.39166259765625
5.23687744140625 -0.39166259765625
5.2369704246521 -0.39166259765625
5.23703813552856 -0.39166259765625
5.23731756210327 -0.3917236328125
5.23745059967041 -0.3917236328125
5.23745822906494 -0.3917236328125
5.23753356933594 -0.3917236328125
5.23801612854004 -0.3917236328125
5.23813629150391 -0.3917236328125
5.23852777481079 -0.3917236328125
5.2385401725769 -0.3917236328125
5.23861312866211 -0.3917236328125
5.23936939239502 -0.3917236328125
5.23982000350952 -0.3917236328125
5.23986482620239 -0.3917236328125
5.2401270866394 -0.3917236328125
5.24023962020874 -0.3917236328125
5.24046421051025 -0.3917236328125
5.24068164825439 -0.3917236328125
5.24077129364014 -0.3917236328125
5.24112558364868 -0.39178466796875
5.2418327331543 -0.39178466796875
5.24184036254883 -0.39178466796875
5.24200963973999 -0.39178466796875
5.24201679229736 -0.39178466796875
5.24214601516724 -0.39178466796875
5.24237251281738 -0.39178466796875
5.24237728118896 -0.39178466796875
5.24265336990356 -0.39178466796875
5.24291658401489 -0.39178466796875
5.24323892593384 -0.39178466796875
5.24325895309448 -0.39178466796875
5.24336290359497 -0.39178466796875
5.2433705329895 -0.39178466796875
5.2437424659729 -0.39178466796875
5.24398756027222 -0.39178466796875
5.24408674240112 -0.39178466796875
5.24427700042725 -0.39178466796875
5.24428462982178 -0.39178466796875
5.24519920349121 -0.39178466796875
5.24527311325073 -0.391845703125
5.24540901184082 -0.391845703125
5.24552249908447 -0.391845703125
5.24558925628662 -0.391845703125
5.24559640884399 -0.391845703125
5.24579906463623 -0.391845703125
5.24675464630127 -0.391845703125
5.24734973907471 -0.391845703125
5.24901723861694 -0.3919677734375
5.24926710128784 -0.3919677734375
5.24937200546265 -0.3919677734375
5.24955558776855 -0.3919677734375
5.24970436096191 -0.3919677734375
5.25041007995605 -0.39202880859375
5.25058078765869 -0.39202880859375
5.2511682510376 -0.39202880859375
5.2514386177063 -0.39202880859375
5.25167942047119 -0.39202880859375
5.25207614898682 -0.39202880859375
5.2525110244751 -0.39202880859375
5.2525520324707 -0.39202880859375
5.25294303894043 -0.39202880859375
5.2530083656311 -0.39202880859375
5.25359487533569 -0.39202880859375
5.25409364700317 -0.39202880859375
5.25432062149048 -0.39202880859375
5.25437879562378 -0.39202880859375
5.25452375411987 -0.39202880859375
5.25459384918213 -0.39202880859375
5.25489377975464 -0.39202880859375
5.25490093231201 -0.39202880859375
5.25524854660034 -0.39202880859375
5.25630855560303 -0.39215087890625
5.25676345825195 -0.39215087890625
5.25684261322021 -0.39215087890625
5.25699424743652 -0.39215087890625
5.25708532333374 -0.39215087890625
5.25744819641113 -0.39215087890625
5.25751781463623 -0.39215087890625
5.257568359375 -0.39215087890625
5.25757312774658 -0.39215087890625
5.25775051116943 -0.39215087890625
5.25788021087646 -0.39215087890625
5.25833797454834 -0.39215087890625
5.25853681564331 -0.39215087890625
5.25871849060059 -0.39215087890625
5.25915193557739 -0.39215087890625
5.25928068161011 -0.3922119140625
5.25929260253906 -0.3922119140625
5.25933122634888 -0.3922119140625
5.25953435897827 -0.3922119140625
5.25957727432251 -0.3922119140625
5.2598876953125 -0.3922119140625
5.25990676879883 -0.3922119140625
5.26039600372314 -0.3922119140625
5.26061534881592 -0.3922119140625
5.26104879379272 -0.3922119140625
5.26115560531616 -0.3922119140625
5.26151990890503 -0.3922119140625
5.26167917251587 -0.3922119140625
5.26193809509277 -0.3922119140625
5.26215219497681 -0.3922119140625
5.26232290267944 -0.3922119140625
5.26253652572632 -0.3922119140625
5.26284027099609 -0.3922119140625
5.26302051544189 -0.3922119140625
5.26308679580688 -0.3922119140625
5.26395082473755 -0.3922119140625
5.26405000686646 -0.3922119140625
5.26405477523804 -0.3922119140625
5.26417303085327 -0.3922119140625
5.26431226730347 -0.3922119140625
5.26450872421265 -0.3922119140625
5.2650089263916 -0.39227294921875
5.26516008377075 -0.39227294921875
5.26560544967651 -0.39227294921875
5.26600360870361 -0.39227294921875
5.26641273498535 -0.39227294921875
5.26653051376343 -0.39227294921875
5.26687812805176 -0.39227294921875
5.26695823669434 -0.39227294921875
5.26700019836426 -0.39227294921875
5.26711988449097 -0.39227294921875
5.267258644104 -0.39227294921875
5.26755666732788 -0.39227294921875
5.26872777938843 -0.39227294921875
5.26901531219482 -0.39227294921875
5.26928186416626 -0.39227294921875
5.26961326599121 -0.392333984375
5.26983737945557 -0.392333984375
5.27039480209351 -0.392333984375
5.27046680450439 -0.392333984375
5.27083253860474 -0.392333984375
5.27089309692383 -0.392333984375
5.27108383178711 -0.392333984375
5.27136516571045 -0.392333984375
5.27154445648193 -0.392333984375
5.27174854278564 -0.392333984375
5.27284145355225 -0.392333984375
5.27290391921997 -0.392333984375
5.2730450630188 -0.392333984375
5.27343893051147 -0.39239501953125
5.27351522445679 -0.39239501953125
5.27407932281494 -0.39239501953125
5.27415084838867 -0.39239501953125
5.27425479888916 -0.39239501953125
5.27453422546387 -0.39239501953125
5.2746844291687 -0.39239501953125
5.27509021759033 -0.39239501953125
5.2751407623291 -0.39239501953125
5.27517318725586 -0.39239501953125
5.27575588226318 -0.39239501953125
5.27589178085327 -0.39239501953125
5.27628040313721 -0.39239501953125
5.2763352394104 -0.39239501953125
5.27645015716553 -0.39239501953125
5.27658128738403 -0.39239501953125
5.27659749984741 -0.39239501953125
5.27660894393921 -0.39239501953125
5.27673959732056 -0.39239501953125
5.27674436569214 -0.39239501953125
5.27820253372192 -0.392578125
5.27831697463989 -0.392578125
5.27835559844971 -0.392578125
5.27847242355347 -0.392578125
5.27871036529541 -0.392578125
5.27891826629639 -0.392578125
5.27903032302856 -0.392578125
5.27932024002075 -0.392578125
5.27971696853638 -0.392578125
5.27981758117676 -0.392578125
5.27994728088379 -0.392578125
5.27995204925537 -0.392578125
5.28235912322998 -0.39276123046875
5.28287124633789 -0.39276123046875
5.28295040130615 -0.39276123046875
5.2830638885498 -0.39276123046875
5.2834324836731 -0.39276123046875
5.28354978561401 -0.39276123046875
5.28359079360962 -0.39276123046875
5.28395652770996 -0.39276123046875
5.28416013717651 -0.39276123046875
5.28416442871094 -0.39276123046875
5.28435611724854 -0.392822265625
5.28442621231079 -0.392822265625
5.28468799591064 -0.392822265625
5.28469896316528 -0.392822265625
5.28496980667114 -0.392822265625
5.28498077392578 -0.392822265625
5.28539991378784 -0.392822265625
5.28567886352539 -0.392822265625
5.28572368621826 -0.392822265625
5.28589916229248 -0.392822265625
5.28592157363892 -0.392822265625
5.28604984283447 -0.392822265625
5.28645181655884 -0.392822265625
5.28675508499146 -0.392822265625
5.28686714172363 -0.392822265625
5.28698825836182 -0.392822265625
5.28732013702393 -0.392822265625
5.28738069534302 -0.392822265625
5.28762245178223 -0.392822265625
5.28778600692749 -0.392822265625
5.28791570663452 -0.392822265625
5.28796052932739 -0.392822265625
5.28814840316772 -0.392822265625
5.28828525543213 -0.392822265625
5.28891944885254 -0.39288330078125
5.28926801681519 -0.39288330078125
5.2893123626709 -0.39288330078125
5.28982734680176 -0.39288330078125
5.29000806808472 -0.39288330078125
5.29071092605591 -0.39288330078125
5.29078245162964 -0.39288330078125
5.29083585739136 -0.39288330078125
5.29090213775635 -0.39288330078125
5.29091787338257 -0.39288330078125
5.29187917709351 -0.3929443359375
5.29205226898193 -0.3929443359375
5.29215431213379 -0.3929443359375
5.2930154800415 -0.3929443359375
5.29305982589722 -0.3929443359375
5.29312610626221 -0.3929443359375
5.29347324371338 -0.3929443359375
5.29396104812622 -0.3929443359375
5.29420185089111 -0.3929443359375
5.29427433013916 -0.3929443359375
5.29479694366455 -0.3929443359375
5.29493093490601 -0.3929443359375
5.29512500762939 -0.3929443359375
5.29514932632446 -0.3929443359375
5.29535388946533 -0.39300537109375
5.29566144943237 -0.39300537109375
5.29577398300171 -0.39300537109375
5.29578924179077 -0.39300537109375
5.29590797424316 -0.39300537109375
5.29618215560913 -0.39300537109375
5.29625940322876 -0.39300537109375
5.29626131057739 -0.39300537109375
5.29675722122192 -0.39300537109375
5.29741048812866 -0.39300537109375
5.29767513275146 -0.39300537109375
5.29773187637329 -0.39300537109375
5.29784154891968 -0.39300537109375
5.29799652099609 -0.39300537109375
5.2983226776123 -0.39300537109375
5.29835510253906 -0.39300537109375
5.29851913452148 -0.39300537109375
5.29875469207764 -0.39300537109375
5.29877662658691 -0.39300537109375
5.29893398284912 -0.39300537109375
5.29952478408813 -0.39306640625
5.30005836486816 -0.39306640625
5.30006694793701 -0.39306640625
5.30019330978394 -0.39306640625
5.30034971237183 -0.39306640625
5.30049324035645 -0.39306640625
5.30065631866455 -0.39306640625
5.30085420608521 -0.39306640625
5.30102586746216 -0.39306640625
5.30123615264893 -0.39306640625
5.30149459838867 -0.39306640625
5.3015398979187 -0.39306640625
5.3018045425415 -0.39306640625
5.30198669433594 -0.39306640625
5.30256271362305 -0.39312744140625
5.30277252197266 -0.39312744140625
5.30285692214966 -0.39312744140625
5.30313110351562 -0.39312744140625
5.30321550369263 -0.39312744140625
5.30356979370117 -0.39312744140625
5.30360841751099 -0.39312744140625
5.30367565155029 -0.39312744140625
5.30377912521362 -0.39312744140625
5.30416965484619 -0.39312744140625
5.30426645278931 -0.39312744140625
5.30464124679565 -0.39312744140625
5.30466079711914 -0.39312744140625
5.30477285385132 -0.39312744140625
5.30515575408936 -0.39312744140625
5.30521821975708 -0.39312744140625
5.30555534362793 -0.39312744140625
5.3056263923645 -0.39312744140625
5.30575323104858 -0.39312744140625
5.30588626861572 -0.39312744140625
5.30605173110962 -0.39312744140625
5.3060622215271 -0.39312744140625
5.30621910095215 -0.39312744140625
5.30646800994873 -0.39312744140625
5.30664157867432 -0.39312744140625
5.30681085586548 -0.39312744140625
5.30684947967529 -0.39312744140625
5.30699300765991 -0.39312744140625
5.30702495574951 -0.39312744140625
5.307288646698 -0.39312744140625
5.30737638473511 -0.39312744140625
5.30748748779297 -0.39312744140625
5.30753231048584 -0.39312744140625
5.30770969390869 -0.3931884765625
5.30785512924194 -0.3931884765625
5.30795574188232 -0.3931884765625
5.30811405181885 -0.3931884765625
5.30927038192749 -0.39324951171875
5.30946636199951 -0.393310546875
5.30986213684082 -0.393310546875
5.30997276306152 -0.393310546875
5.31034278869629 -0.393310546875
5.31038331985474 -0.393310546875
5.31061029434204 -0.393310546875
5.31064653396606 -0.393310546875
5.31076145172119 -0.393310546875
5.31120252609253 -0.393310546875
5.31130456924438 -0.393310546875
5.31139373779297 -0.393310546875
5.3115291595459 -0.393310546875
5.31154632568359 -0.393310546875
5.3118257522583 -0.393310546875
5.31213712692261 -0.393310546875
5.31220054626465 -0.393310546875
5.31228303909302 -0.393310546875
5.31235074996948 -0.393310546875
5.3125114440918 -0.39337158203125
5.31260061264038 -0.39337158203125
5.31288814544678 -0.39337158203125
5.31317520141602 -0.39337158203125
5.31326389312744 -0.39337158203125
5.31346035003662 -0.39337158203125
5.31350040435791 -0.39337158203125
5.3137321472168 -0.39337158203125
5.31382513046265 -0.39337158203125
5.31411170959473 -0.39337158203125
5.31418752670288 -0.39337158203125
5.31439208984375 -0.39337158203125
5.31473064422607 -0.39337158203125
5.31477499008179 -0.39337158203125
5.31484842300415 -0.39337158203125
5.31487989425659 -0.39337158203125
5.31508207321167 -0.39337158203125
5.31508827209473 -0.39337158203125
5.31534242630005 -0.39337158203125
5.31535959243774 -0.39337158203125
5.31549787521362 -0.39337158203125
5.31567859649658 -0.39337158203125
5.31580018997192 -0.39337158203125
5.3158106803894 -0.39337158203125
5.31586742401123 -0.39337158203125
5.31600379943848 -0.39337158203125
5.31621360778809 -0.39337158203125
5.31676912307739 -0.39337158203125
5.31688404083252 -0.39337158203125
5.31697845458984 -0.39337158203125
5.31698274612427 -0.39337158203125
5.31773519515991 -0.3934326171875
5.31795454025269 -0.3934326171875
5.31807994842529 -0.3934326171875
5.31816577911377 -0.3934326171875
5.31835126876831 -0.3934326171875
5.3183741569519 -0.3934326171875
5.31840372085571 -0.3934326171875
5.31857681274414 -0.3934326171875
5.31889152526855 -0.3934326171875
5.31899547576904 -0.3934326171875
5.31909990310669 -0.3934326171875
5.31930828094482 -0.3934326171875
5.31938314437866 -0.3934326171875
5.31950378417969 -0.3934326171875
5.31955575942993 -0.3934326171875
5.31963920593262 -0.3934326171875
5.319655418396 -0.3934326171875
5.31998825073242 -0.3934326171875
5.32000064849854 -0.3934326171875
5.32010078430176 -0.3934326171875
5.32021713256836 -0.3934326171875
5.32055759429932 -0.3934326171875
5.32077121734619 -0.3934326171875
5.32080221176147 -0.3934326171875
5.32094764709473 -0.3934326171875
5.32111978530884 -0.3934326171875
5.32133102416992 -0.3934326171875
5.32151746749878 -0.3934326171875
5.32163572311401 -0.3934326171875
5.32168769836426 -0.3934326171875
5.3219108581543 -0.3934326171875
5.32192754745483 -0.3934326171875
5.32247543334961 -0.39349365234375
5.32251930236816 -0.39349365234375
5.32273578643799 -0.39349365234375
5.32282495498657 -0.39349365234375
5.32314682006836 -0.39349365234375
5.32317590713501 -0.39349365234375
5.32325601577759 -0.39349365234375
5.32333898544312 -0.39349365234375
5.32341718673706 -0.39349365234375
5.32347059249878 -0.39349365234375
5.32460117340088 -0.3935546875
5.32494258880615 -0.39361572265625
5.32494688034058 -0.39361572265625
5.32501649856567 -0.39361572265625
5.32505559921265 -0.39361572265625
5.32505989074707 -0.39361572265625
5.32506370544434 -0.39361572265625
5.32618236541748 -0.3936767578125
5.32641983032227 -0.39373779296875
5.32673311233521 -0.39373779296875
5.32709121704102 -0.39373779296875
5.32710552215576 -0.39373779296875
5.32776975631714 -0.39373779296875
5.32777976989746 -0.39373779296875
5.3278980255127 -0.39373779296875
5.32836532592773 -0.39373779296875
5.32840824127197 -0.39373779296875
5.32853841781616 -0.39373779296875
5.328941822052 -0.39373779296875
5.32895231246948 -0.39373779296875
5.32911920547485 -0.39373779296875
5.32912302017212 -0.39373779296875
5.3291335105896 -0.39373779296875
5.32913541793823 -0.39373779296875
5.32913970947266 -0.39373779296875
5.32918834686279 -0.39373779296875
5.32947111129761 -0.39373779296875
5.32947540283203 -0.39373779296875
5.32954216003418 -0.39373779296875
5.32956647872925 -0.39373779296875
5.32976198196411 -0.39373779296875
5.32976579666138 -0.39373779296875
5.33025121688843 -0.393798828125
5.33054971694946 -0.393798828125
5.33073425292969 -0.393798828125
5.33076858520508 -0.393798828125
5.33076858520508 -0.393798828125
5.33108901977539 -0.393798828125
5.33115005493164 -0.393798828125
5.33120059967041 -0.393798828125
5.3313159942627 -0.393798828125
5.33137655258179 -0.393798828125
5.33140707015991 -0.393798828125
5.33164596557617 -0.393798828125
5.33174514770508 -0.393798828125
5.33211517333984 -0.393798828125
5.33224439620972 -0.393798828125
5.33227682113647 -0.393798828125
5.33229303359985 -0.393798828125
5.33230495452881 -0.393798828125
5.33244848251343 -0.393798828125
5.33266067504883 -0.393798828125
5.33302593231201 -0.393798828125
};
\addplot [ultra thick, blue]
table {%
-inf 0
0 -0.0006103515625
0.30103000998497 -0.00079345703125
0.477121233940125 -0.00103759765625
0.60206001996994 -0.00115966796875
0.60206001996994 -0.001220703125
0.778151273727417 -0.00152587890625
1 -0.0018310546875
1.07918119430542 -0.00213623046875
1.11394333839417 -0.002197265625
1.11394333839417 -0.0023193359375
1.17609131336212 -0.0025634765625
1.25527250766754 -0.002685546875
1.27875363826752 -0.0029296875
1.32221925258636 -0.0030517578125
1.34242272377014 -0.00311279296875
1.38021123409271 -0.00347900390625
1.67209792137146 -0.0091552734375
1.69896996021271 -0.01544189453125
1.77085208892822 -0.0174560546875
1.83250892162323 -0.0189208984375
1.88649070262909 -0.01995849609375
1.92941892147064 -0.02099609375
1.94448268413544 -0.021728515625
1.98677170276642 -0.0233154296875
2.02530574798584 -0.024169921875
2.05307841300964 -0.02520751953125
2.06445789337158 -0.0263671875
2.11394333839417 -0.03076171875
2.15228843688965 -0.0330810546875
2.20139718055725 -0.0340576171875
2.23552846908569 -0.03643798828125
2.29225611686707 -0.0399169921875
2.32221937179565 -0.0426025390625
2.35218262672424 -0.04486083984375
2.40824007987976 -0.05487060546875
2.45024919509888 -0.06072998046875
2.47275638580322 -0.0643310546875
2.50379061698914 -0.06890869140625
2.5365583896637 -0.07366943359375
2.55630254745483 -0.07696533203125
2.58771085739136 -0.0841064453125
2.62117624282837 -0.08740234375
2.6580114364624 -0.0916748046875
2.67302083969116 -0.09478759765625
2.69635629653931 -0.097412109375
2.70927000045776 -0.10009765625
2.73878049850464 -0.10577392578125
2.78604125976562 -0.11138916015625
2.81291341781616 -0.1192626953125
2.83378434181213 -0.13006591796875
2.86451101303101 -0.14031982421875
2.90145826339722 -0.1475830078125
2.91539978981018 -0.15380859375
2.9380190372467 -0.15972900390625
2.94841289520264 -0.1622314453125
2.96047067642212 -0.16424560546875
2.97081160545349 -0.16815185546875
2.99519634246826 -0.17144775390625
3.01367974281311 -0.178955078125
3.02775716781616 -0.180908203125
3.04139280319214 -0.18426513671875
3.04649519920349 -0.1851806640625
3.06182932853699 -0.1923828125
3.07445073127747 -0.19512939453125
3.08206701278687 -0.19720458984375
3.08813619613647 -0.19818115234375
3.09482049942017 -0.19903564453125
3.10414552688599 -0.20147705078125
3.10788798332214 -0.2022705078125
3.12807607650757 -0.2103271484375
3.14082217216492 -0.21343994140625
3.14674806594849 -0.21429443359375
3.15351009368896 -0.21588134765625
3.16106843948364 -0.217041015625
3.17055511474609 -0.21942138671875
3.17983889579773 -0.2227783203125
3.18610835075378 -0.22412109375
3.19173049926758 -0.22540283203125
3.19810700416565 -0.22698974609375
3.20411992073059 -0.22796630859375
3.21853542327881 -0.23358154296875
3.22401475906372 -0.23602294921875
3.23350381851196 -0.23883056640625
3.23879861831665 -0.2401123046875
3.24452447891235 -0.241455078125
3.25839781761169 -0.25048828125
3.26316237449646 -0.25201416015625
3.26951289176941 -0.2530517578125
3.27253770828247 -0.25360107421875
3.28330135345459 -0.25634765625
3.28914284706116 -0.25860595703125
3.29907131195068 -0.262939453125
3.30642509460449 -0.2642822265625
3.31026840209961 -0.26513671875
3.31344532966614 -0.26617431640625
3.32263278961182 -0.27099609375
3.32448816299438 -0.27191162109375
3.33203434944153 -0.2733154296875
3.33805775642395 -0.274169921875
3.34044408798218 -0.27459716796875
3.3479151725769 -0.2762451171875
3.36002516746521 -0.2825927734375
3.36248254776001 -0.28338623046875
3.36903023719788 -0.2840576171875
3.37106776237488 -0.2845458984375
3.38309693336487 -0.29071044921875
3.39164066314697 -0.29248046875
3.39252114295959 -0.29296875
3.39984679222107 -0.29547119140625
3.40191721916199 -0.2958984375
3.41161966323853 -0.2978515625
3.41564106941223 -0.29833984375
3.41713953018188 -0.29876708984375
3.42242574691772 -0.2994384765625
3.42910599708557 -0.30133056640625
3.43088102340698 -0.30181884765625
3.4353666305542 -0.302978515625
3.44263648986816 -0.30340576171875
3.44575977325439 -0.303955078125
3.4504029750824 -0.30450439453125
3.45392966270447 -0.304931640625
3.45606231689453 -0.30535888671875
3.4631462097168 -0.30657958984375
3.46996927261353 -0.3077392578125
3.47143840789795 -0.30816650390625
3.48387241363525 -0.31256103515625
3.4860053062439 -0.31353759765625
3.48967719078064 -0.31378173828125
3.49789667129517 -0.31634521484375
3.50009918212891 -0.31683349609375
3.50447082519531 -0.317138671875
3.51388311386108 -0.3243408203125
3.51798725128174 -0.32586669921875
3.52322602272034 -0.3287353515625
3.5291736125946 -0.33099365234375
3.53326344490051 -0.33233642578125
3.53744125366211 -0.3330078125
3.54973864555359 -0.3388671875
3.55108380317688 -0.33990478515625
3.55303311347961 -0.34014892578125
3.56050443649292 -0.34234619140625
3.57054281234741 -0.3453369140625
3.57403135299683 -0.345947265625
3.57449436187744 -0.3463134765625
3.57829523086548 -0.3468017578125
3.58103895187378 -0.34716796875
3.58399176597595 -0.3475341796875
3.58478331565857 -0.34771728515625
3.58793544769287 -0.3487548828125
3.59195446968079 -0.3489990234375
3.5945029258728 -0.3492431640625
3.59692692756653 -0.3497314453125
3.59944629669189 -0.34991455078125
3.60064625740051 -0.35015869140625
3.60713315010071 -0.35235595703125
3.6077766418457 -0.3526611328125
3.61034059524536 -0.35296630859375
3.61804819107056 -0.35504150390625
3.62024021148682 -0.35552978515625
3.62128019332886 -0.35577392578125
3.62314581871033 -0.35595703125
3.62736582756042 -0.356689453125
3.63083457946777 -0.35711669921875
3.63286209106445 -0.3572998046875
3.63427567481995 -0.35760498046875
3.63688898086548 -0.35797119140625
3.63868880271912 -0.35845947265625
3.64018321037292 -0.35858154296875
3.64087867736816 -0.3587646484375
3.6454222202301 -0.359619140625
3.64650177955627 -0.35980224609375
3.65234303474426 -0.360595703125
3.65590643882751 -0.36181640625
3.65657734870911 -0.36199951171875
3.66209650039673 -0.364501953125
3.66445398330688 -0.36480712890625
3.66651797294617 -0.3653564453125
3.66996741294861 -0.3656005859375
3.67135810852051 -0.3658447265625
3.67172813415527 -0.365966796875
3.67283654212952 -0.3660888671875
3.6741259098053 -0.3663330078125
3.67660212516785 -0.36651611328125
3.67705917358398 -0.3665771484375
3.68259620666504 -0.3682861328125
3.6845760345459 -0.368408203125
3.68574166297913 -0.3685302734375
3.68788552284241 -0.3687744140625
3.68850874900818 -0.368896484375
3.69037342071533 -0.3690185546875
3.69108152389526 -0.36920166015625
3.69399070739746 -0.3695068359375
3.69478058815002 -0.36962890625
3.69513130187988 -0.3697509765625
3.69679307937622 -0.369873046875
3.69731664657593 -0.36993408203125
3.69810056686401 -0.37005615234375
3.69827461242676 -0.37005615234375
3.70372104644775 -0.37066650390625
3.70475101470947 -0.37091064453125
3.70509362220764 -0.3709716796875
3.70612001419067 -0.37103271484375
3.70654702186584 -0.37115478515625
3.70654702186584 -0.3712158203125
3.71541833877563 -0.37432861328125
3.71667098999023 -0.374755859375
3.71916556358337 -0.3748779296875
3.71949696540833 -0.37493896484375
3.72403001785278 -0.37530517578125
3.72476720809937 -0.3753662109375
3.72640109062195 -0.37554931640625
3.72721576690674 -0.3756103515625
3.7290027141571 -0.375732421875
3.72981262207031 -0.3758544921875
3.73287606239319 -0.37615966796875
3.73335790634155 -0.37628173828125
3.73774909973145 -0.37713623046875
3.73909735679626 -0.37725830078125
3.74059963226318 -0.37744140625
3.74217510223389 -0.3775634765625
3.74358820915222 -0.37762451171875
3.74530911445618 -0.37774658203125
3.74741172790527 -0.3778076171875
3.75043129920959 -0.378173828125
3.75097107887268 -0.37823486328125
3.75587487220764 -0.37872314453125
3.75617957115173 -0.37884521484375
3.7575478553772 -0.37896728515625
3.75951671600342 -0.3790283203125
3.76057314872742 -0.379150390625
3.76320338249207 -0.37933349609375
3.76410126686096 -0.37945556640625
3.76656150817871 -0.379638671875
3.76745271682739 -0.3797607421875
3.7678234577179 -0.3798828125
3.77041006088257 -0.37994384765625
3.77202820777893 -0.3802490234375
3.77239513397217 -0.38037109375
3.77268838882446 -0.38037109375
3.77466297149658 -0.38067626953125
3.7749547958374 -0.38079833984375
3.77684640884399 -0.380859375
3.77713680267334 -0.38092041015625
3.7846884727478 -0.38238525390625
3.78490257263184 -0.38275146484375
3.78604125976562 -0.3828125
3.78639650344849 -0.3829345703125
3.78830981254578 -0.3829345703125
3.78830981254578 -0.38299560546875
3.79218149185181 -0.38299560546875
3.79232168197632 -0.383056640625
3.79232168197632 -0.383056640625
3.79253172874451 -0.38311767578125
3.79253172874451 -0.38311767578125
3.79253172874451 -0.3831787109375
3.79413938522339 -0.38330078125
3.79420900344849 -0.38336181640625
3.79434871673584 -0.38336181640625
3.79490613937378 -0.3834228515625
3.79518461227417 -0.3834228515625
3.79539322853088 -0.38348388671875
3.79643559455872 -0.383544921875
3.79650497436523 -0.383544921875
3.79657435417175 -0.383544921875
3.79692101478577 -0.38360595703125
3.79692101478577 -0.38360595703125
3.79823613166809 -0.3836669921875
3.79837441444397 -0.38372802734375
3.79851245880127 -0.3837890625
3.79885768890381 -0.3837890625
3.80044221878052 -0.38385009765625
3.8005108833313 -0.38385009765625
3.8005108833313 -0.3839111328125
3.80057954788208 -0.3839111328125
3.80064845085144 -0.3839111328125
3.80126643180847 -0.38397216796875
3.80154085159302 -0.384033203125
3.80243158340454 -0.38409423828125
3.80263686180115 -0.38409423828125
3.80386662483215 -0.3841552734375
3.8040030002594 -0.3841552734375
3.80413937568665 -0.3841552734375
3.80420756340027 -0.3841552734375
3.80556869506836 -0.38446044921875
3.80577254295349 -0.38446044921875
3.80651903152466 -0.384521484375
3.8065869808197 -0.384521484375
3.80665469169617 -0.384521484375
3.80685806274414 -0.38458251953125
3.80746746063232 -0.38458251953125
3.80746746063232 -0.38458251953125
3.8084135055542 -0.384765625
3.80848097801208 -0.384765625
3.80922293663025 -0.384765625
3.80935764312744 -0.38482666015625
3.80969429016113 -0.3848876953125
3.80989623069763 -0.3848876953125
3.81003069877625 -0.3848876953125
3.81077003479004 -0.38494873046875
3.81110572814941 -0.385009765625
3.81110572814941 -0.385009765625
3.81117272377014 -0.385009765625
3.81123971939087 -0.385009765625
3.81123971939087 -0.38507080078125
3.8113739490509 -0.38507080078125
3.8113739490509 -0.38507080078125
3.81237840652466 -0.3851318359375
3.81318044662476 -0.38519287109375
3.8135142326355 -0.38525390625
3.81371450424194 -0.38525390625
3.81384778022766 -0.38525390625
3.81471371650696 -0.38531494140625
3.8148467540741 -0.38531494140625
3.81491327285767 -0.38531494140625
3.81497979164124 -0.3853759765625
3.81497979164124 -0.3853759765625
3.8153121471405 -0.38543701171875
3.81544494628906 -0.38543701171875
3.81630754470825 -0.385498046875
3.81637382507324 -0.385498046875
3.81644010543823 -0.385498046875
3.81756544113159 -0.385498046875
3.81756544113159 -0.38555908203125
3.81756544113159 -0.38555908203125
3.81769752502441 -0.38555908203125
3.81769752502441 -0.3856201171875
3.81769752502441 -0.3856201171875
3.81796169281006 -0.3856201171875
3.81829190254211 -0.3856201171875
3.81855583190918 -0.38568115234375
3.81868767738342 -0.38568115234375
3.81941223144531 -0.3857421875
3.81954383850098 -0.3857421875
3.81960964202881 -0.3857421875
3.81960964202881 -0.3857421875
3.81967544555664 -0.38580322265625
3.81967544555664 -0.38580322265625
3.81967544555664 -0.38580322265625
3.8198070526123 -0.38580322265625
3.82079243659973 -0.3858642578125
3.82079243659973 -0.3858642578125
3.82079243659973 -0.3858642578125
3.82079243659973 -0.3858642578125
3.82432103157043 -0.38739013671875
3.82464647293091 -0.38763427734375
3.82490634918213 -0.38763427734375
3.82516646385193 -0.38763427734375
3.82516646385193 -0.38763427734375
3.82516646385193 -0.38763427734375
3.8278214931488 -0.3880615234375
3.8278214931488 -0.3880615234375
3.8286600112915 -0.3880615234375
3.82878875732422 -0.38812255859375
3.82885313034058 -0.38812255859375
3.82891750335693 -0.38812255859375
3.83001089096069 -0.38824462890625
3.83007526397705 -0.38824462890625
3.83007526397705 -0.38824462890625
3.83013939857483 -0.38824462890625
3.83020353317261 -0.3883056640625
3.83020353317261 -0.3883056640625
3.83174180984497 -0.38836669921875
3.83180570602417 -0.38836669921875
3.83180570602417 -0.38836669921875
3.83180570602417 -0.38836669921875
3.83238124847412 -0.388427734375
3.83250880241394 -0.388427734375
3.83257269859314 -0.388427734375
3.83352947235107 -0.38848876953125
3.83359336853027 -0.3885498046875
3.83372068405151 -0.3885498046875
3.83372068405151 -0.3885498046875
3.83372068405151 -0.3885498046875
3.83372068405151 -0.3885498046875
3.83524656295776 -0.38861083984375
3.83588075637817 -0.388671875
3.83600735664368 -0.388671875
3.83619737625122 -0.388671875
3.83670377731323 -0.38873291015625
3.83670377731323 -0.38873291015625
3.83683037757874 -0.38873291015625
3.8368935585022 -0.38873291015625
3.8368935585022 -0.38873291015625
3.8368935585022 -0.3887939453125
3.8368935585022 -0.3887939453125
3.83701992034912 -0.3887939453125
3.83701992034912 -0.3887939453125
3.83701992034912 -0.3887939453125
3.83733582496643 -0.3887939453125
3.83784079551697 -0.38885498046875
3.83790397644043 -0.38885498046875
3.83796691894531 -0.38885498046875
3.83796691894531 -0.38885498046875
3.83796691894531 -0.38885498046875
3.83796691894531 -0.388916015625
3.83796691894531 -0.388916015625
3.84060788154602 -0.38916015625
3.84079599380493 -0.38916015625
3.84098386764526 -0.38922119140625
3.84110903739929 -0.38922119140625
3.84135937690735 -0.38922119140625
3.84135937690735 -0.38922119140625
3.84135937690735 -0.38922119140625
3.84135937690735 -0.38922119140625
3.84135937690735 -0.3892822265625
3.84135937690735 -0.3892822265625
3.84135937690735 -0.3892822265625
3.84135937690735 -0.3892822265625
3.84185981750488 -0.3892822265625
3.84185981750488 -0.3892822265625
3.84185981750488 -0.3892822265625
3.84185981750488 -0.3892822265625
3.84185981750488 -0.3892822265625
3.84192228317261 -0.38934326171875
3.84192228317261 -0.38934326171875
3.84192228317261 -0.38934326171875
3.84192228317261 -0.38934326171875
3.84192228317261 -0.38934326171875
3.84210968017578 -0.389404296875
3.84210968017578 -0.389404296875
3.84304571151733 -0.389404296875
3.84310817718506 -0.389404296875
3.8431704044342 -0.389404296875
3.84751105308533 -0.39007568359375
3.84763431549072 -0.39007568359375
3.8479425907135 -0.39007568359375
3.8480658531189 -0.39007568359375
3.84812760353088 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.8482506275177 -0.39013671875
3.84905076026917 -0.39019775390625
3.84905076026917 -0.39019775390625
3.84905076026917 -0.39019775390625
3.84905076026917 -0.39019775390625
3.84905076026917 -0.39019775390625
3.84905076026917 -0.39019775390625
3.84905076026917 -0.39019775390625
3.84929656982422 -0.39019775390625
3.84929656982422 -0.39019775390625
3.84929656982422 -0.39019775390625
3.84929656982422 -0.39019775390625
3.85217499732971 -0.3905029296875
3.85229706764221 -0.3905029296875
3.85229706764221 -0.3905029296875
3.85229706764221 -0.3905029296875
3.85229706764221 -0.3905029296875
3.85229706764221 -0.3905029296875
3.85229706764221 -0.3905029296875
3.85229706764221 -0.3905029296875
3.85229706764221 -0.3905029296875
3.85290670394897 -0.3905029296875
3.85290670394897 -0.39056396484375
3.85290670394897 -0.39056396484375
3.85290670394897 -0.39056396484375
3.85290670394897 -0.39056396484375
3.85327219963074 -0.39056396484375
3.85436677932739 -0.39056396484375
3.85436677932739 -0.39056396484375
3.85436677932739 -0.39056396484375
3.85436677932739 -0.39056396484375
3.85442757606506 -0.39056396484375
3.85442757606506 -0.39056396484375
3.85442757606506 -0.39056396484375
3.85442757606506 -0.39056396484375
3.85442757606506 -0.39056396484375
3.85442757606506 -0.39056396484375
3.85442757606506 -0.39056396484375
3.85442757606506 -0.39056396484375
3.85467028617859 -0.390625
3.85485243797302 -0.390625
3.85485243797302 -0.390625
3.85485243797302 -0.390625
3.85509490966797 -0.390625
3.85678935050964 -0.39068603515625
3.85678935050964 -0.39068603515625
3.85751342773438 -0.39068603515625
3.85757374763489 -0.39068603515625
3.8576340675354 -0.39068603515625
3.8576340675354 -0.39068603515625
3.8576340675354 -0.39068603515625
3.8576340675354 -0.39068603515625
3.8576340675354 -0.3907470703125
3.85775446891785 -0.3907470703125
3.85775446891785 -0.3907470703125
3.85775446891785 -0.3907470703125
3.85781478881836 -0.3907470703125
3.85781478881836 -0.3907470703125
3.85853719711304 -0.3907470703125
3.85853719711304 -0.3907470703125
3.85853719711304 -0.3907470703125
3.85853719711304 -0.3907470703125
3.85853719711304 -0.3907470703125
3.85853719711304 -0.39080810546875
3.85877776145935 -0.39080810546875
3.85877776145935 -0.39080810546875
3.85877776145935 -0.39080810546875
3.85877776145935 -0.39080810546875
3.85877776145935 -0.39080810546875
3.85877776145935 -0.39080810546875
3.8602180480957 -0.39080810546875
3.8602180480957 -0.39080810546875
3.8602180480957 -0.39080810546875
3.8602180480957 -0.39080810546875
3.8602180480957 -0.390869140625
3.8602180480957 -0.390869140625
3.8602180480957 -0.390869140625
3.8602180480957 -0.390869140625
3.8602180480957 -0.390869140625
3.8602180480957 -0.390869140625
3.8602180480957 -0.390869140625
3.86242961883545 -0.39093017578125
3.86248922348022 -0.3909912109375
3.86260843276978 -0.3909912109375
3.86272764205933 -0.3909912109375
3.86272764205933 -0.3909912109375
3.86290621757507 -0.3909912109375
3.86290621757507 -0.3909912109375
3.86302518844604 -0.3909912109375
3.86302518844604 -0.3909912109375
3.86379861831665 -0.39105224609375
3.86385798454285 -0.39105224609375
3.86385798454285 -0.39105224609375
3.86385798454285 -0.39105224609375
3.86385798454285 -0.39105224609375
3.86528158187866 -0.39105224609375
3.86528158187866 -0.39111328125
3.86528158187866 -0.39111328125
3.86540007591248 -0.39111328125
3.86540007591248 -0.39111328125
3.86540007591248 -0.39111328125
3.86540007591248 -0.39111328125
3.86540007591248 -0.39111328125
3.86540007591248 -0.39111328125
3.86540007591248 -0.39111328125
3.86563682556152 -0.39111328125
3.86563682556152 -0.39111328125
3.86563682556152 -0.39111328125
3.86593270301819 -0.39111328125
3.86599183082581 -0.39111328125
3.86605095863342 -0.39111328125
3.86605095863342 -0.39111328125
3.86652374267578 -0.39117431640625
3.86652374267578 -0.39117431640625
3.86758542060852 -0.39117431640625
3.86758542060852 -0.39117431640625
3.86764430999756 -0.39117431640625
3.8677031993866 -0.39117431640625
3.86776208877563 -0.39117431640625
3.86776208877563 -0.39117431640625
3.86776208877563 -0.39117431640625
3.86776208877563 -0.39117431640625
3.86776208877563 -0.39117431640625
3.86923170089722 -0.3912353515625
3.86923170089722 -0.3912353515625
3.86929035186768 -0.3912353515625
3.86929035186768 -0.3912353515625
3.86929035186768 -0.3912353515625
3.86940765380859 -0.3912353515625
3.8701696395874 -0.3912353515625
3.87022829055786 -0.3912353515625
3.87022829055786 -0.3912353515625
3.87093043327332 -0.39129638671875
3.87093043327332 -0.39129638671875
3.87104725837708 -0.39129638671875
3.87116408348083 -0.39129638671875
3.87128090858459 -0.39129638671875
3.87227296829224 -0.39129638671875
3.87227296829224 -0.39129638671875
3.87227296829224 -0.39129638671875
3.87227296829224 -0.39129638671875
3.87227296829224 -0.39129638671875
3.8727388381958 -0.391357421875
3.8728551864624 -0.391357421875
3.8728551864624 -0.391357421875
3.8728551864624 -0.391357421875
3.87308788299561 -0.391357421875
3.87332057952881 -0.391357421875
3.87332057952881 -0.391357421875
3.87332057952881 -0.391357421875
3.87355303764343 -0.391357421875
3.87436580657959 -0.391357421875
3.87436580657959 -0.391357421875
3.87453985214233 -0.391357421875
3.87459778785706 -0.391357421875
3.87465572357178 -0.39141845703125
3.8747136592865 -0.39141845703125
3.8747136592865 -0.39141845703125
3.8747136592865 -0.39141845703125
3.87482953071594 -0.39141845703125
3.87482953071594 -0.39141845703125
3.87482953071594 -0.39141845703125
3.87494540214539 -0.39141845703125
3.87506127357483 -0.39141845703125
3.87558221817017 -0.39141845703125
3.87558221817017 -0.39141845703125
3.87581348419189 -0.39141845703125
3.87581348419189 -0.39141845703125
3.87587118148804 -0.39141845703125
3.87592887878418 -0.39141845703125
3.8759868144989 -0.39141845703125
3.87702560424805 -0.39141845703125
3.87702560424805 -0.39141845703125
3.87748646736145 -0.3914794921875
3.87754416465759 -0.3914794921875
3.87754416465759 -0.3914794921875
3.87754416465759 -0.3914794921875
3.87754416465759 -0.3914794921875
3.87754416465759 -0.3914794921875
3.87754416465759 -0.3914794921875
3.87777423858643 -0.3914794921875
3.87777423858643 -0.3914794921875
3.87777423858643 -0.3914794921875
3.87777423858643 -0.3914794921875
3.87777423858643 -0.3914794921875
3.87777423858643 -0.3914794921875
3.87777423858643 -0.3914794921875
3.8780620098114 -0.3914794921875
3.8780620098114 -0.3914794921875
3.8780620098114 -0.3914794921875
3.8803563117981 -0.39154052734375
3.88047051429749 -0.39154052734375
3.88047051429749 -0.39154052734375
3.88047051429749 -0.39154052734375
3.88047051429749 -0.39154052734375
3.88047051429749 -0.39154052734375
3.88047051429749 -0.39154052734375
3.88047051429749 -0.39154052734375
3.88047051429749 -0.39154052734375
3.88047051429749 -0.39154052734375
3.88132762908936 -0.3916015625
3.88246750831604 -0.3916015625
3.88246750831604 -0.3916015625
3.88246750831604 -0.3916015625
3.88246750831604 -0.39166259765625
3.88269519805908 -0.39166259765625
3.88269519805908 -0.39166259765625
3.88269519805908 -0.39166259765625
3.88297963142395 -0.39166259765625
3.88297963142395 -0.39166259765625
3.88332056999207 -0.39166259765625
3.88366150856018 -0.39166259765625
3.88366150856018 -0.39166259765625
3.88366150856018 -0.39166259765625
3.88394522666931 -0.39166259765625
3.88394522666931 -0.39166259765625
3.88394522666931 -0.39166259765625
3.88394522666931 -0.39166259765625
3.8852481842041 -0.3917236328125
3.8852481842041 -0.3917236328125
3.8852481842041 -0.3917236328125
3.8852481842041 -0.3917236328125
3.8852481842041 -0.3917236328125
3.88547420501709 -0.3917236328125
3.88570046424866 -0.3917236328125
3.8857569694519 -0.3917236328125
3.8857569694519 -0.3917236328125
3.88694167137146 -0.39178466796875
3.88699793815613 -0.39178466796875
3.88727951049805 -0.39178466796875
3.88727951049805 -0.39178466796875
3.88733601570129 -0.39178466796875
3.8875048160553 -0.39178466796875
3.8875048160553 -0.39178466796875
3.8875048160553 -0.39178466796875
3.88761734962463 -0.39178466796875
3.8876736164093 -0.39178466796875
3.88772988319397 -0.39178466796875
3.88784217834473 -0.39178466796875
3.88784217834473 -0.39178466796875
3.88829183578491 -0.39178466796875
3.88834810256958 -0.39178466796875
3.88834810256958 -0.39178466796875
3.88834810256958 -0.39178466796875
3.88834810256958 -0.39178466796875
3.88834810256958 -0.39178466796875
3.88857269287109 -0.39178466796875
3.88890933990479 -0.391845703125
3.88890933990479 -0.391845703125
3.88890933990479 -0.391845703125
3.890700340271 -0.39190673828125
3.8908679485321 -0.39190673828125
3.8908679485321 -0.39190673828125
3.89114713668823 -0.39190673828125
3.89114713668823 -0.39190673828125
3.89114713668823 -0.39190673828125
3.8914258480072 -0.39190673828125
3.8914258480072 -0.39190673828125
3.8914258480072 -0.39190673828125
3.89159321784973 -0.39190673828125
3.89159321784973 -0.39190673828125
3.89159321784973 -0.39190673828125
3.89159321784973 -0.39190673828125
3.89159321784973 -0.39190673828125
3.8918719291687 -0.39190673828125
3.8918719291687 -0.3919677734375
3.89376163482666 -0.39202880859375
3.89453744888306 -0.39208984375
3.89453744888306 -0.39208984375
3.89453744888306 -0.39208984375
3.89453744888306 -0.39208984375
3.89464831352234 -0.39208984375
3.89464831352234 -0.39208984375
3.89464831352234 -0.39208984375
3.89464831352234 -0.39208984375
3.89652633666992 -0.39208984375
3.89658141136169 -0.39208984375
3.89658141136169 -0.39208984375
3.89658141136169 -0.39208984375
3.89768195152283 -0.3922119140625
3.89888954162598 -0.39227294921875
3.89905405044556 -0.39227294921875
3.89905405044556 -0.39227294921875
3.89921832084656 -0.39227294921875
3.9000940322876 -0.39227294921875
3.9000940322876 -0.39227294921875
3.9000940322876 -0.39227294921875
3.9000940322876 -0.39227294921875
3.9000940322876 -0.39227294921875
3.9000940322876 -0.39227294921875
3.90031242370605 -0.39227294921875
3.90031242370605 -0.39227294921875
3.9008584022522 -0.392333984375
3.90091300010681 -0.392333984375
3.90096759796143 -0.392333984375
3.90102219581604 -0.392333984375
3.90113115310669 -0.392333984375
3.90113115310669 -0.392333984375
3.90134930610657 -0.392333984375
3.90162181854248 -0.392333984375
3.90178513526917 -0.392333984375
3.90178513526917 -0.392333984375
3.90178513526917 -0.392333984375
3.90205717086792 -0.392333984375
3.90303564071655 -0.392333984375
3.90303564071655 -0.392333984375
3.90303564071655 -0.392333984375
3.90303564071655 -0.392333984375
3.90303564071655 -0.392333984375
3.90357828140259 -0.39239501953125
3.90357828140259 -0.39239501953125
3.90357828140259 -0.39239501953125
3.90379524230957 -0.39239501953125
3.90379524230957 -0.39239501953125
3.90390348434448 -0.39239501953125
3.90390348434448 -0.39239501953125
3.90417432785034 -0.39239501953125
3.90417432785034 -0.39239501953125
3.90417432785034 -0.39239501953125
3.90417432785034 -0.39239501953125
3.90417432785034 -0.39239501953125
3.90417432785034 -0.39239501953125
3.90417432785034 -0.39239501953125
3.90417432785034 -0.39239501953125
3.90417432785034 -0.39239501953125
3.90493178367615 -0.3924560546875
3.90590381622314 -0.3924560546875
3.90590381622314 -0.3924560546875
3.90590381622314 -0.3924560546875
3.90590381622314 -0.3924560546875
3.90590381622314 -0.3924560546875
3.90611934661865 -0.3924560546875
3.90611934661865 -0.3924560546875
3.90611934661865 -0.3924560546875
3.90633511543274 -0.3924560546875
3.90633511543274 -0.3924560546875
3.90633511543274 -0.3924560546875
3.90633511543274 -0.3924560546875
3.90633511543274 -0.3924560546875
3.90773367881775 -0.39251708984375
3.90773367881775 -0.39251708984375
3.90794849395752 -0.39251708984375
3.90800213813782 -0.39251708984375
3.90800213813782 -0.39251708984375
3.90800213813782 -0.39251708984375
3.90821695327759 -0.39251708984375
3.90821695327759 -0.39251708984375
3.90843152999878 -0.39251708984375
3.9085385799408 -0.39251708984375
3.9085385799408 -0.392578125
3.9085385799408 -0.392578125
3.90859222412109 -0.392578125
3.90859222412109 -0.392578125
3.908860206604 -0.392578125
3.908860206604 -0.392578125
3.908860206604 -0.392578125
3.908860206604 -0.392578125
3.908860206604 -0.392578125
3.908860206604 -0.392578125
3.90993022918701 -0.392578125
3.90993022918701 -0.392578125
3.91019725799561 -0.392578125
3.91019725799561 -0.392578125
3.91019725799561 -0.392578125
3.91019725799561 -0.392578125
3.9104642868042 -0.392578125
3.91073107719421 -0.392578125
3.91078448295593 -0.392578125
3.91099762916565 -0.39263916015625
3.91115760803223 -0.39263916015625
3.91126418113708 -0.39263916015625
3.91126418113708 -0.39263916015625
3.91126418113708 -0.39263916015625
3.91126418113708 -0.39263916015625
3.91126418113708 -0.39263916015625
3.91222214698792 -0.39263916015625
3.91222214698792 -0.39263916015625
3.91238141059875 -0.39263916015625
3.91238141059875 -0.39263916015625
3.91238141059875 -0.39263916015625
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{F2O}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.404066467285156, ymax=0.0192092895507813,
ytick style={color=black},
ytick distance=0.2,
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c10)}
]
\addplot [ultra thick, brown, dashed]
table {%
0.954242527484894 -3.0517578125e-05
1.70757019519806 -9.1552734375e-05
1.86332285404205 -9.1552734375e-05
2.07554697990417 -0.0001220703125
2.32014632225037 -0.000244140625
2.39967370033264 -0.000274658203125
2.41830134391785 -0.00030517578125
2.43456888198853 -0.0003662109375
2.53907608985901 -0.000457763671875
2.55509448051453 -0.000579833984375
2.58658742904663 -0.0006103515625
2.59769511222839 -0.0006103515625
2.71011734008789 -0.00079345703125
2.74818801879883 -0.000885009765625
2.75358295440674 -0.00091552734375
2.7723217010498 -0.0009765625
2.80277371406555 -0.00103759765625
2.82216811180115 -0.0010986328125
2.86153435707092 -0.00115966796875
2.86569595336914 -0.001190185546875
2.91698002815247 -0.00128173828125
2.95760726928711 -0.0013427734375
2.96094608306885 -0.001434326171875
3.03422737121582 -0.001678466796875
3.12221598625183 -0.00341796875
3.14488530158997 -0.007080078125
3.1838390827179 -0.008697509765625
3.21563768386841 -0.009521484375
3.25695824623108 -0.010162353515625
3.29710364341736 -0.01190185546875
3.39040517807007 -0.0194091796875
3.43822574615479 -0.02569580078125
3.49289989471436 -0.0303955078125
3.61108565330505 -0.040313720703125
3.7140781879425 -0.05328369140625
3.78461718559265 -0.071990966796875
3.84167218208313 -0.086181640625
3.86605095863342 -0.090911865234375
3.89619541168213 -0.095001220703125
3.91397261619568 -0.096954345703125
3.93786883354187 -0.101318359375
3.95775079727173 -0.10321044921875
3.98407697677612 -0.111541748046875
4.01665735244751 -0.118072509765625
4.02706384658813 -0.12115478515625
4.06565427780151 -0.134674072265625
4.10390615463257 -0.146759033203125
4.11988258361816 -0.155120849609375
4.13369846343994 -0.160247802734375
4.14804697036743 -0.163818359375
4.15989780426025 -0.16595458984375
4.1687331199646 -0.16839599609375
4.17626476287842 -0.169677734375
4.18650436401367 -0.171600341796875
4.20090532302856 -0.17498779296875
4.21716785430908 -0.18157958984375
4.22523164749146 -0.1851806640625
4.23471975326538 -0.18829345703125
4.24440097808838 -0.190032958984375
4.25377416610718 -0.191741943359375
4.25839757919312 -0.19268798828125
4.26862478256226 -0.196868896484375
4.27639293670654 -0.1982421875
4.28467893600464 -0.19915771484375
4.29338455200195 -0.200531005859375
4.29902744293213 -0.2021484375
4.30616760253906 -0.203125
4.31321334838867 -0.205718994140625
4.32161903381348 -0.206878662109375
4.32976388931274 -0.20843505859375
4.33897399902344 -0.211944580078125
4.34611797332764 -0.2132568359375
4.35191202163696 -0.21453857421875
4.36834287643433 -0.224365234375
4.37278318405151 -0.226959228515625
4.37970447540283 -0.232147216796875
4.38596343994141 -0.23382568359375
4.39937973022461 -0.23699951171875
4.40449142456055 -0.2388916015625
4.41477298736572 -0.243560791015625
4.42509365081787 -0.248046875
4.43142795562744 -0.251190185546875
4.43822574615479 -0.253265380859375
4.4451060295105 -0.25732421875
4.45565176010132 -0.2637939453125
4.45788192749023 -0.266204833984375
4.46469831466675 -0.268157958984375
4.47120380401611 -0.269805908203125
4.48085451126099 -0.277618408203125
4.49641752243042 -0.28594970703125
4.49952220916748 -0.28729248046875
4.50485134124756 -0.28936767578125
4.50711345672607 -0.2901611328125
4.5112681388855 -0.291229248046875
4.51868486404419 -0.292694091796875
4.53104448318481 -0.298553466796875
4.53391170501709 -0.29949951171875
4.53851079940796 -0.300201416015625
4.54049205780029 -0.300506591796875
4.55098628997803 -0.310760498046875
4.55683279037476 -0.31353759765625
4.56016969680786 -0.314178466796875
4.56331491470337 -0.31561279296875
4.56973648071289 -0.316253662109375
4.57491064071655 -0.317596435546875
4.578444480896 -0.31829833984375
4.58296060562134 -0.3193359375
4.59012842178345 -0.32086181640625
4.59262084960938 -0.32159423828125
4.60029745101929 -0.325225830078125
4.60292768478394 -0.32586669921875
4.60817289352417 -0.32696533203125
4.61062812805176 -0.32733154296875
4.61636018753052 -0.327880859375
4.62066698074341 -0.3282470703125
4.62342500686646 -0.328826904296875
4.62794923782349 -0.32989501953125
4.63078355789185 -0.330230712890625
4.63418483734131 -0.33050537109375
4.63770961761475 -0.331024169921875
4.64227676391602 -0.331573486328125
4.64532423019409 -0.332122802734375
4.64877939224243 -0.33258056640625
4.6567211151123 -0.335235595703125
4.65834522247314 -0.33575439453125
4.66260671615601 -0.33648681640625
4.66684532165527 -0.336822509765625
4.67327880859375 -0.338104248046875
4.67986392974854 -0.34185791015625
4.68480968475342 -0.343994140625
4.68789434432983 -0.34503173828125
4.69230031967163 -0.34552001953125
4.69392013549805 -0.345703125
4.7002534866333 -0.34918212890625
4.70365238189697 -0.349822998046875
4.70554733276367 -0.3499755859375
4.70845508575439 -0.3502197265625
4.71271705627441 -0.356170654296875
4.71431303024292 -0.36004638671875
4.71673774719238 -0.360870361328125
4.71811103820801 -0.361358642578125
4.71955490112305 -0.361846923828125
4.72106027603149 -0.36212158203125
4.72357082366943 -0.362823486328125
4.72398090362549 -0.363037109375
4.7257399559021 -0.36328125
4.726881980896 -0.3634033203125
4.72829675674438 -0.363739013671875
4.72930240631104 -0.3638916015625
4.7301926612854 -0.364105224609375
4.73083877563477 -0.3642578125
4.73158884048462 -0.36431884765625
4.73323726654053 -0.364410400390625
4.73406314849854 -0.364501953125
4.73460006713867 -0.36456298828125
4.735511302948 -0.3646240234375
4.73712110519409 -0.36492919921875
4.73841571807861 -0.3651123046875
4.73916864395142 -0.36517333984375
4.73968315124512 -0.365203857421875
4.74067068099976 -0.365325927734375
4.74228525161743 -0.365509033203125
4.7434549331665 -0.365570068359375
4.74628400802612 -0.3662109375
4.74709320068359 -0.366363525390625
4.74793195724487 -0.366424560546875
4.74907112121582 -0.366668701171875
4.75093269348145 -0.366851806640625
4.75187921524048 -0.366943359375
4.75293922424316 -0.36700439453125
4.75302362442017 -0.3670654296875
4.75417232513428 -0.3670654296875
4.75883626937866 -0.37078857421875
4.75943374633789 -0.37139892578125
4.76073169708252 -0.371612548828125
4.76258850097656 -0.3717041015625
4.76328563690186 -0.37176513671875
4.76487064361572 -0.37188720703125
4.76516151428223 -0.371917724609375
4.76574325561523 -0.3719482421875
4.76676988601685 -0.372039794921875
4.76797151565552 -0.37213134765625
4.76885986328125 -0.372161865234375
4.77027750015259 -0.37225341796875
4.77053546905518 -0.372283935546875
4.7708740234375 -0.372314453125
4.77144050598145 -0.372344970703125
4.7724609375 -0.372467041015625
4.77259302139282 -0.37249755859375
4.774582862854 -0.372589111328125
4.77539205551147 -0.3726806640625
4.77644681930542 -0.372802734375
4.77773857116699 -0.372833251953125
4.7783899307251 -0.37286376953125
4.77849864959717 -0.37286376953125
4.77914190292358 -0.372955322265625
4.78068447113037 -0.373291015625
4.78157567977905 -0.37335205078125
4.78230762481689 -0.373382568359375
4.78278064727783 -0.3734130859375
4.78336048126221 -0.37347412109375
4.78449583053589 -0.373565673828125
4.78484535217285 -0.37359619140625
4.78519439697266 -0.373626708984375
4.78595590591431 -0.37371826171875
4.78687191009521 -0.373809814453125
4.78757381439209 -0.373809814453125
4.78781461715698 -0.37384033203125
4.78830289840698 -0.37384033203125
4.79181003570557 -0.3756103515625
4.79267883300781 -0.376068115234375
4.79290962219238 -0.376068115234375
4.79389524459839 -0.376220703125
4.79457855224609 -0.376251220703125
4.79481554031372 -0.376251220703125
4.79548358917236 -0.3763427734375
4.7960467338562 -0.3763427734375
4.79633855819702 -0.376373291015625
4.79764842987061 -0.376373291015625
4.79796648025513 -0.37640380859375
4.79833316802979 -0.37640380859375
4.79941654205322 -0.37646484375
4.79980897903442 -0.376495361328125
4.8007378578186 -0.376556396484375
4.80120468139648 -0.3765869140625
4.80187702178955 -0.3765869140625
4.80201387405396 -0.376617431640625
4.80288982391357 -0.37664794921875
4.803307056427 -0.37664794921875
4.80347061157227 -0.376678466796875
4.80410528182983 -0.376708984375
4.8042893409729 -0.376708984375
4.80583381652832 -0.377197265625
4.80626821517944 -0.377227783203125
4.80638360977173 -0.377227783203125
4.80710887908936 -0.37725830078125
4.80735921859741 -0.37725830078125
4.80787992477417 -0.377288818359375
4.80837965011597 -0.377349853515625
4.80951929092407 -0.377349853515625
4.80994987487793 -0.37738037109375
4.81042766571045 -0.37744140625
4.81086397171021 -0.37744140625
4.81217098236084 -0.3780517578125
4.81231832504272 -0.37811279296875
4.81317377090454 -0.378143310546875
4.81401443481445 -0.378143310546875
4.8157901763916 -0.378631591796875
4.81668519973755 -0.378692626953125
4.8167781829834 -0.378692626953125
4.81733417510986 -0.3787841796875
4.81797504425049 -0.3787841796875
4.81836462020874 -0.378814697265625
4.81852293014526 -0.378814697265625
4.81906986236572 -0.378814697265625
4.81974124908447 -0.37884521484375
4.82041168212891 -0.378875732421875
4.8207859992981 -0.37890625
4.82108736038208 -0.37890625
4.82180166244507 -0.378936767578125
4.82202434539795 -0.37896728515625
4.82312202453613 -0.37896728515625
4.82419109344482 -0.379669189453125
4.82502365112305 -0.3797607421875
4.82554292678833 -0.3797607421875
4.82624340057373 -0.379791259765625
4.82674837112427 -0.37982177734375
4.82703304290771 -0.37982177734375
4.82789897918701 -0.379974365234375
4.8280668258667 -0.3800048828125
4.82833766937256 -0.3800048828125
4.82923316955566 -0.3800048828125
4.82957410812378 -0.380035400390625
4.83028078079224 -0.38006591796875
4.83051824569702 -0.38006591796875
4.83162021636963 -0.380126953125
4.83198499679565 -0.380157470703125
4.8325023651123 -0.38018798828125
4.83319807052612 -0.38018798828125
4.83368253707886 -0.38018798828125
4.83430004119873 -0.380279541015625
4.83499908447266 -0.380279541015625
4.8350305557251 -0.380279541015625
4.83599472045898 -0.38031005859375
4.83655214309692 -0.38031005859375
4.836754322052 -0.380340576171875
4.8372220993042 -0.380340576171875
4.83739280700684 -0.380340576171875
4.83878612518311 -0.380523681640625
4.83910703659058 -0.380523681640625
4.83986139297485 -0.38055419921875
4.84018754959106 -0.38055419921875
4.8405327796936 -0.38055419921875
4.84222841262817 -0.3812255859375
4.84300231933594 -0.38134765625
4.84331369400024 -0.381378173828125
4.84416627883911 -0.381439208984375
4.84430932998657 -0.381439208984375
4.84550714492798 -0.3814697265625
4.84621334075928 -0.381500244140625
4.84656000137329 -0.381500244140625
4.8476095199585 -0.38177490234375
4.84778833389282 -0.3818359375
4.84831857681274 -0.3818359375
4.84882307052612 -0.381866455078125
4.84912443161011 -0.381866455078125
4.84955453872681 -0.381866455078125
4.85029077529907 -0.38189697265625
4.85075664520264 -0.38189697265625
4.85134410858154 -0.38189697265625
4.85177803039551 -0.381927490234375
4.85237646102905 -0.381927490234375
4.85321760177612 -0.381927490234375
4.85411787033081 -0.3819580078125
4.8545184135437 -0.3819580078125
4.8552827835083 -0.381988525390625
4.85619688034058 -0.382110595703125
4.85674715042114 -0.38214111328125
4.85697650909424 -0.38214111328125
4.85734462738037 -0.38214111328125
4.85792922973633 -0.382171630859375
4.85859727859497 -0.3822021484375
4.85873556137085 -0.3822021484375
4.85896396636963 -0.382232666015625
4.85927057266235 -0.382232666015625
4.85973834991455 -0.382232666015625
4.86018228530884 -0.38226318359375
4.86083507537842 -0.38226318359375
4.86105632781982 -0.38226318359375
4.86107397079468 -0.38226318359375
4.86130142211914 -0.38226318359375
4.86161804199219 -0.382293701171875
4.86223888397217 -0.382354736328125
4.86239957809448 -0.382354736328125
4.86302518844604 -0.38238525390625
4.86417293548584 -0.3824462890625
4.86445188522339 -0.382476806640625
4.86471891403198 -0.382476806640625
4.86510992050171 -0.38250732421875
4.86532926559448 -0.38250732421875
4.86567258834839 -0.38250732421875
4.8657431602478 -0.38250732421875
4.86603927612305 -0.382537841796875
4.86695432662964 -0.382537841796875
4.86703729629517 -0.382537841796875
4.86769151687622 -0.382537841796875
4.86772060394287 -0.382537841796875
4.86832714080811 -0.382568359375
4.86880874633789 -0.382598876953125
4.86885595321655 -0.382598876953125
4.86953687667847 -0.38262939453125
4.86957788467407 -0.38262939453125
4.86988258361816 -0.38262939453125
4.86998224258423 -0.38262939453125
4.87059688568115 -0.382659912109375
4.87085437774658 -0.382659912109375
4.87101221084595 -0.382659912109375
4.87133932113647 -0.3826904296875
4.87180614471436 -0.3826904296875
4.87203407287598 -0.3826904296875
4.87208652496338 -0.382720947265625
4.87225532531738 -0.382720947265625
4.87226724624634 -0.382720947265625
4.87265729904175 -0.382720947265625
4.87281465530396 -0.382720947265625
4.87341356277466 -0.382781982421875
4.87366914749146 -0.382781982421875
4.87391328811646 -0.382781982421875
4.8740816116333 -0.3828125
4.87419176101685 -0.3828125
4.87469053268433 -0.382843017578125
4.8750901222229 -0.382843017578125
4.87514209747314 -0.382843017578125
4.87596368789673 -0.382904052734375
4.87607908248901 -0.382904052734375
4.87656402587891 -0.382965087890625
4.87684106826782 -0.382965087890625
4.87711763381958 -0.382965087890625
4.87714672088623 -0.382965087890625
4.8773250579834 -0.382965087890625
4.87753820419312 -0.382965087890625
4.87767648696899 -0.38299560546875
4.8786940574646 -0.383087158203125
4.87908458709717 -0.383087158203125
4.87913036346436 -0.383087158203125
4.87914752960205 -0.383087158203125
4.87959480285645 -0.38311767578125
4.87962341308594 -0.38311767578125
4.88067054748535 -0.38311767578125
4.88106489181519 -0.383148193359375
4.88108777999878 -0.383148193359375
4.88147020339966 -0.3831787109375
4.88149881362915 -0.3831787109375
4.88206911087036 -0.383209228515625
4.88211441040039 -0.383209228515625
4.88214302062988 -0.383209228515625
4.88295698165894 -0.383270263671875
4.88401889801025 -0.38330078125
4.88456296920776 -0.38330078125
4.88472747802734 -0.38330078125
4.88480091094971 -0.38330078125
4.88496541976929 -0.38330078125
4.88538360595703 -0.383331298828125
4.88541221618652 -0.383331298828125
4.88559865951538 -0.383331298828125
4.88581323623657 -0.383331298828125
4.88605070114136 -0.383331298828125
4.88606739044189 -0.383331298828125
4.88612413406372 -0.383331298828125
4.88620281219482 -0.383331298828125
4.88691902160645 -0.38336181640625
4.88709926605225 -0.38336181640625
4.88810634613037 -0.383453369140625
4.88827514648438 -0.383453369140625
4.88852214813232 -0.38348388671875
4.88855028152466 -0.38348388671875
4.88878583908081 -0.38348388671875
4.88934087753296 -0.38348388671875
4.88936901092529 -0.38348388671875
4.8894248008728 -0.38348388671875
4.88994550704956 -0.383514404296875
4.88997936248779 -0.383514404296875
4.89011907577515 -0.383514404296875
4.89020299911499 -0.383514404296875
4.89023113250732 -0.383514404296875
4.89037609100342 -0.383514404296875
4.89049911499023 -0.383514404296875
4.89054393768311 -0.383514404296875
4.8906946182251 -0.383514404296875
4.89115238189697 -0.383544921875
4.89119148254395 -0.383544921875
4.89191627502441 -0.383544921875
4.89194440841675 -0.383544921875
4.89222812652588 -0.383575439453125
4.89225053787231 -0.383575439453125
4.89236164093018 -0.383575439453125
4.89237833023071 -0.383575439453125
4.89240646362305 -0.383575439453125
4.89272308349609 -0.383575439453125
4.8930344581604 -0.383575439453125
4.89311218261719 -0.383575439453125
4.89344549179077 -0.383575439453125
4.89344549179077 -0.383575439453125
4.89361763000488 -0.383575439453125
4.89399480819702 -0.383575439453125
4.89399480819702 -0.383575439453125
4.89406681060791 -0.383575439453125
4.8946704864502 -0.383636474609375
4.89469814300537 -0.383636474609375
4.89504098892212 -0.3836669921875
4.89514064788818 -0.3836669921875
4.89516830444336 -0.3836669921875
4.89519596099854 -0.3836669921875
4.89572095870972 -0.3836669921875
4.89579820632935 -0.3836669921875
4.89597463607788 -0.3836669921875
4.89599657058716 -0.3836669921875
4.89602422714233 -0.3836669921875
4.89685678482056 -0.383697509765625
4.89688968658447 -0.383697509765625
4.89688968658447 -0.383697509765625
4.89805030822754 -0.38372802734375
4.89807748794556 -0.38372802734375
4.8981876373291 -0.383758544921875
4.89854955673218 -0.383758544921875
4.89856052398682 -0.383758544921875
4.89876890182495 -0.383758544921875
4.89881277084351 -0.383758544921875
4.89936065673828 -0.383758544921875
4.89974403381348 -0.383758544921875
4.89990234375 -0.383758544921875
4.90017032623291 -0.3837890625
4.90032339096069 -0.3837890625
4.90035057067871 -0.3837890625
4.90054750442505 -0.3837890625
4.90054750442505 -0.3837890625
4.90193223953247 -0.383819580078125
4.90196466445923 -0.383819580078125
4.90199184417725 -0.383819580078125
4.90205192565918 -0.383819580078125
4.9025411605835 -0.38385009765625
4.90274238586426 -0.38385009765625
4.90312814712524 -0.383880615234375
4.90324735641479 -0.383880615234375
4.90326929092407 -0.383880615234375
4.90358352661133 -0.383880615234375
4.90361070632935 -0.383880615234375
4.90404415130615 -0.383880615234375
4.90463447570801 -0.383880615234375
4.90466165542603 -0.3839111328125
4.90466165542603 -0.3839111328125
4.9047966003418 -0.3839111328125
4.90480756759644 -0.3839111328125
4.90542364120483 -0.383941650390625
4.90614080429077 -0.38397216796875
4.90629196166992 -0.38397216796875
4.90660429000854 -0.38397216796875
4.90686798095703 -0.38397216796875
4.90716934204102 -0.38397216796875
4.90735244750977 -0.38397216796875
4.90737915039062 -0.38397216796875
4.90743827819824 -0.38397216796875
4.90765333175659 -0.38397216796875
4.90768003463745 -0.38397216796875
4.90771770477295 -0.38397216796875
4.90799140930176 -0.38397216796875
4.90821170806885 -0.384002685546875
4.90872097015381 -0.384002685546875
4.908860206604 -0.384002685546875
4.90888690948486 -0.384002685546875
4.90928840637207 -0.384002685546875
4.90938997268677 -0.384002685546875
4.90938997268677 -0.384002685546875
4.91027736663818 -0.384124755859375
4.91045904159546 -0.384124755859375
4.9105281829834 -0.384124755859375
4.9106616973877 -0.384124755859375
4.91117382049561 -0.384124755859375
4.91178607940674 -0.3841552734375
4.91236019134521 -0.3841552734375
4.91271591186523 -0.3841552734375
4.91274261474609 -0.3841552734375
4.91283845901489 -0.3841552734375
4.91324138641357 -0.3841552734375
4.9137716293335 -0.3841552734375
4.91384029388428 -0.3841552734375
4.91386699676514 -0.384185791015625
4.91411018371582 -0.384185791015625
4.91544723510742 -0.384246826171875
4.91549491882324 -0.38427734375
4.9161696434021 -0.38427734375
4.91620111465454 -0.38427734375
4.91645383834839 -0.38427734375
4.91744756698608 -0.38427734375
4.91747379302979 -0.38427734375
4.9177942276001 -0.384307861328125
4.9178204536438 -0.384307861328125
4.91794633865356 -0.384307861328125
4.91797256469727 -0.384307861328125
4.91817188262939 -0.384307861328125
4.91832399368286 -0.384307861328125
4.91836595535278 -0.384307861328125
4.91864347457886 -0.384307861328125
4.92017555236816 -0.384429931640625
4.92051458358765 -0.384429931640625
4.92054080963135 -0.384429931640625
4.92068672180176 -0.384429931640625
4.92071294784546 -0.384429931640625
4.92071294784546 -0.384429931640625
4.92104625701904 -0.384429931640625
4.92153549194336 -0.384429931640625
4.92246055603027 -0.384429931640625
4.92298460006714 -0.384429931640625
4.92302131652832 -0.384429931640625
4.92345666885376 -0.38446044921875
4.92354965209961 -0.38446044921875
4.92357540130615 -0.38446044921875
4.92360162734985 -0.38446044921875
4.92364311218262 -0.38446044921875
4.92366886138916 -0.38446044921875
4.92366886138916 -0.38446044921875
4.92479610443115 -0.384521484375
4.92483234405518 -0.384521484375
4.92551326751709 -0.384521484375
4.92553901672363 -0.384521484375
4.92576599121094 -0.384521484375
4.92577600479126 -0.384521484375
4.92582225799561 -0.384521484375
4.92607498168945 -0.384552001953125
4.92615699768066 -0.384552001953125
4.92625999450684 -0.384552001953125
4.92628049850464 -0.384552001953125
4.92630624771118 -0.384552001953125
4.92651224136353 -0.384552001953125
4.92682600021362 -0.384552001953125
4.92685651779175 -0.384552001953125
4.92694902420044 -0.38458251953125
4.92715978622437 -0.38458251953125
4.92769384384155 -0.38458251953125
4.92772436141968 -0.38458251953125
4.92772436141968 -0.38458251953125
4.93084716796875 -0.384796142578125
4.93123388290405 -0.384796142578125
4.93133592605591 -0.384796142578125
4.93136119842529 -0.384796142578125
4.93137645721436 -0.384796142578125
4.93191003799438 -0.384796142578125
4.93193578720093 -0.384796142578125
4.93220472335815 -0.384796142578125
4.93221998214722 -0.384796142578125
4.93232679367065 -0.384796142578125
4.93232679367065 -0.38482666015625
4.9325852394104 -0.38482666015625
4.93261051177979 -0.38482666015625
4.93263626098633 -0.38482666015625
};
\addplot [ultra thick, blue]
table {%
-inf 0
-inf -6.103515625e-05
-inf -6.103515625e-05
0.84509801864624 -0.0008544921875
0.84509801864624 -0.001007080078125
0.903090000152588 -0.00103759765625
0.903090000152588 -0.001129150390625
0.903090000152588 -0.00115966796875
1.51851391792297 -0.007049560546875
1.57978355884552 -0.0123291015625
1.79934048652649 -0.020751953125
1.89209461212158 -0.02508544921875
1.98677170276642 -0.029815673828125
2.18752074241638 -0.04595947265625
2.35410833358765 -0.06707763671875
2.45636606216431 -0.086456298828125
2.49415469169617 -0.09564208984375
2.52762985229492 -0.099517822265625
2.54777479171753 -0.1014404296875
2.62117624282837 -0.115081787109375
2.67117285728455 -0.131622314453125
2.7411515712738 -0.144866943359375
2.76492309570312 -0.1612548828125
2.79518461227417 -0.171875
2.80821108818054 -0.17559814453125
2.82801508903503 -0.178619384765625
2.83758854866028 -0.1802978515625
2.85612440109253 -0.1815185546875
2.86332273483276 -0.18243408203125
2.89209461212158 -0.190948486328125
2.913813829422 -0.1923828125
2.92272543907166 -0.19342041015625
2.93701601028442 -0.19451904296875
2.95182299613953 -0.19683837890625
2.97497200965881 -0.200714111328125
2.98632383346558 -0.205078125
2.99387693405151 -0.205963134765625
3.01953172683716 -0.2103271484375
3.02978944778442 -0.213165283203125
3.03941416740417 -0.214019775390625
3.05842614173889 -0.226409912109375
3.07188200950623 -0.229766845703125
3.07881927490234 -0.2308349609375
3.11058974266052 -0.253509521484375
3.11793375015259 -0.261199951171875
3.13193941116333 -0.2691650390625
3.13956427574158 -0.271759033203125
3.15228843688965 -0.272979736328125
3.16166734695435 -0.275177001953125
3.16642999649048 -0.276092529296875
3.18412327766418 -0.290130615234375
3.19534611701965 -0.295379638671875
3.20085048675537 -0.296966552734375
3.21192097663879 -0.298858642578125
3.22089219093323 -0.300811767578125
3.22505068778992 -0.301544189453125
3.22968173027039 -0.302276611328125
3.23552846908569 -0.302886962890625
3.24054932594299 -0.303802490234375
3.24674463272095 -0.305419921875
3.2550311088562 -0.30828857421875
3.26030993461609 -0.30914306640625
3.26904582977295 -0.310028076171875
3.27230596542358 -0.310882568359375
3.28239560127258 -0.317413330078125
3.28914284706116 -0.318634033203125
3.301029920578 -0.324005126953125
3.30319595336914 -0.3255615234375
3.30749607086182 -0.325958251953125
3.31302309036255 -0.32684326171875
3.31407809257507 -0.3271484375
3.32387065887451 -0.32904052734375
3.32592606544495 -0.329498291015625
3.32633590698242 -0.32977294921875
3.34222531318665 -0.33172607421875
3.34693956375122 -0.332550048828125
3.35102295875549 -0.332763671875
3.35736298561096 -0.333465576171875
3.35945606231689 -0.333709716796875
3.36548805236816 -0.3338623046875
3.36679649353027 -0.334014892578125
3.37548065185547 -0.3358154296875
3.38345623016357 -0.336151123046875
3.38524866104126 -0.33660888671875
3.38649892807007 -0.336944580078125
3.38810110092163 -0.337249755859375
3.40088319778442 -0.339019775390625
3.40174508094788 -0.33941650390625
3.40959501266479 -0.340057373046875
3.41145133972168 -0.340362548828125
3.41380262374878 -0.340850830078125
3.41713953018188 -0.34130859375
3.42586016654968 -0.343780517578125
3.43200659751892 -0.344573974609375
3.43392968177795 -0.344818115234375
3.44059419631958 -0.346160888671875
3.44731307029724 -0.347259521484375
3.45499730110168 -0.34765625
3.45803308486938 -0.3480224609375
3.46805191040039 -0.349212646484375
3.47070455551147 -0.349761962890625
3.47494435310364 -0.350433349609375
3.49052023887634 -0.35797119140625
3.49136161804199 -0.361358642578125
3.49582171440125 -0.361907958984375
3.49665284156799 -0.362091064453125
3.50133323669434 -0.3624267578125
3.50270009040833 -0.362548828125
3.50650501251221 -0.362762451171875
3.50677561759949 -0.36285400390625
3.50812554359436 -0.362945556640625
3.51081299781799 -0.36346435546875
3.51161599159241 -0.36358642578125
3.51917147636414 -0.363677978515625
3.52061462402344 -0.363739013671875
3.52231383323669 -0.364044189453125
3.52296566963196 -0.3641357421875
3.52400636672974 -0.364166259765625
3.52491521835327 -0.3642578125
3.52517437934875 -0.36431884765625
3.52646851539612 -0.3643798828125
3.52775883674622 -0.364471435546875
3.5291736125946 -0.36468505859375
3.52968692779541 -0.364715576171875
3.53326344490051 -0.364990234375
3.53440690040588 -0.36505126953125
3.53605318069458 -0.365478515625
3.53895044326782 -0.3660888671875
3.54145431518555 -0.366241455078125
3.54170393943787 -0.36627197265625
3.54294991493225 -0.3663330078125
3.5507173538208 -0.368438720703125
3.55096173286438 -0.368804931640625
3.55157208442688 -0.36883544921875
3.55315446853638 -0.368988037109375
3.55327606201172 -0.3690185546875
3.55448913574219 -0.369049072265625
3.55473136901855 -0.36907958984375
3.55581974983215 -0.369140625
3.55630254745483 -0.369232177734375
3.55990672111511 -0.36968994140625
3.56002616882324 -0.3697509765625
3.56074333190918 -0.369781494140625
3.56229281425476 -0.369903564453125
3.56419253349304 -0.370025634765625
3.56419253349304 -0.37005615234375
3.56584787368774 -0.37017822265625
3.56667327880859 -0.3702392578125
3.56679105758667 -0.370269775390625
3.56737923622131 -0.37030029296875
3.57100963592529 -0.37060546875
3.57530331611633 -0.3712158203125
3.57564973831177 -0.371307373046875
3.57611083984375 -0.371337890625
3.57691693305969 -0.37139892578125
3.57714700698853 -0.37139892578125
3.57772159576416 -0.371490478515625
3.58001208305359 -0.371795654296875
3.58012628555298 -0.371826171875
3.58308529853821 -0.371917724609375
3.58421802520752 -0.372100830078125
3.5854606628418 -0.372161865234375
3.58579897880554 -0.372222900390625
3.58748650550842 -0.372406005859375
3.5882716178894 -0.3724365234375
3.58849573135376 -0.372467041015625
3.58849573135376 -0.37249755859375
3.59461355209351 -0.373748779296875
3.59483432769775 -0.373870849609375
3.59527564048767 -0.3739013671875
3.5959370136261 -0.37396240234375
3.59637713432312 -0.373992919921875
3.59802412986755 -0.374053955078125
3.59857177734375 -0.37408447265625
3.59889984130859 -0.3741455078125
3.59944629669189 -0.374176025390625
3.60151672363281 -0.374298095703125
3.60173416137695 -0.37432861328125
3.60173416137695 -0.37432861328125
3.60216856002808 -0.3743896484375
3.60216856002808 -0.3743896484375
3.6036856174469 -0.374542236328125
3.60422611236572 -0.374603271484375
3.60487389564514 -0.3746337890625
3.60487389564514 -0.374664306640625
3.60508942604065 -0.374664306640625
3.60552048683167 -0.37469482421875
3.60552048683167 -0.374725341796875
3.60766935348511 -0.374786376953125
3.60820508003235 -0.374847412109375
3.60991430282593 -0.375091552734375
3.61034059524536 -0.375152587890625
3.61034059524536 -0.375152587890625
3.61172342300415 -0.37518310546875
3.61214780807495 -0.375213623046875
3.61236000061035 -0.375213623046875
3.61278390884399 -0.375244140625
3.61299562454224 -0.375274658203125
3.61489725112915 -0.375335693359375
3.61552929878235 -0.3753662109375
3.61573958396912 -0.375396728515625
3.6164755821228 -0.375457763671875
3.6164755821228 -0.375457763671875
3.62138414382935 -0.37615966796875
3.62159156799316 -0.376220703125
3.62211036682129 -0.376251220703125
3.6222140789032 -0.37628173828125
3.62273192405701 -0.3763427734375
3.62335276603699 -0.37640380859375
3.62355947494507 -0.37640380859375
3.62366271018982 -0.376434326171875
3.62500357627869 -0.376556396484375
3.62675094604492 -0.376556396484375
3.62746834754944 -0.376617431640625
3.62757062911987 -0.37664794921875
3.62767314910889 -0.37664794921875
3.62930774688721 -0.376708984375
3.62951159477234 -0.376739501953125
3.63012266159058 -0.376800537109375
3.63012266159058 -0.376800537109375
3.63032627105713 -0.3768310546875
3.6306312084198 -0.3768310546875
3.63518214225769 -0.377960205078125
3.63538312911987 -0.37811279296875
3.63768982887268 -0.378143310546875
3.63768982887268 -0.378143310546875
3.63778972625732 -0.378173828125
3.63778972625732 -0.378173828125
3.63898825645447 -0.378265380859375
3.63898825645447 -0.378265380859375
3.63898825645447 -0.3782958984375
3.64008378982544 -0.3782958984375
3.64008378982544 -0.378326416015625
3.64266228675842 -0.37908935546875
3.64640378952026 -0.379150390625
3.64659976959229 -0.379180908203125
3.6466977596283 -0.37921142578125
3.6466977596283 -0.37921142578125
3.64748072624207 -0.3792724609375
3.64787173271179 -0.3792724609375
3.64787173271179 -0.379302978515625
3.64923739433289 -0.37933349609375
3.64952945709229 -0.379364013671875
3.65350198745728 -0.379547119140625
3.65369486808777 -0.379730224609375
3.65379118919373 -0.3797607421875
3.65388751029968 -0.3797607421875
3.65475392341614 -0.37982177734375
3.65485000610352 -0.37982177734375
3.65485000610352 -0.37982177734375
3.65533065795898 -0.3798828125
3.65782046318054 -0.379913330078125
3.65829753875732 -0.379913330078125
3.65848827362061 -0.37994384765625
3.65848827362061 -0.37994384765625
3.65906000137329 -0.379974365234375
3.65915536880493 -0.379974365234375
3.65953588485718 -0.379974365234375
3.65991616249084 -0.380035400390625
3.65991616249084 -0.380035400390625
3.65991616249084 -0.38006591796875
3.66086554527283 -0.38006591796875
3.66086554527283 -0.38006591796875
3.6618127822876 -0.380157470703125
3.6618127822876 -0.380157470703125
3.6618127822876 -0.380157470703125
3.66200184822083 -0.380157470703125
3.66200184822083 -0.38018798828125
3.66200184822083 -0.38018798828125
3.66200184822083 -0.38018798828125
3.66275787353516 -0.380218505859375
3.66473603248596 -0.38031005859375
3.66473603248596 -0.38031005859375
3.66473603248596 -0.380340576171875
3.66492390632629 -0.380340576171875
3.66576862335205 -0.38037109375
3.66595602035522 -0.38037109375
3.66689229011536 -0.38043212890625
3.66717267036438 -0.38043212890625
3.66717267036438 -0.38043212890625
3.66717267036438 -0.380462646484375
3.6674530506134 -0.380462646484375
3.66801309585571 -0.3804931640625
3.66819953918457 -0.380523681640625
3.66819953918457 -0.380523681640625
3.6727442741394 -0.381011962890625
3.67311310768127 -0.38104248046875
3.67320537567139 -0.38104248046875
3.67338967323303 -0.381072998046875
3.67605304718018 -0.38128662109375
3.67623615264893 -0.38134765625
3.67641925811768 -0.381378173828125
3.67687654495239 -0.381378173828125
3.67705917358398 -0.381378173828125
3.67724180221558 -0.381378173828125
3.67724180221558 -0.38140869140625
3.67733311653137 -0.38140869140625
3.67733311653137 -0.38140869140625
3.67733311653137 -0.38140869140625
3.67733311653137 -0.381439208984375
3.67733311653137 -0.381439208984375
3.67733311653137 -0.3814697265625
3.68024492263794 -0.38153076171875
3.68024492263794 -0.381561279296875
3.680335521698 -0.381561279296875
3.68042612075806 -0.381561279296875
3.68106031417847 -0.381622314453125
3.68115067481995 -0.381622314453125
3.68124127388 -0.381622314453125
3.68133163452148 -0.381683349609375
3.68142223358154 -0.381683349609375
3.68232560157776 -0.3817138671875
3.68241596221924 -0.3817138671875
3.68250608444214 -0.3817138671875
3.68259620666504 -0.381744384765625
3.68259620666504 -0.381744384765625
3.68475556373596 -0.3818359375
3.68484544754028 -0.3818359375
3.68493509292603 -0.381866455078125
3.68502473831177 -0.381866455078125
3.68511438369751 -0.381866455078125
3.68565225601196 -0.381866455078125
3.68574166297913 -0.381866455078125
3.68583130836487 -0.38189697265625
3.68592071533203 -0.38189697265625
3.68592071533203 -0.38189697265625
3.68609976768494 -0.381927490234375
3.6861891746521 -0.381927490234375
3.6861891746521 -0.381927490234375
3.6861891746521 -0.381927490234375
3.6861891746521 -0.381927490234375
3.68654680252075 -0.3819580078125
3.68654680252075 -0.3819580078125
3.68859767913818 -0.3819580078125
3.68859767913818 -0.3819580078125
3.6888644695282 -0.38201904296875
3.6889533996582 -0.38201904296875
3.6889533996582 -0.38201904296875
3.68904232978821 -0.382049560546875
3.68904232978821 -0.382049560546875
3.68913125991821 -0.382049560546875
3.68921995162964 -0.382049560546875
3.68921995162964 -0.382049560546875
3.69010734558105 -0.382080078125
3.69010734558105 -0.382080078125
3.69010734558105 -0.382080078125
3.69010734558105 -0.382080078125
3.69644379615784 -0.382843017578125
3.69679307937622 -0.3829345703125
3.69688034057617 -0.3829345703125
3.69705486297607 -0.3829345703125
3.69722938537598 -0.382965087890625
3.6974036693573 -0.382965087890625
3.6974036693573 -0.382965087890625
3.6974036693573 -0.382965087890625
3.69749093055725 -0.38299560546875
3.69749093055725 -0.38299560546875
3.69749093055725 -0.38299560546875
3.69749093055725 -0.38299560546875
3.69749093055725 -0.38299560546875
3.69749093055725 -0.38299560546875
3.69749093055725 -0.383026123046875
3.69749093055725 -0.383026123046875
3.69749093055725 -0.383026123046875
3.69766521453857 -0.383026123046875
3.69766521453857 -0.383026123046875
3.69766521453857 -0.383026123046875
3.69766521453857 -0.383026123046875
3.69940400123596 -0.38311767578125
3.69957756996155 -0.38311767578125
3.69966435432434 -0.38311767578125
3.69966435432434 -0.383148193359375
3.69966435432434 -0.383148193359375
3.69966435432434 -0.383148193359375
3.69975113868713 -0.3831787109375
3.69983768463135 -0.3831787109375
3.69983768463135 -0.3831787109375
3.69983768463135 -0.3831787109375
3.69983768463135 -0.3831787109375
3.69983768463135 -0.3831787109375
3.70009779930115 -0.3831787109375
3.70009779930115 -0.383209228515625
3.70018434524536 -0.383209228515625
3.70027089118958 -0.383209228515625
3.70035743713379 -0.383209228515625
3.70035743713379 -0.383209228515625
3.70035743713379 -0.383209228515625
3.70035743713379 -0.383209228515625
3.70337748527527 -0.383544921875
3.70372104644775 -0.383575439453125
3.70372104644775 -0.383575439453125
3.70380711555481 -0.383575439453125
3.70389294624329 -0.383575439453125
3.70697379112244 -0.38360595703125
3.70705890655518 -0.38360595703125
3.70714426040649 -0.38360595703125
3.70714426040649 -0.38360595703125
3.70714426040649 -0.38360595703125
3.70714426040649 -0.38360595703125
3.70714426040649 -0.38360595703125
3.70722937583923 -0.38360595703125
3.70731472969055 -0.38360595703125
3.70731472969055 -0.38360595703125
3.70731472969055 -0.383636474609375
3.70731472969055 -0.383636474609375
3.70731472969055 -0.383636474609375
3.70731472969055 -0.383636474609375
3.70731472969055 -0.383636474609375
3.70731472969055 -0.383636474609375
3.70731472969055 -0.3836669921875
3.70731472969055 -0.3836669921875
3.70825099945068 -0.3836669921875
3.70833587646484 -0.3836669921875
3.70833587646484 -0.3836669921875
3.70833587646484 -0.3836669921875
3.70833587646484 -0.3836669921875
3.70833587646484 -0.3836669921875
3.70833587646484 -0.3836669921875
3.71307039260864 -0.383758544921875
3.71323847770691 -0.383758544921875
3.71323847770691 -0.383758544921875
3.71323847770691 -0.383758544921875
3.71323847770691 -0.3837890625
3.71323847770691 -0.3837890625
3.71323847770691 -0.3837890625
3.71323847770691 -0.3837890625
3.71323847770691 -0.3837890625
3.71323847770691 -0.3837890625
3.71323847770691 -0.3837890625
3.71323847770691 -0.3837890625
3.71332240104675 -0.383819580078125
3.71340656280518 -0.383819580078125
3.71374249458313 -0.383819580078125
3.71382641792297 -0.383819580078125
3.71382641792297 -0.383819580078125
3.71382641792297 -0.383819580078125
3.71382641792297 -0.383819580078125
3.71382641792297 -0.38385009765625
3.71382641792297 -0.38385009765625
3.71458125114441 -0.38385009765625
3.71458125114441 -0.38385009765625
3.71458125114441 -0.38385009765625
3.71458125114441 -0.38385009765625
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{FO2}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.473762512207031, ymax=0.0225601196289062,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c11)}
]
\addplot [ultra thick, brown, dashed]
table {%
0.84509801864624 0
1.69019603729248 -0.000213623046875
2.20139718055725 -0.0003662109375
2.41497325897217 -0.0006103515625
2.52762985229492 -0.0010528564453125
2.5365583896637 -0.0012054443359375
2.67486119270325 -0.002349853515625
2.68124127388 -0.0025634765625
2.77158737182617 -0.003082275390625
2.7972674369812 -0.0035400390625
2.87157297134399 -0.0044403076171875
2.92272543907166 -0.004669189453125
2.97909283638 -0.0049591064453125
2.99869513511658 -0.0051116943359375
3.05115246772766 -0.006011962890625
3.08026552200317 -0.0062408447265625
3.12155985832214 -0.0066680908203125
3.15654921531677 -0.0093841552734375
3.19368100166321 -0.0099945068359375
3.25212454795837 -0.010650634765625
3.28488159179688 -0.012786865234375
3.301029920578 -0.014068603515625
3.33304405212402 -0.0152587890625
3.3479151725769 -0.016021728515625
3.42488169670105 -0.029754638671875
3.46463847160339 -0.03515625
3.54802060127258 -0.04241943359375
3.5718252658844 -0.0450897216796875
3.62951159477234 -0.0503997802734375
3.66996741294861 -0.0600128173828125
3.73822546005249 -0.0720977783203125
3.82026720046997 -0.10003662109375
3.86540007591248 -0.133865356445312
3.88462543487549 -0.153839111328125
3.91307163238525 -0.168533325195312
3.94482803344727 -0.176055908203125
3.96482515335083 -0.182327270507812
3.98632383346558 -0.187347412109375
4.022057056427 -0.191650390625
4.03921556472778 -0.195159912109375
4.05804634094238 -0.197708129882812
4.07787656784058 -0.199920654296875
4.09366703033447 -0.201980590820312
4.11089277267456 -0.207733154296875
4.12739658355713 -0.2100830078125
4.14182567596436 -0.214431762695312
4.1592059135437 -0.219558715820312
4.17935085296631 -0.224822998046875
4.19292974472046 -0.2269287109375
4.20833396911621 -0.231536865234375
4.22078800201416 -0.235626220703125
4.23527574539185 -0.239654541015625
4.24644947052002 -0.24334716796875
4.25947427749634 -0.245635986328125
4.27756357192993 -0.252395629882812
4.29212331771851 -0.256484985351562
4.31576061248779 -0.269149780273438
4.32259130477905 -0.272323608398438
4.3384165763855 -0.2769775390625
4.3458833694458 -0.278274536132812
4.36455106735229 -0.287979125976562
4.3758282661438 -0.29046630859375
4.39267921447754 -0.30181884765625
4.40671062469482 -0.304885864257812
4.41509008407593 -0.305938720703125
4.42696666717529 -0.308609008789062
4.43659210205078 -0.309783935546875
4.45044946670532 -0.314956665039062
4.46307134628296 -0.321670532226562
4.47274160385132 -0.327926635742188
4.47796010971069 -0.331222534179688
4.48855066299438 -0.338241577148438
4.49386215209961 -0.341949462890625
4.50404930114746 -0.350341796875
4.51137542724609 -0.3582763671875
4.51523780822754 -0.3607177734375
4.52512264251709 -0.363845825195312
4.53876209259033 -0.370025634765625
4.54592514038086 -0.371673583984375
4.55897235870361 -0.374710083007812
4.56200742721558 -0.375808715820312
4.56663799285889 -0.377182006835938
4.57908582687378 -0.379669189453125
4.58880949020386 -0.381134033203125
4.60053730010986 -0.384994506835938
4.60510015487671 -0.385589599609375
4.60834407806396 -0.386276245117188
4.61327075958252 -0.387542724609375
4.615234375 -0.3880615234375
4.61730432510376 -0.38848876953125
4.62140464782715 -0.389404296875
4.6249623298645 -0.390884399414062
4.62839937210083 -0.391632080078125
4.63124084472656 -0.393310546875
4.63346862792969 -0.393951416015625
4.6359658241272 -0.394378662109375
4.64021301269531 -0.397964477539062
4.64288949966431 -0.398681640625
4.64522552490234 -0.39923095703125
4.64688396453857 -0.39971923828125
4.64921808242798 -0.400222778320312
4.65157842636108 -0.400924682617188
4.65362739562988 -0.40130615234375
4.65877437591553 -0.406890869140625
4.65997314453125 -0.408599853515625
4.6615948677063 -0.409027099609375
4.66455745697021 -0.409957885742188
4.66680812835693 -0.410476684570312
4.67001390457153 -0.411544799804688
4.67234706878662 -0.4122314453125
4.67399740219116 -0.412521362304688
4.67549419403076 -0.412887573242188
4.67724180221558 -0.413177490234375
4.68188333511353 -0.415924072265625
4.68320035934448 -0.41650390625
4.68427991867065 -0.41668701171875
4.68750238418579 -0.417678833007812
4.688063621521 -0.417831420898438
4.6894154548645 -0.418106079101562
4.69117879867554 -0.418365478515625
4.69273233413696 -0.4188232421875
4.69406986236572 -0.419021606445312
4.69546413421631 -0.419219970703125
4.69668817520142 -0.41937255859375
4.69906568527222 -0.41973876953125
4.70001983642578 -0.420120239257812
4.70209455490112 -0.420242309570312
4.70469093322754 -0.421844482421875
4.70539331436157 -0.422073364257812
4.7067346572876 -0.422348022460938
4.70772361755371 -0.422439575195312
4.70931243896484 -0.422622680664062
4.71027803421021 -0.422775268554688
4.71207714080811 -0.42327880859375
4.71349048614502 -0.423507690429688
4.71519231796265 -0.423919677734375
4.71578598022461 -0.424026489257812
4.7164626121521 -0.424102783203125
4.71907424926758 -0.425857543945312
4.72036600112915 -0.426055908203125
4.7219672203064 -0.426254272460938
4.72358703613281 -0.426422119140625
4.72443962097168 -0.426544189453125
4.72530698776245 -0.4266357421875
4.72759819030762 -0.4271240234375
4.72825622558594 -0.42718505859375
4.73061275482178 -0.42926025390625
4.73156452178955 -0.42950439453125
4.73316526412964 -0.429580688476562
4.73434352874756 -0.429656982421875
4.73552703857422 -0.429779052734375
4.737144947052 -0.429855346679688
4.73731184005737 -0.429931640625
4.7396674156189 -0.430511474609375
4.7422456741333 -0.430755615234375
4.74296092987061 -0.430801391601562
4.74349403381348 -0.43084716796875
4.74498891830444 -0.431182861328125
4.74573040008545 -0.431228637695312
4.74825763702393 -0.43206787109375
4.74925708770752 -0.432296752929688
4.74964380264282 -0.432327270507812
4.7537055015564 -0.433792114257812
4.75520372390747 -0.433914184570312
4.75555467605591 -0.433944702148438
4.75655269622803 -0.433975219726562
4.75802564620972 -0.434097290039062
4.75982666015625 -0.43414306640625
4.76041507720947 -0.434158325195312
4.7613263130188 -0.434295654296875
4.76163482666016 -0.434341430664062
4.7643256187439 -0.434814453125
4.76447486877441 -0.434844970703125
4.76555681228638 -0.434967041015625
4.76914834976196 -0.435867309570312
4.77001953125 -0.436050415039062
4.77050590515137 -0.436080932617188
4.77106523513794 -0.436187744140625
4.77200603485107 -0.43621826171875
4.77323055267334 -0.436431884765625
4.77439308166504 -0.436553955078125
4.77508592605591 -0.43658447265625
4.77556657791138 -0.43670654296875
4.77651977539062 -0.436798095703125
4.77730369567871 -0.43682861328125
4.77767324447632 -0.436859130859375
4.77960395812988 -0.436981201171875
4.78032445907593 -0.43707275390625
4.78059816360474 -0.437103271484375
4.78266620635986 -0.4375
4.78365325927734 -0.437545776367188
4.78398942947388 -0.437576293945312
4.78515195846558 -0.437652587890625
4.78554344177246 -0.43768310546875
4.78622579574585 -0.437728881835938
4.78649568557739 -0.437759399414062
4.78709173202515 -0.437774658203125
4.78827428817749 -0.43792724609375
4.7885856628418 -0.437957763671875
4.79008817672729 -0.438125610351562
4.79157829284668 -0.43829345703125
4.79228639602661 -0.438339233398438
4.79245471954346 -0.4383544921875
4.79794597625732 -0.440628051757812
4.79893350601196 -0.4412841796875
4.8005313873291 -0.441314697265625
4.80097818374634 -0.441329956054688
4.80112218856812 -0.44134521484375
4.80189752578735 -0.441360473632812
4.80385303497314 -0.441802978515625
4.80550098419189 -0.442062377929688
4.80588817596436 -0.44207763671875
4.80658674240112 -0.44219970703125
4.80734539031982 -0.442245483398438
4.80804204940796 -0.4422607421875
4.80850124359131 -0.442276000976562
4.80906772613525 -0.442291259765625
4.80955982208252 -0.442306518554688
4.81074333190918 -0.442398071289062
4.81150817871094 -0.442413330078125
4.81158828735352 -0.442428588867188
4.81253910064697 -0.442489624023438
4.81400775909424 -0.442489624023438
4.81407451629639 -0.4425048828125
4.81442737579346 -0.442520141601562
4.81488656997681 -0.442550659179688
4.81499290466309 -0.44256591796875
4.81657934188843 -0.442703247070312
4.81702947616577 -0.442733764648438
4.81727457046509 -0.442733764648438
4.8173999786377 -0.4427490234375
4.81839752197266 -0.442794799804688
4.81877994537354 -0.442825317382812
4.81907653808594 -0.442825317382812
4.8199782371521 -0.442855834960938
4.8200831413269 -0.44287109375
4.82112693786621 -0.442886352539062
4.82157230377197 -0.442916870117188
4.82203722000122 -0.44293212890625
4.82243633270264 -0.442962646484375
4.82321310043335 -0.442962646484375
4.82358503341675 -0.4429931640625
4.8244252204895 -0.443008422851562
4.82488059997559 -0.443038940429688
4.82567262649536 -0.443069458007812
4.82616567611694 -0.443084716796875
4.82765340805054 -0.4432373046875
4.8282732963562 -0.4432373046875
4.82962512969971 -0.443344116210938
4.82982444763184 -0.443359375
4.83001089096069 -0.443374633789062
4.83029365539551 -0.443374633789062
4.83115911483765 -0.443389892578125
4.83184432983398 -0.443450927734375
4.83200407028198 -0.443466186523438
4.83235549926758 -0.443466186523438
4.83257913589478 -0.4434814453125
4.83308982849121 -0.4434814453125
4.83328104019165 -0.443496704101562
4.83410263061523 -0.443527221679688
4.83466863632202 -0.44354248046875
4.83578586578369 -0.443588256835938
4.83596324920654 -0.443603515625
4.83658981323242 -0.443618774414062
4.83733606338501 -0.443649291992188
4.83737373352051 -0.44366455078125
4.83892440795898 -0.443817138671875
4.83930826187134 -0.443832397460938
4.84022521972656 -0.44384765625
4.84034442901611 -0.443862915039062
4.8408522605896 -0.443862915039062
4.8413405418396 -0.443878173828125
4.84185981750488 -0.44390869140625
4.84235954284668 -0.443923950195312
4.84237813949585 -0.443923950195312
4.84366893768311 -0.444107055664062
4.84502983093262 -0.444122314453125
4.84531497955322 -0.444137573242188
4.84562492370605 -0.444137573242188
4.84636783599854 -0.44415283203125
4.84816455841064 -0.444625854492188
4.84957885742188 -0.44476318359375
4.85025405883789 -0.444793701171875
4.85035800933838 -0.444793701171875
4.85158252716064 -0.444869995117188
4.85182666778564 -0.44488525390625
4.85263872146606 -0.444900512695312
4.85300445556641 -0.444900512695312
4.8533148765564 -0.444915771484375
4.85414218902588 -0.444915771484375
4.85554361343384 -0.445098876953125
4.85588836669922 -0.445114135742188
4.85733270645142 -0.44525146484375
4.85773658752441 -0.445266723632812
4.85825443267822 -0.445281982421875
4.85867547988892 -0.445281982421875
4.85966634750366 -0.4453125
4.86115789413452 -0.445388793945312
4.86169576644897 -0.445388793945312
4.86272764205933 -0.445404052734375
4.86365604400635 -0.445449829101562
4.86416101455688 -0.445449829101562
4.86517524719238 -0.445556640625
4.86576128005981 -0.445571899414062
4.86645889282227 -0.445587158203125
4.86713743209839 -0.445632934570312
4.86810350418091 -0.445648193359375
4.86854457855225 -0.445663452148438
4.8691554069519 -0.4456787109375
4.86948394775391 -0.445693969726562
4.8701343536377 -0.445709228515625
4.87075471878052 -0.445724487304688
4.87169551849365 -0.445755004882812
4.87189388275146 -0.445770263671875
4.87226104736328 -0.445785522460938
4.87346029281616 -0.445846557617188
4.87410497665405 -0.445877075195312
4.87452220916748 -0.445877075195312
4.87493371963501 -0.445892333984375
4.87552404403687 -0.4459228515625
4.87609100341797 -0.445938110351562
4.87667942047119 -0.445938110351562
4.87745761871338 -0.44598388671875
4.87882614135742 -0.446121215820312
4.87950325012207 -0.446151733398438
4.88008165359497 -0.446151733398438
4.88099050521851 -0.446304321289062
4.88243913650513 -0.4464111328125
4.88336038589478 -0.446456909179688
4.88395643234253 -0.446487426757812
4.88425731658936 -0.446502685546875
4.88511800765991 -0.446533203125
4.88567781448364 -0.446548461914062
4.88637208938599 -0.446578979492188
4.88654136657715 -0.446578979492188
4.88802766799927 -0.446884155273438
4.88848829269409 -0.446975708007812
4.88866806030273 -0.446990966796875
4.88978338241577 -0.447036743164062
4.89042091369629 -0.447052001953125
4.89099645614624 -0.44708251953125
4.89188289642334 -0.447158813476562
4.89229488372803 -0.447158813476562
4.89285659790039 -0.44720458984375
4.89331769943237 -0.447219848632812
4.89357328414917 -0.447219848632812
4.89397811889648 -0.447235107421875
4.89443254470825 -0.447250366210938
4.89469242095947 -0.447250366210938
4.89508533477783 -0.447250366210938
4.89577579498291 -0.447265625
4.89650440216064 -0.447280883789062
4.89703845977783 -0.447296142578125
4.89733028411865 -0.447311401367188
4.89755010604858 -0.44732666015625
4.89791297912598 -0.44732666015625
4.8980884552002 -0.447341918945312
4.89949750900269 -0.44744873046875
4.89967823028564 -0.447479248046875
4.90014839172363 -0.447494506835938
4.90043258666992 -0.447509765625
4.90115308761597 -0.447555541992188
4.90139293670654 -0.447555541992188
4.90174722671509 -0.44757080078125
4.90267705917358 -0.447662353515625
4.90312814712524 -0.447708129882812
4.90325260162354 -0.447708129882812
4.90485095977783 -0.447769165039062
4.90508842468262 -0.44781494140625
4.90547752380371 -0.44781494140625
4.90560150146484 -0.447830200195312
4.90607643127441 -0.447845458984375
4.90649127960205 -0.447860717773438
4.90673875808716 -0.447860717773438
4.90704584121704 -0.4478759765625
4.90765857696533 -0.4478759765625
4.90790033340454 -0.447891235351562
4.90794849395752 -0.447891235351562
4.90878534317017 -0.447921752929688
4.90924024581909 -0.447921752929688
4.9095344543457 -0.44793701171875
4.90996217727661 -0.447952270507812
4.91007471084595 -0.447952270507812
4.91055488586426 -0.447952270507812
4.91062450408936 -0.447967529296875
4.91113090515137 -0.447982788085938
4.91214227676392 -0.448043823242188
4.91236019134521 -0.448074340820312
4.91288614273071 -0.448089599609375
4.91356992721558 -0.448089599609375
4.91378736495972 -0.448104858398438
4.91393041610718 -0.448104858398438
4.91571092605591 -0.44830322265625
4.91624355316162 -0.448318481445312
4.91665935516357 -0.448333740234375
4.91749477386475 -0.448333740234375
4.91798305511475 -0.448348999023438
4.91823482513428 -0.448348999023438
4.91905212402344 -0.448455810546875
4.91967964172363 -0.448471069335938
4.92021226882935 -0.448471069335938
4.92078065872192 -0.448532104492188
4.92140531539917 -0.448532104492188
4.92157220840454 -0.448532104492188
4.92240905761719 -0.448562622070312
4.92247104644775 -0.448577880859375
4.92294311523438 -0.448577880859375
4.92321300506592 -0.448593139648438
4.92371559143066 -0.448593139648438
4.9241189956665 -0.4486083984375
4.92483711242676 -0.4486083984375
4.92532253265381 -0.4486083984375
4.92565774917603 -0.448623657226562
4.92603874206543 -0.448623657226562
4.92647123336792 -0.448638916015625
4.92669725418091 -0.448638916015625
4.92714977264404 -0.448654174804688
4.92773962020874 -0.448654174804688
4.92780637741089 -0.448654174804688
4.92785263061523 -0.44866943359375
4.9280834197998 -0.44866943359375
4.92856979370117 -0.44866943359375
4.92883110046387 -0.448684692382812
4.92949533462524 -0.448684692382812
4.93002653121948 -0.448699951171875
4.93037843704224 -0.448699951171875
4.93051099777222 -0.448699951171875
4.93107128143311 -0.448715209960938
4.93161058425903 -0.44873046875
4.93181896209717 -0.44873046875
4.93226051330566 -0.448745727539062
4.93233156204224 -0.448745727539062
4.93310260772705 -0.448760986328125
4.93331003189087 -0.448776245117188
4.9340386390686 -0.448776245117188
4.93410921096802 -0.44879150390625
4.93460464477539 -0.44879150390625
4.93495273590088 -0.44879150390625
4.93521499633789 -0.44879150390625
4.93560314178467 -0.448806762695312
4.93593549728394 -0.448806762695312
4.93672466278076 -0.4488525390625
4.93684530258179 -0.4488525390625
4.93733215332031 -0.4488525390625
4.93753814697266 -0.448867797851562
4.93800926208496 -0.448867797851562
4.93823957443237 -0.448867797851562
4.9387149810791 -0.448883056640625
4.93877506256104 -0.448883056640625
4.93910455703735 -0.448883056640625
4.93929433822632 -0.448898315429688
4.93987369537354 -0.448898315429688
4.94007778167725 -0.448898315429688
4.94013786315918 -0.44891357421875
4.94064092636108 -0.44891357421875
4.94092988967896 -0.448928833007812
4.9413275718689 -0.448928833007812
4.941650390625 -0.448928833007812
4.94176959991455 -0.448944091796875
4.94223642349243 -0.448944091796875
4.94304895401001 -0.44903564453125
4.94332647323608 -0.44903564453125
4.94444799423218 -0.449142456054688
4.94472932815552 -0.44921875
4.94512367248535 -0.44921875
4.94551277160645 -0.44921875
4.94581317901611 -0.449234008789062
4.94601011276245 -0.449234008789062
4.94638824462891 -0.449234008789062
4.94671726226807 -0.449234008789062
4.94697761535645 -0.449249267578125
4.94812440872192 -0.449264526367188
4.94822692871094 -0.449264526367188
4.94887733459473 -0.44927978515625
4.9494047164917 -0.44927978515625
4.95009231567383 -0.449295043945312
4.95045757293701 -0.449295043945312
4.9507007598877 -0.449295043945312
4.95106077194214 -0.449310302734375
4.95157527923584 -0.449310302734375
4.95183277130127 -0.449310302734375
4.95199775695801 -0.449325561523438
4.95252132415771 -0.449325561523438
4.95259380340576 -0.449325561523438
4.95327138900757 -0.4493408203125
4.95371627807617 -0.4493408203125
4.95416069030762 -0.4493408203125
4.95434379577637 -0.4493408203125
4.95524024963379 -0.449508666992188
4.95566368103027 -0.449630737304688
4.95586585998535 -0.449630737304688
4.95648527145386 -0.44964599609375
4.95813369750977 -0.44964599609375
4.95825815200806 -0.44964599609375
4.95843029022217 -0.449661254882812
4.95890283584595 -0.449691772460938
4.95916080474854 -0.44970703125
4.95959949493408 -0.449737548828125
4.95979022979736 -0.449737548828125
4.9601092338562 -0.449752807617188
4.96033763885498 -0.449752807617188
4.96048974990845 -0.44976806640625
4.96067523956299 -0.44976806640625
4.96131658554077 -0.44976806640625
4.96159648895264 -0.44976806640625
4.961838722229 -0.449783325195312
4.96208047866821 -0.449783325195312
4.96232175827026 -0.449798583984375
4.9627480506897 -0.449798583984375
4.96300840377808 -0.449798583984375
4.96375465393066 -0.449859619140625
4.96430206298828 -0.449935913085938
4.96490526199341 -0.449966430664062
4.96511220932007 -0.449981689453125
4.9654746055603 -0.449981689453125
4.96565341949463 -0.449981689453125
4.96586465835571 -0.449981689453125
4.9662823677063 -0.45001220703125
4.96651697158813 -0.45001220703125
4.96686887741089 -0.45001220703125
4.96719694137573 -0.45001220703125
4.96739339828491 -0.45001220703125
4.96802997589111 -0.450057983398438
4.96826791763306 -0.4500732421875
4.9686279296875 -0.450088500976562
4.96904754638672 -0.450088500976562
4.96915006637573 -0.450103759765625
4.96956014633179 -0.450103759765625
4.96973752975464 -0.450103759765625
4.97092771530151 -0.45013427734375
4.97118759155273 -0.450149536132812
4.97130393981934 -0.450149536132812
4.97147512435913 -0.450149536132812
4.9718599319458 -0.450164794921875
4.97249460220337 -0.450164794921875
4.97267007827759 -0.450164794921875
4.97277212142944 -0.450164794921875
4.97332668304443 -0.4501953125
4.97348356246948 -0.4501953125
4.97361278533936 -0.4501953125
4.97560167312622 -0.450393676757812
4.97595071792603 -0.450469970703125
4.97605657577515 -0.450469970703125
4.97649192810059 -0.450469970703125
4.97685432434082 -0.450469970703125
4.97697782516479 -0.450485229492188
4.97743558883667 -0.45050048828125
4.97753143310547 -0.45050048828125
4.97782421112061 -0.450515747070312
4.97793865203857 -0.450531005859375
4.97814846038818 -0.450531005859375
4.97842693328857 -0.450531005859375
4.97853183746338 -0.450531005859375
4.97857284545898 -0.450546264648438
4.97917032241821 -0.450546264648438
4.97950267791748 -0.4505615234375
4.97958469390869 -0.4505615234375
4.97968053817749 -0.4505615234375
4.97996711730957 -0.4505615234375
4.9800853729248 -0.450576782226562
4.98035335540771 -0.450576782226562
4.98042154312134 -0.450576782226562
4.98046255111694 -0.450576782226562
4.98066234588623 -0.450576782226562
4.98101186752319 -0.450576782226562
4.98142004013062 -0.450592041015625
4.98242044448853 -0.450592041015625
4.98251533508301 -0.450592041015625
4.9835991859436 -0.450592041015625
4.98389673233032 -0.450607299804688
4.98392391204834 -0.450607299804688
4.98423910140991 -0.450637817382812
4.98444175720215 -0.450637817382812
4.9846625328064 -0.450637817382812
4.98467588424683 -0.450637817382812
4.98501777648926 -0.450653076171875
4.98507165908813 -0.450653076171875
4.98522424697876 -0.450653076171875
4.98551607131958 -0.450668334960938
4.98605012893677 -0.450698852539062
4.98625183105469 -0.450714111328125
4.98634624481201 -0.450714111328125
4.98640012741089 -0.450714111328125
4.98664617538452 -0.450729370117188
4.98666000366211 -0.450729370117188
4.98728656768799 -0.450729370117188
4.98739385604858 -0.450729370117188
4.9874963760376 -0.450729370117188
4.98764848709106 -0.45074462890625
4.98766183853149 -0.45074462890625
4.98789405822754 -0.45074462890625
4.98796987533569 -0.45074462890625
4.98840284347534 -0.450759887695312
4.98859453201294 -0.450759887695312
4.98889303207397 -0.450759887695312
4.98906230926514 -0.450775146484375
4.98918724060059 -0.450775146484375
4.98972129821777 -0.450775146484375
4.98981904983521 -0.450790405273438
4.9898943901062 -0.450790405273438
4.99001884460449 -0.450790405273438
4.99038314819336 -0.450820922851562
4.99066734313965 -0.450820922851562
4.99103116989136 -0.450836181640625
4.99107980728149 -0.450836181640625
4.99111080169678 -0.450836181640625
4.99123954772949 -0.450836181640625
4.9913592338562 -0.450836181640625
4.99141216278076 -0.450836181640625
4.99174404144287 -0.450836181640625
4.99195671081543 -0.450851440429688
4.99197006225586 -0.450851440429688
4.99226188659668 -0.450851440429688
4.99227046966553 -0.450851440429688
4.99284934997559 -0.450942993164062
4.99320697784424 -0.450958251953125
4.99322032928467 -0.450958251953125
4.99333047866821 -0.450958251953125
4.99350690841675 -0.450958251953125
4.99422025680542 -0.451019287109375
4.99424695968628 -0.451019287109375
4.99475240707397 -0.451019287109375
4.9947657585144 -0.451019287109375
4.99500322341919 -0.451019287109375
4.9953761100769 -0.451019287109375
4.99539375305176 -0.451034545898438
4.99540710449219 -0.451034545898438
4.99553871154785 -0.451034545898438
4.99603414535522 -0.451034545898438
4.99628829956055 -0.451034545898438
4.99637603759766 -0.451034545898438
4.99650287628174 -0.451034545898438
4.99666500091553 -0.451034545898438
4.99670886993408 -0.4510498046875
4.99716806411743 -0.4510498046875
4.99731206893921 -0.4510498046875
4.99732542037964 -0.4510498046875
4.99788856506348 -0.451080322265625
4.99814605712891 -0.451095581054688
4.99859046936035 -0.451095581054688
4.99875164031982 -0.45111083984375
4.99884748458862 -0.45111083984375
4.9988694190979 -0.45111083984375
4.99900007247925 -0.45111083984375
4.99916553497314 -0.45111083984375
4.99918699264526 -0.45111083984375
4.9994740486145 -0.451126098632812
4.9995002746582 -0.451126098632812
4.99983501434326 -0.451126098632812
5.00018215179443 -0.451126098632812
5.00059032440186 -0.451126098632812
5.00068998336792 -0.451126098632812
5.00107574462891 -0.451126098632812
5.00118398666382 -0.451126098632812
5.00118398666382 -0.451126098632812
5.00143527984619 -0.451141357421875
5.00145244598389 -0.451141357421875
5.00148725509644 -0.451156616210938
5.00150442123413 -0.451156616210938
5.00158214569092 -0.451156616210938
5.00203227996826 -0.451156616210938
5.00236463546753 -0.451171875
5.00238227844238 -0.451171875
5.00311994552612 -0.451171875
5.00387811660767 -0.451171875
5.00396871566772 -0.451171875
5.00429105758667 -0.451187133789062
5.00433015823364 -0.451187133789062
5.00464391708374 -0.451187133789062
};
\addplot [ultra thick, blue]
table {%
0 0
0.477121233940125 -0.0001983642578125
0.60206001996994 -0.0003509521484375
1.04139268398285 -0.0015869140625
1.20412003993988 -0.00286865234375
1.30103003978729 -0.003265380859375
1.32221925258636 -0.003509521484375
1.38021123409271 -0.0040283203125
1.46239805221558 -0.0044403076171875
1.49136173725128 -0.004730224609375
1.55630254745483 -0.005035400390625
1.57978355884552 -0.005218505859375
1.6334685087204 -0.0055999755859375
1.66275787353516 -0.0057830810546875
1.74036264419556 -0.00653076171875
1.74818801879883 -0.0066680908203125
1.81954395771027 -0.007781982421875
1.87506127357483 -0.0083770751953125
1.89762711524963 -0.0088958740234375
1.92941892147064 -0.009246826171875
1.9395192861557 -0.0095367431640625
1.96378779411316 -0.0099945068359375
1.99122607707977 -0.0103607177734375
2.0827853679657 -0.0169830322265625
2.21218752861023 -0.0346832275390625
2.24797320365906 -0.0452880859375
2.28780174255371 -0.0483551025390625
2.30963015556335 -0.050201416015625
2.34635305404663 -0.053741455078125
2.36172771453857 -0.0565185546875
2.42324590682983 -0.06414794921875
2.46686768531799 -0.0747528076171875
2.5078558921814 -0.0858001708984375
2.62117624282837 -0.1160888671875
2.6580114364624 -0.149444580078125
2.72509455680847 -0.176986694335938
2.74818801879883 -0.186843872070312
2.7641761302948 -0.189529418945312
2.7972674369812 -0.19439697265625
2.80482077598572 -0.195541381835938
2.83250904083252 -0.204208374023438
2.8709888458252 -0.215850830078125
2.88817954063416 -0.223373413085938
2.90309000015259 -0.225936889648438
2.91855454444885 -0.228286743164062
2.92272543907166 -0.230072021484375
2.94250416755676 -0.23291015625
2.97863698005676 -0.244415283203125
2.99607372283936 -0.2552490234375
3.00902581214905 -0.258026123046875
3.01661562919617 -0.260848999023438
3.03582978248596 -0.265426635742188
3.04766416549683 -0.267730712890625
3.07371830940247 -0.276809692382812
3.08350253105164 -0.278701782226562
3.1065309047699 -0.289306640625
3.1115984916687 -0.290756225585938
3.1325798034668 -0.295867919921875
3.13861846923828 -0.297225952148438
3.17172646522522 -0.310714721679688
3.1838390827179 -0.314620971679688
3.19005131721497 -0.316009521484375
3.21325206756592 -0.320419311523438
3.22010803222656 -0.324203491210938
3.23324990272522 -0.327133178710938
3.25478959083557 -0.347152709960938
3.26717185974121 -0.353775024414062
3.27300119400024 -0.35565185546875
3.28352737426758 -0.3594970703125
3.2920343875885 -0.36370849609375
3.29972505569458 -0.366134643554688
3.31638979911804 -0.379806518554688
3.32242608070374 -0.381698608398438
3.3289909362793 -0.3834228515625
3.33765888214111 -0.383941650390625
3.34084057807922 -0.384414672851562
3.35218262672424 -0.394699096679688
3.35774421691895 -0.397048950195312
3.36642289161682 -0.398193359375
3.37125253677368 -0.399917602539062
3.37511467933655 -0.400680541992188
3.37984919548035 -0.401473999023438
3.38165640830994 -0.4019775390625
3.38863396644592 -0.403228759765625
3.39058184623718 -0.404083251953125
3.40517544746399 -0.40985107421875
3.40671038627625 -0.412200927734375
3.41060853004456 -0.412857055664062
3.41363501548767 -0.413436889648438
3.41763782501221 -0.413833618164062
3.42061567306519 -0.414352416992188
3.42308187484741 -0.414749145507812
3.42748618125916 -0.415176391601562
3.43071985244751 -0.415679931640625
3.43152451515198 -0.415969848632812
3.43600344657898 -0.416519165039062
3.43996381759644 -0.416763305664062
3.44279313087463 -0.41705322265625
3.44404482841492 -0.417221069335938
3.44575977325439 -0.417465209960938
3.4462263584137 -0.417648315429688
3.4504029750824 -0.41802978515625
3.45193982124329 -0.4183349609375
3.45621418952942 -0.418899536132812
3.45969390869141 -0.41912841796875
3.4610481262207 -0.4193115234375
3.4629967212677 -0.419830322265625
3.4683473110199 -0.420181274414062
3.46893787384033 -0.420425415039062
3.47011637687683 -0.420623779296875
3.47114491462708 -0.420761108398438
3.47436189651489 -0.421051025390625
3.47523522377014 -0.421218872070312
3.48043823242188 -0.421783447265625
3.48129940032959 -0.421890258789062
3.48244476318359 -0.422256469726562
3.48586320877075 -0.422500610351562
3.48685526847839 -0.422653198242188
3.48770380020142 -0.422775268554688
3.49037981033325 -0.423202514648438
3.4962375164032 -0.423782348632812
3.49734449386597 -0.423980712890625
3.49872398376465 -0.424118041992188
3.50009918212891 -0.424331665039062
3.50160694122314 -0.424468994140625
3.50256371498108 -0.424713134765625
3.50419902801514 -0.424850463867188
3.50677561759949 -0.425018310546875
3.5100085735321 -0.425369262695312
3.51268434524536 -0.425674438476562
3.51375007629395 -0.425857543945312
3.51521134376526 -0.425979614257812
3.520352602005 -0.426956176757812
3.52153038978577 -0.427047729492188
3.52361631393433 -0.427581787109375
3.52413630485535 -0.42767333984375
3.52891683578491 -0.4278564453125
3.52930212020874 -0.427902221679688
3.537189245224 -0.430084228515625
3.5381965637207 -0.430252075195312
3.53844809532166 -0.430282592773438
3.54170393943787 -0.430404663085938
3.54195356369019 -0.430496215820312
3.54245185852051 -0.430572509765625
3.54319858551025 -0.430633544921875
3.54961633682251 -0.432907104492188
3.55035066604614 -0.433197021484375
3.55461025238037 -0.433273315429688
3.55521535873413 -0.433349609375
3.55606126785278 -0.43341064453125
3.55630254745483 -0.4334716796875
3.5576274394989 -0.43353271484375
3.5591881275177 -0.433609008789062
3.56133985519409 -0.433670043945312
3.56300616264343 -0.433792114257812
3.5635998249054 -0.433868408203125
3.56371831893921 -0.433914184570312
3.56502103805542 -0.433944702148438
3.56690859794617 -0.433990478515625
3.56925678253174 -0.43426513671875
3.57263922691345 -0.434310913085938
3.57263922691345 -0.434326171875
3.57379961013794 -0.434371948242188
3.57391548156738 -0.434417724609375
3.574378490448 -0.434463500976562
3.57530331611633 -0.434524536132812
3.57530331611633 -0.4345703125
3.57645654678345 -0.434600830078125
3.57749176025391 -0.4346923828125
3.57772159576416 -0.434738159179688
3.58149456977844 -0.434783935546875
3.58194971084595 -0.434844970703125
3.58263158798218 -0.434890747070312
3.58319878578186 -0.434951782226562
3.58387851715088 -0.43499755859375
3.58478331565857 -0.435165405273438
3.58568620681763 -0.435256958007812
3.58579897880554 -0.435287475585938
3.58681225776672 -0.435348510742188
3.58737421035767 -0.435394287109375
3.58782315254211 -0.435440063476562
3.58782315254211 -0.435470581054688
3.58849573135376 -0.435501098632812
3.58927917480469 -0.435638427734375
3.58961462974548 -0.4356689453125
3.59239888191223 -0.435867309570312
3.59273171424866 -0.435897827148438
3.59328603744507 -0.435958862304688
3.59372901916504 -0.435989379882812
3.59461355209351 -0.43603515625
3.59604692459106 -0.436126708984375
3.59626722335815 -0.436172485351562
3.59681701660156 -0.436187744140625
3.59681701660156 -0.436233520507812
3.60053730010986 -0.436431884765625
3.60064625740051 -0.436477661132812
3.6011905670166 -0.436508178710938
3.6011905670166 -0.4365234375
3.6051971912384 -0.436859130859375
3.61246585845947 -0.437774658203125
3.61310148239136 -0.438186645507812
3.61373615264893 -0.438217163085938
3.61394739151001 -0.438247680664062
3.61394739151001 -0.438278198242188
3.61436986923218 -0.438308715820312
3.61563444137573 -0.438461303710938
3.61595010757446 -0.438507080078125
3.61700034141541 -0.4385986328125
3.61836194992065 -0.438629150390625
3.61867547035217 -0.43865966796875
3.6187801361084 -0.438690185546875
3.62003183364868 -0.438735961914062
3.62034440040588 -0.438766479492188
3.62044835090637 -0.438796997070312
3.62314581871033 -0.4390869140625
3.62345600128174 -0.439102172851562
3.62355947494507 -0.43914794921875
3.62551832199097 -0.439224243164062
3.62582659721375 -0.439254760742188
3.62767314910889 -0.439285278320312
3.62777543067932 -0.439300537109375
3.6305296421051 -0.4398193359375
3.6306312084198 -0.439849853515625
3.63124084472656 -0.439865112304688
3.63124084472656 -0.43988037109375
3.63134217262268 -0.439895629882812
3.6397852897644 -0.441192626953125
3.64018321037292 -0.441314697265625
3.64058089256287 -0.441329956054688
3.64236569404602 -0.441452026367188
3.64266228675842 -0.44146728515625
3.6466977596283 -0.4415283203125
3.64679574966431 -0.441543579101562
3.64699149131775 -0.441558837890625
3.64718723297119 -0.441574096679688
3.6472852230072 -0.441619873046875
3.64875030517578 -0.441635131835938
3.64914011955261 -0.441665649414062
3.64933490753174 -0.441680908203125
3.64943218231201 -0.44171142578125
3.65011310577393 -0.441726684570312
3.65011310577393 -0.441741943359375
3.65272974967957 -0.4417724609375
3.65552258491516 -0.441864013671875
3.65590643882751 -0.441879272460938
3.65648150444031 -0.441909790039062
3.65676879882812 -0.441940307617188
3.65696024894714 -0.44195556640625
3.65820217132568 -0.442001342773438
3.65829753875732 -0.4420166015625
3.65839314460754 -0.442031860351562
3.65839314460754 -0.442047119140625
3.65991616249084 -0.44207763671875
3.65991616249084 -0.442092895507812
3.66039109230042 -0.442123413085938
3.66039109230042 -0.442153930664062
3.66039109230042 -0.442169189453125
3.66077065467834 -0.44219970703125
3.66077065467834 -0.442214965820312
3.66077065467834 -0.442245483398438
3.66162347793579 -0.4422607421875
3.66435980796814 -0.442367553710938
3.66454792022705 -0.4423828125
3.66454792022705 -0.442398071289062
3.66529941558838 -0.442520141601562
3.6655809879303 -0.442520141601562
3.67015314102173 -0.442962646484375
3.67043137550354 -0.4429931640625
3.67061686515808 -0.443008422851562
3.67080235481262 -0.443023681640625
3.67126536369324 -0.443038940429688
3.67302083969116 -0.443069458007812
3.67329740524292 -0.443084716796875
3.67513656616211 -0.443161010742188
3.67541170120239 -0.44317626953125
3.67550349235535 -0.443191528320312
3.67550349235535 -0.443206787109375
3.6759614944458 -0.443222045898438
3.67660212516785 -0.4432373046875
3.67678499221802 -0.443252563476562
3.67687654495239 -0.443267822265625
3.67970037460327 -0.443450927734375
3.68006348609924 -0.443466186523438
3.68241596221924 -0.443466186523438
3.68268656730652 -0.443496704101562
3.68340730667114 -0.443527221679688
3.68358731269836 -0.44354248046875
3.68385720252991 -0.443557739257812
3.68385720252991 -0.443572998046875
3.68556261062622 -0.443588256835938
3.68565225601196 -0.443588256835938
3.6873505115509 -0.443756103515625
3.68752908706665 -0.44378662109375
3.68779635429382 -0.443801879882812
3.69037342071533 -0.443817138671875
3.69063901901245 -0.443832397460938
3.69063901901245 -0.44384765625
3.69063901901245 -0.443862915039062
3.69081616401672 -0.443862915039062
3.69081616401672 -0.443862915039062
3.69853544235229 -0.445526123046875
3.70156788825989 -0.44598388671875
3.70191311836243 -0.446014404296875
3.70199942588806 -0.446014404296875
3.70234441757202 -0.446029663085938
3.70294713973999 -0.446075439453125
3.70671772956848 -0.446090698242188
3.7068030834198 -0.446090698242188
3.70748496055603 -0.44610595703125
3.70757007598877 -0.446121215820312
3.70799565315247 -0.446136474609375
3.70808076858521 -0.446136474609375
3.70808076858521 -0.4461669921875
3.70867586135864 -0.446182250976562
3.70867586135864 -0.446182250976562
3.70901536941528 -0.446197509765625
3.7091851234436 -0.446197509765625
3.70927000045776 -0.446212768554688
3.71011734008789 -0.44622802734375
3.71028661727905 -0.446243286132812
3.71070957183838 -0.446258544921875
3.71079421043396 -0.446258544921875
3.71138548851013 -0.446273803710938
3.71138548851013 -0.4462890625
3.71315431594849 -0.446517944335938
3.71349048614502 -0.446563720703125
3.71374249458313 -0.446563720703125
3.71491622924805 -0.446563720703125
3.71499991416931 -0.446563720703125
3.71508359909058 -0.446578979492188
3.71575260162354 -0.44659423828125
3.71575260162354 -0.44659423828125
3.71658754348755 -0.44671630859375
3.71700429916382 -0.44671630859375
3.71742081642151 -0.446731567382812
3.71800327301025 -0.446731567382812
3.72024202346802 -0.44683837890625
3.72048997879028 -0.446853637695312
3.72048997879028 -0.446853637695312
3.72238707542419 -0.446975708007812
3.72246932983398 -0.447006225585938
3.72296285629272 -0.447006225585938
3.72353768348694 -0.447021484375
3.72361993789673 -0.447021484375
3.72468543052673 -0.447067260742188
3.72550320625305 -0.447067260742188
3.72550320625305 -0.44708251953125
3.72558498382568 -0.44708251953125
3.72705292701721 -0.447158813476562
3.72713446617126 -0.447158813476562
3.72745990753174 -0.447174072265625
3.72778511047363 -0.447174072265625
3.72786641120911 -0.447189331054688
3.72956967353821 -0.447311401367188
3.72981262207031 -0.44732666015625
3.72981262207031 -0.44732666015625
3.72997426986694 -0.44732666015625
3.73029756546021 -0.447341918945312
3.73102426528931 -0.447372436523438
3.73102426528931 -0.447372436523438
3.73150825500488 -0.447372436523438
3.73183035850525 -0.4473876953125
3.73231339454651 -0.4473876953125
3.73271536827087 -0.447402954101562
3.7330367565155 -0.447402954101562
3.7330367565155 -0.447402954101562
3.7330367565155 -0.447418212890625
3.73407936096191 -0.447433471679688
3.7344799041748 -0.44744873046875
3.73495984077454 -0.447463989257812
3.73495984077454 -0.447463989257812
3.73559880256653 -0.447479248046875
3.73567867279053 -0.447494506835938
3.7363965511322 -0.447494506835938
3.7363965511322 -0.447494506835938
3.7371129989624 -0.447525024414062
3.7371129989624 -0.447525024414062
3.73751068115234 -0.447525024414062
3.7376697063446 -0.447540283203125
3.73798727989197 -0.447555541992188
3.73830485343933 -0.447555541992188
3.73838424682617 -0.447555541992188
3.73980951309204 -0.44757080078125
3.73996782302856 -0.44757080078125
3.74036264419556 -0.447586059570312
3.74107265472412 -0.447601318359375
3.7411515712738 -0.447601318359375
3.74256801605225 -0.4476318359375
3.74264669418335 -0.447647094726562
3.74311757087708 -0.447647094726562
3.74311757087708 -0.447647094726562
3.74343132972717 -0.447647094726562
3.74343132972717 -0.447662353515625
3.74437117576599 -0.447677612304688
3.74437117576599 -0.447677612304688
3.74562120437622 -0.44775390625
3.74632263183594 -0.447784423828125
3.74741172790527 -0.447784423828125
3.74772238731384 -0.447799682617188
3.74780011177063 -0.447799682617188
3.74958181381226 -0.447891235351562
3.74973630905151 -0.447906494140625
3.75004529953003 -0.447921752929688
3.75035405158997 -0.447921752929688
3.75035405158997 -0.447921752929688
3.75035405158997 -0.44793701171875
3.75089383125305 -0.44793701171875
3.75097107887268 -0.44793701171875
3.75204849243164 -0.448013305664062
3.75319981575012 -0.448028564453125
3.75388932228088 -0.448043823242188
3.75404238700867 -0.448043823242188
3.75427198410034 -0.448043823242188
3.75595092773438 -0.44805908203125
3.75610327720642 -0.448074340820312
3.75640773773193 -0.448074340820312
3.75648403167725 -0.448074340820312
3.75663614273071 -0.448074340820312
3.75769972801208 -0.448104858398438
3.75815463066101 -0.4481201171875
3.75823044776917 -0.4481201171875
3.75830626487732 -0.4481201171875
3.75951671600342 -0.448196411132812
3.75996994972229 -0.448211669921875
3.76034712791443 -0.448211669921875
3.76042246818542 -0.448226928710938
3.7609498500824 -0.448226928710938
3.76102519035339 -0.4482421875
3.76245355606079 -0.448287963867188
3.7627534866333 -0.44830322265625
3.76290345191956 -0.44830322265625
3.76440024375916 -0.448318481445312
3.76462435722351 -0.448318481445312
3.76469898223877 -0.448318481445312
3.76492309570312 -0.448318481445312
3.76492309570312 -0.448333740234375
3.7649974822998 -0.448333740234375
3.76529598236084 -0.448333740234375
3.76529598236084 -0.448333740234375
3.76566863059998 -0.4483642578125
3.76566863059998 -0.4483642578125
3.76618957519531 -0.4483642578125
3.76626420021057 -0.448379516601562
3.76663589477539 -0.448379516601562
3.76708173751831 -0.448394775390625
3.76708173751831 -0.448394775390625
3.76708173751831 -0.448394775390625
3.76760101318359 -0.448410034179688
3.76826810836792 -0.448440551757812
3.76826810836792 -0.448440551757812
3.76856422424316 -0.448455810546875
3.76886010169983 -0.448455810546875
3.76893401145935 -0.448455810546875
3.76908183097839 -0.448471069335938
3.7693772315979 -0.448486328125
3.76982021331787 -0.448486328125
3.76982021331787 -0.448501586914062
3.77026271820068 -0.448501586914062
3.77055740356445 -0.448516845703125
3.77055740356445 -0.448516845703125
3.77077841758728 -0.448516845703125
3.77239513397217 -0.448623657226562
3.77254176139832 -0.448654174804688
3.77298140525818 -0.448654174804688
3.77334761619568 -0.448654174804688
3.77334761619568 -0.44866943359375
3.77517342567444 -0.448745727539062
3.77531909942627 -0.448822021484375
3.7754647731781 -0.448837280273438
3.77597427368164 -0.448837280273438
3.77597427368164 -0.448837280273438
3.77684640884399 -0.4488525390625
3.77735424041748 -0.448867797851562
3.77764415740967 -0.448883056640625
3.77771663665771 -0.448883056640625
3.7780065536499 -0.448898315429688
3.77974081039429 -0.448928833007812
3.78010129928589 -0.448974609375
3.78017330169678 -0.448974609375
3.780677318573 -0.448989868164062
3.78103685379028 -0.448989868164062
3.78211402893066 -0.44903564453125
3.78261590003967 -0.449050903320312
3.78318858146667 -0.449066162109375
3.78340339660645 -0.449066162109375
3.78368926048279 -0.449081420898438
3.78433203697205 -0.4490966796875
3.78447461128235 -0.4490966796875
3.78511619567871 -0.449111938476562
3.78547215461731 -0.449111938476562
3.78575682640076 -0.449142456054688
3.78625440597534 -0.449142456054688
3.78746056556702 -0.449188232421875
3.78753137588501 -0.449188232421875
3.78781461715698 -0.449188232421875
3.7885217666626 -0.44921875
3.78915739059448 -0.449234008789062
3.7896511554718 -0.449234008789062
3.7896511554718 -0.449249267578125
3.7896511554718 -0.449249267578125
3.78993320465088 -0.449249267578125
3.79042601585388 -0.449264526367188
3.79049634933472 -0.449264526367188
3.79056668281555 -0.449264526367188
3.79211139678955 -0.4493408203125
3.79211139678955 -0.449356079101562
3.79218149185181 -0.449356079101562
3.79253172874451 -0.449371337890625
3.79316163063049 -0.449386596679688
3.79372048377991 -0.44940185546875
3.79379034042358 -0.44940185546875
3.79386019706726 -0.44940185546875
3.79413938522339 -0.449417114257812
3.79420900344849 -0.449417114257812
3.79476690292358 -0.449417114257812
3.79601907730103 -0.449493408203125
3.7963662147522 -0.449508666992188
3.79664373397827 -0.449508666992188
3.79754447937012 -0.449539184570312
3.79768300056458 -0.449554443359375
3.79802870750427 -0.449554443359375
3.79802870750427 -0.449554443359375
3.79802870750427 -0.449569702148438
3.79968500137329 -0.449722290039062
3.79968500137329 -0.449752807617188
3.80030465126038 -0.44976806640625
3.80044221878052 -0.449783325195312
3.80085444450378 -0.449783325195312
3.80085444450378 -0.449783325195312
3.80174660682678 -0.449798583984375
3.80174660682678 -0.449798583984375
3.80202078819275 -0.449798583984375
3.80297875404358 -0.449859619140625
3.80311560630798 -0.449874877929688
3.80311560630798 -0.449874877929688
3.80475258827209 -0.449935913085938
3.80502486228943 -0.449935913085938
3.80509281158447 -0.449935913085938
3.8051609992981 -0.449951171875
3.8051609992981 -0.449951171875
3.80543279647827 -0.449951171875
3.80543279647827 -0.449966430664062
3.80590844154358 -0.449966430664062
3.80590844154358 -0.449966430664062
3.80597639083862 -0.449966430664062
3.80631566047668 -0.449996948242188
3.80773782730103 -0.449996948242188
3.80780553817749 -0.449996948242188
3.80787324905396 -0.45001220703125
3.80787324905396 -0.45001220703125
3.80814337730408 -0.45001220703125
3.80821084976196 -0.450027465820312
3.80868339538574 -0.450027465820312
3.80875086784363 -0.450027465820312
3.80935764312744 -0.450042724609375
3.80935764312744 -0.450057983398438
3.80942511558533 -0.450057983398438
3.80969429016113 -0.450057983398438
3.80969429016113 -0.450057983398438
3.80969429016113 -0.450057983398438
3.80969429016113 -0.4500732421875
3.81016540527344 -0.4500732421875
3.81029963493347 -0.4500732421875
3.81029963493347 -0.450088500976562
3.81077003479004 -0.450088500976562
3.81103849411011 -0.450088500976562
3.81103849411011 -0.450088500976562
3.81110572814941 -0.450088500976562
3.81164193153381 -0.450103759765625
3.81170892715454 -0.450103759765625
3.81204390525818 -0.450119018554688
3.81211090087891 -0.450119018554688
3.81211090087891 -0.450119018554688
3.81211090087891 -0.450119018554688
3.81237840652466 -0.45013427734375
3.8132472038269 -0.450149536132812
3.81331396102905 -0.450164794921875
3.8133807182312 -0.450164794921875
3.81404781341553 -0.450164794921875
3.8141143321991 -0.450164794921875
3.81418108940125 -0.450180053710938
3.81431412696838 -0.450180053710938
3.81458044052124 -0.4501953125
3.81504607200623 -0.4501953125
3.81504607200623 -0.4501953125
3.81504607200623 -0.4501953125
3.81511259078979 -0.4501953125
3.81511259078979 -0.4501953125
3.81511259078979 -0.4501953125
3.81524562835693 -0.450210571289062
3.81524562835693 -0.450210571289062
3.81524562835693 -0.450210571289062
3.81557774543762 -0.450210571289062
3.81557774543762 -0.450225830078125
3.81557774543762 -0.450225830078125
3.81584334373474 -0.450225830078125
3.81584334373474 -0.450225830078125
3.81584334373474 -0.450225830078125
3.81584334373474 -0.450225830078125
3.81584334373474 -0.450225830078125
3.8166389465332 -0.45025634765625
3.8166389465332 -0.450271606445312
3.81716847419739 -0.450271606445312
3.81716847419739 -0.450286865234375
3.81716847419739 -0.450286865234375
3.81716847419739 -0.450286865234375
3.81716847419739 -0.450286865234375
3.81716847419739 -0.450286865234375
3.81716847419739 -0.450286865234375
3.82000422477722 -0.45037841796875
3.82013583183289 -0.450393676757812
3.82013583183289 -0.450393676757812
3.82020139694214 -0.450393676757812
3.82020139694214 -0.450393676757812
3.82020139694214 -0.450393676757812
3.82039856910706 -0.450393676757812
3.82039856910706 -0.450393676757812
3.82039856910706 -0.450393676757812
3.82046413421631 -0.450408935546875
3.82046413421631 -0.450408935546875
3.82046413421631 -0.450408935546875
3.82072687149048 -0.450408935546875
3.82072687149048 -0.450408935546875
3.82072687149048 -0.450408935546875
3.82072687149048 -0.450408935546875
3.82072687149048 -0.450424194335938
3.82098913192749 -0.450424194335938
3.82098913192749 -0.450424194335938
3.82157897949219 -0.450454711914062
3.82164454460144 -0.450454711914062
3.82177543640137 -0.450454711914062
3.82177543640137 -0.450454711914062
3.82177543640137 -0.450454711914062
3.82184100151062 -0.450454711914062
3.82210254669189 -0.450469970703125
3.82216811180115 -0.450469970703125
3.82223343849182 -0.450469970703125
3.82223343849182 -0.450469970703125
3.82223343849182 -0.450469970703125
3.82223343849182 -0.450469970703125
3.82406067848206 -0.450485229492188
3.82406067848206 -0.450485229492188
3.82425594329834 -0.450485229492188
3.82432103157043 -0.450485229492188
3.82432103157043 -0.450485229492188
3.82432103157043 -0.450485229492188
3.82464647293091 -0.45050048828125
3.82510137557983 -0.45050048828125
3.82516646385193 -0.45050048828125
3.82523131370544 -0.45050048828125
3.82523131370544 -0.45050048828125
3.8256208896637 -0.450515747070312
3.8256208896637 -0.450515747070312
3.82600998878479 -0.450515747070312
3.82613968849182 -0.450515747070312
3.82620429992676 -0.450531005859375
3.82620429992676 -0.450531005859375
3.82659292221069 -0.450531005859375
3.82659292221069 -0.450531005859375
3.82775688171387 -0.4505615234375
3.8279504776001 -0.4505615234375
3.82801508903503 -0.450576782226562
3.82814407348633 -0.450576782226562
3.82814407348633 -0.450576782226562
3.82814407348633 -0.450576782226562
3.82814407348633 -0.450576782226562
3.8286600112915 -0.450576782226562
3.8286600112915 -0.450576782226562
3.83033204078674 -0.450607299804688
3.8304603099823 -0.45062255859375
3.83058857917786 -0.45062255859375
3.83065271377563 -0.45062255859375
3.83071684837341 -0.45062255859375
3.83116555213928 -0.45062255859375
3.83122968673706 -0.45062255859375
3.83122968673706 -0.45062255859375
3.83148574829102 -0.450637817382812
3.83365702629089 -0.450637817382812
3.83365702629089 -0.450637817382812
3.83372068405151 -0.450637817382812
3.83391165733337 -0.450637817382812
3.83391165733337 -0.450637817382812
3.83397531509399 -0.450637817382812
3.83422994613647 -0.450637817382812
3.83422994613647 -0.450653076171875
3.83422994613647 -0.450653076171875
3.83429360389709 -0.450653076171875
3.83461141586304 -0.450653076171875
3.83461141586304 -0.450653076171875
3.8349289894104 -0.450668334960938
3.8349289894104 -0.450668334960938
3.83499264717102 -0.450668334960938
3.83550024032593 -0.450668334960938
3.83569049835205 -0.45068359375
3.83569049835205 -0.45068359375
3.83600735664368 -0.45068359375
3.83600735664368 -0.45068359375
3.83626079559326 -0.45068359375
3.83626079559326 -0.450698852539062
3.83626079559326 -0.450698852539062
3.83714628219604 -0.450698852539062
3.83727264404297 -0.450714111328125
3.83727264404297 -0.450714111328125
3.83727264404297 -0.450714111328125
3.8375883102417 -0.450714111328125
3.83765149116516 -0.450714111328125
3.83765149116516 -0.450714111328125
3.83777785301208 -0.450714111328125
3.83796691894531 -0.450714111328125
3.83809304237366 -0.450729370117188
3.83809304237366 -0.450729370117188
3.83809304237366 -0.450729370117188
3.83866024017334 -0.450729370117188
3.83866024017334 -0.450729370117188
3.83872318267822 -0.450729370117188
3.83928942680359 -0.45074462890625
3.83928942680359 -0.45074462890625
3.83928942680359 -0.45074462890625
3.83941507339478 -0.45074462890625
3.8402316570282 -0.450759887695312
3.8402943611145 -0.450759887695312
3.84035706520081 -0.450759887695312
3.84123420715332 -0.450790405273438
3.84135937690735 -0.450790405273438
3.84198474884033 -0.450790405273438
3.84217214584351 -0.4508056640625
3.8424220085144 -0.4508056640625
3.8424220085144 -0.4508056640625
3.8424220085144 -0.4508056640625
3.84460139274597 -0.45086669921875
3.84478783607483 -0.450897216796875
3.84627532958984 -0.450897216796875
3.84652256965637 -0.450897216796875
3.84658455848694 -0.450897216796875
3.84738755226135 -0.450912475585938
3.84751105308533 -0.450912475585938
3.84769606590271 -0.450912475585938
3.84775757789612 -0.450927734375
3.8483738899231 -0.450927734375
3.84849691390991 -0.450927734375
3.84849691390991 -0.450927734375
3.84972643852234 -0.450942993164062
3.84984922409058 -0.450942993164062
3.85064625740051 -0.450958251953125
3.85064625740051 -0.450958251953125
3.85076880455017 -0.450958251953125
3.85076880455017 -0.450958251953125
3.85205268859863 -0.451004028320312
3.85211396217346 -0.451019287109375
3.85217499732971 -0.451019287109375
3.85223603248596 -0.451019287109375
3.85254096984863 -0.451019287109375
3.85278487205505 -0.451034545898438
3.8530285358429 -0.451034545898438
3.8530285358429 -0.451034545898438
3.85308957099915 -0.451034545898438
3.85375905036926 -0.4510498046875
3.85400223731995 -0.4510498046875
3.85412383079529 -0.4510498046875
3.85412383079529 -0.4510498046875
3.85570073127747 -0.451080322265625
3.85576128959656 -0.451080322265625
3.85582184791565 -0.451080322265625
3.85582184791565 -0.451080322265625
3.85871767997742 -0.451141357421875
3.85883784294128 -0.451171875
3.85907816886902 -0.451171875
3.85931849479675 -0.451171875
3.85931849479675 -0.451171875
3.85943841934204 -0.451171875
3.85943841934204 -0.451171875
3.85973858833313 -0.451171875
3.85985851287842 -0.451187133789062
3.86009836196899 -0.451187133789062
3.86009836196899 -0.451187133789062
3.86009836196899 -0.451187133789062
3.86015820503235 -0.451187133789062
3.86015820503235 -0.451187133789062
3.86045789718628 -0.451187133789062
3.86057758331299 -0.451187133789062
3.86081695556641 -0.451202392578125
3.86081695556641 -0.451202392578125
3.86081695556641 -0.451202392578125
3.86081695556641 -0.451202392578125
3.86081695556641 -0.451202392578125
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{FOOF}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.567008972167969, ymax=0.0270004272460938,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c12)}
]
\addplot [ultra thick, brown, dashed]
table {%
0.60206001996994 0
0.954242527484894 -3.0517578125e-05
1.54406809806824 -3.0517578125e-05
1.61278390884399 -6.103515625e-05
1.79934048652649 -9.1552734375e-05
1.83884906768799 -9.1552734375e-05
2.78318858146667 -0.00299072265625
2.83884906768799 -0.00628662109375
2.89431595802307 -0.006500244140625
3.00603795051575 -0.0074462890625
3.07040739059448 -0.007904052734375
3.10585069656372 -0.008453369140625
3.17753648757935 -0.0086669921875
3.33000779151917 -0.011260986328125
3.37511467933655 -0.012115478515625
3.39759254455566 -0.012420654296875
3.4186327457428 -0.01263427734375
3.44435715675354 -0.0133056640625
3.47741079330444 -0.01397705078125
3.51255106925964 -0.014190673828125
3.53135108947754 -0.014434814453125
3.54666614532471 -0.014556884765625
3.5569052696228 -0.01470947265625
3.57089304924011 -0.014801025390625
3.59006118774414 -0.014923095703125
3.60346913337708 -0.015106201171875
3.615318775177 -0.015228271484375
3.65147185325623 -0.015869140625
3.67070960998535 -0.016693115234375
3.68069791793823 -0.017120361328125
3.69548177719116 -0.017242431640625
3.72222256660461 -0.0186767578125
3.73013591766357 -0.01904296875
3.73231339454651 -0.019287109375
3.74811053276062 -0.01983642578125
3.77217483520508 -0.0201416015625
3.77459001541138 -0.020294189453125
3.79309153556824 -0.020843505859375
3.80044221878052 -0.021087646484375
3.81331396102905 -0.02166748046875
3.8347384929657 -0.022369384765625
3.85369825363159 -0.0235595703125
3.86729073524475 -0.02410888671875
3.91222214698792 -0.029327392578125
3.93262600898743 -0.030975341796875
3.94171023368835 -0.031585693359375
3.95458006858826 -0.03204345703125
3.96736073493958 -0.03253173828125
3.97909283638 -0.03326416015625
4.01266860961914 -0.034271240234375
4.02308797836304 -0.03466796875
4.03590965270996 -0.035491943359375
4.04883003234863 -0.03594970703125
4.05880546569824 -0.036590576171875
4.09215879440308 -0.043121337890625
4.10822677612305 -0.045501708984375
4.12949657440186 -0.047576904296875
4.13770198822021 -0.049102783203125
4.1495885848999 -0.0501708984375
4.18667411804199 -0.06170654296875
4.19548463821411 -0.066741943359375
4.23271656036377 -0.070465087890625
4.23974990844727 -0.072906494140625
4.25367736816406 -0.076751708984375
4.27726554870605 -0.082916259765625
4.31009817123413 -0.097076416015625
4.3335075378418 -0.11175537109375
4.35460758209229 -0.12652587890625
4.360915184021 -0.130950927734375
4.3758282661438 -0.13275146484375
4.38815450668335 -0.134124755859375
4.39604234695435 -0.134765625
4.40442323684692 -0.135833740234375
4.41463899612427 -0.1365966796875
4.416090965271 -0.136810302734375
4.43464851379395 -0.144989013671875
4.44466924667358 -0.147491455078125
4.45150995254517 -0.148468017578125
4.46101808547974 -0.150360107421875
4.46908521652222 -0.1514892578125
4.47712135314941 -0.15277099609375
4.48912858963013 -0.15655517578125
4.49607133865356 -0.15802001953125
4.50308227539062 -0.159423828125
4.50925636291504 -0.160675048828125
4.51963090896606 -0.164276123046875
4.52853107452393 -0.166259765625
4.53424215316772 -0.1673583984375
4.54749155044556 -0.174530029296875
4.55447721481323 -0.179168701171875
4.5629825592041 -0.1817626953125
4.56968975067139 -0.18585205078125
4.57945203781128 -0.188262939453125
4.58635091781616 -0.19085693359375
4.591965675354 -0.1932373046875
4.60011196136475 -0.197998046875
4.61022329330444 -0.20257568359375
4.61891603469849 -0.2061767578125
4.63024473190308 -0.219207763671875
4.6397852897644 -0.23895263671875
4.64752960205078 -0.258209228515625
4.65363693237305 -0.274566650390625
4.66126346588135 -0.283477783203125
4.66418123245239 -0.287628173828125
4.66902828216553 -0.29071044921875
4.67293787002563 -0.292388916015625
4.67905521392822 -0.2998046875
4.68414497375488 -0.3023681640625
4.68789434432983 -0.3046875
4.69260883331299 -0.306365966796875
4.69947338104248 -0.316162109375
4.70537614822388 -0.321075439453125
4.70848894119263 -0.322723388671875
4.71282625198364 -0.32513427734375
4.71697092056274 -0.3275146484375
4.72209882736206 -0.3310546875
4.72645807266235 -0.334075927734375
4.73062896728516 -0.335968017578125
4.73705720901489 -0.34515380859375
4.73878049850464 -0.347808837890625
4.74225378036499 -0.349517822265625
4.7458553314209 -0.350677490234375
4.75105571746826 -0.3543701171875
4.75372838973999 -0.35601806640625
4.76005268096924 -0.361968994140625
4.76219081878662 -0.36376953125
4.76768255233765 -0.367919921875
4.77290105819702 -0.369903564453125
4.77722358703613 -0.372100830078125
4.78013706207275 -0.373138427734375
4.78796339035034 -0.38055419921875
4.79157829284668 -0.38323974609375
4.7961368560791 -0.38507080078125
4.80051755905151 -0.386688232421875
4.80454158782959 -0.387908935546875
4.80856895446777 -0.38916015625
4.81391429901123 -0.3912353515625
4.82001733779907 -0.396331787109375
4.8234806060791 -0.3980712890625
4.82860851287842 -0.399749755859375
4.83401346206665 -0.40118408203125
4.83867931365967 -0.40301513671875
4.84330129623413 -0.405181884765625
4.84817695617676 -0.40740966796875
4.85550689697266 -0.415863037109375
4.86086463928223 -0.4188232421875
4.8653883934021 -0.4219970703125
4.87083101272583 -0.423797607421875
4.87319278717041 -0.424713134765625
4.8822283744812 -0.4393310546875
4.88463115692139 -0.442657470703125
4.89335680007935 -0.448333740234375
4.89921283721924 -0.450042724609375
4.90329599380493 -0.45166015625
4.91179132461548 -0.45330810546875
4.91810894012451 -0.4541015625
4.92264223098755 -0.454986572265625
4.92908143997192 -0.458648681640625
4.93795394897461 -0.463470458984375
4.94176006317139 -0.4647216796875
4.94508457183838 -0.465362548828125
4.94987297058105 -0.47332763671875
4.95172595977783 -0.476531982421875
4.9532036781311 -0.4774169921875
4.95523548126221 -0.480224609375
4.95718574523926 -0.483428955078125
4.95829153060913 -0.4847412109375
4.95932769775391 -0.4853515625
4.96113634109497 -0.487091064453125
4.96342420578003 -0.49078369140625
4.96441030502319 -0.49224853515625
4.96515941619873 -0.49267578125
4.96606683731079 -0.49383544921875
4.96709823608398 -0.494354248046875
4.9682822227478 -0.495147705078125
4.96954154968262 -0.49658203125
4.97123432159424 -0.497467041015625
4.97230005264282 -0.497772216796875
4.97341871261597 -0.4981689453125
4.97425842285156 -0.498382568359375
4.97514677047729 -0.498504638671875
4.97660207748413 -0.499481201171875
4.97759580612183 -0.499755859375
4.98042154312134 -0.503143310546875
4.9815149307251 -0.503997802734375
4.98254251480103 -0.504150390625
4.98357200622559 -0.50439453125
4.98425722122192 -0.504547119140625
4.98495483398438 -0.50469970703125
4.98614883422852 -0.504913330078125
4.98695516586304 -0.505035400390625
4.98790311813354 -0.50531005859375
4.98853206634521 -0.505462646484375
4.98896455764771 -0.5057373046875
4.99016571044922 -0.50604248046875
4.99070739746094 -0.50634765625
4.99110221862793 -0.5064697265625
4.99302577972412 -0.5078125
4.99363040924072 -0.508026123046875
4.99407052993774 -0.508148193359375
4.99447536468506 -0.508270263671875
4.99493265151978 -0.50836181640625
4.99598598480225 -0.508575439453125
4.99696254730225 -0.5086669921875
4.99811124801636 -0.5093994140625
4.99952220916748 -0.509735107421875
5.00124025344849 -0.51171875
5.00215291976929 -0.512115478515625
5.00285243988037 -0.512176513671875
5.00395154953003 -0.5123291015625
5.00436019897461 -0.512420654296875
5.00484991073608 -0.512542724609375
5.00704765319824 -0.514495849609375
5.00781154632568 -0.514801025390625
5.00810623168945 -0.514892578125
5.00877046585083 -0.5150146484375
5.00974416732788 -0.51507568359375
5.01040172576904 -0.515228271484375
5.0107536315918 -0.515350341796875
5.01127433776855 -0.515380859375
5.01266860961914 -0.51641845703125
5.01365852355957 -0.516510009765625
5.01425170898438 -0.51666259765625
5.01503276824951 -0.51690673828125
5.01569509506226 -0.5169677734375
5.01630210876465 -0.517059326171875
5.01672410964966 -0.51708984375
5.01702499389648 -0.51715087890625
5.0173921585083 -0.5172119140625
5.01774263381958 -0.517242431640625
5.01860904693604 -0.517303466796875
5.01896667480469 -0.517364501953125
5.01939058303833 -0.517425537109375
5.01983880996704 -0.51751708984375
5.02094507217407 -0.517669677734375
5.02125549316406 -0.51776123046875
5.02281188964844 -0.5186767578125
5.02303409576416 -0.51873779296875
5.023606300354 -0.518798828125
5.02392721176147 -0.518829345703125
5.02445697784424 -0.51898193359375
5.02497386932373 -0.51910400390625
5.02530574798584 -0.5191650390625
5.02575206756592 -0.519195556640625
5.02754926681519 -0.52056884765625
5.02777338027954 -0.520721435546875
5.02805042266846 -0.520782470703125
5.02842903137207 -0.52081298828125
5.02866888046265 -0.5208740234375
5.02905893325806 -0.52099609375
5.02953004837036 -0.5211181640625
5.02972888946533 -0.521148681640625
5.03040552139282 -0.5213623046875
5.03110122680664 -0.521392822265625
5.03130722045898 -0.521453857421875
5.03199005126953 -0.521575927734375
5.03253412246704 -0.521636962890625
5.03285646438599 -0.52166748046875
5.03417110443115 -0.5220947265625
5.03454828262329 -0.52215576171875
5.03519773483276 -0.522216796875
5.03539371490479 -0.522247314453125
5.03566598892212 -0.522308349609375
5.03604173660278 -0.522430419921875
5.0366849899292 -0.522491455078125
5.03706789016724 -0.522552490234375
5.03743457794189 -0.52264404296875
5.03758573532104 -0.522674560546875
5.03795194625854 -0.522705078125
5.03917598724365 -0.523223876953125
5.03947734832764 -0.523284912109375
5.03985404968262 -0.5233154296875
5.04087924957275 -0.523681640625
5.04132556915283 -0.523834228515625
5.04174375534058 -0.52386474609375
5.04219722747803 -0.523895263671875
5.04311084747314 -0.524139404296875
5.04361391067505 -0.524200439453125
5.04417133331299 -0.5242919921875
5.04447317123413 -0.52435302734375
5.04492378234863 -0.524444580078125
5.04561614990234 -0.52447509765625
5.04613590240479 -0.52459716796875
5.04630374908447 -0.524627685546875
5.04758644104004 -0.52490234375
5.04798698425293 -0.5250244140625
5.04813861846924 -0.525054931640625
5.04908609390259 -0.525299072265625
5.04927253723145 -0.52532958984375
5.04948568344116 -0.525360107421875
5.04971027374268 -0.525421142578125
5.05162334442139 -0.526458740234375
5.05188131332397 -0.52655029296875
5.05214357376099 -0.526580810546875
5.05244016647339 -0.52667236328125
5.05295562744141 -0.526763916015625
5.05314779281616 -0.52679443359375
5.05345106124878 -0.526824951171875
5.05391931533813 -0.52685546875
5.05417251586914 -0.526885986328125
5.05490398406982 -0.52691650390625
5.05579853057861 -0.527496337890625
5.05634069442749 -0.527557373046875
5.05657720565796 -0.527618408203125
5.05744934082031 -0.5277099609375
5.05771923065186 -0.527740478515625
5.05868053436279 -0.52789306640625
5.05885124206543 -0.52789306640625
5.05911636352539 -0.5279541015625
5.0592188835144 -0.5279541015625
5.06037664413452 -0.52874755859375
5.06071662902832 -0.52880859375
5.0608377456665 -0.52880859375
5.06169366836548 -0.52899169921875
5.06193876266479 -0.529022216796875
5.06204795837402 -0.529052734375
5.06246519088745 -0.52911376953125
5.06273603439331 -0.529144287109375
5.06306314468384 -0.5291748046875
5.06325435638428 -0.529205322265625
5.06433057785034 -0.529998779296875
5.0646824836731 -0.529998779296875
5.06580352783203 -0.53076171875
5.06643772125244 -0.530853271484375
5.0666241645813 -0.5308837890625
5.06721210479736 -0.530914306640625
5.06738328933716 -0.53094482421875
5.06756925582886 -0.53094482421875
5.06789970397949 -0.531005859375
5.06854963302612 -0.531036376953125
5.06874990463257 -0.531036376953125
5.06907939910889 -0.5311279296875
5.06929063796997 -0.5311279296875
5.06953477859497 -0.531158447265625
5.06977891921997 -0.531158447265625
5.06998634338379 -0.53118896484375
5.07014131546021 -0.53118896484375
5.07041120529175 -0.531219482421875
5.07069873809814 -0.531219482421875
5.0707802772522 -0.53125
5.07127809524536 -0.531463623046875
5.07174587249756 -0.531463623046875
5.07198143005371 -0.531494140625
5.07212495803833 -0.531524658203125
5.07273483276367 -0.531585693359375
5.07280492782593 -0.5316162109375
5.07302141189575 -0.5316162109375
5.07312059402466 -0.531646728515625
5.07332229614258 -0.531646728515625
5.0734543800354 -0.53167724609375
5.07478713989258 -0.53228759765625
5.07504320144653 -0.532318115234375
5.07538270950317 -0.532379150390625
5.07550668716431 -0.532379150390625
5.07609415054321 -0.53240966796875
5.07622146606445 -0.53240966796875
5.07631635665894 -0.532440185546875
5.07677125930786 -0.532501220703125
5.07694959640503 -0.532501220703125
5.07719326019287 -0.532501220703125
5.07796335220337 -0.532684326171875
5.07839155197144 -0.532684326171875
5.07841682434082 -0.532684326171875
5.07960081100464 -0.532989501953125
5.07981061935425 -0.532989501953125
5.08009958267212 -0.533050537109375
5.08029794692993 -0.533050537109375
5.08117818832397 -0.533203125
5.08131837844849 -0.533233642578125
5.08191251754761 -0.533233642578125
5.08237600326538 -0.53326416015625
5.08260583877563 -0.53326416015625
5.08272457122803 -0.533294677734375
5.08294343948364 -0.533294677734375
5.08306503295898 -0.5333251953125
5.08518362045288 -0.534393310546875
5.08532619476318 -0.534576416015625
5.08546876907349 -0.53460693359375
5.08560466766357 -0.53460693359375
5.08592510223389 -0.534637451171875
5.08595371246338 -0.534637451171875
5.08646297454834 -0.53472900390625
5.08687925338745 -0.53472900390625
5.08693599700928 -0.53472900390625
5.08749389648438 -0.534759521484375
5.08769989013672 -0.5347900390625
5.0879340171814 -0.5347900390625
5.08959054946899 -0.53521728515625
5.09006404876709 -0.535308837890625
5.09021234512329 -0.53533935546875
5.09026145935059 -0.53533935546875
5.09040641784668 -0.53533935546875
5.09057188034058 -0.535369873046875
5.09088897705078 -0.535369873046875
5.09102630615234 -0.535400390625
5.09108257293701 -0.535400390625
5.09164953231812 -0.535400390625
5.09198331832886 -0.535430908203125
5.09202194213867 -0.535430908203125
5.0924506187439 -0.53546142578125
5.09247493743896 -0.535491943359375
5.09311676025391 -0.535552978515625
5.09333753585815 -0.535552978515625
5.09354400634766 -0.53558349609375
5.0936074256897 -0.53558349609375
5.0940203666687 -0.53558349609375
5.09431743621826 -0.535614013671875
5.0943660736084 -0.535614013671875
5.09467029571533 -0.53564453125
5.09478902816772 -0.53564453125
5.09489011764526 -0.53564453125
5.09523916244507 -0.535675048828125
5.09527397155762 -0.535675048828125
5.0957202911377 -0.535675048828125
5.09578990936279 -0.53570556640625
5.09595012664795 -0.53570556640625
5.09606122970581 -0.53570556640625
5.09623527526855 -0.535736083984375
5.0963397026062 -0.535736083984375
5.09635019302368 -0.535736083984375
5.09660768508911 -0.5357666015625
5.09717750549316 -0.5357666015625
5.09805870056152 -0.53607177734375
5.09835290908813 -0.536102294921875
5.09878206253052 -0.536163330078125
5.09894800186157 -0.536163330078125
5.09904861450195 -0.536163330078125
5.09919691085815 -0.53619384765625
5.09936285018921 -0.53619384765625
5.09955644607544 -0.53619384765625
5.09981203079224 -0.536224365234375
5.10008764266968 -0.536224365234375
5.10016345977783 -0.536224365234375
5.10031890869141 -0.5362548828125
5.10058069229126 -0.5362548828125
5.1007251739502 -0.5362548828125
5.10074281692505 -0.536285400390625
5.10088729858398 -0.536285400390625
5.10106945037842 -0.536285400390625
5.10122108459473 -0.53631591796875
5.10168170928955 -0.536376953125
5.10181903839111 -0.536376953125
5.10209035873413 -0.53643798828125
5.102210521698 -0.536468505859375
5.10235834121704 -0.536468505859375
5.10266017913818 -0.536468505859375
5.10313320159912 -0.5364990234375
5.10329723358154 -0.5364990234375
5.10330772399902 -0.5364990234375
5.10512828826904 -0.53759765625
5.10597324371338 -0.537841796875
5.10642194747925 -0.537841796875
5.1072473526001 -0.537872314453125
5.10730838775635 -0.537872314453125
5.10758638381958 -0.537872314453125
5.10789823532104 -0.53790283203125
5.10802364349365 -0.53790283203125
5.10817909240723 -0.53790283203125
5.10825729370117 -0.53790283203125
5.10904836654663 -0.53790283203125
5.10909223556519 -0.537933349609375
5.10971689224243 -0.537933349609375
5.10976076126099 -0.537933349609375
5.10979127883911 -0.5379638671875
5.10988569259644 -0.5379638671875
5.1099967956543 -0.5379638671875
5.11026954650879 -0.5379638671875
5.11041784286499 -0.5379638671875
5.1107006072998 -0.5379638671875
5.11105728149414 -0.5379638671875
5.11121559143066 -0.5379638671875
5.11137342453003 -0.537994384765625
5.11142063140869 -0.537994384765625
5.11154127120972 -0.537994384765625
5.11161518096924 -0.537994384765625
5.11167573928833 -0.537994384765625
5.11178636550903 -0.537994384765625
5.11179685592651 -0.537994384765625
5.112464427948 -0.53802490234375
5.11249780654907 -0.53802490234375
5.11289644241333 -0.538055419921875
5.11312770843506 -0.538055419921875
5.11340856552124 -0.538055419921875
5.11387968063354 -0.5380859375
5.11436748504639 -0.5380859375
5.11479091644287 -0.5380859375
5.11490440368652 -0.538116455078125
5.11530113220215 -0.538116455078125
5.11538743972778 -0.538116455078125
5.11561393737793 -0.53814697265625
5.11605310440063 -0.538177490234375
5.11606597900391 -0.538177490234375
5.11624240875244 -0.538177490234375
5.11653804779053 -0.538177490234375
5.11684322357178 -0.5382080078125
5.11686325073242 -0.5382080078125
5.11691951751709 -0.5382080078125
5.11707544326782 -0.5382080078125
5.117112159729 -0.5382080078125
5.11743354797363 -0.5382080078125
5.11793041229248 -0.538238525390625
5.11798667907715 -0.538238525390625
5.11813879013062 -0.53826904296875
5.11814546585083 -0.53826904296875
5.11824464797974 -0.53826904296875
5.11864185333252 -0.53826904296875
5.11905765533447 -0.53826904296875
5.11918306350708 -0.53826904296875
5.1193151473999 -0.538299560546875
5.11945056915283 -0.538299560546875
5.11946725845337 -0.538299560546875
5.11996793746948 -0.538299560546875
5.12016248703003 -0.538299560546875
5.12093257904053 -0.538330078125
5.12096834182739 -0.538330078125
5.121169090271 -0.538330078125
5.12147760391235 -0.538330078125
5.12171411514282 -0.538360595703125
5.12172412872314 -0.538360595703125
5.12275648117065 -0.538604736328125
5.12304449081421 -0.538665771484375
5.12316560745239 -0.538665771484375
5.12346935272217 -0.538665771484375
5.12381887435913 -0.538665771484375
5.12400197982788 -0.538665771484375
5.12445545196533 -0.538665771484375
5.12497043609619 -0.5386962890625
5.12537717819214 -0.5386962890625
5.12544870376587 -0.5386962890625
5.12561130523682 -0.5386962890625
5.12662172317505 -0.5386962890625
5.12692308425903 -0.538726806640625
5.12698173522949 -0.538726806640625
5.12730550765991 -0.538726806640625
5.12737035751343 -0.538726806640625
5.12750339508057 -0.538726806640625
5.12751960754395 -0.538726806640625
5.12766170501709 -0.538726806640625
5.12774610519409 -0.53875732421875
5.12781715393066 -0.53875732421875
5.12789154052734 -0.53875732421875
5.12801122665405 -0.53875732421875
5.12822151184082 -0.53875732421875
5.1285252571106 -0.538787841796875
5.12855768203735 -0.538787841796875
5.12869310379028 -0.538787841796875
5.12893533706665 -0.538787841796875
5.1290807723999 -0.538787841796875
5.12921905517578 -0.538787841796875
5.12935781478882 -0.538818359375
5.12953186035156 -0.538818359375
5.12957048416138 -0.538818359375
5.12963533401489 -0.538818359375
5.13010835647583 -0.538818359375
5.13028860092163 -0.538818359375
5.13043689727783 -0.538848876953125
5.13052654266357 -0.538848876953125
5.13070344924927 -0.538848876953125
5.13083553314209 -0.538848876953125
5.13149356842041 -0.538848876953125
5.13174676895142 -0.538848876953125
5.13182687759399 -0.538848876953125
5.13190078735352 -0.538848876953125
5.1320481300354 -0.53887939453125
5.13214111328125 -0.53887939453125
5.13222122192383 -0.53887939453125
5.13227558135986 -0.53887939453125
5.13236522674561 -0.53887939453125
5.13244867324829 -0.53887939453125
5.13253498077393 -0.53887939453125
5.13254451751709 -0.53887939453125
5.13271760940552 -0.538909912109375
5.13274955749512 -0.538909912109375
5.13285493850708 -0.538909912109375
5.13295745849609 -0.538909912109375
5.13309478759766 -0.538909912109375
5.13324499130249 -0.538909912109375
5.13338565826416 -0.538909912109375
5.13359022140503 -0.538909912109375
5.13368892669678 -0.538909912109375
5.1338677406311 -0.5389404296875
5.13387727737427 -0.5389404296875
5.13408470153809 -0.5389404296875
5.13462018966675 -0.53900146484375
5.13470268249512 -0.53900146484375
5.13496732711792 -0.53900146484375
5.13504981994629 -0.53900146484375
5.13512945175171 -0.53900146484375
5.13534259796143 -0.539031982421875
5.13542222976685 -0.539031982421875
5.13587951660156 -0.539031982421875
5.13647651672363 -0.5390625
5.13649225234985 -0.5390625
5.13664436340332 -0.5390625
5.1368408203125 -0.539093017578125
5.13685035705566 -0.539093017578125
5.13691377639771 -0.539093017578125
5.13705968856812 -0.539093017578125
5.1370849609375 -0.539093017578125
5.13759756088257 -0.5391845703125
5.13788223266602 -0.539215087890625
5.13794898986816 -0.539215087890625
5.13839101791382 -0.539215087890625
5.13840675354004 -0.539215087890625
5.13863086700439 -0.53924560546875
5.13899707794189 -0.539276123046875
5.13912630081177 -0.539276123046875
5.13923978805542 -0.539276123046875
5.13928365707397 -0.539276123046875
5.13951683044434 -0.539276123046875
5.1397533416748 -0.539276123046875
5.13976907730103 -0.539276123046875
5.13996076583862 -0.539276123046875
5.14008665084839 -0.539306640625
5.14010238647461 -0.539306640625
5.14033508300781 -0.539306640625
5.14049530029297 -0.539306640625
5.14067459106445 -0.539306640625
5.14085674285889 -0.539306640625
5.1410984992981 -0.539306640625
5.14124917984009 -0.539306640625
5.14127111434937 -0.539306640625
5.14133358001709 -0.539337158203125
5.14155960083008 -0.539337158203125
5.14170074462891 -0.539337158203125
5.14194202423096 -0.539337158203125
5.14215803146362 -0.539337158203125
5.14229869842529 -0.539337158203125
5.14250516891479 -0.539337158203125
5.14301490783691 -0.53936767578125
5.14303970336914 -0.53936767578125
5.14318656921387 -0.53936767578125
5.14319610595703 -0.53936767578125
5.14336156845093 -0.53936767578125
5.14352369308472 -0.53936767578125
5.14385747909546 -0.53936767578125
5.14390754699707 -0.53936767578125
5.14425659179688 -0.53936767578125
5.1442723274231 -0.53936767578125
5.14444351196289 -0.539398193359375
5.14445877075195 -0.539398193359375
5.14450263977051 -0.539398193359375
5.14458990097046 -0.539398193359375
5.14488840103149 -0.539398193359375
5.1450252532959 -0.539398193359375
5.14506912231445 -0.539398193359375
5.14528942108154 -0.539398193359375
5.14535474777222 -0.539398193359375
5.14536428451538 -0.539398193359375
5.14548540115356 -0.539398193359375
5.1457371711731 -0.5394287109375
5.14579916000366 -0.539459228515625
5.14600086212158 -0.539459228515625
5.14609384536743 -0.539459228515625
5.14619016647339 -0.539459228515625
5.14620542526245 -0.539459228515625
5.14648771286011 -0.539459228515625
5.14665508270264 -0.539459228515625
5.14679765701294 -0.53948974609375
5.14702367782593 -0.53948974609375
5.14706373214722 -0.53948974609375
5.14713191986084 -0.53948974609375
5.14720630645752 -0.53948974609375
5.14721536636353 -0.53948974609375
5.14826345443726 -0.539764404296875
5.14857482910156 -0.539794921875
5.1489200592041 -0.539794921875
5.14920663833618 -0.539794921875
5.14923763275146 -0.539794921875
5.1493763923645 -0.539794921875
5.14951181411743 -0.539794921875
5.1496376991272 -0.539825439453125
5.14983177185059 -0.539825439453125
5.14994239807129 -0.539825439453125
5.14994239807129 -0.539825439453125
5.15011739730835 -0.539825439453125
5.15011739730835 -0.539825439453125
5.1502833366394 -0.539825439453125
5.1502833366394 -0.539825439453125
5.15046453475952 -0.539825439453125
5.15046453475952 -0.539825439453125
5.15051698684692 -0.539825439453125
5.15058135986328 -0.539825439453125
5.15064573287964 -0.539825439453125
5.15068578720093 -0.539825439453125
5.15075969696045 -0.539825439453125
5.15086078643799 -0.539825439453125
5.15180492401123 -0.539825439453125
5.15193653106689 -0.53985595703125
5.15196704864502 -0.53985595703125
5.15219068527222 -0.53985595703125
5.15219974517822 -0.53985595703125
5.15222406387329 -0.53985595703125
5.15222406387329 -0.53985595703125
5.15227937698364 -0.53985595703125
5.15233421325684 -0.53985595703125
5.15285062789917 -0.53985595703125
5.1530065536499 -0.53985595703125
5.15340042114258 -0.539886474609375
5.1534366607666 -0.539886474609375
5.15347957611084 -0.539886474609375
5.15358018875122 -0.539886474609375
5.15365648269653 -0.539886474609375
5.15397024154663 -0.539886474609375
5.15408611297607 -0.539886474609375
5.15411043167114 -0.539886474609375
5.15412855148315 -0.539886474609375
5.15414714813232 -0.539886474609375
5.15414714813232 -0.539886474609375
5.15423536300659 -0.539886474609375
5.15429306030273 -0.539886474609375
5.1543173789978 -0.539886474609375
5.15478610992432 -0.5399169921875
5.15519618988037 -0.5399169921875
5.15521764755249 -0.5399169921875
5.15524196624756 -0.5399169921875
5.15544843673706 -0.5399169921875
5.15553951263428 -0.5399169921875
5.15594625473022 -0.5399169921875
5.15613412857056 -0.5399169921875
5.15632200241089 -0.5399169921875
5.15633726119995 -0.5399169921875
5.15668821334839 -0.5399169921875
5.15673398971558 -0.5399169921875
5.15681552886963 -0.5399169921875
5.15684270858765 -0.539947509765625
5.15685176849365 -0.539947509765625
5.15686988830566 -0.539947509765625
5.1569881439209 -0.539947509765625
5.15706348419189 -0.539947509765625
5.15742969512939 -0.539947509765625
5.15752935409546 -0.539947509765625
5.15758991241455 -0.539947509765625
5.15759897232056 -0.539947509765625
5.15764713287354 -0.539947509765625
5.15791893005371 -0.539947509765625
5.15793418884277 -0.53997802734375
5.15802478790283 -0.53997802734375
5.15814828872681 -0.53997802734375
5.15820264816284 -0.53997802734375
5.15828990936279 -0.53997802734375
5.15830516815186 -0.53997802734375
5.15841054916382 -0.53997802734375
5.15847730636597 -0.53997802734375
5.15857982635498 -0.53997802734375
5.15859460830688 -0.53997802734375
5.15859460830688 -0.53997802734375
5.15873336791992 -0.53997802734375
5.15889883041382 -0.53997802734375
5.15892934799194 -0.53997802734375
5.15893793106079 -0.53997802734375
5.15927839279175 -0.53997802734375
5.1592903137207 -0.53997802734375
5.15942001342773 -0.53997802734375
5.15943479537964 -0.53997802734375
5.15949201583862 -0.53997802734375
5.15958213806152 -0.53997802734375
5.15958213806152 -0.53997802734375
5.15966033935547 -0.540008544921875
5.15967226028442 -0.540008544921875
5.15975952148438 -0.540008544921875
5.16003608703613 -0.540008544921875
5.16003608703613 -0.540008544921875
5.16010522842407 -0.540008544921875
5.16015338897705 -0.540008544921875
5.16028833389282 -0.540008544921875
5.16031265258789 -0.540008544921875
5.16048336029053 -0.540008544921875
5.16049861907959 -0.540008544921875
};
\addplot [ultra thick, blue]
table {%
-inf 0
0 -3.0517578125e-05
0 -3.0517578125e-05
0 -6.103515625e-05
0.60206001996994 -0.00030517578125
0.778151273727417 -0.0003662109375
0.903090000152588 -0.00048828125
0.903090000152588 -0.00054931640625
0.954242527484894 -0.000579833984375
1.11394333839417 -0.000885009765625
1.20412003993988 -0.00115966796875
1.23044896125793 -0.00140380859375
1.30103003978729 -0.001617431640625
1.36172783374786 -0.001861572265625
1.38021123409271 -0.001983642578125
1.57978355884552 -0.0076904296875
1.69019603729248 -0.011322021484375
1.71600329875946 -0.011688232421875
1.75587487220764 -0.011993408203125
1.79239177703857 -0.01239013671875
1.80618000030518 -0.012542724609375
1.86923170089722 -0.013336181640625
1.87506127357483 -0.013427734375
1.90309000015259 -0.0135498046875
1.9344984292984 -0.013671875
1.94448268413544 -0.01373291015625
2.00432133674622 -0.014007568359375
2.00432133674622 -0.014068603515625
2.01283717155457 -0.014129638671875
2.02530574798584 -0.01422119140625
2.03342366218567 -0.014312744140625
2.05307841300964 -0.014404296875
2.06445789337158 -0.0146484375
2.07188200950623 -0.01470947265625
2.07918119430542 -0.014801025390625
2.09690999984741 -0.014862060546875
2.14921903610229 -0.01519775390625
2.16435289382935 -0.015533447265625
2.18752074241638 -0.015838623046875
2.19312453269958 -0.01593017578125
2.19865703582764 -0.01611328125
2.21218752861023 -0.01641845703125
2.21484375 -0.01654052734375
2.23044896125793 -0.017242431640625
2.2764618396759 -0.0194091796875
2.27875351905823 -0.01995849609375
2.2810332775116 -0.020172119140625
2.28780174255371 -0.0205078125
2.290034532547 -0.020843505859375
2.29225611686707 -0.02105712890625
2.33445382118225 -0.025482177734375
2.34830474853516 -0.027252197265625
2.35218262672424 -0.027923583984375
2.35793495178223 -0.028594970703125
2.37291193008423 -0.02923583984375
2.380211353302 -0.02972412109375
2.39269685745239 -0.03070068359375
2.39619922637939 -0.031005859375
2.41830134391785 -0.031646728515625
2.44870638847351 -0.0323486328125
2.45788192749023 -0.032806396484375
2.47275638580322 -0.03448486328125
2.50105929374695 -0.03570556640625
2.5250449180603 -0.037384033203125
2.55145001411438 -0.0400390625
2.5717089176178 -0.0416259765625
2.57634139060974 -0.0426025390625
2.59659719467163 -0.046417236328125
2.60314440727234 -0.047088623046875
2.6063814163208 -0.04779052734375
2.64345264434814 -0.05450439453125
2.65224623680115 -0.05792236328125
2.67117285728455 -0.061126708984375
2.69284701347351 -0.06378173828125
2.71180725097656 -0.069610595703125
2.74585509300232 -0.07501220703125
2.7839035987854 -0.08135986328125
2.81557774543762 -0.093597412109375
2.85793519020081 -0.10888671875
2.88422870635986 -0.123321533203125
2.9074113368988 -0.130035400390625
2.91222214698792 -0.131439208984375
2.92788338661194 -0.1326904296875
2.94743371009827 -0.1337890625
2.95999479293823 -0.134124755859375
2.97726631164551 -0.13470458984375
2.97909283638 -0.13507080078125
2.99607372283936 -0.1370849609375
3.0056095123291 -0.137603759765625
3.03181219100952 -0.140655517578125
3.03622961044312 -0.141357421875
3.05384635925293 -0.142303466796875
3.06557965278625 -0.14361572265625
3.07845687866211 -0.1444091796875
3.09447121620178 -0.148651123046875
3.11494445800781 -0.154815673828125
3.12254357337952 -0.156890869140625
3.13065528869629 -0.158660888671875
3.14736700057983 -0.1610107421875
3.15624618530273 -0.162811279296875
3.15956711769104 -0.16387939453125
3.18012595176697 -0.1700439453125
3.18920946121216 -0.172210693359375
3.19284605979919 -0.173126220703125
3.2140486240387 -0.187042236328125
3.22737240791321 -0.194793701171875
3.2462522983551 -0.2044677734375
3.26316237449646 -0.209228515625
3.26974630355835 -0.2117919921875
3.29578685760498 -0.2293701171875
3.30941724777222 -0.260223388671875
3.32448816299438 -0.27667236328125
3.32878708839417 -0.28643798828125
3.34458875656128 -0.294830322265625
3.34947180747986 -0.29888916015625
3.36002516746521 -0.30438232421875
3.36380004882812 -0.306732177734375
3.36810088157654 -0.30841064453125
3.38093447685242 -0.3209228515625
3.38596367835999 -0.32550048828125
3.39339971542358 -0.327606201171875
3.39759254455566 -0.3292236328125
3.41043972969055 -0.3355712890625
3.41514039039612 -0.33819580078125
3.42209720611572 -0.3436279296875
3.42699885368347 -0.3460693359375
3.43392968177795 -0.3489990234375
3.43616271018982 -0.3505859375
3.44247984886169 -0.355621337890625
3.45239973068237 -0.357177734375
3.4569730758667 -0.362213134765625
3.46179866790771 -0.36383056640625
3.46523404121399 -0.36474609375
3.47348690032959 -0.36883544921875
3.47654175758362 -0.3704833984375
3.48258781433105 -0.372100830078125
3.48897361755371 -0.3763427734375
3.49554443359375 -0.379180908203125
3.50201725959778 -0.381744384765625
3.51108074188232 -0.3897705078125
3.51375007629395 -0.39276123046875
3.52465581893921 -0.4044189453125
3.52621006965637 -0.407867431640625
3.53339076042175 -0.4112548828125
3.53504085540771 -0.412017822265625
3.54270100593567 -0.422027587890625
3.54851222038269 -0.4248046875
3.55254650115967 -0.425872802734375
3.55642318725586 -0.42669677734375
3.56169748306274 -0.431365966796875
3.56714415550232 -0.43212890625
3.57100963592529 -0.433624267578125
3.57680177688599 -0.438995361328125
3.57909727096558 -0.4404296875
3.58342552185059 -0.44207763671875
3.58804750442505 -0.445648193359375
3.59428215026855 -0.451507568359375
3.59659719467163 -0.4532470703125
3.60031938552856 -0.4541015625
3.60184288024902 -0.45477294921875
3.6084189414978 -0.458251953125
3.61710524559021 -0.4595947265625
3.61888456344604 -0.46044921875
3.62169551849365 -0.4615478515625
3.62562108039856 -0.4622802734375
3.62859320640564 -0.46319580078125
3.63387227058411 -0.465606689453125
3.63518214225769 -0.4671630859375
3.64048147201538 -0.468353271484375
3.64532399177551 -0.46923828125
3.6472852230072 -0.470184326171875
3.64943218231201 -0.470611572265625
3.65676879882812 -0.473388671875
3.65925049781799 -0.474609375
3.66152882575989 -0.475433349609375
3.66567468643188 -0.477020263671875
3.66866540908813 -0.4788818359375
3.67135810852051 -0.47991943359375
3.67815399169922 -0.488525390625
3.68187403678894 -0.490875244140625
3.68529367446899 -0.49169921875
3.68636798858643 -0.492156982421875
3.6895751953125 -0.493255615234375
3.69214153289795 -0.49365234375
3.69661855697632 -0.49468994140625
3.69879627227783 -0.4952392578125
3.70217204093933 -0.49542236328125
3.70294713973999 -0.495697021484375
3.70475101470947 -0.49627685546875
3.70799565315247 -0.496856689453125
3.70850586891174 -0.49700927734375
3.7105405330658 -0.49810791015625
3.71264982223511 -0.498870849609375
3.71424579620361 -0.499847412109375
3.71692109107971 -0.50006103515625
3.71800327301025 -0.5003662109375
3.71850180625916 -0.50048828125
3.72073793411255 -0.50067138671875
3.72106838226318 -0.500823974609375
3.72329139709473 -0.501312255859375
3.72411203384399 -0.501556396484375
3.72680878639221 -0.502349853515625
3.72916483879089 -0.50396728515625
3.73287606239319 -0.504974365234375
3.73551917076111 -0.50537109375
3.73591804504395 -0.5054931640625
3.739018201828 -0.507476806640625
3.74091506004333 -0.50811767578125
3.74178171157837 -0.508270263671875
3.7428822517395 -0.508514404296875
3.74327445030212 -0.508636474609375
3.74476218223572 -0.508819580078125
3.74624490737915 -0.50897216796875
3.74686765670776 -0.509124755859375
3.74756717681885 -0.50921630859375
3.75066256523132 -0.5108642578125
3.75120210647583 -0.51104736328125
3.75212526321411 -0.51123046875
3.75281643867493 -0.5113525390625
3.75495958328247 -0.51165771484375
3.75564622879028 -0.511810302734375
3.75617957115173 -0.51190185546875
3.75769972801208 -0.5120849609375
3.75928997993469 -0.512359619140625
3.75974345207214 -0.51251220703125
3.76140165328979 -0.512725830078125
3.76297855377197 -0.5128173828125
3.76380228996277 -0.513092041015625
3.76454973220825 -0.51318359375
3.76492309570312 -0.513275146484375
3.76663589477539 -0.513397216796875
3.76708173751831 -0.51348876953125
3.76834201812744 -0.513702392578125
3.76863813400269 -0.513763427734375
3.7706310749054 -0.514556884765625
3.77107286453247 -0.5146484375
3.77305459976196 -0.514862060546875
3.77342081069946 -0.51495361328125
3.77371335029602 -0.5150146484375
3.77422499656677 -0.51507568359375
3.77568316459656 -0.515228271484375
3.7780065536499 -0.516265869140625
3.77901887893677 -0.516326904296875
3.78038930892944 -0.516387939453125
3.78182721138 -0.51690673828125
3.78383207321167 -0.51708984375
3.78418922424316 -0.517242431640625
3.7846884727478 -0.51727294921875
3.78483128547668 -0.517303466796875
3.78511619567871 -0.51739501953125
3.78859257698059 -0.518829345703125
3.78986263275146 -0.51898193359375
3.78993320465088 -0.51904296875
3.79162049293518 -0.519317626953125
3.79183101654053 -0.519378662109375
3.79594945907593 -0.520782470703125
3.79643559455872 -0.52142333984375
3.79692101478577 -0.521484375
3.79747533798218 -0.5216064453125
3.79830527305603 -0.52166748046875
3.80023574829102 -0.522064208984375
3.80037331581116 -0.522125244140625
3.80085444450378 -0.52215576171875
3.80386662483215 -0.52288818359375
3.80413937568665 -0.5230712890625
3.80590844154358 -0.523284912109375
3.80611205101013 -0.5233154296875
3.80665469169617 -0.52337646484375
3.80672240257263 -0.523406982421875
3.80814337730408 -0.523529052734375
3.80814337730408 -0.523590087890625
3.8084135055542 -0.52362060546875
3.80854845046997 -0.523681640625
3.81130695343018 -0.52520751953125
3.81164193153381 -0.525299072265625
3.81318044662476 -0.525390625
3.81331396102905 -0.525390625
3.81418108940125 -0.52557373046875
3.8144474029541 -0.525604248046875
3.8144474029541 -0.525634765625
3.81657266616821 -0.525848388671875
3.81683754920959 -0.525909423828125
3.81782960891724 -0.5260009765625
3.81796169281006 -0.526031494140625
3.8182258605957 -0.526092529296875
3.81835794448853 -0.526123046875
3.81868767738342 -0.526153564453125
3.81875348091125 -0.52618408203125
3.82105469703674 -0.526458740234375
3.82118582725525 -0.5264892578125
3.82151341438293 -0.526611328125
3.82242965698242 -0.526702880859375
3.82288694381714 -0.526763916015625
3.8238000869751 -0.526824951171875
3.82406067848206 -0.526885986328125
3.82484149932861 -0.52691650390625
3.82497143745422 -0.526947021484375
3.82503652572632 -0.5269775390625
3.83039617538452 -0.530029296875
3.83084511756897 -0.530548095703125
3.83238124847412 -0.530548095703125
3.83257269859314 -0.530609130859375
3.83282804489136 -0.5306396484375
3.83295583724976 -0.530670166015625
3.83301949501038 -0.53070068359375
3.83308339118958 -0.530731201171875
3.8331470489502 -0.53076171875
3.83333849906921 -0.530792236328125
3.83333849906921 -0.530792236328125
3.83333849906921 -0.53082275390625
3.83467507362366 -0.5308837890625
3.8347384929657 -0.530914306640625
3.83480215072632 -0.53094482421875
3.83505606651306 -0.530975341796875
3.8351194858551 -0.531005859375
3.8351194858551 -0.531036376953125
3.8351194858551 -0.531036376953125
3.83708310127258 -0.531463623046875
3.83727264404297 -0.531463623046875
3.83739900588989 -0.531524658203125
3.83771467208862 -0.53155517578125
3.83903789520264 -0.531585693359375
3.84035706520081 -0.531646728515625
3.84048247337341 -0.531646728515625
3.84054517745972 -0.53167724609375
3.84060788154602 -0.531707763671875
3.84092116355896 -0.531768798828125
3.84110903739929 -0.53179931640625
3.84110903739929 -0.531829833984375
3.84123420715332 -0.531829833984375
3.84167218208313 -0.5318603515625
3.84310817718506 -0.531951904296875
3.84310817718506 -0.531982421875
3.84323287010193 -0.532012939453125
3.84335732460022 -0.53204345703125
3.84360647201538 -0.53204345703125
3.84360647201538 -0.532073974609375
3.84366869926453 -0.532073974609375
3.84373092651367 -0.5321044921875
3.84385538101196 -0.5321044921875
3.8448498249054 -0.5322265625
3.84497404098511 -0.532257080078125
3.84559416770935 -0.532257080078125
3.84559416770935 -0.532257080078125
3.84769606590271 -0.53265380859375
3.84788107872009 -0.532684326171875
3.84788107872009 -0.532684326171875
3.84788107872009 -0.53271484375
3.84911203384399 -0.53271484375
3.8491735458374 -0.532745361328125
3.84929656982422 -0.5328369140625
3.84935808181763 -0.5328369140625
3.84966516494751 -0.532867431640625
3.85046243667603 -0.532867431640625
3.85046243667603 -0.53289794921875
3.85046243667603 -0.53289794921875
3.85046243667603 -0.53289794921875
3.85095238685608 -0.533050537109375
3.85095238685608 -0.533050537109375
3.85205268859863 -0.5330810546875
3.85241889953613 -0.533203125
3.8538806438446 -0.533203125
3.8538806438446 -0.533233642578125
3.85467028617859 -0.53326416015625
3.85479164123535 -0.53326416015625
3.85479164123535 -0.533294677734375
3.85485243797302 -0.533294677734375
3.85497379302979 -0.533294677734375
3.85497379302979 -0.5333251953125
3.85497379302979 -0.5333251953125
3.85497379302979 -0.533355712890625
3.85648727416992 -0.5335693359375
3.85660815238953 -0.533599853515625
3.85690999031067 -0.533660888671875
3.85811591148376 -0.533660888671875
3.85817623138428 -0.53369140625
3.85823631286621 -0.53369140625
3.85835671424866 -0.533721923828125
3.85841679573059 -0.533721923828125
3.8584771156311 -0.53375244140625
3.85853719711304 -0.53375244140625
3.85859727859497 -0.533782958984375
3.85859727859497 -0.533782958984375
3.85859727859497 -0.533782958984375
3.85877776145935 -0.5338134765625
3.85883784294128 -0.5338134765625
3.85937857627869 -0.53387451171875
3.85937857627869 -0.53387451171875
3.85955858230591 -0.533966064453125
3.85985851287842 -0.533966064453125
3.86135506629944 -0.533966064453125
3.86135506629944 -0.53399658203125
3.86159420013428 -0.534088134765625
3.86165380477905 -0.534088134765625
3.8645703792572 -0.534759521484375
3.86498546600342 -0.534912109375
3.86646461486816 -0.534912109375
3.86670064926147 -0.534942626953125
3.86681890487671 -0.534942626953125
3.86687779426575 -0.53497314453125
3.8669958114624 -0.53497314453125
3.8669958114624 -0.535003662109375
3.86705493927002 -0.5350341796875
3.8671727180481 -0.5350341796875
3.86752653121948 -0.5350341796875
3.86758542060852 -0.535064697265625
3.86764430999756 -0.535064697265625
3.86923170089722 -0.53521728515625
3.86934900283813 -0.535247802734375
3.86964225769043 -0.535247802734375
3.86964225769043 -0.535247802734375
3.87028694152832 -0.5352783203125
3.870521068573 -0.535308837890625
3.87063789367676 -0.535308837890625
3.8707549571991 -0.53533935546875
3.87081336975098 -0.53533935546875
3.87081336975098 -0.53533935546875
3.87081336975098 -0.53533935546875
3.8729133605957 -0.53570556640625
3.872971534729 -0.535736083984375
3.87424993515015 -0.535919189453125
3.87465572357178 -0.53594970703125
3.87587118148804 -0.53594970703125
3.87592887878418 -0.535980224609375
3.8759868144989 -0.535980224609375
3.87621784210205 -0.535980224609375
3.87800455093384 -0.536285400390625
3.87932538986206 -0.536346435546875
3.87972640991211 -0.536346435546875
3.88007020950317 -0.536376953125
3.88018465042114 -0.536376953125
3.88029909133911 -0.536407470703125
3.8804132938385 -0.536407470703125
3.88115644454956 -0.53643798828125
3.88132762908936 -0.536468505859375
3.88138461112976 -0.536468505859375
3.88144159317017 -0.5364990234375
3.88326382637024 -0.5364990234375
3.88332056999207 -0.5364990234375
3.88354778289795 -0.536529541015625
3.88360476493835 -0.536529541015625
3.88366150856018 -0.536529541015625
3.88371825218201 -0.53656005859375
3.88377499580383 -0.53656005859375
3.88434219360352 -0.536590576171875
3.88434219360352 -0.536590576171875
3.88434219360352 -0.536590576171875
3.88439893722534 -0.536590576171875
3.88439893722534 -0.53662109375
3.88439893722534 -0.53662109375
3.88439893722534 -0.53662109375
3.88530468940735 -0.53668212890625
3.8853611946106 -0.53668212890625
3.8853611946106 -0.53668212890625
3.8853611946106 -0.53668212890625
3.88541769981384 -0.536712646484375
3.88665986061096 -0.53680419921875
3.88671636581421 -0.53680419921875
3.88705444335938 -0.536865234375
3.88722324371338 -0.536865234375
3.8875048160553 -0.536895751953125
3.88846039772034 -0.536895751953125
3.88846039772034 -0.536895751953125
3.88851642608643 -0.536895751953125
3.88862872123718 -0.53692626953125
3.88874101638794 -0.53692626953125
3.88885307312012 -0.53692626953125
3.89002966880798 -0.5369873046875
3.89019727706909 -0.5369873046875
3.89030933380127 -0.5369873046875
3.89036512374878 -0.5369873046875
3.89042091369629 -0.537017822265625
3.89326238632202 -0.53741455078125
3.8933732509613 -0.537445068359375
3.89359521865845 -0.5374755859375
3.89365077018738 -0.5374755859375
3.89370632171631 -0.5374755859375
3.89376163482666 -0.5374755859375
3.89381718635559 -0.537506103515625
3.89387273788452 -0.537506103515625
3.8939836025238 -0.537506103515625
3.89536714553833 -0.53753662109375
3.89536714553833 -0.53753662109375
3.89536714553833 -0.53753662109375
3.89536714553833 -0.53753662109375
3.89536714553833 -0.53753662109375
3.89553308486938 -0.53759765625
3.89553308486938 -0.53759765625
3.89553308486938 -0.53759765625
3.89757204055786 -0.537628173828125
3.89768195152283 -0.537628173828125
3.8977370262146 -0.53765869140625
3.89779186248779 -0.53765869140625
3.8980667591095 -0.537689208984375
3.89817643165588 -0.537689208984375
3.89828634262085 -0.537689208984375
3.89834117889404 -0.537689208984375
3.90031242370605 -0.5377197265625
3.90031242370605 -0.5377197265625
3.90031242370605 -0.5377197265625
3.90031242370605 -0.5377197265625
3.90053105354309 -0.5377197265625
3.90053105354309 -0.5377197265625
3.90058565139771 -0.537750244140625
3.90058565139771 -0.537750244140625
3.90064024925232 -0.537750244140625
3.90064024925232 -0.537750244140625
3.9008584022522 -0.537750244140625
3.9008584022522 -0.53778076171875
3.9008584022522 -0.53778076171875
3.90102219581604 -0.53778076171875
3.90113115310669 -0.537811279296875
3.9011857509613 -0.537811279296875
3.9011857509613 -0.537811279296875
3.9011857509613 -0.537811279296875
3.90194845199585 -0.53790283203125
3.90205717086792 -0.53790283203125
3.90227484703064 -0.53790283203125
3.90227484703064 -0.53790283203125
3.90227484703064 -0.53790283203125
3.90227484703064 -0.537933349609375
3.90227484703064 -0.537933349609375
3.9044451713562 -0.5380859375
3.90520191192627 -0.538116455078125
3.90520191192627 -0.538116455078125
3.90520191192627 -0.538116455078125
3.90525603294373 -0.538116455078125
3.90536403656006 -0.538116455078125
3.90536403656006 -0.53814697265625
3.90568804740906 -0.53814697265625
3.90687346458435 -0.538177490234375
3.90692734718323 -0.538177490234375
3.90730381011963 -0.5382080078125
3.9074113368988 -0.5382080078125
3.90751886367798 -0.5382080078125
3.90768003463745 -0.538238525390625
3.90778732299805 -0.538238525390625
3.90778732299805 -0.538238525390625
3.90805578231812 -0.538238525390625
3.90816330909729 -0.538238525390625
3.90816330909729 -0.538238525390625
3.90816330909729 -0.538238525390625
3.90816330909729 -0.53826904296875
3.90816330909729 -0.53826904296875
3.90816330909729 -0.53826904296875
3.90816330909729 -0.53826904296875
3.90816330909729 -0.53826904296875
3.90966296195984 -0.538330078125
3.90966296195984 -0.538330078125
3.90966296195984 -0.538330078125
3.90966296195984 -0.538330078125
3.9104642868042 -0.53839111328125
3.91051769256592 -0.53839111328125
3.91259407997131 -0.538421630859375
3.91275334358215 -0.538421630859375
3.91285943984985 -0.5384521484375
3.91296553611755 -0.5384521484375
3.91307163238525 -0.5384521484375
3.91307163238525 -0.5384521484375
3.91307163238525 -0.5384521484375
3.91328382492065 -0.5384521484375
3.91413140296936 -0.538543701171875
3.91418433189392 -0.538543701171875
3.91592717170715 -0.53857421875
3.91597986221313 -0.53857421875
3.91603255271912 -0.53857421875
3.91613793373108 -0.53857421875
3.91613793373108 -0.53857421875
3.916348695755 -0.538604736328125
3.91640138626099 -0.538604736328125
3.91661190986633 -0.538604736328125
3.91661190986633 -0.538604736328125
3.91666436195374 -0.538604736328125
3.9168221950531 -0.538604736328125
3.9168221950531 -0.538604736328125
3.9177680015564 -0.538665771484375
3.9177680015564 -0.5386962890625
3.91923499107361 -0.5386962890625
3.91933965682983 -0.5386962890625
3.92007112503052 -0.5386962890625
3.92012333869934 -0.5386962890625
3.92038416862488 -0.538726806640625
3.92048859596252 -0.538726806640625
3.92048859596252 -0.538726806640625
3.92059278488159 -0.538726806640625
3.92074918746948 -0.538726806640625
3.92080140113831 -0.53875732421875
3.92085361480713 -0.53875732421875
3.92090559005737 -0.53875732421875
3.9209578037262 -0.53875732421875
3.9209578037262 -0.53875732421875
3.9209578037262 -0.53875732421875
3.9209578037262 -0.53875732421875
3.921790599823 -0.538787841796875
3.921790599823 -0.538787841796875
3.9225697517395 -0.538787841796875
3.9225697517395 -0.538787841796875
3.9225697517395 -0.538787841796875
3.92515730857849 -0.53887939453125
3.92520880699158 -0.538909912109375
3.92531204223633 -0.538909912109375
3.92536377906799 -0.5389404296875
3.92546677589417 -0.5389404296875
3.92551827430725 -0.5389404296875
3.92551827430725 -0.5389404296875
3.92572450637817 -0.5389404296875
3.92572450637817 -0.5389404296875
3.92572450637817 -0.5389404296875
3.92577600479126 -0.5389404296875
3.92582750320435 -0.5389404296875
3.92613649368286 -0.538970947265625
3.92613649368286 -0.538970947265625
3.92613649368286 -0.538970947265625
3.92613649368286 -0.538970947265625
3.92613649368286 -0.538970947265625
3.92685675621033 -0.538970947265625
3.92685675621033 -0.538970947265625
3.92685675621033 -0.538970947265625
3.92695951461792 -0.538970947265625
3.92695951461792 -0.538970947265625
3.92695951461792 -0.53900146484375
3.92716503143311 -0.53900146484375
3.92716503143311 -0.53900146484375
3.92716503143311 -0.53900146484375
3.92757558822632 -0.53900146484375
3.92844700813293 -0.539031982421875
3.92844700813293 -0.539031982421875
3.92849826812744 -0.539031982421875
3.92849826812744 -0.539031982421875
3.92849826812744 -0.539031982421875
3.9293167591095 -0.5390625
3.9293167591095 -0.5390625
3.92947006225586 -0.5390625
3.92947006225586 -0.5390625
3.92947006225586 -0.5390625
3.92967438697815 -0.539093017578125
3.92967438697815 -0.539093017578125
3.93003153800964 -0.539093017578125
3.93003153800964 -0.539093017578125
3.93003153800964 -0.539093017578125
3.93110179901123 -0.539093017578125
3.93110179901123 -0.539093017578125
3.93140697479248 -0.53912353515625
3.93140697479248 -0.53912353515625
3.93140697479248 -0.53912353515625
3.93140697479248 -0.53912353515625
3.93140697479248 -0.53912353515625
3.93155956268311 -0.53912353515625
3.93186450004578 -0.539154052734375
3.93186450004578 -0.539154052734375
3.93186450004578 -0.539154052734375
3.93272733688354 -0.539154052734375
3.93272733688354 -0.539154052734375
3.93272733688354 -0.539154052734375
3.93348717689514 -0.5391845703125
3.93348717689514 -0.5391845703125
3.93348717689514 -0.5391845703125
3.93348717689514 -0.5391845703125
3.93348717689514 -0.5391845703125
3.9336895942688 -0.539215087890625
3.9336895942688 -0.539215087890625
3.93464994430542 -0.539215087890625
3.93475079536438 -0.539215087890625
3.93475079536438 -0.539215087890625
3.93480134010315 -0.53924560546875
3.93480134010315 -0.53924560546875
3.93480134010315 -0.53924560546875
3.93726706504822 -0.53936767578125
3.93736743927002 -0.53936767578125
3.93736743927002 -0.53936767578125
3.93736743927002 -0.53936767578125
3.93911981582642 -0.53948974609375
3.93926954269409 -0.53955078125
3.9393196105957 -0.53955078125
3.93936944007874 -0.539581298828125
3.94016766548157 -0.539581298828125
3.9402174949646 -0.539581298828125
3.94026732444763 -0.539581298828125
3.94041681289673 -0.539581298828125
3.94041681289673 -0.539581298828125
3.94041681289673 -0.539581298828125
3.94051647186279 -0.539581298828125
3.94051647186279 -0.53961181640625
3.94051647186279 -0.53961181640625
3.94051647186279 -0.53961181640625
3.94076538085938 -0.53961181640625
3.94076538085938 -0.53961181640625
3.94081521034241 -0.53961181640625
3.94101428985596 -0.53961181640625
3.94101428985596 -0.53961181640625
3.94101428985596 -0.53961181640625
3.94101428985596 -0.53961181640625
3.94101428985596 -0.53961181640625
3.94101428985596 -0.53961181640625
3.94111371040344 -0.539642333984375
3.94116353988647 -0.539642333984375
3.94175982475281 -0.539642333984375
3.94175982475281 -0.539642333984375
3.94175982475281 -0.539642333984375
3.9443838596344 -0.53985595703125
3.94448256492615 -0.53997802734375
3.9445812702179 -0.53997802734375
3.94482803344727 -0.53997802734375
3.94487738609314 -0.53997802734375
3.94492650032043 -0.53997802734375
3.94497585296631 -0.53997802734375
3.94502520561218 -0.53997802734375
3.94507455825806 -0.53997802734375
3.94512367248535 -0.53997802734375
3.94537019729614 -0.53997802734375
3.94537019729614 -0.53997802734375
3.94546866416931 -0.53997802734375
3.94546866416931 -0.53997802734375
3.94551777839661 -0.540008544921875
3.94556713104248 -0.540008544921875
3.94561624526978 -0.540008544921875
3.94561624526978 -0.540008544921875
3.94561624526978 -0.540008544921875
3.94561624526978 -0.540008544921875
3.94561624526978 -0.540008544921875
3.94561624526978 -0.540008544921875
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{O3}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.439251708984375, ymax=0.020916748046875,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c13)}
]
\addplot [ultra thick, brown, dashed]
table {%
2.27415776252747 -1.52587890625e-05
2.50515007972717 -0.00048828125
2.7817554473877 -0.0018768310546875
2.95230793952942 -0.0041046142578125
3.01494026184082 -0.004852294921875
3.05346250534058 -0.00543212890625
3.10243368148804 -0.0065155029296875
3.21351766586304 -0.0076751708984375
3.25719833374023 -0.00787353515625
3.26292538642883 -0.0079193115234375
3.27044582366943 -0.0079803466796875
3.29380440711975 -0.008209228515625
3.31344532966614 -0.0082855224609375
3.38165640830994 -0.0084686279296875
3.40942597389221 -0.008636474609375
3.42373728752136 -0.008697509765625
3.46879029273987 -0.00921630859375
3.49429368972778 -0.0095672607421875
3.52478551864624 -0.0097503662109375
3.56002616882324 -0.0105743408203125
3.58399176597595 -0.011077880859375
3.62179923057556 -0.012786865234375
3.62981724739075 -0.013946533203125
3.67209792137146 -0.0189056396484375
3.68726134300232 -0.019805908203125
3.71783685684204 -0.0205535888671875
3.73830485343933 -0.021514892578125
3.74865317344666 -0.0224151611328125
3.76589202880859 -0.0225677490234375
3.78103685379028 -0.0227508544921875
3.78986263275146 -0.02294921875
3.79733681678772 -0.0230712890625
3.80679035186768 -0.023223876953125
3.82471132278442 -0.0235748291015625
3.91163682937622 -0.0276031494140625
3.93876981735229 -0.040313720703125
4.00026035308838 -0.0539703369140625
4.05872964859009 -0.08203125
4.08841943740845 -0.110031127929688
4.119948387146 -0.124160766601562
4.13007640838623 -0.128402709960938
4.14317083358765 -0.1295166015625
4.15591287612915 -0.130081176757812
4.16696262359619 -0.130615234375
4.18754911422729 -0.134368896484375
4.19706010818481 -0.136001586914062
4.20811891555786 -0.136962890625
4.21587562561035 -0.137863159179688
4.22590351104736 -0.138809204101562
4.23610877990723 -0.139633178710938
4.24762964248657 -0.14239501953125
4.26202392578125 -0.146743774414062
4.27809000015259 -0.1513671875
4.28909826278687 -0.153594970703125
4.3261923789978 -0.167312622070312
4.33674001693726 -0.1739501953125
4.35470390319824 -0.180313110351562
4.37388610839844 -0.186294555664062
4.38733625411987 -0.190841674804688
4.40212392807007 -0.204971313476562
4.41328287124634 -0.21240234375
4.42301654815674 -0.218902587890625
4.42980051040649 -0.225234985351562
4.4389533996582 -0.235153198242188
4.44732856750488 -0.241287231445312
4.45256853103638 -0.245819091796875
4.46304130554199 -0.249954223632812
4.47240543365479 -0.255767822265625
4.48026561737061 -0.261993408203125
4.4929141998291 -0.268798828125
4.49803495407104 -0.270736694335938
4.50618028640747 -0.275558471679688
4.5126576423645 -0.280975341796875
4.51763153076172 -0.285629272460938
4.52280902862549 -0.288345336914062
4.52732038497925 -0.290191650390625
4.53261423110962 -0.292633056640625
4.5387749671936 -0.2952880859375
4.54130458831787 -0.2967529296875
4.54693746566772 -0.298446655273438
4.55213260650635 -0.301620483398438
4.55739879608154 -0.302932739257812
4.5631251335144 -0.303939819335938
4.56947946548462 -0.309661865234375
4.58101606369019 -0.318023681640625
4.58490753173828 -0.319747924804688
4.58932399749756 -0.32080078125
4.59455823898315 -0.321334838867188
4.60392332077026 -0.327880859375
4.60886812210083 -0.3292236328125
4.61576080322266 -0.330734252929688
4.61823654174805 -0.33154296875
4.63466882705688 -0.34808349609375
4.64013338088989 -0.354751586914062
4.64662933349609 -0.356781005859375
4.65003538131714 -0.357986450195312
4.6539454460144 -0.360198974609375
4.65820217132568 -0.363372802734375
4.66255950927734 -0.36614990234375
4.66713523864746 -0.36785888671875
4.67373037338257 -0.374893188476562
4.67755222320557 -0.378646850585938
4.68505191802979 -0.380279541015625
4.69360399246216 -0.383010864257812
4.69527149200439 -0.383880615234375
4.70122241973877 -0.386138916015625
4.70239591598511 -0.386520385742188
4.70550441741943 -0.38714599609375
4.70658111572266 -0.387420654296875
4.71228742599487 -0.390289306640625
4.71365833282471 -0.390823364257812
4.71822738647461 -0.392013549804688
4.71946382522583 -0.39251708984375
4.72119188308716 -0.39276123046875
4.72329950332642 -0.393753051757812
4.72448062896729 -0.394424438476562
4.7260913848877 -0.394760131835938
4.72866201400757 -0.395523071289062
4.7294807434082 -0.395843505859375
4.73060464859009 -0.396453857421875
4.73141956329346 -0.3966064453125
4.73367071151733 -0.397140502929688
4.73482370376587 -0.397293090820312
4.73634052276611 -0.397659301757812
4.73720836639404 -0.39794921875
4.73817014694214 -0.398086547851562
4.73942995071411 -0.398223876953125
4.73995208740234 -0.398300170898438
4.74339199066162 -0.401153564453125
4.74442577362061 -0.401580810546875
4.74502801895142 -0.4017333984375
4.74554300308228 -0.401824951171875
4.74611234664917 -0.401931762695312
4.74676656723022 -0.402053833007812
4.74711656570435 -0.402099609375
4.74789333343506 -0.4022216796875
4.74862194061279 -0.40228271484375
4.74936532974243 -0.402328491210938
4.75127124786377 -0.403366088867188
4.75174856185913 -0.403488159179688
4.75221729278564 -0.403533935546875
4.75346040725708 -0.404144287109375
4.75480699539185 -0.404495239257812
4.75540208816528 -0.404571533203125
4.75608062744141 -0.404632568359375
4.75652980804443 -0.404678344726562
4.75723648071289 -0.404769897460938
4.75777530670166 -0.404815673828125
4.75869989395142 -0.4049072265625
4.75930500030518 -0.404983520507812
4.76090478897095 -0.405593872070312
4.76115322113037 -0.405670166015625
4.7615818977356 -0.40570068359375
4.76335334777832 -0.406402587890625
4.76393699645996 -0.406463623046875
4.76430320739746 -0.406494140625
4.76501274108887 -0.40655517578125
4.76683664321899 -0.406814575195312
4.76709651947021 -0.4068603515625
4.76755666732788 -0.406890869140625
4.767897605896 -0.406936645507812
4.76825332641602 -0.406982421875
4.76863050460815 -0.407012939453125
4.76965045928955 -0.40716552734375
4.7702260017395 -0.407211303710938
4.77096223831177 -0.407272338867188
4.77136707305908 -0.407302856445312
4.77175664901733 -0.4073486328125
4.77234363555908 -0.407379150390625
4.77285671234131 -0.407440185546875
4.77298879623413 -0.407455444335938
4.77453136444092 -0.40838623046875
4.77485990524292 -0.408523559570312
4.77530479431152 -0.408615112304688
4.77558851242065 -0.408645629882812
4.77574157714844 -0.408676147460938
4.77707147598267 -0.40887451171875
4.77806425094604 -0.408920288085938
4.7783031463623 -0.408950805664062
4.77877330780029 -0.409042358398438
4.77933692932129 -0.409072875976562
4.77959632873535 -0.40911865234375
4.78012275695801 -0.409133911132812
4.78041076660156 -0.409149169921875
4.78077793121338 -0.4091796875
4.78112316131592 -0.409210205078125
4.78171968460083 -0.40924072265625
4.78191328048706 -0.409255981445312
4.78316020965576 -0.409698486328125
4.78376770019531 -0.40972900390625
4.78599834442139 -0.410308837890625
4.78650283813477 -0.410446166992188
4.78676557540894 -0.41046142578125
4.78690767288208 -0.410476684570312
4.78771543502808 -0.4105224609375
4.78792762756348 -0.410537719726562
4.78801965713501 -0.410552978515625
4.78829574584961 -0.410568237304688
4.78900909423828 -0.410675048828125
4.7894606590271 -0.410690307617188
4.78986263275146 -0.410720825195312
4.79001045227051 -0.410736083984375
4.79157161712646 -0.411163330078125
4.79192209243774 -0.411361694335938
4.79253196716309 -0.411392211914062
4.79357385635376 -0.411636352539062
4.79392290115356 -0.411666870117188
4.79451608657837 -0.411697387695312
4.79500341415405 -0.411712646484375
4.79546308517456 -0.411727905273438
4.79610919952393 -0.411758422851562
4.79621362686157 -0.411758422851562
4.79638719558716 -0.411773681640625
4.79683113098145 -0.411819458007812
4.79848480224609 -0.412399291992188
4.79866456985474 -0.4124755859375
4.79874706268311 -0.412490844726562
4.79883003234863 -0.412490844726562
4.79928541183472 -0.412582397460938
4.79990530014038 -0.412765502929688
4.80018758773804 -0.41278076171875
4.80075836181641 -0.412796020507812
4.80195903778076 -0.41302490234375
4.80215787887573 -0.413055419921875
4.80245208740234 -0.413070678710938
4.80266427993774 -0.4130859375
4.80357313156128 -0.413253784179688
4.80387353897095 -0.41326904296875
4.80421447753906 -0.413284301757812
4.80445289611816 -0.413314819335938
4.80517435073853 -0.413360595703125
4.80586099624634 -0.413375854492188
4.80604410171509 -0.413375854492188
4.80638360977173 -0.413406372070312
4.80679702758789 -0.413421630859375
4.80721712112427 -0.4134521484375
4.80737257003784 -0.413467407226562
4.80749464035034 -0.413482666015625
4.80798816680908 -0.413497924804688
4.80809593200684 -0.41351318359375
4.8081841468811 -0.41351318359375
4.8083324432373 -0.413528442382812
4.81027269363403 -0.414810180664062
4.81078338623047 -0.41497802734375
4.81101179122925 -0.41497802734375
4.81138038635254 -0.414993286132812
4.81154823303223 -0.415008544921875
4.8119101524353 -0.415008544921875
4.81205749511719 -0.415023803710938
4.81304693222046 -0.415054321289062
4.81312704086304 -0.415069580078125
4.81329393386841 -0.415084838867188
4.81363439559937 -0.415084838867188
4.81422758102417 -0.41510009765625
4.81432771682739 -0.415115356445312
4.81440734863281 -0.415115356445312
4.81451416015625 -0.415130615234375
4.81464052200317 -0.415145874023438
4.81473350524902 -0.415145874023438
4.81485319137573 -0.415176391601562
4.8150463104248 -0.415176391601562
4.81535196304321 -0.415191650390625
4.81561756134033 -0.415191650390625
4.81581687927246 -0.415206909179688
4.81629419326782 -0.415206909179688
4.81631422042847 -0.41522216796875
4.81713533401489 -0.415237426757812
4.81789588928223 -0.415298461914062
4.81814670562744 -0.415298461914062
4.81879329681396 -0.41534423828125
4.81883907318115 -0.415359497070312
4.81926727294922 -0.415374755859375
4.81949806213379 -0.415374755859375
4.82014894485474 -0.415390014648438
4.82031965255737 -0.415390014648438
4.8203330039978 -0.415390014648438
4.82066106796265 -0.415451049804688
4.82124471664429 -0.415481567382812
4.82129716873169 -0.415496826171875
4.82141542434692 -0.415496826171875
4.8215069770813 -0.415496826171875
4.82319355010986 -0.416397094726562
4.82394981384277 -0.416671752929688
4.82415199279785 -0.41668701171875
4.82446432113647 -0.416717529296875
4.82493877410889 -0.416717529296875
4.82525730133057 -0.416748046875
4.82608127593994 -0.416763305664062
4.82645702362061 -0.416763305664062
4.82659292221069 -0.416763305664062
4.82669019699097 -0.416778564453125
4.82676792144775 -0.416778564453125
4.82707166671753 -0.41680908203125
4.82739496231079 -0.41680908203125
4.82797002792358 -0.416839599609375
4.82814407348633 -0.416839599609375
4.82836961746216 -0.416839599609375
4.82884693145752 -0.416854858398438
4.82925891876221 -0.416854858398438
4.82967042922974 -0.416885375976562
4.82990169525146 -0.416885375976562
4.82997226715088 -0.416885375976562
4.83039617538452 -0.416900634765625
4.83043479919434 -0.416900634765625
4.83089637756348 -0.416915893554688
4.83120393753052 -0.41693115234375
4.8312873840332 -0.416946411132812
4.83179950714111 -0.416946411132812
4.83205509185791 -0.416961669921875
4.83265590667725 -0.416976928710938
4.83315992355347 -0.416976928710938
4.83342742919922 -0.416976928710938
4.83409643173218 -0.417007446289062
4.83412790298462 -0.417007446289062
4.83433818817139 -0.417007446289062
4.8353419303894 -0.417129516601562
4.83553218841553 -0.417129516601562
4.83555746078491 -0.417144775390625
4.83615303039551 -0.417160034179688
4.83636856079102 -0.417160034179688
4.83676052093506 -0.417160034179688
4.83683013916016 -0.417160034179688
4.83720970153809 -0.417190551757812
4.83761978149414 -0.417190551757812
4.83782815933228 -0.417205810546875
4.83790397644043 -0.417205810546875
4.83833885192871 -0.417205810546875
4.83851528167725 -0.417205810546875
4.83913230895996 -0.417251586914062
4.83918237686157 -0.417266845703125
4.83927059173584 -0.417266845703125
4.83936500549316 -0.417266845703125
4.84070205688477 -0.417404174804688
4.84155321121216 -0.41741943359375
4.84159708023071 -0.41741943359375
4.84197854995728 -0.41741943359375
4.84205961227417 -0.41741943359375
4.84234714508057 -0.41741943359375
4.84262180328369 -0.417434692382812
4.84288358688354 -0.417434692382812
4.84293985366821 -0.417434692382812
4.84317684173584 -0.417449951171875
4.84389877319336 -0.417465209960938
4.84466981887817 -0.417465209960938
4.84475040435791 -0.417465209960938
4.84485578536987 -0.41748046875
4.84492444992065 -0.41748046875
4.84502983093262 -0.41748046875
4.84518480300903 -0.41748046875
4.84593486785889 -0.417556762695312
4.84638643264771 -0.417556762695312
4.84654140472412 -0.417556762695312
4.84661531448364 -0.417556762695312
4.8468132019043 -0.417572021484375
4.84710359573364 -0.417572021484375
4.84718370437622 -0.417572021484375
4.8480658531189 -0.417617797851562
4.84825086593628 -0.417617797851562
4.84841060638428 -0.417617797851562
4.84860801696777 -0.417617797851562
4.84897708892822 -0.417617797851562
4.84940099716187 -0.417633056640625
4.84946250915527 -0.417633056640625
4.84960985183716 -0.417633056640625
};
\addplot [ultra thick, blue]
table {%
0.60206001996994 0
1.25527250766754 -0.0005645751953125
1.44715809822083 -0.00250244140625
1.53147888183594 -0.0035552978515625
1.59106457233429 -0.0047607421875
1.65321254730225 -0.006439208984375
1.66275787353516 -0.006744384765625
1.70757019519806 -0.0071868896484375
1.72427582740784 -0.0074920654296875
1.77085208892822 -0.007720947265625
1.77815127372742 -0.0078125
1.79239177703857 -0.00787353515625
1.79934048652649 -0.0079345703125
1.81291329860687 -0.0080108642578125
1.86332285404205 -0.008056640625
1.86332285404205 -0.0080718994140625
1.89762711524963 -0.008514404296875
1.90848505496979 -0.008636474609375
1.9344984292984 -0.0088653564453125
2.00432133674622 -0.0089874267578125
2.02530574798584 -0.00933837890625
2.04532289505005 -0.0095977783203125
2.12385153770447 -0.0130615234375
2.17026162147522 -0.01580810546875
2.18469142913818 -0.01739501953125
2.21218752861023 -0.0187225341796875
2.23044896125793 -0.0212554931640625
2.23552846908569 -0.021820068359375
2.25042009353638 -0.0224761962890625
2.25767850875854 -0.022735595703125
2.2764618396759 -0.0230712890625
2.32837963104248 -0.0246734619140625
2.35410833358765 -0.0261993408203125
2.37291193008423 -0.0286102294921875
2.38916611671448 -0.0311279296875
2.42488169670105 -0.04034423828125
2.52374649047852 -0.06365966796875
2.64147400856018 -0.09478759765625
2.67760705947876 -0.117019653320312
2.71264958381653 -0.125595092773438
2.72263383865356 -0.1280517578125
2.72916483879089 -0.128616333007812
2.7435097694397 -0.129165649414062
2.76042246818542 -0.129486083984375
2.7737865447998 -0.130111694335938
2.78247261047363 -0.130569458007812
2.79028511047363 -0.131118774414062
2.80071711540222 -0.131591796875
2.82801508903503 -0.133453369140625
2.8363242149353 -0.13409423828125
2.84010601043701 -0.134414672851562
2.88024187088013 -0.148696899414062
2.89265108108521 -0.156951904296875
2.91592717170715 -0.16033935546875
2.92890763282776 -0.162811279296875
2.98045778274536 -0.181472778320312
2.99431705474854 -0.194473266601562
3.01703333854675 -0.199371337890625
3.02571535110474 -0.201889038085938
3.05192399024963 -0.219635009765625
3.06929802894592 -0.230804443359375
3.08600378036499 -0.235214233398438
3.09933519363403 -0.240951538085938
3.12417817115784 -0.245361328125
3.13417720794678 -0.249282836914062
3.14612793922424 -0.253524780273438
3.15806078910828 -0.256820678710938
3.16375756263733 -0.261001586914062
3.18892860412598 -0.27691650390625
3.20276069641113 -0.282424926757812
3.20709562301636 -0.284088134765625
3.22089219093323 -0.288284301757812
3.23044896125793 -0.292205810546875
3.24600601196289 -0.2952880859375
3.25115132331848 -0.296920776367188
3.26054835319519 -0.300765991210938
3.27184152603149 -0.302017211914062
3.28284859657288 -0.303207397460938
3.30449056625366 -0.312698364257812
3.31386733055115 -0.314208984375
3.32878708839417 -0.318832397460938
3.34419560432434 -0.321380615234375
3.35198950767517 -0.322265625
3.36191654205322 -0.323089599609375
3.36772847175598 -0.32373046875
3.3789427280426 -0.325408935546875
3.38738989830017 -0.326629638671875
3.39375066757202 -0.327545166015625
3.40157294273376 -0.329421997070312
3.42242574691772 -0.338088989257812
3.43104195594788 -0.341384887695312
3.43838405609131 -0.342819213867188
3.44122362136841 -0.343994140625
3.45347118377686 -0.348480224609375
3.4610481262207 -0.35223388671875
3.47319483757019 -0.354629516601562
3.48129940032959 -0.356887817382812
3.48911428451538 -0.3604736328125
3.49789667129517 -0.362945556640625
3.50133323669434 -0.3648681640625
3.50731611251831 -0.367782592773438
3.51188325881958 -0.368942260742188
3.51693177223206 -0.37225341796875
3.52762985229492 -0.378067016601562
3.53160667419434 -0.379898071289062
3.5405797958374 -0.380813598632812
3.54851222038269 -0.38250732421875
3.55181574821472 -0.383544921875
3.56002616882324 -0.3846435546875
3.56229281425476 -0.384994506835938
3.56714415550232 -0.385421752929688
3.57321977615356 -0.386077880859375
3.57611083984375 -0.38653564453125
3.57886838912964 -0.386856079101562
3.58399176597595 -0.387313842773438
3.59206557273865 -0.38885498046875
3.59604692459106 -0.389205932617188
3.60303616523743 -0.389572143554688
3.61012768745422 -0.3924560546875
3.61140465736389 -0.392745971679688
3.6167905330658 -0.393020629882812
3.62055253982544 -0.39324951171875
3.62138414382935 -0.393508911132812
3.63103771209717 -0.3973388671875
3.63225483894348 -0.397903442382812
3.63387227058411 -0.398025512695312
3.63548374176025 -0.398193359375
3.63628721237183 -0.398269653320312
3.64196968078613 -0.398773193359375
3.64246463775635 -0.39886474609375
3.64325523376465 -0.399017333984375
3.64826250076294 -0.400741577148438
3.64914011955261 -0.400909423828125
3.65427279472351 -0.401901245117188
3.65513849258423 -0.402053833007812
3.65609812736511 -0.402114868164062
3.65896487236023 -0.402572631835938
3.65953588485718 -0.402664184570312
3.66077065467834 -0.402816772460938
3.66304087638855 -0.402862548828125
3.66360664367676 -0.402938842773438
3.67135810852051 -0.404678344726562
3.67237496376038 -0.404891967773438
3.6727442741394 -0.405014038085938
3.67394208908081 -0.405075073242188
3.67440176010132 -0.405120849609375
3.67458558082581 -0.405197143554688
3.68069791793823 -0.406051635742188
3.68115067481995 -0.4061279296875
3.68187403678894 -0.40631103515625
3.68286681175232 -0.406387329101562
3.68520402908325 -0.406570434570312
3.68592071533203 -0.406646728515625
3.68699359893799 -0.406753540039062
3.68726134300232 -0.40679931640625
3.68761801719666 -0.4068603515625
3.68788552284241 -0.40692138671875
3.69099307060242 -0.407119750976562
3.69125843048096 -0.407196044921875
3.69187688827515 -0.407257080078125
3.69565677642822 -0.407882690429688
3.69775223731995 -0.407989501953125
3.69810056686401 -0.408035278320312
3.69827461242676 -0.408050537109375
3.70320534706116 -0.408615112304688
3.70380711555481 -0.408981323242188
3.70423626899719 -0.409011840820312
3.704665184021 -0.4090576171875
3.70475101470947 -0.409088134765625
3.70594930648804 -0.409164428710938
3.70791077613831 -0.409194946289062
3.70867586135864 -0.409271240234375
3.70927000045776 -0.409347534179688
3.70935487747192 -0.409378051757812
3.70969390869141 -0.409408569335938
3.70986342430115 -0.409454345703125
3.71222877502441 -0.409469604492188
3.71239709854126 -0.409500122070312
3.71273374557495 -0.409561157226562
3.71357464790344 -0.409866333007812
3.71625375747681 -0.409942626953125
3.71700429916382 -0.409988403320312
3.71808624267578 -0.410110473632812
3.71841859817505 -0.41015625
3.71866774559021 -0.410171508789062
3.71899962425232 -0.410232543945312
3.71933126449585 -0.410263061523438
3.7208206653595 -0.410293579101562
3.7208206653595 -0.410308837890625
3.72197532653809 -0.410446166992188
3.72214007377625 -0.41046142578125
3.72370195388794 -0.410507202148438
3.72997426986694 -0.41082763671875
3.73021674156189 -0.410842895507812
3.73062086105347 -0.410919189453125
3.73086309432983 -0.41094970703125
3.73311710357666 -0.41107177734375
3.73335790634155 -0.411102294921875
3.73335790634155 -0.411117553710938
3.73583841323853 -0.411453247070312
3.73599791526794 -0.411483764648438
3.73790788650513 -0.411514282226562
3.73798727989197 -0.411544799804688
3.73830485343933 -0.41156005859375
3.73870134353638 -0.411590576171875
3.73885989189148 -0.411605834960938
3.74382328987122 -0.412307739257812
3.74405813217163 -0.412353515625
3.74702310562134 -0.412384033203125
3.74733400344849 -0.412399291992188
3.75151014328003 -0.41265869140625
3.7517409324646 -0.412734985351562
3.75197148323059 -0.412734985351562
3.75204849243164 -0.412750244140625
3.75227904319763 -0.412765502929688
3.75342988967896 -0.412948608398438
3.75365972518921 -0.4129638671875
3.75404238700867 -0.412979125976562
3.75518846511841 -0.413070678710938
3.75541734695435 -0.4130859375
3.75541734695435 -0.413101196289062
3.75564622879028 -0.413116455078125
3.75617957115173 -0.413131713867188
3.75709223747253 -0.41314697265625
3.75709223747253 -0.413162231445312
3.75739598274231 -0.413192749023438
3.75777554512024 -0.4132080078125
3.75966787338257 -0.41326904296875
3.75989437103271 -0.413299560546875
3.76042246818542 -0.413314819335938
3.76237845420837 -0.413406372070312
3.76252841949463 -0.413421630859375
3.76252841949463 -0.413436889648438
3.7649974822998 -0.413497924804688
3.76529598236084 -0.413528442382812
3.76723003387451 -0.41357421875
3.76745271682739 -0.413619995117188
3.7678234577179 -0.41363525390625
3.76826810836792 -0.41363525390625
3.76893401145935 -0.4136962890625
3.77041006088257 -0.413726806640625
3.77048373222351 -0.413742065429688
3.77070474624634 -0.413742065429688
3.77611970901489 -0.414443969726562
3.7764105796814 -0.41455078125
3.77670121192932 -0.414566040039062
3.77720928192139 -0.41461181640625
3.77728176116943 -0.41461181640625
3.77930784225464 -0.414627075195312
3.78010129928589 -0.414642333984375
3.7834746837616 -0.414901733398438
3.78411769866943 -0.414947509765625
3.7844033241272 -0.414962768554688
3.7844033241272 -0.41497802734375
3.7845458984375 -0.41497802734375
3.78483128547668 -0.414993286132812
3.78490257263184 -0.415008544921875
3.79007387161255 -0.415390014648438
3.79035544395447 -0.41571044921875
3.79063701629639 -0.415725708007812
3.79077768325806 -0.415740966796875
3.79084777832031 -0.415740966796875
3.79084777832031 -0.415756225585938
3.79091811180115 -0.415771484375
3.79148006439209 -0.415786743164062
3.79155039787292 -0.415817260742188
3.79162049293518 -0.41583251953125
3.79204130172729 -0.41583251953125
3.79232168197632 -0.41583251953125
3.79483652114868 -0.415908813476562
3.79581046104431 -0.41595458984375
3.79608845710754 -0.415985107421875
3.79643559455872 -0.416000366210938
3.79671311378479 -0.416015625
3.79678249359131 -0.416015625
3.79678249359131 -0.416030883789062
3.80448007583618 -0.416946411132812
3.80502486228943 -0.417129516601562
3.80665469169617 -0.417160034179688
3.80685806274414 -0.41717529296875
3.80685806274414 -0.41717529296875
3.80706119537354 -0.41717529296875
3.80733203887939 -0.417190551757812
3.80854845046997 -0.417221069335938
3.80875086784363 -0.417236328125
3.81036686897278 -0.417251586914062
3.81050133705139 -0.417251586914062
3.81063580513 -0.417251586914062
3.81063580513 -0.417266845703125
3.81063580513 -0.417266845703125
3.81063580513 -0.417266845703125
3.81170892715454 -0.417312622070312
3.81177592277527 -0.417312622070312
3.81577682495117 -0.41748046875
3.81590962409973 -0.417510986328125
3.81597590446472 -0.417510986328125
3.81604242324829 -0.417510986328125
3.81637382507324 -0.417510986328125
3.81650638580322 -0.417526245117188
3.81650638580322 -0.417526245117188
3.81650638580322 -0.41754150390625
3.81650638580322 -0.41754150390625
3.81683754920959 -0.41754150390625
3.81776356697083 -0.417556762695312
3.81782960891724 -0.417556762695312
3.81782960891724 -0.417556762695312
3.81782960891724 -0.417572021484375
3.81809377670288 -0.417587280273438
3.81974124908447 -0.417587280273438
3.81974124908447 -0.417587280273438
3.82039856910706 -0.417633056640625
3.82046413421631 -0.417633056640625
3.82072687149048 -0.417633056640625
3.82079243659973 -0.417648315429688
3.82092356681824 -0.417648315429688
3.82098913192749 -0.417648315429688
3.82138252258301 -0.417648315429688
3.82144808769226 -0.41766357421875
3.82301759719849 -0.41766357421875
3.82314801216125 -0.417678833007812
3.82314801216125 -0.417678833007812
3.82321333885193 -0.417678833007812
3.82321333885193 -0.417694091796875
3.8232786655426 -0.417694091796875
3.8232786655426 -0.417694091796875
3.82366991043091 -0.417694091796875
3.82406067848206 -0.417694091796875
3.82406067848206 -0.417709350585938
3.82406067848206 -0.417709350585938
3.82484149932861 -0.417724609375
3.82510137557983 -0.417739868164062
3.82523131370544 -0.417739868164062
3.82529616355896 -0.417739868164062
3.82698130607605 -0.417739868164062
3.82704591751099 -0.417739868164062
3.82704591751099 -0.417755126953125
3.82704591751099 -0.417755126953125
3.82717537879944 -0.417770385742188
3.82723999023438 -0.417770385742188
3.82756304740906 -0.41778564453125
3.82775688171387 -0.41778564453125
3.82827305793762 -0.41778564453125
3.82827305793762 -0.417800903320312
3.82827305793762 -0.417800903320312
3.82827305793762 -0.417800903320312
3.82827305793762 -0.417800903320312
3.82911062240601 -0.417816162109375
3.83135771751404 -0.417831420898438
3.83135771751404 -0.417831420898438
3.83135771751404 -0.417831420898438
3.83225345611572 -0.417877197265625
3.83238124847412 -0.417877197265625
3.83238124847412 -0.417877197265625
3.83238124847412 -0.417892456054688
3.83270049095154 -0.417892456054688
3.83276438713074 -0.417892456054688
3.83282804489136 -0.417892456054688
3.83327460289001 -0.417892456054688
3.83391165733337 -0.41790771484375
3.83391165733337 -0.417922973632812
3.83391165733337 -0.417922973632812
3.83416628837585 -0.417922973632812
3.83416628837585 -0.417922973632812
3.83739900588989 -0.417953491210938
3.83746218681335 -0.417953491210938
3.8375883102417 -0.417953491210938
3.8375883102417 -0.417953491210938
3.8375883102417 -0.41796875
3.83790397644043 -0.41796875
3.83790397644043 -0.41796875
3.83790397644043 -0.41796875
3.83790397644043 -0.417984008789062
3.83790397644043 -0.417984008789062
3.83790397644043 -0.417984008789062
3.83903789520264 -0.41802978515625
3.83903789520264 -0.418045043945312
3.83903789520264 -0.418045043945312
3.83903789520264 -0.418045043945312
3.83903789520264 -0.418045043945312
3.83928942680359 -0.418060302734375
3.83928942680359 -0.418075561523438
3.83928942680359 -0.418075561523438
3.84160971641541 -0.418075561523438
3.84160971641541 -0.418075561523438
3.84160971641541 -0.418075561523438
3.84160971641541 -0.418075561523438
3.84173488616943 -0.418075561523438
3.84179735183716 -0.4180908203125
3.84179735183716 -0.4180908203125
3.84179735183716 -0.4180908203125
3.84198474884033 -0.418106079101562
3.84217214584351 -0.418106079101562
3.84217214584351 -0.418106079101562
3.84217214584351 -0.418106079101562
3.842609167099 -0.418106079101562
3.84267163276672 -0.418106079101562
3.84273409843445 -0.418121337890625
3.84279632568359 -0.418121337890625
3.84279632568359 -0.418121337890625
3.84285879135132 -0.418136596679688
3.84292101860046 -0.418136596679688
3.84348201751709 -0.418136596679688
3.84348201751709 -0.418136596679688
3.84360647201538 -0.41815185546875
3.84360647201538 -0.41815185546875
3.84397983551025 -0.41815185546875
3.84397983551025 -0.41815185546875
3.84397983551025 -0.418167114257812
3.84397983551025 -0.418167114257812
3.84397983551025 -0.418182373046875
3.84397983551025 -0.418182373046875
3.84435296058655 -0.418182373046875
3.84435296058655 -0.418182373046875
3.84447717666626 -0.418197631835938
3.8471405506134 -0.418197631835938
3.8471405506134 -0.418197631835938
3.8471405506134 -0.418197631835938
3.84732580184937 -0.418212890625
3.84751105308533 -0.418212890625
3.84757256507874 -0.418212890625
3.84763431549072 -0.418212890625
3.84769606590271 -0.418228149414062
3.84769606590271 -0.418228149414062
3.8479425907135 -0.418228149414062
3.8479425907135 -0.418243408203125
3.8479425907135 -0.418243408203125
3.8479425907135 -0.418258666992188
3.84831237792969 -0.418258666992188
3.84831237792969 -0.418258666992188
3.84898924827576 -0.41827392578125
3.84905076026917 -0.418289184570312
3.84911203384399 -0.418289184570312
3.84911203384399 -0.418289184570312
3.84911203384399 -0.418289184570312
3.84911203384399 -0.418289184570312
3.84911203384399 -0.418289184570312
3.85027861595154 -0.418289184570312
3.85033988952637 -0.418289184570312
3.85033988952637 -0.418304443359375
3.8504011631012 -0.418304443359375
3.85046243667603 -0.418304443359375
3.85052371025085 -0.418319702148438
3.85076880455017 -0.418319702148438
3.85082983970642 -0.418319702148438
3.85089111328125 -0.4183349609375
3.85095238685608 -0.4183349609375
};
\end{axis}

\begin{axis}[
%\begin{axis}[
tick align=outside,
tick pos=left,
% title={\(\displaystyle S_3\)},
x grid style={darkgray176},
xlabel={COI},
xmin=-0.259942197799683, xmax=6.0,
xtick = {1,2,3,4},
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.25, ymax=0.01,
% ytick = {0,-0.05,-0.1,-0.15,-0.2,-0.25},
ytick style={color=black},
ytick distance = 0.1,
% legend style={at={(0.995,0.97)},
legend style={at={(1.3,1.3)}, draw=none,font=\huge},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={6},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1, font=\large}},
ylabel shift=-6pt,
width=0.35\textwidth,
height=0.25\textwidth,
% y tick label style={
%         /pgf/number format/.cd,
%         fixed,
%         fixed zerofill,
%         precision=2,
%         /tikz/.cd
%     },
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c14)}
]
\addplot [ultra thick, blue] 
table {%
0 0
0.30103000998497 -0.00018310546875
0.698970019817352 -0.00054931640625
0.778151273727417 -0.00067138671875
0.903090000152588 -0.00079345703125
1.04139268398285 -0.00091552734375
1.07918119430542 -0.00103759765625
1.17609131336212 -0.0013427734375
1.25527250766754 -0.00146484375
1.25527250766754 -0.00152587890625
1.49136173725128 -0.0068359375
1.54406809806824 -0.00872802734375
1.6020599603653 -0.00982666015625
1.66275787353516 -0.01025390625
1.74036264419556 -0.0120849609375
1.79239177703857 -0.01287841796875
1.82607483863831 -0.01373291015625
1.89762711524963 -0.01434326171875
1.94939005374908 -0.01507568359375
1.9956351518631 -0.015625
2.02938365936279 -0.01690673828125
2.07188200950623 -0.01763916015625
2.09690999984741 -0.0185546875
2.11058974266052 -0.01953125
2.15836238861084 -0.0216064453125
2.19033169746399 -0.02294921875
2.20411992073059 -0.0238037109375
2.25527238845825 -0.02960205078125
2.27184152603149 -0.03094482421875
2.301029920578 -0.03192138671875
2.31386733055115 -0.03271484375
2.35602593421936 -0.0355224609375
2.38560628890991 -0.03863525390625
2.39794015884399 -0.03955078125
2.44090914726257 -0.0428466796875
2.45331835746765 -0.0440673828125
2.4712917804718 -0.046142578125
2.51982808113098 -0.05670166015625
2.53275442123413 -0.0604248046875
2.54406809806824 -0.06121826171875
2.56229281425476 -0.0638427734375
2.61172342300415 -0.07568359375
2.62117624282837 -0.08428955078125
2.64147400856018 -0.08819580078125
2.65030741691589 -0.0897216796875
2.670245885849 -0.09356689453125
2.68663620948792 -0.09539794921875
2.71096301078796 -0.09942626953125
2.73798727989197 -0.1077880859375
2.74585509300232 -0.112548828125
2.76267862319946 -0.11578369140625
2.78746056556702 -0.12115478515625
2.79379034042358 -0.12481689453125
2.80140376091003 -0.1265869140625
2.81491327285767 -0.128662109375
2.82477641105652 -0.13116455078125
2.8331470489502 -0.1324462890625
2.85430598258972 -0.1392822265625
2.85913825035095 -0.14093017578125
2.86213135719299 -0.14178466796875
2.87563991546631 -0.14471435546875
2.88195490837097 -0.14569091796875
2.8898618221283 -0.14666748046875
2.89542245864868 -0.14727783203125
2.9047155380249 -0.1514892578125
2.91907811164856 -0.15362548828125
2.9232439994812 -0.154052734375
2.95327639579773 -0.16888427734375
2.96189546585083 -0.17535400390625
2.96614170074463 -0.1766357421875
2.97081160545349 -0.17803955078125
2.97818040847778 -0.17901611328125
2.98811292648315 -0.181640625
2.99431705474854 -0.182861328125
3.01367974281311 -0.18853759765625
3.01577877998352 -0.19024658203125
3.02571535110474 -0.1927490234375
3.0301947593689 -0.19366455078125
3.03261876106262 -0.19427490234375
3.04257559776306 -0.19677734375
3.05690479278564 -0.19842529296875
3.05994200706482 -0.1993408203125
3.06445789337158 -0.19989013671875
3.07003784179688 -0.20062255859375
3.081707239151 -0.2030029296875
3.0852906703949 -0.2034912109375
3.09725737571716 -0.20611572265625
3.10037064552307 -0.20654296875
3.10856509208679 -0.2071533203125
3.12123155593872 -0.210205078125
3.12385153770447 -0.21124267578125
3.12613129615784 -0.21160888671875
3.13545060157776 -0.21319580078125
3.14363932609558 -0.21392822265625
3.14519643783569 -0.21417236328125
3.15836238861084 -0.21734619140625
3.1720187664032 -0.22552490234375
3.17666983604431 -0.22821044921875
3.1786892414093 -0.228515625
3.18041253089905 -0.22882080078125
3.18469142913818 -0.2291259765625
3.18610835075378 -0.2293701171875
3.18780255317688 -0.22955322265625
3.19423675537109 -0.23004150390625
3.19589972496033 -0.2303466796875
3.19755625724792 -0.2305908203125
3.19893193244934 -0.230712890625
3.21325206756592 -0.23187255859375
3.21431398391724 -0.232177734375
3.21906042098999 -0.2327880859375
3.22010803222656 -0.233154296875
3.22297644615173 -0.2332763671875
3.2242739200592 -0.23345947265625
3.23248791694641 -0.2337646484375
3.23653721809387 -0.2344970703125
3.24993181228638 -0.235107421875
3.25017595291138 -0.2353515625
3.25188136100769 -0.23541259765625
3.25430631637573 -0.23583984375
3.25839781761169 -0.23602294921875
3.26054835319519 -0.23638916015625
3.2652895450592 -0.236572265625
3.27253770828247 -0.2371826171875
3.27346420288086 -0.23736572265625
3.28194189071655 -0.23834228515625
3.28284859657288 -0.2386474609375
3.28352737426758 -0.23883056640625
3.29819774627686 -0.24676513671875
3.29950737953186 -0.249755859375
3.30211448669434 -0.24993896484375
3.30728197097778 -0.25054931640625
3.30963015556335 -0.2506103515625
3.31281185150146 -0.25079345703125
3.31302309036255 -0.2508544921875
3.31534051895142 -0.25091552734375
3.33102226257324 -0.2518310546875
3.33203434944153 -0.25201416015625
3.33805775642395 -0.25238037109375
3.33865571022034 -0.25250244140625
3.3514096736908 -0.25396728515625
3.35256838798523 -0.25457763671875
3.35449266433716 -0.254638671875
3.35525989532471 -0.2547607421875
3.35831570625305 -0.2550048828125
3.35907626152039 -0.25506591796875
3.36078262329102 -0.25518798828125
3.36229395866394 -0.25531005859375
3.36604928970337 -0.25537109375
3.36623620986938 -0.2554931640625
3.36772847175598 -0.25567626953125
3.36847281455994 -0.2557373046875
3.37364745140076 -0.25592041015625
3.37474822998047 -0.25604248046875
3.37602925300598 -0.25616455078125
3.3769416809082 -0.2562255859375
3.37803435325623 -0.25628662109375
3.37948679924011 -0.25634765625
3.38399481773376 -0.25665283203125
3.38542747497559 -0.2568359375
3.38667726516724 -0.25689697265625
3.38774561882019 -0.25701904296875
3.3879234790802 -0.257080078125
3.40053796768188 -0.2625732421875
3.40140056610107 -0.264404296875
3.40157294273376 -0.2645263671875
3.40243339538574 -0.26458740234375
3.40857911109924 -0.26568603515625
3.40993309020996 -0.26580810546875
3.41027092933655 -0.265869140625
3.41329979896545 -0.26617431640625
3.4148063659668 -0.2662353515625
3.41514039039612 -0.266357421875
3.41697311401367 -0.26641845703125
3.42160391807556 -0.2667236328125
3.42291808128357 -0.266845703125
3.42373728752136 -0.26690673828125
3.42845869064331 -0.26739501953125
3.42942929267883 -0.26751708984375
3.43296933174133 -0.26763916015625
3.43328976631165 -0.2677001953125
3.4401216506958 -0.2694091796875
3.44075179100037 -0.2696533203125
3.44513702392578 -0.270263671875
3.44575977325439 -0.27044677734375
3.4462263584137 -0.27056884765625
3.44669246673584 -0.27069091796875
3.44870638847351 -0.2708740234375
3.45316529273987 -0.27325439453125
3.45377683639526 -0.27362060546875
3.45636606216431 -0.27392578125
3.45863795280457 -0.2742919921875
3.45909070968628 -0.27471923828125
3.46194839477539 -0.2747802734375
3.47026348114014 -0.27801513671875
3.47055745124817 -0.27838134765625
3.47099828720093 -0.278564453125
3.47143840789795 -0.27862548828125
3.47187829017639 -0.27874755859375
3.47202467918396 -0.27874755859375
3.47246384620667 -0.27886962890625
3.47392463684082 -0.279052734375
3.47450757026672 -0.27923583984375
3.47508978843689 -0.279296875
3.47523522377014 -0.27935791015625
3.47683167457581 -0.2794189453125
3.47712135314941 -0.2794189453125
3.48115587234497 -0.27978515625
3.48129940032959 -0.27978515625
3.48187232017517 -0.2799072265625
3.48201560974121 -0.27996826171875
3.48244476318359 -0.27996826171875
3.48244476318359 -0.280029296875
3.4828736782074 -0.280029296875
3.4828736782074 -0.28009033203125
3.48330187797546 -0.28009033203125
3.486572265625 -0.28106689453125
3.48727989196777 -0.2811279296875
3.48742127418518 -0.2811279296875
3.48784518241882 -0.28118896484375
3.48798632621765 -0.28118896484375
3.48995852470398 -0.28125
3.48995852470398 -0.28125
3.48995852470398 -0.28125
3.49066066741943 -0.28131103515625
3.49066066741943 -0.28131103515625
3.49080085754395 -0.2813720703125
3.49317908287048 -0.2816162109375
3.49331855773926 -0.2816162109375
3.49748253822327 -0.2821044921875
3.49762058258057 -0.2821044921875
3.49775862693787 -0.28216552734375
3.49775862693787 -0.28216552734375
3.49858617782593 -0.2822265625
3.49886178970337 -0.2822265625
3.49899935722351 -0.28228759765625
3.49913692474365 -0.28228759765625
3.49913692474365 -0.28228759765625
3.49954962730408 -0.2823486328125
3.49968719482422 -0.2823486328125
3.49982452392578 -0.2823486328125
3.49996185302734 -0.28240966796875
3.50078511238098 -0.28240966796875
3.50092220306396 -0.28240966796875
3.50092220306396 -0.282470703125
3.50133323669434 -0.282470703125
3.50799083709717 -0.2835693359375
3.50852966308594 -0.2838134765625
3.50866436958313 -0.2838134765625
3.50893354415894 -0.28387451171875
3.50893354415894 -0.28387451171875
3.50893354415894 -0.28387451171875
3.50960564613342 -0.283935546875
3.50960564613342 -0.283935546875
3.50974011421204 -0.28399658203125
3.51215052604675 -0.28424072265625
3.51241755485535 -0.2843017578125
3.51241755485535 -0.2843017578125
3.51241755485535 -0.2843017578125
3.51241755485535 -0.2843017578125
3.51281785964966 -0.28436279296875
3.51428198814392 -0.28436279296875
3.51428198814392 -0.28436279296875
3.51428198814392 -0.28436279296875
3.51481318473816 -0.28448486328125
3.51481318473816 -0.28448486328125
3.51534390449524 -0.2845458984375
3.51547646522522 -0.28460693359375
3.5171959400177 -0.28460693359375
3.51745986938477 -0.28460693359375
3.52166104316711 -0.2850341796875
3.52218341827393 -0.28509521484375
3.52231383323669 -0.28509521484375
3.52244424819946 -0.28509521484375
3.52322602272034 -0.28521728515625
3.52335619926453 -0.28521728515625
3.52348637580872 -0.2852783203125
3.52439618110657 -0.2852783203125
3.5245258808136 -0.2852783203125
3.52465581893921 -0.2852783203125
3.52465581893921 -0.28533935546875
3.52478551864624 -0.28533935546875
3.52491521835327 -0.28533935546875
3.52582192420959 -0.28533935546875
3.52595138549805 -0.285400390625
3.52595138549805 -0.285400390625
3.52595138549805 -0.285400390625
3.52608060836792 -0.285400390625
3.52608060836792 -0.285400390625
3.52698516845703 -0.28546142578125
3.52711415290833 -0.28546142578125
3.52711415290833 -0.28546142578125
3.52724313735962 -0.2855224609375
3.52724313735962 -0.2855224609375
3.52762985229492 -0.2855224609375
3.52840232849121 -0.28558349609375
3.52853107452393 -0.28558349609375
3.52968692779541 -0.28570556640625
3.52968692779541 -0.28570556640625
3.52968692779541 -0.28570556640625
3.52994346618652 -0.28570556640625
3.52994346618652 -0.2857666015625
3.52994346618652 -0.2857666015625
3.53237199783325 -0.2860107421875
3.53237199783325 -0.2860107421875
3.53237199783325 -0.2860107421875
3.53326344490051 -0.28607177734375
3.53326344490051 -0.2861328125
3.53339076042175 -0.2861328125
3.53339076042175 -0.2861328125
3.53744125366211 -0.286376953125
3.53756713867188 -0.286376953125
3.53769326210022 -0.286376953125
3.53769326210022 -0.28643798828125
3.5381965637207 -0.28643798828125
3.53832244873047 -0.2864990234375
3.53832244873047 -0.2864990234375
3.53844809532166 -0.2864990234375
3.53882503509521 -0.2864990234375
3.53957796096802 -0.28656005859375
3.53970313072205 -0.28656005859375
3.53970313072205 -0.28662109375
3.53970313072205 -0.28662109375
3.53995394706726 -0.28662109375
3.54007911682129 -0.28662109375
3.54007911682129 -0.28662109375
3.54020428657532 -0.28668212890625
3.54107975959778 -0.28680419921875
3.54145431518555 -0.286865234375
3.54406809806824 -0.28692626953125
3.54444003105164 -0.28692626953125
3.54493570327759 -0.2869873046875
3.54505968093872 -0.2869873046875
3.54518342018127 -0.2869873046875
3.54555439949036 -0.28704833984375
3.54555439949036 -0.28704833984375
3.54555439949036 -0.28704833984375
3.54567813873291 -0.28704833984375
3.54580163955688 -0.28704833984375
3.54592537879944 -0.287109375
3.54617238044739 -0.287109375
3.54666614532471 -0.287109375
3.5469126701355 -0.28717041015625
3.54703593254089 -0.28717041015625
3.54728221893311 -0.28717041015625
3.5474054813385 -0.28717041015625
3.54765176773071 -0.28717041015625
3.54765176773071 -0.2872314453125
3.55035066604614 -0.28765869140625
3.55047297477722 -0.28765869140625
3.5505952835083 -0.28765869140625
3.5505952835083 -0.28765869140625
3.55145001411438 -0.2877197265625
3.55145001411438 -0.2877197265625
3.55145001411438 -0.2877197265625
3.55145001411438 -0.28778076171875
3.55315446853638 -0.28790283203125
3.55327606201172 -0.28790283203125
3.55339741706848 -0.28790283203125
3.55485248565674 -0.2879638671875
3.55485248565674 -0.2879638671875
3.55485248565674 -0.2879638671875
3.55485248565674 -0.2879638671875
3.55569887161255 -0.2880859375
3.55594038963318 -0.2880859375
3.55594038963318 -0.2880859375
3.55594038963318 -0.28814697265625
3.55618190765381 -0.28814697265625
3.55678486824036 -0.28814697265625
3.55678486824036 -0.28814697265625
3.55678486824036 -0.28814697265625
3.55678486824036 -0.28814697265625
3.55882859230042 -0.2882080078125
3.5589485168457 -0.2882080078125
3.5589485168457 -0.2882080078125
3.5594277381897 -0.28826904296875
3.5594277381897 -0.28826904296875
3.55954742431641 -0.28826904296875
3.55954742431641 -0.28826904296875
3.56026530265808 -0.288330078125
3.56026530265808 -0.288330078125
3.56169748306274 -0.28851318359375
3.56205487251282 -0.28857421875
3.56217384338379 -0.28857421875
3.56217384338379 -0.28863525390625
3.563481092453 -0.28863525390625
3.563481092453 -0.28863525390625
3.56525731086731 -0.28863525390625
3.56525731086731 -0.2886962890625
3.56572985649109 -0.2886962890625
3.56572985649109 -0.2886962890625
3.56572985649109 -0.2886962890625
3.56572985649109 -0.2886962890625
3.56620168685913 -0.2886962890625
3.56620168685913 -0.2886962890625
3.56631970405579 -0.2886962890625
3.56631970405579 -0.2886962890625
3.56631970405579 -0.28875732421875
3.56667327880859 -0.28875732421875
3.56679105758667 -0.28875732421875
3.56867098808289 -0.288818359375
3.56890535354614 -0.288818359375
3.56902265548706 -0.288818359375
3.56937384605408 -0.28887939453125
3.56949090957642 -0.28887939453125
3.56949090957642 -0.28887939453125
3.56949090957642 -0.28887939453125
3.56972503662109 -0.28887939453125
3.56972503662109 -0.28887939453125
3.56984186172485 -0.28887939453125
3.57414698600769 -0.28936767578125
3.57460999488831 -0.28955078125
3.57472562789917 -0.28955078125
3.57484126091003 -0.28955078125
3.57507228851318 -0.28955078125
3.57507228851318 -0.28955078125
3.57507228851318 -0.28955078125
3.57518792152405 -0.28955078125
3.57553434371948 -0.28955078125
3.57553434371948 -0.28961181640625
3.57553434371948 -0.28961181640625
3.57553434371948 -0.28961181640625
3.57564973831177 -0.28961181640625
3.57599568367004 -0.28961181640625
3.57611083984375 -0.28961181640625
3.57622623443604 -0.28961181640625
3.57622623443604 -0.28961181640625
3.57622623443604 -0.28961181640625
3.57622623443604 -0.28961181640625
3.57657170295715 -0.28961181640625
3.57668685913086 -0.2896728515625
3.57668685913086 -0.2896728515625
3.57680177688599 -0.2896728515625
3.57680177688599 -0.2896728515625
3.57714700698853 -0.2896728515625
3.57726192474365 -0.2896728515625
3.57795119285583 -0.28973388671875
3.57829523086548 -0.28973388671875
3.57840991020203 -0.28973388671875
3.57840991020203 -0.28973388671875
3.57863926887512 -0.28973388671875
3.57863926887512 -0.28973388671875
3.57875370979309 -0.28973388671875
3.57875370979309 -0.28973388671875
3.57909727096558 -0.28973388671875
3.57921171188354 -0.289794921875
3.57944059371948 -0.289794921875
3.57966923713684 -0.289794921875
3.5798978805542 -0.289794921875
3.58035469055176 -0.289794921875
3.58092498779297 -0.28985595703125
3.58092498779297 -0.28985595703125
3.58103895187378 -0.28985595703125
3.58103895187378 -0.28985595703125
3.58138060569763 -0.28985595703125
3.58138060569763 -0.28985595703125
3.58160829544067 -0.28985595703125
3.58331227302551 -0.28985595703125
3.58331227302551 -0.28985595703125
3.58342552185059 -0.28985595703125
3.58376550674438 -0.2899169921875
3.58387851715088 -0.2899169921875
3.58399176597595 -0.2899169921875
3.58399176597595 -0.2899169921875
3.58444428443909 -0.2899169921875
3.58489632606506 -0.2899169921875
3.58500933647156 -0.2899169921875
3.58500933647156 -0.2899169921875
3.58512210845947 -0.28997802734375
3.58512210845947 -0.28997802734375
3.5854606628418 -0.28997802734375
3.58613705635071 -0.28997802734375
3.58624958992004 -0.2900390625
3.58624958992004 -0.2900390625
3.58681225776672 -0.2900390625
3.58692479133606 -0.2900390625
3.58692479133606 -0.2900390625
3.58692479133606 -0.2900390625
3.58737421035767 -0.2900390625
3.58737421035767 -0.2900390625
3.58815956115723 -0.29010009765625
3.5882716178894 -0.29010009765625
3.5882716178894 -0.29010009765625
3.58838367462158 -0.29010009765625
3.58894371986389 -0.29010009765625
3.58894371986389 -0.2901611328125
3.59106469154358 -0.2904052734375
3.59106469154358 -0.2904052734375
3.59106469154358 -0.2904052734375
3.59117603302002 -0.2904052734375
3.59139847755432 -0.2904052734375
3.59139847755432 -0.29046630859375
3.59173226356506 -0.29046630859375
3.59184336662292 -0.29046630859375
3.59195446968079 -0.29046630859375
3.59195446968079 -0.29046630859375
3.59239888191223 -0.29046630859375
3.59239888191223 -0.29046630859375
3.59306454658508 -0.29052734375
3.59317541122437 -0.29052734375
3.59328603744507 -0.29052734375
3.59328603744507 -0.29052734375
3.59472393989563 -0.2906494140625
3.59472393989563 -0.2906494140625
3.59483432769775 -0.2906494140625
3.59483432769775 -0.2906494140625
3.59549617767334 -0.29071044921875
3.59549617767334 -0.29071044921875
3.59560656547546 -0.29071044921875
3.59571671485901 -0.29071044921875
3.59626722335815 -0.29071044921875
3.59637713432312 -0.29071044921875
3.59648704528809 -0.29071044921875
3.59648704528809 -0.29071044921875
3.59802412986755 -0.29071044921875
3.59802412986755 -0.29071044921875
3.59824323654175 -0.29071044921875
3.59868121147156 -0.290771484375
3.59879064559937 -0.290771484375
3.59879064559937 -0.290771484375
3.59879064559937 -0.290771484375
3.59911870956421 -0.290771484375
3.59922790527344 -0.290771484375
3.60031938552856 -0.2908935546875
3.60042834281921 -0.2908935546875
3.60064625740051 -0.2908935546875
3.60064625740051 -0.2908935546875
3.60086393356323 -0.2908935546875
3.60086393356323 -0.2908935546875
3.60097289085388 -0.2908935546875
3.60140800476074 -0.29095458984375
3.60140800476074 -0.29095458984375
3.60151672363281 -0.29095458984375
3.60151672363281 -0.29095458984375
3.60238552093506 -0.29095458984375
3.60249400138855 -0.29095458984375
3.60260248184204 -0.29095458984375
3.60260248184204 -0.291015625
3.60422611236572 -0.2911376953125
3.60455012321472 -0.29119873046875
3.60465788841248 -0.29119873046875
3.60476589202881 -0.29119873046875
3.60573577880859 -0.29119873046875
3.60573577880859 -0.29119873046875
3.60573577880859 -0.29119873046875
3.60595107078552 -0.291259765625
3.60595107078552 -0.291259765625
3.60605883598328 -0.291259765625
3.60616636276245 -0.291259765625
3.60627388954163 -0.291259765625
3.60691857337952 -0.291259765625
3.60702586174011 -0.291259765625
3.60702586174011 -0.29132080078125
3.60702586174011 -0.29132080078125
3.6077766418457 -0.29132080078125
3.60788369178772 -0.29132080078125
3.60820508003235 -0.29132080078125
3.60831212997437 -0.29132080078125
3.60873985290527 -0.29132080078125
3.60873985290527 -0.2913818359375
3.60873985290527 -0.2913818359375
3.60884690284729 -0.2913818359375
3.60895371437073 -0.2913818359375
3.60895371437073 -0.2913818359375
3.60895371437073 -0.2913818359375
3.60895371437073 -0.2913818359375
3.60895371437073 -0.2913818359375
3.60906052589417 -0.2913818359375
3.60906052589417 -0.2913818359375
3.60959434509277 -0.2913818359375
3.60959434509277 -0.2913818359375
3.61002111434937 -0.29144287109375
3.61012768745422 -0.29144287109375
3.61055374145508 -0.29144287109375
3.61055374145508 -0.29144287109375
3.61066007614136 -0.29144287109375
3.61066007614136 -0.29144287109375
3.61066007614136 -0.29144287109375
3.61140465736389 -0.29144287109375
3.61140465736389 -0.29144287109375
3.61140465736389 -0.29144287109375
3.61151099205017 -0.29144287109375
3.61151099205017 -0.29144287109375
3.61161708831787 -0.29150390625
3.61193561553955 -0.29150390625
3.61193561553955 -0.29150390625
3.61204171180725 -0.29150390625
3.61204171180725 -0.29150390625
3.61204171180725 -0.29150390625
3.61214780807495 -0.29150390625
3.61214780807495 -0.29150390625
3.61257195472717 -0.29150390625
3.61257195472717 -0.29150390625
3.61257195472717 -0.29150390625
3.61320734024048 -0.29156494140625
3.61320734024048 -0.29156494140625
3.61341905593872 -0.29156494140625
3.61341905593872 -0.29156494140625
3.61341905593872 -0.29156494140625
3.61341905593872 -0.29156494140625
3.61341905593872 -0.29156494140625
3.61352467536926 -0.29156494140625
3.61363053321838 -0.29156494140625
3.61363053321838 -0.29156494140625
3.61363053321838 -0.29156494140625
3.61405301094055 -0.29156494140625
3.61405301094055 -0.29156494140625
3.61405301094055 -0.29156494140625
3.61405301094055 -0.29156494140625
3.61415863037109 -0.29156494140625
3.61415863037109 -0.29156494140625
3.61415863037109 -0.29156494140625
3.61458086967468 -0.2916259765625
3.61479187011719 -0.2916259765625
3.61489725112915 -0.2916259765625
3.61489725112915 -0.2916259765625
3.61489725112915 -0.2916259765625
3.61489725112915 -0.2916259765625
3.61489725112915 -0.2916259765625
3.61489725112915 -0.2916259765625
3.61563444137573 -0.2916259765625
3.61573958396912 -0.2916259765625
3.61573958396912 -0.2916259765625
3.61573958396912 -0.29168701171875
3.61573958396912 -0.29168701171875
3.61605525016785 -0.29168701171875
3.61605525016785 -0.29168701171875
3.61616039276123 -0.29168701171875
3.61658048629761 -0.29168701171875
3.6167905330658 -0.29168701171875
3.61710524559021 -0.29168701171875
3.61710524559021 -0.291748046875
3.61721014976501 -0.291748046875
3.61721014976501 -0.291748046875
3.61731481552124 -0.291748046875
3.61731481552124 -0.291748046875
3.61731481552124 -0.291748046875
3.61731481552124 -0.291748046875
3.61804819107056 -0.291748046875
3.61804819107056 -0.291748046875
3.61825728416443 -0.291748046875
3.61825728416443 -0.291748046875
3.61982345581055 -0.29180908203125
3.61982345581055 -0.29180908203125
3.62003183364868 -0.29180908203125
3.62003183364868 -0.29180908203125
3.62003183364868 -0.29180908203125
3.62003183364868 -0.29180908203125
3.62003183364868 -0.29180908203125
3.62003183364868 -0.29180908203125
3.62003183364868 -0.29180908203125
3.62003183364868 -0.29180908203125
3.62592959403992 -0.29217529296875
3.62603235244751 -0.292236328125
3.62613487243652 -0.292236328125
3.62634038925171 -0.292236328125
3.62664818763733 -0.292236328125
3.62675094604492 -0.292236328125
3.62716102600098 -0.292236328125
3.62716102600098 -0.292236328125
3.62716102600098 -0.292236328125
3.62726330757141 -0.292236328125
3.62726330757141 -0.292236328125
3.62726330757141 -0.292236328125
3.62736582756042 -0.292236328125
3.62736582756042 -0.292236328125
3.62736582756042 -0.292236328125
3.62777543067932 -0.29229736328125
3.62777543067932 -0.29229736328125
3.62777543067932 -0.29229736328125
3.62828683853149 -0.29229736328125
3.62828683853149 -0.29229736328125
3.62828683853149 -0.29229736328125
3.62828683853149 -0.29229736328125
3.62838888168335 -0.29229736328125
3.62838888168335 -0.29229736328125
3.62849116325378 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62859320640564 -0.29229736328125
3.62920570373535 -0.29229736328125
3.62920570373535 -0.29229736328125
3.62920570373535 -0.29229736328125
3.62930774688721 -0.2923583984375
3.62971544265747 -0.2923583984375
3.62971544265747 -0.2923583984375
3.62981724739075 -0.2923583984375
3.62981724739075 -0.2923583984375
3.62981724739075 -0.2923583984375
3.62991905212402 -0.2923583984375
3.62991905212402 -0.2923583984375
3.63032627105713 -0.2923583984375
3.63032627105713 -0.2923583984375
3.63032627105713 -0.2923583984375
3.63032627105713 -0.2923583984375
3.63032627105713 -0.2923583984375
3.63032627105713 -0.2923583984375
3.63032627105713 -0.2923583984375
3.63032627105713 -0.2923583984375
3.63032627105713 -0.2923583984375
3.63042783737183 -0.2923583984375
3.63042783737183 -0.2923583984375
3.63042783737183 -0.2923583984375
3.63134217262268 -0.29241943359375
3.63144373893738 -0.29241943359375
3.63144373893738 -0.29241943359375
3.63144373893738 -0.29241943359375
3.63154530525208 -0.29241943359375
3.63154530525208 -0.29241943359375
3.63154530525208 -0.29241943359375
3.63154530525208 -0.29241943359375
3.63195085525513 -0.29241943359375
3.63195085525513 -0.29241943359375
3.63195085525513 -0.29241943359375
3.63195085525513 -0.29241943359375
};
\addplot [ultra thick, brown, dashed]
table {%
1.46239805221558 0
1.65321254730225 -0.0001220703125
2.36172771453857 -0.00030517578125
2.56584787368774 -0.00054931640625
2.61172342300415 -0.0006103515625
2.70329141616821 -0.000732421875
2.84323287010193 -0.0008544921875
2.92890763282776 -0.00091552734375
3.05076622962952 -0.00140380859375
3.15228843688965 -0.0025634765625
3.18892860412598 -0.0030517578125
3.2652895450592 -0.00360107421875
3.29336261749268 -0.0037841796875
3.3062105178833 -0.00390625
3.45591020584106 -0.01666259765625
3.51587390899658 -0.02349853515625
3.55291152000427 -0.02496337890625
3.59933710098267 -0.0284423828125
3.62262845039368 -0.02972412109375
3.680335521698 -0.03485107421875
3.71808624267578 -0.03643798828125
3.75602722167969 -0.0377197265625
3.7839035987854 -0.03961181640625
3.80679035186768 -0.04107666015625
3.84726405143738 -0.05218505859375
3.86664175987244 -0.05755615234375
3.892817735672 -0.05853271484375
3.93176293373108 -0.0650634765625
3.94987773895264 -0.067138671875
3.98788952827454 -0.07415771484375
4.00333118438721 -0.0780029296875
4.01878356933594 -0.07940673828125
4.04571390151978 -0.0867919921875
4.06498193740845 -0.09075927734375
4.07390165328979 -0.0921630859375
4.09933519363403 -0.09576416015625
4.12090301513672 -0.09979248046875
4.13946962356567 -0.1029052734375
4.15390634536743 -0.104736328125
4.16784858703613 -0.1058349609375
4.1923999786377 -0.11370849609375
4.20289659500122 -0.11578369140625
4.21682548522949 -0.11785888671875
4.23006534576416 -0.11981201171875
4.23904895782471 -0.12188720703125
4.24824285507202 -0.12310791015625
4.27395009994507 -0.1297607421875
4.28176021575928 -0.1314697265625
4.29212331771851 -0.13323974609375
4.29904937744141 -0.13433837890625
4.31355094909668 -0.1380615234375
4.334312915802 -0.1435546875
4.3437237739563 -0.14508056640625
4.35268402099609 -0.1458740234375
4.36423206329346 -0.14739990234375
4.37359237670898 -0.1492919921875
4.37861585617065 -0.14996337890625
4.38806581497192 -0.15118408203125
4.39729690551758 -0.15301513671875
4.40282869338989 -0.15362548828125
4.42038488388062 -0.15728759765625
4.42889595031738 -0.15887451171875
4.43725872039795 -0.16015625
4.45200109481812 -0.16229248046875
4.45636606216431 -0.16314697265625
4.46634864807129 -0.1636962890625
4.47699069976807 -0.16595458984375
4.4936671257019 -0.1756591796875
4.50084018707275 -0.17926025390625
4.5080041885376 -0.18035888671875
4.51567506790161 -0.18115234375
4.52150440216064 -0.18182373046875
4.52899360656738 -0.18243408203125
4.53609085083008 -0.1845703125
4.54754066467285 -0.18896484375
4.55425882339478 -0.190185546875
4.56118488311768 -0.19158935546875
4.57259273529053 -0.19512939453125
4.57637596130371 -0.1961669921875
4.58134651184082 -0.19696044921875
4.58908891677856 -0.19891357421875
4.59256553649902 -0.199462890625
4.60017776489258 -0.20068359375
4.60337162017822 -0.20111083984375
4.61272048950195 -0.20343017578125
4.61670637130737 -0.20404052734375
4.62273216247559 -0.204833984375
4.62553882598877 -0.20513916015625
4.63009214401245 -0.205810546875
4.63367033004761 -0.2061767578125
4.63882875442505 -0.20709228515625
4.64539289474487 -0.2100830078125
4.64913988113403 -0.21087646484375
4.65229463577271 -0.21185302734375
4.65544557571411 -0.21234130859375
4.66122579574585 -0.21368408203125
4.66446352005005 -0.2144775390625
4.66785430908203 -0.215576171875
4.67619943618774 -0.216552734375
4.68365049362183 -0.21856689453125
4.6874041557312 -0.2200927734375
4.69312000274658 -0.22216796875
4.69969892501831 -0.22271728515625
4.70221519470215 -0.22296142578125
4.71504163742065 -0.22711181640625
4.71604490280151 -0.227783203125
4.72150564193726 -0.2283935546875
4.72520065307617 -0.22869873046875
4.73642826080322 -0.2296142578125
4.73778867721558 -0.22991943359375
4.74641609191895 -0.2305908203125
4.74815702438354 -0.23077392578125
4.75319242477417 -0.23126220703125
4.75678062438965 -0.23150634765625
4.76330089569092 -0.23193359375
4.76525115966797 -0.232177734375
4.7682900428772 -0.2322998046875
4.77388143539429 -0.23260498046875
4.77996444702148 -0.2327880859375
4.78243684768677 -0.23297119140625
4.78814029693604 -0.233154296875
4.79358768463135 -0.2332763671875
4.80074453353882 -0.234130859375
4.80444622039795 -0.23443603515625
4.80739974975586 -0.23455810546875
4.810387134552 -0.23468017578125
4.82045125961304 -0.23687744140625
4.82233810424805 -0.23724365234375
4.83048582077026 -0.24066162109375
4.83259201049805 -0.24163818359375
4.83555746078491 -0.2421875
4.84082078933716 -0.2427978515625
4.84273386001587 -0.243408203125
4.84500503540039 -0.24383544921875
4.84978771209717 -0.24462890625
4.85503435134888 -0.24627685546875
4.85846519470215 -0.24676513671875
4.86248302459717 -0.2470703125
4.87231969833374 -0.249755859375
4.87329721450806 -0.2498779296875
4.87488174438477 -0.24993896484375
4.88470458984375 -0.25128173828125
4.88774681091309 -0.25140380859375
4.89039850234985 -0.2515869140625
4.8920111656189 -0.25164794921875
4.89452648162842 -0.2518310546875
4.89637184143066 -0.251953125
4.8992075920105 -0.25213623046875
4.90023040771484 -0.252197265625
4.90297603607178 -0.2523193359375
4.90523433685303 -0.25238037109375
4.91182851791382 -0.25445556640625
4.91305065155029 -0.25482177734375
4.91576385498047 -0.2550048828125
4.91640663146973 -0.2550048828125
4.91891574859619 -0.25518798828125
4.91975784301758 -0.25531005859375
4.92337894439697 -0.25543212890625
4.92607975006104 -0.2554931640625
4.92980194091797 -0.25567626953125
4.93365430831909 -0.255859375
4.9362473487854 -0.25616455078125
4.93888473510742 -0.25628662109375
4.94095468521118 -0.25640869140625
4.94386053085327 -0.25665283203125
4.94543409347534 -0.25677490234375
4.94898986816406 -0.25701904296875
4.95098257064819 -0.25714111328125
4.95253562927246 -0.25726318359375
4.95485496520996 -0.2574462890625
4.95707082748413 -0.257568359375
4.95811939239502 -0.25762939453125
4.96190023422241 -0.25787353515625
4.96350908279419 -0.25799560546875
4.96456146240234 -0.25811767578125
4.96737957000732 -0.25836181640625
4.96940183639526 -0.2586669921875
4.97345113754272 -0.25933837890625
4.97713804244995 -0.2601318359375
4.98029899597168 -0.26068115234375
4.98215341567993 -0.2608642578125
4.98371648788452 -0.2611083984375
4.98406362533569 -0.26123046875
4.9872145652771 -0.262451171875
4.98906230926514 -0.26263427734375
4.99050331115723 -0.26287841796875
4.99681806564331 -0.26446533203125
4.99931764602661 -0.26507568359375
5.00069856643677 -0.26513671875
5.00241661071777 -0.2652587890625
5.00571250915527 -0.265380859375
5.00649166107178 -0.26544189453125
5.00842571258545 -0.2655029296875
5.01032543182373 -0.265625
5.0126051902771 -0.26568603515625
5.01453733444214 -0.26580810546875
5.01572036743164 -0.265869140625
5.01871299743652 -0.266357421875
5.01899147033691 -0.2664794921875
5.02107334136963 -0.2666015625
5.02417373657227 -0.26934814453125
5.02534294128418 -0.271728515625
5.02660655975342 -0.27191162109375
5.02798128128052 -0.2723388671875
5.02967977523804 -0.27313232421875
5.03148126602173 -0.27325439453125
5.03378963470459 -0.27386474609375
5.03646516799927 -0.27459716796875
5.03732299804688 -0.2747802734375
5.04221296310425 -0.27618408203125
5.04286289215088 -0.2763671875
5.04818534851074 -0.2772216796875
5.04851579666138 -0.27740478515625
5.04921007156372 -0.27752685546875
5.04949712753296 -0.27764892578125
5.05300521850586 -0.27825927734375
5.05354309082031 -0.27838134765625
5.05439853668213 -0.27850341796875
5.05640172958374 -0.27862548828125
5.05735397338867 -0.27880859375
5.05880165100098 -0.27886962890625
5.05929851531982 -0.2789306640625
5.05953693389893 -0.27899169921875
5.06086015701294 -0.27911376953125
5.06257438659668 -0.2791748046875
5.06276607513428 -0.27923583984375
5.06331062316895 -0.279296875
5.06596040725708 -0.2796630859375
5.0665979385376 -0.27972412109375
5.06740188598633 -0.27978515625
5.06818580627441 -0.27978515625
5.0690279006958 -0.280029296875
5.06965684890747 -0.28009033203125
5.07141780853271 -0.2803955078125
5.07208824157715 -0.28057861328125
5.07292222976685 -0.2806396484375
5.07321977615356 -0.2806396484375
5.07354259490967 -0.2806396484375
5.07416534423828 -0.28070068359375
5.07531690597534 -0.28076171875
5.07555437088013 -0.28082275390625
5.07589721679688 -0.28082275390625
5.07596635818481 -0.28082275390625
5.07647275924683 -0.2808837890625
5.07690238952637 -0.2808837890625
5.07778930664062 -0.28094482421875
5.08079242706299 -0.28204345703125
5.08113098144531 -0.2821044921875
5.08188343048096 -0.2822265625
5.08275651931763 -0.28228759765625
5.08311557769775 -0.28228759765625
5.08344173431396 -0.28228759765625
5.08368539810181 -0.28228759765625
5.08406496047974 -0.2823486328125
5.08419370651245 -0.2823486328125
5.08498001098633 -0.282470703125
5.08530855178833 -0.282470703125
5.08596801757812 -0.28253173828125
5.08660888671875 -0.2825927734375
5.08680438995361 -0.2825927734375
5.08854007720947 -0.2828369140625
5.08944225311279 -0.2828369140625
5.09222936630249 -0.2830810546875
5.0928258895874 -0.28326416015625
5.09318685531616 -0.28326416015625
5.09452342987061 -0.28326416015625
5.09498453140259 -0.2833251953125
5.09566450119019 -0.2833251953125
5.09616231918335 -0.28338623046875
5.09635734558105 -0.28338623046875
5.09792327880859 -0.28350830078125
5.09856081008911 -0.28350830078125
5.09907627105713 -0.28350830078125
5.10058403015137 -0.2835693359375
5.1008358001709 -0.2835693359375
5.10137224197388 -0.28363037109375
5.10225200653076 -0.28363037109375
5.10287618637085 -0.28363037109375
5.10338973999023 -0.28369140625
5.10360527038574 -0.28369140625
5.10482168197632 -0.28375244140625
5.10497522354126 -0.28375244140625
5.10717248916626 -0.283935546875
5.10781669616699 -0.283935546875
5.10837888717651 -0.283935546875
5.10933208465576 -0.28399658203125
5.10955476760864 -0.2840576171875
5.10986518859863 -0.2840576171875
5.11083221435547 -0.2840576171875
5.11096668243408 -0.2840576171875
5.11231327056885 -0.28411865234375
5.11307716369629 -0.2841796875
5.11383628845215 -0.28424072265625
5.11431407928467 -0.28424072265625
5.11565065383911 -0.2843017578125
5.11620235443115 -0.2843017578125
5.11650800704956 -0.2843017578125
5.11696290969849 -0.2843017578125
5.11781120300293 -0.28436279296875
5.11818552017212 -0.28436279296875
5.11979007720947 -0.284423828125
5.12013292312622 -0.28448486328125
5.12064647674561 -0.28448486328125
5.12229442596436 -0.28460693359375
5.12264823913574 -0.28466796875
5.12321424484253 -0.28472900390625
5.12361001968384 -0.28472900390625
5.12369823455811 -0.28472900390625
5.12400817871094 -0.28472900390625
5.1246771812439 -0.28472900390625
5.12890625 -0.285400390625
5.12919664382935 -0.285400390625
5.13006687164307 -0.28546142578125
5.1312689781189 -0.2855224609375
5.13156747817993 -0.2855224609375
5.1327109336853 -0.2855224609375
5.13289356231689 -0.28558349609375
5.13309478759766 -0.28558349609375
5.13362836837769 -0.28558349609375
5.13404655456543 -0.28558349609375
5.13464546203613 -0.28558349609375
5.13551759719849 -0.28564453125
5.1361083984375 -0.28564453125
5.13730669021606 -0.28570556640625
5.13783168792725 -0.28570556640625
5.13804340362549 -0.28570556640625
5.14265203475952 -0.28741455078125
5.14284896850586 -0.2877197265625
5.14319276809692 -0.28778076171875
5.14334583282471 -0.28778076171875
5.14385747909546 -0.287841796875
5.1445460319519 -0.287841796875
5.14538288116455 -0.287841796875
5.14547634124756 -0.287841796875
5.14579296112061 -0.287841796875
5.14593267440796 -0.287841796875
5.1462550163269 -0.28790283203125
5.14640712738037 -0.28790283203125
5.14679765701294 -0.28790283203125
5.14769172668457 -0.28790283203125
5.14803791046143 -0.28790283203125
5.1484637260437 -0.2879638671875
5.14900636672974 -0.2879638671875
5.14914512634277 -0.2879638671875
5.14916372299194 -0.2879638671875
5.15141582489014 -0.28826904296875
5.15189981460571 -0.28826904296875
5.15202236175537 -0.28826904296875
5.15287828445435 -0.288330078125
5.15348863601685 -0.288330078125
5.15379047393799 -0.288330078125
5.15442419052124 -0.288330078125
5.15450286865234 -0.288330078125
5.15713930130005 -0.28863525390625
5.15715456008911 -0.28863525390625
5.15767431259155 -0.28863525390625
5.15779209136963 -0.28863525390625
5.15963649749756 -0.28875732421875
5.16036653518677 -0.28875732421875
5.16075038909912 -0.28875732421875
5.16108655929565 -0.28875732421875
5.16131114959717 -0.28875732421875
5.16149377822876 -0.28875732421875
5.16337919235229 -0.2889404296875
5.16362047195435 -0.2889404296875
5.16372156143188 -0.2889404296875
5.16514921188354 -0.28900146484375
5.1657280921936 -0.28900146484375
5.16608047485352 -0.2890625
5.16630887985229 -0.2890625
5.16740322113037 -0.2890625
5.16752099990845 -0.2890625
5.16767454147339 -0.2890625
5.16798162460327 -0.2890625
5.16825294494629 -0.28912353515625
5.16854476928711 -0.28912353515625
5.16865348815918 -0.28912353515625
5.16915130615234 -0.28912353515625
5.1696834564209 -0.28912353515625
5.17108249664307 -0.289306640625
5.17128467559814 -0.289306640625
5.17268753051758 -0.28936767578125
5.17278671264648 -0.28936767578125
5.17286825180054 -0.28936767578125
5.17299699783325 -0.28936767578125
5.17308712005615 -0.28936767578125
5.17467594146729 -0.28948974609375
5.17549133300781 -0.28948974609375
5.17581033706665 -0.28948974609375
5.17646169662476 -0.28948974609375
5.17676544189453 -0.28955078125
5.17744398117065 -0.28955078125
5.17780208587646 -0.28955078125
5.17815637588501 -0.28955078125
5.17882442474365 -0.28961181640625
5.17897129058838 -0.28961181640625
5.17966365814209 -0.28961181640625
5.17972707748413 -0.28961181640625
5.18007707595825 -0.28961181640625
5.18042707443237 -0.28961181640625
5.18094253540039 -0.28961181640625
5.18096542358398 -0.28961181640625
5.1816577911377 -0.2896728515625
5.18175220489502 -0.2896728515625
5.18227767944336 -0.2896728515625
5.18241453170776 -0.2896728515625
5.18272542953491 -0.2896728515625
5.18314170837402 -0.2896728515625
5.18357181549072 -0.2896728515625
5.18364286422729 -0.2896728515625
5.18372821807861 -0.28973388671875
5.18409204483032 -0.28973388671875
5.18434762954712 -0.28973388671875
5.18456363677979 -0.28973388671875
5.18463754653931 -0.28973388671875
5.18473386764526 -0.28973388671875
5.18518495559692 -0.28973388671875
5.18623304367065 -0.289794921875
5.18630075454712 -0.289794921875
5.18640232086182 -0.289794921875
5.18649005889893 -0.289794921875
5.18664264678955 -0.289794921875
5.18682622909546 -0.289794921875
5.18693113327026 -0.289794921875
5.18721866607666 -0.289794921875
5.18740510940552 -0.289794921875
5.18759393692017 -0.289794921875
5.18879365921021 -0.2899169921875
5.18880748748779 -0.2899169921875
5.18885517120361 -0.2899169921875
5.18959140777588 -0.2899169921875
5.18965864181519 -0.2899169921875
5.19016647338867 -0.2899169921875
5.19028949737549 -0.28997802734375
5.19076299667358 -0.28997802734375
5.19108200073242 -0.28997802734375
5.19167184829712 -0.2900390625
5.19169425964355 -0.2900390625
5.19311332702637 -0.29010009765625
5.19346952438354 -0.2901611328125
5.19418668746948 -0.2901611328125
5.19420051574707 -0.2901611328125
5.19434499740601 -0.2901611328125
5.19437837600708 -0.2901611328125
5.19448661804199 -0.2901611328125
5.19456434249878 -0.2901611328125
5.19568395614624 -0.29034423828125
5.19581937789917 -0.29034423828125
5.19616508483887 -0.29034423828125
5.19650220870972 -0.29034423828125
5.19672584533691 -0.29034423828125
5.1977162361145 -0.2904052734375
5.19850015640259 -0.2904052734375
5.1987943649292 -0.2904052734375
5.19916534423828 -0.2904052734375
5.19962644577026 -0.2904052734375
5.20011711120605 -0.29046630859375
5.2007794380188 -0.29046630859375
5.2008695602417 -0.29046630859375
5.20088338851929 -0.29046630859375
5.20129585266113 -0.29046630859375
5.20160722732544 -0.29046630859375
5.20196771621704 -0.29046630859375
5.2025671005249 -0.29046630859375
5.20264101028442 -0.29046630859375
5.20265436172485 -0.29046630859375
5.20293474197388 -0.29046630859375
5.20320177078247 -0.29052734375
5.20330238342285 -0.29052734375
5.20366096496582 -0.29052734375
5.2037205696106 -0.29052734375
5.20381307601929 -0.29052734375
5.20617246627808 -0.2908935546875
5.2067232131958 -0.29095458984375
5.20673704147339 -0.29095458984375
5.20684766769409 -0.29095458984375
5.20711421966553 -0.29095458984375
5.20750761032104 -0.29095458984375
5.20762348175049 -0.291015625
5.20767211914062 -0.291015625
5.20773124694824 -0.291015625
5.20895433425903 -0.29107666015625
5.20917987823486 -0.29107666015625
5.20927619934082 -0.29107666015625
5.20930051803589 -0.29107666015625
5.20938348770142 -0.29107666015625
5.21033477783203 -0.29107666015625
5.21044445037842 -0.29107666015625
5.21046304702759 -0.29107666015625
5.21053504943848 -0.29107666015625
5.21077871322632 -0.29107666015625
5.21078395843506 -0.29107666015625
5.21089887619019 -0.29107666015625
5.21107530593872 -0.29107666015625
5.2113208770752 -0.29107666015625
5.21179580688477 -0.29107666015625
5.21205949783325 -0.2911376953125
5.21207284927368 -0.2911376953125
5.21262979507446 -0.2911376953125
5.21288251876831 -0.2911376953125
5.21312427520752 -0.2911376953125
5.21426105499268 -0.2911376953125
5.21436977386475 -0.2911376953125
5.21463203430176 -0.2911376953125
5.21476697921753 -0.2911376953125
5.21507167816162 -0.2911376953125
5.21571969985962 -0.2911376953125
5.21580934524536 -0.2911376953125
5.2159571647644 -0.29119873046875
5.21627950668335 -0.29119873046875
5.21654844284058 -0.29119873046875
5.21660661697388 -0.29119873046875
5.21661996841431 -0.29119873046875
5.21706247329712 -0.29119873046875
5.21729707717896 -0.29119873046875
5.21757888793945 -0.29119873046875
5.21774959564209 -0.29119873046875
5.2178258895874 -0.29119873046875
5.21878242492676 -0.291259765625
5.21900272369385 -0.291259765625
5.21908378601074 -0.291259765625
5.2194299697876 -0.291259765625
5.21963691711426 -0.291259765625
5.21965503692627 -0.291259765625
5.21996927261353 -0.291259765625
5.22031450271606 -0.291259765625
5.22036170959473 -0.291259765625
5.220534324646 -0.291259765625
5.22054719924927 -0.291259765625
5.22067022323608 -0.291259765625
5.22106981277466 -0.29132080078125
5.22114562988281 -0.29132080078125
5.22131252288818 -0.29132080078125
5.2213568687439 -0.29132080078125
5.22141933441162 -0.29132080078125
5.22179508209229 -0.29132080078125
5.22232866287231 -0.29132080078125
5.22234201431274 -0.29132080078125
5.22278690338135 -0.29132080078125
5.22314262390137 -0.29132080078125
5.22321557998657 -0.29132080078125
5.22333765029907 -0.29132080078125
5.22339487075806 -0.29132080078125
5.22350883483887 -0.29132080078125
5.22355556488037 -0.29132080078125
5.22386980056763 -0.29132080078125
5.22412109375 -0.29132080078125
5.22440099716187 -0.29132080078125
5.22476100921631 -0.2913818359375
5.22477626800537 -0.2913818359375
5.22486162185669 -0.2913818359375
5.22514629364014 -0.2913818359375
5.22533750534058 -0.2913818359375
5.22538423538208 -0.2913818359375
5.22587251663208 -0.2913818359375
5.22602462768555 -0.2913818359375
5.22608947753906 -0.2913818359375
5.22610235214233 -0.2913818359375
5.22655630111694 -0.2913818359375
5.22697353363037 -0.2913818359375
5.22702217102051 -0.2913818359375
5.22724628448486 -0.2913818359375
5.22726202011108 -0.2913818359375
5.22732591629028 -0.2913818359375
5.22746753692627 -0.2913818359375
5.22757577896118 -0.2913818359375
5.22778129577637 -0.2913818359375
5.22779417037964 -0.2913818359375
5.22792530059814 -0.2913818359375
5.22793054580688 -0.2913818359375
5.22803831100464 -0.2913818359375
5.22914171218872 -0.29144287109375
5.22969961166382 -0.29150390625
5.22982501983643 -0.29150390625
5.23047208786011 -0.29150390625
5.23101043701172 -0.29150390625
5.23110485076904 -0.29150390625
5.23118162155151 -0.29150390625
5.23139810562134 -0.29150390625
5.23156881332397 -0.29150390625
5.23177766799927 -0.29150390625
5.23219299316406 -0.29150390625
5.23240375518799 -0.29150390625
5.23258447647095 -0.29150390625
5.23333358764648 -0.29150390625
5.23337173461914 -0.29150390625
5.23354959487915 -0.29156494140625
5.23400068283081 -0.29156494140625
5.23468685150146 -0.29156494140625
5.23479318618774 -0.29156494140625
5.23489904403687 -0.29156494140625
5.23491430282593 -0.29156494140625
5.2351016998291 -0.29156494140625
5.23536920547485 -0.29156494140625
5.23586416244507 -0.2916259765625
5.23615407943726 -0.2916259765625
5.23619699478149 -0.2916259765625
5.23638868331909 -0.2916259765625
5.23649215698242 -0.2916259765625
5.23663282394409 -0.2916259765625
5.23671627044678 -0.2916259765625
5.23712396621704 -0.2916259765625
5.23723936080933 -0.2916259765625
5.23740816116333 -0.2916259765625
5.23759126663208 -0.2916259765625
5.23782014846802 -0.2916259765625
5.23825168609619 -0.2916259765625
5.23871326446533 -0.2916259765625
5.23882102966309 -0.2916259765625
5.2389965057373 -0.2916259765625
5.23919200897217 -0.2916259765625
5.23920917510986 -0.2916259765625
5.23961496353149 -0.2916259765625
5.24034690856934 -0.29168701171875
5.24059915542603 -0.29168701171875
5.24071645736694 -0.29168701171875
5.24086093902588 -0.29168701171875
5.24100303649902 -0.29168701171875
5.24102830886841 -0.29168701171875
5.24133491516113 -0.29168701171875
5.24140214920044 -0.29168701171875
5.24153423309326 -0.29168701171875
5.24190998077393 -0.29168701171875
5.24200439453125 -0.29168701171875
5.24229049682617 -0.29168701171875
5.24252891540527 -0.29168701171875
5.24256896972656 -0.29168701171875
5.24274778366089 -0.29168701171875
5.24282693862915 -0.29168701171875
5.24289417266846 -0.29168701171875
5.24336528778076 -0.291748046875
5.24356889724731 -0.291748046875
5.24373960494995 -0.291748046875
5.2442102432251 -0.291748046875
5.24439096450806 -0.291748046875
5.24460601806641 -0.291748046875
5.24513483047485 -0.291748046875
5.24535465240479 -0.29180908203125
5.24539184570312 -0.29180908203125
5.24556446075439 -0.29180908203125
5.2457914352417 -0.29180908203125
5.24590730667114 -0.29180908203125
5.24617338180542 -0.29180908203125
5.24637794494629 -0.29180908203125
5.24650859832764 -0.29180908203125
5.24666118621826 -0.29180908203125
5.24679660797119 -0.29180908203125
5.2469687461853 -0.29180908203125
5.24715280532837 -0.29180908203125
5.24725389480591 -0.29180908203125
5.24731540679932 -0.29180908203125
5.24747467041016 -0.29180908203125
5.2475905418396 -0.29180908203125
5.24770307540894 -0.29180908203125
5.24820613861084 -0.29180908203125
5.24833869934082 -0.29180908203125
5.2483434677124 -0.29180908203125
5.24871873855591 -0.29180908203125
5.24895095825195 -0.29180908203125
5.24934768676758 -0.29180908203125
5.24945783615112 -0.29180908203125
5.24982404708862 -0.29180908203125
5.24999046325684 -0.29180908203125
5.24999523162842 -0.29180908203125
5.25002956390381 -0.29180908203125
5.25029325485229 -0.2918701171875
5.25229692459106 -0.29205322265625
5.25254249572754 -0.29205322265625
5.25268793106079 -0.29205322265625
5.2531418800354 -0.29205322265625
5.25338649749756 -0.29205322265625
5.25373792648315 -0.29205322265625
5.25440549850464 -0.29205322265625
5.25522422790527 -0.29205322265625
5.25527715682983 -0.29205322265625
5.25547504425049 -0.29205322265625
5.25553321838379 -0.29205322265625
5.25554037094116 -0.29205322265625
5.25586080551147 -0.2921142578125
5.2560920715332 -0.2921142578125
5.25639057159424 -0.2921142578125
5.25647735595703 -0.2921142578125
5.25651073455811 -0.2921142578125
5.25656127929688 -0.2921142578125
5.25669622421265 -0.2921142578125
5.25679206848145 -0.2921142578125
5.25698947906494 -0.2921142578125
5.25699901580811 -0.2921142578125
5.25764989852905 -0.2921142578125
5.25766181945801 -0.2921142578125
5.25769996643066 -0.2921142578125
5.25777196884155 -0.2921142578125
5.25826835632324 -0.2921142578125
5.2583212852478 -0.2921142578125
5.25834989547729 -0.2921142578125
5.25844573974609 -0.2921142578125
5.25862789154053 -0.2921142578125
5.25866603851318 -0.2921142578125
5.25880002975464 -0.2921142578125
5.25883817672729 -0.2921142578125
5.25908470153809 -0.2921142578125
5.25908470153809 -0.2921142578125
5.2591347694397 -0.2921142578125
5.25922107696533 -0.2921142578125
5.2593789100647 -0.2921142578125
5.25964641571045 -0.2921142578125
5.25967979431152 -0.2921142578125
5.25978517532349 -0.2921142578125
5.26002359390259 -0.2921142578125
5.26018810272217 -0.2921142578125
5.26052236557007 -0.29217529296875
5.26065301895142 -0.29217529296875
5.26065301895142 -0.29217529296875
5.2610034942627 -0.29217529296875
5.26107025146484 -0.29217529296875
5.26128911972046 -0.29217529296875
5.26178121566772 -0.29217529296875
5.26179313659668 -0.29217529296875
5.26189088821411 -0.29217529296875
5.2620096206665 -0.29217529296875
5.26201438903809 -0.29217529296875
5.26223993301392 -0.29217529296875
5.2622447013855 -0.29217529296875
5.26278305053711 -0.292236328125
5.26293516159058 -0.292236328125
5.26358413696289 -0.292236328125
5.26363849639893 -0.292236328125
5.26365280151367 -0.292236328125
5.26378536224365 -0.292236328125
5.26385354995728 -0.292236328125
5.2639741897583 -0.292236328125
5.26414442062378 -0.292236328125
5.26415395736694 -0.292236328125
5.2646689414978 -0.292236328125
5.26503038406372 -0.292236328125
5.26505851745605 -0.292236328125
5.26537704467773 -0.292236328125
5.26553010940552 -0.292236328125
5.265869140625 -0.292236328125
5.26591157913208 -0.292236328125
5.26609754562378 -0.292236328125
5.26631164550781 -0.292236328125
5.26657485961914 -0.29229736328125
5.2667441368103 -0.29229736328125
5.26675605773926 -0.29229736328125
5.26688289642334 -0.29229736328125
5.26705455780029 -0.29229736328125
5.26711797714233 -0.29229736328125
5.26792001724243 -0.29229736328125
5.26793622970581 -0.29229736328125
5.26794815063477 -0.29229736328125
5.26829242706299 -0.29229736328125
5.26872777938843 -0.2923583984375
5.26873922348022 -0.2923583984375
5.26966238021851 -0.2923583984375
5.27003574371338 -0.2923583984375
5.27004957199097 -0.2923583984375
5.27016162872314 -0.2923583984375
5.27017068862915 -0.2923583984375
5.27043437957764 -0.2923583984375
5.27056217193604 -0.2923583984375
5.27056694030762 -0.2923583984375
5.27112579345703 -0.2923583984375
5.27120494842529 -0.2923583984375
5.27120923995972 -0.2923583984375
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{OF}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI},
xtick={0,1,2,3},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={4.9},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=4.9777868270874,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.256587982177734, ymax=0.0122184753417969,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c15)}
]
\addplot [ultra thick, brown,dashed]
table {%
1.04139268398285 0
1.38021123409271 -0.0001220703125
1.6020599603653 -0.0001220703125
1.69896996021271 -0.0001220703125
1.77085208892822 -0.0001220703125
1.83250892162323 -0.0001220703125
2.98045778274536 -0.0013427734375
3.01661562919617 -0.0023193359375
3.0468852519989 -0.00244140625
3.08919835090637 -0.0025634765625
3.12123155593872 -0.002685546875
3.17318630218506 -0.0028076171875
3.29380440711975 -0.0030517578125
3.32715439796448 -0.003173828125
3.41463923454285 -0.0035400390625
3.45086479187012 -0.00390625
3.48685526847839 -0.00439453125
3.49554443359375 -0.0045166015625
3.54082989692688 -0.005859375
3.57391548156738 -0.006591796875
3.59703660011292 -0.0069580078125
3.63688898086548 -0.0086669921875
3.67942786216736 -0.0113525390625
3.70156788825989 -0.012451171875
3.73623704910278 -0.012939453125
3.74554324150085 -0.0133056640625
3.7680459022522 -0.0142822265625
3.78368926048279 -0.0147705078125
3.80229473114014 -0.015869140625
3.84441494941711 -0.0179443359375
3.8728551864624 -0.018798828125
3.9104642868042 -0.02294921875
3.94581317901611 -0.02685546875
3.99158048629761 -0.03076171875
4.01224660873413 -0.035400390625
4.03885841369629 -0.0389404296875
4.04960584640503 -0.0426025390625
4.07976007461548 -0.048828125
4.10250234603882 -0.0546875
4.11915683746338 -0.0587158203125
4.13735389709473 -0.06298828125
4.15048027038574 -0.0662841796875
4.16423368453979 -0.069091796875
4.17713212966919 -0.072509765625
4.18859100341797 -0.0758056640625
4.20357656478882 -0.07763671875
4.21569061279297 -0.0809326171875
4.22476625442505 -0.0828857421875
4.24256610870361 -0.088134765625
4.24983406066895 -0.0909423828125
4.26266479492188 -0.0950927734375
4.28053283691406 -0.099609375
4.29170179367065 -0.1082763671875
4.29769468307495 -0.1112060546875
4.31291770935059 -0.1156005859375
4.3254337310791 -0.121337890625
4.32986545562744 -0.123291015625
4.34020614624023 -0.1270751953125
4.35106134414673 -0.1282958984375
4.35900020599365 -0.1297607421875
4.37147426605225 -0.1319580078125
4.37741565704346 -0.133056640625
4.38767433166504 -0.137939453125
4.39371538162231 -0.13916015625
4.40308618545532 -0.14111328125
4.41092920303345 -0.1439208984375
4.41534090042114 -0.1448974609375
4.42322969436646 -0.1478271484375
4.42618560791016 -0.1495361328125
4.43480825424194 -0.1507568359375
4.43843173980713 -0.1514892578125
4.45417404174805 -0.1605224609375
4.45815420150757 -0.16357421875
4.4638032913208 -0.164306640625
4.47139453887939 -0.166015625
4.47373485565186 -0.1663818359375
4.48251628875732 -0.170654296875
4.48484039306641 -0.17138671875
4.48873376846313 -0.1719970703125
4.49483633041382 -0.1728515625
4.50004434585571 -0.173583984375
4.50699186325073 -0.1741943359375
4.51000833511353 -0.1748046875
4.51586055755615 -0.175537109375
4.52142572402954 -0.1766357421875
4.52478551864624 -0.1771240234375
4.52976369857788 -0.1781005859375
4.53219366073608 -0.1783447265625
4.54352188110352 -0.1868896484375
4.54651784896851 -0.1883544921875
4.55159616470337 -0.189208984375
4.5585765838623 -0.1923828125
4.56278038024902 -0.193359375
4.56750869750977 -0.1953125
4.57016897201538 -0.196044921875
4.576744556427 -0.1981201171875
4.57930326461792 -0.19873046875
4.58887672424316 -0.203369140625
4.59104251861572 -0.2059326171875
4.59404993057251 -0.20654296875
4.59698152542114 -0.20703125
4.60103797912598 -0.2073974609375
4.60622024536133 -0.2109375
4.60954093933105 -0.21142578125
4.61214780807495 -0.2119140625
4.61687421798706 -0.21240234375
4.61933326721191 -0.213134765625
4.62079191207886 -0.2135009765625
4.62433385848999 -0.2142333984375
4.62600135803223 -0.21435546875
4.63069200515747 -0.2164306640625
4.63280153274536 -0.2171630859375
4.63742971420288 -0.2176513671875
4.64454698562622 -0.21923828125
4.64627647399902 -0.219482421875
4.64964628219604 -0.22021484375
4.65222692489624 -0.2205810546875
4.65470600128174 -0.220947265625
4.65936470031738 -0.2215576171875
4.66172742843628 -0.2220458984375
4.66347455978394 -0.222412109375
4.66435050964355 -0.22265625
4.66748094558716 -0.22314453125
4.67777109146118 -0.2294921875
4.67943716049194 -0.2318115234375
4.68320941925049 -0.232177734375
4.68504285812378 -0.2325439453125
4.69078063964844 -0.2335205078125
4.69279384613037 -0.2337646484375
4.70421075820923 -0.237548828125
4.70605182647705 -0.2392578125
4.7106671333313 -0.239990234375
4.71428775787354 -0.240234375
4.71669578552246 -0.240478515625
4.7204737663269 -0.2408447265625
4.72294616699219 -0.2412109375
4.727614402771 -0.24169921875
4.72904300689697 -0.241943359375
4.73232126235962 -0.242919921875
4.73387908935547 -0.2431640625
4.73834466934204 -0.24365234375
4.73901033401489 -0.243896484375
4.74219846725464 -0.244384765625
4.74394845962524 -0.2447509765625
4.74711656570435 -0.2449951171875
4.75675010681152 -0.2493896484375
4.75741863250732 -0.25
4.76039218902588 -0.2508544921875
4.76314353942871 -0.251220703125
4.76366758346558 -0.2513427734375
4.76559400558472 -0.25146484375
4.77042484283447 -0.251708984375
4.77234363555908 -0.251953125
4.77474308013916 -0.252197265625
4.77776002883911 -0.25244140625
4.77859973907471 -0.2528076171875
4.78022384643555 -0.2529296875
4.78272342681885 -0.2530517578125
4.7888822555542 -0.254150390625
4.79206943511963 -0.254638671875
4.79488515853882 -0.2550048828125
4.7973575592041 -0.2554931640625
4.80133533477783 -0.2559814453125
4.80271911621094 -0.25634765625
4.80465745925903 -0.256591796875
4.80635643005371 -0.2567138671875
4.81078338623047 -0.2589111328125
4.81482028961182 -0.260009765625
4.81666564941406 -0.26025390625
4.81906318664551 -0.260498046875
4.82443189620972 -0.2613525390625
4.82586717605591 -0.2623291015625
4.83021640777588 -0.263916015625
4.833580493927 -0.26416015625
4.83537340164185 -0.2645263671875
4.84338855743408 -0.2664794921875
4.84484958648682 -0.2669677734375
4.84764671325684 -0.267333984375
4.84937047958374 -0.2674560546875
4.85565853118896 -0.2691650390625
4.85735654830933 -0.2694091796875
4.85934829711914 -0.2696533203125
4.86033201217651 -0.2696533203125
4.86609220504761 -0.275390625
4.86751461029053 -0.277099609375
4.87045669555664 -0.277587890625
4.87329149246216 -0.2779541015625
4.87547206878662 -0.2784423828125
4.87826299667358 -0.2791748046875
4.88145875930786 -0.27978515625
4.88332653045654 -0.280029296875
4.88507270812988 -0.2803955078125
4.88745403289795 -0.281005859375
4.89335107803345 -0.282470703125
4.89679050445557 -0.283447265625
4.89824247360229 -0.28369140625
4.90036725997925 -0.283935546875
4.9071478843689 -0.2860107421875
4.90859746932983 -0.286376953125
4.9113335609436 -0.2869873046875
4.91490364074707 -0.2872314453125
4.91547393798828 -0.287353515625
4.91632223129272 -0.2874755859375
4.91838693618774 -0.287841796875
4.92038440704346 -0.2879638671875
4.9238600730896 -0.288330078125
4.92431545257568 -0.2886962890625
4.92585849761963 -0.288818359375
4.92926073074341 -0.289794921875
4.9298529624939 -0.2900390625
4.93383646011353 -0.2919921875
4.93528032302856 -0.292236328125
4.9360408782959 -0.2923583984375
4.93991851806641 -0.296142578125
4.94125318527222 -0.2969970703125
4.94373178482056 -0.2978515625
4.94516801834106 -0.298095703125
4.94841766357422 -0.2984619140625
4.95028686523438 -0.298828125
4.95218706130981 -0.2989501953125
4.95365333557129 -0.2991943359375
4.95516300201416 -0.299560546875
4.95686435699463 -0.2996826171875
4.95752096176147 -0.2998046875
4.96054220199585 -0.3004150390625
4.96520185470581 -0.30126953125
4.96604299545288 -0.302001953125
4.96792697906494 -0.30224609375
4.97034692764282 -0.3026123046875
4.97193908691406 -0.3028564453125
4.97357130050659 -0.302978515625
4.97813034057617 -0.308349609375
4.9806079864502 -0.31005859375
4.98158311843872 -0.3101806640625
4.98294496536255 -0.3109130859375
4.98666858673096 -0.3125
4.9882869720459 -0.3128662109375
4.98916959762573 -0.31298828125
4.99014329910278 -0.313232421875
4.99300384521484 -0.3138427734375
4.99349784851074 -0.3140869140625
4.99566173553467 -0.3148193359375
4.99652481079102 -0.31494140625
4.99735164642334 -0.3150634765625
4.99801969528198 -0.315185546875
4.99916076660156 -0.315185546875
4.99979162216187 -0.3153076171875
5.00211429595947 -0.316650390625
5.00303792953491 -0.3170166015625
5.00380086898804 -0.317138671875
5.00529193878174 -0.3173828125
5.00589227676392 -0.3173828125
5.00632047653198 -0.3173828125
5.00743198394775 -0.3175048828125
5.00839567184448 -0.317626953125
5.01049518585205 -0.31787109375
5.01089763641357 -0.31787109375
5.01418018341064 -0.318359375
5.01442813873291 -0.3184814453125
5.01492357254028 -0.3184814453125
5.01548528671265 -0.3184814453125
5.01606750488281 -0.3184814453125
5.01948165893555 -0.31982421875
5.02066802978516 -0.3204345703125
5.02198266983032 -0.320556640625
5.02251100540161 -0.320556640625
5.02346229553223 -0.320556640625
5.02392292022705 -0.3206787109375
5.02508878707886 -0.3206787109375
5.02599763870239 -0.32080078125
5.02641487121582 -0.32080078125
5.02719879150391 -0.32080078125
5.027512550354 -0.32080078125
5.02823352813721 -0.3209228515625
5.02944850921631 -0.3209228515625
5.03028774261475 -0.321044921875
5.0306077003479 -0.321044921875
5.0313720703125 -0.3211669921875
5.03191328048706 -0.3211669921875
5.03247356414795 -0.3211669921875
5.0332145690918 -0.3212890625
5.03372526168823 -0.3212890625
5.03604984283447 -0.321533203125
5.03676843643188 -0.3216552734375
5.03806734085083 -0.3216552734375
5.03821468353271 -0.3216552734375
5.04104518890381 -0.3226318359375
5.04221296310425 -0.3228759765625
5.04305171966553 -0.322998046875
5.04417514801025 -0.322998046875
5.0451192855835 -0.3231201171875
5.04621410369873 -0.3231201171875
5.0475902557373 -0.3231201171875
5.04787063598633 -0.3231201171875
5.04892301559448 -0.3231201171875
5.05090141296387 -0.3233642578125
5.05159616470337 -0.3233642578125
5.0532398223877 -0.32373046875
5.05387306213379 -0.3238525390625
5.05473947525024 -0.323974609375
5.05561923980713 -0.323974609375
5.05629110336304 -0.323974609375
5.05667638778687 -0.323974609375
5.05724382400513 -0.323974609375
5.05853986740112 -0.32421875
5.05926418304443 -0.32421875
5.06055450439453 -0.3243408203125
5.06169748306274 -0.3243408203125
5.06202125549316 -0.324462890625
5.06284141540527 -0.324462890625
5.06341981887817 -0.324462890625
5.06388854980469 -0.324462890625
5.06565809249878 -0.3248291015625
5.06628847122192 -0.3248291015625
5.0677809715271 -0.3248291015625
5.06880521774292 -0.324951171875
5.06937599182129 -0.324951171875
5.0698823928833 -0.324951171875
5.07039976119995 -0.3250732421875
5.07118606567383 -0.3250732421875
5.07183790206909 -0.3250732421875
5.07231998443604 -0.3250732421875
5.07341051101685 -0.3251953125
5.07386493682861 -0.3253173828125
5.07522201538086 -0.3253173828125
5.07553577423096 -0.3253173828125
5.07706594467163 -0.3255615234375
5.07770586013794 -0.32568359375
5.07807588577271 -0.32568359375
5.07836961746216 -0.32568359375
5.07924270629883 -0.32568359375
5.07981061935425 -0.32568359375
5.08042812347412 -0.32568359375
5.08251953125 -0.325927734375
5.08288240432739 -0.3260498046875
5.08353137969971 -0.3260498046875
5.0838680267334 -0.3260498046875
5.0840539932251 -0.3260498046875
5.08464050292969 -0.3260498046875
5.08560800552368 -0.3260498046875
5.08617115020752 -0.3260498046875
5.08666944503784 -0.3260498046875
5.08734464645386 -0.326171875
5.08801889419556 -0.326171875
5.08810758590698 -0.326171875
5.08868885040283 -0.326171875
5.08945989608765 -0.326171875
5.08959436416626 -0.326171875
5.09040975570679 -0.326171875
5.09132242202759 -0.3262939453125
5.09161424636841 -0.3262939453125
5.09203243255615 -0.3262939453125
5.09283304214478 -0.3262939453125
5.0940375328064 -0.326416015625
5.09448862075806 -0.326416015625
5.09476804733276 -0.326416015625
5.09681272506714 -0.3267822265625
5.09702444076538 -0.326904296875
5.0971531867981 -0.326904296875
5.09734392166138 -0.326904296875
5.09848117828369 -0.3270263671875
5.09899663925171 -0.3270263671875
5.09967374801636 -0.3271484375
5.09975337982178 -0.3271484375
5.10060119628906 -0.3271484375
5.10100078582764 -0.3271484375
5.10145854949951 -0.3271484375
5.10340356826782 -0.3272705078125
5.10398149490356 -0.3272705078125
5.10440874099731 -0.3272705078125
5.1049919128418 -0.3272705078125
5.10564994812012 -0.3272705078125
5.1057825088501 -0.3272705078125
5.10673475265503 -0.327392578125
5.10739660263062 -0.327392578125
5.10774564743042 -0.327392578125
5.10849046707153 -0.327392578125
5.10858869552612 -0.327392578125
5.10864639282227 -0.327392578125
5.10883903503418 -0.327392578125
5.10983467102051 -0.3275146484375
5.11077833175659 -0.3275146484375
5.11113119125366 -0.32763671875
5.11155843734741 -0.32763671875
5.11193084716797 -0.32763671875
5.1123571395874 -0.32763671875
5.11242723464966 -0.32763671875
5.11260509490967 -0.32763671875
5.11286640167236 -0.32763671875
5.11481428146362 -0.3277587890625
5.11493110656738 -0.3277587890625
5.11503458023071 -0.3277587890625
5.1151442527771 -0.3277587890625
5.11542415618896 -0.3277587890625
5.11650466918945 -0.327880859375
5.11776494979858 -0.327880859375
5.11828470230103 -0.327880859375
5.11843013763428 -0.327880859375
5.11867475509644 -0.327880859375
5.11882019042969 -0.327880859375
5.11892890930176 -0.327880859375
5.11906433105469 -0.327880859375
5.11970138549805 -0.327880859375
5.11973428726196 -0.327880859375
5.12031745910645 -0.327880859375
5.12060689926147 -0.327880859375
5.12064647674561 -0.327880859375
5.12083721160889 -0.327880859375
5.12097835540771 -0.3280029296875
5.12098503112793 -0.3280029296875
5.12112283706665 -0.3280029296875
5.12134647369385 -0.3280029296875
5.12181234359741 -0.3280029296875
5.12192058563232 -0.3280029296875
5.12225532531738 -0.3280029296875
5.12257957458496 -0.3280029296875
5.1229887008667 -0.3280029296875
5.12299537658691 -0.3280029296875
5.12338447570801 -0.3280029296875
5.12339115142822 -0.3280029296875
5.12349557876587 -0.3280029296875
5.12396907806396 -0.3280029296875
5.12410974502563 -0.3280029296875
5.1248140335083 -0.3280029296875
5.1248984336853 -0.328125
5.1252179145813 -0.328125
5.12543916702271 -0.328125
5.12566995620728 -0.328125
5.12647581100464 -0.328125
5.12706279754639 -0.328125
5.12706899642944 -0.328125
5.12756824493408 -0.328125
5.128005027771 -0.328125
5.12887382507324 -0.328125
5.12903881072998 -0.3282470703125
5.12932872772217 -0.3282470703125
5.12957048416138 -0.3282470703125
5.12964820861816 -0.3282470703125
5.13024044036865 -0.3282470703125
5.130784034729 -0.3282470703125
5.130934715271 -0.3282470703125
5.13143253326416 -0.3282470703125
5.13145160675049 -0.3282470703125
5.13163805007935 -0.3282470703125
5.13167953491211 -0.3282470703125
5.13269805908203 -0.328369140625
5.13351678848267 -0.328369140625
5.13384199142456 -0.328369140625
5.13400173187256 -0.328369140625
5.13420248031616 -0.328369140625
5.13453102111816 -0.328369140625
5.13493204116821 -0.328369140625
5.13510084152222 -0.328369140625
5.13575601577759 -0.328369140625
5.1358699798584 -0.328369140625
5.13611793518066 -0.328369140625
5.13644170761108 -0.328369140625
5.13647651672363 -0.328369140625
5.13684415817261 -0.328369140625
5.13705635070801 -0.328369140625
5.13760709762573 -0.328369140625
5.13770866394043 -0.328369140625
5.13823318481445 -0.3284912109375
5.13861846923828 -0.3284912109375
5.13862466812134 -0.3284912109375
5.14107322692871 -0.32861328125
5.14158153533936 -0.3287353515625
5.14161920547485 -0.3287353515625
5.14278650283813 -0.3287353515625
5.14336776733398 -0.328857421875
5.14355182647705 -0.328857421875
5.14380788803101 -0.328857421875
5.14424085617065 -0.328857421875
5.14432811737061 -0.328857421875
5.14488220214844 -0.328857421875
5.14495992660522 -0.328857421875
5.14515924453735 -0.328857421875
5.14554119110107 -0.328857421875
5.1457462310791 -0.328857421875
5.14615917205811 -0.328857421875
5.14659309387207 -0.328857421875
5.14689970016479 -0.328857421875
5.1469988822937 -0.328857421875
5.1470513343811 -0.328857421875
5.14751577377319 -0.3289794921875
5.14785575866699 -0.3289794921875
5.14795112609863 -0.3289794921875
5.14831876754761 -0.3289794921875
5.14847326278687 -0.3289794921875
5.14865827560425 -0.3289794921875
5.14873218536377 -0.3289794921875
5.14907455444336 -0.3289794921875
5.1509313583374 -0.3289794921875
5.15100479125977 -0.3289794921875
5.15146493911743 -0.3289794921875
5.15155696868896 -0.3289794921875
5.15180158615112 -0.3289794921875
5.15191221237183 -0.3289794921875
5.15233421325684 -0.3291015625
5.15274095535278 -0.3291015625
5.15321731567383 -0.3291015625
5.15346717834473 -0.3291015625
5.15381479263306 -0.3291015625
5.15424728393555 -0.3291015625
5.15459728240967 -0.3291015625
5.15502023696899 -0.3291015625
5.15542411804199 -0.3291015625
5.15564250946045 -0.3291015625
5.15672159194946 -0.3292236328125
5.15712404251099 -0.3292236328125
5.15771055221558 -0.3292236328125
5.15812110900879 -0.329345703125
5.15853118896484 -0.329345703125
5.15888977050781 -0.329345703125
5.1592059135437 -0.329345703125
5.15956735610962 -0.329345703125
5.15989208221436 -0.329345703125
5.16030931472778 -0.329345703125
5.16073560714722 -0.329345703125
5.16106557846069 -0.329345703125
5.16126012802124 -0.329345703125
5.16168546676636 -0.329345703125
5.16241502761841 -0.3294677734375
5.16267204284668 -0.3294677734375
5.16306304931641 -0.3294677734375
5.16335821151733 -0.3294677734375
5.16376638412476 -0.3294677734375
5.16410303115845 -0.3294677734375
5.16470050811768 -0.3297119140625
5.16506624221802 -0.329833984375
5.1654372215271 -0.329833984375
5.16578435897827 -0.3299560546875
5.16607761383057 -0.3299560546875
5.16632652282715 -0.3299560546875
5.1666374206543 -0.3299560546875
5.16685628890991 -0.3299560546875
5.16724920272827 -0.3299560546875
5.16773653030396 -0.330078125
5.16799354553223 -0.330078125
5.16839742660522 -0.330078125
5.16868591308594 -0.3302001953125
5.1689305305481 -0.3302001953125
5.16942739486694 -0.330322265625
5.16967153549194 -0.330322265625
5.17017650604248 -0.330322265625
5.17068386077881 -0.330322265625
5.17087173461914 -0.330322265625
5.17144584655762 -0.3304443359375
5.17189884185791 -0.3304443359375
5.17215299606323 -0.3304443359375
5.1722936630249 -0.3304443359375
5.17255020141602 -0.33056640625
5.17296171188354 -0.33056640625
5.17313385009766 -0.33056640625
5.17357683181763 -0.33056640625
5.17400741577148 -0.33056640625
5.17434787750244 -0.33056640625
5.17449569702148 -0.33056640625
5.17502450942993 -0.3306884765625
5.17525386810303 -0.3306884765625
5.17556381225586 -0.3306884765625
5.1758508682251 -0.3306884765625
5.17632579803467 -0.3306884765625
5.17648506164551 -0.3306884765625
5.17664098739624 -0.3306884765625
5.17669868469238 -0.3306884765625
5.17734909057617 -0.330810546875
5.17746734619141 -0.330810546875
5.17807006835938 -0.330810546875
5.1782169342041 -0.330810546875
5.17872667312622 -0.330810546875
5.17891931533813 -0.330810546875
5.17955732345581 -0.330810546875
5.17977571487427 -0.330810546875
5.17994213104248 -0.330810546875
5.18006277084351 -0.330810546875
5.18051290512085 -0.330810546875
5.18083095550537 -0.330810546875
5.18096542358398 -0.330810546875
5.18113422393799 -0.330810546875
5.18134021759033 -0.330810546875
5.18143177032471 -0.330810546875
5.18184089660645 -0.330810546875
5.18192338943481 -0.330810546875
5.18209505081177 -0.330810546875
5.18231201171875 -0.330810546875
5.18238306045532 -0.330810546875
5.18263721466064 -0.330810546875
5.1827597618103 -0.3309326171875
5.18280267715454 -0.3309326171875
5.18345499038696 -0.3309326171875
5.18351459503174 -0.3309326171875
5.18406105041504 -0.3309326171875
5.18454074859619 -0.3309326171875
5.18462896347046 -0.3309326171875
5.18468284606934 -0.3309326171875
5.18490982055664 -0.3309326171875
5.18493843078613 -0.3309326171875
5.1851282119751 -0.3309326171875
5.1872386932373 -0.3311767578125
5.1883602142334 -0.331298828125
5.18851804733276 -0.331298828125
5.18865585327148 -0.331298828125
5.18890857696533 -0.331298828125
5.18909692764282 -0.331298828125
5.18913078308105 -0.331298828125
5.18926000595093 -0.331298828125
5.18929100036621 -0.331298828125
5.18983268737793 -0.331298828125
5.1900372505188 -0.331298828125
5.19040441513062 -0.331298828125
5.19048023223877 -0.331298828125
5.19049692153931 -0.331298828125
5.19083309173584 -0.3314208984375
5.1914005279541 -0.3314208984375
5.19163274765015 -0.3314208984375
5.19220781326294 -0.3314208984375
5.19240856170654 -0.3314208984375
5.19295215606689 -0.3314208984375
5.19301319122314 -0.3314208984375
5.19301891326904 -0.3314208984375
5.19316339492798 -0.3314208984375
5.19322204589844 -0.3314208984375
5.19344997406006 -0.3314208984375
5.19374513626099 -0.3314208984375
5.19375038146973 -0.3314208984375
5.19401168823242 -0.3314208984375
5.19404792785645 -0.3314208984375
5.19405364990234 -0.3314208984375
5.19436979293823 -0.3314208984375
5.19437551498413 -0.3314208984375
5.19438123703003 -0.3314208984375
5.19439506530762 -0.3314208984375
5.19440078735352 -0.3314208984375
5.19486951828003 -0.3314208984375
5.19511318206787 -0.3314208984375
5.19524335861206 -0.33154296875
5.19533777236938 -0.33154296875
5.19534349441528 -0.33154296875
5.19543170928955 -0.33154296875
5.19543743133545 -0.33154296875
5.19557046890259 -0.33154296875
5.19557571411133 -0.33154296875
5.19558143615723 -0.33154296875
5.19558715820312 -0.33154296875
5.19628381729126 -0.33154296875
5.19628953933716 -0.33154296875
5.19629526138306 -0.33154296875
5.196457862854 -0.33154296875
5.19654941558838 -0.33154296875
5.19655466079712 -0.33154296875
5.19656038284302 -0.33154296875
5.19656562805176 -0.33154296875
5.19674825668335 -0.33154296875
5.19675350189209 -0.33154296875
5.19675922393799 -0.33154296875
5.19676446914673 -0.33154296875
5.19677019119263 -0.33154296875
5.19677019119263 -0.33154296875
5.19787836074829 -0.33154296875
5.19812917709351 -0.33154296875
5.19813442230225 -0.33154296875
5.19814014434814 -0.33154296875
5.19814538955688 -0.33154296875
5.19816207885742 -0.33154296875
5.19816732406616 -0.33154296875
5.19817304611206 -0.33154296875
5.19817876815796 -0.33154296875
5.1982307434082 -0.33154296875
5.1988410949707 -0.33154296875
5.19884395599365 -0.33154296875
};
\addplot [ultra thick, blue]
table {%
0 0
0 -0.0001220703125
0 -0.0001220703125
0 -0.0001220703125
0 -0.0001220703125
0 -0.0001220703125
0.30103000998497 -0.0001220703125
0.30103000998497 -0.0001220703125
0.30103000998497 -0.000244140625
0.30103000998497 -0.000244140625
0.30103000998497 -0.000244140625
0.477121233940125 -0.000244140625
0.477121233940125 -0.0003662109375
0.477121233940125 -0.0003662109375
0.477121233940125 -0.0003662109375
0.698970019817352 -0.0003662109375
0.698970019817352 -0.0003662109375
0.698970019817352 -0.0003662109375
0.778151273727417 -0.00048828125
0.778151273727417 -0.00048828125
0.778151273727417 -0.00048828125
1 -0.001220703125
1.04139268398285 -0.00146484375
1.07918119430542 -0.0015869140625
1.17609131336212 -0.001708984375
1.20412003993988 -0.0018310546875
1.41497337818146 -0.0028076171875
1.50514996051788 -0.0040283203125
1.6334685087204 -0.00537109375
1.65321254730225 -0.0074462890625
1.66275787353516 -0.0079345703125
1.77085208892822 -0.00830078125
1.80618000030518 -0.0093994140625
1.88649070262909 -0.01220703125
1.92941892147064 -0.013671875
1.95424246788025 -0.014404296875
2.00432133674622 -0.0147705078125
2.07918119430542 -0.0172119140625
2.10720992088318 -0.0191650390625
2.17318630218506 -0.019775390625
2.21484375 -0.0230712890625
2.25527238845825 -0.0252685546875
2.26951289176941 -0.0272216796875
2.290034532547 -0.0291748046875
2.36735582351685 -0.033203125
2.40483379364014 -0.0372314453125
2.44090914726257 -0.03955078125
2.48572134971619 -0.0421142578125
2.49968719482422 -0.0439453125
2.53147888183594 -0.0462646484375
2.55145001411438 -0.049072265625
2.57054305076599 -0.0499267578125
2.58883166313171 -0.0516357421875
2.62428212165833 -0.0526123046875
2.6655809879303 -0.0611572265625
2.70415043830872 -0.065673828125
2.767897605896 -0.0762939453125
2.78031730651855 -0.087158203125
2.79934048652649 -0.090576171875
2.8188853263855 -0.094970703125
2.85064625740051 -0.1065673828125
2.86213135719299 -0.1107177734375
2.87390160560608 -0.1138916015625
2.89486956596375 -0.1187744140625
2.9143431186676 -0.12158203125
2.92168641090393 -0.1236572265625
2.94841289520264 -0.132568359375
2.95327639579773 -0.134033203125
2.96189546585083 -0.1351318359375
2.9642596244812 -0.1357421875
2.97954845428467 -0.13720703125
2.99299502372742 -0.1380615234375
3.00173377990723 -0.1396484375
3.00945091247559 -0.140869140625
3.02653336524963 -0.1424560546875
3.03981065750122 -0.1446533203125
3.04493165016174 -0.1455078125
3.06220579147339 -0.1463623046875
3.06744289398193 -0.1470947265625
3.07188200950623 -0.1475830078125
3.08206701278687 -0.14990234375
3.09447121620178 -0.1507568359375
3.10380363464355 -0.1527099609375
3.10822677612305 -0.1534423828125
3.11760258674622 -0.155029296875
3.14270234107971 -0.1566162109375
3.15442395210266 -0.158935546875
3.15896534919739 -0.16015625
3.16583752632141 -0.16064453125
3.17405986785889 -0.161376953125
3.17609119415283 -0.161865234375
3.18808436393738 -0.164794921875
3.20330500602722 -0.1666259765625
3.20601582527161 -0.1671142578125
3.21298623085022 -0.1678466796875
3.22479200363159 -0.17041015625
3.22762966156006 -0.171875
3.23172426223755 -0.17236328125
3.23502326011658 -0.1729736328125
3.24129748344421 -0.1739501953125
3.24551272392273 -0.174560546875
3.2550311088562 -0.1763916015625
3.25767850875854 -0.1776123046875
3.26363611221313 -0.1781005859375
3.26552534103394 -0.178466796875
3.27531147003174 -0.1844482421875
3.28035068511963 -0.185302734375
3.29358339309692 -0.19384765625
3.29710364341736 -0.1962890625
3.30124711990356 -0.1971435546875
3.30984306335449 -0.197998046875
3.31281185150146 -0.1986083984375
3.31993842124939 -0.20068359375
3.32221937179565 -0.2021484375
3.32919430732727 -0.205078125
3.33061671257019 -0.2060546875
3.33344721794128 -0.2066650390625
3.34419560432434 -0.2149658203125
3.35102295875549 -0.217041015625
3.35679054260254 -0.2186279296875
3.35831570625305 -0.219482421875
3.36002516746521 -0.2198486328125
3.36380004882812 -0.2205810546875
3.36567521095276 -0.2213134765625
3.36958694458008 -0.2218017578125
3.37199091911316 -0.22216796875
3.380211353302 -0.228515625
3.38560628890991 -0.23046875
3.38916611671448 -0.23095703125
3.39111161231995 -0.231201171875
3.39776635169983 -0.2313232421875
3.39950060844421 -0.231689453125
3.40277695655823 -0.232421875
3.40534639358521 -0.232666015625
3.40891790390015 -0.2335205078125
3.41027092933655 -0.233642578125
3.41430473327637 -0.2354736328125
3.41912937164307 -0.2364501953125
3.42504477500916 -0.236572265625
3.42975234985352 -0.237548828125
3.43232774734497 -0.23779296875
3.43296933174133 -0.2379150390625
3.43600344657898 -0.2381591796875
3.43838405609131 -0.23828125
3.43901681900024 -0.2384033203125
3.44200921058655 -0.23876953125
3.44653725624084 -0.2393798828125
3.44824242591858 -0.2396240234375
3.44886088371277 -0.23974609375
3.4598445892334 -0.2418212890625
3.46119832992554 -0.2421875
3.46239805221558 -0.2423095703125
3.46448945999146 -0.24267578125
3.46671938896179 -0.2430419921875
3.47348690032959 -0.2435302734375
3.47465324401855 -0.24365234375
3.47625184059143 -0.243896484375
3.48015069961548 -0.2440185546875
3.48129940032959 -0.244140625
3.48727989196777 -0.2447509765625
3.48798632621765 -0.2452392578125
3.48925518989563 -0.245361328125
3.493736743927 -0.24560546875
3.50569248199463 -0.2498779296875
3.50650501251221 -0.251708984375
3.51094698905945 -0.2523193359375
3.51201701164246 -0.25244140625
3.51693177223206 -0.2529296875
3.52153038978577 -0.2535400390625
3.52309584617615 -0.253662109375
3.52698516845703 -0.25390625
3.52814507484436 -0.2540283203125
3.53364491462708 -0.2548828125
3.541579246521 -0.25537109375
3.54257655143738 -0.255615234375
3.55022835731506 -0.25732421875
3.55096173286438 -0.2579345703125
3.55230307579041 -0.258056640625
3.5583484172821 -0.2587890625
3.56086277961731 -0.259033203125
3.56288743019104 -0.259521484375
3.56667327880859 -0.259765625
3.57252311706543 -0.2606201171875
3.57379961013794 -0.2608642578125
3.58035469055176 -0.2623291015625
3.58172225952148 -0.2630615234375
3.58376550674438 -0.263427734375
3.58444428443909 -0.2635498046875
3.59428215026855 -0.268798828125
3.59549617767334 -0.2703857421875
3.59802412986755 -0.270751953125
3.60346913337708 -0.27197265625
3.60691857337952 -0.27294921875
3.61012768745422 -0.2733154296875
3.6133131980896 -0.273681640625
3.61595010757446 -0.27392578125
3.61836194992065 -0.274169921875
3.62190294265747 -0.274658203125
3.62335276603699 -0.275146484375
3.62551832199097 -0.2755126953125
3.62981724739075 -0.275634765625
3.6326596736908 -0.2762451171875
3.63477945327759 -0.2764892578125
3.6403820514679 -0.2789306640625
3.64226651191711 -0.279541015625
3.64463543891907 -0.280029296875
3.6475784778595 -0.2803955078125
3.65417647361755 -0.2828369140625
3.65513849258423 -0.283447265625
3.65648150444031 -0.28369140625
3.66105508804321 -0.2845458984375
3.66417169570923 -0.2850341796875
3.66754627227783 -0.285888671875
3.66857218742371 -0.286376953125
3.67108035087585 -0.2864990234375
3.67329740524292 -0.286865234375
3.67513656616211 -0.2874755859375
3.67760705947876 -0.28759765625
3.68106031417847 -0.2880859375
3.68358731269836 -0.288330078125
3.68547296524048 -0.2890625
3.68788552284241 -0.2891845703125
3.69019603729248 -0.2894287109375
3.69108152389526 -0.28955078125
3.69258260726929 -0.289794921875
3.69810056686401 -0.2923583984375
3.69983768463135 -0.29296875
3.70148158073425 -0.2930908203125
3.70182704925537 -0.293212890625
3.70251679420471 -0.29345703125
3.70517921447754 -0.293701171875
3.70774054527283 -0.294189453125
3.70986342430115 -0.2943115234375
3.71028661727905 -0.2945556640625
3.7106249332428 -0.2945556640625
3.71206021308899 -0.294677734375
3.71424579620361 -0.2950439453125
3.71466493606567 -0.2950439453125
3.7196626663208 -0.297119140625
3.72073793411255 -0.2977294921875
3.7215633392334 -0.2978515625
3.7223048210144 -0.2979736328125
3.72337365150452 -0.298095703125
3.72591161727905 -0.298583984375
3.72729730606079 -0.2987060546875
3.73271536827087 -0.301025390625
3.73311710357666 -0.3016357421875
3.73367857933044 -0.3017578125
3.7367947101593 -0.302001953125
3.73893904685974 -0.30224609375
3.74083614349365 -0.302490234375
3.74327445030212 -0.302734375
3.74429297447205 -0.302978515625
3.75004529953003 -0.3057861328125
3.75089383125305 -0.306396484375
3.7515869140625 -0.306640625
3.75442481040955 -0.3070068359375
3.75587487220764 -0.3074951171875
3.75762367248535 -0.3077392578125
3.75838184356689 -0.3079833984375
3.76027154922485 -0.3082275390625
3.76380228996277 -0.309326171875
3.76462435722351 -0.3096923828125
3.76574301719666 -0.3099365234375
3.76730442047119 -0.310302734375
3.76774930953979 -0.310546875
3.76871204376221 -0.3106689453125
3.76967263221741 -0.3109130859375
3.77004146575928 -0.31103515625
3.77349376678467 -0.311767578125
3.77371335029602 -0.3118896484375
3.77407884597778 -0.3121337890625
3.77553772926331 -0.3121337890625
3.77699160575867 -0.3123779296875
3.77728176116943 -0.3125
3.7775719165802 -0.3126220703125
3.77887439727783 -0.3126220703125
3.7791633605957 -0.312744140625
3.78304553031921 -0.3138427734375
3.78326034545898 -0.31396484375
3.7834746837616 -0.31396484375
3.78354620933533 -0.31396484375
3.7845458984375 -0.314208984375
3.78511619567871 -0.314208984375
3.78518748283386 -0.3143310546875
3.78547215461731 -0.3143310546875
3.78575682640076 -0.3143310546875
3.78575682640076 -0.3143310546875
3.78646755218506 -0.314453125
3.78660941123962 -0.314453125
3.78660941123962 -0.314453125
3.78682231903076 -0.314453125
3.78724789619446 -0.314453125
3.787672996521 -0.3145751953125
3.78859257698059 -0.314697265625
3.79063701629639 -0.31494140625
3.79091811180115 -0.3150634765625
3.79126954078674 -0.315185546875
3.79204130172729 -0.315185546875
3.79232168197632 -0.315185546875
3.79406952857971 -0.3153076171875
3.79469704627991 -0.3153076171875
3.79483652114868 -0.3153076171875
3.79664373397827 -0.3154296875
3.79685163497925 -0.3154296875
3.79775214195251 -0.3154296875
3.79789042472839 -0.3155517578125
3.79802870750427 -0.3155517578125
3.79844355583191 -0.3155517578125
3.79858160018921 -0.315673828125
3.79934048652649 -0.315673828125
3.80016708374023 -0.31591796875
3.80092310905457 -0.31591796875
3.80099177360535 -0.31591796875
3.80119776725769 -0.31591796875
3.80147218704224 -0.31591796875
3.80263686180115 -0.3160400390625
3.80270528793335 -0.3160400390625
3.80338883399963 -0.3160400390625
3.80338883399963 -0.3160400390625
3.80359363555908 -0.3160400390625
3.80509281158447 -0.3160400390625
3.80529689788818 -0.316162109375
3.80543279647827 -0.316162109375
3.80590844154358 -0.316162109375
3.80611205101013 -0.316162109375
3.80651903152466 -0.316162109375
3.80672240257263 -0.3162841796875
3.80719661712646 -0.3162841796875
3.8084135055542 -0.3162841796875
3.80848097801208 -0.3162841796875
3.80868339538574 -0.3162841796875
3.80949234962463 -0.31640625
3.80969429016113 -0.31640625
3.81003069877625 -0.31640625
3.81009793281555 -0.31640625
3.81070280075073 -0.3165283203125
3.81090426445007 -0.3165283203125
3.81090426445007 -0.3165283203125
3.81217765808105 -0.3165283203125
3.81224465370178 -0.316650390625
3.81504607200623 -0.3167724609375
3.81524562835693 -0.31689453125
3.81524562835693 -0.31689453125
3.81557774543762 -0.31689453125
3.81590962409973 -0.3170166015625
3.81617498397827 -0.3170166015625
3.81624126434326 -0.3170166015625
3.81993865966797 -0.3173828125
3.82026720046997 -0.3175048828125
3.82052993774414 -0.3175048828125
3.82072687149048 -0.3175048828125
3.82085800170898 -0.3175048828125
3.82118582725525 -0.3175048828125
3.82138252258301 -0.3175048828125
3.82184100151062 -0.317626953125
3.82210254669189 -0.317626953125
3.82242965698242 -0.317626953125
3.82295227050781 -0.3177490234375
3.82314801216125 -0.3177490234375
3.82477641105652 -0.3177490234375
3.82490634918213 -0.31787109375
3.82510137557983 -0.31787109375
3.82510137557983 -0.31787109375
3.8256208896637 -0.31787109375
3.82581543922424 -0.31787109375
3.82581543922424 -0.31787109375
3.82613968849182 -0.31787109375
3.82846665382385 -0.318359375
3.83078098297119 -0.3184814453125
3.83084511756897 -0.3184814453125
3.8310375213623 -0.3184814453125
3.83122968673706 -0.3184814453125
3.83154988288879 -0.318603515625
3.83186984062195 -0.318603515625
3.83218955993652 -0.318603515625
3.83218955993652 -0.318603515625
3.83276438713074 -0.3187255859375
3.83372068405151 -0.3187255859375
3.83372068405151 -0.3187255859375
3.83391165733337 -0.3187255859375
3.83410263061523 -0.3187255859375
3.83410263061523 -0.3187255859375
3.83435702323914 -0.3187255859375
3.83562707901001 -0.31884765625
3.83562707901001 -0.31884765625
3.83562707901001 -0.3189697265625
3.83657717704773 -0.3189697265625
3.8368935585022 -0.3189697265625
3.83796691894531 -0.319091796875
3.83809304237366 -0.319091796875
3.83834528923035 -0.319091796875
3.83840823173523 -0.319091796875
3.83840823173523 -0.319091796875
3.83922648429871 -0.319091796875
3.83922648429871 -0.319091796875
3.84054517745972 -0.3192138671875
3.84067058563232 -0.3193359375
3.84067058563232 -0.3193359375
3.84248447418213 -0.3193359375
3.84248447418213 -0.3193359375
3.84267163276672 -0.3193359375
3.84323287010193 -0.3193359375
3.84410429000854 -0.3194580078125
3.84416651725769 -0.3194580078125
3.84516000747681 -0.3194580078125
3.8457179069519 -0.319580078125
3.84608960151672 -0.319580078125
3.84608960151672 -0.319580078125
3.84658455848694 -0.319580078125
3.84658455848694 -0.319580078125
3.84701704978943 -0.319580078125
3.84763431549072 -0.3197021484375
3.8485586643219 -0.3197021484375
3.84874320030212 -0.3197021484375
3.84874320030212 -0.3197021484375
3.84984922409058 -0.31982421875
3.84984922409058 -0.31982421875
3.85009455680847 -0.31982421875
3.85076880455017 -0.31982421875
3.85290670394897 -0.3199462890625
3.85290670394897 -0.3199462890625
3.85503435134888 -0.3203125
3.8554584980011 -0.3204345703125
3.85606384277344 -0.3204345703125
3.85648727416992 -0.3204345703125
3.85672879219055 -0.3204345703125
3.8571515083313 -0.3204345703125
3.85883784294128 -0.321044921875
3.8596785068512 -0.3211669921875
3.8602180480957 -0.3212890625
3.86183309555054 -0.321533203125
3.86266803741455 -0.321533203125
3.8628466129303 -0.3216552734375
3.86557769775391 -0.3223876953125
3.86581444740295 -0.32275390625
3.86758542060852 -0.322998046875
3.86882066726685 -0.3231201171875
3.86929035186768 -0.3232421875
3.86970090866089 -0.3232421875
3.87057948112488 -0.3233642578125
3.87087202072144 -0.323486328125
3.87209796905518 -0.32373046875
3.87238931655884 -0.32373046875
3.8726806640625 -0.3238525390625
3.87343692779541 -0.3238525390625
3.87436580657959 -0.3240966796875
3.87453985214233 -0.3243408203125
3.87604451179504 -0.3243408203125
3.87673735618591 -0.324462890625
3.87691020965576 -0.324462890625
3.87714099884033 -0.3245849609375
3.87800455093384 -0.32470703125
3.87823438644409 -0.32470703125
3.87846422195435 -0.3248291015625
3.87915325164795 -0.3248291015625
3.88166999816895 -0.325439453125
3.88195490837097 -0.3255615234375
3.88195490837097 -0.32568359375
3.88201189041138 -0.32568359375
3.88246750831604 -0.3258056640625
3.88303661346436 -0.3258056640625
3.88320708274841 -0.325927734375
3.88337755203247 -0.325927734375
3.88366150856018 -0.325927734375
3.88371825218201 -0.325927734375
3.88400197029114 -0.325927734375
3.88490867614746 -0.325927734375
3.88541769981384 -0.3260498046875
3.88558745384216 -0.3260498046875
3.88581323623657 -0.3260498046875
3.88598275184631 -0.3260498046875
3.88609576225281 -0.326171875
3.88637781143188 -0.326171875
3.88801097869873 -0.3262939453125
3.88817954063416 -0.3262939453125
3.88840413093567 -0.3262939453125
3.88857269287109 -0.3262939453125
3.88857269287109 -0.3262939453125
3.88874101638794 -0.3262939453125
3.88879704475403 -0.3262939453125
3.88879704475403 -0.3262939453125
3.88879704475403 -0.3262939453125
3.88896536827087 -0.326416015625
3.88913345336914 -0.326416015625
3.88935780525208 -0.326416015625
3.88941383361816 -0.326416015625
3.89092373847961 -0.3265380859375
3.89120292663574 -0.32666015625
3.89125871658325 -0.32666015625
3.89265108108521 -0.32666015625
3.892817735672 -0.32666015625
3.892817735672 -0.32666015625
3.8930401802063 -0.3267822265625
3.89315128326416 -0.3267822265625
3.8935399055481 -0.3267822265625
3.89359521865845 -0.3267822265625
3.89359521865845 -0.3267822265625
3.89376163482666 -0.3267822265625
3.89376163482666 -0.3267822265625
3.89392805099487 -0.3267822265625
3.89392805099487 -0.3267822265625
3.89409446716309 -0.3267822265625
3.89431595802307 -0.326904296875
3.89481425285339 -0.326904296875
3.89481425285339 -0.326904296875
3.89481425285339 -0.326904296875
3.8950355052948 -0.326904296875
3.8950355052948 -0.326904296875
3.8950355052948 -0.326904296875
3.89685678482056 -0.3271484375
3.89718699455261 -0.3271484375
3.89729714393616 -0.3271484375
3.89729714393616 -0.3271484375
3.89740705490112 -0.3271484375
3.89757204055786 -0.3271484375
3.89762711524963 -0.3271484375
3.89762711524963 -0.3271484375
3.89834117889404 -0.3271484375
3.89856052398682 -0.3271484375
3.89856052398682 -0.3271484375
3.89861559867859 -0.3271484375
3.89861559867859 -0.3271484375
3.89861559867859 -0.3271484375
3.89861559867859 -0.3271484375
3.89878010749817 -0.3271484375
3.89878010749817 -0.3271484375
3.90014863014221 -0.3272705078125
3.90014863014221 -0.3272705078125
3.90014863014221 -0.3272705078125
3.90113115310669 -0.3272705078125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90140390396118 -0.327392578125
3.90140390396118 -0.327392578125
3.90140390396118 -0.327392578125
3.90140390396118 -0.327392578125
3.90156722068787 -0.327392578125
3.90156722068787 -0.327392578125
3.90162181854248 -0.327392578125
3.90183973312378 -0.327392578125
3.90189409255981 -0.327392578125
3.90194845199585 -0.327392578125
3.90276408195496 -0.327392578125
3.90281844139099 -0.327392578125
3.90363264083862 -0.3275146484375
3.90384936332703 -0.3275146484375
3.90401196479797 -0.3275146484375
3.90417432785034 -0.3275146484375
3.90417432785034 -0.3275146484375
3.9042284488678 -0.3275146484375
3.90428256988525 -0.3275146484375
3.90428256988525 -0.3275146484375
3.90449905395508 -0.3275146484375
3.90455317497253 -0.3275146484375
3.9047155380249 -0.3275146484375
3.90476965904236 -0.3275146484375
3.90476965904236 -0.3275146484375
3.90476965904236 -0.3275146484375
3.90574193000793 -0.32763671875
3.90574193000793 -0.32763671875
3.90590381622314 -0.32763671875
3.90595769882202 -0.32763671875
3.90649676322937 -0.32763671875
3.90725016593933 -0.32763671875
3.90735769271851 -0.32763671875
3.9074113368988 -0.32763671875
3.90762639045715 -0.32763671875
3.90768003463745 -0.32763671875
3.90773367881775 -0.3277587890625
3.90773367881775 -0.3277587890625
3.90773367881775 -0.3277587890625
3.90789484977722 -0.3277587890625
3.90794849395752 -0.3277587890625
3.90794849395752 -0.3277587890625
3.90810966491699 -0.3277587890625
3.90810966491699 -0.3277587890625
3.90816330909729 -0.3277587890625
3.90821695327759 -0.3277587890625
3.90821695327759 -0.3277587890625
3.90821695327759 -0.3277587890625
3.91025066375732 -0.3280029296875
3.91030406951904 -0.3280029296875
3.9104642868042 -0.3280029296875
3.91163682937622 -0.3280029296875
3.91184973716736 -0.3280029296875
3.9119029045105 -0.3280029296875
3.9120626449585 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.328125
3.91264700889587 -0.328125
3.91291260719299 -0.328125
3.91291260719299 -0.328125
3.91296553611755 -0.328125
3.91296553611755 -0.328125
3.91301870346069 -0.328125
3.91301870346069 -0.328125
3.91301870346069 -0.328125
3.91413140296936 -0.328125
3.91429018974304 -0.3282470703125
3.9143431186676 -0.3282470703125
3.9143431186676 -0.3282470703125
3.9143431186676 -0.3282470703125
3.91450190544128 -0.3282470703125
3.91450190544128 -0.3282470703125
3.91455459594727 -0.3282470703125
3.91460752487183 -0.3282470703125
3.91460752487183 -0.3282470703125
3.91466045379639 -0.3282470703125
3.91471338272095 -0.3282470703125
3.91476607322693 -0.3282470703125
3.91492462158203 -0.3282470703125
3.91613793373108 -0.3282470703125
3.9168221950531 -0.328369140625
3.91698002815247 -0.328369140625
3.91703271865845 -0.328369140625
3.91734790802002 -0.328369140625
3.9174530506134 -0.328369140625
3.91865921020508 -0.328369140625
3.91876411437988 -0.328369140625
3.91876411437988 -0.328369140625
3.91876411437988 -0.328369140625
3.91876411437988 -0.328369140625
3.91923499107361 -0.328369140625
3.91923499107361 -0.328369140625
3.91923499107361 -0.328369140625
3.91939187049866 -0.328369140625
3.91944432258606 -0.328369140625
3.91949653625488 -0.328369140625
3.91970562934875 -0.328369140625
3.91970562934875 -0.328369140625
3.91970562934875 -0.328369140625
3.92007112503052 -0.328369140625
3.92007112503052 -0.3284912109375
3.92007112503052 -0.3284912109375
3.92007112503052 -0.3284912109375
3.92022776603699 -0.3284912109375
3.92033195495605 -0.3284912109375
3.92059278488159 -0.3284912109375
3.92064499855042 -0.3284912109375
3.92064499855042 -0.3284912109375
3.92132234573364 -0.3284912109375
3.92132234573364 -0.3284912109375
3.92132234573364 -0.3284912109375
3.92142629623413 -0.3284912109375
3.92147827148438 -0.3284912109375
3.9215304851532 -0.3284912109375
3.9215304851532 -0.3284912109375
3.9215304851532 -0.3284912109375
3.9215304851532 -0.3284912109375
3.92215442657471 -0.3284912109375
3.92231011390686 -0.32861328125
3.92365837097168 -0.32861328125
3.92371010780334 -0.32861328125
3.92376184463501 -0.32861328125
3.92376184463501 -0.32861328125
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{S3}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI}, 
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$},
extra x ticks={5.5},
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.5347697019577,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.307040405273438, ymax=0.0146209716796875,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c16)}
]
\addplot [ultra thick, brown,dashed]
table {%
1.04139268398285 0
1.38021123409271 -0.0001220703125
1.6020599603653 -0.0001220703125
1.69896996021271 -0.0001220703125
1.77085208892822 -0.0001220703125
1.83250892162323 -0.0001220703125
2.98045778274536 -0.0013427734375
3.01661562919617 -0.0023193359375
3.0468852519989 -0.00244140625
3.08919835090637 -0.0025634765625
3.12123155593872 -0.002685546875
3.17318630218506 -0.0028076171875
3.29380440711975 -0.0030517578125
3.32715439796448 -0.003173828125
3.41463923454285 -0.0035400390625
3.45086479187012 -0.00390625
3.48685526847839 -0.00439453125
3.49554443359375 -0.0045166015625
3.54082989692688 -0.005859375
3.57391548156738 -0.006591796875
3.59703660011292 -0.0069580078125
3.63688898086548 -0.0086669921875
3.67942786216736 -0.0113525390625
3.70156788825989 -0.012451171875
3.73623704910278 -0.012939453125
3.74554324150085 -0.0133056640625
3.7680459022522 -0.0142822265625
3.78368926048279 -0.0147705078125
3.80229473114014 -0.015869140625
3.84441494941711 -0.0179443359375
3.8728551864624 -0.018798828125
3.9104642868042 -0.02294921875
3.94581317901611 -0.02685546875
3.99158048629761 -0.03076171875
4.01224660873413 -0.035400390625
4.03885841369629 -0.0389404296875
4.04960584640503 -0.0426025390625
4.07976007461548 -0.048828125
4.10250234603882 -0.0546875
4.11915683746338 -0.0587158203125
4.13735389709473 -0.06298828125
4.15048027038574 -0.0662841796875
4.16423368453979 -0.069091796875
4.17713212966919 -0.072509765625
4.18859100341797 -0.0758056640625
4.20357656478882 -0.07763671875
4.21569061279297 -0.0809326171875
4.22476625442505 -0.0828857421875
4.24256610870361 -0.088134765625
4.24983406066895 -0.0909423828125
4.26266479492188 -0.0950927734375
4.28053283691406 -0.099609375
4.29170179367065 -0.1082763671875
4.29769468307495 -0.1112060546875
4.31291770935059 -0.1156005859375
4.3254337310791 -0.121337890625
4.32986545562744 -0.123291015625
4.34020614624023 -0.1270751953125
4.35106134414673 -0.1282958984375
4.35900020599365 -0.1297607421875
4.37147426605225 -0.1319580078125
4.37741565704346 -0.133056640625
4.38767433166504 -0.137939453125
4.39371538162231 -0.13916015625
4.40308618545532 -0.14111328125
4.41092920303345 -0.1439208984375
4.41534090042114 -0.1448974609375
4.42322969436646 -0.1478271484375
4.42618560791016 -0.1495361328125
4.43480825424194 -0.1507568359375
4.43843173980713 -0.1514892578125
4.45417404174805 -0.1605224609375
4.45815420150757 -0.16357421875
4.4638032913208 -0.164306640625
4.47139453887939 -0.166015625
4.47373485565186 -0.1663818359375
4.48251628875732 -0.170654296875
4.48484039306641 -0.17138671875
4.48873376846313 -0.1719970703125
4.49483633041382 -0.1728515625
4.50004434585571 -0.173583984375
4.50699186325073 -0.1741943359375
4.51000833511353 -0.1748046875
4.51586055755615 -0.175537109375
4.52142572402954 -0.1766357421875
4.52478551864624 -0.1771240234375
4.52976369857788 -0.1781005859375
4.53219366073608 -0.1783447265625
4.54352188110352 -0.1868896484375
4.54651784896851 -0.1883544921875
4.55159616470337 -0.189208984375
4.5585765838623 -0.1923828125
4.56278038024902 -0.193359375
4.56750869750977 -0.1953125
4.57016897201538 -0.196044921875
4.576744556427 -0.1981201171875
4.57930326461792 -0.19873046875
4.58887672424316 -0.203369140625
4.59104251861572 -0.2059326171875
4.59404993057251 -0.20654296875
4.59698152542114 -0.20703125
4.60103797912598 -0.2073974609375
4.60622024536133 -0.2109375
4.60954093933105 -0.21142578125
4.61214780807495 -0.2119140625
4.61687421798706 -0.21240234375
4.61933326721191 -0.213134765625
4.62079191207886 -0.2135009765625
4.62433385848999 -0.2142333984375
4.62600135803223 -0.21435546875
4.63069200515747 -0.2164306640625
4.63280153274536 -0.2171630859375
4.63742971420288 -0.2176513671875
4.64454698562622 -0.21923828125
4.64627647399902 -0.219482421875
4.64964628219604 -0.22021484375
4.65222692489624 -0.2205810546875
4.65470600128174 -0.220947265625
4.65936470031738 -0.2215576171875
4.66172742843628 -0.2220458984375
4.66347455978394 -0.222412109375
4.66435050964355 -0.22265625
4.66748094558716 -0.22314453125
4.67777109146118 -0.2294921875
4.67943716049194 -0.2318115234375
4.68320941925049 -0.232177734375
4.68504285812378 -0.2325439453125
4.69078063964844 -0.2335205078125
4.69279384613037 -0.2337646484375
4.70421075820923 -0.237548828125
4.70605182647705 -0.2392578125
4.7106671333313 -0.239990234375
4.71428775787354 -0.240234375
4.71669578552246 -0.240478515625
4.7204737663269 -0.2408447265625
4.72294616699219 -0.2412109375
4.727614402771 -0.24169921875
4.72904300689697 -0.241943359375
4.73232126235962 -0.242919921875
4.73387908935547 -0.2431640625
4.73834466934204 -0.24365234375
4.73901033401489 -0.243896484375
4.74219846725464 -0.244384765625
4.74394845962524 -0.2447509765625
4.74711656570435 -0.2449951171875
4.75675010681152 -0.2493896484375
4.75741863250732 -0.25
4.76039218902588 -0.2508544921875
4.76314353942871 -0.251220703125
4.76366758346558 -0.2513427734375
4.76559400558472 -0.25146484375
4.77042484283447 -0.251708984375
4.77234363555908 -0.251953125
4.77474308013916 -0.252197265625
4.77776002883911 -0.25244140625
4.77859973907471 -0.2528076171875
4.78022384643555 -0.2529296875
4.78272342681885 -0.2530517578125
4.7888822555542 -0.254150390625
4.79206943511963 -0.254638671875
4.79488515853882 -0.2550048828125
4.7973575592041 -0.2554931640625
4.80133533477783 -0.2559814453125
4.80271911621094 -0.25634765625
4.80465745925903 -0.256591796875
4.80635643005371 -0.2567138671875
4.81078338623047 -0.2589111328125
4.81482028961182 -0.260009765625
4.81666564941406 -0.26025390625
4.81906318664551 -0.260498046875
4.82443189620972 -0.2613525390625
4.82586717605591 -0.2623291015625
4.83021640777588 -0.263916015625
4.833580493927 -0.26416015625
4.83537340164185 -0.2645263671875
4.84338855743408 -0.2664794921875
4.84484958648682 -0.2669677734375
4.84764671325684 -0.267333984375
4.84937047958374 -0.2674560546875
4.85565853118896 -0.2691650390625
4.85735654830933 -0.2694091796875
4.85934829711914 -0.2696533203125
4.86033201217651 -0.2696533203125
4.86609220504761 -0.275390625
4.86751461029053 -0.277099609375
4.87045669555664 -0.277587890625
4.87329149246216 -0.2779541015625
4.87547206878662 -0.2784423828125
4.87826299667358 -0.2791748046875
4.88145875930786 -0.27978515625
4.88332653045654 -0.280029296875
4.88507270812988 -0.2803955078125
4.88745403289795 -0.281005859375
4.89335107803345 -0.282470703125
4.89679050445557 -0.283447265625
4.89824247360229 -0.28369140625
4.90036725997925 -0.283935546875
4.9071478843689 -0.2860107421875
4.90859746932983 -0.286376953125
4.9113335609436 -0.2869873046875
4.91490364074707 -0.2872314453125
4.91547393798828 -0.287353515625
4.91632223129272 -0.2874755859375
4.91838693618774 -0.287841796875
4.92038440704346 -0.2879638671875
4.9238600730896 -0.288330078125
4.92431545257568 -0.2886962890625
4.92585849761963 -0.288818359375
4.92926073074341 -0.289794921875
4.9298529624939 -0.2900390625
4.93383646011353 -0.2919921875
4.93528032302856 -0.292236328125
4.9360408782959 -0.2923583984375
4.93991851806641 -0.296142578125
4.94125318527222 -0.2969970703125
4.94373178482056 -0.2978515625
4.94516801834106 -0.298095703125
4.94841766357422 -0.2984619140625
4.95028686523438 -0.298828125
4.95218706130981 -0.2989501953125
4.95365333557129 -0.2991943359375
4.95516300201416 -0.299560546875
4.95686435699463 -0.2996826171875
4.95752096176147 -0.2998046875
4.96054220199585 -0.3004150390625
4.96520185470581 -0.30126953125
4.96604299545288 -0.302001953125
4.96792697906494 -0.30224609375
4.97034692764282 -0.3026123046875
4.97193908691406 -0.3028564453125
4.97357130050659 -0.302978515625
4.97813034057617 -0.308349609375
4.9806079864502 -0.31005859375
4.98158311843872 -0.3101806640625
4.98294496536255 -0.3109130859375
4.98666858673096 -0.3125
4.9882869720459 -0.3128662109375
4.98916959762573 -0.31298828125
4.99014329910278 -0.313232421875
4.99300384521484 -0.3138427734375
4.99349784851074 -0.3140869140625
4.99566173553467 -0.3148193359375
4.99652481079102 -0.31494140625
4.99735164642334 -0.3150634765625
4.99801969528198 -0.315185546875
4.99916076660156 -0.315185546875
4.99979162216187 -0.3153076171875
5.00211429595947 -0.316650390625
5.00303792953491 -0.3170166015625
5.00380086898804 -0.317138671875
5.00529193878174 -0.3173828125
5.00589227676392 -0.3173828125
5.00632047653198 -0.3173828125
5.00743198394775 -0.3175048828125
5.00839567184448 -0.317626953125
5.01049518585205 -0.31787109375
5.01089763641357 -0.31787109375
5.01418018341064 -0.318359375
5.01442813873291 -0.3184814453125
5.01492357254028 -0.3184814453125
5.01548528671265 -0.3184814453125
5.01606750488281 -0.3184814453125
5.01948165893555 -0.31982421875
5.02066802978516 -0.3204345703125
5.02198266983032 -0.320556640625
5.02251100540161 -0.320556640625
5.02346229553223 -0.320556640625
5.02392292022705 -0.3206787109375
5.02508878707886 -0.3206787109375
5.02599763870239 -0.32080078125
5.02641487121582 -0.32080078125
5.02719879150391 -0.32080078125
5.027512550354 -0.32080078125
5.02823352813721 -0.3209228515625
5.02944850921631 -0.3209228515625
5.03028774261475 -0.321044921875
5.0306077003479 -0.321044921875
5.0313720703125 -0.3211669921875
5.03191328048706 -0.3211669921875
5.03247356414795 -0.3211669921875
5.0332145690918 -0.3212890625
5.03372526168823 -0.3212890625
5.03604984283447 -0.321533203125
5.03676843643188 -0.3216552734375
5.03806734085083 -0.3216552734375
5.03821468353271 -0.3216552734375
5.04104518890381 -0.3226318359375
5.04221296310425 -0.3228759765625
5.04305171966553 -0.322998046875
5.04417514801025 -0.322998046875
5.0451192855835 -0.3231201171875
5.04621410369873 -0.3231201171875
5.0475902557373 -0.3231201171875
5.04787063598633 -0.3231201171875
5.04892301559448 -0.3231201171875
5.05090141296387 -0.3233642578125
5.05159616470337 -0.3233642578125
5.0532398223877 -0.32373046875
5.05387306213379 -0.3238525390625
5.05473947525024 -0.323974609375
5.05561923980713 -0.323974609375
5.05629110336304 -0.323974609375
5.05667638778687 -0.323974609375
5.05724382400513 -0.323974609375
5.05853986740112 -0.32421875
5.05926418304443 -0.32421875
5.06055450439453 -0.3243408203125
5.06169748306274 -0.3243408203125
5.06202125549316 -0.324462890625
5.06284141540527 -0.324462890625
5.06341981887817 -0.324462890625
5.06388854980469 -0.324462890625
5.06565809249878 -0.3248291015625
5.06628847122192 -0.3248291015625
5.0677809715271 -0.3248291015625
5.06880521774292 -0.324951171875
5.06937599182129 -0.324951171875
5.0698823928833 -0.324951171875
5.07039976119995 -0.3250732421875
5.07118606567383 -0.3250732421875
5.07183790206909 -0.3250732421875
5.07231998443604 -0.3250732421875
5.07341051101685 -0.3251953125
5.07386493682861 -0.3253173828125
5.07522201538086 -0.3253173828125
5.07553577423096 -0.3253173828125
5.07706594467163 -0.3255615234375
5.07770586013794 -0.32568359375
5.07807588577271 -0.32568359375
5.07836961746216 -0.32568359375
5.07924270629883 -0.32568359375
5.07981061935425 -0.32568359375
5.08042812347412 -0.32568359375
5.08251953125 -0.325927734375
5.08288240432739 -0.3260498046875
5.08353137969971 -0.3260498046875
5.0838680267334 -0.3260498046875
5.0840539932251 -0.3260498046875
5.08464050292969 -0.3260498046875
5.08560800552368 -0.3260498046875
5.08617115020752 -0.3260498046875
5.08666944503784 -0.3260498046875
5.08734464645386 -0.326171875
5.08801889419556 -0.326171875
5.08810758590698 -0.326171875
5.08868885040283 -0.326171875
5.08945989608765 -0.326171875
5.08959436416626 -0.326171875
5.09040975570679 -0.326171875
5.09132242202759 -0.3262939453125
5.09161424636841 -0.3262939453125
5.09203243255615 -0.3262939453125
5.09283304214478 -0.3262939453125
5.0940375328064 -0.326416015625
5.09448862075806 -0.326416015625
5.09476804733276 -0.326416015625
5.09681272506714 -0.3267822265625
5.09702444076538 -0.326904296875
5.0971531867981 -0.326904296875
5.09734392166138 -0.326904296875
5.09848117828369 -0.3270263671875
5.09899663925171 -0.3270263671875
5.09967374801636 -0.3271484375
5.09975337982178 -0.3271484375
5.10060119628906 -0.3271484375
5.10100078582764 -0.3271484375
5.10145854949951 -0.3271484375
5.10340356826782 -0.3272705078125
5.10398149490356 -0.3272705078125
5.10440874099731 -0.3272705078125
5.1049919128418 -0.3272705078125
5.10564994812012 -0.3272705078125
5.1057825088501 -0.3272705078125
5.10673475265503 -0.327392578125
5.10739660263062 -0.327392578125
5.10774564743042 -0.327392578125
5.10849046707153 -0.327392578125
5.10858869552612 -0.327392578125
5.10864639282227 -0.327392578125
5.10883903503418 -0.327392578125
5.10983467102051 -0.3275146484375
5.11077833175659 -0.3275146484375
5.11113119125366 -0.32763671875
5.11155843734741 -0.32763671875
5.11193084716797 -0.32763671875
5.1123571395874 -0.32763671875
5.11242723464966 -0.32763671875
5.11260509490967 -0.32763671875
5.11286640167236 -0.32763671875
5.11481428146362 -0.3277587890625
5.11493110656738 -0.3277587890625
5.11503458023071 -0.3277587890625
5.1151442527771 -0.3277587890625
5.11542415618896 -0.3277587890625
5.11650466918945 -0.327880859375
5.11776494979858 -0.327880859375
5.11828470230103 -0.327880859375
5.11843013763428 -0.327880859375
5.11867475509644 -0.327880859375
5.11882019042969 -0.327880859375
5.11892890930176 -0.327880859375
5.11906433105469 -0.327880859375
5.11970138549805 -0.327880859375
5.11973428726196 -0.327880859375
5.12031745910645 -0.327880859375
5.12060689926147 -0.327880859375
5.12064647674561 -0.327880859375
5.12083721160889 -0.327880859375
5.12097835540771 -0.3280029296875
5.12098503112793 -0.3280029296875
5.12112283706665 -0.3280029296875
5.12134647369385 -0.3280029296875
5.12181234359741 -0.3280029296875
5.12192058563232 -0.3280029296875
5.12225532531738 -0.3280029296875
5.12257957458496 -0.3280029296875
5.1229887008667 -0.3280029296875
5.12299537658691 -0.3280029296875
5.12338447570801 -0.3280029296875
5.12339115142822 -0.3280029296875
5.12349557876587 -0.3280029296875
5.12396907806396 -0.3280029296875
5.12410974502563 -0.3280029296875
5.1248140335083 -0.3280029296875
5.1248984336853 -0.328125
5.1252179145813 -0.328125
5.12543916702271 -0.328125
5.12566995620728 -0.328125
5.12647581100464 -0.328125
5.12706279754639 -0.328125
5.12706899642944 -0.328125
5.12756824493408 -0.328125
5.128005027771 -0.328125
5.12887382507324 -0.328125
5.12903881072998 -0.3282470703125
5.12932872772217 -0.3282470703125
5.12957048416138 -0.3282470703125
5.12964820861816 -0.3282470703125
5.13024044036865 -0.3282470703125
5.130784034729 -0.3282470703125
5.130934715271 -0.3282470703125
5.13143253326416 -0.3282470703125
5.13145160675049 -0.3282470703125
5.13163805007935 -0.3282470703125
5.13167953491211 -0.3282470703125
5.13269805908203 -0.328369140625
5.13351678848267 -0.328369140625
5.13384199142456 -0.328369140625
5.13400173187256 -0.328369140625
5.13420248031616 -0.328369140625
5.13453102111816 -0.328369140625
5.13493204116821 -0.328369140625
5.13510084152222 -0.328369140625
5.13575601577759 -0.328369140625
5.1358699798584 -0.328369140625
5.13611793518066 -0.328369140625
5.13644170761108 -0.328369140625
5.13647651672363 -0.328369140625
5.13684415817261 -0.328369140625
5.13705635070801 -0.328369140625
5.13760709762573 -0.328369140625
5.13770866394043 -0.328369140625
5.13823318481445 -0.3284912109375
5.13861846923828 -0.3284912109375
5.13862466812134 -0.3284912109375
5.14107322692871 -0.32861328125
5.14158153533936 -0.3287353515625
5.14161920547485 -0.3287353515625
5.14278650283813 -0.3287353515625
5.14336776733398 -0.328857421875
5.14355182647705 -0.328857421875
5.14380788803101 -0.328857421875
5.14424085617065 -0.328857421875
5.14432811737061 -0.328857421875
5.14488220214844 -0.328857421875
5.14495992660522 -0.328857421875
5.14515924453735 -0.328857421875
5.14554119110107 -0.328857421875
5.1457462310791 -0.328857421875
5.14615917205811 -0.328857421875
5.14659309387207 -0.328857421875
5.14689970016479 -0.328857421875
5.1469988822937 -0.328857421875
5.1470513343811 -0.328857421875
5.14751577377319 -0.3289794921875
5.14785575866699 -0.3289794921875
5.14795112609863 -0.3289794921875
5.14831876754761 -0.3289794921875
5.14847326278687 -0.3289794921875
5.14865827560425 -0.3289794921875
5.14873218536377 -0.3289794921875
5.14907455444336 -0.3289794921875
5.1509313583374 -0.3289794921875
5.15100479125977 -0.3289794921875
5.15146493911743 -0.3289794921875
5.15155696868896 -0.3289794921875
5.15180158615112 -0.3289794921875
5.15191221237183 -0.3289794921875
5.15233421325684 -0.3291015625
5.15274095535278 -0.3291015625
5.15321731567383 -0.3291015625
5.15346717834473 -0.3291015625
5.15381479263306 -0.3291015625
5.15424728393555 -0.3291015625
5.15459728240967 -0.3291015625
5.15502023696899 -0.3291015625
5.15542411804199 -0.3291015625
5.15564250946045 -0.3291015625
5.15672159194946 -0.3292236328125
5.15712404251099 -0.3292236328125
5.15771055221558 -0.3292236328125
5.15812110900879 -0.329345703125
5.15853118896484 -0.329345703125
5.15888977050781 -0.329345703125
5.1592059135437 -0.329345703125
5.15956735610962 -0.329345703125
5.15989208221436 -0.329345703125
5.16030931472778 -0.329345703125
5.16073560714722 -0.329345703125
5.16106557846069 -0.329345703125
5.16126012802124 -0.329345703125
5.16168546676636 -0.329345703125
5.16241502761841 -0.3294677734375
5.16267204284668 -0.3294677734375
5.16306304931641 -0.3294677734375
5.16335821151733 -0.3294677734375
5.16376638412476 -0.3294677734375
5.16410303115845 -0.3294677734375
5.16470050811768 -0.3297119140625
5.16506624221802 -0.329833984375
5.1654372215271 -0.329833984375
5.16578435897827 -0.3299560546875
5.16607761383057 -0.3299560546875
5.16632652282715 -0.3299560546875
5.1666374206543 -0.3299560546875
5.16685628890991 -0.3299560546875
5.16724920272827 -0.3299560546875
5.16773653030396 -0.330078125
5.16799354553223 -0.330078125
5.16839742660522 -0.330078125
5.16868591308594 -0.3302001953125
5.1689305305481 -0.3302001953125
5.16942739486694 -0.330322265625
5.16967153549194 -0.330322265625
5.17017650604248 -0.330322265625
5.17068386077881 -0.330322265625
5.17087173461914 -0.330322265625
5.17144584655762 -0.3304443359375
5.17189884185791 -0.3304443359375
5.17215299606323 -0.3304443359375
5.1722936630249 -0.3304443359375
5.17255020141602 -0.33056640625
5.17296171188354 -0.33056640625
5.17313385009766 -0.33056640625
5.17357683181763 -0.33056640625
5.17400741577148 -0.33056640625
5.17434787750244 -0.33056640625
5.17449569702148 -0.33056640625
5.17502450942993 -0.3306884765625
5.17525386810303 -0.3306884765625
5.17556381225586 -0.3306884765625
5.1758508682251 -0.3306884765625
5.17632579803467 -0.3306884765625
5.17648506164551 -0.3306884765625
5.17664098739624 -0.3306884765625
5.17669868469238 -0.3306884765625
5.17734909057617 -0.330810546875
5.17746734619141 -0.330810546875
5.17807006835938 -0.330810546875
5.1782169342041 -0.330810546875
5.17872667312622 -0.330810546875
5.17891931533813 -0.330810546875
5.17955732345581 -0.330810546875
5.17977571487427 -0.330810546875
5.17994213104248 -0.330810546875
5.18006277084351 -0.330810546875
5.18051290512085 -0.330810546875
5.18083095550537 -0.330810546875
5.18096542358398 -0.330810546875
5.18113422393799 -0.330810546875
5.18134021759033 -0.330810546875
5.18143177032471 -0.330810546875
5.18184089660645 -0.330810546875
5.18192338943481 -0.330810546875
5.18209505081177 -0.330810546875
5.18231201171875 -0.330810546875
5.18238306045532 -0.330810546875
5.18263721466064 -0.330810546875
5.1827597618103 -0.3309326171875
5.18280267715454 -0.3309326171875
5.18345499038696 -0.3309326171875
5.18351459503174 -0.3309326171875
5.18406105041504 -0.3309326171875
5.18454074859619 -0.3309326171875
5.18462896347046 -0.3309326171875
5.18468284606934 -0.3309326171875
5.18490982055664 -0.3309326171875
5.18493843078613 -0.3309326171875
5.1851282119751 -0.3309326171875
5.1872386932373 -0.3311767578125
5.1883602142334 -0.331298828125
5.18851804733276 -0.331298828125
5.18865585327148 -0.331298828125
5.18890857696533 -0.331298828125
5.18909692764282 -0.331298828125
5.18913078308105 -0.331298828125
5.18926000595093 -0.331298828125
5.18929100036621 -0.331298828125
5.18983268737793 -0.331298828125
5.1900372505188 -0.331298828125
5.19040441513062 -0.331298828125
5.19048023223877 -0.331298828125
5.19049692153931 -0.331298828125
5.19083309173584 -0.3314208984375
5.1914005279541 -0.3314208984375
5.19163274765015 -0.3314208984375
5.19220781326294 -0.3314208984375
5.19240856170654 -0.3314208984375
5.19295215606689 -0.3314208984375
5.19301319122314 -0.3314208984375
5.19301891326904 -0.3314208984375
5.19316339492798 -0.3314208984375
5.19322204589844 -0.3314208984375
5.19344997406006 -0.3314208984375
5.19374513626099 -0.3314208984375
5.19375038146973 -0.3314208984375
5.19401168823242 -0.3314208984375
5.19404792785645 -0.3314208984375
5.19405364990234 -0.3314208984375
5.19436979293823 -0.3314208984375
5.19437551498413 -0.3314208984375
5.19438123703003 -0.3314208984375
5.19439506530762 -0.3314208984375
5.19440078735352 -0.3314208984375
5.19486951828003 -0.3314208984375
5.19511318206787 -0.3314208984375
5.19524335861206 -0.33154296875
5.19533777236938 -0.33154296875
5.19534349441528 -0.33154296875
5.19543170928955 -0.33154296875
5.19543743133545 -0.33154296875
5.19557046890259 -0.33154296875
5.19557571411133 -0.33154296875
5.19558143615723 -0.33154296875
5.19558715820312 -0.33154296875
5.19628381729126 -0.33154296875
5.19628953933716 -0.33154296875
5.19629526138306 -0.33154296875
5.196457862854 -0.33154296875
5.19654941558838 -0.33154296875
5.19655466079712 -0.33154296875
5.19656038284302 -0.33154296875
5.19656562805176 -0.33154296875
5.19674825668335 -0.33154296875
5.19675350189209 -0.33154296875
5.19675922393799 -0.33154296875
5.19676446914673 -0.33154296875
5.19677019119263 -0.33154296875
5.19677019119263 -0.33154296875
5.19787836074829 -0.33154296875
5.19812917709351 -0.33154296875
5.19813442230225 -0.33154296875
5.19814014434814 -0.33154296875
5.19814538955688 -0.33154296875
5.19816207885742 -0.33154296875
5.19816732406616 -0.33154296875
5.19817304611206 -0.33154296875
5.19817876815796 -0.33154296875
5.1982307434082 -0.33154296875
5.1988410949707 -0.33154296875
5.19884395599365 -0.33154296875
};
\addplot [ultra thick, blue]
table {%
0 0
0 -0.0001220703125
0 -0.0001220703125
0 -0.0001220703125
0 -0.0001220703125
0 -0.0001220703125
0.30103000998497 -0.0001220703125
0.30103000998497 -0.0001220703125
0.30103000998497 -0.000244140625
0.30103000998497 -0.000244140625
0.30103000998497 -0.000244140625
0.477121233940125 -0.000244140625
0.477121233940125 -0.0003662109375
0.477121233940125 -0.0003662109375
0.477121233940125 -0.0003662109375
0.698970019817352 -0.0003662109375
0.698970019817352 -0.0003662109375
0.698970019817352 -0.0003662109375
0.778151273727417 -0.00048828125
0.778151273727417 -0.00048828125
0.778151273727417 -0.00048828125
1 -0.001220703125
1.04139268398285 -0.00146484375
1.07918119430542 -0.0015869140625
1.17609131336212 -0.001708984375
1.20412003993988 -0.0018310546875
1.41497337818146 -0.0028076171875
1.50514996051788 -0.0040283203125
1.6334685087204 -0.00537109375
1.65321254730225 -0.0074462890625
1.66275787353516 -0.0079345703125
1.77085208892822 -0.00830078125
1.80618000030518 -0.0093994140625
1.88649070262909 -0.01220703125
1.92941892147064 -0.013671875
1.95424246788025 -0.014404296875
2.00432133674622 -0.0147705078125
2.07918119430542 -0.0172119140625
2.10720992088318 -0.0191650390625
2.17318630218506 -0.019775390625
2.21484375 -0.0230712890625
2.25527238845825 -0.0252685546875
2.26951289176941 -0.0272216796875
2.290034532547 -0.0291748046875
2.36735582351685 -0.033203125
2.40483379364014 -0.0372314453125
2.44090914726257 -0.03955078125
2.48572134971619 -0.0421142578125
2.49968719482422 -0.0439453125
2.53147888183594 -0.0462646484375
2.55145001411438 -0.049072265625
2.57054305076599 -0.0499267578125
2.58883166313171 -0.0516357421875
2.62428212165833 -0.0526123046875
2.6655809879303 -0.0611572265625
2.70415043830872 -0.065673828125
2.767897605896 -0.0762939453125
2.78031730651855 -0.087158203125
2.79934048652649 -0.090576171875
2.8188853263855 -0.094970703125
2.85064625740051 -0.1065673828125
2.86213135719299 -0.1107177734375
2.87390160560608 -0.1138916015625
2.89486956596375 -0.1187744140625
2.9143431186676 -0.12158203125
2.92168641090393 -0.1236572265625
2.94841289520264 -0.132568359375
2.95327639579773 -0.134033203125
2.96189546585083 -0.1351318359375
2.9642596244812 -0.1357421875
2.97954845428467 -0.13720703125
2.99299502372742 -0.1380615234375
3.00173377990723 -0.1396484375
3.00945091247559 -0.140869140625
3.02653336524963 -0.1424560546875
3.03981065750122 -0.1446533203125
3.04493165016174 -0.1455078125
3.06220579147339 -0.1463623046875
3.06744289398193 -0.1470947265625
3.07188200950623 -0.1475830078125
3.08206701278687 -0.14990234375
3.09447121620178 -0.1507568359375
3.10380363464355 -0.1527099609375
3.10822677612305 -0.1534423828125
3.11760258674622 -0.155029296875
3.14270234107971 -0.1566162109375
3.15442395210266 -0.158935546875
3.15896534919739 -0.16015625
3.16583752632141 -0.16064453125
3.17405986785889 -0.161376953125
3.17609119415283 -0.161865234375
3.18808436393738 -0.164794921875
3.20330500602722 -0.1666259765625
3.20601582527161 -0.1671142578125
3.21298623085022 -0.1678466796875
3.22479200363159 -0.17041015625
3.22762966156006 -0.171875
3.23172426223755 -0.17236328125
3.23502326011658 -0.1729736328125
3.24129748344421 -0.1739501953125
3.24551272392273 -0.174560546875
3.2550311088562 -0.1763916015625
3.25767850875854 -0.1776123046875
3.26363611221313 -0.1781005859375
3.26552534103394 -0.178466796875
3.27531147003174 -0.1844482421875
3.28035068511963 -0.185302734375
3.29358339309692 -0.19384765625
3.29710364341736 -0.1962890625
3.30124711990356 -0.1971435546875
3.30984306335449 -0.197998046875
3.31281185150146 -0.1986083984375
3.31993842124939 -0.20068359375
3.32221937179565 -0.2021484375
3.32919430732727 -0.205078125
3.33061671257019 -0.2060546875
3.33344721794128 -0.2066650390625
3.34419560432434 -0.2149658203125
3.35102295875549 -0.217041015625
3.35679054260254 -0.2186279296875
3.35831570625305 -0.219482421875
3.36002516746521 -0.2198486328125
3.36380004882812 -0.2205810546875
3.36567521095276 -0.2213134765625
3.36958694458008 -0.2218017578125
3.37199091911316 -0.22216796875
3.380211353302 -0.228515625
3.38560628890991 -0.23046875
3.38916611671448 -0.23095703125
3.39111161231995 -0.231201171875
3.39776635169983 -0.2313232421875
3.39950060844421 -0.231689453125
3.40277695655823 -0.232421875
3.40534639358521 -0.232666015625
3.40891790390015 -0.2335205078125
3.41027092933655 -0.233642578125
3.41430473327637 -0.2354736328125
3.41912937164307 -0.2364501953125
3.42504477500916 -0.236572265625
3.42975234985352 -0.237548828125
3.43232774734497 -0.23779296875
3.43296933174133 -0.2379150390625
3.43600344657898 -0.2381591796875
3.43838405609131 -0.23828125
3.43901681900024 -0.2384033203125
3.44200921058655 -0.23876953125
3.44653725624084 -0.2393798828125
3.44824242591858 -0.2396240234375
3.44886088371277 -0.23974609375
3.4598445892334 -0.2418212890625
3.46119832992554 -0.2421875
3.46239805221558 -0.2423095703125
3.46448945999146 -0.24267578125
3.46671938896179 -0.2430419921875
3.47348690032959 -0.2435302734375
3.47465324401855 -0.24365234375
3.47625184059143 -0.243896484375
3.48015069961548 -0.2440185546875
3.48129940032959 -0.244140625
3.48727989196777 -0.2447509765625
3.48798632621765 -0.2452392578125
3.48925518989563 -0.245361328125
3.493736743927 -0.24560546875
3.50569248199463 -0.2498779296875
3.50650501251221 -0.251708984375
3.51094698905945 -0.2523193359375
3.51201701164246 -0.25244140625
3.51693177223206 -0.2529296875
3.52153038978577 -0.2535400390625
3.52309584617615 -0.253662109375
3.52698516845703 -0.25390625
3.52814507484436 -0.2540283203125
3.53364491462708 -0.2548828125
3.541579246521 -0.25537109375
3.54257655143738 -0.255615234375
3.55022835731506 -0.25732421875
3.55096173286438 -0.2579345703125
3.55230307579041 -0.258056640625
3.5583484172821 -0.2587890625
3.56086277961731 -0.259033203125
3.56288743019104 -0.259521484375
3.56667327880859 -0.259765625
3.57252311706543 -0.2606201171875
3.57379961013794 -0.2608642578125
3.58035469055176 -0.2623291015625
3.58172225952148 -0.2630615234375
3.58376550674438 -0.263427734375
3.58444428443909 -0.2635498046875
3.59428215026855 -0.268798828125
3.59549617767334 -0.2703857421875
3.59802412986755 -0.270751953125
3.60346913337708 -0.27197265625
3.60691857337952 -0.27294921875
3.61012768745422 -0.2733154296875
3.6133131980896 -0.273681640625
3.61595010757446 -0.27392578125
3.61836194992065 -0.274169921875
3.62190294265747 -0.274658203125
3.62335276603699 -0.275146484375
3.62551832199097 -0.2755126953125
3.62981724739075 -0.275634765625
3.6326596736908 -0.2762451171875
3.63477945327759 -0.2764892578125
3.6403820514679 -0.2789306640625
3.64226651191711 -0.279541015625
3.64463543891907 -0.280029296875
3.6475784778595 -0.2803955078125
3.65417647361755 -0.2828369140625
3.65513849258423 -0.283447265625
3.65648150444031 -0.28369140625
3.66105508804321 -0.2845458984375
3.66417169570923 -0.2850341796875
3.66754627227783 -0.285888671875
3.66857218742371 -0.286376953125
3.67108035087585 -0.2864990234375
3.67329740524292 -0.286865234375
3.67513656616211 -0.2874755859375
3.67760705947876 -0.28759765625
3.68106031417847 -0.2880859375
3.68358731269836 -0.288330078125
3.68547296524048 -0.2890625
3.68788552284241 -0.2891845703125
3.69019603729248 -0.2894287109375
3.69108152389526 -0.28955078125
3.69258260726929 -0.289794921875
3.69810056686401 -0.2923583984375
3.69983768463135 -0.29296875
3.70148158073425 -0.2930908203125
3.70182704925537 -0.293212890625
3.70251679420471 -0.29345703125
3.70517921447754 -0.293701171875
3.70774054527283 -0.294189453125
3.70986342430115 -0.2943115234375
3.71028661727905 -0.2945556640625
3.7106249332428 -0.2945556640625
3.71206021308899 -0.294677734375
3.71424579620361 -0.2950439453125
3.71466493606567 -0.2950439453125
3.7196626663208 -0.297119140625
3.72073793411255 -0.2977294921875
3.7215633392334 -0.2978515625
3.7223048210144 -0.2979736328125
3.72337365150452 -0.298095703125
3.72591161727905 -0.298583984375
3.72729730606079 -0.2987060546875
3.73271536827087 -0.301025390625
3.73311710357666 -0.3016357421875
3.73367857933044 -0.3017578125
3.7367947101593 -0.302001953125
3.73893904685974 -0.30224609375
3.74083614349365 -0.302490234375
3.74327445030212 -0.302734375
3.74429297447205 -0.302978515625
3.75004529953003 -0.3057861328125
3.75089383125305 -0.306396484375
3.7515869140625 -0.306640625
3.75442481040955 -0.3070068359375
3.75587487220764 -0.3074951171875
3.75762367248535 -0.3077392578125
3.75838184356689 -0.3079833984375
3.76027154922485 -0.3082275390625
3.76380228996277 -0.309326171875
3.76462435722351 -0.3096923828125
3.76574301719666 -0.3099365234375
3.76730442047119 -0.310302734375
3.76774930953979 -0.310546875
3.76871204376221 -0.3106689453125
3.76967263221741 -0.3109130859375
3.77004146575928 -0.31103515625
3.77349376678467 -0.311767578125
3.77371335029602 -0.3118896484375
3.77407884597778 -0.3121337890625
3.77553772926331 -0.3121337890625
3.77699160575867 -0.3123779296875
3.77728176116943 -0.3125
3.7775719165802 -0.3126220703125
3.77887439727783 -0.3126220703125
3.7791633605957 -0.312744140625
3.78304553031921 -0.3138427734375
3.78326034545898 -0.31396484375
3.7834746837616 -0.31396484375
3.78354620933533 -0.31396484375
3.7845458984375 -0.314208984375
3.78511619567871 -0.314208984375
3.78518748283386 -0.3143310546875
3.78547215461731 -0.3143310546875
3.78575682640076 -0.3143310546875
3.78575682640076 -0.3143310546875
3.78646755218506 -0.314453125
3.78660941123962 -0.314453125
3.78660941123962 -0.314453125
3.78682231903076 -0.314453125
3.78724789619446 -0.314453125
3.787672996521 -0.3145751953125
3.78859257698059 -0.314697265625
3.79063701629639 -0.31494140625
3.79091811180115 -0.3150634765625
3.79126954078674 -0.315185546875
3.79204130172729 -0.315185546875
3.79232168197632 -0.315185546875
3.79406952857971 -0.3153076171875
3.79469704627991 -0.3153076171875
3.79483652114868 -0.3153076171875
3.79664373397827 -0.3154296875
3.79685163497925 -0.3154296875
3.79775214195251 -0.3154296875
3.79789042472839 -0.3155517578125
3.79802870750427 -0.3155517578125
3.79844355583191 -0.3155517578125
3.79858160018921 -0.315673828125
3.79934048652649 -0.315673828125
3.80016708374023 -0.31591796875
3.80092310905457 -0.31591796875
3.80099177360535 -0.31591796875
3.80119776725769 -0.31591796875
3.80147218704224 -0.31591796875
3.80263686180115 -0.3160400390625
3.80270528793335 -0.3160400390625
3.80338883399963 -0.3160400390625
3.80338883399963 -0.3160400390625
3.80359363555908 -0.3160400390625
3.80509281158447 -0.3160400390625
3.80529689788818 -0.316162109375
3.80543279647827 -0.316162109375
3.80590844154358 -0.316162109375
3.80611205101013 -0.316162109375
3.80651903152466 -0.316162109375
3.80672240257263 -0.3162841796875
3.80719661712646 -0.3162841796875
3.8084135055542 -0.3162841796875
3.80848097801208 -0.3162841796875
3.80868339538574 -0.3162841796875
3.80949234962463 -0.31640625
3.80969429016113 -0.31640625
3.81003069877625 -0.31640625
3.81009793281555 -0.31640625
3.81070280075073 -0.3165283203125
3.81090426445007 -0.3165283203125
3.81090426445007 -0.3165283203125
3.81217765808105 -0.3165283203125
3.81224465370178 -0.316650390625
3.81504607200623 -0.3167724609375
3.81524562835693 -0.31689453125
3.81524562835693 -0.31689453125
3.81557774543762 -0.31689453125
3.81590962409973 -0.3170166015625
3.81617498397827 -0.3170166015625
3.81624126434326 -0.3170166015625
3.81993865966797 -0.3173828125
3.82026720046997 -0.3175048828125
3.82052993774414 -0.3175048828125
3.82072687149048 -0.3175048828125
3.82085800170898 -0.3175048828125
3.82118582725525 -0.3175048828125
3.82138252258301 -0.3175048828125
3.82184100151062 -0.317626953125
3.82210254669189 -0.317626953125
3.82242965698242 -0.317626953125
3.82295227050781 -0.3177490234375
3.82314801216125 -0.3177490234375
3.82477641105652 -0.3177490234375
3.82490634918213 -0.31787109375
3.82510137557983 -0.31787109375
3.82510137557983 -0.31787109375
3.8256208896637 -0.31787109375
3.82581543922424 -0.31787109375
3.82581543922424 -0.31787109375
3.82613968849182 -0.31787109375
3.82846665382385 -0.318359375
3.83078098297119 -0.3184814453125
3.83084511756897 -0.3184814453125
3.8310375213623 -0.3184814453125
3.83122968673706 -0.3184814453125
3.83154988288879 -0.318603515625
3.83186984062195 -0.318603515625
3.83218955993652 -0.318603515625
3.83218955993652 -0.318603515625
3.83276438713074 -0.3187255859375
3.83372068405151 -0.3187255859375
3.83372068405151 -0.3187255859375
3.83391165733337 -0.3187255859375
3.83410263061523 -0.3187255859375
3.83410263061523 -0.3187255859375
3.83435702323914 -0.3187255859375
3.83562707901001 -0.31884765625
3.83562707901001 -0.31884765625
3.83562707901001 -0.3189697265625
3.83657717704773 -0.3189697265625
3.8368935585022 -0.3189697265625
3.83796691894531 -0.319091796875
3.83809304237366 -0.319091796875
3.83834528923035 -0.319091796875
3.83840823173523 -0.319091796875
3.83840823173523 -0.319091796875
3.83922648429871 -0.319091796875
3.83922648429871 -0.319091796875
3.84054517745972 -0.3192138671875
3.84067058563232 -0.3193359375
3.84067058563232 -0.3193359375
3.84248447418213 -0.3193359375
3.84248447418213 -0.3193359375
3.84267163276672 -0.3193359375
3.84323287010193 -0.3193359375
3.84410429000854 -0.3194580078125
3.84416651725769 -0.3194580078125
3.84516000747681 -0.3194580078125
3.8457179069519 -0.319580078125
3.84608960151672 -0.319580078125
3.84608960151672 -0.319580078125
3.84658455848694 -0.319580078125
3.84658455848694 -0.319580078125
3.84701704978943 -0.319580078125
3.84763431549072 -0.3197021484375
3.8485586643219 -0.3197021484375
3.84874320030212 -0.3197021484375
3.84874320030212 -0.3197021484375
3.84984922409058 -0.31982421875
3.84984922409058 -0.31982421875
3.85009455680847 -0.31982421875
3.85076880455017 -0.31982421875
3.85290670394897 -0.3199462890625
3.85290670394897 -0.3199462890625
3.85503435134888 -0.3203125
3.8554584980011 -0.3204345703125
3.85606384277344 -0.3204345703125
3.85648727416992 -0.3204345703125
3.85672879219055 -0.3204345703125
3.8571515083313 -0.3204345703125
3.85883784294128 -0.321044921875
3.8596785068512 -0.3211669921875
3.8602180480957 -0.3212890625
3.86183309555054 -0.321533203125
3.86266803741455 -0.321533203125
3.8628466129303 -0.3216552734375
3.86557769775391 -0.3223876953125
3.86581444740295 -0.32275390625
3.86758542060852 -0.322998046875
3.86882066726685 -0.3231201171875
3.86929035186768 -0.3232421875
3.86970090866089 -0.3232421875
3.87057948112488 -0.3233642578125
3.87087202072144 -0.323486328125
3.87209796905518 -0.32373046875
3.87238931655884 -0.32373046875
3.8726806640625 -0.3238525390625
3.87343692779541 -0.3238525390625
3.87436580657959 -0.3240966796875
3.87453985214233 -0.3243408203125
3.87604451179504 -0.3243408203125
3.87673735618591 -0.324462890625
3.87691020965576 -0.324462890625
3.87714099884033 -0.3245849609375
3.87800455093384 -0.32470703125
3.87823438644409 -0.32470703125
3.87846422195435 -0.3248291015625
3.87915325164795 -0.3248291015625
3.88166999816895 -0.325439453125
3.88195490837097 -0.3255615234375
3.88195490837097 -0.32568359375
3.88201189041138 -0.32568359375
3.88246750831604 -0.3258056640625
3.88303661346436 -0.3258056640625
3.88320708274841 -0.325927734375
3.88337755203247 -0.325927734375
3.88366150856018 -0.325927734375
3.88371825218201 -0.325927734375
3.88400197029114 -0.325927734375
3.88490867614746 -0.325927734375
3.88541769981384 -0.3260498046875
3.88558745384216 -0.3260498046875
3.88581323623657 -0.3260498046875
3.88598275184631 -0.3260498046875
3.88609576225281 -0.326171875
3.88637781143188 -0.326171875
3.88801097869873 -0.3262939453125
3.88817954063416 -0.3262939453125
3.88840413093567 -0.3262939453125
3.88857269287109 -0.3262939453125
3.88857269287109 -0.3262939453125
3.88874101638794 -0.3262939453125
3.88879704475403 -0.3262939453125
3.88879704475403 -0.3262939453125
3.88879704475403 -0.3262939453125
3.88896536827087 -0.326416015625
3.88913345336914 -0.326416015625
3.88935780525208 -0.326416015625
3.88941383361816 -0.326416015625
3.89092373847961 -0.3265380859375
3.89120292663574 -0.32666015625
3.89125871658325 -0.32666015625
3.89265108108521 -0.32666015625
3.892817735672 -0.32666015625
3.892817735672 -0.32666015625
3.8930401802063 -0.3267822265625
3.89315128326416 -0.3267822265625
3.8935399055481 -0.3267822265625
3.89359521865845 -0.3267822265625
3.89359521865845 -0.3267822265625
3.89376163482666 -0.3267822265625
3.89376163482666 -0.3267822265625
3.89392805099487 -0.3267822265625
3.89392805099487 -0.3267822265625
3.89409446716309 -0.3267822265625
3.89431595802307 -0.326904296875
3.89481425285339 -0.326904296875
3.89481425285339 -0.326904296875
3.89481425285339 -0.326904296875
3.8950355052948 -0.326904296875
3.8950355052948 -0.326904296875
3.8950355052948 -0.326904296875
3.89685678482056 -0.3271484375
3.89718699455261 -0.3271484375
3.89729714393616 -0.3271484375
3.89729714393616 -0.3271484375
3.89740705490112 -0.3271484375
3.89757204055786 -0.3271484375
3.89762711524963 -0.3271484375
3.89762711524963 -0.3271484375
3.89834117889404 -0.3271484375
3.89856052398682 -0.3271484375
3.89856052398682 -0.3271484375
3.89861559867859 -0.3271484375
3.89861559867859 -0.3271484375
3.89861559867859 -0.3271484375
3.89861559867859 -0.3271484375
3.89878010749817 -0.3271484375
3.89878010749817 -0.3271484375
3.90014863014221 -0.3272705078125
3.90014863014221 -0.3272705078125
3.90014863014221 -0.3272705078125
3.90113115310669 -0.3272705078125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90124034881592 -0.327392578125
3.90140390396118 -0.327392578125
3.90140390396118 -0.327392578125
3.90140390396118 -0.327392578125
3.90140390396118 -0.327392578125
3.90156722068787 -0.327392578125
3.90156722068787 -0.327392578125
3.90162181854248 -0.327392578125
3.90183973312378 -0.327392578125
3.90189409255981 -0.327392578125
3.90194845199585 -0.327392578125
3.90276408195496 -0.327392578125
3.90281844139099 -0.327392578125
3.90363264083862 -0.3275146484375
3.90384936332703 -0.3275146484375
3.90401196479797 -0.3275146484375
3.90417432785034 -0.3275146484375
3.90417432785034 -0.3275146484375
3.9042284488678 -0.3275146484375
3.90428256988525 -0.3275146484375
3.90428256988525 -0.3275146484375
3.90449905395508 -0.3275146484375
3.90455317497253 -0.3275146484375
3.9047155380249 -0.3275146484375
3.90476965904236 -0.3275146484375
3.90476965904236 -0.3275146484375
3.90476965904236 -0.3275146484375
3.90574193000793 -0.32763671875
3.90574193000793 -0.32763671875
3.90590381622314 -0.32763671875
3.90595769882202 -0.32763671875
3.90649676322937 -0.32763671875
3.90725016593933 -0.32763671875
3.90735769271851 -0.32763671875
3.9074113368988 -0.32763671875
3.90762639045715 -0.32763671875
3.90768003463745 -0.32763671875
3.90773367881775 -0.3277587890625
3.90773367881775 -0.3277587890625
3.90773367881775 -0.3277587890625
3.90789484977722 -0.3277587890625
3.90794849395752 -0.3277587890625
3.90794849395752 -0.3277587890625
3.90810966491699 -0.3277587890625
3.90810966491699 -0.3277587890625
3.90816330909729 -0.3277587890625
3.90821695327759 -0.3277587890625
3.90821695327759 -0.3277587890625
3.90821695327759 -0.3277587890625
3.91025066375732 -0.3280029296875
3.91030406951904 -0.3280029296875
3.9104642868042 -0.3280029296875
3.91163682937622 -0.3280029296875
3.91184973716736 -0.3280029296875
3.9119029045105 -0.3280029296875
3.9120626449585 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.3280029296875
3.91211581230164 -0.328125
3.91264700889587 -0.328125
3.91291260719299 -0.328125
3.91291260719299 -0.328125
3.91296553611755 -0.328125
3.91296553611755 -0.328125
3.91301870346069 -0.328125
3.91301870346069 -0.328125
3.91301870346069 -0.328125
3.91413140296936 -0.328125
3.91429018974304 -0.3282470703125
3.9143431186676 -0.3282470703125
3.9143431186676 -0.3282470703125
3.9143431186676 -0.3282470703125
3.91450190544128 -0.3282470703125
3.91450190544128 -0.3282470703125
3.91455459594727 -0.3282470703125
3.91460752487183 -0.3282470703125
3.91460752487183 -0.3282470703125
3.91466045379639 -0.3282470703125
3.91471338272095 -0.3282470703125
3.91476607322693 -0.3282470703125
3.91492462158203 -0.3282470703125
3.91613793373108 -0.3282470703125
3.9168221950531 -0.328369140625
3.91698002815247 -0.328369140625
3.91703271865845 -0.328369140625
3.91734790802002 -0.328369140625
3.9174530506134 -0.328369140625
3.91865921020508 -0.328369140625
3.91876411437988 -0.328369140625
3.91876411437988 -0.328369140625
3.91876411437988 -0.328369140625
3.91876411437988 -0.328369140625
3.91923499107361 -0.328369140625
3.91923499107361 -0.328369140625
3.91923499107361 -0.328369140625
3.91939187049866 -0.328369140625
3.91944432258606 -0.328369140625
3.91949653625488 -0.328369140625
3.91970562934875 -0.328369140625
3.91970562934875 -0.328369140625
3.91970562934875 -0.328369140625
3.92007112503052 -0.328369140625
3.92007112503052 -0.3284912109375
3.92007112503052 -0.3284912109375
3.92007112503052 -0.3284912109375
3.92022776603699 -0.3284912109375
3.92033195495605 -0.3284912109375
3.92059278488159 -0.3284912109375
3.92064499855042 -0.3284912109375
3.92064499855042 -0.3284912109375
3.92132234573364 -0.3284912109375
3.92132234573364 -0.3284912109375
3.92132234573364 -0.3284912109375
3.92142629623413 -0.3284912109375
3.92147827148438 -0.3284912109375
3.9215304851532 -0.3284912109375
3.9215304851532 -0.3284912109375
3.9215304851532 -0.3284912109375
3.9215304851532 -0.3284912109375
3.92215442657471 -0.3284912109375
3.92231011390686 -0.32861328125
3.92365837097168 -0.32861328125
3.92371010780334 -0.32861328125
3.92376184463501 -0.32861328125
3.92376184463501 -0.32861328125
};
\end{axis}

\begin{axis}[
tick align=outside,
tick pos=left,
% title={\Huge\ce{S4}},
title style={yshift=20pt}, 
x grid style={darkgray176},
xlabel={COI}, 
xtick={0,1,2,3,4},
extra x tick labels={\small$\text{log}_{10}$}, 
extra x ticks={5.5}, 
extra x tick style={grid=none, tickwidth=0, tick label style={opacity=1}},
xmin=-0.23, xmax=5.53596482276916,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Energy (Ha)},
ymin=-0.471807861328125, ymax=0.022467041015625,
ytick style={color=black},
legend style = { column sep = 10pt, legend columns = -1, legend to name = grouplegend, draw=none, fill=none},
ylabel shift=-5pt,
width=0.35\textwidth,
height=0.25\textwidth,
every axis y label/.style={
    at={(-0.20,1.13)},
    anchor=west,
    },
ylabel style={align=center, inner sep=0pt, yshift=3pt, font=\large\bfseries\boldmath},
xlabel style={align=center, inner sep=0pt, font=\large\bfseries\boldmath},
x tick label style={font=\large\bfseries\boldmath},
y tick label style={font=\large\bfseries\boldmath},
at={(c17)}
]
\addplot [ultra thick, brown, dashed]
table {%
0.903090000152588 0
1.17609131336212 -0.0001220703125
1.38021123409271 -0.0001220703125
1.57978355884552 -0.0001220703125
1.73239374160767 -0.0001220703125
1.97312784194946 -0.0001220703125
2.17609119415283 -0.0001220703125
2.25527238845825 -0.0001220703125
2.290034532547 -0.0001220703125
2.44715809822083 -0.0001220703125
2.46686768531799 -0.0001220703125
2.48855066299438 -0.000244140625
2.50379061698914 -0.000244140625
2.52891659736633 -0.000244140625
2.53907608985901 -0.000244140625
2.55630254745483 -0.000244140625
2.62117624282837 -0.000244140625
2.66086554527283 -0.000244140625
2.69548177719116 -0.000244140625
2.81756544113159 -0.0003662109375
2.82607483863831 -0.0003662109375
2.83569049835205 -0.0003662109375
2.84135937690735 -0.0003662109375
2.84818911552429 -0.0003662109375
3.26997971534729 -0.0020751953125
3.29710364341736 -0.0052490234375
3.39181685447693 -0.0057373046875
3.40500473976135 -0.006591796875
3.44575977325439 -0.00732421875
3.45924162864685 -0.0076904296875
3.5156090259552 -0.00830078125
3.61193561553955 -0.01611328125
3.63758969306946 -0.021728515625
3.6749529838562 -0.0240478515625
3.70782566070557 -0.025634765625
3.74233222007751 -0.0302734375
3.77298140525818 -0.033935546875
3.84048247337341 -0.043212890625
3.86805629730225 -0.053466796875
3.92350316047668 -0.0601806640625
3.95727205276489 -0.0673828125
3.97717475891113 -0.07666015625
3.99808478355408 -0.0841064453125
4.02800178527832 -0.091064453125
4.04020643234253 -0.096435546875
4.07007503509521 -0.1009521484375
4.0873908996582 -0.104248046875
4.10856485366821 -0.1080322265625
4.12277269363403 -0.110107421875
4.13836574554443 -0.1114501953125
4.14986562728882 -0.113037109375
4.16755342483521 -0.1199951171875
4.18012571334839 -0.1219482421875
4.19614839553833 -0.1265869140625
4.20588064193726 -0.1285400390625
4.21290636062622 -0.1295166015625
4.22608423233032 -0.13330078125
4.23482084274292 -0.1356201171875
4.24954080581665 -0.1390380859375
4.25642919540405 -0.140380859375
4.26401472091675 -0.142333984375
4.27107429504395 -0.1439208984375
4.27854776382446 -0.14599609375
4.28786897659302 -0.148681640625
4.29959440231323 -0.1583251953125
4.30990695953369 -0.17041015625
4.31580257415771 -0.174072265625
4.32397365570068 -0.17578125
4.33245849609375 -0.17822265625
4.3443922996521 -0.1812744140625
4.35139036178589 -0.1832275390625
4.35466527938843 -0.184326171875
4.37080907821655 -0.201416015625
4.37723350524902 -0.2064208984375
4.38257551193237 -0.2083740234375
4.38776350021362 -0.2109375
4.39501190185547 -0.2158203125
4.40174531936646 -0.2183837890625
4.40684652328491 -0.2193603515625
4.41006851196289 -0.2200927734375
4.41580772399902 -0.221923828125
4.42112636566162 -0.2230224609375
4.42785930633545 -0.224365234375
4.43247222900391 -0.2259521484375
4.43741750717163 -0.2269287109375
4.44169521331787 -0.22802734375
4.44566631317139 -0.2286376953125
4.45663928985596 -0.2327880859375
4.46178340911865 -0.23583984375
4.46529340744019 -0.2369384765625
4.46884918212891 -0.23779296875
4.4717903137207 -0.2386474609375
4.4787540435791 -0.2423095703125
4.48255920410156 -0.2431640625
4.48599100112915 -0.2437744140625
4.49190759658813 -0.2486572265625
4.49627923965454 -0.249755859375
4.50045585632324 -0.2513427734375
4.50696468353271 -0.253662109375
4.5112681388855 -0.2548828125
4.51418876647949 -0.256103515625
4.51720905303955 -0.257568359375
4.52071905136108 -0.25830078125
4.5250186920166 -0.25927734375
4.52778434753418 -0.260009765625
4.53443241119385 -0.2685546875
4.54186630249023 -0.2733154296875
4.54510927200317 -0.275390625
4.55035066604614 -0.2784423828125
4.55379819869995 -0.2806396484375
4.55672454833984 -0.2821044921875
4.56108951568604 -0.2828369140625
4.56255435943604 -0.283447265625
4.56616640090942 -0.2843017578125
4.57106781005859 -0.286376953125
4.57532644271851 -0.28857421875
4.57658338546753 -0.2896728515625
4.5826997756958 -0.29052734375
4.58726167678833 -0.2945556640625
4.58972644805908 -0.2952880859375
4.59183216094971 -0.2962646484375
4.59496688842773 -0.29736328125
4.59722328186035 -0.2979736328125
4.59914064407349 -0.2984619140625
4.60178852081299 -0.2987060546875
4.61086225509644 -0.3037109375
4.61280488967896 -0.3045654296875
4.61501312255859 -0.305419921875
4.61654901504517 -0.3057861328125
4.61978197097778 -0.3070068359375
4.62119722366333 -0.307373046875
4.62302160263062 -0.307861328125
4.62512731552124 -0.308349609375
4.62716102600098 -0.3087158203125
4.62922620773315 -0.3109130859375
4.63212299346924 -0.3114013671875
4.63329696655273 -0.3115234375
4.63531303405762 -0.31201171875
4.63646793365479 -0.312255859375
4.63838958740234 -0.3131103515625
4.64270210266113 -0.314453125
4.64489126205444 -0.3155517578125
4.64699172973633 -0.3165283203125
4.6504340171814 -0.3170166015625
4.65260410308838 -0.3172607421875
4.6609034538269 -0.322998046875
4.66273880004883 -0.323974609375
4.66374778747559 -0.32421875
4.66477346420288 -0.3243408203125
4.66637754440308 -0.324462890625
4.66772365570068 -0.32470703125
4.66905641555786 -0.3248291015625
4.67026424407959 -0.3250732421875
4.67094135284424 -0.3251953125
4.67500782012939 -0.3262939453125
4.67651987075806 -0.3267822265625
4.67875480651855 -0.326904296875
4.68040800094604 -0.3275146484375
4.68256902694702 -0.3277587890625
4.68356037139893 -0.3280029296875
4.69088697433472 -0.3310546875
4.69221210479736 -0.331298828125
4.69329595565796 -0.33154296875
4.6953501701355 -0.331787109375
4.69663572311401 -0.33203125
4.70016717910767 -0.3321533203125
4.70277500152588 -0.3323974609375
4.70759582519531 -0.33349609375
4.70842933654785 -0.3341064453125
4.70984649658203 -0.334228515625
4.71479892730713 -0.33447265625
4.71594476699829 -0.3348388671875
4.71710443496704 -0.3350830078125
4.71803665161133 -0.335205078125
4.71910762786865 -0.3353271484375
4.72033309936523 -0.3355712890625
4.72104358673096 -0.335693359375
4.72192573547363 -0.335693359375
4.73145961761475 -0.3397216796875
4.73242616653442 -0.3406982421875
4.73624515533447 -0.3411865234375
4.73881244659424 -0.3416748046875
4.74001502990723 -0.341796875
4.74258375167847 -0.3419189453125
4.74637746810913 -0.34228515625
4.74950456619263 -0.342529296875
4.75045442581177 -0.3426513671875
4.75175619125366 -0.3427734375
4.75296211242676 -0.3428955078125
4.75807905197144 -0.34326171875
4.76060342788696 -0.3436279296875
4.76108551025391 -0.3436279296875
4.76678466796875 -0.344482421875
4.77120542526245 -0.3453369140625
4.77266645431519 -0.3453369140625
4.77899026870728 -0.3477783203125
4.7801947593689 -0.3482666015625
4.78618335723877 -0.35009765625
4.78792762756348 -0.3505859375
4.79108667373657 -0.3509521484375
4.79443216323853 -0.351318359375
4.79813957214355 -0.351806640625
4.80169868469238 -0.3521728515625
4.80499076843262 -0.3526611328125
4.81083726882935 -0.353759765625
4.81255912780762 -0.3546142578125
4.81792879104614 -0.35546875
4.82161855697632 -0.355712890625
4.82562065124512 -0.3565673828125
4.82694244384766 -0.3568115234375
4.83026123046875 -0.357177734375
4.83270025253296 -0.357421875
4.84017515182495 -0.3663330078125
4.84285879135132 -0.3699951171875
4.85086679458618 -0.372802734375
4.85186958312988 -0.3731689453125
4.85535573959351 -0.375
4.85816431045532 -0.3756103515625
4.86072111129761 -0.3760986328125
4.86404800415039 -0.376708984375
4.86899709701538 -0.377685546875
4.87099456787109 -0.3782958984375
4.87357616424561 -0.3787841796875
4.87767648696899 -0.3802490234375
4.87933111190796 -0.380615234375
4.8808422088623 -0.3807373046875
4.88291692733765 -0.3809814453125
4.88463687896729 -0.381103515625
4.892333984375 -0.3843994140625
4.89582586288452 -0.385009765625
4.89780855178833 -0.38525390625
4.89948654174805 -0.3853759765625
4.90054750442505 -0.385498046875
4.90182876586914 -0.3857421875
4.90324211120605 -0.3858642578125
4.90467214584351 -0.385986328125
4.90854406356812 -0.3865966796875
4.91089105606079 -0.3868408203125
4.9116530418396 -0.386962890625
4.91243457794189 -0.386962890625
4.91542625427246 -0.38720703125
4.91811943054199 -0.3876953125
4.91876411437988 -0.387939453125
4.9212441444397 -0.38818359375
4.92221689224243 -0.3883056640625
4.92503881454468 -0.3885498046875
4.92703676223755 -0.388671875
4.92829847335815 -0.388671875
4.93061780929565 -0.38916015625
4.9324836730957 -0.3892822265625
4.93412971496582 -0.389404296875
4.93537139892578 -0.3895263671875
4.93623208999634 -0.3896484375
4.93828439712524 -0.39013671875
4.94060134887695 -0.3902587890625
4.94226598739624 -0.3902587890625
4.94318771362305 -0.390380859375
4.94574403762817 -0.3909912109375
4.94721794128418 -0.39111328125
4.94940948486328 -0.391357421875
4.95170164108276 -0.391845703125
4.95327615737915 -0.3919677734375
4.95370674133301 -0.3922119140625
4.95623111724854 -0.3929443359375
4.95726251602173 -0.39306640625
4.95891237258911 -0.393310546875
4.96006155014038 -0.3935546875
4.96335315704346 -0.39501953125
4.96481561660767 -0.395263671875
4.9666953086853 -0.3953857421875
4.96868371963501 -0.3956298828125
4.97034215927124 -0.395751953125
4.97130393981934 -0.3958740234375
4.97292470932007 -0.396240234375
4.9749584197998 -0.3963623046875
4.97831773757935 -0.3968505859375
4.98209953308105 -0.3970947265625
4.98284530639648 -0.3973388671875
4.98698663711548 -0.3983154296875
4.98832273483276 -0.3985595703125
4.9902811050415 -0.3988037109375
4.99161148071289 -0.39892578125
4.9939603805542 -0.399169921875
4.99679613113403 -0.3997802734375
4.99774026870728 -0.400146484375
4.99916982650757 -0.400390625
5.00073337554932 -0.4005126953125
5.00194120407104 -0.400634765625
5.0041708946228 -0.4010009765625
5.00591373443604 -0.4013671875
5.00683832168579 -0.4014892578125
5.01084661483765 -0.4039306640625
5.01244497299194 -0.404296875
5.01434421539307 -0.4046630859375
5.02021598815918 -0.4075927734375
5.02093696594238 -0.4085693359375
5.02272510528564 -0.408935546875
5.02485513687134 -0.4091796875
5.02828645706177 -0.41259765625
5.02944469451904 -0.413818359375
5.0318284034729 -0.4141845703125
5.03273153305054 -0.414306640625
5.03440380096436 -0.41455078125
5.03558158874512 -0.4146728515625
5.0366849899292 -0.4149169921875
5.03845310211182 -0.415283203125
5.03976678848267 -0.4158935546875
5.04073667526245 -0.416015625
5.04344892501831 -0.418212890625
5.04454374313354 -0.4185791015625
5.04590940475464 -0.4188232421875
5.04658079147339 -0.4189453125
5.04905128479004 -0.4205322265625
5.04932641983032 -0.4207763671875
5.05110216140747 -0.4210205078125
5.05234003067017 -0.4210205078125
5.05354309082031 -0.421142578125
5.05439853668213 -0.421142578125
5.05490398406982 -0.4212646484375
5.05608129501343 -0.4212646484375
5.0576434135437 -0.42138671875
5.05845642089844 -0.4215087890625
5.05938148498535 -0.4215087890625
5.05977535247803 -0.4215087890625
5.06094694137573 -0.421630859375
5.06217956542969 -0.4217529296875
5.06376838684082 -0.422607421875
5.0648136138916 -0.4228515625
5.06595659255981 -0.4228515625
5.06702995300293 -0.4229736328125
5.06797409057617 -0.423095703125
5.06865692138672 -0.4232177734375
5.06965684890747 -0.42333984375
5.07082796096802 -0.423583984375
5.07110118865967 -0.423583984375
5.07350206375122 -0.4259033203125
5.07421636581421 -0.42626953125
5.0753755569458 -0.4263916015625
5.076247215271 -0.4263916015625
5.07709884643555 -0.4263916015625
5.07821750640869 -0.426513671875
5.07912349700928 -0.426513671875
5.08027267456055 -0.4266357421875
5.08137989044189 -0.4267578125
5.08200931549072 -0.4267578125
5.08306884765625 -0.4267578125
5.08396482467651 -0.4267578125
5.08544397354126 -0.427001953125
5.08680105209351 -0.4271240234375
5.08756494522095 -0.42724609375
5.08879518508911 -0.42724609375
5.08964014053345 -0.4273681640625
5.09071636199951 -0.4273681640625
5.09217309951782 -0.4276123046875
5.0928783416748 -0.4278564453125
5.09450960159302 -0.4278564453125
5.09540319442749 -0.427978515625
5.09632587432861 -0.4281005859375
5.09707689285278 -0.4281005859375
5.09870958328247 -0.4283447265625
5.10001182556152 -0.428466796875
5.10026693344116 -0.4285888671875
5.10104560852051 -0.4287109375
5.1018123626709 -0.4287109375
5.10255718231201 -0.4287109375
5.10321521759033 -0.4287109375
5.10398483276367 -0.4287109375
5.10587120056152 -0.4290771484375
5.10614347457886 -0.42919921875
5.10680961608887 -0.42919921875
5.10728454589844 -0.42919921875
5.11021566390991 -0.4300537109375
5.11056280136108 -0.4302978515625
5.11099672317505 -0.4302978515625
5.11429405212402 -0.4315185546875
5.11474084854126 -0.4320068359375
5.11546421051025 -0.4320068359375
5.11589670181274 -0.43212890625
5.11672735214233 -0.43212890625
5.11730766296387 -0.4322509765625
5.11813592910767 -0.4322509765625
5.11846303939819 -0.432373046875
5.11897850036621 -0.432373046875
5.11925935745239 -0.432373046875
5.1195592880249 -0.432373046875
5.12067937850952 -0.4324951171875
5.12082386016846 -0.4324951171875
5.12154674530029 -0.4326171875
5.12226819992065 -0.4326171875
5.12340068817139 -0.4327392578125
5.12378644943237 -0.4327392578125
5.12413883209229 -0.4327392578125
5.12537717819214 -0.433349609375
5.12692642211914 -0.4334716796875
5.12830877304077 -0.4337158203125
5.12865781784058 -0.433837890625
5.12941598892212 -0.4339599609375
5.1299090385437 -0.4339599609375
5.13079357147217 -0.43408203125
5.13156747817993 -0.4342041015625
5.13223743438721 -0.434326171875
5.13257646560669 -0.4344482421875
5.13356781005859 -0.4344482421875
5.13408136367798 -0.4345703125
5.1343207359314 -0.4346923828125
5.13460111618042 -0.4346923828125
5.13504981994629 -0.434814453125
5.13579702377319 -0.434814453125
5.13614654541016 -0.4349365234375
5.13727188110352 -0.435302734375
5.13748693466187 -0.435302734375
5.13795518875122 -0.435302734375
5.13969039916992 -0.435546875
5.13996076583862 -0.435546875
5.14115476608276 -0.4356689453125
5.14135551452637 -0.4356689453125
5.14191675186157 -0.4356689453125
5.14217042922974 -0.4356689453125
5.14232397079468 -0.435791015625
5.14426612854004 -0.4361572265625
5.14466142654419 -0.4361572265625
5.14503765106201 -0.4361572265625
5.14543867111206 -0.4361572265625
5.14564371109009 -0.436279296875
5.14745044708252 -0.436279296875
5.14769506454468 -0.436279296875
5.14893245697021 -0.4364013671875
5.14898490905762 -0.4364013671875
5.15055084228516 -0.4365234375
5.15090990066528 -0.4365234375
5.15113067626953 -0.4365234375
5.15173768997192 -0.4366455078125
5.15201616287231 -0.4366455078125
5.15219354629517 -0.4366455078125
5.15421676635742 -0.43701171875
5.15466451644897 -0.43701171875
5.15517807006836 -0.43701171875
5.15527248382568 -0.43701171875
5.15565156936646 -0.43701171875
5.15623712539673 -0.4371337890625
5.15774393081665 -0.437255859375
5.15793418884277 -0.437255859375
5.15876960754395 -0.437255859375
5.15894412994385 -0.437255859375
5.16192483901978 -0.4381103515625
5.16216993331909 -0.438232421875
5.16240310668945 -0.438232421875
5.16255855560303 -0.438232421875
5.16266584396362 -0.438232421875
5.16286897659302 -0.438232421875
5.16325092315674 -0.438232421875
5.16343259811401 -0.438232421875
5.16375732421875 -0.438232421875
5.1641001701355 -0.438232421875
5.16419506072998 -0.4383544921875
5.16464424133301 -0.4383544921875
5.16475105285645 -0.4383544921875
5.16595315933228 -0.4383544921875
5.16647434234619 -0.4384765625
5.16692399978638 -0.4384765625
5.16739130020142 -0.4384765625
5.167884349823 -0.4384765625
5.17140483856201 -0.4390869140625
5.17163562774658 -0.4390869140625
5.17164468765259 -0.4390869140625
5.17206573486328 -0.439208984375
5.17303466796875 -0.439208984375
5.1731743812561 -0.439208984375
5.17435073852539 -0.4393310546875
5.17445802688599 -0.4393310546875
5.17496919631958 -0.4393310546875
5.17532634735107 -0.439453125
5.17605638504028 -0.439453125
5.17687225341797 -0.439453125
5.1793966293335 -0.4395751953125
5.1796350479126 -0.4398193359375
5.1798849105835 -0.4398193359375
5.1810941696167 -0.43994140625
5.18173217773438 -0.43994140625
5.18205785751343 -0.43994140625
5.18325853347778 -0.4400634765625
5.18350887298584 -0.4400634765625
5.18383026123047 -0.4400634765625
5.18503189086914 -0.440185546875
5.18577146530151 -0.440185546875
5.18643665313721 -0.4403076171875
5.18662595748901 -0.4403076171875
5.18663454055786 -0.4403076171875
5.18882465362549 -0.44091796875
5.18895959854126 -0.44091796875
5.18899869918823 -0.44091796875
5.1901159286499 -0.4410400390625
5.19033432006836 -0.4410400390625
5.19045495986938 -0.4410400390625
5.19157123565674 -0.4410400390625
5.19190073013306 -0.441162109375
5.19221305847168 -0.441162109375
5.19493579864502 -0.4422607421875
5.1954927444458 -0.4423828125
5.19573068618774 -0.4423828125
5.19583034515381 -0.4423828125
5.19638633728027 -0.4423828125
5.19725561141968 -0.4425048828125
5.1976113319397 -0.4425048828125
5.19801902770996 -0.4425048828125
5.20145463943481 -0.44287109375
5.20168924331665 -0.443115234375
5.2023549079895 -0.4432373046875
5.2028694152832 -0.4432373046875
5.20326662063599 -0.4432373046875
5.20357656478882 -0.443359375
5.20382118225098 -0.443359375
5.20424461364746 -0.443359375
5.20450782775879 -0.443359375
5.20520973205566 -0.443359375
5.20596981048584 -0.4434814453125
5.20665073394775 -0.4434814453125
5.20731925964355 -0.4434814453125
5.20873165130615 -0.443603515625
5.2089729309082 -0.443603515625
5.20958185195923 -0.4437255859375
5.2097053527832 -0.4437255859375
5.21002149581909 -0.4437255859375
5.21056461334229 -0.4437255859375
5.21057271957397 -0.4437255859375
5.21106433868408 -0.4437255859375
5.21133947372437 -0.4437255859375
5.2144250869751 -0.4442138671875
5.21451807022095 -0.4442138671875
5.21454429626465 -0.4442138671875
5.21463203430176 -0.4442138671875
5.21479082107544 -0.4443359375
5.21548938751221 -0.4443359375
5.21599674224854 -0.4443359375
5.21610260009766 -0.4443359375
5.21638774871826 -0.4443359375
5.21732091903687 -0.4444580078125
5.2178258895874 -0.4444580078125
5.21939086914062 -0.4447021484375
5.21972846984863 -0.4447021484375
5.22004270553589 -0.4447021484375
5.22069120407104 -0.44482421875
5.22101736068726 -0.44482421875
5.22109842300415 -0.44482421875
5.22173500061035 -0.44482421875
5.22188854217529 -0.44482421875
5.22214412689209 -0.44482421875
5.22257089614868 -0.44482421875
5.22341537475586 -0.4449462890625
5.22420167922974 -0.4449462890625
5.22467803955078 -0.4449462890625
5.22486162185669 -0.4449462890625
5.22496509552002 -0.4449462890625
5.22528600692749 -0.4449462890625
5.22561168670654 -0.445068359375
5.22575378417969 -0.445068359375
5.22600936889648 -0.445068359375
5.22606611251831 -0.445068359375
5.22717666625977 -0.4451904296875
5.22721290588379 -0.4451904296875
5.22726964950562 -0.4451904296875
5.2274112701416 -0.4451904296875
5.22821283340454 -0.4451904296875
5.22829532623291 -0.4453125
5.22854423522949 -0.4453125
5.22883415222168 -0.4453125
5.22906446456909 -0.4453125
5.23060464859009 -0.4454345703125
5.23067617416382 -0.4454345703125
5.23127603530884 -0.445556640625
5.23164796829224 -0.445556640625
5.2319712638855 -0.445556640625
5.23223876953125 -0.445556640625
5.23234033584595 -0.445556640625
5.2323784828186 -0.445556640625
5.23257446289062 -0.445556640625
5.23308515548706 -0.445556640625
5.23312330245972 -0.4456787109375
5.23349618911743 -0.4456787109375
5.23360013961792 -0.4456787109375
5.23380565643311 -0.4456787109375
5.23430442810059 -0.4456787109375
5.23431205749512 -0.4456787109375
5.23439598083496 -0.4456787109375
5.2348461151123 -0.4456787109375
5.23485374450684 -0.4456787109375
5.23489427566528 -0.4456787109375
5.23502063751221 -0.4456787109375
5.2354679107666 -0.4456787109375
5.23626756668091 -0.44580078125
5.23635578155518 -0.44580078125
5.23638105392456 -0.44580078125
5.23687219619751 -0.44580078125
5.23720455169678 -0.44580078125
5.23724222183228 -0.44580078125
5.2386908531189 -0.446044921875
5.23876333236694 -0.446044921875
5.23882627487183 -0.446044921875
5.23900651931763 -0.446044921875
5.23917198181152 -0.4461669921875
5.23996210098267 -0.4461669921875
5.24040174484253 -0.4461669921875
5.24049425125122 -0.4461669921875
5.24083137512207 -0.4461669921875
5.24102306365967 -0.4461669921875
5.2411904335022 -0.4461669921875
5.24143934249878 -0.4461669921875
5.24162626266479 -0.4461669921875
5.24174070358276 -0.4461669921875
5.24189519882202 -0.4461669921875
5.24201202392578 -0.4461669921875
5.24210405349731 -0.4461669921875
5.24245929718018 -0.4462890625
5.24252891540527 -0.4462890625
5.2425365447998 -0.4462890625
5.24279975891113 -0.4462890625
5.24283456802368 -0.4462890625
5.24298334121704 -0.4462890625
5.24344968795776 -0.4462890625
5.24346446990967 -0.4462890625
5.2436580657959 -0.4462890625
5.24388122558594 -0.4462890625
5.24447250366211 -0.4462890625
5.24550533294678 -0.4464111328125
5.24575710296631 -0.446533203125
5.24590969085693 -0.446533203125
5.24593210220337 -0.446533203125
5.24712610244751 -0.44677734375
5.24739646911621 -0.4468994140625
5.24760484695435 -0.4468994140625
5.24761962890625 -0.4468994140625
5.24775981903076 -0.4468994140625
5.24799776077271 -0.447021484375
5.2481107711792 -0.447021484375
5.24823331832886 -0.447021484375
5.24836826324463 -0.447021484375
5.24868202209473 -0.447021484375
5.24884080886841 -0.447021484375
5.24884605407715 -0.447021484375
5.2488751411438 -0.447021484375
5.249107837677 -0.447021484375
5.24928140640259 -0.447021484375
5.24956512451172 -0.447021484375
5.2495698928833 -0.447021484375
5.24997806549072 -0.447021484375
5.25003433227539 -0.447021484375
5.25005149841309 -0.447021484375
5.25016117095947 -0.447021484375
5.25016641616821 -0.447021484375
5.25042486190796 -0.447021484375
5.25044202804565 -0.4471435546875
5.25073957443237 -0.4471435546875
5.25074434280396 -0.4471435546875
5.25111961364746 -0.4471435546875
5.25136566162109 -0.4471435546875
5.25137042999268 -0.4471435546875
5.25174045562744 -0.4471435546875
5.25195693969727 -0.4471435546875
5.25208330154419 -0.447265625
5.25215864181519 -0.447265625
5.252197265625 -0.447265625
5.25225353240967 -0.447265625
5.25265884399414 -0.447265625
5.25270986557007 -0.447265625
5.25271463394165 -0.447265625
5.25275373458862 -0.447265625
5.25306415557861 -0.447265625
5.2532000541687 -0.447265625
5.25335025787354 -0.447265625
5.25356817245483 -0.447265625
5.25377416610718 -0.447265625
5.2540111541748 -0.447265625
5.25407409667969 -0.447265625
5.25407886505127 -0.447265625
5.25421667098999 -0.447265625
5.25449991226196 -0.447265625
5.25459384918213 -0.447265625
5.25459861755371 -0.447265625
5.25460386276245 -0.447265625
5.25471258163452 -0.447265625
5.2547173500061 -0.447265625
5.25488138198853 -0.447265625
5.25488615036011 -0.447265625
5.25491523742676 -0.4473876953125
5.25513029098511 -0.4473876953125
5.25537395477295 -0.4473876953125
5.25554275512695 -0.4473876953125
5.25554752349854 -0.4473876953125
5.25555229187012 -0.4473876953125
5.25586080551147 -0.4473876953125
5.25590419769287 -0.4473876953125
5.25596904754639 -0.4473876953125
5.25602960586548 -0.4473876953125
5.25603437423706 -0.4473876953125
5.25643873214722 -0.4473876953125
5.2564435005188 -0.4473876953125
5.25661897659302 -0.4473876953125
5.25706148147583 -0.447509765625
5.25737619400024 -0.447509765625
5.2574315071106 -0.447509765625
5.25749158859253 -0.447509765625
5.2576208114624 -0.447509765625
5.25770473480225 -0.447509765625
5.25793743133545 -0.447509765625
5.25803375244141 -0.447509765625
5.25805044174194 -0.447509765625
5.25805521011353 -0.447509765625
5.25838327407837 -0.447509765625
5.25844812393188 -0.447509765625
5.25845289230347 -0.447509765625
5.25846719741821 -0.447509765625
5.25875234603882 -0.447509765625
5.25876665115356 -0.447509765625
5.2588095664978 -0.447509765625
5.25881433486938 -0.447509765625
5.2596583366394 -0.44775390625
5.25978517532349 -0.44775390625
5.25985193252563 -0.44775390625
5.2600212097168 -0.44775390625
5.2601261138916 -0.44775390625
5.26013088226318 -0.44775390625
5.26013565063477 -0.44775390625
5.26027679443359 -0.44775390625
5.260329246521 -0.44775390625
5.26033401489258 -0.44775390625
5.26053190231323 -0.44775390625
5.26071500778198 -0.44775390625
5.26071977615356 -0.44775390625
5.26072454452515 -0.44775390625
5.26080560684204 -0.44775390625
5.26083898544312 -0.44775390625
5.26088190078735 -0.44775390625
5.26088666915894 -0.44775390625
5.26093196868896 -0.44775390625
5.26120090484619 -0.4478759765625
5.26138401031494 -0.4478759765625
5.26140069961548 -0.4478759765625
5.26152467727661 -0.4478759765625
5.2617244720459 -0.4478759765625
5.26172924041748 -0.4478759765625
5.26200723648071 -0.4478759765625
5.26210689544678 -0.4478759765625
5.26230144500732 -0.4478759765625
5.26230621337891 -0.4478759765625
5.2624888420105 -0.4478759765625
5.26279497146606 -0.4478759765625
5.26291131973267 -0.4478759765625
5.26291608810425 -0.4478759765625
5.26292085647583 -0.4478759765625
5.26294183731079 -0.4478759765625
5.26308441162109 -0.4478759765625
5.26316022872925 -0.4478759765625
5.26334476470947 -0.4478759765625
5.26348447799683 -0.4478759765625
5.26351070404053 -0.4478759765625
5.26351547241211 -0.4478759765625
5.26398372650146 -0.447998046875
5.26400995254517 -0.447998046875
5.2642936706543 -0.447998046875
5.26435041427612 -0.447998046875
5.26467847824097 -0.447998046875
5.26468324661255 -0.447998046875
5.26468801498413 -0.447998046875
5.26468801498413 -0.447998046875
5.26682186126709 -0.44873046875
5.26696968078613 -0.4488525390625
5.26701927185059 -0.4488525390625
5.26708936691284 -0.4488525390625
5.26716947555542 -0.4488525390625
5.26760339736938 -0.448974609375
5.26770210266113 -0.448974609375
5.26770687103271 -0.448974609375
5.26773691177368 -0.448974609375
5.26789426803589 -0.448974609375
5.26789903640747 -0.448974609375
5.26848459243774 -0.448974609375
5.26858949661255 -0.448974609375
5.26897811889648 -0.448974609375
5.26902914047241 -0.448974609375
5.26909255981445 -0.448974609375
5.26922798156738 -0.448974609375
5.26928663253784 -0.448974609375
5.26931428909302 -0.448974609375
5.26935434341431 -0.448974609375
5.26967620849609 -0.448974609375
5.26982116699219 -0.448974609375
5.27004051208496 -0.4490966796875
5.27018022537231 -0.4490966796875
5.27020359039307 -0.4490966796875
5.27047395706177 -0.4490966796875
5.2705717086792 -0.4490966796875
5.27069282531738 -0.4490966796875
5.27076244354248 -0.4490966796875
5.27081155776978 -0.4490966796875
5.27117013931274 -0.4490966796875
5.27119064331055 -0.4490966796875
5.27119541168213 -0.4490966796875
5.27120018005371 -0.4490966796875
5.2712140083313 -0.4490966796875
5.27140235900879 -0.4490966796875
5.27142333984375 -0.4490966796875
5.27142810821533 -0.4490966796875
5.27143287658691 -0.4490966796875
5.27143716812134 -0.4490966796875
5.27144193649292 -0.4490966796875
5.2714467048645 -0.4490966796875
5.27154445648193 -0.4490966796875
5.27165126800537 -0.4490966796875
5.27165555953979 -0.4490966796875
5.27166032791138 -0.4490966796875
5.27194356918335 -0.4490966796875
5.27194833755493 -0.4490966796875
5.27195310592651 -0.4490966796875
5.2719578742981 -0.4490966796875
5.27226400375366 -0.4490966796875
5.27234745025635 -0.4490966796875
};
\addplot [ultra thick, blue]
table {%
-inf 0
0 -0.0001220703125
0 -0.0001220703125
0 -0.0001220703125
0 -0.000244140625
0 -0.000244140625
0 -0.000244140625
0 -0.000244140625
0 -0.000244140625
0.477121233940125 -0.0003662109375
0.477121233940125 -0.0003662109375
0.477121233940125 -0.0003662109375
0.477121233940125 -0.0003662109375
0.477121233940125 -0.0003662109375
0.84509801864624 -0.0009765625
0.84509801864624 -0.0013427734375
1.14612805843353 -0.001708984375
1.14612805843353 -0.0025634765625
1.20412003993988 -0.0028076171875
1.23044896125793 -0.0029296875
1.34242272377014 -0.0032958984375
1.36172783374786 -0.0035400390625
1.47712123394012 -0.0040283203125
1.49136173725128 -0.0042724609375
1.51851391792297 -0.00439453125
1.72427582740784 -0.00732421875
1.89209461212158 -0.0130615234375
1.913813829422 -0.0137939453125
1.97772359848022 -0.016357421875
2.06445789337158 -0.0191650390625
2.21218752861023 -0.025390625
2.23804616928101 -0.02880859375
2.37657690048218 -0.0386962890625
2.43296933174133 -0.049072265625
2.53147888183594 -0.060791015625
2.58206343650818 -0.07177734375
2.63346838951111 -0.0848388671875
2.65127801895142 -0.091552734375
2.67669367790222 -0.0938720703125
2.70927000045776 -0.09765625
2.71933126449585 -0.099365234375
2.74585509300232 -0.101318359375
2.767897605896 -0.1038818359375
2.77451705932617 -0.1048583984375
2.79169058799744 -0.105712890625
2.8182258605957 -0.1072998046875
2.82801508903503 -0.10888671875
2.84509801864624 -0.10986328125
2.86153435707092 -0.112060546875
2.87215638160706 -0.1129150390625
2.88761734962463 -0.1143798828125
2.90633511543274 -0.117431640625
2.91222214698792 -0.1190185546875
2.94101428985596 -0.127197265625
2.95230793952942 -0.1292724609375
2.98855900764465 -0.14013671875
2.99607372283936 -0.1502685546875
3.00689363479614 -0.1539306640625
3.01703333854675 -0.1568603515625
3.03462839126587 -0.160400390625
3.04883003234863 -0.168212890625
3.05766606330872 -0.171875
3.07700443267822 -0.1768798828125
3.0852906703949 -0.179443359375
3.09621453285217 -0.18359375
3.12123155593872 -0.1851806640625
3.13640356063843 -0.1942138671875
3.14705777168274 -0.1971435546875
3.15228843688965 -0.198486328125
3.16465020179749 -0.2001953125
3.18241453170776 -0.20166015625
3.18892860412598 -0.2041015625
3.20628595352173 -0.2061767578125
3.2161660194397 -0.20849609375
3.22219610214233 -0.210693359375
3.23095965385437 -0.213623046875
3.23603320121765 -0.2152099609375
3.24254131317139 -0.216552734375
3.24551272392273 -0.2177734375
3.24821853637695 -0.2186279296875
3.25382232666016 -0.219482421875
3.27369546890259 -0.227783203125
3.27966690063477 -0.232177734375
3.28981184959412 -0.233154296875
3.2920343875885 -0.2337646484375
3.29841637611389 -0.2359619140625
3.30535125732422 -0.23779296875
3.31659936904907 -0.246337890625
3.32263278961182 -0.251708984375
3.32939791679382 -0.25341796875
3.33485579490662 -0.255859375
3.34004735946655 -0.2567138671875
3.35082936286926 -0.261474609375
3.35410833358765 -0.2625732421875
3.36304759979248 -0.26318359375
3.36604928970337 -0.26416015625
3.37419819831848 -0.2691650390625
3.37675929069519 -0.270751953125
3.3789427280426 -0.271240234375
3.38453269004822 -0.2733154296875
3.3863205909729 -0.273681640625
3.3907585144043 -0.2769775390625
3.39445161819458 -0.2777099609375
3.39654803276062 -0.2783203125
3.40397787094116 -0.2808837890625
3.40671038627625 -0.281982421875
3.41094589233398 -0.2828369140625
3.41313195228577 -0.2833251953125
3.41514039039612 -0.28369140625
3.42520809173584 -0.285888671875
3.42716145515442 -0.286376953125
3.43616271018982 -0.291015625
3.43790912628174 -0.2916259765625
3.44435715675354 -0.2960205078125
3.44638180732727 -0.296630859375
3.45499730110168 -0.3016357421875
3.45621418952942 -0.30322265625
3.4631462097168 -0.303466796875
3.46938014030457 -0.3089599609375
3.4708514213562 -0.309814453125
3.47683167457581 -0.3115234375
3.47856640815735 -0.312255859375
3.48086881637573 -0.313232421875
3.48244476318359 -0.31396484375
3.48472690582275 -0.314453125
3.48557949066162 -0.314697265625
3.49415469169617 -0.322265625
3.49554443359375 -0.32421875
3.49651455879211 -0.324462890625
3.49858617782593 -0.3250732421875
3.50133323669434 -0.326171875
3.50365447998047 -0.3267822265625
3.50542140007019 -0.3272705078125
3.50933694839478 -0.3277587890625
3.51067900657654 -0.327880859375
3.51174974441528 -0.3280029296875
3.51772356033325 -0.33251953125
3.52113819122314 -0.3333740234375
3.52750110626221 -0.3336181640625
3.5287880897522 -0.333984375
3.53019976615906 -0.3341064453125
3.53109550476074 -0.3343505859375
3.53756713867188 -0.33544921875
3.53832244873047 -0.335693359375
3.5393271446228 -0.3358154296875
3.54032945632935 -0.3359375
3.54641938209534 -0.3367919921875
3.5467894077301 -0.3367919921875
3.54826664924622 -0.3370361328125
3.5505952835083 -0.337158203125
3.55400443077087 -0.3375244140625
3.55726647377014 -0.3387451171875
3.55846858024597 -0.3389892578125
3.56371831893921 -0.3392333984375
3.56466603279114 -0.33935546875
3.56561183929443 -0.33935546875
3.56867098808289 -0.3399658203125
3.57333588600159 -0.3402099609375
3.5749568939209 -0.34033203125
3.57806587219238 -0.3408203125
3.57863926887512 -0.3409423828125
3.58160829544067 -0.3411865234375
3.58681225776672 -0.341552734375
3.58714962005615 -0.341796875
3.59061908721924 -0.34228515625
3.595055103302 -0.3424072265625
3.60249400138855 -0.3431396484375
3.60314440727234 -0.343505859375
3.60433411598206 -0.3436279296875
3.6133131980896 -0.34619140625
3.61447525024414 -0.3485107421875
3.61573958396912 -0.348876953125
3.62024021148682 -0.34912109375
3.62242126464844 -0.349365234375
3.62314581871033 -0.3494873046875
3.62572383880615 -0.350341796875
3.63225483894348 -0.3507080078125
3.63508152961731 -0.35107421875
3.63558435440063 -0.351318359375
3.63878870010376 -0.3524169921875
3.64216756820679 -0.3525390625
3.65069603919983 -0.3565673828125
3.65272974967957 -0.357177734375
3.65886950492859 -0.358154296875
3.66039109230042 -0.3583984375
3.6629467010498 -0.358642578125
3.66360664367676 -0.35888671875
3.66726613044739 -0.35986328125
3.66866540908813 -0.3602294921875
3.67191290855408 -0.3604736328125
3.67292881011963 -0.3607177734375
3.6801540851593 -0.3624267578125
3.68106031417847 -0.3629150390625
3.68439650535583 -0.36376953125
3.68868684768677 -0.3643798828125
3.6907274723053 -0.36474609375
3.69319915771484 -0.3651123046875
3.69574427604675 -0.3656005859375
3.69749093055725 -0.3660888671875
3.70087671279907 -0.3668212890625
3.70243048667908 -0.3670654296875
3.70960903167725 -0.3701171875
3.71231293678284 -0.3709716796875
3.71508359909058 -0.3714599609375
3.71700429916382 -0.3717041015625
3.71941423416138 -0.372314453125
3.72255158424377 -0.3729248046875
3.7251763343811 -0.373291015625
3.72989344596863 -0.3741455078125
3.73054003715515 -0.3746337890625
3.73623704910278 -0.3775634765625
3.73719263076782 -0.3780517578125
3.73957228660583 -0.3782958984375
3.74146676063538 -0.3790283203125
3.74523091316223 -0.37939453125
3.74616694450378 -0.3797607421875
3.74787759780884 -0.3800048828125
3.75327658653259 -0.38232421875
3.75388932228088 -0.3826904296875
3.7563316822052 -0.383056640625
3.75891184806824 -0.3836669921875
3.76004528999329 -0.384033203125
3.76290345191956 -0.3841552734375
3.76425075531006 -0.3843994140625
3.76462435722351 -0.384521484375
3.76611518859863 -0.3848876953125
3.76663589477539 -0.385009765625
3.7723217010498 -0.385986328125
3.77437090873718 -0.3863525390625
3.77582883834839 -0.3865966796875
3.77735424041748 -0.38671875
3.78383207321167 -0.389892578125
3.78433203697205 -0.39111328125
3.79126954078674 -0.3917236328125
3.79176092147827 -0.39208984375
3.79497575759888 -0.392333984375
3.79574108123779 -0.3927001953125
3.79747533798218 -0.3929443359375
3.79934048652649 -0.3931884765625
3.80147218704224 -0.3934326171875
3.80461645126343 -0.39404296875
3.80550074577332 -0.3941650390625
3.80746746063232 -0.3944091796875
3.80922293663025 -0.394775390625
3.81077003479004 -0.39501953125
3.81204390525818 -0.395263671875
3.81384778022766 -0.3955078125
3.81544494628906 -0.39599609375
3.81690382957458 -0.3963623046875
3.81815981864929 -0.396484375
3.8198070526123 -0.3968505859375
3.82131695747375 -0.397216796875
3.82393050193787 -0.3978271484375
3.82549095153809 -0.3980712890625
3.82756304740906 -0.3985595703125
3.83257269859314 -0.402099609375
3.83308339118958 -0.4027099609375
3.83378434181213 -0.40283203125
3.83569049835205 -0.4029541015625
3.83607077598572 -0.403076171875
3.8402316570282 -0.4052734375
3.84160971641541 -0.40576171875
3.84310817718506 -0.4058837890625
3.84577989578247 -0.40625
3.84646081924438 -0.406494140625
3.84751105308533 -0.40673828125
3.85168623924255 -0.4083251953125
3.85193061828613 -0.4085693359375
3.85497379302979 -0.4093017578125
3.8554584980011 -0.409423828125
3.85709118843079 -0.4095458984375
3.85781478881836 -0.40966796875
3.8584771156311 -0.4097900390625
3.86141490936279 -0.41015625
3.86195230484009 -0.4102783203125
3.86320376396179 -0.410400390625
3.86362028121948 -0.4105224609375
3.86905574798584 -0.4119873046875
3.86975955963135 -0.4122314453125
3.87005257606506 -0.412353515625
3.87046241760254 -0.4124755859375
3.87128090858459 -0.41259765625
3.87349510192871 -0.413330078125
3.87540864944458 -0.41357421875
3.87592887878418 -0.4136962890625
3.87627553939819 -0.4139404296875
3.87811946868896 -0.41455078125
3.88024187088013 -0.414794921875
3.88138461112976 -0.4151611328125
3.88326382637024 -0.41552734375
3.88564395904541 -0.416015625
3.88649082183838 -0.416259765625
3.89075613021851 -0.4197998046875
3.8918719291687 -0.42138671875
3.89470362663269 -0.4215087890625
3.89630579948425 -0.4217529296875
3.89790177345276 -0.4222412109375
3.89845085144043 -0.42236328125
3.89943742752075 -0.4224853515625
3.90227484703064 -0.423583984375
3.90260124206543 -0.423828125
3.90449905395508 -0.424072265625
3.90487766265869 -0.42431640625
3.90611934661865 -0.4244384765625
3.9084849357605 -0.42578125
3.90875291824341 -0.4259033203125
3.91073107719421 -0.4266357421875
3.91099762916565 -0.4268798828125
3.91270017623901 -0.4271240234375
3.91307163238525 -0.4273681640625
3.91354894638062 -0.427490234375
3.91376090049744 -0.427490234375
3.91397261619568 -0.4276123046875
3.91587448120117 -0.4281005859375
3.91597986221313 -0.4281005859375
3.91619062423706 -0.4281005859375
3.91624331474304 -0.42822265625
3.91640138626099 -0.42822265625
3.91640138626099 -0.42822265625
3.91692757606506 -0.4283447265625
3.91834497451782 -0.4283447265625
3.91839742660522 -0.4283447265625
3.91860699653625 -0.428466796875
3.91886878013611 -0.428466796875
3.91913032531738 -0.428466796875
3.91918277740479 -0.428466796875
3.91918277740479 -0.428466796875
3.92246603965759 -0.429443359375
3.92272543907166 -0.4295654296875
3.92334771156311 -0.4296875
3.92417597770691 -0.4298095703125
3.92443442344666 -0.4298095703125
3.92531204223633 -0.4298095703125
3.92557001113892 -0.429931640625
3.92567300796509 -0.429931640625
3.92623949050903 -0.429931640625
3.92623949050903 -0.429931640625
3.92711353302002 -0.429931640625
3.9274218082428 -0.4300537109375
3.92757558822632 -0.4300537109375
3.92870306968689 -0.43017578125
3.92880535125732 -0.43017578125
3.92998051643372 -0.4302978515625
3.93043971061707 -0.4302978515625
3.93099999427795 -0.4302978515625
3.93110179901123 -0.430419921875
3.93145775794983 -0.430419921875
3.93155956268311 -0.430419921875
3.9331328868866 -0.4306640625
3.93409419059753 -0.4306640625
3.93419528007507 -0.4306640625
3.93454885482788 -0.4306640625
3.93490219116211 -0.4306640625
3.93490219116211 -0.4306640625
3.93520498275757 -0.4306640625
3.93881988525391 -0.4320068359375
3.93916964530945 -0.4324951171875
3.93961906433105 -0.4324951171875
3.93996834754944 -0.4324951171875
3.94071555137634 -0.4326171875
3.94081521034241 -0.4327392578125
3.94161081314087 -0.4327392578125
3.9423553943634 -0.432861328125
3.942702293396 -0.432861328125
3.94290065765381 -0.432861328125
3.94384074211121 -0.4329833984375
3.94384074211121 -0.4329833984375
3.94502520561218 -0.43310546875
3.94566559791565 -0.4332275390625
3.94600987434387 -0.4332275390625
3.94679594039917 -0.433349609375
3.94684505462646 -0.433349609375
3.94855976104736 -0.4337158203125
3.94890165328979 -0.4337158203125
3.94914603233337 -0.4337158203125
3.94992637634277 -0.4339599609375
3.95041346549988 -0.43408203125
3.95080280303955 -0.43408203125
3.95133757591248 -0.43408203125
3.9516773223877 -0.4342041015625
3.95196866989136 -0.4342041015625
3.95245337486267 -0.434326171875
3.9538562297821 -0.4349365234375
3.95419430732727 -0.4351806640625
3.95467662811279 -0.4351806640625
3.95511031150818 -0.435302734375
3.95559144020081 -0.4354248046875
3.95583200454712 -0.4354248046875
3.95602416992188 -0.435546875
3.95669651031494 -0.435546875
3.95717620849609 -0.4356689453125
3.95755934715271 -0.4356689453125
3.95775079727173 -0.4356689453125
3.95894598960876 -0.4359130859375
3.95913672447205 -0.4359130859375
3.96132612228394 -0.436279296875
3.96161079406738 -0.4364013671875
3.96180057525635 -0.4365234375
3.96189546585083 -0.4365234375
3.96189546585083 -0.4365234375
3.96213245391846 -0.4365234375
3.96236944198608 -0.4365234375
3.96270084381104 -0.4366455078125
3.96392941474915 -0.436767578125
3.96402382850647 -0.436767578125
3.9642596244812 -0.4368896484375
3.9642596244812 -0.4368896484375
3.96444821357727 -0.4368896484375
3.96444821357727 -0.4368896484375
3.96444821357727 -0.4368896484375
3.96496629714966 -0.43701171875
3.96576595306396 -0.43701171875
3.96576595306396 -0.43701171875
3.9659538269043 -0.43701171875
3.96600079536438 -0.43701171875
3.96600079536438 -0.43701171875
3.96698594093323 -0.4371337890625
3.9671733379364 -0.4371337890625
3.96726703643799 -0.4371337890625
3.96736073493958 -0.4371337890625
3.96736073493958 -0.4371337890625
3.96834278106689 -0.4371337890625
3.96834278106689 -0.4371337890625
3.96969532966614 -0.4373779296875
3.96974205970764 -0.4373779296875
3.97011423110962 -0.4373779296875
3.97020745277405 -0.4375
3.97160053253174 -0.4375
3.9719250202179 -0.4375
3.97224903106689 -0.4375
3.97234177589417 -0.4376220703125
3.97275805473328 -0.4376220703125
3.97275805473328 -0.4376220703125
3.97303533554077 -0.4376220703125
3.97312784194946 -0.4376220703125
3.97312784194946 -0.4376220703125
3.97441959381104 -0.4378662109375
3.97441959381104 -0.4378662109375
3.97441959381104 -0.4378662109375
3.9752938747406 -0.4378662109375
3.97616648674011 -0.43798828125
3.97621250152588 -0.43798828125
3.97621250152588 -0.43798828125
3.97968482971191 -0.438720703125
3.97995781898499 -0.43896484375
3.98068499565125 -0.43896484375
3.98082113265991 -0.43896484375
3.98091197013855 -0.4390869140625
3.98091197013855 -0.4390869140625
3.9843921661377 -0.440185546875
3.98479723930359 -0.4404296875
3.98574066162109 -0.4404296875
3.98574066162109 -0.4404296875
3.98578572273254 -0.4404296875
3.9860098361969 -0.4405517578125
3.9860098361969 -0.4405517578125
3.98762154579163 -0.4407958984375
3.98780035972595 -0.4407958984375
3.99020552635193 -0.4410400390625
3.99029445648193 -0.4410400390625
3.9906051158905 -0.441162109375
3.99211144447327 -0.441162109375
3.99219989776611 -0.441162109375
3.99259757995605 -0.441162109375
3.99277448654175 -0.441162109375
3.99277448654175 -0.441162109375
3.99321579933167 -0.441162109375
3.9932599067688 -0.4412841796875
3.99576687812805 -0.44189453125
3.99598598480225 -0.4420166015625
3.99703669548035 -0.4420166015625
3.99721169471741 -0.4420166015625
3.99729895591736 -0.4420166015625
3.9989128112793 -0.442138671875
3.99913048744202 -0.442138671875
3.99930453300476 -0.442138671875
3.9994785785675 -0.442138671875
3.9994785785675 -0.442138671875
3.99969577789307 -0.442138671875
3.99969577789307 -0.4422607421875
3.99991321563721 -0.4422607421875
4.00212287902832 -0.44287109375
4.00220918655396 -0.4429931640625
4.00281381607056 -0.4429931640625
4.0031156539917 -0.4429931640625
4.00393438339233 -0.4429931640625
4.00410652160645 -0.4429931640625
4.0042781829834 -0.4429931640625
4.0042781829834 -0.443115234375
4.00440740585327 -0.443115234375
4.00466537475586 -0.443115234375
4.00466537475586 -0.443115234375
4.00492286682129 -0.443115234375
4.00513744354248 -0.443115234375
4.00569534301758 -0.443115234375
4.00693655014038 -0.443359375
4.00723552703857 -0.4434814453125
4.00740623474121 -0.4434814453125
4.00825929641724 -0.4434814453125
4.00825929641724 -0.4434814453125
4.00868511199951 -0.4434814453125
4.01063919067383 -0.44384765625
4.01072406768799 -0.44384765625
4.01186656951904 -0.44384765625
4.01224660873413 -0.44384765625
4.01233100891113 -0.44384765625
4.01233100891113 -0.44384765625
4.01275300979614 -0.4439697265625
4.01300573348999 -0.444091796875
4.01300573348999 -0.444091796875
4.0145206451416 -0.4442138671875
4.01477241516113 -0.4443359375
4.01548528671265 -0.4443359375
4.01565313339233 -0.4443359375
4.01577854156494 -0.4443359375
4.01607179641724 -0.4443359375
4.01628112792969 -0.4444580078125
4.01648998260498 -0.4444580078125
4.01665735244751 -0.4444580078125
4.01745080947876 -0.4444580078125
4.01749229431152 -0.4444580078125
4.01761770248413 -0.4444580078125
4.01782608032227 -0.4444580078125
4.02015399932861 -0.4447021484375
4.02019548416138 -0.4447021484375
4.02052688598633 -0.44482421875
4.02069282531738 -0.44482421875
4.02069282531738 -0.44482421875
4.02085828781128 -0.44482421875
4.02102375030518 -0.44482421875
4.0212721824646 -0.44482421875
4.02139616012573 -0.4449462890625
4.02201557159424 -0.4449462890625
4.02391052246094 -0.4451904296875
4.02403402328491 -0.4453125
4.02415704727173 -0.4453125
4.02448558807373 -0.4454345703125
4.02460861206055 -0.4454345703125
4.02460861206055 -0.4454345703125
4.02497816085815 -0.4454345703125
4.02559280395508 -0.4454345703125
4.02575635910034 -0.4454345703125
4.02575635910034 -0.4454345703125
4.02591991424561 -0.4454345703125
4.02608346939087 -0.4454345703125
4.02608346939087 -0.4454345703125
4.02624702453613 -0.4454345703125
4.02637004852295 -0.445556640625
4.02657413482666 -0.445556640625
4.02657413482666 -0.445556640625
4.02665567398071 -0.445556640625
4.02681922912598 -0.445556640625
4.02681922912598 -0.445556640625
4.02681922912598 -0.445556640625
4.02730894088745 -0.4456787109375
4.02730894088745 -0.4456787109375
4.02832698822021 -0.4456787109375
4.02832698822021 -0.4456787109375
4.02844905853271 -0.4456787109375
4.02881526947021 -0.4456787109375
4.02885580062866 -0.4456787109375
4.02897787094116 -0.4456787109375
4.02934312820435 -0.4456787109375
4.02934312820435 -0.44580078125
4.02995157241821 -0.44580078125
4.03015422821045 -0.44580078125
4.03031635284424 -0.44580078125
4.03096389770508 -0.44580078125
4.03100442886353 -0.44580078125
4.03108501434326 -0.44580078125
4.03140830993652 -0.44580078125
4.03140830993652 -0.44580078125
4.0316104888916 -0.44580078125
4.0316104888916 -0.4459228515625
4.03217554092407 -0.4459228515625
4.03306150436401 -0.4459228515625
4.03322267532349 -0.446044921875
4.03322267532349 -0.446044921875
4.03322267532349 -0.446044921875
4.03334331512451 -0.446044921875
4.03358459472656 -0.446044921875
4.03362464904785 -0.446044921875
4.03438758850098 -0.446044921875
4.03458833694458 -0.446044921875
4.03482913970947 -0.446044921875
4.03486919403076 -0.4461669921875
4.03522968292236 -0.4461669921875
4.03522968292236 -0.4461669921875
4.03526973724365 -0.4461669921875
4.03526973724365 -0.4461669921875
4.03538990020752 -0.4461669921875
4.03538990020752 -0.4461669921875
4.03618955612183 -0.4461669921875
4.03638935089111 -0.4461669921875
4.0365891456604 -0.4461669921875
4.0365891456604 -0.4461669921875
4.03738689422607 -0.4461669921875
4.03742647171021 -0.4462890625
4.03742647171021 -0.4462890625
4.03762578964233 -0.4462890625
4.03790426254272 -0.4462890625
4.03790426254272 -0.4462890625
4.03925561904907 -0.4462890625
4.0394139289856 -0.4462890625
4.0394139289856 -0.4462890625
4.03977108001709 -0.4464111328125
4.03992938995361 -0.4464111328125
4.04048347473145 -0.4464111328125
4.04056262969971 -0.4464111328125
4.04115581512451 -0.4464111328125
4.04166889190674 -0.4464111328125
4.04166889190674 -0.4464111328125
4.04269361495972 -0.446533203125
4.04269361495972 -0.446533203125
4.04277229309082 -0.446533203125
4.04292964935303 -0.446533203125
4.04292964935303 -0.446533203125
4.04316568374634 -0.446533203125
4.04316568374634 -0.446533203125
4.04391241073608 -0.446533203125
4.04410839080811 -0.4466552734375
4.04430437088013 -0.4466552734375
4.04446125030518 -0.4466552734375
4.04446125030518 -0.4466552734375
4.04461812973022 -0.4466552734375
4.04536199569702 -0.4466552734375
4.04540109634399 -0.4466552734375
4.04555749893188 -0.4466552734375
4.04559659957886 -0.44677734375
4.04583120346069 -0.44677734375
4.04590940475464 -0.44677734375
4.04676818847656 -0.44677734375
4.04692411422729 -0.44677734375
4.04692411422729 -0.44677734375
4.0478196144104 -0.4468994140625
4.04785871505737 -0.4468994140625
4.04816961288452 -0.4468994140625
4.04859733581543 -0.4468994140625
4.04871368408203 -0.4468994140625
4.04890775680542 -0.4468994140625
4.04890775680542 -0.4468994140625
4.04906272888184 -0.4468994140625
4.04914045333862 -0.4468994140625
4.04925680160522 -0.4468994140625
4.04941177368164 -0.4468994140625
4.04945087432861 -0.4468994140625
4.05041837692261 -0.447021484375
4.05049562454224 -0.447021484375
4.05065059661865 -0.447021484375
4.05099821090698 -0.4471435546875
4.05107545852661 -0.4471435546875
4.05122995376587 -0.4471435546875
4.05138397216797 -0.4471435546875
4.05142259597778 -0.4471435546875
4.05142259597778 -0.4471435546875
4.05149984359741 -0.4471435546875
4.05169248580933 -0.4471435546875
4.05242443084717 -0.4471435546875
4.05242443084717 -0.4471435546875
4.05277109146118 -0.4471435546875
4.05284786224365 -0.4471435546875
4.05284786224365 -0.4471435546875
4.05296325683594 -0.4471435546875
4.05307865142822 -0.447265625
4.05307865142822 -0.447265625
4.05327033996582 -0.447265625
4.05327033996582 -0.447265625
4.05342435836792 -0.447265625
4.05357789993286 -0.447265625
4.05357789993286 -0.447265625
4.05357789993286 -0.447265625
4.05388498306274 -0.447265625
4.05388498306274 -0.447265625
4.054114818573 -0.447265625
4.054114818573 -0.447265625
4.054114818573 -0.447265625
4.05488109588623 -0.447265625
4.05625677108765 -0.447509765625
4.05637121200562 -0.447509765625
4.05644750595093 -0.447509765625
4.05644750595093 -0.447509765625
4.05663824081421 -0.4476318359375
4.05667638778687 -0.4476318359375
4.05671453475952 -0.4476318359375
4.05686664581299 -0.4476318359375
4.05690479278564 -0.4476318359375
4.0569429397583 -0.4476318359375
4.0569429397583 -0.4476318359375
4.05705738067627 -0.4476318359375
4.05709552764893 -0.4476318359375
4.05713319778442 -0.4476318359375
4.05713319778442 -0.4476318359375
4.05713319778442 -0.4476318359375
4.05713319778442 -0.4476318359375
4.05713319778442 -0.4476318359375
4.0573616027832 -0.4476318359375
4.05751419067383 -0.4476318359375
4.05755186080933 -0.4476318359375
4.05804634094238 -0.4476318359375
4.05804634094238 -0.4476318359375
4.05804634094238 -0.4476318359375
4.05812215805054 -0.4476318359375
4.05812215805054 -0.4476318359375
4.05812215805054 -0.4476318359375
4.05812215805054 -0.4476318359375
4.058274269104 -0.4476318359375
4.0583119392395 -0.4476318359375
4.05835008621216 -0.44775390625
4.05838823318481 -0.44775390625
4.05846405029297 -0.44775390625
4.05861568450928 -0.44775390625
4.05869150161743 -0.44775390625
4.05872964859009 -0.44775390625
4.05872964859009 -0.44775390625
4.05872964859009 -0.44775390625
4.05872964859009 -0.44775390625
4.05872964859009 -0.44775390625
4.05872964859009 -0.44775390625
4.0588436126709 -0.44775390625
4.06016874313354 -0.4478759765625
4.0602445602417 -0.4478759765625
4.0602445602417 -0.4478759765625
4.0602445602417 -0.4478759765625
4.06043338775635 -0.4478759765625
4.0605092048645 -0.447998046875
4.060546875 -0.447998046875
4.060546875 -0.447998046875
4.060546875 -0.447998046875
4.060622215271 -0.447998046875
4.060622215271 -0.447998046875
4.060622215271 -0.447998046875
4.060622215271 -0.447998046875
4.06073570251465 -0.447998046875
4.06073570251465 -0.447998046875
4.06073570251465 -0.447998046875
4.06073570251465 -0.447998046875
4.0608868598938 -0.447998046875
4.0608868598938 -0.447998046875
4.0608868598938 -0.447998046875
4.0608868598938 -0.447998046875
4.0619797706604 -0.4481201171875
4.0619797706604 -0.4481201171875
4.0619797706604 -0.4481201171875
4.0619797706604 -0.4481201171875
4.0619797706604 -0.4481201171875
4.0619797706604 -0.4481201171875
4.0619797706604 -0.4481201171875
4.06209278106689 -0.4481201171875
4.06209278106689 -0.4481201171875
4.06209278106689 -0.4481201171875
4.06209278106689 -0.4481201171875
4.06209278106689 -0.4481201171875
4.06220579147339 -0.4481201171875
4.06220579147339 -0.4481201171875
4.06220579147339 -0.4481201171875
4.06220579147339 -0.4481201171875
4.06427097320557 -0.4483642578125
4.0643458366394 -0.448486328125
4.06438302993774 -0.448486328125
4.06438302993774 -0.448486328125
4.06445789337158 -0.448486328125
4.06449556350708 -0.448486328125
4.06457042694092 -0.448486328125
4.06464529037476 -0.448486328125
4.0646824836731 -0.448486328125
4.06475734710693 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06483221054077 -0.448486328125
4.06851959228516 -0.4490966796875
4.06859397888184 -0.4490966796875
4.06859397888184 -0.4490966796875
4.06859397888184 -0.4490966796875
4.06859397888184 -0.4490966796875
4.0688533782959 -0.4490966796875
4.0688533782959 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06889057159424 -0.4490966796875
4.06911277770996 -0.4490966796875
4.0691499710083 -0.4490966796875
4.07000112533569 -0.44921875
4.07081317901611 -0.44921875
4.07088708877563 -0.44921875
4.07092380523682 -0.44921875
4.07096099853516 -0.44921875
4.07096099853516 -0.44921875
4.07103490829468 -0.44921875
4.07107162475586 -0.44921875
4.07107162475586 -0.44921875
4.07110834121704 -0.44921875
4.07110834121704 -0.44921875
4.07110834121704 -0.44921875
4.07110834121704 -0.44921875
4.07114505767822 -0.44921875
4.07118225097656 -0.44921875
4.07125568389893 -0.44921875
4.07125568389893 -0.44921875
4.07125568389893 -0.44921875
4.07125568389893 -0.44921875
4.07125568389893 -0.44921875
4.07140350341797 -0.44921875
4.07155084609985 -0.44921875
4.07155084609985 -0.4493408203125
4.07155084609985 -0.4493408203125
4.07155084609985 -0.4493408203125
4.07155084609985 -0.4493408203125
4.07155084609985 -0.4493408203125
4.07210302352905 -0.4493408203125
4.07210302352905 -0.4493408203125
4.07210302352905 -0.4493408203125
4.07217645645142 -0.4493408203125
4.07217645645142 -0.4493408203125
4.0722131729126 -0.4493408203125
4.0722131729126 -0.4493408203125
4.0722131729126 -0.4493408203125
};
\end{axis}

==> Figures/n_distribution.tex <==
\begin{subfigure}[b]{0.23\textwidth}
\centering
\captionsetup{justification=raggedright,singlelinecheck=false}
\caption{}
\includegraphics[scale=.4]{Figures/png/n0_and_n1_trig.png}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\centering
\captionsetup{justification=raggedright,singlelinecheck=false}
\caption{}
\includegraphics[scale=.4]{Figures/png/n0_and_n1_softmax.png}
\end{subfigure}


\begin{subfigure}[b]{0.44\textwidth}
\centering
\captionsetup{justification=raggedright,singlelinecheck=false}
\caption{}
\includegraphics[scale=.55]{Figures/png/occ_num_hist.png}

\end{subfigure}
